T-STAR: Truthful Style Transfer using AMR Graph as Intermediate Representation

Unavailability of parallel corpora for training text style transfer (TST) models is a very challenging yet common scenario. Also, TST models implicitly need to preserve the content while transforming a source sentence into the target style. To tackle these problems, an intermediate representation is often constructed that is devoid of style while still preserving the meaning of the source sentence. In this work, we study the usefulness of Abstract Meaning Representation (AMR) graph as the intermediate style agnostic representation. We posit that semantic notations like AMR are a natural choice for an intermediate representation. Hence, we propose T-STAR: a model comprising of two components, text-to-AMR encoder and a AMR-to-text decoder. We propose several modeling improvements to enhance the style agnosticity of the generated AMR. To the best of our knowledge, T-STAR is the first work that uses AMR as an intermediate representation for TST. With thorough experimental evaluation we show T-STAR significantly outperforms state of the art techniques by achieving on an average 15.2% higher content preservation with negligible loss (3% approx.) in style accuracy. Through detailed human evaluation with 90,000 ratings, we also show that T-STAR has up to 50% lesser hallucinations compared to state of the art TST models.

==> Figures/mrpc_boxplot <==
Last login: Mon Jun 20 12:58:11 on ttys000
preksh-macbookpro:~ preksh$ wc -l ~/Downloads/st
standalone-dfigdc (1).png  stopwords.txt
standalone-dfigdc.png      sts_dataset/
preksh-macbookpro:~ preksh$ wc -l ~/Downloads/sts_dataset/
wc: /Users/preksh/Downloads/sts_dataset/: read: Is a directory
preksh-macbookpro:~ preksh$ wc -l ~/Downloads/sts_dataset/*
    7251 /Users/preksh/Downloads/sts_dataset/score.txt
    7251 /Users/preksh/Downloads/sts_dataset/sent1.txt
    7251 /Users/preksh/Downloads/sts_dataset/sent2.txt
   21753 total
preksh-macbookpro:~ preksh$ pip install sklearn 
pipDefaulting to user installation because normal site-packages is not writeable
 Collecting sklearn
  Downloading sklearn-0.0.tar.gz (1.1 kB)
insCollecting scikit-learn
  Downloading scikit_learn-1.1.1-cp38-cp38-macosx_10_13_x86_64.whl (8.5 MB)
     |████████████████████████████████| 8.5 MB 7.2 MB/s 
Requirement already satisfied: numpy>=1.17.3 in /Library/Python/3.8/site-packages (from scikit-learn->sklearn) (1.20.3)
Requirement already satisfied: joblib>=1.0.0 in /Library/Python/3.8/site-packages (from scikit-learn->sklearn) (1.0.1)
Requirement already satisfied: scipy>=1.3.2 in ./Library/Python/3.8/lib/python/site-packages (from scikit-learn->sklearn) (1.8.1)
Collecting threadpoolctl>=2.0.0
  Downloading threadpoolctl-3.1.0-py3-none-any.whl (14 kB)
Building wheels for collected packages: sklearn
  Building wheel for sklearn (setup.py) ... done
  Created wheel for sklearn: filename=sklearn-0.0-py2.py3-none-any.whl size=1315 sha256=baff32cc02cc94ffd4445c5c6cacafcfd741eb738300584fe46c25c9340fd328
  Stored in directory: /Users/preksh/Library/Caches/pip/wheels/22/0b/40/fd3f795caaa1fb4c6cb738bc1f56100be1e57da95849bfc897
Successfully built sklearn
Installing collected packages: threadpoolctl, scikit-learn, sklearn
Successfully installed scikit-learn-1.1.1 sklearn-0.0 threadpoolctl-3.1.0
WARNING: You are using pip version 21.1.1; however, version 22.1.2 is available.
You should consider upgrading via the '/Library/Developer/CommandLineTools/usr/bin/python3 -m pip install --upgrade pip' command.
preksh-macbookpro:~ preksh$ pip install seaborn 
Defaulting to user installation because normal site-packages is not writeable
Collecting seaborn
  Downloading seaborn-0.11.2-py3-none-any.whl (292 kB)
     |████████████████████████████████| 292 kB 2.8 MB/s 
Requirement already satisfied: pandas>=0.23 in /Library/Python/3.8/site-packages (from seaborn) (1.2.4)
Requirement already satisfied: scipy>=1.0 in ./Library/Python/3.8/lib/python/site-packages (from seaborn) (1.8.1)
Requirement already satisfied: numpy>=1.15 in /Library/Python/3.8/site-packages (from seaborn) (1.20.3)
Requirement already satisfied: matplotlib>=2.2 in /Library/Python/3.8/site-packages (from seaborn) (3.4.2)
Requirement already satisfied: cycler>=0.10 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (0.10.0)
Requirement already satisfied: pillow>=6.2.0 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (8.2.0)
Requirement already satisfied: kiwisolver>=1.0.1 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (1.3.1)
Requirement already satisfied: pyparsing>=2.2.1 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (2.4.7)
Requirement already satisfied: python-dateutil>=2.7 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (2.8.1)
Requirement already satisfied: six in /Library/Developer/CommandLineTools/Library/Frameworks/Python3.framework/Versions/3.8/lib/python3.8/site-packages (from cycler>=0.10->matplotlib>=2.2->seaborn) (1.15.0)
Requirement already satisfied: pytz>=2017.3 in /Library/Python/3.8/site-packages (from pandas>=0.23->seaborn) (2021.1)
Installing collected packages: seaborn
Successfully installed seaborn-0.11.2
WARNING: You are using pip version 21.1.1; however, version 22.1.2 is available.
You should consider upgrading via the '/Library/Developer/CommandLineTools/usr/bin/python3 -m pip install --upgrade pip' command.
preksh-macbookpro:~ preksh$ pip install matplotlib
Defaulting to user installation because normal site-packages is not writeable
Requirement already satisfied: matplotlib in /Library/Python/3.8/site-packages (3.4.2)
Requirement already satisfied: numpy>=1.16 in /Library/Python/3.8/site-packages (from matplotlib) (1.20.3)
Requirement already satisfied: cycler>=0.10 in /Library/Python/3.8/site-packages (from matplotlib) (0.10.0)
Requirement already satisfied: python-dateutil>=2.7 in /Library/Python/3.8/site-packages (from matplotlib) (2.8.1)
Requirement already satisfied: pillow>=6.2.0 in /Library/Python/3.8/site-packages (from matplotlib) (8.2.0)
Requirement already satisfied: pyparsing>=2.2.1 in /Library/Python/3.8/site-packages (from matplotlib) (2.4.7)
Requirement already satisfied: kiwisolver>=1.0.1 in /Library/Python/3.8/site-packages (from matplotlib) (1.3.1)
Requirement already satisfied: six in /Library/Developer/CommandLineTools/Library/Frameworks/Python3.framework/Versions/3.8/lib/python3.8/site-packages (from cycler>=0.10->matplotlib) (1.15.0)
WARNING: You are using pip version 21.1.1; however, version 22.1.2 is available.
You should consider upgrading via the '/Library/Developer/CommandLineTools/usr/bin/python3 -m pip install --upgrade pip' command.
preksh-macbookpro:~ preksh$ pip install seaborn
Defaulting to user installation because normal site-packages is not writeable
Requirement already satisfied: seaborn in ./Library/Python/3.8/lib/python/site-packages (0.11.2)
Requirement already satisfied: scipy>=1.0 in ./Library/Python/3.8/lib/python/site-packages (from seaborn) (1.8.1)
Requirement already satisfied: numpy>=1.15 in /Library/Python/3.8/site-packages (from seaborn) (1.20.3)
Requirement already satisfied: matplotlib>=2.2 in /Library/Python/3.8/site-packages (from seaborn) (3.4.2)
Requirement already satisfied: pandas>=0.23 in /Library/Python/3.8/site-packages (from seaborn) (1.2.4)
Requirement already satisfied: cycler>=0.10 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (0.10.0)
Requirement already satisfied: pyparsing>=2.2.1 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (2.4.7)
Requirement already satisfied: python-dateutil>=2.7 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (2.8.1)
Requirement already satisfied: pillow>=6.2.0 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (8.2.0)
Requirement already satisfied: kiwisolver>=1.0.1 in /Library/Python/3.8/site-packages (from matplotlib>=2.2->seaborn) (1.3.1)
Requirement already satisfied: six in /Library/Developer/CommandLineTools/Library/Frameworks/Python3.framework/Versions/3.8/lib/python3.8/site-packages (from cycler>=0.10->matplotlib>=2.2->seaborn) (1.15.0)
Requirement already satisfied: pytz>=2017.3 in /Library/Python/3.8/site-packages (from pandas>=0.23->seaborn) (2021.1)
WARNING: You are using pip version 21.1.1; however, version 22.1.2 is available.
You should consider upgrading via the '/Library/Developer/CommandLineTools/usr/bin/python3 -m pip install --upgrade pip' command.
preksh-macbookpro:~ preksh$ cd ~/Downloads/Generated\ Output
preksh-macbookpro:Generated Output preksh$ ls
final_bible_bible.tsv.tsv		final_df.tsv				final_poetry_switchboard.tsv.tsv	final_shakespeare_switchboard.tsv.tsv	final_switchboard_switchboard.tsv.tsv
final_bible_poetry.tsv.tsv		final_poetry_bible.tsv.tsv		final_shakespeare_bible.tsv.tsv		final_switchboard_bible.tsv.tsv		gcp_gist_generated
final_bible_shakespeare.tsv.tsv		final_poetry_poetry.tsv.tsv		final_shakespeare_poetry.tsv.tsv	final_switchboard_poetry.tsv.tsv	gcp_silverinvpara_generated
final_bible_switchboard.tsv.tsv		final_poetry_shakespeare.tsv.tsv	final_shakespeare_shakespeare.tsv.tsv	final_switchboard_shakespeare.tsv.tsv	strap_generated
preksh-macbookpro:Generated Output preksh$ cd ../
preksh-macbookpro:Downloads preksh$ cd ~/Downloads/Generated\ Output
Generated Output/                          Generated Output-20220620T064112Z-001.zip  Generated Output-20220622T135634Z-001.zip  
Generated Output 2/                        Generated Output-20220620T072607Z-001.zip  Generated Output-20220622T201501Z-001.zip  
preksh-macbookpro:Downloads preksh$ cd ~/Downloads/Generated\ Output\ 2/
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/
bible/       poetry/      shakespeare/ switchboard/ 
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/poetry/
dev.txt.features.nowiki    test.txt.features.nowiki   train.txt.features.nowiki  
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/shakespeare/dev.txt.features.nowiki  SilverInvPara-generated-amrs/shakespeare/dev.txt.features.nowiki 
2 files to edit
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/bible/dev.txt.features.nowiki  SilverInvPara-generated-amrs/bible/dev.txt.features.nowiki 
2 files to edit
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/bible/poetry.txt.features.nowiki  SilverInvPara-generated-amrs/poetry/dev.txt.features.nowiki 
2 files to edit
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/poetry/dev.txt.features.nowiki  SilverInvPara-generated-amrs/poetry/dev.txt.features.nowiki 
2 files to edit
preksh-macbookpro:Generated Output 2 preksh$ vimdiff GIST-generated-amrs/shakespeare/dev.txt.features.nowiki  SilverInvPara-generated-amrs/shakespeare/dev.txt.features.nowiki 
2 files to edit
preksh-macbookpro:Generated Output 2 preksh$ cd ~/sts
preksh-macbookpro:Generated Output 2 preksh$ cd ~/Downloads/sts_dataset
sts_dataset/                          sts_dataset-20220623T044229Z-001.zip
sts_dataset 2/                        
preksh-macbookpro:Generated Output 2 preksh$ cd ~/Downloads/sts_dataset\ 2/
preksh-macbookpro:sts_dataset 2 preksh$ ls
score.txt	sent1.txt	sent2.txt	sts
preksh-macbookpro:sts_dataset 2 preksh$ vimdiff sent1.txt sts/sent1.txt 
2 files to edit
preksh-macbookpro:sts_dataset 2 preksh$ vimdiff sent2.txt sts/sent2.txt 
2 files to edit
preksh-macbookpro:sts_dataset 2 preksh$ cd ~/Downloads/Generated\ Output\ 2/
preksh-macbookpro:Generated Output 2 preksh$ ls
GIST-generated-amrs			final_shakespeare_bible.tsv_round2.tsv
SilverInvPara-generated-amrs		final_shakespeare_poetry.tsv_round2.tsv
SilverInvParaRound2V2-generated-amrs	gcp_gist_generated
final_bible_poetry.tsv_round2.tsv	gcp_silverinvpara_generated
final_bible_shakespeare.tsv_round2.tsv	silverinvpara_round2_v2
final_df.tsv				silverinvpara_round2_v3
final_poetry_bible.tsv_round2.tsv	strap_generated
final_poetry_shakespeare.tsv_round2.tsv
preksh-macbookpro:Generated Output 2 preksh$ ipython 
Python 3.8.2 (default, Dec 21 2020, 15:06:04) 
Type 'copyright', 'credits' or 'license' for more information
IPython 7.23.1 -- An enhanced Interactive Python. Type '?' for help.

In [1]: import pandas as pd
de
   ...: new_df_merge2 = pd.DataFrame({})
   ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
   ...: style_specific_dfs = pd.DataFrame({})
   ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, stra
   ...: p_outputs, tstar_round_1):
   ...:     print (dire)
   ...:     if dire in same_styles:
   ...:         continue
   ...:     strap_df = get_df(strap)
   ...:     tstar2_df = get_df(tstar2)
   ...:     tstar2_df.drop([0], axis=0, inplace=True)
   ...:     tstar1_df = get_df(tstar1)
   ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
   ...:     new_df["input"] = strap_df["input"]
   ...:     new_df["tstar2_output"] = tstar2_df["output"]
   ...:     new_df["strap_output"] = strap_df["output"]
   ...:     new_df["tstar1_output"] = tstar1_df["output"]
   ...:     new_df["direction"] = [dire]*len(new_df)
   ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ig
   ...: nore_index=False)
   ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=Fa
   ...: lse)
   ...: 
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-2-2ab4c6e96068> in <module>
      9 new_df = pd.DataFrame({})
     10 new_df_merge2 = pd.DataFrame({})
---> 11 same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
     12 style_specific_dfs = pd.DataFrame({})
     13 for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):

NameError: name 'styles_i' is not defined

In [3]: def get_df(filename):
   ...:     df = open(filename).readlines()
   ...:     df = [i.split("\t") for i in df]
   ...:     new_df = pd.DataFrame({})
   ...:     new_df["input"] = [i[0] for i in df]
   ...:     new_df["output"] = [i[1] for i in df]
   ...:     return new_df
   ...: 
   ...: new_df = pd.DataFrame({})
   ...: new_df_merge2 = pd.DataFrame({})
   ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
   ...: style_specific_dfs = pd.DataFrame({})
   ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
   ...:     print (dire)
   ...:     if dire in same_styles:
   ...:         continue
   ...:     strap_df = get_df(strap)
   ...:     tstar2_df = get_df(tstar2)
   ...:     tstar2_df.drop([0], axis=0, inplace=True)
   ...:     tstar1_df = get_df(tstar1)
   ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
   ...:     new_df["input"] = strap_df["input"]
   ...:     new_df["tstar2_output"] = tstar2_df["output"]
   ...:     new_df["strap_output"] = strap_df["output"]
   ...:     new_df["tstar1_output"] = tstar1_df["output"]
   ...:     new_df["direction"] = [dire]*len(new_df)
   ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
   ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
   ...: 
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-3-2ab4c6e96068> in <module>
      9 new_df = pd.DataFrame({})
     10 new_df_merge2 = pd.DataFrame({})
---> 11 same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
     12 style_specific_dfs = pd.DataFrame({})
     13 for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):

NameError: name 'styles_i' is not defined

In [4]: directions = ["bible_bible.tsv","bible_shakespeare.tsv","poetry_poetry.tsv","shakespeare_bible.tsv","shakespeare_shakespeare.tsv","bible_poetry.tsv","poetry_bible.tsv","poetry_shakespeare.tsv", "shakespeare_poetry.tsv"]

In [5]: 

In [5]: tstar_round_1 = ["gcp_silverinvpara_generated/{}".format(i) for i in directions]

In [6]: 

In [6]: tstar_round_2 = ["silverinvpara_round2_v2/{}".format(i) for i in directions]

In [7]: 

In [7]: strap_outputs = ["strap_generated/{}".format(i) for i in directions]

In [8]: ls
GIST-generated-amrs/                     final_bible_poetry.tsv_round2.tsv        final_poetry_bible.tsv_round2.tsv        final_shakespeare_poetry.tsv_round2.tsv  silverinvpara_round2_v2/
SilverInvPara-generated-amrs/            final_bible_shakespeare.tsv_round2.tsv   final_poetry_shakespeare.tsv_round2.tsv  gcp_gist_generated/                      silverinvpara_round2_v3/
SilverInvParaRound2V2-generated-amrs/    final_df.tsv                             final_shakespeare_bible.tsv_round2.tsv   gcp_silverinvpara_generated/             strap_generated/

In [9]: def get_df(filename):
   ...:     df = open(filename).readlines()
   ...:     df = [i.split("\t") for i in df]
   ...:     new_df = pd.DataFrame({})
   ...:     new_df["input"] = [i[0] for i in df]
   ...:     new_df["output"] = [i[1] for i in df]
   ...:     return new_df
   ...: 
   ...: new_df = pd.DataFrame({})
   ...: new_df_merge2 = pd.DataFrame({})
   ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
   ...: style_specific_dfs = pd.DataFrame({})
   ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
   ...:     print (dire)
   ...:     if dire in same_styles:
   ...:         continue
   ...:     strap_df = get_df(strap)
   ...:     tstar2_df = get_df(tstar2)
   ...:     tstar2_df.drop([0], axis=0, inplace=True)
   ...:     tstar1_df = get_df(tstar1)
   ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
   ...:     new_df["input"] = strap_df["input"]
   ...:     new_df["tstar2_output"] = tstar2_df["output"]
   ...:     new_df["strap_output"] = strap_df["output"]
   ...:     new_df["tstar1_output"] = tstar1_df["output"]
   ...:     new_df["direction"] = [dire]*len(new_df)
   ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
   ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
   ...: 
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-9-2ab4c6e96068> in <module>
      9 new_df = pd.DataFrame({})
     10 new_df_merge2 = pd.DataFrame({})
---> 11 same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
     12 style_specific_dfs = pd.DataFrame({})
     13 for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):

NameError: name 'styles_i' is not defined

In [10]: styles_i = ["bible", "poetry", "shakespeare", "switchboard"]

In [11]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df.drop([0], axis=0, inplace=True)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = strap_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
poetry_poetry.tsv
shakespeare_bible.tsv
shakespeare_shakespeare.tsv
bible_poetry.tsv
poetry_bible.tsv
poetry_shakespeare.tsv
shakespeare_poetry.tsv

In [12]: style_specific_ids
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-12-b1dbe0e8d56b> in <module>
----> 1 style_specific_ids

NameError: name 'style_specific_ids' is not defined

In [13]: 

In [13]: style_specific_ids
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-13-b1dbe0e8d56b> in <module>
----> 1 style_specific_ids

NameError: name 'style_specific_ids' is not defined

In [14]: style_specific_dfs
Out[14]: 
                                                 input                                      tstar2_output                                       strap_output                                      tstar1_output               direction
0    So he arose from the earth, and sat upon the bed.                                                NaN  And the bed he fell upon, and rose up again, W...       He rose from the earth and sat on the bed.\n   bible_shakespeare.tsv
1    And the heavens shall declare his righteousnes...         He rose from the earth and sat on a bed.\n  The heavens will unfold God’s justice:        ...                             God be judge of you.\n   bible_shakespeare.tsv
2    Remember thy servants, Abraham, Isaac, and Jac...         The heavens declare That God judge thee!\n  Remember, Abraham, Isaac, and Jacob, Look not ...  Remember, sir, you were your servants— Abraham...   bible_shakespeare.tsv
3    only let us consent unto them, and they will d...  Remember Abraham, Isaac, and Jacob; For look n...  We have only agreed these words to them, And t...          Let us only consent and live with them.\n   bible_shakespeare.tsv
4    And, behold, thy cousin Elisabeth, she hath al...          Only let us consent and live with them.\n  And in her old age she had a son, And she was ...  And at thy old age thy cousin Elisabeth hath a...   bible_shakespeare.tsv
..                                                 ...                                                ...                                                ...                                                ...                     ...
495  A sick man in sadness makes his will, A word i...  Not one upon a grave, nor another on a grave o...               A sick man in sorrow makes a word,\n          And ill-worded sorrow makes a sick man,\n  shakespeare_poetry.tsv
496                                He speaks not true.  Sad sick makes willing, ill-worded urged by so...    He's not telling the truth,--nor should he be\n  He speaks not the truth, he speaks not the lie...  shakespeare_poetry.tsv
497                              And stay, good Nurse.  He speaks not of the true, he speaks not of th...               Stay, good nurse, and let me pray,\n        O stay, good Nurse, stay! I pray, I pray,\n  shakespeare_poetry.tsv
498                                Here's goodly gear!                        O stay, good Nurse, stay!\n                       Here is gear to every man!\n              Here's a' the good gear that's awa;\n  shakespeare_poetry.tsv
499                            It is not yet near day.                   Here's good gear o' the pow'r,\n                      Is not even of the day yet.\n                       It is not yet near the day\n  shakespeare_poetry.tsv

[3000 rows x 5 columns]

In [15]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = strap_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
poetry_poetry.tsv
shakespeare_bible.tsv
shakespeare_shakespeare.tsv
bible_poetry.tsv
poetry_bible.tsv
poetry_shakespeare.tsv
shakespeare_poetry.tsv

In [16]: style_specific_dfs
Out[16]: 
                                                 input                                      tstar2_output                                       strap_output                                      tstar1_output               direction
0    So he arose from the earth, and sat upon the bed.                               Generated Sentence\n  And the bed he fell upon, and rose up again, W...       He rose from the earth and sat on the bed.\n   bible_shakespeare.tsv
1    And the heavens shall declare his righteousnes...         He rose from the earth and sat on a bed.\n  The heavens will unfold God’s justice:        ...                             God be judge of you.\n   bible_shakespeare.tsv
2    Remember thy servants, Abraham, Isaac, and Jac...         The heavens declare That God judge thee!\n  Remember, Abraham, Isaac, and Jacob, Look not ...  Remember, sir, you were your servants— Abraham...   bible_shakespeare.tsv
3    only let us consent unto them, and they will d...  Remember Abraham, Isaac, and Jacob; For look n...  We have only agreed these words to them, And t...          Let us only consent and live with them.\n   bible_shakespeare.tsv
4    And, behold, thy cousin Elisabeth, she hath al...          Only let us consent and live with them.\n  And in her old age she had a son, And she was ...  And at thy old age thy cousin Elisabeth hath a...   bible_shakespeare.tsv
..                                                 ...                                                ...                                                ...                                                ...                     ...
495  A sick man in sadness makes his will, A word i...  Not one upon a grave, nor another on a grave o...               A sick man in sorrow makes a word,\n          And ill-worded sorrow makes a sick man,\n  shakespeare_poetry.tsv
496                                He speaks not true.  Sad sick makes willing, ill-worded urged by so...    He's not telling the truth,--nor should he be\n  He speaks not the truth, he speaks not the lie...  shakespeare_poetry.tsv
497                              And stay, good Nurse.  He speaks not of the true, he speaks not of th...               Stay, good nurse, and let me pray,\n        O stay, good Nurse, stay! I pray, I pray,\n  shakespeare_poetry.tsv
498                                Here's goodly gear!                        O stay, good Nurse, stay!\n                       Here is gear to every man!\n              Here's a' the good gear that's awa;\n  shakespeare_poetry.tsv
499                            It is not yet near day.                   Here's good gear o' the pow'r,\n                      Is not even of the day yet.\n                       It is not yet near the day\n  shakespeare_poetry.tsv

[3000 rows x 5 columns]

In [17]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df.drop([0], axis=0, inplace=True)
    ...:     print(tstar2_df)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = strap_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
                                                  input                                             output
1           Thus he rose from the earth and sat on bed.         He rose from the earth and sat on a bed.\n
2     And as God doth judge, heavens declare his rig...         The heavens declare That God judge thee!\n
3     Remember whom Abraham, Isaac, and Jacob serve;...  Remember Abraham, Isaac, and Jacob; For look n...
4     Only let us consent ’twixt them, And dwell wit...          Only let us consent and live with them.\n
5     And in her old age, and also in her cousin Eli...  Your cousin Elisabeth was born a son, too, at ...
...                                                 ...                                                ...
1710  And when the children came, they of Israel spa...  When in time your children shall ask their fat...
1711  And when they eat, he says, verily, he says on...  Truly, when they do eat, one of you will betra...
1712  God, great former of all things, reward the fo...  The great God that hath formed all things rewa...
1713  And so I said, my lord, you did not impute me ...  I should not impute iniquity to myself, nor re...
1714             Then, Jew, said he would kill himself?                             Did he kill himself?\n

[1714 rows x 2 columns]
poetry_poetry.tsv
shakespeare_bible.tsv
                                                  input                                             output
1         give me that mattock, and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2       One whom God hath made marrieth, O gentlewoman.  First, I say unto you, O lady, God hath made m...
3     Shall Rosaline, so dearly beloved, be forsaken...     How soon shall thy beloved Rosaline be lost?\n
4              Oh that I had a soul ill divided, O God!          I have an ill soul: the LORD is my God.\n
5                                          by what way?                                  is there a way?\n
...                                                 ...                                                ...
1289          To morrow good, come, madam; let us away.  And I said unto my cousin, Let me go away to m...
1290  Thou shalt take upon thine eye some new infect...  And he said unto him, Take some new iniquity u...
1291                               set the cock a hoop.             Woe unto you that set the cockahoop!\n
1292           from henceforward ye shall rule over me.               for thou hast ruled over me alway.\n
1293  Is there ever a book bind that containeth such...  Is the book of such matters ever so fair bound?\n

[1293 rows x 2 columns]
shakespeare_shakespeare.tsv
bible_poetry.tsv
                                                  input                                             output
1             So from the earth he rose, and sat on bed         Arose from the earth, and sat on the bed\n
2     And Heaven declare his righteousness, for 'tis...   The heavens declare that God shall judge them,\n
3     Remember Abraham, Isaac, Jacob, not these stub...  Remember Abraham, Isaac, Jacob,--look not on t...
4           Only let us consent them, and with us dwell  We only should consent them, and with them live\n
5     And Elisabeth's cousin conceived her son also ...  And old age, this sixth month, your cousin bor...
...                                                 ...                                                ...
1710  And spake to his children:--what mean these st...  "What mean these stones when thy children ask ...
1711  And while they eat, one of you verily say'd be...      One of you truly betray'd me, when they eat\n
1712  Great God who formed all things rewards the fo...  The great God who formed all things rewards th...
1713  And said, "King! not perversely didst thou do ...  Not perverse should I impute iniquity, nor rem...
1714                Then did the Jew say he'd kill him,            And will he kill him? And he is dead,\n

[1714 rows x 2 columns]
poetry_bible.tsv
                                                  input                                             output
1     A soul that may be healed, which hath ever new...  A soul that cannot be supplanted, and whose he...
2             Before he walked; and as if he were anew.        As before he walked, so is he in the way.\n
3     Through their shafts the pillars of jasper let...  And the jasper pillars, letting the light thro...
4          But a young warrior, whose step is in grace.  But there is a young warrior, whose step is of...
5              wandering about in pine gloom and cedar.  wandering about in the gloom of pine and cedar.\n
...                                                 ...                                                ...
1466  That the dead hearing may rouse themselves by ...  That the dead, being slumbing, may be roused t...
1467  Go with the family, with the canter as with a ...             Go to fame, and canter like a filly.\n
1468        The cowslips bowed with their golden drops.    And the cowslips bowed upon the golden drops.\n
1469  And all her populous streets and her temples w...  And all her populous streets and her temples a...
1470     I thought, that this might be Pope or Stephen.  And I thought, that this might be Pontius Pila...

[1470 rows x 2 columns]
poetry_shakespeare.tsv
                                                  input                                             output
1     A soul that can heal and have ever new heartache.     A soul unalterable, with ever new heartache.\n
2              Before he walks; and like himself, anew.                              As before he walks.\n
3            Plaids of jasper let through their shafts.     The jasper pillars let through their shafts.\n
4              But a young warrior that steps in grace.        But a young warrior, that steps in grace.\n
5              Wandering about in pine and cedar gloom.  I have been wandering about in the gloom of pi...
...                                                 ...                                                ...
1466             A slumbring death might rouse to hear.              A slumbing death may rouse to hear.\n
1467                Go, Fame, and canter, like a filly.                   Go, fame, canter like a filly.\n
1468            Cowslips have bow'd their golden drops.                Cowslips bowed with golden drops.\n
1469  And all her populous streets and temples Are l...  And all her populous streets and temples are l...
1470            I think this may be the pope or Steeve.   I thought thou couldst be the pope or Stewart.\n

[1470 rows x 2 columns]
shakespeare_poetry.tsv
                                                  input                                             output
1              Give me that mattock and wrenching iron;         Give me that mattock and wrenching iron,\n
2         Gentlewoman! one whom God had marr'd and made                First, Lady! God has made her wed\n
3         So soon has Rosaline forsaken, thy dear love?             How soon will thy love rosaline lose\n
4                 O God, I have a soul that ill divides                  God, I have a ill soul in mine,\n
5                             O wha's the way, the way,                  Is there a way? Is there a way?\n
...                                                 ...                                                ...
1289   Come madam, cousin, let us away; for good morrow                Good morrow, cousin, let go away;\n
1290  To take some new infection from thine eye, and...  Take some new infection, and your rank poison ...
1291                         Ye'll set you cock-a-hoop,                       Ye'll set the cock-a-hoop!\n
1292              Henceforward thou hast ever ruled me;                   For thou hast always ruled me.\n
1293  So fair is the ever-book with such vile matter...     A book containing such matter so fair never?\n

[1293 rows x 2 columns]

In [18]: style_specific_dfs
Out[18]: 
                                                 input                                      tstar2_output                                       strap_output                                      tstar1_output               direction
0    So he arose from the earth, and sat upon the bed.                                                NaN  And the bed he fell upon, and rose up again, W...       He rose from the earth and sat on the bed.\n   bible_shakespeare.tsv
1    And the heavens shall declare his righteousnes...         He rose from the earth and sat on a bed.\n  The heavens will unfold God’s justice:        ...                             God be judge of you.\n   bible_shakespeare.tsv
2    Remember thy servants, Abraham, Isaac, and Jac...         The heavens declare That God judge thee!\n  Remember, Abraham, Isaac, and Jacob, Look not ...  Remember, sir, you were your servants— Abraham...   bible_shakespeare.tsv
3    only let us consent unto them, and they will d...  Remember Abraham, Isaac, and Jacob; For look n...  We have only agreed these words to them, And t...          Let us only consent and live with them.\n   bible_shakespeare.tsv
4    And, behold, thy cousin Elisabeth, she hath al...          Only let us consent and live with them.\n  And in her old age she had a son, And she was ...  And at thy old age thy cousin Elisabeth hath a...   bible_shakespeare.tsv
..                                                 ...                                                ...                                                ...                                                ...                     ...
495  A sick man in sadness makes his will, A word i...  Not one upon a grave, nor another on a grave o...               A sick man in sorrow makes a word,\n          And ill-worded sorrow makes a sick man,\n  shakespeare_poetry.tsv
496                                He speaks not true.  Sad sick makes willing, ill-worded urged by so...    He's not telling the truth,--nor should he be\n  He speaks not the truth, he speaks not the lie...  shakespeare_poetry.tsv
497                              And stay, good Nurse.  He speaks not of the true, he speaks not of th...               Stay, good nurse, and let me pray,\n        O stay, good Nurse, stay! I pray, I pray,\n  shakespeare_poetry.tsv
498                                Here's goodly gear!                        O stay, good Nurse, stay!\n                       Here is gear to every man!\n              Here's a' the good gear that's awa;\n  shakespeare_poetry.tsv
499                            It is not yet near day.                   Here's good gear o' the pow'r,\n                      Is not even of the day yet.\n                       It is not yet near the day\n  shakespeare_poetry.tsv

[3000 rows x 5 columns]

In [19]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df.drop([0], axis=0, inplace=True)
    ...:     print(len(strap_df), len(tstar2_df))
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = strap_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
1714 1714
poetry_poetry.tsv
shakespeare_bible.tsv
1293 1293
shakespeare_shakespeare.tsv
bible_poetry.tsv
1714 1714
poetry_bible.tsv
1470 1470
poetry_shakespeare.tsv
1470 1470
shakespeare_poetry.tsv
1293 1293

In [20]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df.drop([0], axis=0, inplace=True)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df = pd.merge(strap_df, tstar2_df, on="input", how="inner")
    ...:     print("strap", len(strap_df))
    ...:     print("tstar2", len(tstar2_df))
    ...:     print (tstar2_df)
    ...:     print ("tstar1",  len(tstar1_df))
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     new_df["strap_output"] = new_df["output_x"]
    ...:     new_df["tstar2_output"] = new_df["output_y"]
    ...:     new_df_merge2 = pd.merge(new_df, tstar1_df, on="input", how="inner")
    ...:     new_df_merge2 = new_df_merge2.dropna().drop_duplicates()
    ...:     new_df_merge2 = new_df_merge2.sample(frac=1)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df_merge2.iloc[:500], ignore_index=False)
    ...:     new_df_merge2.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
strap 1714
tstar2 1714
                                                  input                                             output
1           Thus he rose from the earth and sat on bed.         He rose from the earth and sat on a bed.\n
2     And as God doth judge, heavens declare his rig...         The heavens declare That God judge thee!\n
3     Remember whom Abraham, Isaac, and Jacob serve;...  Remember Abraham, Isaac, and Jacob; For look n...
4     Only let us consent ’twixt them, And dwell wit...          Only let us consent and live with them.\n
5     And in her old age, and also in her cousin Eli...  Your cousin Elisabeth was born a son, too, at ...
...                                                 ...                                                ...
1710  And when the children came, they of Israel spa...  When in time your children shall ask their fat...
1711  And when they eat, he says, verily, he says on...  Truly, when they do eat, one of you will betra...
1712  God, great former of all things, reward the fo...  The great God that hath formed all things rewa...
1713  And so I said, my lord, you did not impute me ...  I should not impute iniquity to myself, nor re...
1714             Then, Jew, said he would kill himself?                             Did he kill himself?\n

[1714 rows x 2 columns]
tstar1 1714
poetry_poetry.tsv
shakespeare_bible.tsv
strap 1293
tstar2 1293
                                                  input                                             output
1         give me that mattock, and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2       One whom God hath made marrieth, O gentlewoman.  First, I say unto you, O lady, God hath made m...
3     Shall Rosaline, so dearly beloved, be forsaken...     How soon shall thy beloved Rosaline be lost?\n
4              Oh that I had a soul ill divided, O God!          I have an ill soul: the LORD is my God.\n
5                                          by what way?                                  is there a way?\n
...                                                 ...                                                ...
1289          To morrow good, come, madam; let us away.  And I said unto my cousin, Let me go away to m...
1290  Thou shalt take upon thine eye some new infect...  And he said unto him, Take some new iniquity u...
1291                               set the cock a hoop.             Woe unto you that set the cockahoop!\n
1292           from henceforward ye shall rule over me.               for thou hast ruled over me alway.\n
1293  Is there ever a book bind that containeth such...  Is the book of such matters ever so fair bound?\n

[1293 rows x 2 columns]
tstar1 1293
shakespeare_shakespeare.tsv
bible_poetry.tsv
strap 1714
tstar2 1714
                                                  input                                             output
1             So from the earth he rose, and sat on bed         Arose from the earth, and sat on the bed\n
2     And Heaven declare his righteousness, for 'tis...   The heavens declare that God shall judge them,\n
3     Remember Abraham, Isaac, Jacob, not these stub...  Remember Abraham, Isaac, Jacob,--look not on t...
4           Only let us consent them, and with us dwell  We only should consent them, and with them live\n
5     And Elisabeth's cousin conceived her son also ...  And old age, this sixth month, your cousin bor...
...                                                 ...                                                ...
1710  And spake to his children:--what mean these st...  "What mean these stones when thy children ask ...
1711  And while they eat, one of you verily say'd be...      One of you truly betray'd me, when they eat\n
1712  Great God who formed all things rewards the fo...  The great God who formed all things rewards th...
1713  And said, "King! not perversely didst thou do ...  Not perverse should I impute iniquity, nor rem...
1714                Then did the Jew say he'd kill him,            And will he kill him? And he is dead,\n

[1714 rows x 2 columns]
tstar1 1714
poetry_bible.tsv
strap 1470
tstar2 1470
                                                  input                                             output
1     A soul that may be healed, which hath ever new...  A soul that cannot be supplanted, and whose he...
2             Before he walked; and as if he were anew.        As before he walked, so is he in the way.\n
3     Through their shafts the pillars of jasper let...  And the jasper pillars, letting the light thro...
4          But a young warrior, whose step is in grace.  But there is a young warrior, whose step is of...
5              wandering about in pine gloom and cedar.  wandering about in the gloom of pine and cedar.\n
...                                                 ...                                                ...
1466  That the dead hearing may rouse themselves by ...  That the dead, being slumbing, may be roused t...
1467  Go with the family, with the canter as with a ...             Go to fame, and canter like a filly.\n
1468        The cowslips bowed with their golden drops.    And the cowslips bowed upon the golden drops.\n
1469  And all her populous streets and her temples w...  And all her populous streets and her temples a...
1470     I thought, that this might be Pope or Stephen.  And I thought, that this might be Pontius Pila...

[1470 rows x 2 columns]
tstar1 1470
poetry_shakespeare.tsv
strap 1470
tstar2 1470
                                                  input                                             output
1     A soul that can heal and have ever new heartache.     A soul unalterable, with ever new heartache.\n
2              Before he walks; and like himself, anew.                              As before he walks.\n
3            Plaids of jasper let through their shafts.     The jasper pillars let through their shafts.\n
4              But a young warrior that steps in grace.        But a young warrior, that steps in grace.\n
5              Wandering about in pine and cedar gloom.  I have been wandering about in the gloom of pi...
...                                                 ...                                                ...
1466             A slumbring death might rouse to hear.              A slumbing death may rouse to hear.\n
1467                Go, Fame, and canter, like a filly.                   Go, fame, canter like a filly.\n
1468            Cowslips have bow'd their golden drops.                Cowslips bowed with golden drops.\n
1469  And all her populous streets and temples Are l...  And all her populous streets and temples are l...
1470            I think this may be the pope or Steeve.   I thought thou couldst be the pope or Stewart.\n

[1470 rows x 2 columns]
tstar1 1470
shakespeare_poetry.tsv
strap 1293
tstar2 1293
                                                  input                                             output
1              Give me that mattock and wrenching iron;         Give me that mattock and wrenching iron,\n
2         Gentlewoman! one whom God had marr'd and made                First, Lady! God has made her wed\n
3         So soon has Rosaline forsaken, thy dear love?             How soon will thy love rosaline lose\n
4                 O God, I have a soul that ill divides                  God, I have a ill soul in mine,\n
5                             O wha's the way, the way,                  Is there a way? Is there a way?\n
...                                                 ...                                                ...
1289   Come madam, cousin, let us away; for good morrow                Good morrow, cousin, let go away;\n
1290  To take some new infection from thine eye, and...  Take some new infection, and your rank poison ...
1291                         Ye'll set you cock-a-hoop,                       Ye'll set the cock-a-hoop!\n
1292              Henceforward thou hast ever ruled me;                   For thou hast always ruled me.\n
1293  So fair is the ever-book with such vile matter...     A book containing such matter so fair never?\n

[1293 rows x 2 columns]
tstar1 1293

In [21]: style_specific_dfs
Out[21]: 
                                               input                                           output_x  ...                                             output                                      tstar1_output
2                Will he reserve his anger for ever?                             Will he ever go mad?\n  ...            Did he ever reserve anger at himself?\n            Did he ever reserve anger at himself?\n
0                  All that are with me salute thee.           For my part, all my honor is with you.\n  ...                         I salute thee, good sir.\n                         I salute thee, good sir.\n
4                    But we have the mind of Christ.                         But we think God’s mind.\n  ...                       But we have Christ’s mind.\n                       But we have Christ’s mind.\n
7                               And they brought it.                             They have been here.\n  ...                             And they brought it.\n                             And they brought it.\n
6                         But they held their peace.                         But silence’s now in ’t.\n  ...                             But they held peace.\n                             But they held peace.\n
5                              Bring thy son hither.                   Come, son, bring thy ladyship.\n  ...                            Bring thy son hither.\n                            Bring thy son hither.\n
3                   The churches of Asia salute you.  These are the Armenian churches that make the ...  ...                 The churches of Asia salute you.\n                 The churches of Asia salute you.\n
1                              My bowels, my bowels!                            My bowels, do bowels!\n  ...                                       My bowels!\n                                       My bowels!\n
19                                 Alas, poor Romeo!         O Romeo, I know that thou art in sorrow.\n  ...              The poor and unlucky son of Rimmon.\n              The poor and unlucky son of Rimmon.\n
1                          I will bring you thither.                and I will bring you up unto him.\n  ...                   And he said, I will bring you.\n                   And he said, I will bring you.\n
18                               Go thy ways, wench.  And he said, Go thy way: depart from me, ye sc...  ...        And he saith unto him, Witch, go thy way.\n        And he saith unto him, Witch, go thy way.\n
31                             Do as I bid thee, go.                      go forth as I command thee.\n  ...    And he said unto them, Do as I commanded you.\n    And he said unto them, Do as I commanded you.\n
39   She hath not seen the change of fourteen years.  The life of Adonijah fourteen years was not ch...  ...  She hath not seen the change of days of fourte...  She hath not seen the change of days of fourte...
17       Any man that can write may answer a letter.  That any man, whether he be a lawyer, or an of...  ...  Whosoever shall write a letter, he may answer ...  Whosoever shall write a letter, he may answer ...
40                                I will follow you.  And I will follow thee: I will do all thy work...  ...                 And he said, I will follow thee.\n                 And he said, I will follow thee.\n
41                              All this is comfort.                      All things are but comfort.\n  ...                         For all this is comfort.\n                         For all this is comfort.\n
28                                        Serve God.                  serve God: for the Lord liveth.\n  ...                       Serve God: for he is good.\n                       Serve God: for he is good.\n
35                                    I like it not.                     I cannot be merry with this.\n  ...                         And he said, I abhor it.\n                         And he said, I abhor it.\n
20                       I thought all for the best.                And I considered the best of all.\n  ...           I thought all for that which was good.\n           I thought all for that which was good.\n
0                                  What day is this?          And he said unto them, What is the day?\n  ...         And he said unto them, What day is this?\n         And he said unto them, What day is this?\n
26                          Hold thy desperate hand.  hold your desperate hand, that your soul may b...  ...    Take hold of thine hand in thy desperateness.\n    Take hold of thine hand in thy desperateness.\n
34                                  I will not fail.                             for I will not fail.\n  ...                                 I will not fail.\n                                 I will not fail.\n
30                        Therefore love moderately.  So love is made mild, that it may be sweet unt...  ...                So love is moderate unto all men.\n                So love is moderate unto all men.\n
5                          I will bring you thither.                    I will deliver thee unto him.\n  ...                   And he said, I will bring you.\n                   And he said, I will bring you.\n
22                                I will come again.                               let me come again.\n  ...                  And he said, I will come again.\n                  And he said, I will come again.\n
9                                              Anon.                    Anonymously, and anonymously,\n  ...  The children of Anon, three hundred forty and ...  The children of Anon, three hundred forty and ...
3                          I will bring you thither.                and I will bring you up unto him.\n  ...                   And he said, I will bring you.\n                   And he said, I will bring you.\n
27                              Mass, and well said.                                                I\n  ...                           Massed, and well said.\n                           Massed, and well said.\n
24         These times of woe afford no time to woo.  for in these times there is no time to rejoice...  ...  Woe is come, and woe is come, and woe is come:...  Woe is come, and woe is come, and woe is come:...
42                               Some others search.                 some are sought after of others.\n  ...          And there are some others which search.\n          And there are some others which search.\n
45                            What shall I swear by?  And the angel said unto him, What is the hope ...  ...                           What shall I swear by?\n                           What shall I swear by?\n
36                         All men call thee fickle.            And all the people called him a fool.\n  ...  All men call you fickle: for ye are a rebellio...  All men call you fickle: for ye are a rebellio...
25                          Thou knowest my lodging.   And ye know that I have dwelt at my own house.\n  ...       And he said unto them, Ye know where I am.\n       And he said unto them, Ye know where I am.\n
32                      Not life, but love in death.  Not life, but the life of the flesh; and the l...  ...  For in death there is not life; but love is in...  For in death there is not life; but love is in...
7                          I will bring you thither.                    I will deliver thee unto him.\n  ...                   And he said, I will bring you.\n                   And he said, I will bring you.\n
38                          Is thy news good or bad?                     have ye good or bad tidings?\n  ...                      Is thy tidings good or bad?\n                      Is thy tidings good or bad?\n
43                                  I will go along.                And he said, I will go with thee.\n  ...                    And he said, I will go along.\n                    And he said, I will go along.\n
23                              I drew to part them.    I have drawn them out unto their own purpose.\n  ...           And he said, I drew to part with them.\n           And he said, I drew to part with them.\n
29                             I will kiss thy lips.                And I will kiss thee on the lips.\n  ...                            I will kiss thy lips.\n                            I will kiss thy lips.\n
33                                     This is well.              And he said, Now is the time to go.\n  ...                               And he said, Amen.\n                               And he said, Amen.\n
21                         I hear some noise within.  And there was a voice, I believe, which I hear...  ...           And he said, I hear some noise within.\n           And he said, I hear some noise within.\n
44                                           I have.                                    And I did so.\n  ...                             And he said, I have.\n                             And he said, I have.\n
1                  And Abdon, and Zichri, and Hanan,               Abdon, and Zichri, and hanan'tan',\n  ...           Abdon, Zichri, and Hanan are the boys,\n           Abdon, Zichri, and Hanan are the boys,\n
0                Will he reserve his anger for ever?                Will he ever blaw an angry heart?\n  ...             And never will he reserve his anger?\n             And never will he reserve his anger?\n
2          And they brought a sword before the king.               And a sword was by the king's arm,\n  ...          The sword they brought before the king,\n          The sword they brought before the king,\n
0                When shall I know that sleep again?  When shall I know That this sleep shall yet re...  ...                When shall I know to sleep again?\n                When shall I know to sleep again?\n
1   Roll the barbarian tide, and sue to be forgiven.  Take the barbarian tide, And let it be forgone.\n  ...  O, roll the barbarous tide, and sue to be pard...  O, roll the barbarous tide, and sue to be pard...
3       Where hissing snakes run to the flood below.  Where the snakes run to Bottom, And hunt to th...  ...          The hissing snakes run below the flood.\n          The hissing snakes run below the flood.\n
2             I must be near the middle of my story.                The middle is where I should lie.\n  ...           I must be near the middle of my story.\n           I must be near the middle of my story.\n
1                            Hast thou slain Tybalt?      Have thou slain Tybalt?  didst thou dost so\n  ...              Hast thou slain a' Tybalt's rivals?\n              Hast thou slain a' Tybalt's rivals?\n
0           I'll call them back again to comfort me.    I'll call them once more, and I shall comfort\n  ...            I call them back again to comfort me.\n            I call them back again to comfort me.\n
2          Yet tell me not, for I have heard it all.     But I have heard it all, and heard it still.\n  ...         Yet tell me not, as I have heard it all.\n         Yet tell me not, as I have heard it all.\n

[52 rows x 8 columns]

In [22]: style_specific_dfs[["input", "tstar1_output", "tstar2_output"]]
Out[22]: 
                                               input                                      tstar1_output                                      tstar2_output
2                Will he reserve his anger for ever?            Did he ever reserve anger at himself?\n                  Reserved he his anger for ever?\n
0                  All that are with me salute thee.                         I salute thee, good sir.\n                         All with me salute thee.\n
4                    But we have the mind of Christ.                       But we have Christ’s mind.\n                              But we have a mind.\n
7                               And they brought it.                             And they brought it.\n                            They brought it, sir.\n
6                         But they held their peace.                             But they held peace.\n                       But they held their peace.\n
5                              Bring thy son hither.                            Bring thy son hither.\n                            Bring thy son hither.\n
3                   The churches of Asia salute you.                 The churches of Asia salute you.\n                   The Church of Asia salute you.\n
1                              My bowels, my bowels!                                       My bowels!\n                                    O, my bowels!\n
19                                 Alas, poor Romeo!              The poor and unlucky son of Rimmon.\n        And they said, Alas, Romam, thou poorest!\n
1                          I will bring you thither.                   And he said, I will bring you.\n           And he said, I will bring you thither.\n
18                               Go thy ways, wench.        And he saith unto him, Witch, go thy way.\n  Then said the LORD unto me, Witch, go thy ways.\n
31                             Do as I bid thee, go.    And he said unto them, Do as I commanded you.\n  And he said unto them, Do as I have commanded ...
39   She hath not seen the change of fourteen years.  She hath not seen the change of days of fourte...  She hath not seen the change of the fourteenth...
17       Any man that can write may answer a letter.  Whosoever shall write a letter, he may answer ...  And whosoever shall write him, he may answer t...
40                                I will follow you.                 And he said, I will follow thee.\n                  And he said, I will follow you.\n
41                              All this is comfort.                         For all this is comfort.\n                  All this comfort hath the LORD.\n
28                                        Serve God.                       Serve God: for he is good.\n                                       Serve God.\n
35                                    I like it not.                         And he said, I abhor it.\n                      And he said, I like it not.\n
20                       I thought all for the best.           I thought all for that which was good.\n                      I thought all for the best.\n
0                                  What day is this?         And he said unto them, What day is this?\n                   And he said, What day is this?\n
26                          Hold thy desperate hand.    Take hold of thine hand in thy desperateness.\n                Hold thine hand, O desperate man.\n
34                                  I will not fail.                                 I will not fail.\n                    And he said, I will not fail.\n
30                        Therefore love moderately.                So love is moderate unto all men.\n                    Therefore love ye moderately.\n
5                          I will bring you thither.                   And he said, I will bring you.\n           And he said, I will bring you thither.\n
22                                I will come again.                  And he said, I will come again.\n                  And he said, I will come again.\n
9                                              Anon.  The children of Anon, three hundred forty and ...                               And he said, Anon.\n
3                          I will bring you thither.                   And he said, I will bring you.\n        And he said, I will bring you in thither.\n
27                              Mass, and well said.                           Massed, and well said.\n  And the word of the LORD came unto me in mass,...
24         These times of woe afford no time to woo.  Woe is come, and woe is come, and woe is come:...  For these times, when there is trouble, afford...
42                               Some others search.          And there are some others which search.\n                          And some others search.\n
45                            What shall I swear by?                           What shall I swear by?\n                      What shall I swear by thee?\n
36                         All men call thee fickle.  All men call you fickle: for ye are a rebellio...                        All men call thee fickle.\n
25                          Thou knowest my lodging.       And he said unto them, Ye know where I am.\n  And he said unto them, Ye shall know where I a...
32                      Not life, but love in death.  For in death there is not life; but love is in...      For life is not of life; but love in death.\n
7                          I will bring you thither.                   And he said, I will bring you.\n        And he said, I will bring you in thither.\n
38                          Is thy news good or bad?                      Is thy tidings good or bad?\n                     Is thy tidings good, or bad?\n
43                                  I will go along.                    And he said, I will go along.\n                    And he said, I will go along.\n
23                              I drew to part them.           And he said, I drew to part with them.\n                    And I drew to part with them.\n
29                             I will kiss thy lips.                            I will kiss thy lips.\n                    I will kiss thy lips, O LORD.\n
33                                     This is well.                               And he said, Amen.\n                       And he said, This is well.\n
21                         I hear some noise within.           And he said, I hear some noise within.\n                    And I hear some noise within.\n
44                                           I have.                             And he said, I have.\n                             And he said, I have.\n
1                  And Abdon, and Zichri, and Hanan,           Abdon, Zichri, and Hanan are the boys,\n                       Adam and Zichri and Hanan,\n
0                Will he reserve his anger for ever?             And never will he reserve his anger?\n         And would he reserve his wrath for ever?\n
2          And they brought a sword before the king.          The sword they brought before the king,\n                They brought the sword with them;\n
0                When shall I know that sleep again?                When shall I know to sleep again?\n                When shall I know to sleep again?\n
1   Roll the barbarian tide, and sue to be forgiven.  O, roll the barbarous tide, and sue to be pard...  Roll the barbarous tide and sue to be forgiven.\n
3       Where hissing snakes run to the flood below.          The hissing snakes run below the flood.\n      Here hissing snakes run to the flood below.\n
2             I must be near the middle of my story.           I must be near the middle of my story.\n           I must be near the middle of my story.\n
1                            Hast thou slain Tybalt?              Hast thou slain a' Tybalt's rivals?\n              And hast thou slain Tybalt in vain?\n
0           I'll call them back again to comfort me.            I call them back again to comfort me.\n         I'll call them back again to comfort me.\n
2          Yet tell me not, for I have heard it all.         Yet tell me not, as I have heard it all.\n            Yet tell it not all to me: let it be;\n

In [23]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df = pd.merge(strap_df, tstar2_df, on="input", how="inner")
    ...:     print("strap", len(strap_df))
    ...:     print("tstar2", len(tstar2_df))
    ...:     print (tstar2_df)
    ...:     print ("tstar1",  len(tstar1_df))
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     new_df["strap_output"] = new_df["output_x"]
    ...:     new_df["tstar2_output"] = new_df["output_y"]
    ...:     new_df_merge2 = pd.merge(new_df, tstar1_df, on="input", how="inner")
    ...:     new_df_merge2 = new_df_merge2.dropna().drop_duplicates()
    ...:     new_df_merge2 = new_df_merge2.sample(frac=1)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df_merge2.iloc[:500], ignore_index=False)
    ...:     new_df_merge2.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
strap 1714
tstar2 1715
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1           Thus he rose from the earth and sat on bed.         He rose from the earth and sat on a bed.\n
2     And as God doth judge, heavens declare his rig...         The heavens declare That God judge thee!\n
3     Remember whom Abraham, Isaac, and Jacob serve;...  Remember Abraham, Isaac, and Jacob; For look n...
4     Only let us consent ’twixt them, And dwell wit...          Only let us consent and live with them.\n
...                                                 ...                                                ...
1710  And when the children came, they of Israel spa...  When in time your children shall ask their fat...
1711  And when they eat, he says, verily, he says on...  Truly, when they do eat, one of you will betra...
1712  God, great former of all things, reward the fo...  The great God that hath formed all things rewa...
1713  And so I said, my lord, you did not impute me ...  I should not impute iniquity to myself, nor re...
1714             Then, Jew, said he would kill himself?                             Did he kill himself?\n

[1715 rows x 2 columns]
tstar1 1714
poetry_poetry.tsv
shakespeare_bible.tsv
strap 1293
tstar2 1294
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1         give me that mattock, and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2       One whom God hath made marrieth, O gentlewoman.  First, I say unto you, O lady, God hath made m...
3     Shall Rosaline, so dearly beloved, be forsaken...     How soon shall thy beloved Rosaline be lost?\n
4              Oh that I had a soul ill divided, O God!          I have an ill soul: the LORD is my God.\n
...                                                 ...                                                ...
1289          To morrow good, come, madam; let us away.  And I said unto my cousin, Let me go away to m...
1290  Thou shalt take upon thine eye some new infect...  And he said unto him, Take some new iniquity u...
1291                               set the cock a hoop.             Woe unto you that set the cockahoop!\n
1292           from henceforward ye shall rule over me.               for thou hast ruled over me alway.\n
1293  Is there ever a book bind that containeth such...  Is the book of such matters ever so fair bound?\n

[1294 rows x 2 columns]
tstar1 1293
shakespeare_shakespeare.tsv
bible_poetry.tsv
strap 1714
tstar2 1715
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1             So from the earth he rose, and sat on bed         Arose from the earth, and sat on the bed\n
2     And Heaven declare his righteousness, for 'tis...   The heavens declare that God shall judge them,\n
3     Remember Abraham, Isaac, Jacob, not these stub...  Remember Abraham, Isaac, Jacob,--look not on t...
4           Only let us consent them, and with us dwell  We only should consent them, and with them live\n
...                                                 ...                                                ...
1710  And spake to his children:--what mean these st...  "What mean these stones when thy children ask ...
1711  And while they eat, one of you verily say'd be...      One of you truly betray'd me, when they eat\n
1712  Great God who formed all things rewards the fo...  The great God who formed all things rewards th...
1713  And said, "King! not perversely didst thou do ...  Not perverse should I impute iniquity, nor rem...
1714                Then did the Jew say he'd kill him,            And will he kill him? And he is dead,\n

[1715 rows x 2 columns]
tstar1 1714
poetry_bible.tsv
strap 1470
tstar2 1471
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1     A soul that may be healed, which hath ever new...  A soul that cannot be supplanted, and whose he...
2             Before he walked; and as if he were anew.        As before he walked, so is he in the way.\n
3     Through their shafts the pillars of jasper let...  And the jasper pillars, letting the light thro...
4          But a young warrior, whose step is in grace.  But there is a young warrior, whose step is of...
...                                                 ...                                                ...
1466  That the dead hearing may rouse themselves by ...  That the dead, being slumbing, may be roused t...
1467  Go with the family, with the canter as with a ...             Go to fame, and canter like a filly.\n
1468        The cowslips bowed with their golden drops.    And the cowslips bowed upon the golden drops.\n
1469  And all her populous streets and her temples w...  And all her populous streets and her temples a...
1470     I thought, that this might be Pope or Stephen.  And I thought, that this might be Pontius Pila...

[1471 rows x 2 columns]
tstar1 1470
poetry_shakespeare.tsv
strap 1470
tstar2 1471
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1     A soul that can heal and have ever new heartache.     A soul unalterable, with ever new heartache.\n
2              Before he walks; and like himself, anew.                              As before he walks.\n
3            Plaids of jasper let through their shafts.     The jasper pillars let through their shafts.\n
4              But a young warrior that steps in grace.        But a young warrior, that steps in grace.\n
...                                                 ...                                                ...
1466             A slumbring death might rouse to hear.              A slumbing death may rouse to hear.\n
1467                Go, Fame, and canter, like a filly.                   Go, fame, canter like a filly.\n
1468            Cowslips have bow'd their golden drops.                Cowslips bowed with golden drops.\n
1469  And all her populous streets and temples Are l...  And all her populous streets and temples are l...
1470            I think this may be the pope or Steeve.   I thought thou couldst be the pope or Stewart.\n

[1471 rows x 2 columns]
tstar1 1470
shakespeare_poetry.tsv
strap 1293
tstar2 1294
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1              Give me that mattock and wrenching iron;         Give me that mattock and wrenching iron,\n
2         Gentlewoman! one whom God had marr'd and made                First, Lady! God has made her wed\n
3         So soon has Rosaline forsaken, thy dear love?             How soon will thy love rosaline lose\n
4                 O God, I have a soul that ill divides                  God, I have a ill soul in mine,\n
...                                                 ...                                                ...
1289   Come madam, cousin, let us away; for good morrow                Good morrow, cousin, let go away;\n
1290  To take some new infection from thine eye, and...  Take some new infection, and your rank poison ...
1291                         Ye'll set you cock-a-hoop,                       Ye'll set the cock-a-hoop!\n
1292              Henceforward thou hast ever ruled me;                   For thou hast always ruled me.\n
1293  So fair is the ever-book with such vile matter...     A book containing such matter so fair never?\n

[1294 rows x 2 columns]
tstar1 1293

In [24]: tstar2_df = tstar2_df.iloc[1:]

In [25]: tstar2_df
Out[25]: 
                                                  input                                             output
1              Give me that mattock and wrenching iron;         Give me that mattock and wrenching iron,\n
2         Gentlewoman! one whom God had marr'd and made                First, Lady! God has made her wed\n
3         So soon has Rosaline forsaken, thy dear love?             How soon will thy love rosaline lose\n
4                 O God, I have a soul that ill divides                  God, I have a ill soul in mine,\n
5                             O wha's the way, the way,                  Is there a way? Is there a way?\n
...                                                 ...                                                ...
1289   Come madam, cousin, let us away; for good morrow                Good morrow, cousin, let go away;\n
1290  To take some new infection from thine eye, and...  Take some new infection, and your rank poison ...
1291                         Ye'll set you cock-a-hoop,                       Ye'll set the cock-a-hoop!\n
1292              Henceforward thou hast ever ruled me;                   For thou hast always ruled me.\n
1293  So fair is the ever-book with such vile matter...     A book containing such matter so fair never?\n

[1293 rows x 2 columns]

In [26]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df = tstar2_df.iloc[1:]
    ...:     print(len(strap_df), len(tstar2_df))
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = strap_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
1714 1714
poetry_poetry.tsv
shakespeare_bible.tsv
1293 1293
shakespeare_shakespeare.tsv
bible_poetry.tsv
1714 1714
poetry_bible.tsv
1470 1470
poetry_shakespeare.tsv
1470 1470
shakespeare_poetry.tsv
1293 1293

In [27]: style_specific_dfs
Out[27]: 
                                                 input                                      tstar2_output                                       strap_output                                      tstar1_output               direction
0    So he arose from the earth, and sat upon the bed.                                                NaN  And the bed he fell upon, and rose up again, W...       He rose from the earth and sat on the bed.\n   bible_shakespeare.tsv
1    And the heavens shall declare his righteousnes...         He rose from the earth and sat on a bed.\n  The heavens will unfold God’s justice:        ...                             God be judge of you.\n   bible_shakespeare.tsv
2    Remember thy servants, Abraham, Isaac, and Jac...         The heavens declare That God judge thee!\n  Remember, Abraham, Isaac, and Jacob, Look not ...  Remember, sir, you were your servants— Abraham...   bible_shakespeare.tsv
3    only let us consent unto them, and they will d...  Remember Abraham, Isaac, and Jacob; For look n...  We have only agreed these words to them, And t...          Let us only consent and live with them.\n   bible_shakespeare.tsv
4    And, behold, thy cousin Elisabeth, she hath al...          Only let us consent and live with them.\n  And in her old age she had a son, And she was ...  And at thy old age thy cousin Elisabeth hath a...   bible_shakespeare.tsv
..                                                 ...                                                ...                                                ...                                                ...                     ...
495  A sick man in sadness makes his will, A word i...  Not one upon a grave, nor another on a grave o...               A sick man in sorrow makes a word,\n          And ill-worded sorrow makes a sick man,\n  shakespeare_poetry.tsv
496                                He speaks not true.  Sad sick makes willing, ill-worded urged by so...    He's not telling the truth,--nor should he be\n  He speaks not the truth, he speaks not the lie...  shakespeare_poetry.tsv
497                              And stay, good Nurse.  He speaks not of the true, he speaks not of th...               Stay, good nurse, and let me pray,\n        O stay, good Nurse, stay! I pray, I pray,\n  shakespeare_poetry.tsv
498                                Here's goodly gear!                        O stay, good Nurse, stay!\n                       Here is gear to every man!\n              Here's a' the good gear that's awa;\n  shakespeare_poetry.tsv
499                            It is not yet near day.                   Here's good gear o' the pow'r,\n                      Is not even of the day yet.\n                       It is not yet near the day\n  shakespeare_poetry.tsv

[3000 rows x 5 columns]

In [28]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df = tstar2_df.iloc[1:]
    ...:     print(len(strap_df), len(tstar2_df))
    ...:     print(tstar2_df, strap_df)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = strap_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
1714 1714
                                                  input                                             output
1           Thus he rose from the earth and sat on bed.         He rose from the earth and sat on a bed.\n
2     And as God doth judge, heavens declare his rig...         The heavens declare That God judge thee!\n
3     Remember whom Abraham, Isaac, and Jacob serve;...  Remember Abraham, Isaac, and Jacob; For look n...
4     Only let us consent ’twixt them, And dwell wit...          Only let us consent and live with them.\n
5     And in her old age, and also in her cousin Eli...  Your cousin Elisabeth was born a son, too, at ...
...                                                 ...                                                ...
1710  And when the children came, they of Israel spa...  When in time your children shall ask their fat...
1711  And when they eat, he says, verily, he says on...  Truly, when they do eat, one of you will betra...
1712  God, great former of all things, reward the fo...  The great God that hath formed all things rewa...
1713  And so I said, my lord, you did not impute me ...  I should not impute iniquity to myself, nor re...
1714             Then, Jew, said he would kill himself?                             Did he kill himself?\n

[1714 rows x 2 columns]                                                   input                                             output
0     So he arose from the earth, and sat upon the bed.  And the bed he fell upon, and rose up again, W...
1     And the heavens shall declare his righteousnes...  The heavens will unfold God’s justice:        ...
2     Remember thy servants, Abraham, Isaac, and Jac...  Remember, Abraham, Isaac, and Jacob, Look not ...
3     only let us consent unto them, and they will d...  We have only agreed these words to them, And t...
4     And, behold, thy cousin Elisabeth, she hath al...  And in her old age she had a son, And she was ...
...                                                 ...                                                ...
1709  And he spake unto the children of Israel, sayi...  And when your children ask for something, What...
1710  And as they did eat, he said, Verily I say unt...       And said, verily, one of you’ll betray me.\n
1711  The great God that formed all things both rewa...  The great God that made all things, That rewar...
1712  And said unto the king, Let not my lord impute...  Let your Grace not impute to me, Nor let your ...
1713          Then said the Jews, Will he kill himself?  And when he was thus he answered, will he be s...

[1714 rows x 2 columns]
poetry_poetry.tsv
shakespeare_bible.tsv
1293 1293
                                                  input                                             output
1         give me that mattock, and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2       One whom God hath made marrieth, O gentlewoman.  First, I say unto you, O lady, God hath made m...
3     Shall Rosaline, so dearly beloved, be forsaken...     How soon shall thy beloved Rosaline be lost?\n
4              Oh that I had a soul ill divided, O God!          I have an ill soul: the LORD is my God.\n
5                                          by what way?                                  is there a way?\n
...                                                 ...                                                ...
1289          To morrow good, come, madam; let us away.  And I said unto my cousin, Let me go away to m...
1290  Thou shalt take upon thine eye some new infect...  And he said unto him, Take some new iniquity u...
1291                               set the cock a hoop.             Woe unto you that set the cockahoop!\n
1292           from henceforward ye shall rule over me.               for thou hast ruled over me alway.\n
1293  Is there ever a book bind that containeth such...  Is the book of such matters ever so fair bound?\n

[1293 rows x 2 columns]                                                   input                                             output
0          Give me that mattock and the wrenching iron.               give me the hammer and the mallet.\n
1     One, gentlewoman, that God hath made for himse...  Greet ye gentiles, that God hath made himself ...
2     Is Rosaline, whom thou didst love so dear, So ...  Hast thou loved so dearly, that so soon after ...
3                   O God, I have an ill-divining soul.  For God hath forgiven me my iniquity; for the ...
4                                            Which way?             And he said, Wherewithal shall I go?\n
...                                                 ...                                                ...
1288      Come, madam, let's away, Good morrow, cousin.  come, and hear me: O my dear cousin, arise, an...
1289  Take thou some new infection to thy eye, And t...  Make thee a new infirmity in thine eye; and th...
1290                          You will set cock-a-hoop!  And the children of Israel said, Thou art a co...
1291               Henceforward I am ever rul'd by you.              so will I always reign in thy name.\n
1292  Was ever book containing such vile matter So f...  Was not there a book, and such abominations, w...

[1293 rows x 2 columns]
shakespeare_shakespeare.tsv
bible_poetry.tsv
1714 1714
                                                  input                                             output
1             So from the earth he rose, and sat on bed         Arose from the earth, and sat on the bed\n
2     And Heaven declare his righteousness, for 'tis...   The heavens declare that God shall judge them,\n
3     Remember Abraham, Isaac, Jacob, not these stub...  Remember Abraham, Isaac, Jacob,--look not on t...
4           Only let us consent them, and with us dwell  We only should consent them, and with them live\n
5     And Elisabeth's cousin conceived her son also ...  And old age, this sixth month, your cousin bor...
...                                                 ...                                                ...
1710  And spake to his children:--what mean these st...  "What mean these stones when thy children ask ...
1711  And while they eat, one of you verily say'd be...      One of you truly betray'd me, when they eat\n
1712  Great God who formed all things rewards the fo...  The great God who formed all things rewards th...
1713  And said, "King! not perversely didst thou do ...  Not perverse should I impute iniquity, nor rem...
1714                Then did the Jew say he'd kill him,            And will he kill him? And he is dead,\n

[1714 rows x 2 columns]                                                   input                                             output
0     So he arose from the earth, and sat upon the bed.   And rose on the bed; his feet are up and down,\n
1     And the heavens shall declare his righteousnes...  For God's righteousness shall be revealed to t...
2     Remember thy servants, Abraham, Isaac, and Jac...  Remember, Abraham, Isaac, and Jacob, turn not ...
3     only let us consent unto them, and they will d...       We'll only agree with them, and be by them\n
4     And, behold, thy cousin Elisabeth, she hath al...           And cousin Elisabeth, for her old age,\n
...                                                 ...                                                ...
1709  And he spake unto the children of Israel, sayi...  And what is this to the stones? When your chil...
1710  And as they did eat, he said, Verily I say unt...    And said, verily, one of you would betray me,\n
1711  The great God that formed all things both rewa...  The mighty God who made all, rewards the knave...
1712  And said unto the king, Let not my lord impute...  O let not my Lord impute to me, nor do ye reme...
1713          Then said the Jews, Will he kill himself?                 And said, will he then be slain?\n

[1714 rows x 2 columns]
poetry_bible.tsv
1470 1470
                                                  input                                             output
1     A soul that may be healed, which hath ever new...  A soul that cannot be supplanted, and whose he...
2             Before he walked; and as if he were anew.        As before he walked, so is he in the way.\n
3     Through their shafts the pillars of jasper let...  And the jasper pillars, letting the light thro...
4          But a young warrior, whose step is in grace.  But there is a young warrior, whose step is of...
5              wandering about in pine gloom and cedar.  wandering about in the gloom of pine and cedar.\n
...                                                 ...                                                ...
1466  That the dead hearing may rouse themselves by ...  That the dead, being slumbing, may be roused t...
1467  Go with the family, with the canter as with a ...             Go to fame, and canter like a filly.\n
1468        The cowslips bowed with their golden drops.    And the cowslips bowed upon the golden drops.\n
1469  And all her populous streets and her temples w...  And all her populous streets and her temples a...
1470     I thought, that this might be Pope or Stephen.  And I thought, that this might be Pontius Pila...

[1470 rows x 2 columns]                                                   input                                             output
0     The immedicable soul,  with heart-aches ever new.  The soul of the eminent, the heart of a new ma...
1             Before his footsteps; as when heav'd anew  And he cried unto him, saying, As though he ha...
2       By jasper pillars, letting through their shafts  By the pillars of Jasper they let down the sha...
3          While the young warrior with a step of grace  while the young warrior walketh in the way of ...
4               Wandering about in pine and cedar gloom  And in the dark shall the pine and cedar trees...
...                                                 ...                                                ...
1465          Might rous'd the slumb'ring dead to hear;            maybe he will rouse the dead to hear;\n
1466                  Go, Fame, an' canter like a filly  Go thou, Fame, an' ride thee; for thou art as ...
1467             The cowslips bowed their golden drops,  And the cowlips bowed themselves unto the gold...
1468     And all her populous streets and temples lewd,  And the streets and the chapiters of the city ...
1469            Thought I, "Can this be Pope or Steele,  And they said unto him, Can it be the Pope or ...

[1470 rows x 2 columns]
poetry_shakespeare.tsv
1470 1470
                                                  input                                             output
1     A soul that can heal and have ever new heartache.     A soul unalterable, with ever new heartache.\n
2              Before he walks; and like himself, anew.                              As before he walks.\n
3            Plaids of jasper let through their shafts.     The jasper pillars let through their shafts.\n
4              But a young warrior that steps in grace.        But a young warrior, that steps in grace.\n
5              Wandering about in pine and cedar gloom.  I have been wandering about in the gloom of pi...
...                                                 ...                                                ...
1466             A slumbring death might rouse to hear.              A slumbing death may rouse to hear.\n
1467                Go, Fame, and canter, like a filly.                   Go, fame, canter like a filly.\n
1468            Cowslips have bow'd their golden drops.                Cowslips bowed with golden drops.\n
1469  And all her populous streets and temples Are l...  And all her populous streets and temples are l...
1470            I think this may be the pope or Steeve.   I thought thou couldst be the pope or Stewart.\n

[1470 rows x 2 columns]                                                   input                                             output
0     The immedicable soul,  with heart-aches ever new.  The soul of that immeasurable, The heart of a ...
1             Before his footsteps; as when heav'd anew                 As if he had lifted up his legs.\n
2       By jasper pillars, letting through their shafts  By the pillars of Jasper, And by the summit of...
3          While the young warrior with a step of grace  while the young warrior is a step In the right...
4               Wandering about in pine and cedar gloom                     Pine and cedar trees wander?\n
...                                                 ...                                                ...
1465          Might rous'd the slumb'ring dead to hear;  It might rouse the dead; and, in a most fearfu...
1466                  Go, Fame, an' canter like a filly                         Go, Fame, an' horse you.\n
1467             The cowslips bowed their golden drops,  The cowslips, As we did before, bow'd their he...
1468     And all her populous streets and temples lewd,  And all the streets and temples of all the cit...
1469            Thought I, "Can this be Pope or Steele,  To which I answered, “can “it be the Pope or t...

[1470 rows x 2 columns]
shakespeare_poetry.tsv
1293 1293
                                                  input                                             output
1              Give me that mattock and wrenching iron;         Give me that mattock and wrenching iron,\n
2         Gentlewoman! one whom God had marr'd and made                First, Lady! God has made her wed\n
3         So soon has Rosaline forsaken, thy dear love?             How soon will thy love rosaline lose\n
4                 O God, I have a soul that ill divides                  God, I have a ill soul in mine,\n
5                             O wha's the way, the way,                  Is there a way? Is there a way?\n
...                                                 ...                                                ...
1289   Come madam, cousin, let us away; for good morrow                Good morrow, cousin, let go away;\n
1290  To take some new infection from thine eye, and...  Take some new infection, and your rank poison ...
1291                         Ye'll set you cock-a-hoop,                       Ye'll set the cock-a-hoop!\n
1292              Henceforward thou hast ever ruled me;                   For thou hast always ruled me.\n
1293  So fair is the ever-book with such vile matter...     A book containing such matter so fair never?\n

[1293 rows x 2 columns]                                                   input                                             output
0          Give me that mattock and the wrenching iron.           And give me the hammer and the wrench,\n
1     One, gentlewoman, that God hath made for himse...          Gentle maid, that God hath made himself\n
2     Is Rosaline, whom thou didst love so dear, So ...  Hadst thou loved Rosaline so long, so forgotte...
3                   O God, I have an ill-divining soul.                   For God sake, my wretched soul\n
4                                            Which way?                 Where canst thou wish for a way?\n
...                                                 ...                                                ...
1288      Come, madam, let's away, Good morrow, cousin.                Come hither, cousin Good-morning,\n
1289  Take thou some new infection to thy eye, And t...  Make new infection to your eye,--and old poiso...
1290                          You will set cock-a-hoop!             Ye'll hae a cock-a-hoop o' the wail!\n
1291               Henceforward I am ever rul'd by you.                That I must always reign in thee,\n
1292  Was ever book containing such vile matter So f...            Was there no book of so vile a thing?\n

[1293 rows x 2 columns]

In [29]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df = tstar2_df.iloc[1:]
    ...:     print(len(strap_df), len(tstar2_df))
    ...:     print(tstar2_df, strap_df)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = tstar2_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
1714 1714
                                                  input                                             output
1           Thus he rose from the earth and sat on bed.         He rose from the earth and sat on a bed.\n
2     And as God doth judge, heavens declare his rig...         The heavens declare That God judge thee!\n
3     Remember whom Abraham, Isaac, and Jacob serve;...  Remember Abraham, Isaac, and Jacob; For look n...
4     Only let us consent ’twixt them, And dwell wit...          Only let us consent and live with them.\n
5     And in her old age, and also in her cousin Eli...  Your cousin Elisabeth was born a son, too, at ...
...                                                 ...                                                ...
1710  And when the children came, they of Israel spa...  When in time your children shall ask their fat...
1711  And when they eat, he says, verily, he says on...  Truly, when they do eat, one of you will betra...
1712  God, great former of all things, reward the fo...  The great God that hath formed all things rewa...
1713  And so I said, my lord, you did not impute me ...  I should not impute iniquity to myself, nor re...
1714             Then, Jew, said he would kill himself?                             Did he kill himself?\n

[1714 rows x 2 columns]                                                   input                                             output
0     So he arose from the earth, and sat upon the bed.  And the bed he fell upon, and rose up again, W...
1     And the heavens shall declare his righteousnes...  The heavens will unfold God’s justice:        ...
2     Remember thy servants, Abraham, Isaac, and Jac...  Remember, Abraham, Isaac, and Jacob, Look not ...
3     only let us consent unto them, and they will d...  We have only agreed these words to them, And t...
4     And, behold, thy cousin Elisabeth, she hath al...  And in her old age she had a son, And she was ...
...                                                 ...                                                ...
1709  And he spake unto the children of Israel, sayi...  And when your children ask for something, What...
1710  And as they did eat, he said, Verily I say unt...       And said, verily, one of you’ll betray me.\n
1711  The great God that formed all things both rewa...  The great God that made all things, That rewar...
1712  And said unto the king, Let not my lord impute...  Let your Grace not impute to me, Nor let your ...
1713          Then said the Jews, Will he kill himself?  And when he was thus he answered, will he be s...

[1714 rows x 2 columns]
poetry_poetry.tsv
shakespeare_bible.tsv
1293 1293
                                                  input                                             output
1         give me that mattock, and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2       One whom God hath made marrieth, O gentlewoman.  First, I say unto you, O lady, God hath made m...
3     Shall Rosaline, so dearly beloved, be forsaken...     How soon shall thy beloved Rosaline be lost?\n
4              Oh that I had a soul ill divided, O God!          I have an ill soul: the LORD is my God.\n
5                                          by what way?                                  is there a way?\n
...                                                 ...                                                ...
1289          To morrow good, come, madam; let us away.  And I said unto my cousin, Let me go away to m...
1290  Thou shalt take upon thine eye some new infect...  And he said unto him, Take some new iniquity u...
1291                               set the cock a hoop.             Woe unto you that set the cockahoop!\n
1292           from henceforward ye shall rule over me.               for thou hast ruled over me alway.\n
1293  Is there ever a book bind that containeth such...  Is the book of such matters ever so fair bound?\n

[1293 rows x 2 columns]                                                   input                                             output
0          Give me that mattock and the wrenching iron.               give me the hammer and the mallet.\n
1     One, gentlewoman, that God hath made for himse...  Greet ye gentiles, that God hath made himself ...
2     Is Rosaline, whom thou didst love so dear, So ...  Hast thou loved so dearly, that so soon after ...
3                   O God, I have an ill-divining soul.  For God hath forgiven me my iniquity; for the ...
4                                            Which way?             And he said, Wherewithal shall I go?\n
...                                                 ...                                                ...
1288      Come, madam, let's away, Good morrow, cousin.  come, and hear me: O my dear cousin, arise, an...
1289  Take thou some new infection to thy eye, And t...  Make thee a new infirmity in thine eye; and th...
1290                          You will set cock-a-hoop!  And the children of Israel said, Thou art a co...
1291               Henceforward I am ever rul'd by you.              so will I always reign in thy name.\n
1292  Was ever book containing such vile matter So f...  Was not there a book, and such abominations, w...

[1293 rows x 2 columns]
shakespeare_shakespeare.tsv
bible_poetry.tsv
1714 1714
                                                  input                                             output
1             So from the earth he rose, and sat on bed         Arose from the earth, and sat on the bed\n
2     And Heaven declare his righteousness, for 'tis...   The heavens declare that God shall judge them,\n
3     Remember Abraham, Isaac, Jacob, not these stub...  Remember Abraham, Isaac, Jacob,--look not on t...
4           Only let us consent them, and with us dwell  We only should consent them, and with them live\n
5     And Elisabeth's cousin conceived her son also ...  And old age, this sixth month, your cousin bor...
...                                                 ...                                                ...
1710  And spake to his children:--what mean these st...  "What mean these stones when thy children ask ...
1711  And while they eat, one of you verily say'd be...      One of you truly betray'd me, when they eat\n
1712  Great God who formed all things rewards the fo...  The great God who formed all things rewards th...
1713  And said, "King! not perversely didst thou do ...  Not perverse should I impute iniquity, nor rem...
1714                Then did the Jew say he'd kill him,            And will he kill him? And he is dead,\n

[1714 rows x 2 columns]                                                   input                                             output
0     So he arose from the earth, and sat upon the bed.   And rose on the bed; his feet are up and down,\n
1     And the heavens shall declare his righteousnes...  For God's righteousness shall be revealed to t...
2     Remember thy servants, Abraham, Isaac, and Jac...  Remember, Abraham, Isaac, and Jacob, turn not ...
3     only let us consent unto them, and they will d...       We'll only agree with them, and be by them\n
4     And, behold, thy cousin Elisabeth, she hath al...           And cousin Elisabeth, for her old age,\n
...                                                 ...                                                ...
1709  And he spake unto the children of Israel, sayi...  And what is this to the stones? When your chil...
1710  And as they did eat, he said, Verily I say unt...    And said, verily, one of you would betray me,\n
1711  The great God that formed all things both rewa...  The mighty God who made all, rewards the knave...
1712  And said unto the king, Let not my lord impute...  O let not my Lord impute to me, nor do ye reme...
1713          Then said the Jews, Will he kill himself?                 And said, will he then be slain?\n

[1714 rows x 2 columns]
poetry_bible.tsv
1470 1470
                                                  input                                             output
1     A soul that may be healed, which hath ever new...  A soul that cannot be supplanted, and whose he...
2             Before he walked; and as if he were anew.        As before he walked, so is he in the way.\n
3     Through their shafts the pillars of jasper let...  And the jasper pillars, letting the light thro...
4          But a young warrior, whose step is in grace.  But there is a young warrior, whose step is of...
5              wandering about in pine gloom and cedar.  wandering about in the gloom of pine and cedar.\n
...                                                 ...                                                ...
1466  That the dead hearing may rouse themselves by ...  That the dead, being slumbing, may be roused t...
1467  Go with the family, with the canter as with a ...             Go to fame, and canter like a filly.\n
1468        The cowslips bowed with their golden drops.    And the cowslips bowed upon the golden drops.\n
1469  And all her populous streets and her temples w...  And all her populous streets and her temples a...
1470     I thought, that this might be Pope or Stephen.  And I thought, that this might be Pontius Pila...

[1470 rows x 2 columns]                                                   input                                             output
0     The immedicable soul,  with heart-aches ever new.  The soul of the eminent, the heart of a new ma...
1             Before his footsteps; as when heav'd anew  And he cried unto him, saying, As though he ha...
2       By jasper pillars, letting through their shafts  By the pillars of Jasper they let down the sha...
3          While the young warrior with a step of grace  while the young warrior walketh in the way of ...
4               Wandering about in pine and cedar gloom  And in the dark shall the pine and cedar trees...
...                                                 ...                                                ...
1465          Might rous'd the slumb'ring dead to hear;            maybe he will rouse the dead to hear;\n
1466                  Go, Fame, an' canter like a filly  Go thou, Fame, an' ride thee; for thou art as ...
1467             The cowslips bowed their golden drops,  And the cowlips bowed themselves unto the gold...
1468     And all her populous streets and temples lewd,  And the streets and the chapiters of the city ...
1469            Thought I, "Can this be Pope or Steele,  And they said unto him, Can it be the Pope or ...

[1470 rows x 2 columns]
poetry_shakespeare.tsv
1470 1470
                                                  input                                             output
1     A soul that can heal and have ever new heartache.     A soul unalterable, with ever new heartache.\n
2              Before he walks; and like himself, anew.                              As before he walks.\n
3            Plaids of jasper let through their shafts.     The jasper pillars let through their shafts.\n
4              But a young warrior that steps in grace.        But a young warrior, that steps in grace.\n
5              Wandering about in pine and cedar gloom.  I have been wandering about in the gloom of pi...
...                                                 ...                                                ...
1466             A slumbring death might rouse to hear.              A slumbing death may rouse to hear.\n
1467                Go, Fame, and canter, like a filly.                   Go, fame, canter like a filly.\n
1468            Cowslips have bow'd their golden drops.                Cowslips bowed with golden drops.\n
1469  And all her populous streets and temples Are l...  And all her populous streets and temples are l...
1470            I think this may be the pope or Steeve.   I thought thou couldst be the pope or Stewart.\n

[1470 rows x 2 columns]                                                   input                                             output
0     The immedicable soul,  with heart-aches ever new.  The soul of that immeasurable, The heart of a ...
1             Before his footsteps; as when heav'd anew                 As if he had lifted up his legs.\n
2       By jasper pillars, letting through their shafts  By the pillars of Jasper, And by the summit of...
3          While the young warrior with a step of grace  while the young warrior is a step In the right...
4               Wandering about in pine and cedar gloom                     Pine and cedar trees wander?\n
...                                                 ...                                                ...
1465          Might rous'd the slumb'ring dead to hear;  It might rouse the dead; and, in a most fearfu...
1466                  Go, Fame, an' canter like a filly                         Go, Fame, an' horse you.\n
1467             The cowslips bowed their golden drops,  The cowslips, As we did before, bow'd their he...
1468     And all her populous streets and temples lewd,  And all the streets and temples of all the cit...
1469            Thought I, "Can this be Pope or Steele,  To which I answered, “can “it be the Pope or t...

[1470 rows x 2 columns]
shakespeare_poetry.tsv
1293 1293
                                                  input                                             output
1              Give me that mattock and wrenching iron;         Give me that mattock and wrenching iron,\n
2         Gentlewoman! one whom God had marr'd and made                First, Lady! God has made her wed\n
3         So soon has Rosaline forsaken, thy dear love?             How soon will thy love rosaline lose\n
4                 O God, I have a soul that ill divides                  God, I have a ill soul in mine,\n
5                             O wha's the way, the way,                  Is there a way? Is there a way?\n
...                                                 ...                                                ...
1289   Come madam, cousin, let us away; for good morrow                Good morrow, cousin, let go away;\n
1290  To take some new infection from thine eye, and...  Take some new infection, and your rank poison ...
1291                         Ye'll set you cock-a-hoop,                       Ye'll set the cock-a-hoop!\n
1292              Henceforward thou hast ever ruled me;                   For thou hast always ruled me.\n
1293  So fair is the ever-book with such vile matter...     A book containing such matter so fair never?\n

[1293 rows x 2 columns]                                                   input                                             output
0          Give me that mattock and the wrenching iron.           And give me the hammer and the wrench,\n
1     One, gentlewoman, that God hath made for himse...          Gentle maid, that God hath made himself\n
2     Is Rosaline, whom thou didst love so dear, So ...  Hadst thou loved Rosaline so long, so forgotte...
3                   O God, I have an ill-divining soul.                   For God sake, my wretched soul\n
4                                            Which way?                 Where canst thou wish for a way?\n
...                                                 ...                                                ...
1288      Come, madam, let's away, Good morrow, cousin.                Come hither, cousin Good-morning,\n
1289  Take thou some new infection to thy eye, And t...  Make new infection to your eye,--and old poiso...
1290                          You will set cock-a-hoop!             Ye'll hae a cock-a-hoop o' the wail!\n
1291               Henceforward I am ever rul'd by you.                That I must always reign in thee,\n
1292  Was ever book containing such vile matter So f...            Was there no book of so vile a thing?\n

[1293 rows x 2 columns]

In [30]: style_specific_dfs
Out[30]: 
                                                 input                                      tstar2_output                                       strap_output                                      tstar1_output               direction
1          Thus he rose from the earth and sat on bed.         He rose from the earth and sat on a bed.\n  The heavens will unfold God’s justice:        ...                             God be judge of you.\n   bible_shakespeare.tsv
2    And as God doth judge, heavens declare his rig...         The heavens declare That God judge thee!\n  Remember, Abraham, Isaac, and Jacob, Look not ...  Remember, sir, you were your servants— Abraham...   bible_shakespeare.tsv
3    Remember whom Abraham, Isaac, and Jacob serve;...  Remember Abraham, Isaac, and Jacob; For look n...  We have only agreed these words to them, And t...          Let us only consent and live with them.\n   bible_shakespeare.tsv
4    Only let us consent ’twixt them, And dwell wit...          Only let us consent and live with them.\n  And in her old age she had a son, And she was ...  And at thy old age thy cousin Elisabeth hath a...   bible_shakespeare.tsv
5    And in her old age, and also in her cousin Eli...  Your cousin Elisabeth was born a son, too, at ...  Now, when the high-prince, the high-prince, an...  Hero, on his birthday, Made dinner with his lo...   bible_shakespeare.tsv
..                                                 ...                                                ...                                                ...                                                ...                     ...
496  The sick sad man's will, ill-words urged on on...  Sad sick makes willing, ill-worded urged by so...    He's not telling the truth,--nor should he be\n  He speaks not the truth, he speaks not the lie...  shakespeare_poetry.tsv
497                  He speaks not in truth, he speaks  He speaks not of the true, he speaks not of th...               Stay, good nurse, and let me pray,\n        O stay, good Nurse, stay! I pray, I pray,\n  shakespeare_poetry.tsv
498                        And stay, good Nurse, stay!                        O stay, good Nurse, stay!\n                       Here is gear to every man!\n              Here's a' the good gear that's awa;\n  shakespeare_poetry.tsv
499                         Here's a' the goodly gear,                   Here's good gear o' the pow'r,\n                      Is not even of the day yet.\n                       It is not yet near the day\n  shakespeare_poetry.tsv
500                           The day is not yet near,                      It is not yet near the day,\n                       And here I will hide, too.\n                 Here will I hide my dear laddie,\n  shakespeare_poetry.tsv

[3000 rows x 5 columns]

In [31]: cd ../Generated\ Output\ 3
/Users/preksh/Downloads/Generated Output 3

In [32]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar2_df = tstar2_df.iloc[1:]
    ...:     print(len(strap_df), len(tstar2_df))
    ...:     print(tstar2_df, strap_df)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["input"] = tstar2_df["input"]
    ...:     new_df["tstar2_output"] = tstar2_df["output"]
    ...:     new_df["strap_output"] = strap_df["output"]
    ...:     new_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df.iloc[:500], ignore_index=False)
    ...:     new_df.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
1714 1714
                                                  input                                             output
1     So he arose from the earth, and sat upon the bed.         He rose from the earth and sat on a bed.\n
2     And the heavens shall declare his righteousnes...         The heavens declare That God judge thee!\n
3     Remember thy servants, Abraham, Isaac, and Jac...  Remember Abraham, Isaac, and Jacob; For look n...
4     only let us consent unto them, and they will d...          Only let us consent and live with them.\n
5     And, behold, thy cousin Elisabeth, she hath al...  Your cousin Elisabeth was born a son, too, at ...
...                                                 ...                                                ...
1710  And he spake unto the children of Israel, sayi...  When in time your children shall ask their fat...
1711  And as they did eat, he said, Verily I say unt...  Truly, when they do eat, one of you will betra...
1712  The great God that formed all things both rewa...  The great God that hath formed all things rewa...
1713  And said unto the king, Let not my lord impute...  I should not impute iniquity to myself, nor re...
1714          Then said the Jews, Will he kill himself?                             Did he kill himself?\n

[1714 rows x 2 columns]                                                   input                                             output
0     So he arose from the earth, and sat upon the bed.  And the bed he fell upon, and rose up again, W...
1     And the heavens shall declare his righteousnes...  The heavens will unfold God’s justice:        ...
2     Remember thy servants, Abraham, Isaac, and Jac...  Remember, Abraham, Isaac, and Jacob, Look not ...
3     only let us consent unto them, and they will d...  We have only agreed these words to them, And t...
4     And, behold, thy cousin Elisabeth, she hath al...  And in her old age she had a son, And she was ...
...                                                 ...                                                ...
1709  And he spake unto the children of Israel, sayi...  And when your children ask for something, What...
1710  And as they did eat, he said, Verily I say unt...       And said, verily, one of you’ll betray me.\n
1711  The great God that formed all things both rewa...  The great God that made all things, That rewar...
1712  And said unto the king, Let not my lord impute...  Let your Grace not impute to me, Nor let your ...
1713          Then said the Jews, Will he kill himself?  And when he was thus he answered, will he be s...

[1714 rows x 2 columns]
poetry_poetry.tsv
shakespeare_bible.tsv
1293 1293
                                                  input                                             output
1          Give me that mattock and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2     One, gentlewoman, that God hath made for himse...  First, I say unto you, O lady, God hath made m...
3     Is Rosaline, whom thou didst love so dear, So ...     How soon shall thy beloved Rosaline be lost?\n
4                   O God, I have an ill-divining soul.          I have an ill soul: the LORD is my God.\n
5                                            Which way?                                  is there a way?\n
...                                                 ...                                                ...
1289      Come, madam, let's away, Good morrow, cousin.  And I said unto my cousin, Let me go away to m...
1290  Take thou some new infection to thy eye, And t...  And he said unto him, Take some new iniquity u...
1291                          You will set cock-a-hoop!             Woe unto you that set the cockahoop!\n
1292               Henceforward I am ever rul'd by you.               for thou hast ruled over me alway.\n
1293  Was ever book containing such vile matter So f...  Is the book of such matters ever so fair bound?\n

[1293 rows x 2 columns]                                                   input                                             output
0          Give me that mattock and the wrenching iron.               give me the hammer and the mallet.\n
1     One, gentlewoman, that God hath made for himse...  Greet ye gentiles, that God hath made himself ...
2     Is Rosaline, whom thou didst love so dear, So ...  Hast thou loved so dearly, that so soon after ...
3                   O God, I have an ill-divining soul.  For God hath forgiven me my iniquity; for the ...
4                                            Which way?             And he said, Wherewithal shall I go?\n
...                                                 ...                                                ...
1288      Come, madam, let's away, Good morrow, cousin.  come, and hear me: O my dear cousin, arise, an...
1289  Take thou some new infection to thy eye, And t...  Make thee a new infirmity in thine eye; and th...
1290                          You will set cock-a-hoop!  And the children of Israel said, Thou art a co...
1291               Henceforward I am ever rul'd by you.              so will I always reign in thy name.\n
1292  Was ever book containing such vile matter So f...  Was not there a book, and such abominations, w...

[1293 rows x 2 columns]
shakespeare_shakespeare.tsv
bible_poetry.tsv
1714 1714
                                                  input                                             output
1     So he arose from the earth, and sat upon the bed.         Arose from the earth, and sat on the bed\n
2     And the heavens shall declare his righteousnes...   The heavens declare that God shall judge them,\n
3     Remember thy servants, Abraham, Isaac, and Jac...  Remember Abraham, Isaac, Jacob,--look not on t...
4     only let us consent unto them, and they will d...  We only should consent them, and with them live\n
5     And, behold, thy cousin Elisabeth, she hath al...  And old age, this sixth month, your cousin bor...
...                                                 ...                                                ...
1710  And he spake unto the children of Israel, sayi...  "What mean these stones when thy children ask ...
1711  And as they did eat, he said, Verily I say unt...      One of you truly betray'd me, when they eat\n
1712  The great God that formed all things both rewa...  The great God who formed all things rewards th...
1713  And said unto the king, Let not my lord impute...  Not perverse should I impute iniquity, nor rem...
1714          Then said the Jews, Will he kill himself?            And will he kill him? And he is dead,\n

[1714 rows x 2 columns]                                                   input                                             output
0     So he arose from the earth, and sat upon the bed.   And rose on the bed; his feet are up and down,\n
1     And the heavens shall declare his righteousnes...  For God's righteousness shall be revealed to t...
2     Remember thy servants, Abraham, Isaac, and Jac...  Remember, Abraham, Isaac, and Jacob, turn not ...
3     only let us consent unto them, and they will d...       We'll only agree with them, and be by them\n
4     And, behold, thy cousin Elisabeth, she hath al...           And cousin Elisabeth, for her old age,\n
...                                                 ...                                                ...
1709  And he spake unto the children of Israel, sayi...  And what is this to the stones? When your chil...
1710  And as they did eat, he said, Verily I say unt...    And said, verily, one of you would betray me,\n
1711  The great God that formed all things both rewa...  The mighty God who made all, rewards the knave...
1712  And said unto the king, Let not my lord impute...  O let not my Lord impute to me, nor do ye reme...
1713          Then said the Jews, Will he kill himself?                 And said, will he then be slain?\n

[1714 rows x 2 columns]
poetry_bible.tsv
1470 1470
                                                  input                                             output
1     The immedicable soul,  with heart-aches ever new.  A soul that cannot be supplanted, and whose he...
2             Before his footsteps; as when heav'd anew        As before he walked, so is he in the way.\n
3       By jasper pillars, letting through their shafts  And the jasper pillars, letting the light thro...
4          While the young warrior with a step of grace  But there is a young warrior, whose step is of...
5               Wandering about in pine and cedar gloom  wandering about in the gloom of pine and cedar.\n
...                                                 ...                                                ...
1466          Might rous'd the slumb'ring dead to hear;  That the dead, being slumbing, may be roused t...
1467                  Go, Fame, an' canter like a filly             Go to fame, and canter like a filly.\n
1468             The cowslips bowed their golden drops,    And the cowslips bowed upon the golden drops.\n
1469     And all her populous streets and temples lewd,  And all her populous streets and her temples a...
1470            Thought I, "Can this be Pope or Steele,  And I thought, that this might be Pontius Pila...

[1470 rows x 2 columns]                                                   input                                             output
0     The immedicable soul,  with heart-aches ever new.  The soul of the eminent, the heart of a new ma...
1             Before his footsteps; as when heav'd anew  And he cried unto him, saying, As though he ha...
2       By jasper pillars, letting through their shafts  By the pillars of Jasper they let down the sha...
3          While the young warrior with a step of grace  while the young warrior walketh in the way of ...
4               Wandering about in pine and cedar gloom  And in the dark shall the pine and cedar trees...
...                                                 ...                                                ...
1465          Might rous'd the slumb'ring dead to hear;            maybe he will rouse the dead to hear;\n
1466                  Go, Fame, an' canter like a filly  Go thou, Fame, an' ride thee; for thou art as ...
1467             The cowslips bowed their golden drops,  And the cowlips bowed themselves unto the gold...
1468     And all her populous streets and temples lewd,  And the streets and the chapiters of the city ...
1469            Thought I, "Can this be Pope or Steele,  And they said unto him, Can it be the Pope or ...

[1470 rows x 2 columns]
poetry_shakespeare.tsv
1470 1470
                                                  input                                             output
1     The immedicable soul,  with heart-aches ever new.     A soul unalterable, with ever new heartache.\n
2             Before his footsteps; as when heav'd anew                              As before he walks.\n
3       By jasper pillars, letting through their shafts     The jasper pillars let through their shafts.\n
4          While the young warrior with a step of grace        But a young warrior, that steps in grace.\n
5               Wandering about in pine and cedar gloom  I have been wandering about in the gloom of pi...
...                                                 ...                                                ...
1466          Might rous'd the slumb'ring dead to hear;              A slumbing death may rouse to hear.\n
1467                  Go, Fame, an' canter like a filly                   Go, fame, canter like a filly.\n
1468             The cowslips bowed their golden drops,                Cowslips bowed with golden drops.\n
1469     And all her populous streets and temples lewd,  And all her populous streets and temples are l...
1470            Thought I, "Can this be Pope or Steele,   I thought thou couldst be the pope or Stewart.\n

[1470 rows x 2 columns]                                                   input                                             output
0     The immedicable soul,  with heart-aches ever new.  The soul of that immeasurable, The heart of a ...
1             Before his footsteps; as when heav'd anew                 As if he had lifted up his legs.\n
2       By jasper pillars, letting through their shafts  By the pillars of Jasper, And by the summit of...
3          While the young warrior with a step of grace  while the young warrior is a step In the right...
4               Wandering about in pine and cedar gloom                     Pine and cedar trees wander?\n
...                                                 ...                                                ...
1465          Might rous'd the slumb'ring dead to hear;  It might rouse the dead; and, in a most fearfu...
1466                  Go, Fame, an' canter like a filly                         Go, Fame, an' horse you.\n
1467             The cowslips bowed their golden drops,  The cowslips, As we did before, bow'd their he...
1468     And all her populous streets and temples lewd,  And all the streets and temples of all the cit...
1469            Thought I, "Can this be Pope or Steele,  To which I answered, “can “it be the Pope or t...

[1470 rows x 2 columns]
shakespeare_poetry.tsv
1293 1293
                                                  input                                             output
1          Give me that mattock and the wrenching iron.         Give me that mattock and wrenching iron,\n
2     One, gentlewoman, that God hath made for himse...                First, Lady! God has made her wed\n
3     Is Rosaline, whom thou didst love so dear, So ...             How soon will thy love rosaline lose\n
4                   O God, I have an ill-divining soul.                  God, I have a ill soul in mine,\n
5                                            Which way?                  Is there a way? Is there a way?\n
...                                                 ...                                                ...
1289      Come, madam, let's away, Good morrow, cousin.                Good morrow, cousin, let go away;\n
1290  Take thou some new infection to thy eye, And t...  Take some new infection, and your rank poison ...
1291                          You will set cock-a-hoop!                       Ye'll set the cock-a-hoop!\n
1292               Henceforward I am ever rul'd by you.                   For thou hast always ruled me.\n
1293  Was ever book containing such vile matter So f...     A book containing such matter so fair never?\n

[1293 rows x 2 columns]                                                   input                                             output
0          Give me that mattock and the wrenching iron.           And give me the hammer and the wrench,\n
1     One, gentlewoman, that God hath made for himse...          Gentle maid, that God hath made himself\n
2     Is Rosaline, whom thou didst love so dear, So ...  Hadst thou loved Rosaline so long, so forgotte...
3                   O God, I have an ill-divining soul.                   For God sake, my wretched soul\n
4                                            Which way?                 Where canst thou wish for a way?\n
...                                                 ...                                                ...
1288      Come, madam, let's away, Good morrow, cousin.                Come hither, cousin Good-morning,\n
1289  Take thou some new infection to thy eye, And t...  Make new infection to your eye,--and old poiso...
1290                          You will set cock-a-hoop!             Ye'll hae a cock-a-hoop o' the wail!\n
1291               Henceforward I am ever rul'd by you.                That I must always reign in thee,\n
1292  Was ever book containing such vile matter So f...            Was there no book of so vile a thing?\n

[1293 rows x 2 columns]

In [33]: style_specific_dfs
Out[33]: 
                                                 input                                      tstar2_output                                       strap_output                                      tstar1_output               direction
1    So he arose from the earth, and sat upon the bed.         He rose from the earth and sat on a bed.\n  The heavens will unfold God’s justice:        ...                             God be judge of you.\n   bible_shakespeare.tsv
2    And the heavens shall declare his righteousnes...         The heavens declare That God judge thee!\n  Remember, Abraham, Isaac, and Jacob, Look not ...  Remember, sir, you were your servants— Abraham...   bible_shakespeare.tsv
3    Remember thy servants, Abraham, Isaac, and Jac...  Remember Abraham, Isaac, and Jacob; For look n...  We have only agreed these words to them, And t...          Let us only consent and live with them.\n   bible_shakespeare.tsv
4    only let us consent unto them, and they will d...          Only let us consent and live with them.\n  And in her old age she had a son, And she was ...  And at thy old age thy cousin Elisabeth hath a...   bible_shakespeare.tsv
5    And, behold, thy cousin Elisabeth, she hath al...  Your cousin Elisabeth was born a son, too, at ...  Now, when the high-prince, the high-prince, an...  Hero, on his birthday, Made dinner with his lo...   bible_shakespeare.tsv
..                                                 ...                                                ...                                                ...                                                ...                     ...
496  A sick man in sadness makes his will, A word i...  Sad sick makes willing, ill-worded urged by so...    He's not telling the truth,--nor should he be\n  He speaks not the truth, he speaks not the lie...  shakespeare_poetry.tsv
497                                He speaks not true.  He speaks not of the true, he speaks not of th...               Stay, good nurse, and let me pray,\n        O stay, good Nurse, stay! I pray, I pray,\n  shakespeare_poetry.tsv
498                              And stay, good Nurse.                        O stay, good Nurse, stay!\n                       Here is gear to every man!\n              Here's a' the good gear that's awa;\n  shakespeare_poetry.tsv
499                                Here's goodly gear!                   Here's good gear o' the pow'r,\n                      Is not even of the day yet.\n                       It is not yet near the day\n  shakespeare_poetry.tsv
500                            It is not yet near day.                      It is not yet near the day,\n                       And here I will hide, too.\n                 Here will I hide my dear laddie,\n  shakespeare_poetry.tsv

[3000 rows x 5 columns]

In [34]: def get_df(filename):
    ...:     df = open(filename).readlines()
    ...:     df = [i.split("\t") for i in df]
    ...:     new_df = pd.DataFrame({})
    ...:     new_df["input"] = [i[0] for i in df]
    ...:     new_df["output"] = [i[1] for i in df]
    ...:     return new_df
    ...: 
    ...: new_df = pd.DataFrame({})
    ...: new_df_merge2 = pd.DataFrame({})
    ...: same_styles = ["{}_{}.tsv".format(i,i) for i in styles_i]
    ...: style_specific_dfs = pd.DataFrame({})
    ...: for (dire, tstar2, strap, tstar1) in zip(directions, tstar_round_2, strap_outputs, tstar_round_1):
    ...:     print (dire)
    ...:     if dire in same_styles:
    ...:         continue
    ...:     strap_df = get_df(strap)
    ...:     tstar2_df = get_df(tstar2)
    ...:     tstar1_df = get_df(tstar1)
    ...:     tstar1_df["tstar1_output"] = tstar1_df["output"]
    ...:     new_df = pd.merge(strap_df, tstar2_df, on="input", how="inner")
    ...:     print("strap", len(strap_df))
    ...:     print("tstar2", len(tstar2_df))
    ...:     print (tstar2_df)
    ...:     print ("tstar1",  len(tstar1_df))
    ...:     new_df["direction"] = [dire]*len(new_df)
    ...:     new_df["strap_output"] = new_df["output_x"]
    ...:     new_df["tstar2_output"] = new_df["output_y"]
    ...:     new_df_merge2 = pd.merge(new_df, tstar1_df, on="input", how="inner")
    ...:     new_df_merge2 = new_df_merge2.dropna().drop_duplicates()
    ...:     new_df_merge2 = new_df_merge2.sample(frac=1)
    ...:     style_specific_dfs = style_specific_dfs.append(new_df_merge2.iloc[:500], ignore_index=False)
    ...:     new_df_merge2.to_csv("final_{}_round2.tsv".format(dire), sep="\t", index=False)
    ...: 
bible_bible.tsv
bible_shakespeare.tsv
strap 1714
tstar2 1715
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1     So he arose from the earth, and sat upon the bed.         He rose from the earth and sat on a bed.\n
2     And the heavens shall declare his righteousnes...         The heavens declare That God judge thee!\n
3     Remember thy servants, Abraham, Isaac, and Jac...  Remember Abraham, Isaac, and Jacob; For look n...
4     only let us consent unto them, and they will d...          Only let us consent and live with them.\n
...                                                 ...                                                ...
1710  And he spake unto the children of Israel, sayi...  When in time your children shall ask their fat...
1711  And as they did eat, he said, Verily I say unt...  Truly, when they do eat, one of you will betra...
1712  The great God that formed all things both rewa...  The great God that hath formed all things rewa...
1713  And said unto the king, Let not my lord impute...  I should not impute iniquity to myself, nor re...
1714          Then said the Jews, Will he kill himself?                             Did he kill himself?\n

[1715 rows x 2 columns]
tstar1 1714
poetry_poetry.tsv
shakespeare_bible.tsv
strap 1293
tstar2 1294
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1          Give me that mattock and the wrenching iron.    Give me that mattock, and the wrenching iron.\n
2     One, gentlewoman, that God hath made for himse...  First, I say unto you, O lady, God hath made m...
3     Is Rosaline, whom thou didst love so dear, So ...     How soon shall thy beloved Rosaline be lost?\n
4                   O God, I have an ill-divining soul.          I have an ill soul: the LORD is my God.\n
...                                                 ...                                                ...
1289      Come, madam, let's away, Good morrow, cousin.  And I said unto my cousin, Let me go away to m...
1290  Take thou some new infection to thy eye, And t...  And he said unto him, Take some new iniquity u...
1291                          You will set cock-a-hoop!             Woe unto you that set the cockahoop!\n
1292               Henceforward I am ever rul'd by you.               for thou hast ruled over me alway.\n
1293  Was ever book containing such vile matter So f...  Is the book of such matters ever so fair bound?\n

[1294 rows x 2 columns]
tstar1 1293
shakespeare_shakespeare.tsv
bible_poetry.tsv
strap 1714
tstar2 1715
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1     So he arose from the earth, and sat upon the bed.         Arose from the earth, and sat on the bed\n
2     And the heavens shall declare his righteousnes...   The heavens declare that God shall judge them,\n
3     Remember thy servants, Abraham, Isaac, and Jac...  Remember Abraham, Isaac, Jacob,--look not on t...
4     only let us consent unto them, and they will d...  We only should consent them, and with them live\n
...                                                 ...                                                ...
1710  And he spake unto the children of Israel, sayi...  "What mean these stones when thy children ask ...
1711  And as they did eat, he said, Verily I say unt...      One of you truly betray'd me, when they eat\n
1712  The great God that formed all things both rewa...  The great God who formed all things rewards th...
1713  And said unto the king, Let not my lord impute...  Not perverse should I impute iniquity, nor rem...
1714          Then said the Jews, Will he kill himself?            And will he kill him? And he is dead,\n

[1715 rows x 2 columns]
tstar1 1714
poetry_bible.tsv
strap 1470
tstar2 1471
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1     The immedicable soul,  with heart-aches ever new.  A soul that cannot be supplanted, and whose he...
2             Before his footsteps; as when heav'd anew        As before he walked, so is he in the way.\n
3       By jasper pillars, letting through their shafts  And the jasper pillars, letting the light thro...
4          While the young warrior with a step of grace  But there is a young warrior, whose step is of...
...                                                 ...                                                ...
1466          Might rous'd the slumb'ring dead to hear;  That the dead, being slumbing, may be roused t...
1467                  Go, Fame, an' canter like a filly             Go to fame, and canter like a filly.\n
1468             The cowslips bowed their golden drops,    And the cowslips bowed upon the golden drops.\n
1469     And all her populous streets and temples lewd,  And all her populous streets and her temples a...
1470            Thought I, "Can this be Pope or Steele,  And I thought, that this might be Pontius Pila...

[1471 rows x 2 columns]
tstar1 1470
poetry_shakespeare.tsv
strap 1470
tstar2 1471
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1     The immedicable soul,  with heart-aches ever new.     A soul unalterable, with ever new heartache.\n
2             Before his footsteps; as when heav'd anew                              As before he walks.\n
3       By jasper pillars, letting through their shafts     The jasper pillars let through their shafts.\n
4          While the young warrior with a step of grace        But a young warrior, that steps in grace.\n
...                                                 ...                                                ...
1466          Might rous'd the slumb'ring dead to hear;              A slumbing death may rouse to hear.\n
1467                  Go, Fame, an' canter like a filly                   Go, fame, canter like a filly.\n
1468             The cowslips bowed their golden drops,                Cowslips bowed with golden drops.\n
1469     And all her populous streets and temples lewd,  And all her populous streets and temples are l...
1470            Thought I, "Can this be Pope or Steele,   I thought thou couldst be the pope or Stewart.\n

[1471 rows x 2 columns]
tstar1 1470
shakespeare_poetry.tsv
strap 1293
tstar2 1294
                                                  input                                             output
0                                        Input Sentence                               Generated Sentence\n
1          Give me that mattock and the wrenching iron.         Give me that mattock and wrenching iron,\n
2     One, gentlewoman, that God hath made for himse...                First, Lady! God has made her wed\n
3     Is Rosaline, whom thou didst love so dear, So ...             How soon will thy love rosaline lose\n
4                   O God, I have an ill-divining soul.                  God, I have a ill soul in mine,\n
...                                                 ...                                                ...
1289      Come, madam, let's away, Good morrow, cousin.                Good morrow, cousin, let go away;\n
1290  Take thou some new infection to thy eye, And t...  Take some new infection, and your rank poison ...
1291                          You will set cock-a-hoop!                       Ye'll set the cock-a-hoop!\n
1292               Henceforward I am ever rul'd by you.                   For thou hast always ruled me.\n
1293  Was ever book containing such vile matter So f...     A book containing such matter so fair never?\n

[1294 rows x 2 columns]
tstar1 1293

In [35]: style_specific_dfs
Out[35]: 
                                                  input                                           output_x  ...                                             output                                      tstar1_output
772   Many are the afflictions of the righteous: but...  But there are many faults of the just, and the...  ...  Many a righteous man suffers, But the Lord del...  Many a righteous man suffers, But the Lord del...
1460  And the city was broken up, and all the men of...  And all the men of the army which were about t...  ...  The city is broke, and all the afflictors are ...  The city is broke, and all the afflictors are ...
1236                Salute every saint in Christ Jesus.                   To the saints of God, salutes.\n  ...                              Salute every saint!\n                              Salute every saint!\n
174   But every woman that prayeth or prophesieth wi...  But every woman that prays or prophesies With ...  ...  But every woman, even with her uncovered head,...  But every woman, even with her uncovered head,...
1145  As a dog returneth to his vomit, so a fool ret...  An as dog returns from his vomit, so a fool re...  ...  The fool returns to vomit, as the dog does to ...  The fool returns to vomit, as the dog does to ...
...                                                 ...                                                ...  ...                                                ...                                                ...
990   Dear love, adieu.— Anon, good Nurse!—Sweet Mon...          And love, farewell.-- Anon, fair nurse!\n  ...           And gratefu' grateful Montgomery's way\n           And gratefu' grateful Montgomery's way\n
1695                      Come forth, thou fearful man.  Come, thou whose frighted man thou shouldst be,\n  ...                   Come, come, thou fearful man!"\n                   Come, come, thou fearful man!"\n
1345  The gray-eyed morn smiles on the frowning nigh...  The grey-eyed dawn smiles on frowning night, a...  ...  Gray Morn smiled night, checking out clouds fl...  Gray Morn smiled night, checking out clouds fl...
109                               Have at thee, coward!               Behold, coward! thou must'st flee!\n  ...  Have, coward! thou wilt find grace in thy tong...  Have, coward! thou wilt find grace in thy tong...
1376                          Hang thee, young baggage!      And hang ye down, ye young fellows, to some\n  ...          Hang on young baggage, O thou art free,\n          Hang on young baggage, O thou art free,\n

[3000 rows x 8 columns]

In [36]: style_specific_dfs[["input", "tstar1_output", "tstar2_output"]]
Out[36]: 
                                                  input                                      tstar1_output                                      tstar2_output
772   Many are the afflictions of the righteous: but...  Many a righteous man suffers, But the Lord del...  There is many a right-winger affected, But he ...
1460  And the city was broken up, and all the men of...  The city is broke, and all the afflictors are ...  The city is broke up, and nighttime all the lo...
1236                Salute every saint in Christ Jesus.                              Salute every saint!\n             Hail to every saint in Christ Jesus.\n
174   But every woman that prayeth or prophesieth wi...  But every woman, even with her uncovered head,...  But every woman that prays with her head and p...
1145  As a dog returneth to his vomit, so a fool ret...  The fool returns to vomit, as the dog does to ...  The fool returns his folly as the dog does ret...
...                                                 ...                                                ...                                                ...
990   Dear love, adieu.— Anon, good Nurse!—Sweet Mon...           And gratefu' grateful Montgomery's way\n            Farewell, dear Love! good Nurse Anon!\n
1695                      Come forth, thou fearful man.                   Come, come, thou fearful man!"\n            Come fearful, fearful, o'er the hill,\n
1345  The gray-eyed morn smiles on the frowning nigh...  Gray Morn smiled night, checking out clouds fl...  Night frowning Titan smiles, checking east clo...
109                               Have at thee, coward!  Have, coward! thou wilt find grace in thy tong...                Have it, coward, hae ye been fain\n
1376                          Hang thee, young baggage!          Hang on young baggage, O thou art free,\n        Hang yon young baggage, ye youthfu' gent,\n

[3000 rows x 3 columns]

In [37]: style_specific_dfs.to_csv("final_df.tsv", sep="\t", index=False)

In [38]: cd /Users/preksh/Downloads/sts_dataset\ 2
/Users/preksh/Downloads/sts_dataset 2

In [39]: ls
score.txt                sent2.txt                sts_smatch_analysis.tsv
sent1.txt                sts/

In [40]: sts_scores = open("score.txt").readlines()

In [41]: sts_scores = [float(i.strip()) for i in sts_scores]

In [42]: sts_scores
Out[42]: 
[0.0,
 5.0,
 4.75,
 5.0,
 2.4,
 2.75,
 2.615,
 5.0,
 2.333,
 3.75,
 5.0,
 3.2,
 1.583,
 5.0,
 5.0,
 4.909,
 0.8,
 2.4,
 5.0,
 4.0,
 0.636,
 3.0,
 1.714,
 3.2,
 2.167,
 1.0,
 1.917,
 4.25,
 3.0,
 1.0,
 0.6,
 2.6,
 5.0,
 4.6,
 5.0,
 4.8,
 3.8,
 5.0,
 5.0,
 4.2,
 1.4,
 3.6,
 2.8,
 1.6,
 3.0,
 1.4,
 0.25,
 0.25,
 0.0,
 4.0,
 4.5,
 0.5,
 3.8,
 4.8,
 5.0,
 0.25,
 1.2,
 0.6,
 0.8,
 3.8,
 0.0,
 3.5,
 4.5,
 2.8,
 3.8,
 3.8,
 0.0,
 4.0,
 4.25,
 2.812,
 4.25,
 3.0,
 1.0,
 3.75,
 0.0,
 0.4,
 4.0,
 2.8,
 3.75,
 1.154,
 2.75,
 2.8,
 0.0,
 0.0,
 3.4,
 5.0,
 0.8,
 2.25,
 2.75,
 4.5,
 2.6,
 3.8,
 2.8,
 1.6,
 0.0,
 1.333,
 2.6,
 0.6,
 0.0,
 0.0,
 3.0,
 0.0,
 0.2,
 3.2,
 2.0,
 0.0,
 3.0,
 3.091,
 2.75,
 1.2,
 0.5,
 0.25,
 0.0,
 0.0,
 0.5,
 0.0,
 0.6,
 4.0,
 3.4,
 0.0,
 0.0,
 1.0,
 0.0,
 2.4,
 0.4,
 1.8,
 2.5,
 0.083,
 0.0,
 1.0,
 4.5,
 0.0,
 3.6,
 5.0,
 5.0,
 5.0,
 5.0,
 3.8,
 5.0,
 2.5,
 3.824,
 1.6,
 5.0,
 5.0,
 2.375,
 5.0,
 1.25,
 1.25,
 3.0,
 2.167,
 1.4,
 4.0,
 3.6,
 4.857,
 0.4,
 0.2,
 1.3,
 1.2,
 1.2,
 4.4,
 1.8,
 1.4,
 0.4,
 4.4,
 3.25,
 0.778,
 2.25,
 2.75,
 2.0,
 0.833,
 3.75,
 1.8,
 4.333,
 4.214,
 0.0,
 3.4,
 4.2,
 0.8,
 4.2,
 2.75,
 2.2,
 1.2,
 1.0,
 1.533,
 0.2,
 3.0,
 3.8,
 0.75,
 3.0,
 0.4,
 3.4,
 3.8,
 1.4,
 3.4,
 3.2,
 2.333,
 0.8,
 0.0,
 3.0,
 3.75,
 0.0,
 0.0,
 0.0,
 0.5,
 0.5,
 0.4,
 0.75,
 2.5,
 1.8,
 2.5,
 0.5,
 0.4,
 1.2,
 2.75,
 0.4,
 0.6,
 0.8,
 3.0,
 0.4,
 3.2,
 1.25,
 5.0,
 0.2,
 3.0,
 1.4,
 3.8,
 2.75,
 0.0,
 2.8,
 0.0,
 0.0,
 2.6,
 0.1,
 0.0,
 2.0,
 3.75,
 3.1,
 2.692,
 4.429,
 5.0,
 0.0,
 0.8,
 1.333,
 0.0,
 0.6,
 0.0,
 0.0,
 0.0,
 3.4,
 2.2,
 0.0,
 3.6,
 0.0,
 1.4,
 2.2,
 3.8,
 2.6,
 0.4,
 4.0,
 2.25,
 3.2,
 0.0,
 0.4,
 3.8,
 0.8,
 4.2,
 3.6,
 2.0,
 4.2,
 3.4,
 3.0,
 3.4,
 3.6,
 3.0,
 2.4,
 2.0,
 4.0,
 0.0,
 4.0,
 4.2,
 0.8,
 2.2,
 3.8,
 3.2,
 4.4,
 0.0,
 1.4,
 2.6,
 0.4,
 0.0,
 3.2,
 4.6,
 0.0,
 0.6,
 1.2,
 3.8,
 3.2,
 2.6,
 5.0,
 0.0,
 3.2,
 4.0,
 1.2,
 4.4,
 3.4,
 4.4,
 0.8,
 4.6,
 4.2,
 0.0,
 3.2,
 0.0,
 1.4,
 3.2,
 1.8,
 1.8,
 0.0,
 3.8,
 3.8,
 4.0,
 0.0,
 3.2,
 1.6,
 3.6,
 1.0,
 3.6,
 2.0,
 3.6,
 4.0,
 3.6,
 3.2,
 2.8,
 2.4,
 3.6,
 1.8,
 0.2,
 3.4,
 1.2,
 1.4,
 2.6,
 2.4,
 0.0,
 4.0,
 3.0,
 4.0,
 4.0,
 2.0,
 4.0,
 2.2,
 2.2,
 3.4,
 3.2,
 4.0,
 3.2,
 3.8,
 3.0,
 4.0,
 2.2,
 3.4,
 3.8,
 0.0,
 0.0,
 4.8,
 3.0,
 0.8,
 4.2,
 4.2,
 0.0,
 4.2,
 4.6,
 5.0,
 0.0,
 3.2,
 2.6,
 2.2,
 4.6,
 5.0,
 4.6,
 4.6,
 4.8,
 0.6,
 0.2,
 2.2,
 4.8,
 1.2,
 2.2,
 4.6,
 2.6,
 3.6,
 0.8,
 2.4,
 4.8,
 5.0,
 0.4,
 3.2,
 1.8,
 3.2,
 3.4,
 4.8,
 4.2,
 2.6,
 2.2,
 1.4,
 2.6,
 1.2,
 1.8,
 4.0,
 0.4,
 0.0,
 0.4,
 3.0,
 4.0,
 1.4,
 0.4,
 2.4,
 2.8,
 4.6,
 4.2,
 3.2,
 1.2,
 1.8,
 2.6,
 1.6,
 0.0,
 3.8,
 4.0,
 4.8,
 2.4,
 5.0,
 0.0,
 3.6,
 2.4,
 4.2,
 0.2,
 4.2,
 3.2,
 0.6,
 1.6,
 0.0,
 1.4,
 4.8,
 4.0,
 3.0,
 0.2,
 1.6,
 4.4,
 4.8,
 0.4,
 2.4,
 3.0,
 2.0,
 4.6,
 1.0,
 5.0,
 1.4,
 0.0,
 3.0,
 0.6,
 0.0,
 2.6,
 1.2,
 5.0,
 3.4,
 0.8,
 0.8,
 1.0,
 0.0,
 0.0,
 2.0,
 2.4,
 2.2,
 3.8,
 2.2,
 4.6,
 2.8,
 2.0,
 4.2,
 4.5,
 0.0,
 1.8,
 4.2,
 4.2,
 1.4,
 3.6,
 0.6,
 5.0,
 0.8,
 0.0,
 0.0,
 1.8,
 0.8,
 2.8,
 0.0,
 0.8,
 1.8,
 1.4,
 1.8,
 2.4,
 1.6,
 3.8,
 4.8,
 0.2,
 1.0,
 0.4,
 0.4,
 4.0,
 3.4,
 3.0,
 1.8,
 2.2,
 3.6,
 0.4,
 0.2,
 3.8,
 4.2,
 1.2,
 3.4,
 2.4,
 3.2,
 2.2,
 4.4,
 2.6,
 0.2,
 3.2,
 2.2,
 5.0,
 5.0,
 2.2,
 0.4,
 1.0,
 2.2,
 2.0,
 1.2,
 4.0,
 1.0,
 4.2,
 3.4,
 4.0,
 4.8,
 0.4,
 4.4,
 0.4,
 0.0,
 3.0,
 4.6,
 0.4,
 1.4,
 3.0,
 1.6,
 2.4,
 0.0,
 1.6,
 1.6,
 0.2,
 2.2,
 2.0,
 0.4,
 4.8,
 2.0,
 0.2,
 3.8,
 2.2,
 2.0,
 4.0,
 4.6,
 1.4,
 0.8,
 0.6,
 1.2,
 1.6,
 0.0,
 0.6,
 3.0,
 2.4,
 0.6,
 4.6,
 0.6,
 4.8,
 5.0,
 0.2,
 0.6,
 0.8,
 3.6,
 0.0,
 4.4,
 4.6,
 2.8,
 4.0,
 1.0,
 5.0,
 0.4,
 0.8,
 0.4,
 0.0,
 1.6,
 1.6,
 3.6,
 3.0,
 2.8,
 0.2,
 1.0,
 1.4,
 2.8,
 3.0,
 1.6,
 2.8,
 4.0,
 0.8,
 2.0,
 4.4,
 4.6,
 2.4,
 4.4,
 0.8,
 3.8,
 1.4,
 2.8,
 3.0,
 1.6,
 1.0,
 2.6,
 1.6,
 0.2,
 3.0,
 3.0,
 3.2,
 3.0,
 0.6,
 1.0,
 0.6,
 0.8,
 2.4,
 1.0,
 0.2,
 0.6,
 3.6,
 0.2,
 0.2,
 0.0,
 0.0,
 1.2,
 0.0,
 0.4,
 0.4,
 3.0,
 4.4,
 3.2,
 3.4,
 3.4,
 3.6,
 0.8,
 0.8,
 1.0,
 1.6,
 1.0,
 3.2,
 2.0,
 0.0,
 0.6,
 0.0,
 1.4,
 2.0,
 2.6,
 4.2,
 2.8,
 0.0,
 0.0,
 2.0,
 0.0,
 2.6,
 2.6,
 0.0,
 2.6,
 0.0,
 1.6,
 0.0,
 0.6,
 1.8,
 3.8,
 1.6,
 3.2,
 2.6,
 3.0,
 1.4,
 1.6,
 1.6,
 1.0,
 1.8,
 1.8,
 1.4,
 2.6,
 2.0,
 1.0,
 1.4,
 0.6,
 1.4,
 0.4,
 1.8,
 4.0,
 0.6,
 2.8,
 2.6,
 2.6,
 0.6,
 4.4,
 2.2,
 1.0,
 0.0,
 1.6,
 1.8,
 3.8,
 3.0,
 1.4,
 3.0,
 0.4,
 3.6,
 3.4,
 2.8,
 4.2,
 4.2,
 1.8,
 1.0,
 2.0,
 1.0,
 1.6,
 2.6,
 3.2,
 0.4,
 0.0,
 0.0,
 2.2,
 1.5,
 0.6,
 4.0,
 1.8,
 0.6,
 1.6,
 2.4,
 1.0,
 2.0,
 1.6,
 0.2,
 0.2,
 2.0,
 0.0,
 3.2,
 1.0,
 2.0,
 2.4,
 0.0,
 1.6,
 3.8,
 1.2,
 2.0,
 1.0,
 2.0,
 0.6,
 0.0,
 0.0,
 3.4,
 2.6,
 0.4,
 2.8,
 2.0,
 1.6,
 1.4,
 1.2,
 2.2,
 0.6,
 2.6,
 3.0,
 2.2,
 1.8,
 0.6,
 0.0,
 1.6,
 0.8,
 0.2,
 1.0,
 2.8,
 0.6,
 2.8,
 1.6,
 1.4,
 1.4,
 3.0,
 3.2,
 2.8,
 3.4,
 2.0,
 2.8,
 0.0,
 0.2,
 0.8,
 0.0,
 4.2,
 0.2,
 3.2,
 0.0,
 0.6,
 0.0,
 4.8,
 3.8,
 1.8,
 0.4,
 2.6,
 1.6,
 1.4,
 2.0,
 1.8,
 1.2,
 0.8,
 2.2,
 3.2,
 1.4,
 1.4,
 0.0,
 1.6,
 0.8,
 2.8,
 1.8,
 0.67,
 2.6,
 0.4,
 2.4,
 2.8,
 2.0,
 3.0,
 2.6,
 1.8,
 3.8,
 3.0,
 1.4,
 1.6,
 0.0,
 0.6,
 0.0,
 3.4,
 3.6,
 2.2,
 3.0,
 1.8,
 2.4,
 2.6,
 1.4,
 1.6,
 1.6,
 1.4,
 2.8,
 3.8,
 3.4,
 0.0,
 2.0,
 0.0,
 3.8,
 0.2,
 0.6,
 1.8,
 1.8,
 1.2,
 0.0,
 1.0,
 0.4,
 0.8,
 3.0,
 3.8,
 3.2,
 2.6,
 3.0,
 2.6,
 1.8,
 2.6,
 0.8,
 1.6,
 0.6,
 2.6,
 1.2,
 0.0,
 2.4,
 0.4,
 0.6,
 1.0,
 2.6,
 4.0,
 3.6,
 2.6,
 1.6,
 4.0,
 3.0,
 0.6,
 0.0,
 0.4,
 0.4,
 2.0,
 0.6,
 0.0,
 3.2,
 2.8,
 2.6,
 2.8,
 0.2,
 3.2,
 0.6,
 3.6,
 0.0,
 0.0,
 0.0,
 0.0,
 2.2,
 0.0,
 0.4,
 0.0,
 2.6,
 0.8,
 0.4,
 3.0,
 2.2,
 0.6,
 3.4,
 2.2,
 1.8,
 0.8,
 0.0,
 1.6,
 2.8,
 1.67,
 1.8,
 2.8,
 0.0,
 0.6,
 1.8,
 0.4,
 0.2,
 0.0,
 1.4,
 0.0,
 0.6,
 0.8,
 0.2,
 2.2,
 1.8,
 0.2,
 4.0,
 4.2,
 4.4,
 3.0,
 2.6,
 0.6,
 3.2,
 2.6,
 1.2,
 3.0,
 0.0,
 2.6,
 1.2,
 2.8,
 0.2,
 1.8,
 0.0,
 0.0,
 3.0,
 0.0,
 2.4,
 0.4,
 2.6,
 0.0,
 3.6,
 1.8,
 1.6,
 2.0,
 2.0,
 0.0,
 2.6,
 0.4,
 0.0,
 0.2,
 1.8,
 1.6,
 1.0,
 0.6,
 1.0,
 2.8,
 2.6,
 3.4,
 1.6,
 4.0,
 1.8,
 0.2,
 0.0,
 1.4,
 0.0,
 1.2,
 3.6,
 3.0,
 1.2,
 1.8,
 0.8,
 1.2,
 0.0,
 3.2,
 ...]

In [43]: 

In [43]: smatch_scores = open("sts/smatch.txt").readlines()

In [44]: smatch_scores = [i.strip().split("F: ")[1] for i in smatch_scores]

In [45]: smatch_scores = [float(i) for i in smatch_scores]

In [46]: smatch_scores
Out[46]: 
[0.8,
 0.7,
 0.8571428571428571,
 1.0,
 0.8333333333333334,
 0.8333333333333334,
 0.8333333333333334,
 1.0,
 0.7692307692307692,
 0.6666666666666665,
 1.0,
 0.8333333333333334,
 0.8333333333333334,
 1.0,
 0.7777777777777777,
 1.0,
 0.6666666666666666,
 0.6666666666666666,
 1.0,
 0.6666666666666666,
 0.75,
 0.8333333333333334,
 0.8333333333333334,
 0.7142857142857143,
 0.8333333333333334,
 0.8333333333333334,
 0.8333333333333334,
 0.8571428571428571,
 0.7777777777777777,
 0.6,
 0.5,
 0.75,
 0.6666666666666666,
 0.4444444444444445,
 1.0,
 0.8181818181818182,
 0.875,
 1.0,
 1.0,
 0.8333333333333334,
 0.8333333333333334,
 0.7777777777777777,
 0.6,
 0.6,
 0.7142857142857143,
 0.8333333333333334,
 0.5,
 0.4,
 0.5,
 0.5555555555555556,
 0.5555555555555556,
 0.5263157894736842,
 0.5555555555555556,
 0.5555555555555556,
 0.7,
 0.5,
 0.7142857142857143,
 0.6666666666666666,
 0.6666666666666666,
 0.6666666666666666,
 0.42857142857142855,
 0.7142857142857143,
 0.6,
 0.7142857142857143,
 0.6666666666666666,
 0.6086956521739131,
 0.5,
 0.8333333333333334,
 0.5,
 0.28571428571428575,
 0.5555555555555556,
 0.5555555555555556,
 0.6666666666666666,
 0.64,
 0.33333333333333326,
 0.42857142857142855,
 0.4444444444444445,
 0.6666666666666665,
 0.375,
 0.5,
 0.625,
 0.5,
 0.4615384615384615,
 0.3333333333333333,
 0.42857142857142855,
 0.6956521739130435,
 0.5,
 0.4444444444444445,
 0.5714285714285715,
 0.8333333333333334,
 0.5714285714285715,
 0.5161290322580646,
 0.5714285714285715,
 0.6666666666666666,
 0.3333333333333333,
 0.5,
 0.5,
 0.5,
 0.43478260869565216,
 0.5,
 0.28571428571428564,
 0.4,
 0.5714285714285715,
 0.7142857142857143,
 0.3333333333333333,
 0.3333333333333333,
 0.888888888888889,
 0.625,
 0.5714285714285715,
 0.4,
 0.5,
 0.42857142857142855,
 0.4,
 0.14285714285714288,
 0.6666666666666666,
 0.4444444444444445,
 0.6,
 0.47058823529411764,
 0.34782608695652173,
 0.2,
 0.3333333333333333,
 0.4210526315789474,
 0.37499999999999994,
 0.7142857142857143,
 0.4,
 0.4444444444444444,
 0.5714285714285715,
 0.42857142857142855,
 0.125,
 0.4444444444444445,
 0.3157894736842105,
 0.22222222222222224,
 0.8333333333333334,
 0.8333333333333334,
 0.875,
 1.0,
 1.0,
 0.8333333333333334,
 0.7142857142857143,
 0.8333333333333334,
 0.888888888888889,
 0.6666666666666666,
 0.8571428571428571,
 0.8571428571428571,
 0.8333333333333334,
 1.0,
 0.75,
 0.75,
 0.6666666666666666,
 0.8333333333333334,
 0.6666666666666666,
 0.8333333333333334,
 0.8333333333333334,
 1.0,
 0.6666666666666666,
 0.6,
 0.6666666666666665,
 0.75,
 0.75,
 0.5714285714285715,
 0.8333333333333334,
 0.6666666666666666,
 0.6666666666666666,
 0.9166666666666666,
 0.7142857142857143,
 0.5714285714285715,
 0.8333333333333334,
 0.6363636363636364,
 0.42857142857142855,
 0.5714285714285715,
 0.7777777777777777,
 0.7142857142857143,
 0.8000000000000002,
 0.5714285714285715,
 0.5,
 0.5,
 0.7,
 0.6666666666666666,
 0.5,
 0.4000000000000001,
 0.8333333333333334,
 0.5714285714285715,
 0.6666666666666666,
 0.6666666666666666,
 0.6,
 0.6666666666666666,
 0.7272727272727272,
 0.6666666666666666,
 0.8,
 0.5,
 0.6,
 0.6666666666666667,
 0.7142857142857143,
 0.7142857142857143,
 0.5263157894736842,
 0.5333333333333333,
 0.375,
 0.4,
 0.5217391304347826,
 0.888888888888889,
 0.42857142857142855,
 0.42857142857142855,
 0.42857142857142855,
 0.5,
 0.6,
 0.6666666666666666,
 0.6666666666666666,
 0.42857142857142855,
 0.5,
 0.5,
 0.6666666666666666,
 0.6153846153846153,
 0.5,
 0.631578947368421,
 0.375,
 0.5714285714285715,
 0.5714285714285715,
 0.4615384615384615,
 0.28571428571428575,
 0.4761904761904762,
 0.3529411764705882,
 0.8333333333333334,
 0.5714285714285715,
 0.5,
 0.33333333333333326,
 0.5,
 0.2857142857142857,
 0.28571428571428575,
 0.37499999999999994,
 0.5,
 0.42857142857142855,
 0.37499999999999994,
 0.28571428571428575,
 0.375,
 0.6666666666666667,
 0.6,
 0.6153846153846153,
 0.5263157894736842,
 0.5714285714285715,
 0.8181818181818182,
 0.25,
 0.4444444444444444,
 0.4,
 0.375,
 0.380952380952381,
 0.5,
 0.2727272727272727,
 0.3333333333333333,
 0.380952380952381,
 0.5,
 0.28571428571428575,
 0.5,
 0.2222222222222222,
 0.5555555555555556,
 0.4375,
 0.36363636363636365,
 0.5,
 0.2,
 0.4,
 0.5,
 0.3125,
 0.380952380952381,
 0.4444444444444445,
 0.64,
 0.6666666666666666,
 0.5,
 0.75,
 0.28571428571428575,
 0.5,
 0.15,
 0.33333333333333326,
 0.6060606060606061,
 0.6666666666666665,
 0.7368421052631577,
 0.6666666666666665,
 0.3,
 0.5555555555555556,
 0.2,
 0.6250000000000001,
 0.6363636363636365,
 0.20000000000000004,
 0.625,
 0.7,
 0.7,
 0.6666666666666666,
 0.28571428571428575,
 0.6,
 0.4444444444444445,
 0.5555555555555556,
 0.21428571428571427,
 0.5882352941176471,
 0.6153846153846153,
 0.17391304347826086,
 0.5714285714285715,
 0.625,
 0.4545454545454546,
 0.39999999999999997,
 0.75,
 0.9166666666666666,
 0.1,
 0.5714285714285714,
 0.7777777777777777,
 0.5,
 0.5599999999999999,
 0.3448275862068966,
 0.48484848484848486,
 0.5333333333333333,
 0.8181818181818182,
 0.8750000000000001,
 0.25,
 0.625,
 0.38461538461538464,
 0.5454545454545454,
 0.6666666666666667,
 0.4444444444444445,
 0.26666666666666666,
 0.16,
 0.75,
 0.3,
 0.3157894736842105,
 0.36363636363636365,
 0.4000000000000001,
 0.45454545454545453,
 0.35294117647058826,
 0.4666666666666667,
 0.4210526315789474,
 0.2631578947368421,
 0.5714285714285715,
 0.5555555555555556,
 0.5333333333333333,
 0.23076923076923078,
 0.36363636363636365,
 0.3243243243243243,
 0.4000000000000001,
 0.39999999999999997,
 0.25,
 0.6000000000000001,
 0.33333333333333326,
 0.3333333333333333,
 0.5,
 0.7777777777777777,
 0.4,
 0.7142857142857142,
 0.3448275862068965,
 0.8,
 0.30769230769230765,
 0.4444444444444445,
 0.4444444444444445,
 0.4444444444444445,
 0.6428571428571429,
 0.5555555555555556,
 0.7000000000000001,
 0.6666666666666665,
 0.5454545454545454,
 0.5,
 0.7826086956521738,
 0.6363636363636365,
 0.7428571428571429,
 0.888888888888889,
 0.5714285714285715,
 0.2727272727272727,
 0.16,
 0.9285714285714286,
 0.4117647058823529,
 0.3636363636363636,
 0.5,
 0.7692307692307693,
 0.4444444444444445,
 0.875,
 0.6923076923076923,
 0.8888888888888888,
 0.20689655172413793,
 0.44444444444444436,
 0.5454545454545454,
 0.5,
 0.9166666666666666,
 0.608695652173913,
 0.56,
 0.5714285714285715,
 0.8461538461538461,
 0.47058823529411764,
 0.3636363636363636,
 0.4166666666666667,
 0.7407407407407408,
 0.29787234042553196,
 0.5185185185185185,
 0.5714285714285715,
 0.32,
 0.6,
 0.3225806451612903,
 0.5714285714285714,
 0.6666666666666667,
 0.7692307692307692,
 0.3448275862068965,
 0.5,
 0.75,
 0.8,
 0.5833333333333334,
 0.875,
 0.6,
 0.6666666666666665,
 0.4615384615384615,
 0.3157894736842105,
 0.3,
 0.3157894736842105,
 0.4848484848484849,
 0.6000000000000001,
 0.36363636363636365,
 0.3,
 0.3243243243243243,
 0.6896551724137931,
 0.6363636363636364,
 0.25,
 0.34782608695652173,
 0.26086956521739135,
 0.21428571428571427,
 0.8000000000000002,
 0.8333333333333333,
 0.5454545454545454,
 0.45454545454545453,
 0.7142857142857143,
 0.75,
 0.6250000000000001,
 0.25,
 0.7142857142857143,
 0.6666666666666666,
 0.5714285714285715,
 0.6666666666666665,
 0.5454545454545454,
 0.20000000000000004,
 0.6428571428571429,
 0.3333333333333333,
 0.8571428571428571,
 0.25,
 0.7333333333333334,
 0.8571428571428571,
 0.5,
 0.6,
 0.14285714285714288,
 0.38888888888888884,
 1.0,
 0.7499999999999999,
 0.6666666666666666,
 0.22222222222222224,
 0.5714285714285713,
 0.5925925925925926,
 0.875,
 0.24242424242424246,
 0.35714285714285715,
 0.9,
 0.6666666666666667,
 0.8888888888888888,
 0.3,
 0.8333333333333334,
 0.14285714285714285,
 0.3529411764705882,
 0.6315789473684211,
 0.34782608695652173,
 0.10526315789473685,
 0.5,
 0.3636363636363636,
 0.8000000000000002,
 0.4444444444444445,
 0.29629629629629634,
 0.21621621621621623,
 0.36363636363636365,
 0.3870967741935484,
 0.25,
 0.5833333333333334,
 0.3703703703703704,
 0.3846153846153846,
 0.42857142857142855,
 0.5882352941176471,
 0.6666666666666665,
 0.4117647058823529,
 0.5,
 0.6,
 0.380952380952381,
 0.3333333333333333,
 0.25,
 0.8750000000000001,
 0.7777777777777778,
 0.4,
 0.3255813953488372,
 0.28571428571428575,
 0.6363636363636365,
 0.6,
 0.2631578947368421,
 0.28571428571428575,
 0.7692307692307692,
 0.20689655172413793,
 0.8,
 0.3157894736842105,
 0.6666666666666665,
 0.31578947368421056,
 0.4,
 0.42857142857142855,
 0.48648648648648646,
 0.6,
 0.6666666666666667,
 0.875,
 0.15384615384615383,
 0.2,
 0.20512820512820512,
 0.1379310344827586,
 0.6,
 0.5833333333333334,
 0.24242424242424243,
 0.625,
 0.5555555555555556,
 0.5714285714285715,
 0.3636363636363637,
 0.23529411764705885,
 0.8095238095238096,
 0.8333333333333334,
 0.4150943396226415,
 0.5,
 0.5,
 0.875,
 0.6666666666666666,
 0.8571428571428571,
 0.7000000000000001,
 0.18749999999999997,
 0.5,
 0.36363636363636365,
 0.4666666666666667,
 0.5333333333333333,
 0.5,
 0.25,
 0.3157894736842105,
 0.4,
 0.4,
 0.46153846153846156,
 0.4,
 0.6,
 0.9375,
 0.75,
 0.28571428571428575,
 0.888888888888889,
 0.34285714285714286,
 0.8571428571428571,
 0.33333333333333337,
 0.2105263157894737,
 0.4666666666666667,
 0.7741935483870968,
 0.10526315789473685,
 0.380952380952381,
 0.5384615384615384,
 0.875,
 0.6153846153846153,
 0.18181818181818182,
 0.5833333333333334,
 0.358974358974359,
 0.3,
 0.631578947368421,
 0.42105263157894735,
 0.29629629629629634,
 0.6666666666666665,
 0.4444444444444444,
 0.13793103448275862,
 0.8571428571428571,
 0.6666666666666665,
 0.3846153846153846,
 0.8571428571428571,
 0.6451612903225806,
 0.34285714285714286,
 0.3684210526315789,
 0.5263157894736842,
 0.4444444444444445,
 0.4,
 0.2105263157894737,
 0.1,
 0.2631578947368421,
 0.875,
 0.25,
 0.5925925925925926,
 0.5,
 0.8571428571428571,
 0.4,
 0.28571428571428575,
 0.5555555555555556,
 0.3703703703703704,
 0.4736842105263158,
 0.07142857142857142,
 0.8571428571428571,
 1.0,
 0.18181818181818182,
 0.7,
 0.35714285714285715,
 1.0,
 0.3,
 0.36363636363636365,
 0.3,
 0.31250000000000006,
 0.21621621621621623,
 0.5,
 0.625,
 0.7692307692307692,
 0.6,
 0.16666666666666666,
 0.2962962962962963,
 0.32,
 0.9,
 0.2,
 0.1875,
 0.625,
 0.5882352941176471,
 0.3333333333333333,
 0.47058823529411764,
 0.8571428571428571,
 0.7777777777777778,
 0.75,
 0.5,
 0.16666666666666666,
 0.9090909090909091,
 0.4081632653061225,
 0.56,
 0.38461538461538464,
 0.75,
 0.3846153846153846,
 0.3157894736842105,
 0.25,
 0.1818181818181818,
 0.8333333333333334,
 0.7142857142857143,
 0.5,
 0.339622641509434,
 0.28571428571428575,
 0.15384615384615383,
 0.2758620689655172,
 0.3050847457627119,
 0.35,
 0.35294117647058826,
 0.3846153846153846,
 0.22222222222222224,
 0.32653061224489793,
 0.17543859649122806,
 0.18867924528301885,
 0.20408163265306123,
 0.22857142857142854,
 0.2105263157894737,
 0.163265306122449,
 0.11320754716981132,
 0.22727272727272724,
 0.3571428571428571,
 0.3076923076923077,
 0.375,
 0.23809523809523808,
 0.2631578947368421,
 0.28571428571428575,
 0.25,
 0.17142857142857143,
 0.20689655172413793,
 0.2105263157894737,
 0.14285714285714285,
 0.425531914893617,
 0.2857142857142857,
 0.17777777777777778,
 0.23529411764705882,
 0.11764705882352941,
 0.24999999999999994,
 0.23255813953488372,
 0.26865671641791045,
 0.1904761904761905,
 0.20408163265306123,
 0.25,
 0.12903225806451615,
 0.17777777777777778,
 0.17142857142857143,
 0.21739130434782608,
 0.25,
 0.1886792452830189,
 0.15,
 0.22857142857142854,
 0.2692307692307692,
 0.2711864406779661,
 0.25,
 0.15,
 0.6530612244897959,
 0.2711864406779661,
 0.2222222222222222,
 0.24242424242424246,
 0.4444444444444444,
 0.20833333333333334,
 0.2105263157894737,
 0.3913043478260869,
 0.21739130434782608,
 0.35294117647058826,
 0.26666666666666666,
 0.19607843137254902,
 0.125,
 0.21739130434782608,
 0.10526315789473684,
 0.057142857142857134,
 0.13793103448275862,
 0.208955223880597,
 0.509090909090909,
 0.3529411764705882,
 0.39999999999999997,
 0.26666666666666666,
 0.5333333333333333,
 0.35000000000000003,
 0.3125,
 0.2,
 0.3913043478260869,
 0.40816326530612246,
 0.2790697674418605,
 0.22727272727272727,
 0.18181818181818182,
 0.07017543859649122,
 0.28571428571428575,
 0.16666666666666666,
 0.17857142857142855,
 0.3076923076923077,
 0.1904761904761905,
 0.15789473684210525,
 0.16666666666666669,
 0.253968253968254,
 0.4489795918367347,
 0.37500000000000006,
 0.18867924528301888,
 0.2745098039215686,
 0.24137931034482757,
 0.2127659574468085,
 0.1923076923076923,
 0.14285714285714288,
 0.2580645161290323,
 0.22222222222222224,
 0.24999999999999994,
 0.1923076923076923,
 0.1818181818181818,
 0.32,
 0.28571428571428575,
 0.3846153846153846,
 0.30769230769230765,
 0.17391304347826086,
 0.2,
 0.13636363636363638,
 0.25,
 0.1818181818181818,
 0.19230769230769232,
 0.35000000000000003,
 0.13333333333333333,
 0.25641025641025644,
 0.3018867924528302,
 0.2222222222222222,
 0.23076923076923078,
 0.16666666666666666,
 0.34782608695652173,
 0.23529411764705882,
 0.16216216216216214,
 0.32558139534883723,
 0.14634146341463414,
 0.4545454545454545,
 0.2790697674418605,
 0.411764705882353,
 0.13953488372093023,
 0.22950819672131148,
 0.2909090909090909,
 0.5,
 0.25,
 0.25,
 0.21052631578947367,
 0.33333333333333326,
 0.1791044776119403,
 0.35294117647058826,
 0.3050847457627119,
 0.273972602739726,
 0.3714285714285714,
 0.44897959183673464,
 0.372093023255814,
 0.26229508196721313,
 0.23809523809523808,
 0.1081081081081081,
 0.22857142857142856,
 0.40816326530612246,
 0.2153846153846154,
 0.13043478260869565,
 0.1951219512195122,
 0.28571428571428575,
 0.21052631578947367,
 0.391304347826087,
 0.3125,
 0.27586206896551724,
 0.339622641509434,
 0.35555555555555557,
 0.34285714285714286,
 0.15384615384615385,
 0.2666666666666666,
 0.21818181818181817,
 0.23529411764705882,
 0.13793103448275862,
 0.2,
 0.32727272727272727,
 0.13333333333333333,
 0.2,
 0.3225806451612903,
 0.23255813953488372,
 0.25,
 0.21818181818181817,
 0.1694915254237288,
 0.6206896551724139,
 0.3902439024390244,
 0.22857142857142854,
 0.23809523809523808,
 0.2127659574468085,
 0.30188679245283023,
 0.21621621621621623,
 0.2857142857142857,
 0.25,
 0.2790697674418605,
 0.2545454545454545,
 0.2666666666666666,
 0.28571428571428575,
 0.2413793103448276,
 0.1587301587301587,
 0.23076923076923078,
 0.4,
 0.339622641509434,
 0.2807017543859649,
 0.17857142857142858,
 0.14634146341463417,
 0.19230769230769232,
 0.22580645161290322,
 0.33333333333333326,
 0.41025641025641024,
 0.3703703703703704,
 0.2941176470588235,
 0.2745098039215686,
 0.31818181818181823,
 0.5555555555555556,
 0.3333333333333333,
 0.27272727272727276,
 0.3243243243243243,
 0.09523809523809522,
 0.21538461538461542,
 0.23529411764705882,
 0.17543859649122806,
 0.2941176470588235,
 0.18181818181818182,
 0.2380952380952381,
 0.15384615384615385,
 0.32142857142857145,
 0.1818181818181818,
 0.18181818181818185,
 0.17391304347826086,
 0.1724137931034483,
 0.25,
 0.5405405405405405,
 0.4666666666666667,
 0.30769230769230765,
 0.2105263157894737,
 0.2580645161290323,
 0.3333333333333333,
 0.41025641025641024,
 0.27027027027027023,
 0.13043478260869565,
 0.15,
 0.34615384615384615,
 0.21052631578947367,
 0.21739130434782608,
 0.27777777777777773,
 0.2,
 0.1904761904761905,
 0.45714285714285713,
 0.40579710144927533,
 0.20408163265306123,
 0.20000000000000004,
 0.21621621621621623,
 0.3278688524590164,
 0.1917808219178082,
 0.23809523809523808,
 0.4,
 0.23333333333333334,
 0.10714285714285714,
 0.16901408450704225,
 0.27450980392156865,
 0.2222222222222222,
 0.22222222222222224,
 0.16,
 0.1702127659574468,
 0.2926829268292683,
 0.20000000000000004,
 0.3768115942028986,
 0.5945945945945946,
 0.37499999999999994,
 0.30188679245283023,
 0.4878048780487805,
 0.26666666666666666,
 0.0930232558139535,
 0.15384615384615383,
 0.27906976744186046,
 0.19512195121951217,
 0.2702702702702703,
 0.2647058823529412,
 0.2,
 0.38461538461538464,
 0.2641509433962264,
 0.2857142857142857,
 0.39285714285714285,
 0.24000000000000002,
 0.5306122448979592,
 0.42553191489361697,
 0.4210526315789474,
 0.3225806451612903,
 0.27027027027027023,
 0.11320754716981131,
 0.24242424242424243,
 0.22222222222222224,
 0.3255813953488372,
 0.27027027027027023,
 0.24242424242424243,
 0.2769230769230769,
 0.2,
 0.1923076923076923,
 0.3666666666666667,
 0.15999999999999998,
 0.1818181818181818,
 0.11320754716981131,
 0.37209302325581395,
 0.14285714285714285,
 0.2222222222222222,
 0.12244897959183673,
 0.14285714285714282,
 0.37837837837837834,
 0.4067796610169492,
 0.25,
 0.42105263157894735,
 0.16666666666666663,
 0.21052631578947367,
 0.3793103448275862,
 0.3673469387755102,
 0.13636363636363638,
 0.2222222222222222,
 0.22727272727272727,
 0.1754385964912281,
 0.24137931034482757,
 0.3125,
 0.16666666666666666,
 0.25641025641025644,
 0.375,
 0.23529411764705882,
 0.8823529411764706,
 0.5490196078431373,
 0.4761904761904762,
 0.36065573770491804,
 0.25925925925925924,
 0.2608695652173913,
 0.3174603174603175,
 0.17647058823529413,
 0.2857142857142857,
 0.35294117647058826,
 0.45454545454545453,
 0.20512820512820512,
 0.15999999999999998,
 0.35294117647058826,
 0.27027027027027023,
 0.16666666666666666,
 0.16666666666666663,
 0.14285714285714288,
 0.2857142857142857,
 0.2711864406779661,
 0.3404255319148936,
 0.04761904761904762,
 0.43636363636363634,
 0.25925925925925924,
 0.5789473684210527,
 0.20833333333333331,
 0.4827586206896552,
 0.34782608695652173,
 0.26666666666666666,
 0.23809523809523808,
 0.23076923076923078,
 0.2285714285714286,
 0.25,
 0.2191780821917808,
 0.14545454545454545,
 0.11428571428571428,
 0.2857142857142857,
 0.18518518518518517,
 0.09302325581395349,
 0.3013698630136986,
 0.5,
 0.2222222222222222,
 0.22222222222222224,
 0.3333333333333333,
 0.27450980392156865,
 0.20408163265306123,
 0.2631578947368421,
 0.19999999999999998,
 0.20512820512820512,
 0.21276595744680848,
 0.3243243243243243,
 0.22727272727272724,
 0.2222222222222222,
 0.1818181818181818,
 0.13333333333333333,
 0.1724137931034483,
 0.23529411764705882,
 0.17777777777777778,
 ...]

In [47]: sts_dict={}

In [48]: def get_key(i):
    ...:     for ind in [0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1]:
    ...:         if i <= ind:
    ...:             return ind
    ...: 

In [49]: import seaborn as sns
sns.
In [50]: sns.set_style("white")

In [51]: sns
Out[51]: <module 'seaborn' from '/Users/preksh/Library/Python/3.8/lib/python/site-packages/seaborn/__init__.py'>

In [52]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     print(k)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(smatch_scores[ind])
    ...: 
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.7
None
None
None
None
1
None
None
None
1
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
0.3
0.1
None
None
0.5
None
None
None
0.3
None
0.6
0.8
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
1
None
0.1
0.4
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
0.6
0.1
0.1
None
0.1
0.2
None
None
0.1
None
None
None
None
0.5
0.3
0.1
0.1
0.5
0.1
0.6
None
None
0.1
0.1
1
0.1
None
0.4
None
None
0.1
0.1
1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
None
None
0.8
None
None
None
0.9
None
None
None
None
0.1
None
None
0.8
None
None
None
None
1
None
0.2
None
None
0.8
None
0.4
None
None
None
None
None
None
0.8
0.1
None
None
0.1
0.1
0.1
0.5
0.5
0.4
0.8
None
None
None
0.5
0.4
None
None
0.4
0.6
0.8
None
0.4
None
None
None
0.2
None
None
None
None
0.1
None
0.1
0.1
None
0.1
0.1
None
None
None
None
None
None
0.1
0.8
None
0.1
0.6
0.1
0.1
0.1
None
None
0.1
None
0.1
None
None
None
None
0.4
None
None
None
0.1
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.8
None
None
None
None
0.1
None
None
0.4
0.1
None
None
0.1
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
0.8
None
None
0.1
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
None
None
1
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
0.4
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.2
None
None
0.6
None
0.1
None
None
None
None
0.2
None
None
None
0.4
None
None
None
None
1
None
None
0.1
None
0.6
0.1
None
None
None
None
0.8
0.8
1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
None
0.8
0.1
0.1
None
0.8
None
0.1
0.8
None
None
None
None
None
None
None
0.2
1
0.4
0.4
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.4
1
None
None
None
None
1
None
None
None
None
0.4
None
0.4
0.1
None
None
0.4
None
None
None
None
0.1
None
None
0.2
None
None
0.4
None
None
0.2
None
None
None
None
None
None
0.8
0.6
None
None
0.1
0.6
None
None
0.6
None
0.6
None
None
0.2
0.6
0.8
None
0.1
None
None
None
None
1
None
0.4
0.8
0.4
0.1
None
None
None
None
None
0.2
1
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
None
None
None
1
None
None
0.2
None
None
None
None
0.6
1
0.6
0.8
None
1
0.2
0.6
None
0.2
0.2
0.1
0.1
None
0.1
0.4
0.4
None
None
None
None
None
None
0.8
0.8
1
None
1
None
None
0.1
0.6
0.1
None
None
None
None
None
0.1
0.1
None
0.1
None
None
0.1
None
0.1
None
0.1
0.6
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
1
None
0.6
None
0.4
None
None
0.6
None
None
None
0.6
None
None
1
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
1
None
1
None
None
None
0.4
0.1
0.1
None
None
0.6
None
None
0.6
None
None
1
None
None
0.2
0.2
None
0.1
None
1
None
None
0.1
None
None
None
None
1
None
0.6
0.1
0.1
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
0.6
0.1
None
0.8
0.2
1
None
0.6
None
None
None
None
None
None
None
None
None
None
0.1
0.2
0.8
0.1
None
0.2
None
0.1
0.6
0.1
None
None
None
0.4
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
0.8
None
None
0.7
None
0.4
None
None
None
None
None
None
None
None
None
None
0.1
0.6
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.2
0.6
None
None
None
0.1
1
0.4
0.8
None
None
None
None
None
None
None
None
0.8
None
0.6
None
None
0.1
None
0.4
0.6
1
None
None
None
None
None
None
None
0.6
0.1
0.4
0.4
None
0.6
0.1
None
None
None
None
0.2
None
0.6
None
0.1
0.1
0.1
0.1
None
0.1
0.4
0.1
None
0.8
0.4
None
None
0.6
None
None
None
0.8
0.1
None
None
None
None
None
0.1
0.6
None
0.4
0.2
0.1
None
0.1
0.6
0.8
0.2
None
None
0.2
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
None
0.2
None
0.1
0.1
None
0.1
None
0.4
None
0.1
None
None
None
None
None
0.1
None
0.4
0.1
0.2
None
None
1
0.6
1
None
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
None
None
0.8
None
0.1
None
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
0.6
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.4
None
None
None
None
None
None
None
None
None
None
None
1
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
1
None
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
None
None
None
1
None
None
0.1
None
0.4
None
0.6
None
0.1
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
0.1
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
0.1
0.2
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.4
None
None
None
None
1
None
None
None
None
None
None
0.1
0.1
None
None
0.2
None
0.1
0.4
None
0.8
0.4
None
None
None
None
1
1
None
0.4
0.2
0.1
0.1
0.1
0.6
0.6
None
0.1
0.8
None
None
None
None
1
None
None
None
None
0.4
0.1
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
0.1
0.1
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
1
None
0.2
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.7
None
None
None
None
None
None
None
None
None
None
1
1
0.6
0.4
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
0.5
None
None
None
None
None
None
None
None
0.1
0.1
0.3
None
None
0.8
None
None
None
0.2
0.8
None
None
0.4
0.8
None
None
None
None
0.1
1
0.1
None
0.4
0.4
0.6
None
0.4
0.4
0.4
None
0.6
0.8
None
None
0.6
0.6
0.1
None
None
None
None
0.6
0.4
None
None
None
None
None
0.2
0.4
None
None
0.6
None
None
None
None
None
0.4
None
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
0.5
0.1
0.1
0.8
0.9
None
0.4
None
None
0.8
0.1
0.1
None
None
None
None
None
None
None
None
0.1
0.3
None
None
0.1
None
None
None
None
None
None
1
None
None
None
0.1
0.1
None
None
0.2
None
None
0.1
None
0.1
None
None
None
None
0.9
0.1
None
None
None
0.2
None
None
None
0.4
0.1
0.1
0.1
0.2
0.1
0.1
None
None
None
None
None
0.4
0.1
0.4
0.6
1
None
None
None
None
0.1
0.1
0.1
0.4
0.4
None
None
0.8
0.2
0.1
0.1
None
0.8
0.1
0.3
0.5
None
None
None
0.4
0.1
1
0.8
0.1
None
None
None
None
None
None
None
None
None
None
0.2
1
0.4
None
0.1
None
None
None
0.1
0.1
None
None
None
None
0.8
0.8
None
None
0.1
0.1
0.1
None
None
None
0.8
None
None
None
None
0.8
0.1
0.1
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
0.1
0.5
0.1
1
None
0.1
None
None
0.1
0.1
None
None
None
None
None
0.1
1
None
None
None
0.1
0.1
0.1
0.1
None
0.7
0.1
None
None
None
0.1
0.2
0.5
0.1
None
0.1
1
0.1
0.1
0.1
None
None
0.6
0.3
None
None
None
None
0.8
None
None
None
None
0.1
None
None
None
0.2
0.1
0.1
0.8
0.1
0.1
0.1
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.5
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.1
None
None
0.1
1
None
None
None
None
None
1
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.3
None
None
None
None
None
None
1
None
0.4
None
None
None
1
None
None
None
None
None
None
0.5
None
None
1
None
None
0.4
0.4
None
None
0.3
0.3
0.3
None
None
0.1
None
None
None
None
None
0.8
None
None
None
0.8
None
0.1
0.7
None
None
0.4
None
None
0.8
0.8
0.8
0.8
1
0.8
None
None
None
None
None
None
0.3
None
None
0.8
0.8
0.8
0.3
None
None
0.5
0.1
0.5
0.6
None
None
None
None
None
0.1
None
0.1
None
0.1
0.4
0.1
None
None
0.1
None
1
0.1
None
None
0.3
0.4
None
None
None
None
None
1
None
None
None
None
None
None
None
None
0.2
None
0.8
0.8
0.8
0.3
None
None
None
None
None
None
None
0.4
None
0.4
None
None
0.5
0.5
None
None
None
None
None
None
0.8
0.3
0.8
None
0.8
0.1
None
None
0.1
0.3
0.1
None
None
0.4
0.8
None
None
None
0.2
0.2
0.5
0.1
None
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
0.5
None
0.1
0.1
0.1
1
None
0.6
None
0.5
None
None
None
0.1
0.8
0.8
0.4
0.1
0.1
0.1
0.4
0.1
None
0.3
0.1
0.5
0.1
None
0.8
None
0.1
None
None
0.1
None
0.8
0.5
None
None
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
1
None
None
None
None
1
0.1
0.1
None
0.4
0.4
None
0.1
0.1
0.1
0.1
0.4
1
0.3
None
0.2
1
0.4
0.1
0.1
None
0.8
None
None
None
0.1
None
0.1
0.1
0.1
None
None
0.6
0.1
None
0.4
0.4
None
None
0.1
0.8
0.1
0.1
0.8
None
0.1
None
0.3
None
0.7
None
0.4
None
None
1
None
0.4
0.1
0.3
None
None
None
None
None
0.2
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.8
1
None
None
None
None
0.1
0.6
1
0.1
0.1
1
0.1
None
0.1
None
0.1
0.8
0.1
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.6
None
None
None
0.6
0.1
None
None
0.1
None
None
None
None
1
None
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.8
0.6
0.1
None
None
None
0.2
None
None
None
None
0.4
0.6
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
None
None
0.1
None
1
None
None
None
None
0.1
None
None
None
None
0.1
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
None
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1
None
None
0.2
None
None
None
None
None
None
None
None
None
0.6
None
0.1
0.8
None
0.2
None
0.1
0.2
None
None
0.1
None
None
None
0.4
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.4
0.4
0.1
None
None
None
None
None
None
None
None
1
None
None
0.1
None
0.4
None
0.1
None
None
0.4
None
0.4
None
0.1
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
1
None
0.1
None
0.1
None
None
0.8
None
None
None
None
None
None
0.1
None
0.1
None
None
None
0.4
None
None
None
None
None
None
None
1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
1
0.1
0.8
0.1
0.1
0.1
None
None
None
None
1
None
None
None
0.8
0.8
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
0.4
None
1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
0.4
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
None
None
None
0.1
None
None
None
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.1
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.8
None
None
None
None
None
0.4
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.6
None
0.4
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
0.4
0.1
None
0.1
None
None
0.6
0.6
None
None
0.6
None
0.1
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
None
None
None
None
None
0.6
None
None
0.1
None
None
None
None
None
None
0.1
None
None
0.1
1
None
0.1
None
None
0.2
None
0.8
0.8
None
None
None
None
1
None
None
None
None
None
None
0.4
None
None
None
None
0.2
0.1
0.2
None
None
None
None
None
0.5
None
None
None
None
None
0.8
None
None
0.1
None
None
None
None
None
0.1
0.4
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
0.8
None
0.1
None
None
None
None
None
0.4
None
None
0.1
0.1
None
None
None
None
None
None
0.4
None
0.4
None
0.1
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
1
None
0.1
None
None
0.1
0.1
None
0.1
None
0.1
None
None
0.8
None
None
None
0.1
None
0.1
None
0.1
None
None
None
0.1
None
0.8
None
None
0.4
1
1
None
None
None
None
0.1
0.6
None
None
None
None
1
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
0.1
0.1
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1
0.2
None
0.1
None
None
None
None
None
None
None
0.2
None
None
1
None
0.1
None
0.1
None
0.1
None
None
0.2
None
None
0.6
0.8
None
None
None
0.6
0.4
None
None
None
None
None
0.1
None
0.6
None
0.4
None
None
0.6
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
1
None
0.6
None
0.8
0.4
0.8
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.8
0.4
None
None
None
None
0.1
None
None
None
1
None
None
None
None
None
None
None
None
None
0.4
None
0.1
None
0.1
None
0.6
0.4
None
None
None
None
0.1
None
None
None
None
None
None
1
None
0.8
0.2
None
None
None
None
1
0.1
0.1
None
None
None
None
None
None
None
1
1
None
None
0.8
None
None
None
None
None
0.8
1
None
None
None
None
None
None
None
None
None
None
None
0.2
0.1
None
None
None
None
0.1
0.1
None
None
None
None
0.5
None
None
None
None
1
None
None
None
None
0.4
None
None
1
1
0.1
None
0.6
None
0.1
0.6
0.1
0.1
None
None
None
None
1
None
0.8
None
1
0.4
None
None
None
None
0.6
1
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
1
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
0.1
None
None
None
None
None
None
None
1
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
1
0.8
None
0.2
None
1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
1
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
1
None
None
None
None
0.8
None
None
None
None
None
1
None
None
None
1
None
None
None
None
1
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.8
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.1
None
None
None
None
None
None
None
None
None
None
1
0.4
1
None
None
None
None
0.8
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1
0.2
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
1
0.6
None
None
None
None
0.6
None
0.4
None
None
None
None
0.8
None
0.6
None
None
1
0.6
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
None
None
1
0.4
None
0.8
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1
None
None
0.4
None
None
None
1
None
None
None
None
None
0.8
0.2
None
None
None
None
1
None
0.8
None
None
None
None
None
None
0.2
1
None
None
0.4
0.1
None
None
None
None
0.1
0.1
None
0.6
None
None
1
None
None
None
0.8
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.4
1
None
None
0.8
None
None
1
None
1
None
0.6
None
None
0.1
None
None
None
0.1
None
None
None
1
None
None
None
None
1
None
None
None
None
1
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.6
None
None
None
None
None
None
1
None
0.8
None
None
None
0.8
None
None
None
None
0.6
None
None
None
None
None
0.1
None
None
None
0.8
None
None
None
None
None
0.4
None
0.4
0.2
None
0.8
None
None
None
None
None
None
None
None
1
None
0.6
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
1
None
None
None
None
None
None
0.8
1
None
None
None
None
None
None
None
None
None
None
None
1
None
0.5
1
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.6
1
None
None
None
None
0.2
None
0.6
None
None
None
1
None
None
None
0.8
None
0.4
0.8
None
None
None
0.4
None
None
None
None
None
None
0.1
1
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
1
None
None
0.6
None
None
None
None
None
None
None
None
None
None
1
None
None
1
None
1
0.8
None
None
None
0.8
None
None
None
None
None
0.8
None
None
0.8
0.1
None
None
0.2
None
0.1
None
0.8
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.1
1
None
None
None
0.8
None
None
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
0.6
None
0.8
None
0.2
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.6
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.8
None
None
1
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
None
1
None
None
None
None
None
None
0.6
1
None
None
None
None
None
0.4
None
None
None
None
0.4
0.6
None
1
None
None
None
None
None
1
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.8
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.8
0.6
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
1
None
None
None
1
0.2
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
0.8
1
None
None
1
1
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1
0.1
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
0.6
None
0.6
None
None
0.1
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
None
None
None
1
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
1
None
0.1
0.8
None
0.8
None
None
0.1
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.1
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
None
0.1
None
0.1
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
0.6
None
None
None
1
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
1
None
0.2
None
None
None
None
None
None
None
0.1
None
None
1
0.4
None
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
0.6
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.4
None
None
1
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
None
0.4
0.4
1
None
0.1
0.1
None
None
None
0.4
None
0.1
1
1
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
0.2
None
1
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1
None
0.6
0.4
None
None
None
None
1
None
None
0.4
None
0.6
None
None
0.1
0.4
None
0.1
None
None
None
None
None
None
None
None
None
None
None
1
0.8
None
0.6
None
None
None
0.6
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
0.4
None
0.8
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
0.1
None
None
1
None
None
1
0.1
None
None
None
None
None
None
None
None
None
0.8
1
0.1
None
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.6
None
None
None
0.4
None
None
None
None
0.8
0.8
1
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.4
0.6
None
1
None
None
None
None
None
None
None
0.1
None
None
0.1
0.2
None
None
None
None
None
None
0.1
None
None
None
0.1
0.2
None
0.2
None
None
0.1
None
0.6
None
None
None
None
None
0.4
None
1
None
None
None
None
0.1
None
None
0.2
None
1
None
None
0.2
None
None
None
None
None
None
None
1
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.2
None
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
0.1
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
0.4
0.6
None
0.1
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.2
None
None
None
None
0.4
None
None
None
0.2
1
None
0.1
0.6
None
1
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
0.4
None
0.1
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1
1
None
None
None
None
0.1
None
1
None
None
None
None
1
None
1
1
None
1
None
None
0.1
None
0.1
None
None
1
None
None
None
None
None
None
1
None
None
None
None
1
1
None
None
None
None
None
1
None
1
None
None
None
None
0.1
None
None
None
1
0.1
None
None
None
None
None
1
0.1
None
None
None
None
None
1
1
None
0.1
None
None
1
1
None
1
1
0.1
None
1
None
1
1
1
0.1
0.1
None
1
None
0.1
0.1
1
1
1
1
0.1
0.1
0.1
0.1
1
0.1
1
0.1
None
None
0.1
1
0.1
0.1
0.1
0.1
0.1
0.1
1
0.1
0.1
None
None
0.1
0.1
0.1
0.1
0.1

In [53]: sts_dict
Out[53]: 
{0.1: [511,
  [0.8,
   0.5,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.43478260869565216,
   0.5,
   0.4,
   0.3333333333333333,
   0.4,
   0.14285714285714288,
   0.4444444444444445,
   0.2,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.125,
   0.22222222222222224,
   0.5,
   0.4,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.28571428571428575,
   0.5,
   0.42857142857142855,
   0.28571428571428575,
   0.375,
   0.25,
   0.375,
   0.5,
   0.2727272727272727,
   0.3333333333333333,
   0.28571428571428575,
   0.2222222222222222,
   0.380952380952381,
   0.2,
   0.28571428571428575,
   0.21428571428571427,
   0.17391304347826086,
   0.1,
   0.25,
   0.38461538461538464,
   0.16,
   0.36363636363636365,
   0.4,
   0.2727272727272727,
   0.16,
   0.4444444444444445,
   0.20689655172413793,
   0.3,
   0.25,
   0.20000000000000004,
   0.14285714285714288,
   0.3529411764705882,
   0.10526315789473685,
   0.3870967741935484,
   0.25,
   0.3333333333333333,
   0.2631578947368421,
   0.28571428571428575,
   0.3157894736842105,
   0.2105263157894737,
   0.18181818181818182,
   0.2105263157894737,
   0.07142857142857142,
   0.31250000000000006,
   0.20408163265306123,
   0.22857142857142854,
   0.163265306122449,
   0.17777777777777778,
   0.11764705882352941,
   0.25,
   0.12903225806451615,
   0.17142857142857143,
   0.1886792452830189,
   0.22857142857142854,
   0.2711864406779661,
   0.22727272727272727,
   0.24999999999999994,
   0.1923076923076923,
   0.3018867924528302,
   0.23529411764705882,
   0.22950819672131148,
   0.2909090909090909,
   0.22857142857142856,
   0.13793103448275862,
   0.13333333333333333,
   0.25,
   0.1694915254237288,
   0.23076923076923078,
   0.09523809523809522,
   0.23529411764705882,
   0.2105263157894737,
   0.3333333333333333,
   0.21739130434782608,
   0.2222222222222222,
   0.15384615384615383,
   0.2,
   0.3225806451612903,
   0.27027027027027023,
   0.11320754716981131,
   0.24242424242424243,
   0.3255813953488372,
   0.24242424242424243,
   0.12244897959183673,
   0.16666666666666663,
   0.2222222222222222,
   0.1754385964912281,
   0.45454545454545453,
   0.16666666666666663,
   0.14285714285714288,
   0.2711864406779661,
   0.25925925925925924,
   0.23809523809523808,
   0.25,
   0.2631578947368421,
   0.20512820512820512,
   0.23529411764705882,
   0.2,
   0.33333333333333337,
   0.38888888888888884,
   0.2857142857142857,
   0.4186046511627907,
   0.4285714285714286,
   0.3448275862068966,
   0.30303030303030304,
   0.42105263157894735,
   0.5625,
   0.25641025641025644,
   0.16,
   0.4375,
   0.26315789473684204,
   0.5365853658536585,
   0.23529411764705882,
   0.3428571428571428,
   0.4571428571428572,
   0.4090909090909091,
   0.4313725490196078,
   0.8,
   0.5,
   0.5,
   0.6666666666666666,
   0.6,
   0.4,
   0.5,
   0.3333333333333333,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.39999999999999997,
   0.28571428571428575,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.4615384615384615,
   0.3333333333333333,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.5,
   0.4,
   0.5,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.28571428571428575,
   0.3333333333333333,
   0.28571428571428575,
   0.26666666666666666,
   0.39999999999999997,
   0.26666666666666666,
   0.42857142857142855,
   0.380952380952381,
   0.2857142857142857,
   0.1739130434782609,
   0.4,
   0.28571428571428575,
   0.3157894736842105,
   0.5333333333333333,
   0.28571428571428575,
   0.3333333333333333,
   0.3333333333333333,
   0.4,
   0.25,
   0.3,
   0.16,
   0.21052631578947364,
   0.25,
   0.30769230769230765,
   0.3333333333333333,
   0.42857142857142855,
   0.39999999999999997,
   0.5,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.2857142857142857,
   0.4705882352941177,
   0.4,
   0.5,
   0.5,
   0.16666666666666666,
   0.42857142857142855,
   0.3636363636363636,
   0.375,
   0.4,
   0.42857142857142855,
   0.26666666666666666,
   0.42857142857142855,
   0.3333333333333333,
   0.42857142857142855,
   0.13333333333333333,
   0.26666666666666666,
   0.28571428571428575,
   0.4444444444444445,
   0.42857142857142855,
   0.5,
   0.4,
   0.28571428571428575,
   0.35294117647058826,
   0.5,
   0.26666666666666666,
   0.5,
   0.37499999999999994,
   0.23529411764705885,
   0.3333333333333333,
   0.4,
   0.3333333333333333,
   0.42857142857142855,
   0.3333333333333333,
   0.5,
   0.3333333333333333,
   0.3333333333333333,
   0.37499999999999994,
   0.4,
   0.37499999999999994,
   0.42857142857142855,
   0.37499999999999994,
   0.2105263157894737,
   0.3157894736842105,
   0.375,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.375,
   0.28571428571428575,
   0.5555555555555556,
   0.2758620689655172,
   0.25,
   0.25,
   0.34285714285714286,
   0.11111111111111112,
   0.1818181818181818,
   0.19354838709677416,
   0.47058823529411764,
   0.21428571428571427,
   0.32,
   0.3333333333333333,
   0.25,
   0.3636363636363636,
   0.11764705882352942,
   0.3,
   0.3,
   0.4,
   0.4166666666666667,
   0.3181818181818182,
   0.25,
   0.28571428571428575,
   0.2727272727272727,
   0.37499999999999994,
   0.3157894736842105,
   0.18749999999999997,
   0.27586206896551724,
   0.42857142857142855,
   0.3157894736842105,
   0.29411764705882354,
   0.31250000000000006,
   0.5217391304347826,
   0.3,
   0.24000000000000002,
   0.17391304347826086,
   0.4444444444444445,
   0.4,
   0.19999999999999998,
   0.375,
   0.33333333333333337,
   0.43478260869565216,
   0.380952380952381,
   0.42857142857142855,
   0.09090909090909091,
   0.5,
   0.5555555555555556,
   0.25,
   0.3478260869565218,
   0.18181818181818182,
   0.16666666666666666,
   0.29629629629629634,
   0.4000000000000001,
   0.25,
   0.26666666666666666,
   0.2727272727272727,
   0.16,
   0.1904761904761905,
   0.19354838709677422,
   0.3870967741935483,
   0.3333333333333333,
   0.24000000000000002,
   0.28571428571428564,
   0.14285714285714288,
   0.32,
   0.3225806451612903,
   0.31250000000000006,
   0.08695652173913043,
   0.17391304347826086,
   0.3,
   0.3076923076923077,
   0.27586206896551724,
   0.2777777777777778,
   0.2857142857142857,
   0.33333333333333326,
   0.36363636363636365,
   0.4000000000000001,
   0.33333333333333326,
   0.4666666666666667,
   0.21428571428571427,
   0.19047619047619047,
   0.5,
   0.23999999999999996,
   0.2,
   0.375,
   0.21428571428571427,
   0.3333333333333333,
   0.2631578947368421,
   0.3333333333333333,
   0.26086956521739135,
   0.30769230769230765,
   0.23076923076923075,
   0.375,
   0.3,
   0.25,
   0.16666666666666663,
   0.16,
   0.28571428571428575,
   0.24242424242424246,
   0.15384615384615385,
   0.33333333333333337,
   0.3157894736842105,
   0.6666666666666665,
   0.3225806451612903,
   0.23076923076923075,
   0.25,
   0.4000000000000001,
   0.23076923076923075,
   0.2,
   0.6206896551724138,
   0.25,
   0.5517241379310344,
   0.3636363636363636,
   0.4680851063829788,
   0.15384615384615383,
   0.26666666666666666,
   0.631578947368421,
   0.5161290322580646,
   0.5625,
   0.39999999999999997,
   0.631578947368421,
   0.6153846153846153,
   0.36842105263157887,
   0.42105263157894735,
   0.22857142857142856,
   0.2857142857142857,
   0.30769230769230765,
   0.4375,
   0.30769230769230765,
   0.3,
   0.27777777777777773,
   0.42857142857142855,
   0.3225806451612903,
   0.13333333333333333,
   0.4444444444444444,
   0.625,
   0.25,
   0.36363636363636365,
   0.36363636363636365,
   0.35714285714285715,
   0.3111111111111111,
   0.2162162162162162,
   0.6666666666666666,
   0.22222222222222224,
   0.4,
   0.26666666666666666,
   0.3333333333333333,
   0.5416666666666667,
   0.22857142857142856,
   0.3333333333333333,
   0.3333333333333333,
   0.4,
   0.18181818181818182,
   0.3076923076923077,
   0.3448275862068966,
   0.43902439024390244,
   0.34285714285714286,
   0.4210526315789474,
   0.35000000000000003,
   0.46808510638297873,
   0.34285714285714286,
   0.24999999999999994,
   0.358974358974359,
   0.6153846153846153,
   0.375,
   0.22222222222222224,
   0.358974358974359,
   0.34782608695652173,
   0.35294117647058826,
   0.3448275862068966,
   0.43999999999999995,
   0.2424242424242424,
   0.23076923076923075,
   0.13333333333333333,
   0.45161290322580644,
   0.33333333333333326,
   0.3684210526315789,
   0.6842105263157895,
   0.35294117647058826,
   0.26666666666666666,
   0.26666666666666666,
   0.4897959183673469,
   0.3333333333333333,
   0.6060606060606061,
   0.7027027027027027,
   0.22857142857142856,
   0.3448275862068966,
   0.16666666666666666,
   0.2631578947368421,
   0.3181818181818182,
   0.4090909090909091,
   0.18181818181818182,
   0.3,
   0.35294117647058826,
   0.3333333333333333,
   0.5106382978723405,
   0.2777777777777778,
   0.3888888888888889,
   0.3125,
   0.24242424242424243,
   0.3333333333333333,
   0.6046511627906976,
   0.45,
   0.5555555555555556,
   0.11764705882352941,
   0.29411764705882354,
   0.34285714285714286,
   0.6666666666666666,
   0.5957446808510638,
   0.4166666666666667,
   0.6818181818181819,
   0.6382978723404256,
   0.8181818181818182,
   0.5217391304347826,
   0.4615384615384615,
   0.52,
   0.6285714285714286,
   0.5,
   0.4848484848484849,
   0.14814814814814817,
   0.4444444444444444,
   0.4150943396226415,
   0.5714285714285715,
   0.4864864864864864,
   0.375,
   0.36,
   0.29411764705882354,
   0.46511627906976744,
   0.558139534883721,
   0.4444444444444445,
   0.3333333333333333,
   0.38095238095238093,
   0.42424242424242425,
   0.41025641025641024,
   0.34285714285714286,
   0.3333333333333333,
   0.47619047619047616,
   0.30769230769230765,
   0.1904761904761905]],
 None: [5757,
  [0.7,
   0.8571428571428571,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.7692307692307692,
   0.6666666666666665,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.7777777777777777,
   1.0,
   0.6666666666666666,
   1.0,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.8333333333333334,
   0.8571428571428571,
   0.7777777777777777,
   0.75,
   0.6666666666666666,
   0.4444444444444445,
   1.0,
   0.8181818181818182,
   0.875,
   1.0,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   0.7777777777777777,
   0.6,
   0.6,
   0.7142857142857143,
   0.8333333333333334,
   0.5555555555555556,
   0.5555555555555556,
   0.5555555555555556,
   0.5555555555555556,
   0.7,
   0.7142857142857143,
   0.6666666666666666,
   0.7142857142857143,
   0.6,
   0.7142857142857143,
   0.6666666666666666,
   0.6086956521739131,
   0.8333333333333334,
   0.5,
   0.28571428571428575,
   0.5555555555555556,
   0.5555555555555556,
   0.64,
   0.4444444444444445,
   0.6666666666666665,
   0.375,
   0.5,
   0.625,
   0.5,
   0.42857142857142855,
   0.6956521739130435,
   0.4444444444444445,
   0.5714285714285715,
   0.8333333333333334,
   0.5714285714285715,
   0.5161290322580646,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.5,
   0.28571428571428564,
   0.7142857142857143,
   0.3333333333333333,
   0.888888888888889,
   0.625,
   0.5714285714285715,
   0.4,
   0.47058823529411764,
   0.34782608695652173,
   0.7142857142857143,
   0.4444444444444444,
   0.5714285714285715,
   0.3157894736842105,
   0.8333333333333334,
   0.8333333333333334,
   0.875,
   1.0,
   1.0,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.888888888888889,
   0.6666666666666666,
   0.8571428571428571,
   0.8571428571428571,
   0.8333333333333334,
   1.0,
   0.75,
   0.75,
   0.6666666666666666,
   0.8333333333333334,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.6666666666666665,
   0.75,
   0.75,
   0.5714285714285715,
   0.8333333333333334,
   0.6666666666666666,
   0.9166666666666666,
   0.7142857142857143,
   0.8333333333333334,
   0.6363636363636364,
   0.42857142857142855,
   0.7777777777777777,
   0.7142857142857143,
   0.8000000000000002,
   0.5714285714285715,
   0.5,
   0.7,
   0.5,
   0.4000000000000001,
   0.8333333333333334,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.7272727272727272,
   0.8,
   0.6,
   0.6666666666666667,
   0.7142857142857143,
   0.7142857142857143,
   0.5263157894736842,
   0.5333333333333333,
   0.5217391304347826,
   0.888888888888889,
   0.42857142857142855,
   0.5,
   0.5,
   0.5,
   0.631578947368421,
   0.4615384615384615,
   0.4761904761904762,
   0.3529411764705882,
   0.8333333333333334,
   0.5,
   0.33333333333333326,
   0.5,
   0.2857142857142857,
   0.37499999999999994,
   0.37499999999999994,
   0.6666666666666667,
   0.6,
   0.6153846153846153,
   0.5263157894736842,
   0.5714285714285715,
   0.8181818181818182,
   0.4,
   0.380952380952381,
   0.5,
   0.5,
   0.5555555555555556,
   0.4375,
   0.36363636363636365,
   0.5,
   0.4,
   0.5,
   0.3125,
   0.64,
   0.5,
   0.75,
   0.28571428571428575,
   0.5,
   0.15,
   0.33333333333333326,
   0.6060606060606061,
   0.6666666666666665,
   0.7368421052631577,
   0.6666666666666665,
   0.3,
   0.5555555555555556,
   0.6250000000000001,
   0.6363636363636365,
   0.625,
   0.7,
   0.7,
   0.6666666666666666,
   0.6,
   0.4444444444444445,
   0.5882352941176471,
   0.6153846153846153,
   0.625,
   0.4545454545454546,
   0.39999999999999997,
   0.75,
   0.9166666666666666,
   0.5714285714285714,
   0.7777777777777777,
   0.5,
   0.5599999999999999,
   0.3448275862068966,
   0.48484848484848486,
   0.8181818181818182,
   0.8750000000000001,
   0.625,
   0.5454545454545454,
   0.6666666666666667,
   0.4444444444444445,
   0.26666666666666666,
   0.75,
   0.3,
   0.3157894736842105,
   0.4000000000000001,
   0.45454545454545453,
   0.35294117647058826,
   0.4210526315789474,
   0.2631578947368421,
   0.5714285714285715,
   0.5555555555555556,
   0.5333333333333333,
   0.23076923076923078,
   0.36363636363636365,
   0.3243243243243243,
   0.4000000000000001,
   0.39999999999999997,
   0.6000000000000001,
   0.33333333333333326,
   0.3333333333333333,
   0.5,
   0.7777777777777777,
   0.7142857142857142,
   0.3448275862068965,
   0.8,
   0.30769230769230765,
   0.4444444444444445,
   0.4444444444444445,
   0.4444444444444445,
   0.6428571428571429,
   0.5555555555555556,
   0.7000000000000001,
   0.6666666666666665,
   0.5454545454545454,
   0.5,
   0.7826086956521738,
   0.6363636363636365,
   0.7428571428571429,
   0.888888888888889,
   0.5714285714285715,
   0.9285714285714286,
   0.4117647058823529,
   0.5,
   0.7692307692307693,
   0.875,
   0.6923076923076923,
   0.8888888888888888,
   0.44444444444444436,
   0.5454545454545454,
   0.5,
   0.9166666666666666,
   0.608695652173913,
   0.56,
   0.5714285714285715,
   0.8461538461538461,
   0.4166666666666667,
   0.7407407407407408,
   0.29787234042553196,
   0.5185185185185185,
   0.5714285714285715,
   0.32,
   0.6,
   0.5714285714285714,
   0.6666666666666667,
   0.7692307692307692,
   0.5,
   0.75,
   0.8,
   0.5833333333333334,
   0.875,
   0.6,
   0.6666666666666665,
   0.4615384615384615,
   0.3157894736842105,
   0.3,
   0.3157894736842105,
   0.4848484848484849,
   0.6000000000000001,
   0.6896551724137931,
   0.6363636363636364,
   0.25,
   0.26086956521739135,
   0.21428571428571427,
   0.8000000000000002,
   0.8333333333333333,
   0.5454545454545454,
   0.45454545454545453,
   0.7142857142857143,
   0.75,
   0.6250000000000001,
   0.7142857142857143,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666665,
   0.5454545454545454,
   0.6428571428571429,
   0.3333333333333333,
   0.8571428571428571,
   0.7333333333333334,
   0.8571428571428571,
   0.6,
   0.38888888888888884,
   1.0,
   0.7499999999999999,
   0.6666666666666666,
   0.5714285714285713,
   0.5925925925925926,
   0.875,
   0.35714285714285715,
   0.9,
   0.6666666666666667,
   0.8888888888888888,
   0.8333333333333334,
   0.14285714285714285,
   0.6315789473684211,
   0.5,
   0.3636363636363636,
   0.8000000000000002,
   0.4444444444444445,
   0.5833333333333334,
   0.3703703703703704,
   0.3846153846153846,
   0.42857142857142855,
   0.5882352941176471,
   0.6666666666666665,
   0.4117647058823529,
   0.5,
   0.6,
   0.380952380952381,
   0.25,
   0.8750000000000001,
   0.7777777777777778,
   0.4,
   0.3255813953488372,
   0.6363636363636365,
   0.7692307692307692,
   0.8,
   0.31578947368421056,
   0.4,
   0.42857142857142855,
   0.48648648648648646,
   0.6,
   0.6666666666666667,
   0.875,
   0.6,
   0.5833333333333334,
   0.24242424242424243,
   0.625,
   0.5555555555555556,
   0.5714285714285715,
   0.8095238095238096,
   0.8333333333333334,
   0.4150943396226415,
   0.5,
   0.5,
   0.875,
   0.6666666666666666,
   0.8571428571428571,
   0.7000000000000001,
   0.5,
   0.36363636363636365,
   0.4666666666666667,
   0.5333333333333333,
   0.5,
   0.4,
   0.4,
   0.46153846153846156,
   0.4,
   0.9375,
   0.75,
   0.28571428571428575,
   0.888888888888889,
   0.8571428571428571,
   0.4666666666666667,
   0.7741935483870968,
   0.380952380952381,
   0.5384615384615384,
   0.875,
   0.6153846153846153,
   0.5833333333333334,
   0.358974358974359,
   0.631578947368421,
   0.42105263157894735,
   0.6666666666666665,
   0.4444444444444444,
   0.8571428571428571,
   0.6666666666666665,
   0.3846153846153846,
   0.8571428571428571,
   0.6451612903225806,
   0.34285714285714286,
   0.4444444444444445,
   0.4,
   0.2631578947368421,
   0.875,
   0.5925925925925926,
   0.8571428571428571,
   0.4,
   0.4736842105263158,
   0.8571428571428571,
   1.0,
   0.18181818181818182,
   0.7,
   1.0,
   0.21621621621621623,
   0.5,
   0.625,
   0.7692307692307692,
   0.6,
   0.32,
   0.9,
   0.2,
   0.1875,
   0.625,
   0.5882352941176471,
   0.47058823529411764,
   0.8571428571428571,
   0.7777777777777778,
   0.75,
   0.5,
   0.9090909090909091,
   0.4081632653061225,
   0.56,
   0.38461538461538464,
   0.75,
   0.3157894736842105,
   0.25,
   0.8333333333333334,
   0.7142857142857143,
   0.5,
   0.339622641509434,
   0.35,
   0.32653061224489793,
   0.2105263157894737,
   0.3571428571428571,
   0.3076923076923077,
   0.375,
   0.23809523809523808,
   0.2631578947368421,
   0.28571428571428575,
   0.2105263157894737,
   0.425531914893617,
   0.2857142857142857,
   0.24999999999999994,
   0.23255813953488372,
   0.26865671641791045,
   0.1904761904761905,
   0.20408163265306123,
   0.17777777777777778,
   0.21739130434782608,
   0.25,
   0.15,
   0.2692307692307692,
   0.15,
   0.6530612244897959,
   0.2711864406779661,
   0.2222222222222222,
   0.24242424242424246,
   0.4444444444444444,
   0.20833333333333334,
   0.2105263157894737,
   0.3913043478260869,
   0.35294117647058826,
   0.26666666666666666,
   0.19607843137254902,
   0.125,
   0.21739130434782608,
   0.057142857142857134,
   0.208955223880597,
   0.3529411764705882,
   0.39999999999999997,
   0.5333333333333333,
   0.35000000000000003,
   0.3125,
   0.3913043478260869,
   0.40816326530612246,
   0.18181818181818182,
   0.07017543859649122,
   0.28571428571428575,
   0.16666666666666666,
   0.17857142857142855,
   0.3076923076923077,
   0.15789473684210525,
   0.16666666666666669,
   0.253968253968254,
   0.4489795918367347,
   0.37500000000000006,
   0.18867924528301888,
   0.24137931034482757,
   0.1923076923076923,
   0.14285714285714288,
   0.2580645161290323,
   0.1818181818181818,
   0.32,
   0.3846153846153846,
   0.30769230769230765,
   0.2,
   0.13636363636363638,
   0.1818181818181818,
   0.19230769230769232,
   0.25641025641025644,
   0.2222222222222222,
   0.16666666666666666,
   0.34782608695652173,
   0.16216216216216214,
   0.32558139534883723,
   0.14634146341463414,
   0.4545454545454545,
   0.411764705882353,
   0.5,
   0.25,
   0.21052631578947367,
   0.33333333333333326,
   0.1791044776119403,
   0.35294117647058826,
   0.3050847457627119,
   0.273972602739726,
   0.44897959183673464,
   0.372093023255814,
   0.26229508196721313,
   0.23809523809523808,
   0.40816326530612246,
   0.28571428571428575,
   0.391304347826087,
   0.3125,
   0.27586206896551724,
   0.339622641509434,
   0.35555555555555557,
   0.34285714285714286,
   0.15384615384615385,
   0.2666666666666666,
   0.21818181818181817,
   0.23529411764705882,
   0.2,
   0.23255813953488372,
   0.6206896551724139,
   0.3902439024390244,
   0.22857142857142854,
   0.2127659574468085,
   0.30188679245283023,
   0.21621621621621623,
   0.2857142857142857,
   0.25,
   0.2790697674418605,
   0.2666666666666666,
   0.28571428571428575,
   0.2413793103448276,
   0.1587301587301587,
   0.4,
   0.2807017543859649,
   0.17857142857142858,
   0.19230769230769232,
   0.33333333333333326,
   0.41025641025641024,
   0.3703703703703704,
   0.2941176470588235,
   0.2745098039215686,
   0.31818181818181823,
   0.5555555555555556,
   0.3333333333333333,
   0.27272727272727276,
   0.3243243243243243,
   0.17543859649122806,
   0.2941176470588235,
   0.18181818181818182,
   0.2380952380952381,
   0.15384615384615385,
   0.32142857142857145,
   0.1818181818181818,
   0.18181818181818185,
   0.17391304347826086,
   0.1724137931034483,
   0.25,
   0.5405405405405405,
   0.4666666666666667,
   0.30769230769230765,
   0.2580645161290323,
   0.41025641025641024,
   0.15,
   0.34615384615384615,
   0.21052631578947367,
   0.45714285714285713,
   0.40579710144927533,
   0.20408163265306123,
   0.20000000000000004,
   0.21621621621621623,
   0.3278688524590164,
   0.1917808219178082,
   0.23809523809523808,
   0.23333333333333334,
   0.16901408450704225,
   0.27450980392156865,
   0.22222222222222224,
   0.20000000000000004,
   0.3768115942028986,
   0.5945945945945946,
   0.37499999999999994,
   0.30188679245283023,
   0.4878048780487805,
   0.26666666666666666,
   0.2702702702702703,
   0.38461538461538464,
   0.2641509433962264,
   0.2857142857142857,
   0.39285714285714285,
   0.5306122448979592,
   0.4210526315789474,
   0.22222222222222224,
   0.2769230769230769,
   0.3666666666666667,
   0.15999999999999998,
   0.11320754716981131,
   0.37209302325581395,
   0.14285714285714285,
   0.14285714285714282,
   0.37837837837837834,
   0.4067796610169492,
   0.25,
   0.42105263157894735,
   0.3793103448275862,
   0.22727272727272727,
   0.25641025641025644,
   0.375,
   0.8823529411764706,
   0.5490196078431373,
   0.4761904761904762,
   0.36065573770491804,
   0.25925925925925924,
   0.3174603174603175,
   0.17647058823529413,
   0.2857142857142857,
   0.35294117647058826,
   0.20512820512820512,
   0.15999999999999998,
   0.35294117647058826,
   0.16666666666666666,
   0.2857142857142857,
   0.3404255319148936,
   0.43636363636363634,
   0.5789473684210527,
   0.20833333333333331,
   0.4827586206896552,
   0.34782608695652173,
   0.26666666666666666,
   0.23076923076923078,
   0.14545454545454545,
   0.11428571428571428,
   0.3013698630136986,
   0.5,
   0.2222222222222222,
   0.22222222222222224,
   0.3333333333333333,
   0.27450980392156865,
   0.19999999999999998,
   0.21276595744680848,
   0.3243243243243243,
   0.22727272727272724,
   0.2222222222222222,
   0.1818181818181818,
   0.1724137931034483,
   0.17777777777777778,
   0.5660377358490567,
   0.7142857142857143,
   0.7241379310344828,
   0.7042253521126761,
   0.5842696629213484,
   0.853658536585366,
   0.56,
   0.7012987012987012,
   0.2666666666666666,
   0.5714285714285714,
   0.5245901639344263,
   0.7777777777777778,
   0.8387096774193549,
   0.45161290322580644,
   0.5396825396825397,
   0.3870967741935483,
   0.6666666666666666,
   0.6545454545454545,
   0.6024096385542168,
   0.7058823529411765,
   0.6329113924050633,
   0.4301075268817204,
   0.44067796610169496,
   0.717948717948718,
   0.5116279069767442,
   0.5714285714285714,
   0.634920634920635,
   0.7605633802816901,
   0.7469879518072288,
   0.6451612903225806,
   0.42424242424242425,
   0.5714285714285715,
   0.8787878787878788,
   0.6067415730337078,
   0.6410256410256411,
   0.7368421052631577,
   0.625,
   0.7857142857142857,
   0.9459459459459459,
   0.6,
   0.7027027027027025,
   0.746268656716418,
   0.6885245901639345,
   0.6896551724137931,
   0.32727272727272727,
   0.5217391304347826,
   0.6530612244897959,
   0.8125,
   0.716417910447761,
   0.5454545454545455,
   0.5,
   0.8,
   0.7058823529411765,
   0.7457627118644068,
   0.5,
   0.6666666666666667,
   0.7666666666666666,
   0.4166666666666667,
   0.782608695652174,
   0.6382978723404256,
   0.6585365853658536,
   0.5633802816901409,
   0.5625,
   0.42500000000000004,
   0.49056603773584906,
   0.6842105263157894,
   0.65625,
   0.7333333333333333,
   0.45161290322580644,
   0.5666666666666667,
   0.48837209302325585,
   0.767123287671233,
   0.5977011494252873,
   0.5483870967741935,
   0.7297297297297297,
   0.7428571428571429,
   0.6779661016949153,
   0.509090909090909,
   0.48275862068965514,
   0.47058823529411764,
   0.5116279069767442,
   0.5581395348837209,
   0.5633802816901409,
   0.6153846153846153,
   0.7692307692307692,
   0.5263157894736842,
   0.48484848484848486,
   0.761904761904762,
   0.5882352941176471,
   0.8,
   0.6578947368421053,
   0.24390243902439024,
   0.48888888888888893,
   0.5970149253731343,
   0.9090909090909091,
   0.5128205128205129,
   0.6363636363636364,
   0.7631578947368423,
   0.5901639344262296,
   0.575,
   0.5757575757575757,
   0.6075949367088608,
   0.8524590163934426,
   0.5977011494252874,
   0.7692307692307693,
   0.5970149253731343,
   0.6370370370370371,
   0.5151515151515151,
   0.47887323943661964,
   0.8809523809523809,
   0.5625,
   0.8260869565217391,
   0.711111111111111,
   0.509090909090909,
   0.48387096774193544,
   0.48,
   0.759493670886076,
   0.5283018867924528,
   0.7142857142857142,
   0.46511627906976744,
   0.2553191489361702,
   0.4545454545454546,
   0.490566037735849,
   0.4137931034482759,
   0.72,
   0.3859649122807018,
   0.7415730337078651,
   0.8282828282828283,
   0.5970149253731343,
   0.42424242424242425,
   0.6666666666666666,
   0.7234042553191491,
   0.6000000000000001,
   0.6153846153846153,
   0.5365853658536585,
   0.7500000000000001,
   0.4210526315789474,
   0.45454545454545453,
   0.7472527472527473,
   0.7,
   0.3225806451612903,
   0.5866666666666667,
   0.6333333333333333,
   0.5964912280701755,
   0.6739130434782609,
   0.7294117647058824,
   0.6857142857142857,
   0.417910447761194,
   0.4528301886792453,
   0.4307692307692308,
   0.7407407407407408,
   0.4489795918367347,
   0.41025641025641024,
   0.4675324675324676,
   0.9534883720930233,
   0.72,
   0.490566037735849,
   0.7142857142857143,
   0.7323943661971832,
   0.7526881720430108,
   0.35000000000000003,
   0.23333333333333336,
   0.5970149253731343,
   0.42857142857142855,
   0.49056603773584906,
   0.7037037037037037,
   0.6756756756756758,
   0.6521739130434783,
   0.7466666666666666,
   0.5116279069767442,
   0.7671232876712328,
   0.5818181818181818,
   0.5454545454545455,
   0.5306122448979591,
   0.6153846153846154,
   0.9166666666666666,
   0.576923076923077,
   0.5666666666666667,
   0.5476190476190477,
   0.634920634920635,
   0.7555555555555556,
   0.5423728813559322,
   0.5263157894736841,
   0.5833333333333333,
   0.796116504854369,
   0.4,
   0.5084745762711865,
   0.6666666666666666,
   0.7692307692307693,
   0.7659574468085106,
   0.6111111111111112,
   0.34782608695652173,
   0.7241379310344828,
   0.4897959183673469,
   0.5176470588235293,
   0.5084745762711865,
   0.5806451612903226,
   0.7628865979381443,
   0.6024096385542168,
   0.509090909090909,
   0.634920634920635,
   0.5434782608695652,
   0.7012987012987012,
   0.547945205479452,
   0.5434782608695652,
   0.29787234042553196,
   0.6933333333333334,
   0.47457627118644063,
   0.5483870967741935,
   0.7272727272727273,
   0.5783132530120482,
   0.4000000000000001,
   0.676923076923077,
   0.46428571428571425,
   0.7529411764705882,
   0.8571428571428572,
   0.5373134328358209,
   0.6,
   0.7678571428571429,
   0.3636363636363636,
   0.4444444444444445,
   0.56,
   0.36363636363636365,
   0.6250000000000001,
   0.5263157894736842,
   0.8705882352941177,
   0.7547169811320756,
   0.5365853658536586,
   0.735294117647059,
   0.6933333333333334,
   0.7441860465116279,
   0.7951807228915663,
   0.6823529411764706,
   0.5853658536585366,
   0.5454545454545455,
   0.6415094339622641,
   0.7789473684210527,
   0.5777777777777778,
   0.6666666666666666,
   0.8214285714285715,
   0.9714285714285714,
   0.576923076923077,
   0.6181818181818182,
   0.8484848484848484,
   0.49122807017543857,
   0.4827586206896552,
   0.7692307692307693,
   0.56,
   0.4,
   1.0,
   0.6666666666666667,
   0.717948717948718,
   0.4444444444444445,
   0.6206896551724137,
   0.7142857142857143,
   0.625,
   0.6,
   0.8,
   0.3333333333333333,
   0.8125,
   0.5625,
   0.6571428571428571,
   0.7234042553191491,
   0.5531914893617023,
   0.6363636363636364,
   0.43243243243243246,
   0.75,
   0.6486486486486486,
   0.8333333333333333,
   0.8571428571428571,
   0.9285714285714286,
   0.875,
   0.56,
   0.4848484848484848,
   0.3636363636363636,
   0.46808510638297873,
   0.7692307692307692,
   0.5714285714285713,
   0.48000000000000004,
   0.31746031746031744,
   0.5263157894736842,
   0.625,
   0.6470588235294117,
   0.4666666666666666,
   0.6976744186046512,
   0.46808510638297873,
   0.6956521739130435,
   0.823529411764706,
   0.5945945945945945,
   0.5,
   0.42857142857142855,
   0.6250000000000001,
   0.41025641025641024,
   0.5714285714285715,
   0.6363636363636364,
   0.5384615384615385,
   0.7804878048780488,
   0.8571428571428572,
   0.9259259259259259,
   0.28571428571428575,
   0.5853658536585366,
   0.5641025641025642,
   0.8771929824561403,
   0.6222222222222223,
   0.7777777777777777,
   0.25,
   0.9090909090909091,
   0.6086956521739131,
   0.5333333333333333,
   0.6500000000000001,
   0.6545454545454547,
   0.65,
   0.7857142857142856,
   0.7894736842105263,
   0.8888888888888888,
   0.5,
   0.8648648648648648,
   0.5853658536585366,
   0.8400000000000001,
   0.7619047619047619,
   0.8000000000000002,
   0.65,
   0.8181818181818182,
   0.5294117647058824,
   ...]],
 0.8: [205,
  [0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.375,
   0.6666666666666666,
   0.5714285714285715,
   0.4444444444444444,
   0.6666666666666666,
   0.20000000000000004,
   0.5333333333333333,
   0.3636363636363636,
   0.3225806451612903,
   0.29629629629629634,
   0.21621621621621623,
   0.6,
   0.20689655172413793,
   0.6666666666666665,
   0.3684210526315789,
   0.3703703703703704,
   0.36363636363636365,
   0.3333333333333333,
   0.16666666666666666,
   0.3050847457627119,
   0.25,
   0.17142857142857143,
   0.2153846153846154,
   0.32727272727272727,
   0.2545454545454545,
   0.339622641509434,
   0.1904761904761905,
   0.4,
   0.2,
   0.2222222222222222,
   0.3125,
   0.13333333333333333,
   0.5,
   0.3829787234042554,
   0.3255813953488372,
   0.29166666666666663,
   0.3684210526315789,
   0.375,
   0.5882352941176471,
   0.358974358974359,
   0.48648648648648646,
   0.6521739130434783,
   0.6111111111111112,
   0.5909090909090909,
   0.75,
   0.5,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.4444444444444445,
   0.6,
   0.5714285714285715,
   0.3529411764705882,
   0.6250000000000001,
   0.5714285714285715,
   0.5333333333333333,
   0.5714285714285715,
   0.4210526315789474,
   0.36363636363636365,
   0.5714285714285715,
   0.6666666666666665,
   0.5,
   0.75,
   0.6666666666666666,
   0.7142857142857143,
   0.5714285714285715,
   0.5,
   0.5714285714285715,
   0.6,
   0.6666666666666666,
   0.3333333333333333,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.6,
   0.5,
   0.6153846153846153,
   0.6,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.5714285714285715,
   0.35294117647058826,
   0.5,
   0.4444444444444445,
   0.37499999999999994,
   0.6,
   0.28571428571428564,
   0.4,
   0.5,
   0.4,
   0.4000000000000001,
   0.23076923076923078,
   0.3636363636363636,
   0.14285714285714288,
   0.625,
   0.30769230769230765,
   0.2857142857142857,
   0.625,
   0.6666666666666666,
   0.33333333333333326,
   0.5,
   0.2727272727272727,
   0.48484848484848486,
   0.6666666666666665,
   0.4444444444444445,
   0.3703703703703704,
   0.37499999999999994,
   0.6153846153846153,
   0.25,
   0.1875,
   0.41379310344827586,
   0.3333333333333333,
   0.3636363636363637,
   0.3,
   0.41379310344827586,
   0.2,
   0.3571428571428571,
   0.46153846153846156,
   0.5714285714285715,
   0.4666666666666667,
   0.35714285714285715,
   0.36363636363636365,
   0.47058823529411764,
   0.47058823529411764,
   0.5454545454545454,
   0.7450980392156864,
   0.7272727272727273,
   0.5925925925925926,
   0.5,
   0.4210526315789474,
   0.6666666666666665,
   0.23076923076923078,
   0.5,
   0.3888888888888889,
   0.5333333333333332,
   0.3255813953488372,
   0.23529411764705882,
   0.4814814814814815,
   0.7407407407407408,
   0.5531914893617023,
   0.4680851063829788,
   0.5,
   0.39024390243902435,
   0.6938775510204083,
   0.3448275862068966,
   0.5555555555555556,
   0.7142857142857142,
   0.5714285714285714,
   0.35,
   0.5454545454545455,
   0.5777777777777778,
   0.4,
   0.6190476190476191,
   0.6666666666666666,
   0.34285714285714286,
   0.7058823529411765,
   0.6086956521739131,
   0.29411764705882354,
   0.7500000000000001,
   0.3404255319148936,
   0.46511627906976744,
   0.37499999999999994,
   0.5142857142857143,
   0.625,
   0.3902439024390244,
   0.7741935483870969,
   0.6818181818181818,
   0.3529411764705882,
   0.39999999999999997,
   0.35897435897435903,
   0.5454545454545454,
   0.43749999999999994,
   0.5625,
   0.25925925925925924,
   0.43243243243243246,
   0.5625,
   0.5416666666666667,
   0.7368421052631577,
   0.33333333333333337,
   0.6315789473684211,
   0.5454545454545454,
   0.3,
   0.5161290322580646,
   0.3728813559322034,
   0.43749999999999994,
   0.7894736842105263,
   0.7333333333333334,
   0.7741935483870968,
   0.34146341463414637,
   0.5185185185185186,
   0.6666666666666666,
   0.5405405405405405,
   0.39999999999999997,
   0.6896551724137931,
   0.41025641025641024,
   0.3714285714285715]],
 0.7: [6,
  [0.75,
   0.14634146341463417,
   0.6666666666666666,
   0.375,
   0.42857142857142855,
   0.42857142857142855]],
 1: [258,
  [0.8333333333333334,
   0.6,
   0.6666666666666666,
   0.4210526315789474,
   0.4444444444444445,
   0.6666666666666666,
   0.4666666666666667,
   0.3,
   0.36363636363636365,
   0.2,
   0.3157894736842105,
   0.6,
   0.35714285714285715,
   0.2962962962962963,
   0.3846153846153846,
   0.15384615384615383,
   0.35294117647058826,
   0.20689655172413793,
   0.14285714285714285,
   0.21739130434782608,
   0.10526315789473684,
   0.2790697674418605,
   0.2745098039215686,
   0.2127659574468085,
   0.25,
   0.23076923076923078,
   0.2790697674418605,
   0.1951219512195122,
   0.27777777777777773,
   0.2926829268292683,
   0.2857142857142857,
   0.09302325581395349,
   0.3829787234042554,
   0.3636363636363636,
   0.39024390243902435,
   0.5405405405405405,
   0.5128205128205129,
   0.2222222222222222,
   0.42424242424242425,
   0.25,
   0.6470588235294117,
   0.4,
   0.5217391304347826,
   0.358974358974359,
   0.372093023255814,
   0.6666666666666666,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6666666666666666,
   0.5,
   0.5,
   0.4,
   0.5714285714285715,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.5882352941176471,
   0.4705882352941177,
   0.6666666666666666,
   0.6666666666666666,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.6153846153846153,
   0.5714285714285715,
   0.4,
   0.42857142857142855,
   0.6666666666666666,
   0.4615384615384615,
   0.47619047619047616,
   0.6666666666666666,
   0.5,
   0.37499999999999994,
   0.4444444444444444,
   0.42857142857142855,
   0.5333333333333333,
   0.4444444444444444,
   0.4166666666666667,
   0.47058823529411764,
   0.4761904761904762,
   0.35714285714285715,
   0.2758620689655172,
   0.5555555555555556,
   0.33333333333333326,
   0.36363636363636365,
   0.16,
   0.5,
   0.47058823529411764,
   0.375,
   0.0909090909090909,
   0.33333333333333326,
   0.375,
   0.34782608695652173,
   0.2222222222222222,
   0.23076923076923075,
   0.25,
   0.3076923076923077,
   0.22857142857142854,
   0.35714285714285715,
   0.5517241379310345,
   0.6666666666666666,
   0.2,
   0.18181818181818182,
   0.5,
   0.4000000000000001,
   0.1702127659574468,
   0.35294117647058826,
   0.6875,
   0.6,
   0.4210526315789474,
   0.47058823529411764,
   0.7142857142857143,
   0.6363636363636365,
   0.3157894736842105,
   0.8461538461538461,
   0.7142857142857143,
   0.8000000000000002,
   0.5,
   0.8648648648648649,
   0.6666666666666666,
   0.5454545454545455,
   0.6428571428571429,
   0.6,
   0.3404255319148936,
   0.3333333333333333,
   0.5483870967741935,
   0.617283950617284,
   0.4888888888888888,
   0.3636363636363636,
   0.4523809523809524,
   0.6666666666666666,
   0.5964912280701754,
   0.42857142857142855,
   0.3404255319148936,
   0.4,
   0.4197530864197531,
   0.8461538461538461,
   0.45714285714285713,
   0.24615384615384617,
   0.4444444444444444,
   0.5405405405405405,
   0.5925925925925926,
   0.48484848484848486,
   0.4,
   0.358974358974359,
   0.6111111111111113,
   0.41666666666666663,
   0.4666666666666667,
   0.48000000000000004,
   0.5,
   0.35714285714285715,
   0.6,
   0.45,
   0.4375,
   0.6428571428571429,
   0.49056603773584906,
   0.31818181818181823,
   0.4888888888888889,
   0.6857142857142857,
   0.4516129032258065,
   0.6923076923076924,
   0.7741935483870968,
   0.5862068965517241,
   0.47058823529411764,
   0.47368421052631576,
   0.5806451612903225,
   0.76,
   0.5625000000000001,
   0.4255319148936171,
   0.3333333333333333,
   0.28571428571428575,
   0.375,
   0.6376811594202899,
   0.4878048780487805,
   0.7857142857142857,
   0.5925925925925927,
   0.5116279069767442,
   0.4090909090909091,
   0.3902439024390244,
   0.6666666666666666,
   0.5652173913043478,
   0.5714285714285713,
   0.5384615384615384,
   0.3636363636363636,
   0.6666666666666667,
   0.75,
   0.5128205128205129,
   0.6206896551724139,
   0.4827586206896552,
   0.4782608695652174,
   0.5,
   0.5263157894736842,
   0.4583333333333333,
   0.4897959183673469,
   0.875,
   0.4736842105263158,
   0.46511627906976744,
   0.5833333333333334,
   0.43902439024390244,
   0.6666666666666666,
   0.358974358974359,
   0.3448275862068966,
   0.606060606060606,
   0.42857142857142855,
   0.3636363636363636,
   0.6666666666666666,
   0.3428571428571428,
   0.425531914893617,
   0.5,
   0.3902439024390244,
   0.4117647058823529,
   0.2285714285714286,
   0.85,
   0.5500000000000002,
   0.3829787234042554,
   0.5652173913043479,
   0.3888888888888889,
   0.43478260869565216,
   0.3636363636363636,
   0.409090909090909,
   0.3888888888888889,
   0.5925925925925926,
   0.45454545454545453,
   0.358974358974359,
   0.358974358974359,
   0.52,
   0.5625000000000001,
   0.3,
   0.22727272727272727,
   0.40816326530612246,
   0.9090909090909091,
   0.8636363636363636,
   0.6976744186046512,
   0.7692307692307692,
   0.7857142857142856,
   0.6206896551724138,
   0.4242424242424242,
   0.4242424242424242,
   0.7857142857142857,
   0.6274509803921569,
   0.6666666666666666,
   0.46808510638297873,
   0.5,
   0.6285714285714287,
   0.6315789473684211,
   0.7222222222222222,
   0.48484848484848486,
   0.6875000000000001,
   0.358974358974359,
   0.4324324324324324,
   0.42857142857142855,
   0.46511627906976744,
   0.5945945945945946,
   0.4666666666666667,
   0.5762711864406779,
   0.7199999999999999]],
 0.6: [160,
  [0.5,
   0.6666666666666666,
   0.5,
   0.6,
   0.5714285714285715,
   0.380952380952381,
   0.5714285714285715,
   0.47058823529411764,
   0.5,
   0.34782608695652173,
   0.28571428571428575,
   0.5263157894736842,
   0.1,
   0.25,
   0.5,
   0.5555555555555556,
   0.28571428571428575,
   0.2758620689655172,
   0.22222222222222224,
   0.23529411764705882,
   0.25,
   0.13793103448275862,
   0.26666666666666666,
   0.2,
   0.28571428571428575,
   0.17391304347826086,
   0.13953488372093023,
   0.3714285714285714,
   0.1081081081081081,
   0.21052631578947367,
   0.21818181818181817,
   0.21538461538461542,
   0.13043478260869565,
   0.10714285714285714,
   0.1702127659574468,
   0.0930232558139535,
   0.2647058823529412,
   0.42553191489361697,
   0.1818181818181818,
   0.21052631578947367,
   0.24137931034482757,
   0.2608695652173913,
   0.18518518518518517,
   0.5714285714285714,
   0.5625000000000001,
   0.39999999999999997,
   0.43902439024390244,
   0.38888888888888884,
   0.1904761904761905,
   0.75,
   0.6,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.625,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.5714285714285715,
   0.42857142857142855,
   0.3333333333333333,
   0.42857142857142855,
   0.6666666666666666,
   0.37499999999999994,
   0.5,
   0.5714285714285715,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.2857142857142857,
   0.5,
   0.17647058823529413,
   0.1904761904761905,
   0.6,
   0.22727272727272727,
   0.21428571428571427,
   0.22222222222222224,
   0.20000000000000004,
   0.6666666666666666,
   0.45454545454545453,
   0.3703703703703704,
   0.27027027027027023,
   0.5,
   0.08695652173913043,
   0.2105263157894737,
   0.38709677419354843,
   0.14634146341463414,
   0.29629629629629634,
   0.37499999999999994,
   0.24242424242424243,
   0.23076923076923075,
   0.6666666666666666,
   0.3333333333333333,
   0.2,
   0.35714285714285715,
   0.5,
   0.33333333333333337,
   0.5714285714285715,
   0.3157894736842105,
   0.46153846153846156,
   0.32653061224489793,
   0.7142857142857142,
   0.31249999999999994,
   0.5652173913043478,
   0.6666666666666666,
   0.4090909090909091,
   0.35714285714285715,
   0.16666666666666666,
   0.64,
   0.33333333333333337,
   0.6829268292682927,
   0.7500000000000001,
   0.5,
   0.2857142857142857,
   0.3636363636363636,
   0.6315789473684211,
   0.5625000000000001,
   0.6666666666666667,
   0.6451612903225806,
   0.28571428571428575,
   0.5555555555555556,
   0.3225806451612903,
   0.37837837837837834,
   0.2580645161290323,
   0.5263157894736842,
   0.4489795918367347,
   0.2727272727272727,
   0.6829268292682927,
   0.851063829787234,
   0.3783783783783784,
   0.7916666666666667,
   0.42857142857142855,
   0.3255813953488372,
   0.2926829268292683,
   0.4137931034482759,
   0.42857142857142855,
   0.2857142857142857,
   0.6341463414634146,
   0.6428571428571429,
   0.26666666666666666,
   0.47058823529411764,
   0.45,
   0.5777777777777777,
   0.4444444444444444,
   0.30769230769230765,
   0.39999999999999997,
   0.6428571428571429,
   0.6829268292682927,
   0.7272727272727272,
   0.6875,
   0.4,
   0.7142857142857143,
   0.358974358974359,
   0.6111111111111113,
   0.6000000000000001,
   0.3846153846153846,
   0.4615384615384615,
   0.35,
   0.4615384615384615,
   0.4736842105263158]],
 0.3: [23,
  [0.5,
   0.4,
   0.5,
   0.42857142857142855,
   0.6666666666666666,
   0.13333333333333333,
   0.5,
   0.28571428571428575,
   0.6666666666666666,
   0.3333333333333333,
   0.6153846153846153,
   0.42857142857142855,
   0.6,
   0.6,
   0.5,
   0.5714285714285714,
   0.5,
   0.375,
   0.25,
   0.5,
   0.375,
   0.5,
   0.3829787234042554]],
 0.5: [30,
  [0.5263157894736842,
   0.5,
   0.6666666666666666,
   0.5,
   0.6,
   0.6666666666666666,
   0.75,
   0.75,
   0.75,
   0.6153846153846153,
   0.39999999999999997,
   0.5384615384615384,
   0.42857142857142855,
   0.5454545454545454,
   0.3333333333333333,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.5714285714285715,
   0.5,
   0.5,
   0.5714285714285715,
   0.6,
   0.5,
   0.4615384615384615,
   0.5555555555555556,
   0.3636363636363636,
   0.2,
   0.4814814814814815]],
 0.4: [191,
  [0.42857142857142855,
   0.4,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6153846153846153,
   0.375,
   0.28571428571428575,
   0.2,
   0.4444444444444445,
   0.5555555555555556,
   0.3448275862068965,
   0.36363636363636365,
   0.3243243243243243,
   0.34782608695652173,
   0.24242424242424246,
   0.20512820512820512,
   0.1379310344827586,
   0.3636363636363637,
   0.25,
   0.34285714285714286,
   0.33333333333333337,
   0.10526315789473685,
   0.29629629629629634,
   0.3,
   0.3,
   0.11320754716981132,
   0.22727272727272724,
   0.509090909090909,
   0.1904761904761905,
   0.22222222222222224,
   0.25,
   0.23809523809523808,
   0.22580645161290322,
   0.2,
   0.16,
   0.27906976744186046,
   0.19512195121951217,
   0.27027027027027023,
   0.1923076923076923,
   0.3673469387755102,
   0.04761904761904762,
   0.2285714285714286,
   0.3333333333333333,
   0.43749999999999994,
   0.5,
   0.3636363636363636,
   0.1764705882352941,
   0.4864864864864865,
   0.5,
   0.4680851063829788,
   0.6470588235294118,
   0.5652173913043479,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.26666666666666666,
   0.6666666666666666,
   0.6,
   0.5,
   0.5333333333333333,
   0.6666666666666666,
   0.4210526315789474,
   0.375,
   0.42857142857142855,
   0.5,
   0.2857142857142857,
   0.5882352941176471,
   0.37499999999999994,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6666666666666666,
   0.5714285714285715,
   0.5714285714285715,
   0.5714285714285715,
   0.5,
   0.3333333333333333,
   0.5,
   0.4,
   0.6666666666666666,
   0.4444444444444444,
   0.4705882352941177,
   0.6666666666666666,
   0.375,
   0.6666666666666666,
   0.5,
   0.28571428571428575,
   0.2857142857142857,
   0.5,
   0.3703703703703703,
   0.48000000000000004,
   0.42857142857142855,
   0.39999999999999997,
   0.30303030303030304,
   0.29411764705882354,
   0.3076923076923077,
   0.28571428571428575,
   0.25,
   0.47619047619047616,
   0.33333333333333326,
   0.26666666666666666,
   0.3,
   0.25,
   0.47058823529411764,
   0.4444444444444445,
   0.625,
   0.3,
   0.3636363636363637,
   0.18749999999999997,
   0.3333333333333333,
   0.26666666666666666,
   0.45454545454545453,
   0.22222222222222224,
   0.2727272727272727,
   0.30769230769230765,
   0.3,
   0.5714285714285714,
   0.24390243902439024,
   0.2,
   0.5806451612903225,
   0.14814814814814817,
   0.2857142857142857,
   0.3333333333333333,
   0.2380952380952381,
   0.5714285714285715,
   0.7407407407407408,
   0.75,
   0.5714285714285714,
   0.3333333333333333,
   0.4680851063829787,
   0.8571428571428571,
   0.31250000000000006,
   0.5,
   0.3404255319148936,
   0.3902439024390244,
   0.4477611940298507,
   0.358974358974359,
   0.2727272727272727,
   0.5128205128205129,
   0.30769230769230765,
   0.33333333333333326,
   0.711111111111111,
   0.4090909090909091,
   0.22857142857142856,
   0.14814814814814814,
   0.35,
   0.35000000000000003,
   0.380952380952381,
   0.5555555555555556,
   0.8275862068965518,
   0.3829787234042554,
   0.34285714285714286,
   0.45,
   0.34782608695652173,
   0.4324324324324324,
   0.5789473684210527,
   0.45161290322580644,
   0.4864864864864865,
   0.48000000000000004,
   0.43750000000000006,
   0.3684210526315789,
   0.48484848484848486,
   0.27586206896551724,
   0.47619047619047616,
   0.5384615384615384,
   0.3636363636363636,
   0.42857142857142855,
   0.3243243243243243,
   0.3243243243243243,
   0.43750000000000006,
   0.45714285714285713,
   0.6428571428571429,
   0.7647058823529411,
   0.4444444444444445,
   0.3913043478260869,
   0.42857142857142855,
   0.4444444444444444,
   0.3571428571428571,
   0.5517241379310345,
   0.35294117647058826,
   0.5405405405405405,
   0.5806451612903226,
   0.37735849056603776,
   0.5,
   0.3414634146341463]],
 0.2: [104,
  [0.5714285714285715,
   0.6,
   0.6,
   0.5714285714285715,
   0.25,
   0.3636363636363636,
   0.25,
   0.22222222222222224,
   0.15384615384615383,
   0.23529411764705885,
   0.18749999999999997,
   0.3,
   0.13793103448275862,
   0.28571428571428575,
   0.16666666666666666,
   0.1818181818181818,
   0.3846153846153846,
   0.17543859649122806,
   0.18867924528301885,
   0.35000000000000003,
   0.13333333333333333,
   0.13043478260869565,
   0.2,
   0.3225806451612903,
   0.27027027027027023,
   0.24000000000000002,
   0.13636363636363638,
   0.16666666666666666,
   0.23529411764705882,
   0.27027027027027023,
   0.2191780821917808,
   0.20408163265306123,
   0.41025641025641024,
   0.3571428571428571,
   0.37209302325581395,
   0.39999999999999997,
   0.4666666666666667,
   0.5,
   0.5,
   0.6666666666666666,
   0.30769230769230765,
   0.4,
   0.42857142857142855,
   0.3333333333333333,
   0.42857142857142855,
   0.3157894736842105,
   0.37499999999999994,
   0.75,
   0.5,
   0.5,
   0.6666666666666666,
   0.5714285714285715,
   0.5,
   0.5714285714285715,
   0.37499999999999994,
   0.375,
   0.20000000000000004,
   0.16666666666666666,
   0.4210526315789474,
   0.22222222222222224,
   0.2758620689655172,
   0.33333333333333337,
   0.20689655172413793,
   0.07142857142857144,
   0.5,
   0.24999999999999994,
   0.37499999999999994,
   0.22222222222222224,
   0.3636363636363636,
   0.22857142857142854,
   0.48,
   0.5333333333333333,
   0.2608695652173913,
   0.41025641025641024,
   0.5,
   0.4390243902439024,
   0.4666666666666667,
   0.3414634146341463,
   0.14814814814814814,
   0.3870967741935483,
   0.3333333333333333,
   0.25641025641025644,
   0.5853658536585366,
   0.411764705882353,
   0.7199999999999999,
   0.16,
   0.3870967741935484,
   0.3225806451612903,
   0.4,
   0.5581395348837209,
   0.13333333333333333,
   0.4864864864864865,
   0.5217391304347826,
   0.5306122448979592,
   0.4074074074074074,
   0.7647058823529412,
   0.3,
   0.39999999999999997,
   0.22857142857142856,
   0.47058823529411764,
   0.3333333333333333,
   0.1904761904761905,
   0.3888888888888889,
   0.4081632653061225]],
 0.9: [6,
  [0.5714285714285715,
   0.5,
   0.6666666666666666,
   0.4666666666666667,
   0.4666666666666667,
   0.3555555555555555]]}

In [54]: def get_key(i):
    ...:     for ind in [0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1.0]:
    ...:         if i <= ind:
    ...:             return ind
    ...: 

In [55]: 

In [55]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     print(k)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(smatch_scores[ind])
    ...: 
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.7
None
None
None
None
1.0
None
None
None
1.0
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
0.3
0.1
None
None
0.5
None
None
None
0.3
None
0.6
0.8
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
1.0
None
0.1
0.4
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
0.6
0.1
0.1
None
0.1
0.2
None
None
0.1
None
None
None
None
0.5
0.3
0.1
0.1
0.5
0.1
0.6
None
None
0.1
0.1
1.0
0.1
None
0.4
None
None
0.1
0.1
1.0
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
None
None
0.8
None
None
None
0.9
None
None
None
None
0.1
None
None
0.8
None
None
None
None
1.0
None
0.2
None
None
0.8
None
0.4
None
None
None
None
None
None
0.8
0.1
None
None
0.1
0.1
0.1
0.5
0.5
0.4
0.8
None
None
None
0.5
0.4
None
None
0.4
0.6
0.8
None
0.4
None
None
None
0.2
None
None
None
None
0.1
None
0.1
0.1
None
0.1
0.1
None
None
None
None
None
None
0.1
0.8
None
0.1
0.6
0.1
0.1
0.1
None
None
0.1
None
0.1
None
None
None
None
0.4
None
None
None
0.1
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.8
None
None
None
None
0.1
None
None
0.4
0.1
None
None
0.1
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
0.8
None
None
0.1
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
0.4
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.2
None
None
0.6
None
0.1
None
None
None
None
0.2
None
None
None
0.4
None
None
None
None
1.0
None
None
0.1
None
0.6
0.1
None
None
None
None
0.8
0.8
1.0
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
None
0.8
0.1
0.1
None
0.8
None
0.1
0.8
None
None
None
None
None
None
None
0.2
1.0
0.4
0.4
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.4
1.0
None
None
None
None
1.0
None
None
None
None
0.4
None
0.4
0.1
None
None
0.4
None
None
None
None
0.1
None
None
0.2
None
None
0.4
None
None
0.2
None
None
None
None
None
None
0.8
0.6
None
None
0.1
0.6
None
None
0.6
None
0.6
None
None
0.2
0.6
0.8
None
0.1
None
None
None
None
1.0
None
0.4
0.8
0.4
0.1
None
None
None
None
None
0.2
1.0
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
0.6
1.0
0.6
0.8
None
1.0
0.2
0.6
None
0.2
0.2
0.1
0.1
None
0.1
0.4
0.4
None
None
None
None
None
None
0.8
0.8
1.0
None
1.0
None
None
0.1
0.6
0.1
None
None
None
None
None
0.1
0.1
None
0.1
None
None
0.1
None
0.1
None
0.1
0.6
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
1.0
None
0.6
None
0.4
None
None
0.6
None
None
None
0.6
None
None
1.0
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
1.0
None
1.0
None
None
None
0.4
0.1
0.1
None
None
0.6
None
None
0.6
None
None
1.0
None
None
0.2
0.2
None
0.1
None
1.0
None
None
0.1
None
None
None
None
1.0
None
0.6
0.1
0.1
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
0.6
0.1
None
0.8
0.2
1.0
None
0.6
None
None
None
None
None
None
None
None
None
None
0.1
0.2
0.8
0.1
None
0.2
None
0.1
0.6
0.1
None
None
None
0.4
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
0.8
None
None
0.7
None
0.4
None
None
None
None
None
None
None
None
None
None
0.1
0.6
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.2
0.6
None
None
None
0.1
1.0
0.4
0.8
None
None
None
None
None
None
None
None
0.8
None
0.6
None
None
0.1
None
0.4
0.6
1.0
None
None
None
None
None
None
None
0.6
0.1
0.4
0.4
None
0.6
0.1
None
None
None
None
0.2
None
0.6
None
0.1
0.1
0.1
0.1
None
0.1
0.4
0.1
None
0.8
0.4
None
None
0.6
None
None
None
0.8
0.1
None
None
None
None
None
0.1
0.6
None
0.4
0.2
0.1
None
0.1
0.6
0.8
0.2
None
None
0.2
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
None
0.2
None
0.1
0.1
None
0.1
None
0.4
None
0.1
None
None
None
None
None
0.1
None
0.4
0.1
0.2
None
None
1.0
0.6
1.0
None
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
None
None
0.8
None
0.1
None
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.4
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
None
None
None
1.0
None
None
0.1
None
0.4
None
0.6
None
0.1
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
0.1
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
0.1
0.2
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.4
None
None
None
None
1.0
None
None
None
None
None
None
0.1
0.1
None
None
0.2
None
0.1
0.4
None
0.8
0.4
None
None
None
None
1.0
1.0
None
0.4
0.2
0.1
0.1
0.1
0.6
0.6
None
0.1
0.8
None
None
None
None
1.0
None
None
None
None
0.4
0.1
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
0.1
0.1
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.7
None
None
None
None
None
None
None
None
None
None
1.0
1.0
0.6
0.4
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
0.5
None
None
None
None
None
None
None
None
0.1
0.1
0.3
None
None
0.8
None
None
None
0.2
0.8
None
None
0.4
0.8
None
None
None
None
0.1
1.0
0.1
None
0.4
0.4
0.6
None
0.4
0.4
0.4
None
0.6
0.8
None
None
0.6
0.6
0.1
None
None
None
None
0.6
0.4
None
None
None
None
None
0.2
0.4
None
None
0.6
None
None
None
None
None
0.4
None
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
0.5
0.1
0.1
0.8
0.9
None
0.4
None
None
0.8
0.1
0.1
None
None
None
None
None
None
None
None
0.1
0.3
None
None
0.1
None
None
None
None
None
None
1.0
None
None
None
0.1
0.1
None
None
0.2
None
None
0.1
None
0.1
None
None
None
None
0.9
0.1
None
None
None
0.2
None
None
None
0.4
0.1
0.1
0.1
0.2
0.1
0.1
None
None
None
None
None
0.4
0.1
0.4
0.6
1.0
None
None
None
None
0.1
0.1
0.1
0.4
0.4
None
None
0.8
0.2
0.1
0.1
None
0.8
0.1
0.3
0.5
None
None
None
0.4
0.1
1.0
0.8
0.1
None
None
None
None
None
None
None
None
None
None
0.2
1.0
0.4
None
0.1
None
None
None
0.1
0.1
None
None
None
None
0.8
0.8
None
None
0.1
0.1
0.1
None
None
None
0.8
None
None
None
None
0.8
0.1
0.1
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
0.1
0.5
0.1
1.0
None
0.1
None
None
0.1
0.1
None
None
None
None
None
0.1
1.0
None
None
None
0.1
0.1
0.1
0.1
None
0.7
0.1
None
None
None
0.1
0.2
0.5
0.1
None
0.1
1.0
0.1
0.1
0.1
None
None
0.6
0.3
None
None
None
None
0.8
None
None
None
None
0.1
None
None
None
0.2
0.1
0.1
0.8
0.1
0.1
0.1
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.5
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.1
None
None
0.1
1.0
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.3
None
None
None
None
None
None
1.0
None
0.4
None
None
None
1.0
None
None
None
None
None
None
0.5
None
None
1.0
None
None
0.4
0.4
None
None
0.3
0.3
0.3
None
None
0.1
None
None
None
None
None
0.8
None
None
None
0.8
None
0.1
0.7
None
None
0.4
None
None
0.8
0.8
0.8
0.8
1.0
0.8
None
None
None
None
None
None
0.3
None
None
0.8
0.8
0.8
0.3
None
None
0.5
0.1
0.5
0.6
None
None
None
None
None
0.1
None
0.1
None
0.1
0.4
0.1
None
None
0.1
None
1.0
0.1
None
None
0.3
0.4
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.2
None
0.8
0.8
0.8
0.3
None
None
None
None
None
None
None
0.4
None
0.4
None
None
0.5
0.5
None
None
None
None
None
None
0.8
0.3
0.8
None
0.8
0.1
None
None
0.1
0.3
0.1
None
None
0.4
0.8
None
None
None
0.2
0.2
0.5
0.1
None
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
0.5
None
0.1
0.1
0.1
1.0
None
0.6
None
0.5
None
None
None
0.1
0.8
0.8
0.4
0.1
0.1
0.1
0.4
0.1
None
0.3
0.1
0.5
0.1
None
0.8
None
0.1
None
None
0.1
None
0.8
0.5
None
None
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
1.0
None
None
None
None
1.0
0.1
0.1
None
0.4
0.4
None
0.1
0.1
0.1
0.1
0.4
1.0
0.3
None
0.2
1.0
0.4
0.1
0.1
None
0.8
None
None
None
0.1
None
0.1
0.1
0.1
None
None
0.6
0.1
None
0.4
0.4
None
None
0.1
0.8
0.1
0.1
0.8
None
0.1
None
0.3
None
0.7
None
0.4
None
None
1.0
None
0.4
0.1
0.3
None
None
None
None
None
0.2
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.8
1.0
None
None
None
None
0.1
0.6
1.0
0.1
0.1
1.0
0.1
None
0.1
None
0.1
0.8
0.1
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.6
None
None
None
0.6
0.1
None
None
0.1
None
None
None
None
1.0
None
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.8
0.6
0.1
None
None
None
0.2
None
None
None
None
0.4
0.6
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
None
None
0.1
None
1.0
None
None
None
None
0.1
None
None
None
None
0.1
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
None
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
None
None
None
None
None
0.6
None
0.1
0.8
None
0.2
None
0.1
0.2
None
None
0.1
None
None
None
0.4
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.4
0.4
0.1
None
None
None
None
None
None
None
None
1.0
None
None
0.1
None
0.4
None
0.1
None
None
0.4
None
0.4
None
0.1
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
1.0
None
0.1
None
0.1
None
None
0.8
None
None
None
None
None
None
0.1
None
0.1
None
None
None
0.4
None
None
None
None
None
None
None
1.0
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
1.0
0.1
0.8
0.1
0.1
0.1
None
None
None
None
1.0
None
None
None
0.8
0.8
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
0.4
None
1.0
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
0.4
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
None
None
None
0.1
None
None
None
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.1
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.8
None
None
None
None
None
0.4
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.6
None
0.4
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
0.4
0.1
None
0.1
None
None
0.6
0.6
None
None
0.6
None
0.1
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
None
None
None
None
None
0.6
None
None
0.1
None
None
None
None
None
None
0.1
None
None
0.1
1.0
None
0.1
None
None
0.2
None
0.8
0.8
None
None
None
None
1.0
None
None
None
None
None
None
0.4
None
None
None
None
0.2
0.1
0.2
None
None
None
None
None
0.5
None
None
None
None
None
0.8
None
None
0.1
None
None
None
None
None
0.1
0.4
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
0.8
None
0.1
None
None
None
None
None
0.4
None
None
0.1
0.1
None
None
None
None
None
None
0.4
None
0.4
None
0.1
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
1.0
None
0.1
None
None
0.1
0.1
None
0.1
None
0.1
None
None
0.8
None
None
None
0.1
None
0.1
None
0.1
None
None
None
0.1
None
0.8
None
None
0.4
1.0
1.0
None
None
None
None
0.1
0.6
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
0.1
0.1
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
0.1
None
None
None
None
None
None
None
0.2
None
None
1.0
None
0.1
None
0.1
None
0.1
None
None
0.2
None
None
0.6
0.8
None
None
None
0.6
0.4
None
None
None
None
None
0.1
None
0.6
None
0.4
None
None
0.6
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
1.0
None
0.6
None
0.8
0.4
0.8
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.8
0.4
None
None
None
None
0.1
None
None
None
1.0
None
None
None
None
None
None
None
None
None
0.4
None
0.1
None
0.1
None
0.6
0.4
None
None
None
None
0.1
None
None
None
None
None
None
1.0
None
0.8
0.2
None
None
None
None
1.0
0.1
0.1
None
None
None
None
None
None
None
1.0
1.0
None
None
0.8
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
0.2
0.1
None
None
None
None
0.1
0.1
None
None
None
None
0.5
None
None
None
None
1.0
None
None
None
None
0.4
None
None
1.0
1.0
0.1
None
0.6
None
0.1
0.6
0.1
0.1
None
None
None
None
1.0
None
0.8
None
1.0
0.4
None
None
None
None
0.6
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.1
None
None
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
1.0
0.8
None
0.2
None
1.0
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
1.0
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
1.0
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.1
None
None
None
None
None
None
None
None
None
None
1.0
0.4
1.0
None
None
None
None
0.8
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
0.6
None
0.4
None
None
None
None
0.8
None
0.6
None
None
1.0
0.6
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
None
None
1.0
0.4
None
0.8
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1.0
None
None
0.4
None
None
None
1.0
None
None
None
None
None
0.8
0.2
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.2
1.0
None
None
0.4
0.1
None
None
None
None
0.1
0.1
None
0.6
None
None
1.0
None
None
None
0.8
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.4
1.0
None
None
0.8
None
None
1.0
None
1.0
None
0.6
None
None
0.1
None
None
None
0.1
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.6
None
None
None
None
None
None
1.0
None
0.8
None
None
None
0.8
None
None
None
None
0.6
None
None
None
None
None
0.1
None
None
None
0.8
None
None
None
None
None
0.4
None
0.4
0.2
None
0.8
None
None
None
None
None
None
None
None
1.0
None
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
1.0
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.5
1.0
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.6
1.0
None
None
None
None
0.2
None
0.6
None
None
None
1.0
None
None
None
0.8
None
0.4
0.8
None
None
None
0.4
None
None
None
None
None
None
0.1
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
1.0
0.8
None
None
None
0.8
None
None
None
None
None
0.8
None
None
0.8
0.1
None
None
0.2
None
0.1
None
0.8
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.1
1.0
None
None
None
0.8
None
None
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
0.6
None
0.8
None
0.2
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.6
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.8
None
None
1.0
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
None
1.0
None
None
None
None
None
None
0.6
1.0
None
None
None
None
None
0.4
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
1.0
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.8
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
1.0
None
None
None
1.0
0.2
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
0.8
1.0
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.0
0.1
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
0.6
None
0.6
None
None
0.1
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
None
None
None
1.0
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
1.0
None
0.1
0.8
None
0.8
None
None
0.1
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.1
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
None
0.1
None
0.1
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
0.6
None
None
None
1.0
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
0.1
None
None
1.0
0.4
None
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
0.6
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.4
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
None
0.4
0.4
1.0
None
0.1
0.1
None
None
None
0.4
None
0.1
1.0
1.0
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
0.2
None
1.0
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
0.6
0.4
None
None
None
None
1.0
None
None
0.4
None
0.6
None
None
0.1
0.4
None
0.1
None
None
None
None
None
None
None
None
None
None
None
1.0
0.8
None
0.6
None
None
None
0.6
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
0.4
None
0.8
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
0.1
None
None
1.0
None
None
1.0
0.1
None
None
None
None
None
None
None
None
None
0.8
1.0
0.1
None
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.6
None
None
None
0.4
None
None
None
None
0.8
0.8
1.0
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
None
None
0.1
None
None
0.1
0.2
None
None
None
None
None
None
0.1
None
None
None
0.1
0.2
None
0.2
None
None
0.1
None
0.6
None
None
None
None
None
0.4
None
1.0
None
None
None
None
0.1
None
None
0.2
None
1.0
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.2
None
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
0.1
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
0.4
0.6
None
0.1
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.2
None
None
None
None
0.4
None
None
None
0.2
1.0
None
0.1
0.6
None
1.0
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
0.4
None
0.1
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
0.1
None
1.0
None
None
None
None
1.0
None
1.0
1.0
None
1.0
None
None
0.1
None
0.1
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
1.0
1.0
None
None
None
None
None
1.0
None
1.0
None
None
None
None
0.1
None
None
None
1.0
0.1
None
None
None
None
None
1.0
0.1
None
None
None
None
None
1.0
1.0
None
0.1
None
None
1.0
1.0
None
1.0
1.0
0.1
None
1.0
None
1.0
1.0
1.0
0.1
0.1
None
1.0
None
0.1
0.1
1.0
1.0
1.0
1.0
0.1
0.1
0.1
0.1
1.0
0.1
1.0
0.1
None
None
0.1
1.0
0.1
0.1
0.1
0.1
0.1
0.1
1.0
0.1
0.1
None
None
0.1
0.1
0.1
0.1
0.1

In [56]: def get_key(i):
    ...:     for ind in [0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8, 0.9,1.1]:
    ...:         if i <= ind:
    ...:             return ind
    ...: 
    ...: 

In [57]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     print(k)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(smatch_scores[ind])
    ...: 
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.7
None
None
None
None
1.1
None
None
None
1.1
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
0.3
0.1
None
None
0.5
None
None
None
0.3
None
0.6
0.8
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
1.1
None
0.1
0.4
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
0.6
0.1
0.1
None
0.1
0.2
None
None
0.1
None
None
None
None
0.5
0.3
0.1
0.1
0.5
0.1
0.6
None
None
0.1
0.1
1.1
0.1
None
0.4
None
None
0.1
0.1
1.1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
None
None
0.8
None
None
None
0.9
None
None
None
None
0.1
None
None
0.8
None
None
None
None
1.1
None
0.2
None
None
0.8
None
0.4
None
None
None
None
None
None
0.8
0.1
None
None
0.1
0.1
0.1
0.5
0.5
0.4
0.8
None
None
None
0.5
0.4
None
None
0.4
0.6
0.8
None
0.4
None
None
None
0.2
None
None
None
None
0.1
None
0.1
0.1
None
0.1
0.1
None
None
None
None
None
None
0.1
0.8
None
0.1
0.6
0.1
0.1
0.1
None
None
0.1
None
0.1
None
None
None
None
0.4
None
None
None
0.1
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.8
None
None
None
None
0.1
None
None
0.4
0.1
None
None
0.1
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
0.8
None
None
0.1
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
0.4
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.2
None
None
0.6
None
0.1
None
None
None
None
0.2
None
None
None
0.4
None
None
None
None
1.1
None
None
0.1
None
0.6
0.1
None
None
None
None
0.8
0.8
1.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
None
0.8
0.1
0.1
None
0.8
None
0.1
0.8
None
None
None
None
None
None
None
0.2
1.1
0.4
0.4
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.4
1.1
None
None
None
None
1.1
None
None
None
None
0.4
None
0.4
0.1
None
None
0.4
None
None
None
None
0.1
None
None
0.2
None
None
0.4
None
None
0.2
None
None
None
None
None
None
0.8
0.6
None
None
0.1
0.6
None
None
0.6
None
0.6
None
None
0.2
0.6
0.8
None
0.1
None
None
None
None
1.1
None
0.4
0.8
0.4
0.1
None
None
None
None
None
0.2
1.1
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
None
None
None
1.1
None
None
0.2
None
None
None
None
0.6
1.1
0.6
0.8
None
1.1
0.2
0.6
None
0.2
0.2
0.1
0.1
None
0.1
0.4
0.4
None
None
None
None
None
None
0.8
0.8
1.1
None
1.1
None
None
0.1
0.6
0.1
None
None
None
None
None
0.1
0.1
None
0.1
None
None
0.1
None
0.1
None
0.1
0.6
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
1.1
None
0.6
None
0.4
None
None
0.6
None
None
None
0.6
None
None
1.1
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
1.1
None
1.1
None
None
None
0.4
0.1
0.1
None
None
0.6
None
None
0.6
None
None
1.1
None
None
0.2
0.2
None
0.1
None
1.1
None
None
0.1
None
None
None
None
1.1
None
0.6
0.1
0.1
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
0.6
0.1
None
0.8
0.2
1.1
None
0.6
None
None
None
None
None
None
None
None
None
None
0.1
0.2
0.8
0.1
None
0.2
None
0.1
0.6
0.1
None
None
None
0.4
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
0.8
None
None
0.7
None
0.4
None
None
None
None
None
None
None
None
None
None
0.1
0.6
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.2
0.6
None
None
None
0.1
1.1
0.4
0.8
None
None
None
None
None
None
None
None
0.8
None
0.6
None
None
0.1
None
0.4
0.6
1.1
None
None
None
None
None
None
None
0.6
0.1
0.4
0.4
None
0.6
0.1
None
None
None
None
0.2
None
0.6
None
0.1
0.1
0.1
0.1
None
0.1
0.4
0.1
None
0.8
0.4
None
None
0.6
None
None
None
0.8
0.1
None
None
None
None
None
0.1
0.6
None
0.4
0.2
0.1
None
0.1
0.6
0.8
0.2
None
None
0.2
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
None
0.2
None
0.1
0.1
None
0.1
None
0.4
None
0.1
None
None
None
None
None
0.1
None
0.4
0.1
0.2
None
None
1.1
0.6
1.1
None
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
None
None
0.8
None
0.1
None
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
0.6
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.4
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
1.1
None
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
None
None
None
1.1
None
None
0.1
None
0.4
None
0.6
None
0.1
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
0.1
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
0.1
0.2
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.4
None
None
None
None
1.1
None
None
None
None
None
None
0.1
0.1
None
None
0.2
None
0.1
0.4
None
0.8
0.4
None
None
None
None
1.1
1.1
None
0.4
0.2
0.1
0.1
0.1
0.6
0.6
None
0.1
0.8
None
None
None
None
1.1
None
None
None
None
0.4
0.1
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
0.1
0.1
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
1.1
None
0.2
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.7
None
None
None
None
None
None
None
None
None
None
1.1
1.1
0.6
0.4
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
0.5
None
None
None
None
None
None
None
None
0.1
0.1
0.3
None
None
0.8
None
None
None
0.2
0.8
None
None
0.4
0.8
None
None
None
None
0.1
1.1
0.1
None
0.4
0.4
0.6
None
0.4
0.4
0.4
None
0.6
0.8
None
None
0.6
0.6
0.1
None
None
None
None
0.6
0.4
None
None
None
None
None
0.2
0.4
None
None
0.6
None
None
None
None
None
0.4
None
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
0.5
0.1
0.1
0.8
0.9
None
0.4
None
None
0.8
0.1
0.1
None
None
None
None
None
None
None
None
0.1
0.3
None
None
0.1
None
None
None
None
None
None
1.1
None
None
None
0.1
0.1
None
None
0.2
None
None
0.1
None
0.1
None
None
None
None
0.9
0.1
None
None
None
0.2
None
None
None
0.4
0.1
0.1
0.1
0.2
0.1
0.1
None
None
None
None
None
0.4
0.1
0.4
0.6
1.1
None
None
None
None
0.1
0.1
0.1
0.4
0.4
None
None
0.8
0.2
0.1
0.1
None
0.8
0.1
0.3
0.5
None
None
None
0.4
0.1
1.1
0.8
0.1
None
None
None
None
None
None
None
None
None
None
0.2
1.1
0.4
None
0.1
None
None
None
0.1
0.1
None
None
None
None
0.8
0.8
None
None
0.1
0.1
0.1
None
None
None
0.8
None
None
None
None
0.8
0.1
0.1
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
0.1
0.5
0.1
1.1
None
0.1
None
None
0.1
0.1
None
None
None
None
None
0.1
1.1
None
None
None
0.1
0.1
0.1
0.1
None
0.7
0.1
None
None
None
0.1
0.2
0.5
0.1
None
0.1
1.1
0.1
0.1
0.1
None
None
0.6
0.3
None
None
None
None
0.8
None
None
None
None
0.1
None
None
None
0.2
0.1
0.1
0.8
0.1
0.1
0.1
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.5
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.1
None
None
0.1
1.1
None
None
None
None
None
1.1
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.3
None
None
None
None
None
None
1.1
None
0.4
None
None
None
1.1
None
None
None
None
None
None
0.5
None
None
1.1
None
None
0.4
0.4
None
None
0.3
0.3
0.3
None
None
0.1
None
None
None
None
None
0.8
None
None
None
0.8
None
0.1
0.7
None
None
0.4
None
None
0.8
0.8
0.8
0.8
1.1
0.8
None
None
None
None
None
None
0.3
None
None
0.8
0.8
0.8
0.3
None
None
0.5
0.1
0.5
0.6
None
None
None
None
None
0.1
None
0.1
None
0.1
0.4
0.1
None
None
0.1
None
1.1
0.1
None
None
0.3
0.4
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
0.2
None
0.8
0.8
0.8
0.3
None
None
None
None
None
None
None
0.4
None
0.4
None
None
0.5
0.5
None
None
None
None
None
None
0.8
0.3
0.8
None
0.8
0.1
None
None
0.1
0.3
0.1
None
None
0.4
0.8
None
None
None
0.2
0.2
0.5
0.1
None
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
0.5
None
0.1
0.1
0.1
1.1
None
0.6
None
0.5
None
None
None
0.1
0.8
0.8
0.4
0.1
0.1
0.1
0.4
0.1
None
0.3
0.1
0.5
0.1
None
0.8
None
0.1
None
None
0.1
None
0.8
0.5
None
None
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
1.1
None
None
None
None
1.1
0.1
0.1
None
0.4
0.4
None
0.1
0.1
0.1
0.1
0.4
1.1
0.3
None
0.2
1.1
0.4
0.1
0.1
None
0.8
None
None
None
0.1
None
0.1
0.1
0.1
None
None
0.6
0.1
None
0.4
0.4
None
None
0.1
0.8
0.1
0.1
0.8
None
0.1
None
0.3
None
0.7
None
0.4
None
None
1.1
None
0.4
0.1
0.3
None
None
None
None
None
0.2
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.8
1.1
None
None
None
None
0.1
0.6
1.1
0.1
0.1
1.1
0.1
None
0.1
None
0.1
0.8
0.1
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.6
None
None
None
0.6
0.1
None
None
0.1
None
None
None
None
1.1
None
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.8
0.6
0.1
None
None
None
0.2
None
None
None
None
0.4
0.6
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
None
None
0.1
None
1.1
None
None
None
None
0.1
None
None
None
None
0.1
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
None
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1.1
None
None
0.2
None
None
None
None
None
None
None
None
None
0.6
None
0.1
0.8
None
0.2
None
0.1
0.2
None
None
0.1
None
None
None
0.4
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.4
0.4
0.1
None
None
None
None
None
None
None
None
1.1
None
None
0.1
None
0.4
None
0.1
None
None
0.4
None
0.4
None
0.1
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
1.1
None
0.1
None
0.1
None
None
0.8
None
None
None
None
None
None
0.1
None
0.1
None
None
None
0.4
None
None
None
None
None
None
None
1.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
1.1
0.1
0.8
0.1
0.1
0.1
None
None
None
None
1.1
None
None
None
0.8
0.8
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
0.4
None
1.1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
0.4
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
None
None
None
0.1
None
None
None
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.1
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.8
None
None
None
None
None
0.4
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.6
None
0.4
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
0.4
0.1
None
0.1
None
None
0.6
0.6
None
None
0.6
None
0.1
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
None
None
None
None
None
0.6
None
None
0.1
None
None
None
None
None
None
0.1
None
None
0.1
1.1
None
0.1
None
None
0.2
None
0.8
0.8
None
None
None
None
1.1
None
None
None
None
None
None
0.4
None
None
None
None
0.2
0.1
0.2
None
None
None
None
None
0.5
None
None
None
None
None
0.8
None
None
0.1
None
None
None
None
None
0.1
0.4
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
0.8
None
0.1
None
None
None
None
None
0.4
None
None
0.1
0.1
None
None
None
None
None
None
0.4
None
0.4
None
0.1
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
1.1
None
0.1
None
None
0.1
0.1
None
0.1
None
0.1
None
None
0.8
None
None
None
0.1
None
0.1
None
0.1
None
None
None
0.1
None
0.8
None
None
0.4
1.1
1.1
None
None
None
None
0.1
0.6
None
None
None
None
1.1
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
0.1
0.1
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.1
0.2
None
0.1
None
None
None
None
None
None
None
0.2
None
None
1.1
None
0.1
None
0.1
None
0.1
None
None
0.2
None
None
0.6
0.8
None
None
None
0.6
0.4
None
None
None
None
None
0.1
None
0.6
None
0.4
None
None
0.6
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
1.1
None
0.6
None
0.8
0.4
0.8
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.8
0.4
None
None
None
None
0.1
None
None
None
1.1
None
None
None
None
None
None
None
None
None
0.4
None
0.1
None
0.1
None
0.6
0.4
None
None
None
None
0.1
None
None
None
None
None
None
1.1
None
0.8
0.2
None
None
None
None
1.1
0.1
0.1
None
None
None
None
None
None
None
1.1
1.1
None
None
0.8
None
None
None
None
None
0.8
1.1
None
None
None
None
None
None
None
None
None
None
None
0.2
0.1
None
None
None
None
0.1
0.1
None
None
None
None
0.5
None
None
None
None
1.1
None
None
None
None
0.4
None
None
1.1
1.1
0.1
None
0.6
None
0.1
0.6
0.1
0.1
None
None
None
None
1.1
None
0.8
None
1.1
0.4
None
None
None
None
0.6
1.1
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
1.1
None
None
None
None
None
0.8
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
0.1
None
None
None
None
None
None
None
1.1
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
1.1
0.8
None
0.2
None
1.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
1.1
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
0.1
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
1.1
None
None
None
None
0.8
None
None
None
None
None
1.1
None
None
None
1.1
None
None
None
None
1.1
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.8
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.1
None
None
None
None
None
None
None
None
None
None
1.1
0.4
1.1
None
None
None
None
0.8
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.1
0.2
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
1.1
0.6
None
None
None
None
0.6
None
0.4
None
None
None
None
0.8
None
0.6
None
None
1.1
0.6
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
None
None
1.1
0.4
None
0.8
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1.1
None
None
0.4
None
None
None
1.1
None
None
None
None
None
0.8
0.2
None
None
None
None
1.1
None
0.8
None
None
None
None
None
None
0.2
1.1
None
None
0.4
0.1
None
None
None
None
0.1
0.1
None
0.6
None
None
1.1
None
None
None
0.8
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.4
1.1
None
None
0.8
None
None
1.1
None
1.1
None
0.6
None
None
0.1
None
None
None
0.1
None
None
None
1.1
None
None
None
None
1.1
None
None
None
None
1.1
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.6
None
None
None
None
None
None
1.1
None
0.8
None
None
None
0.8
None
None
None
None
0.6
None
None
None
None
None
0.1
None
None
None
0.8
None
None
None
None
None
0.4
None
0.4
0.2
None
0.8
None
None
None
None
None
None
None
None
1.1
None
0.6
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
1.1
None
None
None
None
None
None
0.8
1.1
None
None
None
None
None
None
None
None
None
None
None
1.1
None
0.5
1.1
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.6
1.1
None
None
None
None
0.2
None
0.6
None
None
None
1.1
None
None
None
0.8
None
0.4
0.8
None
None
None
0.4
None
None
None
None
None
None
0.1
1.1
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
1.1
None
None
0.6
None
None
None
None
None
None
None
None
None
None
1.1
None
None
1.1
None
1.1
0.8
None
None
None
0.8
None
None
None
None
None
0.8
None
None
0.8
0.1
None
None
0.2
None
0.1
None
0.8
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.1
1.1
None
None
None
0.8
None
None
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
0.6
None
0.8
None
0.2
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.6
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.8
None
None
1.1
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
None
1.1
None
None
None
None
None
None
0.6
1.1
None
None
None
None
None
0.4
None
None
None
None
0.4
0.6
None
1.1
None
None
None
None
None
1.1
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.8
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.8
0.6
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
1.1
None
None
None
1.1
0.2
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
0.8
1.1
None
None
1.1
1.1
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.1
0.1
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
0.6
None
0.6
None
None
0.1
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
None
None
None
1.1
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
1.1
None
0.1
0.8
None
0.8
None
None
0.1
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.1
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
None
0.1
None
0.1
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
0.6
None
None
None
1.1
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
1.1
None
0.2
None
None
None
None
None
None
None
0.1
None
None
1.1
0.4
None
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
0.6
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.4
None
None
1.1
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
None
0.4
0.4
1.1
None
0.1
0.1
None
None
None
0.4
None
0.1
1.1
1.1
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
0.2
None
1.1
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.1
None
0.6
0.4
None
None
None
None
1.1
None
None
0.4
None
0.6
None
None
0.1
0.4
None
0.1
None
None
None
None
None
None
None
None
None
None
None
1.1
0.8
None
0.6
None
None
None
0.6
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
0.4
None
0.8
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
0.1
None
None
1.1
None
None
1.1
0.1
None
None
None
None
None
None
None
None
None
0.8
1.1
0.1
None
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.6
None
None
None
0.4
None
None
None
None
0.8
0.8
1.1
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.4
0.6
None
1.1
None
None
None
None
None
None
None
0.1
None
None
0.1
0.2
None
None
None
None
None
None
0.1
None
None
None
0.1
0.2
None
0.2
None
None
0.1
None
0.6
None
None
None
None
None
0.4
None
1.1
None
None
None
None
0.1
None
None
0.2
None
1.1
None
None
0.2
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.2
None
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
0.1
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
0.4
0.6
None
0.1
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.2
None
None
None
None
0.4
None
None
None
0.2
1.1
None
0.1
0.6
None
1.1
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
0.4
None
0.1
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.1
1.1
None
None
None
None
0.1
None
1.1
None
None
None
None
1.1
None
1.1
1.1
None
1.1
None
None
0.1
None
0.1
None
None
1.1
None
None
None
None
None
None
1.1
None
None
None
None
1.1
1.1
None
None
None
None
None
1.1
None
1.1
None
None
None
None
0.1
None
None
None
1.1
0.1
None
None
None
None
None
1.1
0.1
None
None
None
None
None
1.1
1.1
None
0.1
None
None
1.1
1.1
None
1.1
1.1
0.1
None
1.1
None
1.1
1.1
1.1
0.1
0.1
None
1.1
None
0.1
0.1
1.1
1.1
1.1
1.1
0.1
0.1
0.1
0.1
1.1
0.1
1.1
0.1
None
None
0.1
1.1
0.1
0.1
0.1
0.1
0.1
0.1
1.1
0.1
0.1
None
None
0.1
0.1
0.1
0.1
0.1

In [58]: df = pd.DataFrame({})

In [59]: for i in sts_dict:
    ...:     print (sts_dict[i][0])
    ...: 
511
5755
205
6
260
160
23
30
191
104
6

In [60]: def get_key(i):
    ...:     for ind in [0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8, 0.9,1.0]:
    ...:         if i <= ind:
    ...:             return ind
    ...: 
    ...: 

In [61]: 

In [61]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     print(k)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(smatch_scores[ind])
    ...: 
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.7
None
None
None
None
1.0
None
None
None
1.0
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
0.3
0.1
None
None
0.5
None
None
None
0.3
None
0.6
0.8
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
1.0
None
0.1
0.4
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
0.6
0.1
0.1
None
0.1
0.2
None
None
0.1
None
None
None
None
0.5
0.3
0.1
0.1
0.5
0.1
0.6
None
None
0.1
0.1
1.0
0.1
None
0.4
None
None
0.1
0.1
1.0
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
None
None
0.8
None
None
None
0.9
None
None
None
None
0.1
None
None
0.8
None
None
None
None
1.0
None
0.2
None
None
0.8
None
0.4
None
None
None
None
None
None
0.8
0.1
None
None
0.1
0.1
0.1
0.5
0.5
0.4
0.8
None
None
None
0.5
0.4
None
None
0.4
0.6
0.8
None
0.4
None
None
None
0.2
None
None
None
None
0.1
None
0.1
0.1
None
0.1
0.1
None
None
None
None
None
None
0.1
0.8
None
0.1
0.6
0.1
0.1
0.1
None
None
0.1
None
0.1
None
None
None
None
0.4
None
None
None
0.1
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.8
None
None
None
None
0.1
None
None
0.4
0.1
None
None
0.1
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
0.8
None
None
0.1
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
0.8
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
0.4
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.2
None
None
0.6
None
0.1
None
None
None
None
0.2
None
None
None
0.4
None
None
None
None
1.0
None
None
0.1
None
0.6
0.1
None
None
None
None
0.8
0.8
1.0
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
None
0.8
0.1
0.1
None
0.8
None
0.1
0.8
None
None
None
None
None
None
None
0.2
1.0
0.4
0.4
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.4
1.0
None
None
None
None
1.0
None
None
None
None
0.4
None
0.4
0.1
None
None
0.4
None
None
None
None
0.1
None
None
0.2
None
None
0.4
None
None
0.2
None
None
None
None
None
None
0.8
0.6
None
None
0.1
0.6
None
None
0.6
None
0.6
None
None
0.2
0.6
0.8
None
0.1
None
None
None
None
1.0
None
0.4
0.8
0.4
0.1
None
None
None
None
None
0.2
1.0
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
0.6
1.0
0.6
0.8
None
1.0
0.2
0.6
None
0.2
0.2
0.1
0.1
None
0.1
0.4
0.4
None
None
None
None
None
None
0.8
0.8
1.0
None
1.0
None
None
0.1
0.6
0.1
None
None
None
None
None
0.1
0.1
None
0.1
None
None
0.1
None
0.1
None
0.1
0.6
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
1.0
None
0.6
None
0.4
None
None
0.6
None
None
None
0.6
None
None
1.0
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
1.0
None
1.0
None
None
None
0.4
0.1
0.1
None
None
0.6
None
None
0.6
None
None
1.0
None
None
0.2
0.2
None
0.1
None
1.0
None
None
0.1
None
None
None
None
1.0
None
0.6
0.1
0.1
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
0.6
0.1
None
0.8
0.2
1.0
None
0.6
None
None
None
None
None
None
None
None
None
None
0.1
0.2
0.8
0.1
None
0.2
None
0.1
0.6
0.1
None
None
None
0.4
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
0.8
None
None
0.7
None
0.4
None
None
None
None
None
None
None
None
None
None
0.1
0.6
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.2
0.6
None
None
None
0.1
1.0
0.4
0.8
None
None
None
None
None
None
None
None
0.8
None
0.6
None
None
0.1
None
0.4
0.6
1.0
None
None
None
None
None
None
None
0.6
0.1
0.4
0.4
None
0.6
0.1
None
None
None
None
0.2
None
0.6
None
0.1
0.1
0.1
0.1
None
0.1
0.4
0.1
None
0.8
0.4
None
None
0.6
None
None
None
0.8
0.1
None
None
None
None
None
0.1
0.6
None
0.4
0.2
0.1
None
0.1
0.6
0.8
0.2
None
None
0.2
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
None
0.2
None
0.1
0.1
None
0.1
None
0.4
None
0.1
None
None
None
None
None
0.1
None
0.4
0.1
0.2
None
None
1.0
0.6
1.0
None
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
None
None
0.8
None
0.1
None
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.4
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
None
None
None
1.0
None
None
0.1
None
0.4
None
0.6
None
0.1
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
0.1
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
0.1
0.2
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.4
None
None
None
None
1.0
None
None
None
None
None
None
0.1
0.1
None
None
0.2
None
0.1
0.4
None
0.8
0.4
None
None
None
None
1.0
1.0
None
0.4
0.2
0.1
0.1
0.1
0.6
0.6
None
0.1
0.8
None
None
None
None
1.0
None
None
None
None
0.4
0.1
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
0.1
0.1
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.7
None
None
None
None
None
None
None
None
None
None
1.0
1.0
0.6
0.4
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
0.5
None
None
None
None
None
None
None
None
0.1
0.1
0.3
None
None
0.8
None
None
None
0.2
0.8
None
None
0.4
0.8
None
None
None
None
0.1
1.0
0.1
None
0.4
0.4
0.6
None
0.4
0.4
0.4
None
0.6
0.8
None
None
0.6
0.6
0.1
None
None
None
None
0.6
0.4
None
None
None
None
None
0.2
0.4
None
None
0.6
None
None
None
None
None
0.4
None
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
0.5
0.1
0.1
0.8
0.9
None
0.4
None
None
0.8
0.1
0.1
None
None
None
None
None
None
None
None
0.1
0.3
None
None
0.1
None
None
None
None
None
None
1.0
None
None
None
0.1
0.1
None
None
0.2
None
None
0.1
None
0.1
None
None
None
None
0.9
0.1
None
None
None
0.2
None
None
None
0.4
0.1
0.1
0.1
0.2
0.1
0.1
None
None
None
None
None
0.4
0.1
0.4
0.6
1.0
None
None
None
None
0.1
0.1
0.1
0.4
0.4
None
None
0.8
0.2
0.1
0.1
None
0.8
0.1
0.3
0.5
None
None
None
0.4
0.1
1.0
0.8
0.1
None
None
None
None
None
None
None
None
None
None
0.2
1.0
0.4
None
0.1
None
None
None
0.1
0.1
None
None
None
None
0.8
0.8
None
None
0.1
0.1
0.1
None
None
None
0.8
None
None
None
None
0.8
0.1
0.1
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
0.1
0.5
0.1
1.0
None
0.1
None
None
0.1
0.1
None
None
None
None
None
0.1
1.0
None
None
None
0.1
0.1
0.1
0.1
None
0.7
0.1
None
None
None
0.1
0.2
0.5
0.1
None
0.1
1.0
0.1
0.1
0.1
None
None
0.6
0.3
None
None
None
None
0.8
None
None
None
None
0.1
None
None
None
0.2
0.1
0.1
0.8
0.1
0.1
0.1
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.5
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.5
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.1
None
None
0.1
1.0
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.3
None
None
None
None
None
None
1.0
None
0.4
None
None
None
1.0
None
None
None
None
None
None
0.5
None
None
1.0
None
None
0.4
0.4
None
None
0.3
0.3
0.3
None
None
0.1
None
None
None
None
None
0.8
None
None
None
0.8
None
0.1
0.7
None
None
0.4
None
None
0.8
0.8
0.8
0.8
1.0
0.8
None
None
None
None
None
None
0.3
None
None
0.8
0.8
0.8
0.3
None
None
0.5
0.1
0.5
0.6
None
None
None
None
None
0.1
None
0.1
None
0.1
0.4
0.1
None
None
0.1
None
1.0
0.1
None
None
0.3
0.4
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.2
None
0.8
0.8
0.8
0.3
None
None
None
None
None
None
None
0.4
None
0.4
None
None
0.5
0.5
None
None
None
None
None
None
0.8
0.3
0.8
None
0.8
0.1
None
None
0.1
0.3
0.1
None
None
0.4
0.8
None
None
None
0.2
0.2
0.5
0.1
None
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
0.5
None
0.1
0.1
0.1
1.0
None
0.6
None
0.5
None
None
None
0.1
0.8
0.8
0.4
0.1
0.1
0.1
0.4
0.1
None
0.3
0.1
0.5
0.1
None
0.8
None
0.1
None
None
0.1
None
0.8
0.5
None
None
None
0.1
None
None
None
None
0.1
None
None
None
0.1
None
1.0
None
None
None
None
1.0
0.1
0.1
None
0.4
0.4
None
0.1
0.1
0.1
0.1
0.4
1.0
0.3
None
0.2
1.0
0.4
0.1
0.1
None
0.8
None
None
None
0.1
None
0.1
0.1
0.1
None
None
0.6
0.1
None
0.4
0.4
None
None
0.1
0.8
0.1
0.1
0.8
None
0.1
None
0.3
None
0.7
None
0.4
None
None
1.0
None
0.4
0.1
0.3
None
None
None
None
None
0.2
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.8
1.0
None
None
None
None
0.1
0.6
1.0
0.1
0.1
1.0
0.1
None
0.1
None
0.1
0.8
0.1
0.1
0.1
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.6
None
None
None
0.6
0.1
None
None
0.1
None
None
None
None
1.0
None
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.8
0.6
0.1
None
None
None
0.2
None
None
None
None
0.4
0.6
None
None
None
None
None
None
None
None
None
None
0.8
0.1
None
None
None
0.1
None
1.0
None
None
None
None
0.1
None
None
None
None
0.1
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
None
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
None
None
None
None
None
0.6
None
0.1
0.8
None
0.2
None
0.1
0.2
None
None
0.1
None
None
None
0.4
0.1
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.4
0.4
0.1
None
None
None
None
None
None
None
None
1.0
None
None
0.1
None
0.4
None
0.1
None
None
0.4
None
0.4
None
0.1
None
None
None
None
None
0.2
0.1
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
1.0
None
0.1
None
0.1
None
None
0.8
None
None
None
None
None
None
0.1
None
0.1
None
None
None
0.4
None
None
None
None
None
None
None
1.0
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
1.0
0.1
0.8
0.1
0.1
0.1
None
None
None
None
1.0
None
None
None
0.8
0.8
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
0.4
None
1.0
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
0.4
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.1
0.8
None
0.1
0.1
None
None
None
None
None
0.1
None
None
None
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.1
None
0.2
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.8
None
None
None
None
None
0.4
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.6
None
0.4
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
0.4
0.1
None
0.1
None
None
0.6
0.6
None
None
0.6
None
0.1
0.1
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.1
None
0.1
None
0.1
None
None
None
None
None
0.6
None
None
0.1
None
None
None
None
None
None
0.1
None
None
0.1
1.0
None
0.1
None
None
0.2
None
0.8
0.8
None
None
None
None
1.0
None
None
None
None
None
None
0.4
None
None
None
None
0.2
0.1
0.2
None
None
None
None
None
0.5
None
None
None
None
None
0.8
None
None
0.1
None
None
None
None
None
0.1
0.4
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
0.8
None
0.1
None
None
None
None
None
0.4
None
None
0.1
0.1
None
None
None
None
None
None
0.4
None
0.4
None
0.1
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
1.0
None
0.1
None
None
0.1
0.1
None
0.1
None
0.1
None
None
0.8
None
None
None
0.1
None
0.1
None
0.1
None
None
None
0.1
None
0.8
None
None
0.4
1.0
1.0
None
None
None
None
0.1
0.6
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
0.1
0.1
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
0.1
None
None
None
None
None
None
None
0.2
None
None
1.0
None
0.1
None
0.1
None
0.1
None
None
0.2
None
None
0.6
0.8
None
None
None
0.6
0.4
None
None
None
None
None
0.1
None
0.6
None
0.4
None
None
0.6
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
0.1
None
None
None
None
None
None
None
None
1.0
None
0.6
None
0.8
0.4
0.8
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.8
0.4
None
None
None
None
0.1
None
None
None
1.0
None
None
None
None
None
None
None
None
None
0.4
None
0.1
None
0.1
None
0.6
0.4
None
None
None
None
0.1
None
None
None
None
None
None
1.0
None
0.8
0.2
None
None
None
None
1.0
0.1
0.1
None
None
None
None
None
None
None
1.0
1.0
None
None
0.8
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
0.2
0.1
None
None
None
None
0.1
0.1
None
None
None
None
0.5
None
None
None
None
1.0
None
None
None
None
0.4
None
None
1.0
1.0
0.1
None
0.6
None
0.1
0.6
0.1
0.1
None
None
None
None
1.0
None
0.8
None
1.0
0.4
None
None
None
None
0.6
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.1
None
None
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
1.0
0.8
None
0.2
None
1.0
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
1.0
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
1.0
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.3
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.9
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.1
None
None
None
None
None
None
None
None
None
None
1.0
0.4
1.0
None
None
None
None
0.8
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
0.4
None
0.6
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
0.6
None
0.4
None
None
None
None
0.8
None
0.6
None
None
1.0
0.6
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
None
None
1.0
0.4
None
0.8
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.6
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
1.0
None
None
0.4
None
None
None
1.0
None
None
None
None
None
0.8
0.2
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.2
1.0
None
None
0.4
0.1
None
None
None
None
0.1
0.1
None
0.6
None
None
1.0
None
None
None
0.8
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.1
None
None
0.4
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.4
1.0
None
None
0.8
None
None
1.0
None
1.0
None
0.6
None
None
0.1
None
None
None
0.1
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.8
0.1
None
0.6
None
None
None
None
None
None
1.0
None
0.8
None
None
None
0.8
None
None
None
None
0.6
None
None
None
None
None
0.1
None
None
None
0.8
None
None
None
None
None
0.4
None
0.4
0.2
None
0.8
None
None
None
None
None
None
None
None
1.0
None
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
1.0
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.5
1.0
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.6
1.0
None
None
None
None
0.2
None
0.6
None
None
None
1.0
None
None
None
0.8
None
0.4
0.8
None
None
None
0.4
None
None
None
None
None
None
0.1
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
1.0
0.8
None
None
None
0.8
None
None
None
None
None
0.8
None
None
0.8
0.1
None
None
0.2
None
0.1
None
0.8
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
0.1
1.0
None
None
None
0.8
None
None
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
0.6
None
0.8
None
0.2
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.6
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.8
None
None
1.0
0.4
None
None
None
0.1
None
None
None
None
None
None
None
0.1
None
None
1.0
None
None
None
None
None
None
0.6
1.0
None
None
None
None
None
0.4
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
1.0
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.8
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
1.0
None
None
None
1.0
0.2
None
None
None
None
None
0.1
None
None
None
None
0.1
None
None
None
None
None
0.8
1.0
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
0.1
None
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.0
0.1
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
0.6
None
0.6
None
None
0.1
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
None
None
None
1.0
None
None
None
None
None
0.1
None
None
None
None
None
None
0.1
None
None
None
None
1.0
None
0.1
0.8
None
0.8
None
None
0.1
None
0.8
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.1
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
0.1
None
None
0.1
None
0.1
None
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
None
0.6
0.6
None
None
None
1.0
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
0.1
None
None
1.0
0.4
None
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
0.6
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.1
0.4
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
None
0.4
0.4
1.0
None
0.1
0.1
None
None
None
0.4
None
0.1
1.0
1.0
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
0.2
None
1.0
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
0.6
0.4
None
None
None
None
1.0
None
None
0.4
None
0.6
None
None
0.1
0.4
None
0.1
None
None
None
None
None
None
None
None
None
None
None
1.0
0.8
None
0.6
None
None
None
0.6
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
0.4
None
0.8
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
0.1
None
None
1.0
None
None
1.0
0.1
None
None
None
None
None
None
None
None
None
0.8
1.0
0.1
None
None
0.1
0.1
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.6
None
None
None
0.4
None
None
None
None
0.8
0.8
1.0
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
None
None
0.1
None
None
0.1
0.2
None
None
None
None
None
None
0.1
None
None
None
0.1
0.2
None
0.2
None
None
0.1
None
0.6
None
None
None
None
None
0.4
None
1.0
None
None
None
None
0.1
None
None
0.2
None
1.0
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.2
None
0.1
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
0.1
None
None
None
0.1
0.1
None
None
None
None
None
None
None
None
0.4
0.6
None
0.1
None
None
0.1
None
None
None
None
None
None
None
0.1
None
0.1
None
None
None
None
None
None
None
None
None
None
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.1
None
None
0.6
0.2
None
None
None
None
0.4
None
None
None
0.2
1.0
None
0.1
0.6
None
1.0
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.1
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
0.4
0.1
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
0.4
None
0.1
None
0.4
None
None
None
None
None
None
0.1
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
0.1
None
1.0
None
None
None
None
1.0
None
1.0
1.0
None
1.0
None
None
0.1
None
0.1
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
1.0
1.0
None
None
None
None
None
1.0
None
1.0
None
None
None
None
0.1
None
None
None
1.0
0.1
None
None
None
None
None
1.0
0.1
None
None
None
None
None
1.0
1.0
None
0.1
None
None
1.0
1.0
None
1.0
1.0
0.1
None
1.0
None
1.0
1.0
1.0
0.1
0.1
None
1.0
None
0.1
0.1
1.0
1.0
1.0
1.0
0.1
0.1
0.1
0.1
1.0
0.1
1.0
0.1
None
None
0.1
1.0
0.1
0.1
0.1
0.1
0.1
0.1
1.0
0.1
0.1
None
None
0.1
0.1
0.1
0.1
0.1

In [62]: for i in sts_dict:
    ...:     print (sts_dict[i][0])
    ...: 
511
5757
205
6
258
160
23
30
191
104
6

In [63]: def get_key(i):
    ...:     for ind in [0.2,0.4,0.6,0.8,1.0]:
    ...:         if i <= ind:
    ...:             return ind
    ...: 
    ...: 

In [64]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     print(k)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(smatch_scores[ind])
    ...: 
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.8
None
None
None
None
1.0
None
None
None
1.0
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
0.2
None
None
0.6
None
None
None
0.4
None
0.6
0.8
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
1.0
None
0.2
0.4
None
None
None
None
None
None
0.2
0.2
None
None
0.8
None
None
None
None
None
None
None
0.2
None
None
0.6
0.2
0.2
None
0.2
0.2
None
None
0.2
None
None
None
None
0.6
0.4
0.2
0.2
0.6
0.2
0.6
None
None
0.2
0.2
1.0
0.2
None
0.4
None
None
0.2
0.2
1.0
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
None
None
0.8
None
None
None
1.0
None
None
None
None
0.2
None
None
0.8
None
None
None
None
1.0
None
0.2
None
None
0.8
None
0.4
None
None
None
None
None
None
0.8
0.2
None
None
0.2
0.2
0.2
0.6
0.6
0.4
0.8
None
None
None
0.6
0.4
None
None
0.4
0.6
0.8
None
0.4
None
None
None
0.2
None
None
None
None
0.2
None
0.2
0.2
None
0.2
0.2
None
None
None
None
None
None
0.2
0.8
None
0.2
0.6
0.2
0.2
0.2
None
None
0.2
None
0.2
None
None
None
None
0.4
None
None
None
0.2
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.8
None
None
None
None
0.2
None
None
0.4
0.2
None
None
0.2
0.6
None
None
None
None
None
0.2
None
None
None
None
None
None
0.8
None
None
0.2
None
0.2
None
None
None
None
0.2
None
None
None
0.2
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
None
0.8
None
None
0.2
None
None
None
0.2
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
0.4
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
0.2
None
None
0.6
None
0.2
None
None
None
None
0.2
None
None
None
0.4
None
None
None
None
1.0
None
None
0.2
None
0.6
0.2
None
None
None
None
0.8
0.8
1.0
0.2
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.6
None
0.8
0.2
0.2
None
0.8
None
0.2
0.8
None
None
None
None
None
None
None
0.2
1.0
0.4
0.4
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.4
1.0
None
None
None
None
1.0
None
None
None
None
0.4
None
0.4
0.2
None
None
0.4
None
None
None
None
0.2
None
None
0.2
None
None
0.4
None
None
0.2
None
None
None
None
None
None
0.8
0.6
None
None
0.2
0.6
None
None
0.6
None
0.6
None
None
0.2
0.6
0.8
None
0.2
None
None
None
None
1.0
None
0.4
0.8
0.4
0.2
None
None
None
None
None
0.2
1.0
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
0.6
1.0
0.6
0.8
None
1.0
0.2
0.6
None
0.2
0.2
0.2
0.2
None
0.2
0.4
0.4
None
None
None
None
None
None
0.8
0.8
1.0
None
1.0
None
None
0.2
0.6
0.2
None
None
None
None
None
0.2
0.2
None
0.2
None
None
0.2
None
0.2
None
0.2
0.6
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
1.0
None
0.6
None
0.4
None
None
0.6
None
None
None
0.6
None
None
1.0
0.2
None
None
None
None
None
None
0.4
None
None
None
None
None
None
1.0
None
1.0
None
None
None
0.4
0.2
0.2
None
None
0.6
None
None
0.6
None
None
1.0
None
None
0.2
0.2
None
0.2
None
1.0
None
None
0.2
None
None
None
None
1.0
None
0.6
0.2
0.2
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
0.6
0.2
None
0.8
0.2
1.0
None
0.6
None
None
None
None
None
None
None
None
None
None
0.2
0.2
0.8
0.2
None
0.2
None
0.2
0.6
0.2
None
None
None
0.4
None
None
None
None
None
None
0.8
None
None
None
None
0.2
None
0.8
None
None
0.8
None
0.4
None
None
None
None
None
None
None
None
None
None
0.2
0.6
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.2
None
0.2
0.6
None
None
None
0.2
1.0
0.4
0.8
None
None
None
None
None
None
None
None
0.8
None
0.6
None
None
0.2
None
0.4
0.6
1.0
None
None
None
None
None
None
None
0.6
0.2
0.4
0.4
None
0.6
0.2
None
None
None
None
0.2
None
0.6
None
0.2
0.2
0.2
0.2
None
0.2
0.4
0.2
None
0.8
0.4
None
None
0.6
None
None
None
0.8
0.2
None
None
None
None
None
0.2
0.6
None
0.4
0.2
0.2
None
0.2
0.6
0.8
0.2
None
None
0.2
None
None
None
None
None
0.6
None
None
None
None
0.2
None
None
None
0.2
None
0.2
0.2
None
0.2
None
0.4
None
0.2
None
None
None
None
None
0.2
None
0.4
0.2
0.2
None
None
1.0
0.6
1.0
None
None
None
None
None
None
0.2
0.2
None
0.2
None
None
None
None
None
0.8
None
0.2
None
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.4
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
None
None
None
1.0
None
None
0.2
None
0.4
None
0.6
None
0.2
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
0.2
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
1.0
None
None
None
None
None
None
0.2
0.2
None
None
0.2
None
0.2
0.4
None
0.8
0.4
None
None
None
None
1.0
1.0
None
0.4
0.2
0.2
0.2
0.2
0.6
0.6
None
0.2
0.8
None
None
None
None
1.0
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.2
None
0.2
None
0.2
0.2
0.2
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.6
None
None
None
0.2
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
1.0
1.0
0.6
0.4
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
0.2
0.4
None
None
0.8
None
None
None
0.2
0.8
None
None
0.4
0.8
None
None
None
None
0.2
1.0
0.2
None
0.4
0.4
0.6
None
0.4
0.4
0.4
None
0.6
0.8
None
None
0.6
0.6
0.2
None
None
None
None
0.6
0.4
None
None
None
None
None
0.2
0.4
None
None
0.6
None
None
None
None
None
0.4
None
0.2
0.2
0.8
None
None
None
None
None
None
None
None
None
0.6
0.2
0.2
0.8
1.0
None
0.4
None
None
0.8
0.2
0.2
None
None
None
None
None
None
None
None
0.2
0.4
None
None
0.2
None
None
None
None
None
None
1.0
None
None
None
0.2
0.2
None
None
0.2
None
None
0.2
None
0.2
None
None
None
None
1.0
0.2
None
None
None
0.2
None
None
None
0.4
0.2
0.2
0.2
0.2
0.2
0.2
None
None
None
None
None
0.4
0.2
0.4
0.6
1.0
None
None
None
None
0.2
0.2
0.2
0.4
0.4
None
None
0.8
0.2
0.2
0.2
None
0.8
0.2
0.4
0.6
None
None
None
0.4
0.2
1.0
0.8
0.2
None
None
None
None
None
None
None
None
None
None
0.2
1.0
0.4
None
0.2
None
None
None
0.2
0.2
None
None
None
None
0.8
0.8
None
None
0.2
0.2
0.2
None
None
None
0.8
None
None
None
None
0.8
0.2
0.2
None
None
None
None
None
0.2
0.8
None
0.2
0.2
None
None
0.2
0.6
0.2
1.0
None
0.2
None
None
0.2
0.2
None
None
None
None
None
0.2
1.0
None
None
None
0.2
0.2
0.2
0.2
None
0.8
0.2
None
None
None
0.2
0.2
0.6
0.2
None
0.2
1.0
0.2
0.2
0.2
None
None
0.6
0.4
None
None
None
None
0.8
None
None
None
None
0.2
None
None
None
0.2
0.2
0.2
0.8
0.2
0.2
0.2
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
0.2
None
0.6
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.2
None
None
0.2
1.0
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.4
None
None
None
None
None
None
1.0
None
0.4
None
None
None
1.0
None
None
None
None
None
None
0.6
None
None
1.0
None
None
0.4
0.4
None
None
0.4
0.4
0.4
None
None
0.2
None
None
None
None
None
0.8
None
None
None
0.8
None
0.2
0.8
None
None
0.4
None
None
0.8
0.8
0.8
0.8
1.0
0.8
None
None
None
None
None
None
0.4
None
None
0.8
0.8
0.8
0.4
None
None
0.6
0.2
0.6
0.6
None
None
None
None
None
0.2
None
0.2
None
0.2
0.4
0.2
None
None
0.2
None
1.0
0.2
None
None
0.4
0.4
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.2
None
0.8
0.8
0.8
0.4
None
None
None
None
None
None
None
0.4
None
0.4
None
None
0.6
0.6
None
None
None
None
None
None
0.8
0.4
0.8
None
0.8
0.2
None
None
0.2
0.4
0.2
None
None
0.4
0.8
None
None
None
0.2
0.2
0.6
0.2
None
0.2
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
0.6
None
0.2
0.2
0.2
1.0
None
0.6
None
0.6
None
None
None
0.2
0.8
0.8
0.4
0.2
0.2
0.2
0.4
0.2
None
0.4
0.2
0.6
0.2
None
0.8
None
0.2
None
None
0.2
None
0.8
0.6
None
None
None
0.2
None
None
None
None
0.2
None
None
None
0.2
None
1.0
None
None
None
None
1.0
0.2
0.2
None
0.4
0.4
None
0.2
0.2
0.2
0.2
0.4
1.0
0.4
None
0.2
1.0
0.4
0.2
0.2
None
0.8
None
None
None
0.2
None
0.2
0.2
0.2
None
None
0.6
0.2
None
0.4
0.4
None
None
0.2
0.8
0.2
0.2
0.8
None
0.2
None
0.4
None
0.8
None
0.4
None
None
1.0
None
0.4
0.2
0.4
None
None
None
None
None
0.2
None
0.6
None
None
None
None
0.2
None
None
0.4
None
None
0.8
1.0
None
None
None
None
0.2
0.6
1.0
0.2
0.2
1.0
0.2
None
0.2
None
0.2
0.8
0.2
0.2
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.6
None
None
None
0.6
0.2
None
None
0.2
None
None
None
None
1.0
None
0.4
None
None
None
0.2
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.8
0.6
0.2
None
None
None
0.2
None
None
None
None
0.4
0.6
None
None
None
None
None
None
None
None
None
None
0.8
0.2
None
None
None
0.2
None
1.0
None
None
None
None
0.2
None
None
None
None
0.2
None
None
0.2
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
0.4
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
None
None
None
None
None
0.6
None
0.2
0.8
None
0.2
None
0.2
0.2
None
None
0.2
None
None
None
0.4
0.2
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.4
0.4
0.2
None
None
None
None
None
None
None
None
1.0
None
None
0.2
None
0.4
None
0.2
None
None
0.4
None
0.4
None
0.2
None
None
None
None
None
0.2
0.2
None
0.2
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
1.0
None
0.2
None
0.2
None
None
0.8
None
None
None
None
None
None
0.2
None
0.2
None
None
None
0.4
None
None
None
None
None
None
None
1.0
None
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
0.2
0.8
0.2
0.2
0.2
None
None
None
None
1.0
None
None
None
0.8
0.8
None
None
None
None
None
0.2
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
0.4
None
1.0
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.4
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
0.8
None
0.2
0.2
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.2
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.8
None
None
None
None
None
0.4
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.6
None
0.4
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
0.4
0.2
None
0.2
None
None
0.6
0.6
None
None
0.6
None
0.2
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
0.2
None
0.2
None
None
None
None
None
0.6
None
None
0.2
None
None
None
None
None
None
0.2
None
None
0.2
1.0
None
0.2
None
None
0.2
None
0.8
0.8
None
None
None
None
1.0
None
None
None
None
None
None
0.4
None
None
None
None
0.2
0.2
0.2
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
None
0.2
None
None
None
None
None
0.2
0.4
None
None
None
None
None
None
0.2
None
0.4
None
0.6
None
None
None
0.8
None
0.2
None
None
None
None
None
0.4
None
None
0.2
0.2
None
None
None
None
None
None
0.4
None
0.4
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.0
None
0.2
None
None
0.2
0.2
None
0.2
None
0.2
None
None
0.8
None
None
None
0.2
None
0.2
None
0.2
None
None
None
0.2
None
0.8
None
None
0.4
1.0
1.0
None
None
None
None
0.2
0.6
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
0.2
0.2
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
0.2
None
None
None
None
None
None
None
0.2
None
None
1.0
None
0.2
None
0.2
None
0.2
None
None
0.2
None
None
0.6
0.8
None
None
None
0.6
0.4
None
None
None
None
None
0.2
None
0.6
None
0.4
None
None
0.6
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
0.2
None
None
None
None
None
None
None
None
1.0
None
0.6
None
0.8
0.4
0.8
0.6
0.2
None
0.2
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
0.8
0.4
None
None
None
None
0.2
None
None
None
1.0
None
None
None
None
None
None
None
None
None
0.4
None
0.2
None
0.2
None
0.6
0.4
None
None
None
None
0.2
None
None
None
None
None
None
1.0
None
0.8
0.2
None
None
None
None
1.0
0.2
0.2
None
None
None
None
None
None
None
1.0
1.0
None
None
0.8
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
None
None
None
0.2
0.2
None
None
None
None
0.6
None
None
None
None
1.0
None
None
None
None
0.4
None
None
1.0
1.0
0.2
None
0.6
None
0.2
0.6
0.2
0.2
None
None
None
None
1.0
None
0.8
None
1.0
0.4
None
None
None
None
0.6
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.2
None
None
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
1.0
0.8
None
0.2
None
1.0
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
1.0
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
1.0
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
1.0
0.4
1.0
None
None
None
None
0.8
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
0.6
None
0.4
None
None
None
None
0.8
None
0.6
None
None
1.0
0.6
None
0.2
0.2
0.2
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
None
None
1.0
0.4
None
0.8
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
0.4
None
None
None
1.0
None
None
None
None
None
0.8
0.2
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.2
1.0
None
None
0.4
0.2
None
None
None
None
0.2
0.2
None
0.6
None
None
1.0
None
None
None
0.8
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.2
None
None
0.4
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.4
1.0
None
None
0.8
None
None
1.0
None
1.0
None
0.6
None
None
0.2
None
None
None
0.2
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.2
None
None
None
None
0.2
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
0.2
None
0.6
None
None
None
None
None
None
1.0
None
0.8
None
None
None
0.8
None
None
None
None
0.6
None
None
None
None
None
0.2
None
None
None
0.8
None
None
None
None
None
0.4
None
0.4
0.2
None
0.8
None
None
None
None
None
None
None
None
1.0
None
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
1.0
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.6
1.0
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.6
1.0
None
None
None
None
0.2
None
0.6
None
None
None
1.0
None
None
None
0.8
None
0.4
0.8
None
None
None
0.4
None
None
None
None
None
None
0.2
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
1.0
0.8
None
None
None
0.8
None
None
None
None
None
0.8
None
None
0.8
0.2
None
None
0.2
None
0.2
None
0.8
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
0.2
1.0
None
None
None
0.8
None
None
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
0.6
None
0.8
None
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.6
None
0.6
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.8
None
None
1.0
0.4
None
None
None
0.2
None
None
None
None
None
None
None
0.2
None
None
1.0
None
None
None
None
None
None
0.6
1.0
None
None
None
None
None
0.4
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
1.0
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.8
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
1.0
None
None
None
1.0
0.2
None
None
None
None
None
0.2
None
None
None
None
0.2
None
None
None
None
None
0.8
1.0
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.0
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
0.6
None
0.6
None
None
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
None
None
None
1.0
None
None
None
None
None
0.2
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
0.2
0.8
None
0.8
None
None
0.2
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.2
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
None
None
0.2
None
0.2
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.6
0.6
None
None
None
1.0
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
0.2
None
None
1.0
0.4
None
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
0.6
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
0.6
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
None
0.4
0.4
1.0
None
0.2
0.2
None
None
None
0.4
None
0.2
1.0
1.0
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
0.2
None
1.0
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
0.6
0.4
None
None
None
None
1.0
None
None
0.4
None
0.6
None
None
0.2
0.4
None
0.2
None
None
None
None
None
None
None
None
None
None
None
1.0
0.8
None
0.6
None
None
None
0.6
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
0.4
None
0.8
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
0.2
None
None
1.0
None
None
1.0
0.2
None
None
None
None
None
None
None
None
None
0.8
1.0
0.2
None
None
0.2
0.2
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.6
None
None
None
0.4
None
None
None
None
0.8
0.8
1.0
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
None
None
0.2
None
None
0.2
0.2
None
None
None
None
None
None
0.2
None
None
None
0.2
0.2
None
0.2
None
None
0.2
None
0.6
None
None
None
None
None
0.4
None
1.0
None
None
None
None
0.2
None
None
0.2
None
1.0
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.2
None
0.2
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
0.2
None
None
None
0.2
0.2
None
None
None
None
None
None
None
None
0.4
0.6
None
0.2
None
None
0.2
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
0.6
0.2
None
None
None
None
0.4
None
None
None
0.2
1.0
None
0.2
0.6
None
1.0
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
0.4
None
0.2
None
0.4
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
0.2
None
1.0
None
None
None
None
1.0
None
1.0
1.0
None
1.0
None
None
0.2
None
0.2
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
1.0
1.0
None
None
None
None
None
1.0
None
1.0
None
None
None
None
0.2
None
None
None
1.0
0.2
None
None
None
None
None
1.0
0.2
None
None
None
None
None
1.0
1.0
None
0.2
None
None
1.0
1.0
None
1.0
1.0
0.2
None
1.0
None
1.0
1.0
1.0
0.2
0.2
None
1.0
None
0.2
0.2
1.0
1.0
1.0
1.0
0.2
0.2
0.2
0.2
1.0
0.2
1.0
0.2
None
None
0.2
1.0
0.2
0.2
0.2
0.2
0.2
0.2
1.0
0.2
0.2
None
None
0.2
0.2
0.2
0.2
0.2

In [65]: for i in sts_dict:
    ...:     print (sts_dict[i][0])
    ...: 
615
5757
211
264
190
214

In [66]: 190*5
Out[66]: 950

In [67]: 

In [67]: 200*5
Out[67]: 1000

In [68]: 210
Out[68]: 210

In [69]: 210*5
Out[69]: 1050

In [70]: df = pd.DataFrame({})

In [71]: count = 200
    ...: for i in sts_dict:
    ...:     df = df.append(pd.DataFrame("sts_bucket":[i]*210, "smatch":sts_dict[i][1][:210]), ignore_index=T
    ...: rue)
    ...: 
    ...: 
  File "<ipython-input-71-3153cfca8952>", line 3
    df = df.append(pd.DataFrame("sts_bucket":[i]*210, "smatch":sts_dict[i][1][:210]), ignore_index=True)
                                            ^
SyntaxError: invalid syntax


In [72]: count = 200
    ...: for i in sts_dict:
    ...:     df = df.append(pd.DataFrame({"sts_bucket":[i]*210, "smatch":sts_dict[i][1][:210]}), ignore_index
    ...: =True)
    ...: 
    ...: 
    ...: 
---------------------------------------------------------------------------
ValueError                                Traceback (most recent call last)
<ipython-input-72-dfb3d83b3409> in <module>
      1 count = 200
      2 for i in sts_dict:
----> 3     df = df.append(pd.DataFrame({"sts_bucket":[i]*210, "smatch":sts_dict[i][1][:210]}), ignore_index=True)
      4 
      5 

/Library/Python/3.8/site-packages/pandas/core/frame.py in __init__(self, data, index, columns, dtype, copy)
    527 
    528         elif isinstance(data, dict):
--> 529             mgr = init_dict(data, index, columns, dtype=dtype)
    530         elif isinstance(data, ma.MaskedArray):
    531             import numpy.ma.mrecords as mrecords

/Library/Python/3.8/site-packages/pandas/core/internals/construction.py in init_dict(data, index, columns, dtype)
    285             arr if not is_datetime64tz_dtype(arr) else arr.copy() for arr in arrays
    286         ]
--> 287     return arrays_to_mgr(arrays, data_names, index, columns, dtype=dtype)
    288 
    289 

/Library/Python/3.8/site-packages/pandas/core/internals/construction.py in arrays_to_mgr(arrays, arr_names, index, columns, dtype, verify_integrity)
     78         # figure out the index, if necessary
     79         if index is None:
---> 80             index = extract_index(arrays)
     81         else:
     82             index = ensure_index(index)

/Library/Python/3.8/site-packages/pandas/core/internals/construction.py in extract_index(data)
    399             lengths = list(set(raw_lengths))
    400             if len(lengths) > 1:
--> 401                 raise ValueError("arrays must all be same length")
    402 
    403             if have_dicts:

ValueError: arrays must all be same length

In [73]: count = 200
    ...: for i in sts_dict:
    ...:     temp_df = pd.DataFrame({})
    ...:     temp_df["sts_bucket"] = [i]*210
    ...:     temp_df["smatch"] = sts_dict[i][1][:210]
    ...:     df = df.append(temp_df, ignore_index=True)
    ...: 
    ...: 
    ...: 
---------------------------------------------------------------------------
ValueError                                Traceback (most recent call last)
<ipython-input-73-3ffe50797d78> in <module>
      3     temp_df = pd.DataFrame({})
      4     temp_df["sts_bucket"] = [i]*210
----> 5     temp_df["smatch"] = sts_dict[i][1][:210]
      6     df = df.append(temp_df, ignore_index=True)
      7 

/Library/Python/3.8/site-packages/pandas/core/frame.py in __setitem__(self, key, value)
   3161         else:
   3162             # set column
-> 3163             self._set_item(key, value)
   3164 
   3165     def _setitem_slice(self, key: slice, value):

/Library/Python/3.8/site-packages/pandas/core/frame.py in _set_item(self, key, value)
   3240         """
   3241         self._ensure_valid_index(value)
-> 3242         value = self._sanitize_column(key, value)
   3243         NDFrame._set_item(self, key, value)
   3244 

/Library/Python/3.8/site-packages/pandas/core/frame.py in _sanitize_column(self, key, value, broadcast)
   3897 
   3898             # turn me into an ndarray
-> 3899             value = sanitize_index(value, self.index)
   3900             if not isinstance(value, (np.ndarray, Index)):
   3901                 if isinstance(value, list) and len(value) > 0:

/Library/Python/3.8/site-packages/pandas/core/internals/construction.py in sanitize_index(data, index)
    749     """
    750     if len(data) != len(index):
--> 751         raise ValueError(
    752             "Length of values "
    753             f"({len(data)}) "

ValueError: Length of values (190) does not match length of index (210)

In [74]: count = 200
    ...: for i in sts_dict:
    ...:     temp_df = pd.DataFrame({})
    ...:     temp_df["sts_bucket"] = [i]*190
    ...:     temp_df["smatch"] = sts_dict[i][1][:190]
    ...:     df = df.append(temp_df, ignore_index=True)
    ...: 
    ...: 
    ...: 

In [75]: df
Out[75]: 
      sts_bucket    smatch
0            0.2  0.800000
1            0.2  0.500000
2            0.2  0.428571
3            0.2  0.500000
4            0.2  0.333333
...          ...       ...
2815         0.4  0.451613
2816         0.4  0.486486
2817         0.4  0.480000
2818         0.4  0.437500
2819         0.4  0.368421

[2820 rows x 2 columns]

In [76]: sns.boxplot(x="sts_bucket", y="smatch", data=df)
Out[76]: <AxesSubplot:xlabel='sts_bucket', ylabel='smatch'>

In [77]: plt.show()
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-77-1eb00ff78cf2> in <module>
----> 1 plt.show()

NameError: name 'plt' is not defined

In [78]: import matplotlib.pyplot as plt

In [79]: plt.show()

In [80]: plt.show()

In [81]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     print(k)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [i], [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(i)
    ...:         sts_dict[k][2].append(smatch_scores[ind])
    ...: 
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.8
None
None
None
None
1.0
None
None
None
1.0
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
0.2
None
None
0.6
None
None
None
0.4
None
0.6
0.8
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
1.0
None
0.2
0.4
None
None
None
None
None
None
0.2
0.2
None
None
0.8
None
None
None
None
None
None
None
0.2
None
None
0.6
0.2
0.2
None
0.2
0.2
None
None
0.2
None
None
None
None
0.6
0.4
0.2
0.2
0.6
0.2
0.6
None
None
0.2
0.2
1.0
0.2
None
0.4
None
None
0.2
0.2
1.0
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
None
None
0.8
None
None
None
1.0
None
None
None
None
0.2
None
None
0.8
None
None
None
None
1.0
None
0.2
None
None
0.8
None
0.4
None
None
None
None
None
None
0.8
0.2
None
None
0.2
0.2
0.2
0.6
0.6
0.4
0.8
None
None
None
0.6
0.4
None
None
0.4
0.6
0.8
None
0.4
None
None
None
0.2
None
None
None
None
0.2
None
0.2
0.2
None
0.2
0.2
None
None
None
None
None
None
0.2
0.8
None
0.2
0.6
0.2
0.2
0.2
None
None
0.2
None
0.2
None
None
None
None
0.4
None
None
None
0.2
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.8
None
None
None
None
0.2
None
None
0.4
0.2
None
None
0.2
0.6
None
None
None
None
None
0.2
None
None
None
None
None
None
0.8
None
None
0.2
None
0.2
None
None
None
None
0.2
None
None
None
0.2
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
None
0.8
None
None
0.2
None
None
None
0.2
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
0.4
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
0.2
None
None
0.6
None
0.2
None
None
None
None
0.2
None
None
None
0.4
None
None
None
None
1.0
None
None
0.2
None
0.6
0.2
None
None
None
None
0.8
0.8
1.0
0.2
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.6
None
0.8
0.2
0.2
None
0.8
None
0.2
0.8
None
None
None
None
None
None
None
0.2
1.0
0.4
0.4
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.4
1.0
None
None
None
None
1.0
None
None
None
None
0.4
None
0.4
0.2
None
None
0.4
None
None
None
None
0.2
None
None
0.2
None
None
0.4
None
None
0.2
None
None
None
None
None
None
0.8
0.6
None
None
0.2
0.6
None
None
0.6
None
0.6
None
None
0.2
0.6
0.8
None
0.2
None
None
None
None
1.0
None
0.4
0.8
0.4
0.2
None
None
None
None
None
0.2
1.0
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
0.6
1.0
0.6
0.8
None
1.0
0.2
0.6
None
0.2
0.2
0.2
0.2
None
0.2
0.4
0.4
None
None
None
None
None
None
0.8
0.8
1.0
None
1.0
None
None
0.2
0.6
0.2
None
None
None
None
None
0.2
0.2
None
0.2
None
None
0.2
None
0.2
None
0.2
0.6
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
1.0
None
0.6
None
0.4
None
None
0.6
None
None
None
0.6
None
None
1.0
0.2
None
None
None
None
None
None
0.4
None
None
None
None
None
None
1.0
None
1.0
None
None
None
0.4
0.2
0.2
None
None
0.6
None
None
0.6
None
None
1.0
None
None
0.2
0.2
None
0.2
None
1.0
None
None
0.2
None
None
None
None
1.0
None
0.6
0.2
0.2
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
0.6
0.2
None
0.8
0.2
1.0
None
0.6
None
None
None
None
None
None
None
None
None
None
0.2
0.2
0.8
0.2
None
0.2
None
0.2
0.6
0.2
None
None
None
0.4
None
None
None
None
None
None
0.8
None
None
None
None
0.2
None
0.8
None
None
0.8
None
0.4
None
None
None
None
None
None
None
None
None
None
0.2
0.6
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.2
None
0.2
0.6
None
None
None
0.2
1.0
0.4
0.8
None
None
None
None
None
None
None
None
0.8
None
0.6
None
None
0.2
None
0.4
0.6
1.0
None
None
None
None
None
None
None
0.6
0.2
0.4
0.4
None
0.6
0.2
None
None
None
None
0.2
None
0.6
None
0.2
0.2
0.2
0.2
None
0.2
0.4
0.2
None
0.8
0.4
None
None
0.6
None
None
None
0.8
0.2
None
None
None
None
None
0.2
0.6
None
0.4
0.2
0.2
None
0.2
0.6
0.8
0.2
None
None
0.2
None
None
None
None
None
0.6
None
None
None
None
0.2
None
None
None
0.2
None
0.2
0.2
None
0.2
None
0.4
None
0.2
None
None
None
None
None
0.2
None
0.4
0.2
0.2
None
None
1.0
0.6
1.0
None
None
None
None
None
None
0.2
0.2
None
0.2
None
None
None
None
None
0.8
None
0.2
None
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.4
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
None
None
None
1.0
None
None
0.2
None
0.4
None
0.6
None
0.2
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
0.2
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
1.0
None
None
None
None
None
None
0.2
0.2
None
None
0.2
None
0.2
0.4
None
0.8
0.4
None
None
None
None
1.0
1.0
None
0.4
0.2
0.2
0.2
0.2
0.6
0.6
None
0.2
0.8
None
None
None
None
1.0
None
None
None
None
0.4
0.2
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.2
None
0.2
None
0.2
0.2
0.2
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
0.6
None
None
None
0.2
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
1.0
1.0
0.6
0.4
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
0.2
0.4
None
None
0.8
None
None
None
0.2
0.8
None
None
0.4
0.8
None
None
None
None
0.2
1.0
0.2
None
0.4
0.4
0.6
None
0.4
0.4
0.4
None
0.6
0.8
None
None
0.6
0.6
0.2
None
None
None
None
0.6
0.4
None
None
None
None
None
0.2
0.4
None
None
0.6
None
None
None
None
None
0.4
None
0.2
0.2
0.8
None
None
None
None
None
None
None
None
None
0.6
0.2
0.2
0.8
1.0
None
0.4
None
None
0.8
0.2
0.2
None
None
None
None
None
None
None
None
0.2
0.4
None
None
0.2
None
None
None
None
None
None
1.0
None
None
None
0.2
0.2
None
None
0.2
None
None
0.2
None
0.2
None
None
None
None
1.0
0.2
None
None
None
0.2
None
None
None
0.4
0.2
0.2
0.2
0.2
0.2
0.2
None
None
None
None
None
0.4
0.2
0.4
0.6
1.0
None
None
None
None
0.2
0.2
0.2
0.4
0.4
None
None
0.8
0.2
0.2
0.2
None
0.8
0.2
0.4
0.6
None
None
None
0.4
0.2
1.0
0.8
0.2
None
None
None
None
None
None
None
None
None
None
0.2
1.0
0.4
None
0.2
None
None
None
0.2
0.2
None
None
None
None
0.8
0.8
None
None
0.2
0.2
0.2
None
None
None
0.8
None
None
None
None
0.8
0.2
0.2
None
None
None
None
None
0.2
0.8
None
0.2
0.2
None
None
0.2
0.6
0.2
1.0
None
0.2
None
None
0.2
0.2
None
None
None
None
None
0.2
1.0
None
None
None
0.2
0.2
0.2
0.2
None
0.8
0.2
None
None
None
0.2
0.2
0.6
0.2
None
0.2
1.0
0.2
0.2
0.2
None
None
0.6
0.4
None
None
None
None
0.8
None
None
None
None
0.2
None
None
None
0.2
0.2
0.2
0.8
0.2
0.2
0.2
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
0.2
None
0.6
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.2
None
None
0.2
1.0
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.4
None
None
None
None
None
None
1.0
None
0.4
None
None
None
1.0
None
None
None
None
None
None
0.6
None
None
1.0
None
None
0.4
0.4
None
None
0.4
0.4
0.4
None
None
0.2
None
None
None
None
None
0.8
None
None
None
0.8
None
0.2
0.8
None
None
0.4
None
None
0.8
0.8
0.8
0.8
1.0
0.8
None
None
None
None
None
None
0.4
None
None
0.8
0.8
0.8
0.4
None
None
0.6
0.2
0.6
0.6
None
None
None
None
None
0.2
None
0.2
None
0.2
0.4
0.2
None
None
0.2
None
1.0
0.2
None
None
0.4
0.4
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.2
None
0.8
0.8
0.8
0.4
None
None
None
None
None
None
None
0.4
None
0.4
None
None
0.6
0.6
None
None
None
None
None
None
0.8
0.4
0.8
None
0.8
0.2
None
None
0.2
0.4
0.2
None
None
0.4
0.8
None
None
None
0.2
0.2
0.6
0.2
None
0.2
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
0.6
None
0.2
0.2
0.2
1.0
None
0.6
None
0.6
None
None
None
0.2
0.8
0.8
0.4
0.2
0.2
0.2
0.4
0.2
None
0.4
0.2
0.6
0.2
None
0.8
None
0.2
None
None
0.2
None
0.8
0.6
None
None
None
0.2
None
None
None
None
0.2
None
None
None
0.2
None
1.0
None
None
None
None
1.0
0.2
0.2
None
0.4
0.4
None
0.2
0.2
0.2
0.2
0.4
1.0
0.4
None
0.2
1.0
0.4
0.2
0.2
None
0.8
None
None
None
0.2
None
0.2
0.2
0.2
None
None
0.6
0.2
None
0.4
0.4
None
None
0.2
0.8
0.2
0.2
0.8
None
0.2
None
0.4
None
0.8
None
0.4
None
None
1.0
None
0.4
0.2
0.4
None
None
None
None
None
0.2
None
0.6
None
None
None
None
0.2
None
None
0.4
None
None
0.8
1.0
None
None
None
None
0.2
0.6
1.0
0.2
0.2
1.0
0.2
None
0.2
None
0.2
0.8
0.2
0.2
0.2
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.6
None
None
None
0.6
0.2
None
None
0.2
None
None
None
None
1.0
None
0.4
None
None
None
0.2
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.8
0.6
0.2
None
None
None
0.2
None
None
None
None
0.4
0.6
None
None
None
None
None
None
None
None
None
None
0.8
0.2
None
None
None
0.2
None
1.0
None
None
None
None
0.2
None
None
None
None
0.2
None
None
0.2
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
0.4
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
0.2
None
None
None
None
None
None
None
None
None
0.6
None
0.2
0.8
None
0.2
None
0.2
0.2
None
None
0.2
None
None
None
0.4
0.2
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.4
0.4
0.2
None
None
None
None
None
None
None
None
1.0
None
None
0.2
None
0.4
None
0.2
None
None
0.4
None
0.4
None
0.2
None
None
None
None
None
0.2
0.2
None
0.2
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
1.0
None
0.2
None
0.2
None
None
0.8
None
None
None
None
None
None
0.2
None
0.2
None
None
None
0.4
None
None
None
None
None
None
None
1.0
None
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
0.2
0.8
0.2
0.2
0.2
None
None
None
None
1.0
None
None
None
0.8
0.8
None
None
None
None
None
0.2
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
0.4
None
1.0
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.4
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
0.8
None
0.2
0.2
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.2
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.8
None
None
None
None
None
0.4
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.6
None
0.4
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
0.6
None
None
0.4
0.2
None
0.2
None
None
0.6
0.6
None
None
0.6
None
0.2
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
0.2
None
0.2
None
0.2
None
None
None
None
None
0.6
None
None
0.2
None
None
None
None
None
None
0.2
None
None
0.2
1.0
None
0.2
None
None
0.2
None
0.8
0.8
None
None
None
None
1.0
None
None
None
None
None
None
0.4
None
None
None
None
0.2
0.2
0.2
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
None
0.2
None
None
None
None
None
0.2
0.4
None
None
None
None
None
None
0.2
None
0.4
None
0.6
None
None
None
0.8
None
0.2
None
None
None
None
None
0.4
None
None
0.2
0.2
None
None
None
None
None
None
0.4
None
0.4
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.0
None
0.2
None
None
0.2
0.2
None
0.2
None
0.2
None
None
0.8
None
None
None
0.2
None
0.2
None
0.2
None
None
None
0.2
None
0.8
None
None
0.4
1.0
1.0
None
None
None
None
0.2
0.6
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
0.2
0.2
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
0.2
None
None
None
None
None
None
None
0.2
None
None
1.0
None
0.2
None
0.2
None
0.2
None
None
0.2
None
None
0.6
0.8
None
None
None
0.6
0.4
None
None
None
None
None
0.2
None
0.6
None
0.4
None
None
0.6
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
0.2
None
None
None
None
None
None
None
None
1.0
None
0.6
None
0.8
0.4
0.8
0.6
0.2
None
0.2
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
0.8
0.4
None
None
None
None
0.2
None
None
None
1.0
None
None
None
None
None
None
None
None
None
0.4
None
0.2
None
0.2
None
0.6
0.4
None
None
None
None
0.2
None
None
None
None
None
None
1.0
None
0.8
0.2
None
None
None
None
1.0
0.2
0.2
None
None
None
None
None
None
None
1.0
1.0
None
None
0.8
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
0.2
0.2
None
None
None
None
0.2
0.2
None
None
None
None
0.6
None
None
None
None
1.0
None
None
None
None
0.4
None
None
1.0
1.0
0.2
None
0.6
None
0.2
0.6
0.2
0.2
None
None
None
None
1.0
None
0.8
None
1.0
0.4
None
None
None
None
0.6
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.2
None
None
None
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
1.0
0.8
None
0.2
None
1.0
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
1.0
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
0.8
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
1.0
None
None
None
None
0.8
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
0.8
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
1.0
0.4
1.0
None
None
None
None
0.8
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
0.4
None
0.6
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.4
None
1.0
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
1.0
0.6
None
None
None
None
0.6
None
0.4
None
None
None
None
0.8
None
0.6
None
None
1.0
0.6
None
0.2
0.2
0.2
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
None
None
1.0
0.4
None
0.8
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
0.4
None
None
None
1.0
None
None
None
None
None
0.8
0.2
None
None
None
None
1.0
None
0.8
None
None
None
None
None
None
0.2
1.0
None
None
0.4
0.2
None
None
None
None
0.2
0.2
None
0.6
None
None
1.0
None
None
None
0.8
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.2
None
None
0.4
None
None
0.4
None
None
None
None
None
None
0.6
None
None
None
None
None
None
0.4
1.0
None
None
0.8
None
None
1.0
None
1.0
None
0.6
None
None
0.2
None
None
None
0.2
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
1.0
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
0.2
None
None
None
None
0.2
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.8
0.2
None
0.6
None
None
None
None
None
None
1.0
None
0.8
None
None
None
0.8
None
None
None
None
0.6
None
None
None
None
None
0.2
None
None
None
0.8
None
None
None
None
None
0.4
None
0.4
0.2
None
0.8
None
None
None
None
None
None
None
None
1.0
None
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
1.0
None
None
None
None
None
None
0.8
1.0
None
None
None
None
None
None
None
None
None
None
None
1.0
None
0.6
1.0
None
None
None
0.8
None
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
0.6
1.0
None
None
None
None
0.2
None
0.6
None
None
None
1.0
None
None
None
0.8
None
0.4
0.8
None
None
None
0.4
None
None
None
None
None
None
0.2
1.0
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
None
1.0
None
None
1.0
None
1.0
0.8
None
None
None
0.8
None
None
None
None
None
0.8
None
None
0.8
0.2
None
None
0.2
None
0.2
None
0.8
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
0.2
1.0
None
None
None
0.8
None
None
None
0.2
0.4
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
0.6
None
0.8
None
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
0.6
None
0.6
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.8
None
None
1.0
0.4
None
None
None
0.2
None
None
None
None
None
None
None
0.2
None
None
1.0
None
None
None
None
None
None
0.6
1.0
None
None
None
None
None
0.4
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
1.0
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
0.8
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.8
0.6
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
0.4
None
None
None
None
0.6
None
None
1.0
None
None
None
1.0
0.2
None
None
None
None
None
0.2
None
None
None
None
0.2
None
None
None
None
None
0.8
1.0
None
None
1.0
1.0
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
0.8
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
1.0
0.2
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
0.6
None
0.6
None
None
0.2
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.4
None
None
None
1.0
None
None
None
None
None
0.2
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
0.2
0.8
None
0.8
None
None
0.2
None
0.8
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
0.2
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
None
None
0.2
None
0.2
None
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
None
0.6
0.6
None
None
None
1.0
0.6
0.8
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
0.2
None
None
None
None
None
None
None
0.2
None
None
1.0
0.4
None
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
0.6
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
0.2
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.8
None
None
None
None
None
None
None
None
None
None
0.8
0.6
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
0.4
None
None
1.0
None
None
0.6
None
None
None
None
None
None
None
None
None
0.4
None
0.4
0.4
1.0
None
0.2
0.2
None
None
None
0.4
None
0.2
1.0
1.0
None
None
None
0.8
None
None
None
None
None
None
0.4
None
None
None
0.2
None
1.0
0.4
None
None
0.6
None
None
None
None
None
None
None
None
0.2
None
None
None
None
1.0
None
0.6
0.4
None
None
None
None
1.0
None
None
0.4
None
0.6
None
None
0.2
0.4
None
0.2
None
None
None
None
None
None
None
None
None
None
None
1.0
0.8
None
0.6
None
None
None
0.6
None
0.8
None
None
None
None
None
None
None
None
None
None
0.6
None
None
None
None
None
0.8
None
0.4
None
0.8
None
None
None
None
None
None
None
None
0.4
None
None
None
0.8
0.2
None
None
1.0
None
None
1.0
0.2
None
None
None
None
None
None
None
None
None
0.8
1.0
0.2
None
None
0.2
0.2
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.6
None
None
None
0.4
None
None
None
None
0.8
0.8
1.0
None
0.4
None
None
None
None
None
None
None
None
None
None
None
0.4
0.6
None
1.0
None
None
None
None
None
None
None
0.2
None
None
0.2
0.2
None
None
None
None
None
None
0.2
None
None
None
0.2
0.2
None
0.2
None
None
0.2
None
0.6
None
None
None
None
None
0.4
None
1.0
None
None
None
None
0.2
None
None
0.2
None
1.0
None
None
0.2
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
0.2
None
0.2
None
None
None
None
None
None
0.4
None
None
None
None
None
None
None
None
None
0.2
None
None
0.4
None
None
None
None
0.2
None
None
None
0.2
0.2
None
None
None
None
None
None
None
None
0.4
0.6
None
0.2
None
None
0.2
None
None
None
None
None
None
None
0.2
None
0.2
None
None
None
None
None
None
None
None
None
None
0.4
None
0.8
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
0.4
0.2
None
None
0.6
0.2
None
None
None
None
0.4
None
None
None
0.2
1.0
None
0.2
0.6
None
1.0
None
None
None
None
None
None
0.6
None
None
None
None
None
None
None
None
None
None
None
None
0.2
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
0.4
0.2
None
None
None
None
None
None
None
None
None
None
None
None
0.4
None
0.4
None
0.2
None
0.4
None
None
None
None
None
None
0.2
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
None
1.0
1.0
None
None
None
None
0.2
None
1.0
None
None
None
None
1.0
None
1.0
1.0
None
1.0
None
None
0.2
None
0.2
None
None
1.0
None
None
None
None
None
None
1.0
None
None
None
None
1.0
1.0
None
None
None
None
None
1.0
None
1.0
None
None
None
None
0.2
None
None
None
1.0
0.2
None
None
None
None
None
1.0
0.2
None
None
None
None
None
1.0
1.0
None
0.2
None
None
1.0
1.0
None
1.0
1.0
0.2
None
1.0
None
1.0
1.0
1.0
0.2
0.2
None
1.0
None
0.2
0.2
1.0
1.0
1.0
1.0
0.2
0.2
0.2
0.2
1.0
0.2
1.0
0.2
None
None
0.2
1.0
0.2
0.2
0.2
0.2
0.2
0.2
1.0
0.2
0.2
None
None
0.2
0.2
0.2
0.2
0.2

In [82]: sts_dict
Out[82]: 
{0.2: [615,
  [0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.083,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.1,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.143,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.067,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.118,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.17,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0],
  [0.8,
   0.5,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.43478260869565216,
   0.5,
   0.4,
   0.5714285714285715,
   0.3333333333333333,
   0.4,
   0.14285714285714288,
   0.4444444444444445,
   0.2,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.125,
   0.22222222222222224,
   0.6,
   0.5,
   0.6,
   0.4,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.5714285714285715,
   0.28571428571428575,
   0.5,
   0.42857142857142855,
   0.28571428571428575,
   0.375,
   0.25,
   0.375,
   0.5,
   0.2727272727272727,
   0.3333333333333333,
   0.28571428571428575,
   0.2222222222222222,
   0.380952380952381,
   0.2,
   0.28571428571428575,
   0.21428571428571427,
   0.17391304347826086,
   0.1,
   0.25,
   0.38461538461538464,
   0.16,
   0.36363636363636365,
   0.25,
   0.4,
   0.2727272727272727,
   0.16,
   0.4444444444444445,
   0.20689655172413793,
   0.3636363636363636,
   0.3,
   0.25,
   0.20000000000000004,
   0.25,
   0.14285714285714288,
   0.22222222222222224,
   0.3529411764705882,
   0.10526315789473685,
   0.3870967741935484,
   0.25,
   0.3333333333333333,
   0.2631578947368421,
   0.28571428571428575,
   0.3157894736842105,
   0.15384615384615383,
   0.23529411764705885,
   0.18749999999999997,
   0.2105263157894737,
   0.18181818181818182,
   0.3,
   0.13793103448275862,
   0.2105263157894737,
   0.28571428571428575,
   0.07142857142857142,
   0.31250000000000006,
   0.16666666666666666,
   0.1818181818181818,
   0.3846153846153846,
   0.17543859649122806,
   0.18867924528301885,
   0.20408163265306123,
   0.22857142857142854,
   0.163265306122449,
   0.17777777777777778,
   0.11764705882352941,
   0.25,
   0.12903225806451615,
   0.17142857142857143,
   0.1886792452830189,
   0.22857142857142854,
   0.2711864406779661,
   0.22727272727272727,
   0.24999999999999994,
   0.1923076923076923,
   0.35000000000000003,
   0.13333333333333333,
   0.3018867924528302,
   0.23529411764705882,
   0.22950819672131148,
   0.2909090909090909,
   0.22857142857142856,
   0.13043478260869565,
   0.13793103448275862,
   0.2,
   0.13333333333333333,
   0.3225806451612903,
   0.25,
   0.1694915254237288,
   0.23076923076923078,
   0.09523809523809522,
   0.23529411764705882,
   0.2105263157894737,
   0.3333333333333333,
   0.27027027027027023,
   0.21739130434782608,
   0.2222222222222222,
   0.15384615384615383,
   0.2,
   0.24000000000000002,
   0.3225806451612903,
   0.27027027027027023,
   0.11320754716981131,
   0.24242424242424243,
   0.3255813953488372,
   0.24242424242424243,
   0.12244897959183673,
   0.16666666666666663,
   0.13636363636363638,
   0.2222222222222222,
   0.1754385964912281,
   0.16666666666666666,
   0.23529411764705882,
   0.45454545454545453,
   0.27027027027027023,
   0.16666666666666663,
   0.14285714285714288,
   0.2711864406779661,
   0.25925925925925924,
   0.23809523809523808,
   0.25,
   0.2191780821917808,
   0.20408163265306123,
   0.2631578947368421,
   0.20512820512820512,
   0.23529411764705882,
   0.41025641025641024,
   0.3571428571428571,
   0.2,
   0.33333333333333337,
   0.38888888888888884,
   0.2857142857142857,
   0.4186046511627907,
   0.4285714285714286,
   0.37209302325581395,
   0.3448275862068966,
   0.30303030303030304,
   0.42105263157894735,
   0.39999999999999997,
   0.5625,
   0.4666666666666667,
   0.25641025641025644,
   0.16,
   0.4375,
   0.26315789473684204,
   0.5365853658536585,
   0.23529411764705882,
   0.3428571428571428,
   0.4571428571428572,
   0.4090909090909091,
   0.4313725490196078,
   0.8,
   0.5,
   0.5,
   0.5,
   0.6666666666666666,
   0.5,
   0.6,
   0.4,
   0.5,
   0.6666666666666666,
   0.3333333333333333,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.30769230769230765,
   0.39999999999999997,
   0.28571428571428575,
   0.5,
   0.4,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.28571428571428575,
   0.3333333333333333,
   0.28571428571428575,
   0.26666666666666666,
   0.39999999999999997,
   0.26666666666666666,
   0.42857142857142855,
   0.380952380952381,
   0.2857142857142857,
   0.1739130434782609,
   0.4,
   0.28571428571428575,
   0.3157894736842105,
   0.5333333333333333,
   0.28571428571428575,
   0.3333333333333333,
   0.3157894736842105,
   0.3333333333333333,
   0.4,
   0.25,
   0.3,
   0.16,
   0.21052631578947364,
   0.37499999999999994,
   0.25,
   0.30769230769230765,
   0.3333333333333333,
   0.42857142857142855,
   0.39999999999999997,
   0.75,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.5714285714285715,
   0.2857142857142857,
   0.4705882352941177,
   0.4,
   0.5,
   0.5714285714285715,
   0.5,
   0.5,
   0.16666666666666666,
   0.42857142857142855,
   0.3636363636363636,
   0.375,
   0.4,
   0.42857142857142855,
   0.26666666666666666,
   0.42857142857142855,
   0.3333333333333333,
   0.42857142857142855,
   0.13333333333333333,
   0.26666666666666666,
   0.28571428571428575,
   0.4444444444444445,
   0.42857142857142855,
   0.5,
   0.4,
   0.28571428571428575,
   0.35294117647058826,
   0.5,
   0.26666666666666666,
   0.37499999999999994,
   0.5,
   0.37499999999999994,
   0.23529411764705885,
   0.3333333333333333,
   0.4,
   0.3333333333333333,
   0.42857142857142855,
   0.3333333333333333,
   0.5,
   0.3333333333333333,
   0.3333333333333333,
   0.37499999999999994,
   0.375,
   0.4,
   0.37499999999999994,
   0.42857142857142855,
   0.37499999999999994,
   0.2105263157894737,
   0.3157894736842105,
   0.375,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.375,
   0.28571428571428575,
   0.5555555555555556,
   0.2758620689655172,
   0.25,
   0.20000000000000004,
   0.25,
   0.34285714285714286,
   0.11111111111111112,
   0.1818181818181818,
   0.19354838709677416,
   0.47058823529411764,
   0.21428571428571427,
   0.16666666666666666,
   0.32,
   0.4210526315789474,
   0.3333333333333333,
   0.22222222222222224,
   0.25,
   0.3636363636363636,
   0.11764705882352942,
   0.3,
   0.3,
   0.4,
   0.2758620689655172,
   0.4166666666666667,
   0.3181818181818182,
   0.25,
   0.28571428571428575,
   0.2727272727272727,
   0.37499999999999994,
   0.3157894736842105,
   0.18749999999999997,
   0.27586206896551724,
   0.42857142857142855,
   0.3157894736842105,
   0.29411764705882354,
   0.31250000000000006,
   0.5217391304347826,
   0.3,
   0.24000000000000002,
   0.17391304347826086,
   0.4444444444444445,
   0.4,
   0.19999999999999998,
   0.375,
   0.33333333333333337,
   0.43478260869565216,
   0.33333333333333337,
   0.380952380952381,
   0.42857142857142855,
   0.09090909090909091,
   0.5,
   0.20689655172413793,
   0.5555555555555556,
   0.07142857142857144,
   0.25,
   0.3478260869565218,
   0.18181818181818182,
   0.16666666666666666,
   0.29629629629629634,
   0.4000000000000001,
   0.25,
   0.26666666666666666,
   0.2727272727272727,
   0.16,
   0.1904761904761905,
   0.19354838709677422,
   0.3870967741935483,
   0.3333333333333333,
   0.24000000000000002,
   0.28571428571428564,
   0.14285714285714288,
   0.5,
   0.24999999999999994,
   0.32,
   0.37499999999999994,
   0.3225806451612903,
   0.31250000000000006,
   0.08695652173913043,
   0.17391304347826086,
   0.3,
   0.3076923076923077,
   0.27586206896551724,
   0.2777777777777778,
   0.2857142857142857,
   0.33333333333333326,
   0.36363636363636365,
   0.4000000000000001,
   0.33333333333333326,
   0.4666666666666667,
   0.21428571428571427,
   0.19047619047619047,
   0.5,
   0.23999999999999996,
   0.2,
   0.375,
   0.22222222222222224,
   0.21428571428571427,
   0.3636363636363636,
   0.3333333333333333,
   0.2631578947368421,
   0.3333333333333333,
   0.22857142857142854,
   0.26086956521739135,
   0.48,
   0.30769230769230765,
   0.23076923076923075,
   0.375,
   0.3,
   0.25,
   0.16666666666666663,
   0.16,
   0.28571428571428575,
   0.24242424242424246,
   0.15384615384615385,
   0.5333333333333333,
   0.33333333333333337,
   0.3157894736842105,
   0.2608695652173913,
   0.6666666666666665,
   0.3225806451612903,
   0.23076923076923075,
   0.25,
   0.4000000000000001,
   0.23076923076923075,
   0.2,
   0.6206896551724138,
   0.41025641025641024,
   0.25,
   0.5517241379310344,
   0.3636363636363636,
   0.4680851063829788,
   0.15384615384615383,
   0.26666666666666666,
   0.631578947368421,
   0.5,
   0.5161290322580646,
   0.5625,
   0.39999999999999997,
   0.4390243902439024,
   0.631578947368421,
   0.6153846153846153,
   0.36842105263157887,
   0.42105263157894735,
   0.22857142857142856,
   0.4666666666666667,
   0.3414634146341463,
   0.2857142857142857,
   0.30769230769230765,
   0.4375,
   0.30769230769230765,
   0.3,
   0.27777777777777773,
   0.42857142857142855,
   0.3225806451612903,
   0.13333333333333333,
   0.4444444444444444,
   0.625,
   0.14814814814814814,
   0.3870967741935483,
   0.25,
   0.36363636363636365,
   0.3333333333333333,
   0.36363636363636365,
   0.35714285714285715,
   0.3111111111111111,
   0.2162162162162162,
   0.25641025641025644,
   0.5853658536585366,
   0.411764705882353,
   0.6666666666666666,
   0.22222222222222224,
   0.7199999999999999,
   0.4,
   0.26666666666666666,
   0.3333333333333333,
   0.5416666666666667,
   0.16,
   0.22857142857142856,
   0.3333333333333333,
   0.3333333333333333,
   0.4,
   0.18181818181818182,
   0.3076923076923077,
   0.3870967741935484,
   0.3448275862068966,
   0.3225806451612903,
   0.43902439024390244,
   0.34285714285714286,
   0.4210526315789474,
   0.35000000000000003,
   0.46808510638297873,
   0.34285714285714286,
   0.24999999999999994,
   0.358974358974359,
   0.4,
   0.6153846153846153,
   0.375,
   0.22222222222222224,
   0.358974358974359,
   0.34782608695652173,
   0.35294117647058826,
   0.3448275862068966,
   0.5581395348837209,
   0.43999999999999995,
   0.2424242424242424,
   0.23076923076923075,
   0.13333333333333333,
   0.13333333333333333,
   0.45161290322580644,
   0.33333333333333326,
   0.3684210526315789,
   0.6842105263157895,
   0.4864864864864865,
   0.5217391304347826,
   0.35294117647058826,
   0.26666666666666666,
   0.26666666666666666,
   0.4897959183673469,
   0.3333333333333333,
   0.6060606060606061,
   0.7027027027027027,
   0.22857142857142856,
   0.5306122448979592,
   0.3448275862068966,
   0.16666666666666666,
   0.4074074074074074,
   0.2631578947368421,
   0.3181818181818182,
   0.7647058823529412,
   0.3,
   0.4090909090909091,
   0.18181818181818182,
   0.39999999999999997,
   0.22857142857142856,
   0.47058823529411764,
   0.3333333333333333,
   0.3,
   0.1904761904761905,
   0.35294117647058826,
   0.3333333333333333,
   0.5106382978723405,
   0.2777777777777778,
   0.3888888888888889,
   0.3125,
   0.24242424242424243,
   0.3333333333333333,
   0.3888888888888889,
   0.4081632653061225,
   0.6046511627906976,
   0.45,
   0.5555555555555556,
   0.11764705882352941,
   0.29411764705882354,
   0.34285714285714286,
   0.6666666666666666,
   0.5957446808510638,
   0.4166666666666667,
   0.6818181818181819,
   0.6382978723404256,
   0.8181818181818182,
   0.5217391304347826,
   0.4615384615384615,
   0.52,
   0.6285714285714286,
   0.5,
   0.4848484848484849,
   0.14814814814814817,
   0.4444444444444444,
   0.4150943396226415,
   0.5714285714285715,
   0.4864864864864864,
   0.375,
   0.36,
   0.29411764705882354,
   0.46511627906976744,
   0.558139534883721,
   0.4444444444444445,
   0.3333333333333333,
   0.38095238095238093,
   0.42424242424242425,
   0.41025641025641024,
   0.34285714285714286,
   0.3333333333333333,
   0.47619047619047616,
   0.30769230769230765,
   0.1904761904761905]],
 None: [5757,
  [5.0,
   4.75,
   5.0,
   2.4,
   2.75,
   2.615,
   5.0,
   2.333,
   3.75,
   5.0,
   3.2,
   1.583,
   5.0,
   5.0,
   4.909,
   2.4,
   5.0,
   4.0,
   3.0,
   1.714,
   3.2,
   2.167,
   1.917,
   4.25,
   3.0,
   2.6,
   5.0,
   4.6,
   5.0,
   4.8,
   3.8,
   5.0,
   5.0,
   4.2,
   1.4,
   3.6,
   2.8,
   1.6,
   3.0,
   1.4,
   4.0,
   4.5,
   3.8,
   4.8,
   5.0,
   1.2,
   3.8,
   3.5,
   4.5,
   2.8,
   3.8,
   3.8,
   4.0,
   4.25,
   2.812,
   4.25,
   3.0,
   3.75,
   4.0,
   2.8,
   3.75,
   1.154,
   2.75,
   2.8,
   3.4,
   5.0,
   2.25,
   2.75,
   4.5,
   2.6,
   3.8,
   2.8,
   1.6,
   1.333,
   2.6,
   3.0,
   3.2,
   2.0,
   3.0,
   3.091,
   2.75,
   1.2,
   4.0,
   3.4,
   2.4,
   1.8,
   2.5,
   4.5,
   3.6,
   5.0,
   5.0,
   5.0,
   5.0,
   3.8,
   5.0,
   2.5,
   3.824,
   1.6,
   5.0,
   5.0,
   2.375,
   5.0,
   1.25,
   1.25,
   3.0,
   2.167,
   1.4,
   4.0,
   3.6,
   4.857,
   1.3,
   1.2,
   1.2,
   4.4,
   1.8,
   1.4,
   4.4,
   3.25,
   2.25,
   2.75,
   2.0,
   3.75,
   1.8,
   4.333,
   4.214,
   3.4,
   4.2,
   4.2,
   2.75,
   2.2,
   1.2,
   1.533,
   3.0,
   3.8,
   3.0,
   3.4,
   3.8,
   1.4,
   3.4,
   3.2,
   2.333,
   3.0,
   3.75,
   2.5,
   1.8,
   2.5,
   1.2,
   2.75,
   3.0,
   3.2,
   1.25,
   5.0,
   3.0,
   1.4,
   3.8,
   2.75,
   2.8,
   2.6,
   2.0,
   3.75,
   3.1,
   2.692,
   4.429,
   5.0,
   1.333,
   3.4,
   2.2,
   3.6,
   1.4,
   2.2,
   3.8,
   2.6,
   4.0,
   2.25,
   3.2,
   3.8,
   4.2,
   3.6,
   2.0,
   4.2,
   3.4,
   3.0,
   3.4,
   3.6,
   3.0,
   2.4,
   2.0,
   4.0,
   4.0,
   4.2,
   2.2,
   3.8,
   3.2,
   4.4,
   1.4,
   2.6,
   3.2,
   4.6,
   1.2,
   3.8,
   3.2,
   2.6,
   5.0,
   3.2,
   4.0,
   1.2,
   4.4,
   3.4,
   4.4,
   4.6,
   4.2,
   3.2,
   1.4,
   3.2,
   1.8,
   1.8,
   3.8,
   3.8,
   4.0,
   3.2,
   1.6,
   3.6,
   3.6,
   2.0,
   3.6,
   4.0,
   3.6,
   3.2,
   2.8,
   2.4,
   3.6,
   1.8,
   3.4,
   1.2,
   1.4,
   2.6,
   2.4,
   4.0,
   3.0,
   4.0,
   4.0,
   2.0,
   4.0,
   2.2,
   2.2,
   3.4,
   3.2,
   4.0,
   3.2,
   3.8,
   3.0,
   4.0,
   2.2,
   3.4,
   3.8,
   4.8,
   3.0,
   4.2,
   4.2,
   4.2,
   4.6,
   5.0,
   3.2,
   2.6,
   2.2,
   4.6,
   5.0,
   4.6,
   4.6,
   4.8,
   2.2,
   4.8,
   1.2,
   2.2,
   4.6,
   2.6,
   3.6,
   2.4,
   4.8,
   5.0,
   3.2,
   1.8,
   3.2,
   3.4,
   4.8,
   4.2,
   2.6,
   2.2,
   1.4,
   2.6,
   1.2,
   1.8,
   4.0,
   3.0,
   4.0,
   1.4,
   2.4,
   2.8,
   4.6,
   4.2,
   3.2,
   1.2,
   1.8,
   2.6,
   1.6,
   3.8,
   4.0,
   4.8,
   2.4,
   5.0,
   3.6,
   2.4,
   4.2,
   4.2,
   3.2,
   1.6,
   1.4,
   4.8,
   4.0,
   3.0,
   1.6,
   4.4,
   4.8,
   2.4,
   3.0,
   2.0,
   4.6,
   5.0,
   1.4,
   3.0,
   2.6,
   1.2,
   5.0,
   3.4,
   2.0,
   2.4,
   2.2,
   3.8,
   2.2,
   4.6,
   2.8,
   2.0,
   4.2,
   4.5,
   1.8,
   4.2,
   4.2,
   1.4,
   3.6,
   5.0,
   1.8,
   2.8,
   1.8,
   1.4,
   1.8,
   2.4,
   1.6,
   3.8,
   4.8,
   4.0,
   3.4,
   3.0,
   1.8,
   2.2,
   3.6,
   3.8,
   4.2,
   1.2,
   3.4,
   2.4,
   3.2,
   2.2,
   4.4,
   2.6,
   3.2,
   2.2,
   5.0,
   5.0,
   2.2,
   2.2,
   2.0,
   1.2,
   4.0,
   4.2,
   3.4,
   4.0,
   4.8,
   4.4,
   3.0,
   4.6,
   1.4,
   3.0,
   1.6,
   2.4,
   1.6,
   1.6,
   2.2,
   2.0,
   4.8,
   2.0,
   3.8,
   2.2,
   2.0,
   4.0,
   4.6,
   1.4,
   1.2,
   1.6,
   3.0,
   2.4,
   4.6,
   4.8,
   5.0,
   3.6,
   4.4,
   4.6,
   2.8,
   4.0,
   5.0,
   1.6,
   1.6,
   3.6,
   3.0,
   2.8,
   1.4,
   2.8,
   3.0,
   1.6,
   2.8,
   4.0,
   2.0,
   4.4,
   4.6,
   2.4,
   4.4,
   3.8,
   1.4,
   2.8,
   3.0,
   1.6,
   2.6,
   1.6,
   3.0,
   3.0,
   3.2,
   3.0,
   2.4,
   3.6,
   1.2,
   3.0,
   4.4,
   3.2,
   3.4,
   3.4,
   3.6,
   1.6,
   3.2,
   2.0,
   1.4,
   2.0,
   2.6,
   4.2,
   2.8,
   2.0,
   2.6,
   2.6,
   2.6,
   1.6,
   1.8,
   3.8,
   1.6,
   3.2,
   2.6,
   3.0,
   1.4,
   1.6,
   1.6,
   1.8,
   1.8,
   1.4,
   2.6,
   2.0,
   1.4,
   1.4,
   1.8,
   4.0,
   2.8,
   2.6,
   2.6,
   4.4,
   2.2,
   1.6,
   1.8,
   3.8,
   3.0,
   1.4,
   3.0,
   3.6,
   3.4,
   2.8,
   4.2,
   4.2,
   1.8,
   2.0,
   1.6,
   2.6,
   3.2,
   2.2,
   1.5,
   4.0,
   1.8,
   1.6,
   2.4,
   2.0,
   1.6,
   2.0,
   3.2,
   2.0,
   2.4,
   1.6,
   3.8,
   1.2,
   2.0,
   2.0,
   3.4,
   2.6,
   2.8,
   2.0,
   1.6,
   1.4,
   1.2,
   2.2,
   2.6,
   3.0,
   2.2,
   1.8,
   1.6,
   2.8,
   2.8,
   1.6,
   1.4,
   1.4,
   3.0,
   3.2,
   2.8,
   3.4,
   2.0,
   2.8,
   4.2,
   3.2,
   4.8,
   3.8,
   1.8,
   2.6,
   1.6,
   1.4,
   2.0,
   1.8,
   1.2,
   2.2,
   3.2,
   1.4,
   1.4,
   1.6,
   2.8,
   1.8,
   2.6,
   2.4,
   2.8,
   2.0,
   3.0,
   2.6,
   1.8,
   3.8,
   3.0,
   1.4,
   1.6,
   3.4,
   3.6,
   2.2,
   3.0,
   1.8,
   2.4,
   2.6,
   1.4,
   1.6,
   1.6,
   1.4,
   2.8,
   3.8,
   3.4,
   2.0,
   3.8,
   1.8,
   1.8,
   1.2,
   3.0,
   3.8,
   3.2,
   2.6,
   3.0,
   2.6,
   1.8,
   2.6,
   1.6,
   2.6,
   1.2,
   2.4,
   2.6,
   4.0,
   3.6,
   2.6,
   1.6,
   4.0,
   3.0,
   2.0,
   3.2,
   2.8,
   2.6,
   2.8,
   3.2,
   3.6,
   2.2,
   2.6,
   3.0,
   2.2,
   3.4,
   2.2,
   1.8,
   1.6,
   2.8,
   1.67,
   1.8,
   2.8,
   1.8,
   1.4,
   2.2,
   1.8,
   4.0,
   4.2,
   4.4,
   3.0,
   2.6,
   3.2,
   2.6,
   1.2,
   3.0,
   2.6,
   1.2,
   2.8,
   1.8,
   3.0,
   2.4,
   2.6,
   3.6,
   1.8,
   1.6,
   2.0,
   2.0,
   2.6,
   1.8,
   1.6,
   2.8,
   2.6,
   3.4,
   1.6,
   4.0,
   1.8,
   1.4,
   1.2,
   3.6,
   3.0,
   1.2,
   1.8,
   1.2,
   3.2,
   3.6,
   5.0,
   1.4,
   2.6,
   2.0,
   3.75,
   4.0,
   3.75,
   3.2,
   4.0,
   2.4,
   4.4,
   4.2,
   3.2,
   3.0,
   3.2,
   3.8,
   3.0,
   2.4,
   5.0,
   3.8,
   3.2,
   3.8,
   3.8,
   3.75,
   3.2,
   3.4,
   4.6,
   3.333,
   3.5,
   1.75,
   3.0,
   4.4,
   3.8,
   3.0,
   4.5,
   2.2,
   4.0,
   4.6,
   3.5,
   3.0,
   4.0,
   4.333,
   3.25,
   3.25,
   1.75,
   4.4,
   3.0,
   3.0,
   3.25,
   4.4,
   5.0,
   5.0,
   3.2,
   2.2,
   3.25,
   3.75,
   3.2,
   4.4,
   2.6,
   3.5,
   3.75,
   3.5,
   4.25,
   2.4,
   3.25,
   3.8,
   3.4,
   3.5,
   2.4,
   3.8,
   3.8,
   4.0,
   3.4,
   3.25,
   4.6,
   3.714,
   3.333,
   3.4,
   2.8,
   3.0,
   3.0,
   3.75,
   4.4,
   2.8,
   3.25,
   1.75,
   1.75,
   5.0,
   3.6,
   3.0,
   2.8,
   3.6,
   3.0,
   5.0,
   3.5,
   4.5,
   4.8,
   3.5,
   3.692,
   4.0,
   3.5,
   4.75,
   3.2,
   2.6,
   3.0,
   3.25,
   2.2,
   3.5,
   4.75,
   3.2,
   3.25,
   3.75,
   3.0,
   2.6,
   3.25,
   3.4,
   1.333,
   5.0,
   4.0,
   3.6,
   3.5,
   3.0,
   1.667,
   3.75,
   2.25,
   4.2,
   3.6,
   3.4,
   3.0,
   3.25,
   3.6,
   3.0,
   1.75,
   3.25,
   4.4,
   2.8,
   2.75,
   3.0,
   3.6,
   3.0,
   2.0,
   3.0,
   4.4,
   2.4,
   4.4,
   4.4,
   2.6,
   3.0,
   4.5,
   3.0,
   1.75,
   2.0,
   2.4,
   4.8,
   4.0,
   4.0,
   4.4,
   4.2,
   3.6,
   2.5,
   1.5,
   5.0,
   3.75,
   1.75,
   4.4,
   3.0,
   3.8,
   3.25,
   2.75,
   3.4,
   3.2,
   2.0,
   3.0,
   3.25,
   5.0,
   3.333,
   3.6,
   3.8,
   3.0,
   4.25,
   3.5,
   3.2,
   2.4,
   4.0,
   4.667,
   3.333,
   3.0,
   3.25,
   4.0,
   3.5,
   2.0,
   3.6,
   3.4,
   3.5,
   2.4,
   3.5,
   2.8,
   4.8,
   3.0,
   3.4,
   3.25,
   4.75,
   3.6,
   4.2,
   2.0,
   3.8,
   1.6,
   3.25,
   5.0,
   3.417,
   2.75,
   4.111,
   3.6,
   3.6,
   4.333,
   3.2,
   2.25,
   4.5,
   2.75,
   4.0,
   3.4,
   2.2,
   3.25,
   3.667,
   4.75,
   3.5,
   3.0,
   3.25,
   3.6,
   3.8,
   3.333,
   4.25,
   1.75,
   2.75,
   3.25,
   2.5,
   3.091,
   4.4,
   4.8,
   5.0,
   3.0,
   3.2,
   4.4,
   1.8,
   4.0,
   4.6,
   1.8,
   1.2,
   4.6,
   1.4,
   3.2,
   2.8,
   3.8,
   3.8,
   4.2,
   1.6,
   3.8,
   1.4,
   3.6,
   1.8,
   3.8,
   1.6,
   2.33333333333333,
   3.6,
   3.4,
   2.6,
   2.2,
   2.6,
   4.8,
   4.8,
   4.8,
   2.6,
   1.6,
   2.2,
   1.2,
   3.4,
   3.2,
   3.2,
   1.8,
   1.2,
   1.6,
   4.8,
   3.6,
   3.8,
   3.0,
   3.6,
   4.4,
   2.0,
   2.4,
   3.2,
   3.4,
   2.8,
   3.2,
   1.8,
   2.8,
   3.4,
   4.6,
   3.8,
   1.6,
   2.6,
   4.2,
   4.4,
   2.2,
   2.6,
   2.8,
   4.0,
   3.2,
   1.8,
   2.6,
   2.75,
   3.2,
   1.8,
   4.2,
   4.2,
   2.6,
   4.2,
   2.0,
   5.0,
   3.8,
   1.6,
   3.4,
   1.4,
   3.8,
   ...],
  [0.7,
   0.8571428571428571,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.7692307692307692,
   0.6666666666666665,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.7777777777777777,
   1.0,
   0.6666666666666666,
   1.0,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.8333333333333334,
   0.8571428571428571,
   0.7777777777777777,
   0.75,
   0.6666666666666666,
   0.4444444444444445,
   1.0,
   0.8181818181818182,
   0.875,
   1.0,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   0.7777777777777777,
   0.6,
   0.6,
   0.7142857142857143,
   0.8333333333333334,
   0.5555555555555556,
   0.5555555555555556,
   0.5555555555555556,
   0.5555555555555556,
   0.7,
   0.7142857142857143,
   0.6666666666666666,
   0.7142857142857143,
   0.6,
   0.7142857142857143,
   0.6666666666666666,
   0.6086956521739131,
   0.8333333333333334,
   0.5,
   0.28571428571428575,
   0.5555555555555556,
   0.5555555555555556,
   0.64,
   0.4444444444444445,
   0.6666666666666665,
   0.375,
   0.5,
   0.625,
   0.5,
   0.42857142857142855,
   0.6956521739130435,
   0.4444444444444445,
   0.5714285714285715,
   0.8333333333333334,
   0.5714285714285715,
   0.5161290322580646,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.5,
   0.28571428571428564,
   0.7142857142857143,
   0.3333333333333333,
   0.888888888888889,
   0.625,
   0.5714285714285715,
   0.4,
   0.47058823529411764,
   0.34782608695652173,
   0.7142857142857143,
   0.4444444444444444,
   0.5714285714285715,
   0.3157894736842105,
   0.8333333333333334,
   0.8333333333333334,
   0.875,
   1.0,
   1.0,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.888888888888889,
   0.6666666666666666,
   0.8571428571428571,
   0.8571428571428571,
   0.8333333333333334,
   1.0,
   0.75,
   0.75,
   0.6666666666666666,
   0.8333333333333334,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.6666666666666665,
   0.75,
   0.75,
   0.5714285714285715,
   0.8333333333333334,
   0.6666666666666666,
   0.9166666666666666,
   0.7142857142857143,
   0.8333333333333334,
   0.6363636363636364,
   0.42857142857142855,
   0.7777777777777777,
   0.7142857142857143,
   0.8000000000000002,
   0.5714285714285715,
   0.5,
   0.7,
   0.5,
   0.4000000000000001,
   0.8333333333333334,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.7272727272727272,
   0.8,
   0.6,
   0.6666666666666667,
   0.7142857142857143,
   0.7142857142857143,
   0.5263157894736842,
   0.5333333333333333,
   0.5217391304347826,
   0.888888888888889,
   0.42857142857142855,
   0.5,
   0.5,
   0.5,
   0.631578947368421,
   0.4615384615384615,
   0.4761904761904762,
   0.3529411764705882,
   0.8333333333333334,
   0.5,
   0.33333333333333326,
   0.5,
   0.2857142857142857,
   0.37499999999999994,
   0.37499999999999994,
   0.6666666666666667,
   0.6,
   0.6153846153846153,
   0.5263157894736842,
   0.5714285714285715,
   0.8181818181818182,
   0.4,
   0.380952380952381,
   0.5,
   0.5,
   0.5555555555555556,
   0.4375,
   0.36363636363636365,
   0.5,
   0.4,
   0.5,
   0.3125,
   0.64,
   0.5,
   0.75,
   0.28571428571428575,
   0.5,
   0.15,
   0.33333333333333326,
   0.6060606060606061,
   0.6666666666666665,
   0.7368421052631577,
   0.6666666666666665,
   0.3,
   0.5555555555555556,
   0.6250000000000001,
   0.6363636363636365,
   0.625,
   0.7,
   0.7,
   0.6666666666666666,
   0.6,
   0.4444444444444445,
   0.5882352941176471,
   0.6153846153846153,
   0.625,
   0.4545454545454546,
   0.39999999999999997,
   0.75,
   0.9166666666666666,
   0.5714285714285714,
   0.7777777777777777,
   0.5,
   0.5599999999999999,
   0.3448275862068966,
   0.48484848484848486,
   0.8181818181818182,
   0.8750000000000001,
   0.625,
   0.5454545454545454,
   0.6666666666666667,
   0.4444444444444445,
   0.26666666666666666,
   0.75,
   0.3,
   0.3157894736842105,
   0.4000000000000001,
   0.45454545454545453,
   0.35294117647058826,
   0.4210526315789474,
   0.2631578947368421,
   0.5714285714285715,
   0.5555555555555556,
   0.5333333333333333,
   0.23076923076923078,
   0.36363636363636365,
   0.3243243243243243,
   0.4000000000000001,
   0.39999999999999997,
   0.6000000000000001,
   0.33333333333333326,
   0.3333333333333333,
   0.5,
   0.7777777777777777,
   0.7142857142857142,
   0.3448275862068965,
   0.8,
   0.30769230769230765,
   0.4444444444444445,
   0.4444444444444445,
   0.4444444444444445,
   0.6428571428571429,
   0.5555555555555556,
   0.7000000000000001,
   0.6666666666666665,
   0.5454545454545454,
   0.5,
   0.7826086956521738,
   0.6363636363636365,
   0.7428571428571429,
   0.888888888888889,
   0.5714285714285715,
   0.9285714285714286,
   0.4117647058823529,
   0.5,
   0.7692307692307693,
   0.875,
   0.6923076923076923,
   0.8888888888888888,
   0.44444444444444436,
   0.5454545454545454,
   0.5,
   0.9166666666666666,
   0.608695652173913,
   0.56,
   0.5714285714285715,
   0.8461538461538461,
   0.4166666666666667,
   0.7407407407407408,
   0.29787234042553196,
   0.5185185185185185,
   0.5714285714285715,
   0.32,
   0.6,
   0.5714285714285714,
   0.6666666666666667,
   0.7692307692307692,
   0.5,
   0.75,
   0.8,
   0.5833333333333334,
   0.875,
   0.6,
   0.6666666666666665,
   0.4615384615384615,
   0.3157894736842105,
   0.3,
   0.3157894736842105,
   0.4848484848484849,
   0.6000000000000001,
   0.6896551724137931,
   0.6363636363636364,
   0.25,
   0.26086956521739135,
   0.21428571428571427,
   0.8000000000000002,
   0.8333333333333333,
   0.5454545454545454,
   0.45454545454545453,
   0.7142857142857143,
   0.75,
   0.6250000000000001,
   0.7142857142857143,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666665,
   0.5454545454545454,
   0.6428571428571429,
   0.3333333333333333,
   0.8571428571428571,
   0.7333333333333334,
   0.8571428571428571,
   0.6,
   0.38888888888888884,
   1.0,
   0.7499999999999999,
   0.6666666666666666,
   0.5714285714285713,
   0.5925925925925926,
   0.875,
   0.35714285714285715,
   0.9,
   0.6666666666666667,
   0.8888888888888888,
   0.8333333333333334,
   0.14285714285714285,
   0.6315789473684211,
   0.5,
   0.3636363636363636,
   0.8000000000000002,
   0.4444444444444445,
   0.5833333333333334,
   0.3703703703703704,
   0.3846153846153846,
   0.42857142857142855,
   0.5882352941176471,
   0.6666666666666665,
   0.4117647058823529,
   0.5,
   0.6,
   0.380952380952381,
   0.25,
   0.8750000000000001,
   0.7777777777777778,
   0.4,
   0.3255813953488372,
   0.6363636363636365,
   0.7692307692307692,
   0.8,
   0.31578947368421056,
   0.4,
   0.42857142857142855,
   0.48648648648648646,
   0.6,
   0.6666666666666667,
   0.875,
   0.6,
   0.5833333333333334,
   0.24242424242424243,
   0.625,
   0.5555555555555556,
   0.5714285714285715,
   0.8095238095238096,
   0.8333333333333334,
   0.4150943396226415,
   0.5,
   0.5,
   0.875,
   0.6666666666666666,
   0.8571428571428571,
   0.7000000000000001,
   0.5,
   0.36363636363636365,
   0.4666666666666667,
   0.5333333333333333,
   0.5,
   0.4,
   0.4,
   0.46153846153846156,
   0.4,
   0.9375,
   0.75,
   0.28571428571428575,
   0.888888888888889,
   0.8571428571428571,
   0.4666666666666667,
   0.7741935483870968,
   0.380952380952381,
   0.5384615384615384,
   0.875,
   0.6153846153846153,
   0.5833333333333334,
   0.358974358974359,
   0.631578947368421,
   0.42105263157894735,
   0.6666666666666665,
   0.4444444444444444,
   0.8571428571428571,
   0.6666666666666665,
   0.3846153846153846,
   0.8571428571428571,
   0.6451612903225806,
   0.34285714285714286,
   0.4444444444444445,
   0.4,
   0.2631578947368421,
   0.875,
   0.5925925925925926,
   0.8571428571428571,
   0.4,
   0.4736842105263158,
   0.8571428571428571,
   1.0,
   0.18181818181818182,
   0.7,
   1.0,
   0.21621621621621623,
   0.5,
   0.625,
   0.7692307692307692,
   0.6,
   0.32,
   0.9,
   0.2,
   0.1875,
   0.625,
   0.5882352941176471,
   0.47058823529411764,
   0.8571428571428571,
   0.7777777777777778,
   0.75,
   0.5,
   0.9090909090909091,
   0.4081632653061225,
   0.56,
   0.38461538461538464,
   0.75,
   0.3157894736842105,
   0.25,
   0.8333333333333334,
   0.7142857142857143,
   0.5,
   0.339622641509434,
   0.35,
   0.32653061224489793,
   0.2105263157894737,
   0.3571428571428571,
   0.3076923076923077,
   0.375,
   0.23809523809523808,
   0.2631578947368421,
   0.28571428571428575,
   0.2105263157894737,
   0.425531914893617,
   0.2857142857142857,
   0.24999999999999994,
   0.23255813953488372,
   0.26865671641791045,
   0.1904761904761905,
   0.20408163265306123,
   0.17777777777777778,
   0.21739130434782608,
   0.25,
   0.15,
   0.2692307692307692,
   0.15,
   0.6530612244897959,
   0.2711864406779661,
   0.2222222222222222,
   0.24242424242424246,
   0.4444444444444444,
   0.20833333333333334,
   0.2105263157894737,
   0.3913043478260869,
   0.35294117647058826,
   0.26666666666666666,
   0.19607843137254902,
   0.125,
   0.21739130434782608,
   0.057142857142857134,
   0.208955223880597,
   0.3529411764705882,
   0.39999999999999997,
   0.5333333333333333,
   0.35000000000000003,
   0.3125,
   0.3913043478260869,
   0.40816326530612246,
   0.18181818181818182,
   0.07017543859649122,
   0.28571428571428575,
   0.16666666666666666,
   0.17857142857142855,
   0.3076923076923077,
   0.15789473684210525,
   0.16666666666666669,
   0.253968253968254,
   0.4489795918367347,
   0.37500000000000006,
   0.18867924528301888,
   0.24137931034482757,
   0.1923076923076923,
   0.14285714285714288,
   0.2580645161290323,
   0.1818181818181818,
   0.32,
   0.3846153846153846,
   0.30769230769230765,
   0.2,
   0.13636363636363638,
   0.1818181818181818,
   0.19230769230769232,
   0.25641025641025644,
   0.2222222222222222,
   0.16666666666666666,
   0.34782608695652173,
   0.16216216216216214,
   0.32558139534883723,
   0.14634146341463414,
   0.4545454545454545,
   0.411764705882353,
   0.5,
   0.25,
   0.21052631578947367,
   0.33333333333333326,
   0.1791044776119403,
   0.35294117647058826,
   0.3050847457627119,
   0.273972602739726,
   0.44897959183673464,
   0.372093023255814,
   0.26229508196721313,
   0.23809523809523808,
   0.40816326530612246,
   0.28571428571428575,
   0.391304347826087,
   0.3125,
   0.27586206896551724,
   0.339622641509434,
   0.35555555555555557,
   0.34285714285714286,
   0.15384615384615385,
   0.2666666666666666,
   0.21818181818181817,
   0.23529411764705882,
   0.2,
   0.23255813953488372,
   0.6206896551724139,
   0.3902439024390244,
   0.22857142857142854,
   0.2127659574468085,
   0.30188679245283023,
   0.21621621621621623,
   0.2857142857142857,
   0.25,
   0.2790697674418605,
   0.2666666666666666,
   0.28571428571428575,
   0.2413793103448276,
   0.1587301587301587,
   0.4,
   0.2807017543859649,
   0.17857142857142858,
   0.19230769230769232,
   0.33333333333333326,
   0.41025641025641024,
   0.3703703703703704,
   0.2941176470588235,
   0.2745098039215686,
   0.31818181818181823,
   0.5555555555555556,
   0.3333333333333333,
   0.27272727272727276,
   0.3243243243243243,
   0.17543859649122806,
   0.2941176470588235,
   0.18181818181818182,
   0.2380952380952381,
   0.15384615384615385,
   0.32142857142857145,
   0.1818181818181818,
   0.18181818181818185,
   0.17391304347826086,
   0.1724137931034483,
   0.25,
   0.5405405405405405,
   0.4666666666666667,
   0.30769230769230765,
   0.2580645161290323,
   0.41025641025641024,
   0.15,
   0.34615384615384615,
   0.21052631578947367,
   0.45714285714285713,
   0.40579710144927533,
   0.20408163265306123,
   0.20000000000000004,
   0.21621621621621623,
   0.3278688524590164,
   0.1917808219178082,
   0.23809523809523808,
   0.23333333333333334,
   0.16901408450704225,
   0.27450980392156865,
   0.22222222222222224,
   0.20000000000000004,
   0.3768115942028986,
   0.5945945945945946,
   0.37499999999999994,
   0.30188679245283023,
   0.4878048780487805,
   0.26666666666666666,
   0.2702702702702703,
   0.38461538461538464,
   0.2641509433962264,
   0.2857142857142857,
   0.39285714285714285,
   0.5306122448979592,
   0.4210526315789474,
   0.22222222222222224,
   0.2769230769230769,
   0.3666666666666667,
   0.15999999999999998,
   0.11320754716981131,
   0.37209302325581395,
   0.14285714285714285,
   0.14285714285714282,
   0.37837837837837834,
   0.4067796610169492,
   0.25,
   0.42105263157894735,
   0.3793103448275862,
   0.22727272727272727,
   0.25641025641025644,
   0.375,
   0.8823529411764706,
   0.5490196078431373,
   0.4761904761904762,
   0.36065573770491804,
   0.25925925925925924,
   0.3174603174603175,
   0.17647058823529413,
   0.2857142857142857,
   0.35294117647058826,
   0.20512820512820512,
   0.15999999999999998,
   0.35294117647058826,
   0.16666666666666666,
   0.2857142857142857,
   0.3404255319148936,
   0.43636363636363634,
   0.5789473684210527,
   0.20833333333333331,
   0.4827586206896552,
   0.34782608695652173,
   0.26666666666666666,
   0.23076923076923078,
   0.14545454545454545,
   0.11428571428571428,
   0.3013698630136986,
   0.5,
   0.2222222222222222,
   0.22222222222222224,
   0.3333333333333333,
   0.27450980392156865,
   0.19999999999999998,
   0.21276595744680848,
   0.3243243243243243,
   0.22727272727272724,
   0.2222222222222222,
   0.1818181818181818,
   0.1724137931034483,
   0.17777777777777778,
   0.5660377358490567,
   0.7142857142857143,
   0.7241379310344828,
   0.7042253521126761,
   0.5842696629213484,
   0.853658536585366,
   0.56,
   0.7012987012987012,
   0.2666666666666666,
   0.5714285714285714,
   0.5245901639344263,
   0.7777777777777778,
   0.8387096774193549,
   0.45161290322580644,
   0.5396825396825397,
   0.3870967741935483,
   0.6666666666666666,
   0.6545454545454545,
   0.6024096385542168,
   0.7058823529411765,
   0.6329113924050633,
   0.4301075268817204,
   0.44067796610169496,
   0.717948717948718,
   0.5116279069767442,
   0.5714285714285714,
   0.634920634920635,
   0.7605633802816901,
   0.7469879518072288,
   0.6451612903225806,
   0.42424242424242425,
   0.5714285714285715,
   0.8787878787878788,
   0.6067415730337078,
   0.6410256410256411,
   0.7368421052631577,
   0.625,
   0.7857142857142857,
   0.9459459459459459,
   0.6,
   0.7027027027027025,
   0.746268656716418,
   0.6885245901639345,
   0.6896551724137931,
   0.32727272727272727,
   0.5217391304347826,
   0.6530612244897959,
   0.8125,
   0.716417910447761,
   0.5454545454545455,
   0.5,
   0.8,
   0.7058823529411765,
   0.7457627118644068,
   0.5,
   0.6666666666666667,
   0.7666666666666666,
   0.4166666666666667,
   0.782608695652174,
   0.6382978723404256,
   0.6585365853658536,
   0.5633802816901409,
   0.5625,
   0.42500000000000004,
   0.49056603773584906,
   0.6842105263157894,
   0.65625,
   0.7333333333333333,
   0.45161290322580644,
   0.5666666666666667,
   0.48837209302325585,
   0.767123287671233,
   0.5977011494252873,
   0.5483870967741935,
   0.7297297297297297,
   0.7428571428571429,
   0.6779661016949153,
   0.509090909090909,
   0.48275862068965514,
   0.47058823529411764,
   0.5116279069767442,
   0.5581395348837209,
   0.5633802816901409,
   0.6153846153846153,
   0.7692307692307692,
   0.5263157894736842,
   0.48484848484848486,
   0.761904761904762,
   0.5882352941176471,
   0.8,
   0.6578947368421053,
   0.24390243902439024,
   0.48888888888888893,
   0.5970149253731343,
   0.9090909090909091,
   0.5128205128205129,
   0.6363636363636364,
   0.7631578947368423,
   0.5901639344262296,
   0.575,
   0.5757575757575757,
   0.6075949367088608,
   0.8524590163934426,
   0.5977011494252874,
   0.7692307692307693,
   0.5970149253731343,
   0.6370370370370371,
   0.5151515151515151,
   0.47887323943661964,
   0.8809523809523809,
   0.5625,
   0.8260869565217391,
   0.711111111111111,
   0.509090909090909,
   0.48387096774193544,
   0.48,
   0.759493670886076,
   0.5283018867924528,
   0.7142857142857142,
   0.46511627906976744,
   0.2553191489361702,
   0.4545454545454546,
   0.490566037735849,
   0.4137931034482759,
   0.72,
   0.3859649122807018,
   0.7415730337078651,
   0.8282828282828283,
   0.5970149253731343,
   0.42424242424242425,
   0.6666666666666666,
   0.7234042553191491,
   0.6000000000000001,
   0.6153846153846153,
   0.5365853658536585,
   0.7500000000000001,
   0.4210526315789474,
   0.45454545454545453,
   0.7472527472527473,
   0.7,
   0.3225806451612903,
   0.5866666666666667,
   0.6333333333333333,
   0.5964912280701755,
   0.6739130434782609,
   0.7294117647058824,
   0.6857142857142857,
   0.417910447761194,
   0.4528301886792453,
   0.4307692307692308,
   0.7407407407407408,
   0.4489795918367347,
   0.41025641025641024,
   0.4675324675324676,
   0.9534883720930233,
   0.72,
   0.490566037735849,
   0.7142857142857143,
   0.7323943661971832,
   0.7526881720430108,
   0.35000000000000003,
   0.23333333333333336,
   0.5970149253731343,
   0.42857142857142855,
   0.49056603773584906,
   0.7037037037037037,
   0.6756756756756758,
   0.6521739130434783,
   0.7466666666666666,
   0.5116279069767442,
   0.7671232876712328,
   0.5818181818181818,
   0.5454545454545455,
   0.5306122448979591,
   0.6153846153846154,
   0.9166666666666666,
   0.576923076923077,
   0.5666666666666667,
   0.5476190476190477,
   0.634920634920635,
   0.7555555555555556,
   0.5423728813559322,
   0.5263157894736841,
   0.5833333333333333,
   0.796116504854369,
   0.4,
   0.5084745762711865,
   0.6666666666666666,
   0.7692307692307693,
   0.7659574468085106,
   0.6111111111111112,
   0.34782608695652173,
   0.7241379310344828,
   0.4897959183673469,
   0.5176470588235293,
   0.5084745762711865,
   0.5806451612903226,
   0.7628865979381443,
   0.6024096385542168,
   0.509090909090909,
   0.634920634920635,
   0.5434782608695652,
   0.7012987012987012,
   0.547945205479452,
   0.5434782608695652,
   0.29787234042553196,
   0.6933333333333334,
   0.47457627118644063,
   0.5483870967741935,
   0.7272727272727273,
   0.5783132530120482,
   0.4000000000000001,
   0.676923076923077,
   0.46428571428571425,
   0.7529411764705882,
   0.8571428571428572,
   0.5373134328358209,
   0.6,
   0.7678571428571429,
   0.3636363636363636,
   0.4444444444444445,
   0.56,
   0.36363636363636365,
   0.6250000000000001,
   0.5263157894736842,
   0.8705882352941177,
   0.7547169811320756,
   0.5365853658536586,
   0.735294117647059,
   0.6933333333333334,
   0.7441860465116279,
   0.7951807228915663,
   0.6823529411764706,
   0.5853658536585366,
   0.5454545454545455,
   0.6415094339622641,
   0.7789473684210527,
   0.5777777777777778,
   0.6666666666666666,
   0.8214285714285715,
   0.9714285714285714,
   0.576923076923077,
   0.6181818181818182,
   0.8484848484848484,
   0.49122807017543857,
   0.4827586206896552,
   0.7692307692307693,
   0.56,
   0.4,
   1.0,
   0.6666666666666667,
   0.717948717948718,
   0.4444444444444445,
   0.6206896551724137,
   0.7142857142857143,
   0.625,
   0.6,
   0.8,
   0.3333333333333333,
   0.8125,
   0.5625,
   0.6571428571428571,
   0.7234042553191491,
   0.5531914893617023,
   0.6363636363636364,
   0.43243243243243246,
   0.75,
   0.6486486486486486,
   0.8333333333333333,
   0.8571428571428571,
   0.9285714285714286,
   0.875,
   0.56,
   0.4848484848484848,
   0.3636363636363636,
   0.46808510638297873,
   0.7692307692307692,
   0.5714285714285713,
   0.48000000000000004,
   0.31746031746031744,
   0.5263157894736842,
   0.625,
   0.6470588235294117,
   0.4666666666666666,
   0.6976744186046512,
   0.46808510638297873,
   0.6956521739130435,
   0.823529411764706,
   0.5945945945945945,
   0.5,
   0.42857142857142855,
   0.6250000000000001,
   0.41025641025641024,
   0.5714285714285715,
   0.6363636363636364,
   0.5384615384615385,
   0.7804878048780488,
   0.8571428571428572,
   0.9259259259259259,
   0.28571428571428575,
   0.5853658536585366,
   0.5641025641025642,
   0.8771929824561403,
   0.6222222222222223,
   0.7777777777777777,
   0.25,
   0.9090909090909091,
   0.6086956521739131,
   0.5333333333333333,
   0.6500000000000001,
   0.6545454545454547,
   0.65,
   0.7857142857142856,
   0.7894736842105263,
   0.8888888888888888,
   0.5,
   0.8648648648648648,
   0.5853658536585366,
   0.8400000000000001,
   0.7619047619047619,
   0.8000000000000002,
   0.65,
   0.8181818181818182,
   0.5294117647058824,
   ...]],
 0.8: [211,
  [0.8,
   0.636,
   0.8,
   0.8,
   0.778,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.67,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.667,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.643,
   0.75,
   0.8,
   0.727,
   0.8,
   0.8,
   0.8,
   0.8,
   0.667,
   0.8,
   0.8,
   0.75,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.8,
   0.75,
   0.8,
   0.8,
   0.75,
   0.75,
   0.75,
   0.75,
   0.8,
   0.667,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.75,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8],
  [0.6666666666666666,
   0.75,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.375,
   0.6666666666666666,
   0.5714285714285715,
   0.4444444444444444,
   0.6666666666666666,
   0.20000000000000004,
   0.5333333333333333,
   0.3636363636363636,
   0.3225806451612903,
   0.29629629629629634,
   0.21621621621621623,
   0.6,
   0.20689655172413793,
   0.6666666666666665,
   0.3684210526315789,
   0.3703703703703704,
   0.36363636363636365,
   0.3333333333333333,
   0.16666666666666666,
   0.3050847457627119,
   0.25,
   0.17142857142857143,
   0.2153846153846154,
   0.32727272727272727,
   0.2545454545454545,
   0.339622641509434,
   0.14634146341463417,
   0.1904761904761905,
   0.4,
   0.2,
   0.2222222222222222,
   0.3125,
   0.13333333333333333,
   0.5,
   0.3829787234042554,
   0.3255813953488372,
   0.29166666666666663,
   0.3684210526315789,
   0.375,
   0.5882352941176471,
   0.358974358974359,
   0.48648648648648646,
   0.6521739130434783,
   0.6111111111111112,
   0.5909090909090909,
   0.75,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.4444444444444445,
   0.6,
   0.5714285714285715,
   0.3529411764705882,
   0.6250000000000001,
   0.5714285714285715,
   0.5333333333333333,
   0.5714285714285715,
   0.4210526315789474,
   0.36363636363636365,
   0.5714285714285715,
   0.375,
   0.6666666666666665,
   0.5,
   0.75,
   0.6666666666666666,
   0.7142857142857143,
   0.5714285714285715,
   0.5,
   0.42857142857142855,
   0.5714285714285715,
   0.6,
   0.6666666666666666,
   0.3333333333333333,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.6,
   0.5,
   0.6153846153846153,
   0.6,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.5714285714285715,
   0.35294117647058826,
   0.5,
   0.4444444444444445,
   0.37499999999999994,
   0.6,
   0.28571428571428564,
   0.42857142857142855,
   0.4,
   0.5,
   0.4,
   0.4000000000000001,
   0.23076923076923078,
   0.3636363636363636,
   0.14285714285714288,
   0.625,
   0.30769230769230765,
   0.2857142857142857,
   0.625,
   0.6666666666666666,
   0.33333333333333326,
   0.5,
   0.2727272727272727,
   0.48484848484848486,
   0.6666666666666665,
   0.4444444444444445,
   0.3703703703703704,
   0.37499999999999994,
   0.6153846153846153,
   0.25,
   0.1875,
   0.41379310344827586,
   0.3333333333333333,
   0.3636363636363637,
   0.3,
   0.41379310344827586,
   0.2,
   0.3571428571428571,
   0.46153846153846156,
   0.5714285714285715,
   0.4666666666666667,
   0.35714285714285715,
   0.36363636363636365,
   0.47058823529411764,
   0.47058823529411764,
   0.5454545454545454,
   0.7450980392156864,
   0.7272727272727273,
   0.5925925925925926,
   0.5,
   0.4210526315789474,
   0.6666666666666665,
   0.23076923076923078,
   0.5,
   0.3888888888888889,
   0.5333333333333332,
   0.3255813953488372,
   0.23529411764705882,
   0.4814814814814815,
   0.7407407407407408,
   0.5531914893617023,
   0.4680851063829788,
   0.5,
   0.39024390243902435,
   0.6938775510204083,
   0.3448275862068966,
   0.5555555555555556,
   0.7142857142857142,
   0.5714285714285714,
   0.35,
   0.5454545454545455,
   0.5777777777777778,
   0.4,
   0.6190476190476191,
   0.6666666666666666,
   0.34285714285714286,
   0.7058823529411765,
   0.6086956521739131,
   0.29411764705882354,
   0.7500000000000001,
   0.3404255319148936,
   0.46511627906976744,
   0.37499999999999994,
   0.5142857142857143,
   0.625,
   0.3902439024390244,
   0.7741935483870969,
   0.6818181818181818,
   0.3529411764705882,
   0.39999999999999997,
   0.35897435897435903,
   0.5454545454545454,
   0.43749999999999994,
   0.5625,
   0.25925925925925924,
   0.43243243243243246,
   0.5625,
   0.5416666666666667,
   0.7368421052631577,
   0.33333333333333337,
   0.6315789473684211,
   0.5454545454545454,
   0.3,
   0.5161290322580646,
   0.3728813559322034,
   0.43749999999999994,
   0.7894736842105263,
   0.7333333333333334,
   0.7741935483870968,
   0.34146341463414637,
   0.5185185185185186,
   0.6666666666666666,
   0.5405405405405405,
   0.39999999999999997,
   0.6896551724137931,
   0.41025641025641024,
   0.3714285714285715]],
 1.0: [264,
  [1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.833,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.85,
   1.0,
   0.833,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.9,
   0.9,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.944,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.889,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0],
  [0.8333333333333334,
   0.6,
   0.6666666666666666,
   0.4210526315789474,
   0.4444444444444445,
   0.5714285714285715,
   0.6666666666666666,
   0.4666666666666667,
   0.3,
   0.36363636363636365,
   0.2,
   0.3157894736842105,
   0.6,
   0.35714285714285715,
   0.2962962962962963,
   0.3846153846153846,
   0.15384615384615383,
   0.35294117647058826,
   0.20689655172413793,
   0.14285714285714285,
   0.21739130434782608,
   0.10526315789473684,
   0.2790697674418605,
   0.2745098039215686,
   0.2127659574468085,
   0.25,
   0.23076923076923078,
   0.2790697674418605,
   0.1951219512195122,
   0.27777777777777773,
   0.2926829268292683,
   0.2857142857142857,
   0.09302325581395349,
   0.3829787234042554,
   0.3636363636363636,
   0.39024390243902435,
   0.5405405405405405,
   0.5128205128205129,
   0.2222222222222222,
   0.42424242424242425,
   0.25,
   0.6470588235294117,
   0.4,
   0.5217391304347826,
   0.358974358974359,
   0.372093023255814,
   0.6666666666666666,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6666666666666666,
   0.5,
   0.5,
   0.4,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.5882352941176471,
   0.4705882352941177,
   0.6666666666666666,
   0.6666666666666666,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.6153846153846153,
   0.5714285714285715,
   0.4,
   0.42857142857142855,
   0.6666666666666666,
   0.4615384615384615,
   0.47619047619047616,
   0.6666666666666666,
   0.5,
   0.37499999999999994,
   0.4444444444444444,
   0.42857142857142855,
   0.5333333333333333,
   0.4444444444444444,
   0.4166666666666667,
   0.47058823529411764,
   0.4761904761904762,
   0.35714285714285715,
   0.2758620689655172,
   0.5555555555555556,
   0.33333333333333326,
   0.36363636363636365,
   0.16,
   0.5,
   0.47058823529411764,
   0.375,
   0.0909090909090909,
   0.33333333333333326,
   0.375,
   0.34782608695652173,
   0.2222222222222222,
   0.23076923076923075,
   0.25,
   0.3076923076923077,
   0.22857142857142854,
   0.35714285714285715,
   0.5517241379310345,
   0.6666666666666666,
   0.2,
   0.18181818181818182,
   0.5,
   0.4000000000000001,
   0.1702127659574468,
   0.35294117647058826,
   0.6875,
   0.6,
   0.4210526315789474,
   0.47058823529411764,
   0.7142857142857143,
   0.6363636363636365,
   0.3157894736842105,
   0.8461538461538461,
   0.7142857142857143,
   0.4666666666666667,
   0.4666666666666667,
   0.8000000000000002,
   0.5,
   0.8648648648648649,
   0.6666666666666666,
   0.5454545454545455,
   0.6428571428571429,
   0.6,
   0.3404255319148936,
   0.3333333333333333,
   0.5483870967741935,
   0.617283950617284,
   0.4888888888888888,
   0.3636363636363636,
   0.4523809523809524,
   0.6666666666666666,
   0.5964912280701754,
   0.42857142857142855,
   0.3404255319148936,
   0.4,
   0.3555555555555555,
   0.4197530864197531,
   0.8461538461538461,
   0.45714285714285713,
   0.24615384615384617,
   0.4444444444444444,
   0.5405405405405405,
   0.5925925925925926,
   0.48484848484848486,
   0.4,
   0.358974358974359,
   0.6111111111111113,
   0.41666666666666663,
   0.4666666666666667,
   0.48000000000000004,
   0.5,
   0.35714285714285715,
   0.6,
   0.45,
   0.4375,
   0.6428571428571429,
   0.49056603773584906,
   0.31818181818181823,
   0.4888888888888889,
   0.6857142857142857,
   0.4516129032258065,
   0.6923076923076924,
   0.7741935483870968,
   0.5862068965517241,
   0.47058823529411764,
   0.47368421052631576,
   0.5806451612903225,
   0.76,
   0.5625000000000001,
   0.4255319148936171,
   0.3333333333333333,
   0.28571428571428575,
   0.375,
   0.6376811594202899,
   0.4878048780487805,
   0.7857142857142857,
   0.5925925925925927,
   0.5116279069767442,
   0.4090909090909091,
   0.3902439024390244,
   0.6666666666666666,
   0.5652173913043478,
   0.5714285714285713,
   0.5384615384615384,
   0.3636363636363636,
   0.6666666666666667,
   0.75,
   0.5128205128205129,
   0.6206896551724139,
   0.4827586206896552,
   0.4782608695652174,
   0.5,
   0.5263157894736842,
   0.4583333333333333,
   0.4897959183673469,
   0.875,
   0.4736842105263158,
   0.46511627906976744,
   0.5833333333333334,
   0.43902439024390244,
   0.6666666666666666,
   0.358974358974359,
   0.3448275862068966,
   0.606060606060606,
   0.42857142857142855,
   0.3636363636363636,
   0.6666666666666666,
   0.3428571428571428,
   0.425531914893617,
   0.5,
   0.3902439024390244,
   0.4117647058823529,
   0.2285714285714286,
   0.85,
   0.5500000000000002,
   0.3829787234042554,
   0.5652173913043479,
   0.3888888888888889,
   0.43478260869565216,
   0.3636363636363636,
   0.409090909090909,
   0.3888888888888889,
   0.5925925925925926,
   0.45454545454545453,
   0.358974358974359,
   0.358974358974359,
   0.52,
   0.5625000000000001,
   0.3,
   0.22727272727272727,
   0.40816326530612246,
   0.9090909090909091,
   0.8636363636363636,
   0.6976744186046512,
   0.7692307692307692,
   0.7857142857142856,
   0.6206896551724138,
   0.4242424242424242,
   0.4242424242424242,
   0.7857142857142857,
   0.6274509803921569,
   0.6666666666666666,
   0.46808510638297873,
   0.5,
   0.6285714285714287,
   0.6315789473684211,
   0.7222222222222222,
   0.48484848484848486,
   0.6875000000000001,
   0.358974358974359,
   0.4324324324324324,
   0.42857142857142855,
   0.46511627906976744,
   0.5945945945945946,
   0.4666666666666667,
   0.5762711864406779,
   0.7199999999999999]],
 0.6: [190,
  [0.6,
   0.5,
   0.6,
   0.6,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.5,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.5,
   0.417,
   0.5,
   0.6,
   0.6,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6],
  [0.5,
   0.5263157894736842,
   0.6666666666666666,
   0.5,
   0.5,
   0.6666666666666666,
   0.6,
   0.5,
   0.6,
   0.6666666666666666,
   0.5714285714285715,
   0.380952380952381,
   0.5714285714285715,
   0.47058823529411764,
   0.5,
   0.34782608695652173,
   0.28571428571428575,
   0.5263157894736842,
   0.1,
   0.25,
   0.5,
   0.5555555555555556,
   0.28571428571428575,
   0.2758620689655172,
   0.22222222222222224,
   0.23529411764705882,
   0.25,
   0.13793103448275862,
   0.26666666666666666,
   0.2,
   0.28571428571428575,
   0.17391304347826086,
   0.13953488372093023,
   0.3714285714285714,
   0.1081081081081081,
   0.21052631578947367,
   0.21818181818181817,
   0.21538461538461542,
   0.13043478260869565,
   0.10714285714285714,
   0.1702127659574468,
   0.0930232558139535,
   0.2647058823529412,
   0.42553191489361697,
   0.1818181818181818,
   0.21052631578947367,
   0.24137931034482757,
   0.2608695652173913,
   0.18518518518518517,
   0.5714285714285714,
   0.5625000000000001,
   0.39999999999999997,
   0.43902439024390244,
   0.38888888888888884,
   0.1904761904761905,
   0.75,
   0.75,
   0.75,
   0.75,
   0.6,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6153846153846153,
   0.625,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.5714285714285715,
   0.42857142857142855,
   0.39999999999999997,
   0.3333333333333333,
   0.5384615384615384,
   0.42857142857142855,
   0.5454545454545454,
   0.42857142857142855,
   0.6666666666666666,
   0.3333333333333333,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.5714285714285715,
   0.37499999999999994,
   0.5,
   0.5,
   0.5714285714285715,
   0.6,
   0.5,
   0.5,
   0.4615384615384615,
   0.5555555555555556,
   0.5714285714285715,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.2857142857142857,
   0.5,
   0.17647058823529413,
   0.1904761904761905,
   0.6,
   0.22727272727272727,
   0.21428571428571427,
   0.22222222222222224,
   0.20000000000000004,
   0.6666666666666666,
   0.45454545454545453,
   0.3703703703703704,
   0.27027027027027023,
   0.5,
   0.3636363636363636,
   0.08695652173913043,
   0.2105263157894737,
   0.38709677419354843,
   0.14634146341463414,
   0.29629629629629634,
   0.37499999999999994,
   0.24242424242424243,
   0.23076923076923075,
   0.6666666666666666,
   0.3333333333333333,
   0.2,
   0.35714285714285715,
   0.2,
   0.5,
   0.33333333333333337,
   0.5714285714285715,
   0.3157894736842105,
   0.46153846153846156,
   0.32653061224489793,
   0.7142857142857142,
   0.31249999999999994,
   0.5652173913043478,
   0.6666666666666666,
   0.4090909090909091,
   0.35714285714285715,
   0.16666666666666666,
   0.64,
   0.33333333333333337,
   0.6829268292682927,
   0.7500000000000001,
   0.5,
   0.2857142857142857,
   0.3636363636363636,
   0.6315789473684211,
   0.5625000000000001,
   0.6666666666666667,
   0.6451612903225806,
   0.28571428571428575,
   0.4814814814814815,
   0.5555555555555556,
   0.3225806451612903,
   0.37837837837837834,
   0.2580645161290323,
   0.5263157894736842,
   0.4489795918367347,
   0.2727272727272727,
   0.6829268292682927,
   0.851063829787234,
   0.3783783783783784,
   0.7916666666666667,
   0.42857142857142855,
   0.3255813953488372,
   0.2926829268292683,
   0.4137931034482759,
   0.42857142857142855,
   0.2857142857142857,
   0.6341463414634146,
   0.6428571428571429,
   0.26666666666666666,
   0.47058823529411764,
   0.45,
   0.5777777777777777,
   0.4444444444444444,
   0.30769230769230765,
   0.39999999999999997,
   0.6428571428571429,
   0.6829268292682927,
   0.7272727272727272,
   0.6875,
   0.4,
   0.7142857142857143,
   0.358974358974359,
   0.6111111111111113,
   0.6000000000000001,
   0.3846153846153846,
   0.4615384615384615,
   0.35,
   0.4615384615384615,
   0.4736842105263158]],
 0.4: [214,
  [0.25,
   0.25,
   0.25,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.333,
   0.333,
   0.25,
   0.4,
   0.4,
   0.25,
   0.25,
   0.4,
   0.4,
   0.4,
   0.25,
   0.25,
   0.25,
   0.4,
   0.25,
   0.25,
   0.4,
   0.25,
   0.4,
   0.25,
   0.4,
   0.4,
   0.25,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.231,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.25,
   0.333,
   0.4,
   0.25,
   0.333,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4],
  [0.5,
   0.4,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6153846153846153,
   0.375,
   0.28571428571428575,
   0.2,
   0.4444444444444445,
   0.5555555555555556,
   0.3448275862068965,
   0.36363636363636365,
   0.3243243243243243,
   0.34782608695652173,
   0.24242424242424246,
   0.20512820512820512,
   0.1379310344827586,
   0.3636363636363637,
   0.25,
   0.34285714285714286,
   0.33333333333333337,
   0.10526315789473685,
   0.29629629629629634,
   0.3,
   0.3,
   0.11320754716981132,
   0.22727272727272724,
   0.509090909090909,
   0.1904761904761905,
   0.22222222222222224,
   0.25,
   0.23809523809523808,
   0.22580645161290322,
   0.2,
   0.16,
   0.27906976744186046,
   0.19512195121951217,
   0.27027027027027023,
   0.1923076923076923,
   0.3673469387755102,
   0.04761904761904762,
   0.2285714285714286,
   0.3333333333333333,
   0.43749999999999994,
   0.5,
   0.3636363636363636,
   0.1764705882352941,
   0.4864864864864865,
   0.5,
   0.4680851063829788,
   0.6470588235294118,
   0.5652173913043479,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.26666666666666666,
   0.6666666666666666,
   0.6,
   0.5,
   0.5333333333333333,
   0.6666666666666666,
   0.4210526315789474,
   0.13333333333333333,
   0.375,
   0.42857142857142855,
   0.5,
   0.2857142857142857,
   0.5882352941176471,
   0.5,
   0.37499999999999994,
   0.6,
   0.28571428571428575,
   0.6666666666666666,
   0.6,
   0.6,
   0.5,
   0.3333333333333333,
   0.6153846153846153,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.6,
   0.5714285714285715,
   0.5,
   0.5714285714285715,
   0.5714285714285714,
   0.5714285714285715,
   0.5,
   0.5,
   0.375,
   0.3333333333333333,
   0.5,
   0.4,
   0.6666666666666666,
   0.25,
   0.4444444444444444,
   0.4705882352941177,
   0.6666666666666666,
   0.5,
   0.375,
   0.6666666666666666,
   0.5,
   0.375,
   0.28571428571428575,
   0.2857142857142857,
   0.5,
   0.5,
   0.3703703703703703,
   0.48000000000000004,
   0.42857142857142855,
   0.39999999999999997,
   0.30303030303030304,
   0.29411764705882354,
   0.3076923076923077,
   0.28571428571428575,
   0.25,
   0.47619047619047616,
   0.33333333333333326,
   0.26666666666666666,
   0.3,
   0.25,
   0.47058823529411764,
   0.4444444444444445,
   0.625,
   0.3,
   0.3636363636363637,
   0.18749999999999997,
   0.3333333333333333,
   0.26666666666666666,
   0.45454545454545453,
   0.22222222222222224,
   0.2727272727272727,
   0.30769230769230765,
   0.3,
   0.5714285714285714,
   0.24390243902439024,
   0.2,
   0.5806451612903225,
   0.14814814814814817,
   0.2857142857142857,
   0.3333333333333333,
   0.2380952380952381,
   0.5714285714285715,
   0.7407407407407408,
   0.75,
   0.5714285714285714,
   0.3333333333333333,
   0.3829787234042554,
   0.4680851063829787,
   0.8571428571428571,
   0.31250000000000006,
   0.5,
   0.3404255319148936,
   0.3902439024390244,
   0.4477611940298507,
   0.358974358974359,
   0.2727272727272727,
   0.5128205128205129,
   0.30769230769230765,
   0.33333333333333326,
   0.711111111111111,
   0.4090909090909091,
   0.22857142857142856,
   0.14814814814814814,
   0.35,
   0.35000000000000003,
   0.380952380952381,
   0.5555555555555556,
   0.8275862068965518,
   0.3829787234042554,
   0.34285714285714286,
   0.45,
   0.34782608695652173,
   0.4324324324324324,
   0.5789473684210527,
   0.45161290322580644,
   0.4864864864864865,
   0.48000000000000004,
   0.43750000000000006,
   0.3684210526315789,
   0.48484848484848486,
   0.27586206896551724,
   0.47619047619047616,
   0.5384615384615384,
   0.3636363636363636,
   0.42857142857142855,
   0.3243243243243243,
   0.3243243243243243,
   0.43750000000000006,
   0.45714285714285713,
   0.6428571428571429,
   0.7647058823529411,
   0.4444444444444445,
   0.3913043478260869,
   0.42857142857142855,
   0.4444444444444444,
   0.3571428571428571,
   0.5517241379310345,
   0.35294117647058826,
   0.5405405405405405,
   0.5806451612903226,
   0.37735849056603776,
   0.5,
   0.3414634146341463]]}

In [83]: count = 200
    ...: for i in sts_dict:
    ...:     temp_df = pd.DataFrame({})
    ...:     temp_df["sts_bucket"] = [i]*190
    ...:     temp_df["smatch"] = sts_dict[i][2][:190]
    ...:     temp_df["sts_score"] = sts_dict[i][1][:190]
    ...:     df = df.append(temp_df, ignore_index=True)
    ...: 
    ...: 
    ...: 
    ...: 

In [84]: df
Out[84]: 
      sts_bucket    smatch  sts_score
0            0.2  0.800000        NaN
1            0.2  0.500000        NaN
2            0.2  0.428571        NaN
3            0.2  0.500000        NaN
4            0.2  0.333333        NaN
...          ...       ...        ...
3955         0.4  0.451613        0.4
3956         0.4  0.486486        0.4
3957         0.4  0.480000        0.4
3958         0.4  0.437500        0.4
3959         0.4  0.368421        0.4

[3960 rows x 3 columns]

In [85]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [i], [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(i)
    ...:         sts_dict[k][2].append(smatch_scores[ind])
    ...: 

In [86]: 

In [86]: sts_dict
Out[86]: 
{0.2: [615,
  [0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.083,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.1,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.143,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.067,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.118,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.17,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0],
  [0.8,
   0.5,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.43478260869565216,
   0.5,
   0.4,
   0.5714285714285715,
   0.3333333333333333,
   0.4,
   0.14285714285714288,
   0.4444444444444445,
   0.2,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.125,
   0.22222222222222224,
   0.6,
   0.5,
   0.6,
   0.4,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.5714285714285715,
   0.28571428571428575,
   0.5,
   0.42857142857142855,
   0.28571428571428575,
   0.375,
   0.25,
   0.375,
   0.5,
   0.2727272727272727,
   0.3333333333333333,
   0.28571428571428575,
   0.2222222222222222,
   0.380952380952381,
   0.2,
   0.28571428571428575,
   0.21428571428571427,
   0.17391304347826086,
   0.1,
   0.25,
   0.38461538461538464,
   0.16,
   0.36363636363636365,
   0.25,
   0.4,
   0.2727272727272727,
   0.16,
   0.4444444444444445,
   0.20689655172413793,
   0.3636363636363636,
   0.3,
   0.25,
   0.20000000000000004,
   0.25,
   0.14285714285714288,
   0.22222222222222224,
   0.3529411764705882,
   0.10526315789473685,
   0.3870967741935484,
   0.25,
   0.3333333333333333,
   0.2631578947368421,
   0.28571428571428575,
   0.3157894736842105,
   0.15384615384615383,
   0.23529411764705885,
   0.18749999999999997,
   0.2105263157894737,
   0.18181818181818182,
   0.3,
   0.13793103448275862,
   0.2105263157894737,
   0.28571428571428575,
   0.07142857142857142,
   0.31250000000000006,
   0.16666666666666666,
   0.1818181818181818,
   0.3846153846153846,
   0.17543859649122806,
   0.18867924528301885,
   0.20408163265306123,
   0.22857142857142854,
   0.163265306122449,
   0.17777777777777778,
   0.11764705882352941,
   0.25,
   0.12903225806451615,
   0.17142857142857143,
   0.1886792452830189,
   0.22857142857142854,
   0.2711864406779661,
   0.22727272727272727,
   0.24999999999999994,
   0.1923076923076923,
   0.35000000000000003,
   0.13333333333333333,
   0.3018867924528302,
   0.23529411764705882,
   0.22950819672131148,
   0.2909090909090909,
   0.22857142857142856,
   0.13043478260869565,
   0.13793103448275862,
   0.2,
   0.13333333333333333,
   0.3225806451612903,
   0.25,
   0.1694915254237288,
   0.23076923076923078,
   0.09523809523809522,
   0.23529411764705882,
   0.2105263157894737,
   0.3333333333333333,
   0.27027027027027023,
   0.21739130434782608,
   0.2222222222222222,
   0.15384615384615383,
   0.2,
   0.24000000000000002,
   0.3225806451612903,
   0.27027027027027023,
   0.11320754716981131,
   0.24242424242424243,
   0.3255813953488372,
   0.24242424242424243,
   0.12244897959183673,
   0.16666666666666663,
   0.13636363636363638,
   0.2222222222222222,
   0.1754385964912281,
   0.16666666666666666,
   0.23529411764705882,
   0.45454545454545453,
   0.27027027027027023,
   0.16666666666666663,
   0.14285714285714288,
   0.2711864406779661,
   0.25925925925925924,
   0.23809523809523808,
   0.25,
   0.2191780821917808,
   0.20408163265306123,
   0.2631578947368421,
   0.20512820512820512,
   0.23529411764705882,
   0.41025641025641024,
   0.3571428571428571,
   0.2,
   0.33333333333333337,
   0.38888888888888884,
   0.2857142857142857,
   0.4186046511627907,
   0.4285714285714286,
   0.37209302325581395,
   0.3448275862068966,
   0.30303030303030304,
   0.42105263157894735,
   0.39999999999999997,
   0.5625,
   0.4666666666666667,
   0.25641025641025644,
   0.16,
   0.4375,
   0.26315789473684204,
   0.5365853658536585,
   0.23529411764705882,
   0.3428571428571428,
   0.4571428571428572,
   0.4090909090909091,
   0.4313725490196078,
   0.8,
   0.5,
   0.5,
   0.5,
   0.6666666666666666,
   0.5,
   0.6,
   0.4,
   0.5,
   0.6666666666666666,
   0.3333333333333333,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.30769230769230765,
   0.39999999999999997,
   0.28571428571428575,
   0.5,
   0.4,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.28571428571428575,
   0.3333333333333333,
   0.28571428571428575,
   0.26666666666666666,
   0.39999999999999997,
   0.26666666666666666,
   0.42857142857142855,
   0.380952380952381,
   0.2857142857142857,
   0.1739130434782609,
   0.4,
   0.28571428571428575,
   0.3157894736842105,
   0.5333333333333333,
   0.28571428571428575,
   0.3333333333333333,
   0.3157894736842105,
   0.3333333333333333,
   0.4,
   0.25,
   0.3,
   0.16,
   0.21052631578947364,
   0.37499999999999994,
   0.25,
   0.30769230769230765,
   0.3333333333333333,
   0.42857142857142855,
   0.39999999999999997,
   0.75,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.5714285714285715,
   0.2857142857142857,
   0.4705882352941177,
   0.4,
   0.5,
   0.5714285714285715,
   0.5,
   0.5,
   0.16666666666666666,
   0.42857142857142855,
   0.3636363636363636,
   0.375,
   0.4,
   0.42857142857142855,
   0.26666666666666666,
   0.42857142857142855,
   0.3333333333333333,
   0.42857142857142855,
   0.13333333333333333,
   0.26666666666666666,
   0.28571428571428575,
   0.4444444444444445,
   0.42857142857142855,
   0.5,
   0.4,
   0.28571428571428575,
   0.35294117647058826,
   0.5,
   0.26666666666666666,
   0.37499999999999994,
   0.5,
   0.37499999999999994,
   0.23529411764705885,
   0.3333333333333333,
   0.4,
   0.3333333333333333,
   0.42857142857142855,
   0.3333333333333333,
   0.5,
   0.3333333333333333,
   0.3333333333333333,
   0.37499999999999994,
   0.375,
   0.4,
   0.37499999999999994,
   0.42857142857142855,
   0.37499999999999994,
   0.2105263157894737,
   0.3157894736842105,
   0.375,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.375,
   0.28571428571428575,
   0.5555555555555556,
   0.2758620689655172,
   0.25,
   0.20000000000000004,
   0.25,
   0.34285714285714286,
   0.11111111111111112,
   0.1818181818181818,
   0.19354838709677416,
   0.47058823529411764,
   0.21428571428571427,
   0.16666666666666666,
   0.32,
   0.4210526315789474,
   0.3333333333333333,
   0.22222222222222224,
   0.25,
   0.3636363636363636,
   0.11764705882352942,
   0.3,
   0.3,
   0.4,
   0.2758620689655172,
   0.4166666666666667,
   0.3181818181818182,
   0.25,
   0.28571428571428575,
   0.2727272727272727,
   0.37499999999999994,
   0.3157894736842105,
   0.18749999999999997,
   0.27586206896551724,
   0.42857142857142855,
   0.3157894736842105,
   0.29411764705882354,
   0.31250000000000006,
   0.5217391304347826,
   0.3,
   0.24000000000000002,
   0.17391304347826086,
   0.4444444444444445,
   0.4,
   0.19999999999999998,
   0.375,
   0.33333333333333337,
   0.43478260869565216,
   0.33333333333333337,
   0.380952380952381,
   0.42857142857142855,
   0.09090909090909091,
   0.5,
   0.20689655172413793,
   0.5555555555555556,
   0.07142857142857144,
   0.25,
   0.3478260869565218,
   0.18181818181818182,
   0.16666666666666666,
   0.29629629629629634,
   0.4000000000000001,
   0.25,
   0.26666666666666666,
   0.2727272727272727,
   0.16,
   0.1904761904761905,
   0.19354838709677422,
   0.3870967741935483,
   0.3333333333333333,
   0.24000000000000002,
   0.28571428571428564,
   0.14285714285714288,
   0.5,
   0.24999999999999994,
   0.32,
   0.37499999999999994,
   0.3225806451612903,
   0.31250000000000006,
   0.08695652173913043,
   0.17391304347826086,
   0.3,
   0.3076923076923077,
   0.27586206896551724,
   0.2777777777777778,
   0.2857142857142857,
   0.33333333333333326,
   0.36363636363636365,
   0.4000000000000001,
   0.33333333333333326,
   0.4666666666666667,
   0.21428571428571427,
   0.19047619047619047,
   0.5,
   0.23999999999999996,
   0.2,
   0.375,
   0.22222222222222224,
   0.21428571428571427,
   0.3636363636363636,
   0.3333333333333333,
   0.2631578947368421,
   0.3333333333333333,
   0.22857142857142854,
   0.26086956521739135,
   0.48,
   0.30769230769230765,
   0.23076923076923075,
   0.375,
   0.3,
   0.25,
   0.16666666666666663,
   0.16,
   0.28571428571428575,
   0.24242424242424246,
   0.15384615384615385,
   0.5333333333333333,
   0.33333333333333337,
   0.3157894736842105,
   0.2608695652173913,
   0.6666666666666665,
   0.3225806451612903,
   0.23076923076923075,
   0.25,
   0.4000000000000001,
   0.23076923076923075,
   0.2,
   0.6206896551724138,
   0.41025641025641024,
   0.25,
   0.5517241379310344,
   0.3636363636363636,
   0.4680851063829788,
   0.15384615384615383,
   0.26666666666666666,
   0.631578947368421,
   0.5,
   0.5161290322580646,
   0.5625,
   0.39999999999999997,
   0.4390243902439024,
   0.631578947368421,
   0.6153846153846153,
   0.36842105263157887,
   0.42105263157894735,
   0.22857142857142856,
   0.4666666666666667,
   0.3414634146341463,
   0.2857142857142857,
   0.30769230769230765,
   0.4375,
   0.30769230769230765,
   0.3,
   0.27777777777777773,
   0.42857142857142855,
   0.3225806451612903,
   0.13333333333333333,
   0.4444444444444444,
   0.625,
   0.14814814814814814,
   0.3870967741935483,
   0.25,
   0.36363636363636365,
   0.3333333333333333,
   0.36363636363636365,
   0.35714285714285715,
   0.3111111111111111,
   0.2162162162162162,
   0.25641025641025644,
   0.5853658536585366,
   0.411764705882353,
   0.6666666666666666,
   0.22222222222222224,
   0.7199999999999999,
   0.4,
   0.26666666666666666,
   0.3333333333333333,
   0.5416666666666667,
   0.16,
   0.22857142857142856,
   0.3333333333333333,
   0.3333333333333333,
   0.4,
   0.18181818181818182,
   0.3076923076923077,
   0.3870967741935484,
   0.3448275862068966,
   0.3225806451612903,
   0.43902439024390244,
   0.34285714285714286,
   0.4210526315789474,
   0.35000000000000003,
   0.46808510638297873,
   0.34285714285714286,
   0.24999999999999994,
   0.358974358974359,
   0.4,
   0.6153846153846153,
   0.375,
   0.22222222222222224,
   0.358974358974359,
   0.34782608695652173,
   0.35294117647058826,
   0.3448275862068966,
   0.5581395348837209,
   0.43999999999999995,
   0.2424242424242424,
   0.23076923076923075,
   0.13333333333333333,
   0.13333333333333333,
   0.45161290322580644,
   0.33333333333333326,
   0.3684210526315789,
   0.6842105263157895,
   0.4864864864864865,
   0.5217391304347826,
   0.35294117647058826,
   0.26666666666666666,
   0.26666666666666666,
   0.4897959183673469,
   0.3333333333333333,
   0.6060606060606061,
   0.7027027027027027,
   0.22857142857142856,
   0.5306122448979592,
   0.3448275862068966,
   0.16666666666666666,
   0.4074074074074074,
   0.2631578947368421,
   0.3181818181818182,
   0.7647058823529412,
   0.3,
   0.4090909090909091,
   0.18181818181818182,
   0.39999999999999997,
   0.22857142857142856,
   0.47058823529411764,
   0.3333333333333333,
   0.3,
   0.1904761904761905,
   0.35294117647058826,
   0.3333333333333333,
   0.5106382978723405,
   0.2777777777777778,
   0.3888888888888889,
   0.3125,
   0.24242424242424243,
   0.3333333333333333,
   0.3888888888888889,
   0.4081632653061225,
   0.6046511627906976,
   0.45,
   0.5555555555555556,
   0.11764705882352941,
   0.29411764705882354,
   0.34285714285714286,
   0.6666666666666666,
   0.5957446808510638,
   0.4166666666666667,
   0.6818181818181819,
   0.6382978723404256,
   0.8181818181818182,
   0.5217391304347826,
   0.4615384615384615,
   0.52,
   0.6285714285714286,
   0.5,
   0.4848484848484849,
   0.14814814814814817,
   0.4444444444444444,
   0.4150943396226415,
   0.5714285714285715,
   0.4864864864864864,
   0.375,
   0.36,
   0.29411764705882354,
   0.46511627906976744,
   0.558139534883721,
   0.4444444444444445,
   0.3333333333333333,
   0.38095238095238093,
   0.42424242424242425,
   0.41025641025641024,
   0.34285714285714286,
   0.3333333333333333,
   0.47619047619047616,
   0.30769230769230765,
   0.1904761904761905]],
 None: [5757,
  [5.0,
   4.75,
   5.0,
   2.4,
   2.75,
   2.615,
   5.0,
   2.333,
   3.75,
   5.0,
   3.2,
   1.583,
   5.0,
   5.0,
   4.909,
   2.4,
   5.0,
   4.0,
   3.0,
   1.714,
   3.2,
   2.167,
   1.917,
   4.25,
   3.0,
   2.6,
   5.0,
   4.6,
   5.0,
   4.8,
   3.8,
   5.0,
   5.0,
   4.2,
   1.4,
   3.6,
   2.8,
   1.6,
   3.0,
   1.4,
   4.0,
   4.5,
   3.8,
   4.8,
   5.0,
   1.2,
   3.8,
   3.5,
   4.5,
   2.8,
   3.8,
   3.8,
   4.0,
   4.25,
   2.812,
   4.25,
   3.0,
   3.75,
   4.0,
   2.8,
   3.75,
   1.154,
   2.75,
   2.8,
   3.4,
   5.0,
   2.25,
   2.75,
   4.5,
   2.6,
   3.8,
   2.8,
   1.6,
   1.333,
   2.6,
   3.0,
   3.2,
   2.0,
   3.0,
   3.091,
   2.75,
   1.2,
   4.0,
   3.4,
   2.4,
   1.8,
   2.5,
   4.5,
   3.6,
   5.0,
   5.0,
   5.0,
   5.0,
   3.8,
   5.0,
   2.5,
   3.824,
   1.6,
   5.0,
   5.0,
   2.375,
   5.0,
   1.25,
   1.25,
   3.0,
   2.167,
   1.4,
   4.0,
   3.6,
   4.857,
   1.3,
   1.2,
   1.2,
   4.4,
   1.8,
   1.4,
   4.4,
   3.25,
   2.25,
   2.75,
   2.0,
   3.75,
   1.8,
   4.333,
   4.214,
   3.4,
   4.2,
   4.2,
   2.75,
   2.2,
   1.2,
   1.533,
   3.0,
   3.8,
   3.0,
   3.4,
   3.8,
   1.4,
   3.4,
   3.2,
   2.333,
   3.0,
   3.75,
   2.5,
   1.8,
   2.5,
   1.2,
   2.75,
   3.0,
   3.2,
   1.25,
   5.0,
   3.0,
   1.4,
   3.8,
   2.75,
   2.8,
   2.6,
   2.0,
   3.75,
   3.1,
   2.692,
   4.429,
   5.0,
   1.333,
   3.4,
   2.2,
   3.6,
   1.4,
   2.2,
   3.8,
   2.6,
   4.0,
   2.25,
   3.2,
   3.8,
   4.2,
   3.6,
   2.0,
   4.2,
   3.4,
   3.0,
   3.4,
   3.6,
   3.0,
   2.4,
   2.0,
   4.0,
   4.0,
   4.2,
   2.2,
   3.8,
   3.2,
   4.4,
   1.4,
   2.6,
   3.2,
   4.6,
   1.2,
   3.8,
   3.2,
   2.6,
   5.0,
   3.2,
   4.0,
   1.2,
   4.4,
   3.4,
   4.4,
   4.6,
   4.2,
   3.2,
   1.4,
   3.2,
   1.8,
   1.8,
   3.8,
   3.8,
   4.0,
   3.2,
   1.6,
   3.6,
   3.6,
   2.0,
   3.6,
   4.0,
   3.6,
   3.2,
   2.8,
   2.4,
   3.6,
   1.8,
   3.4,
   1.2,
   1.4,
   2.6,
   2.4,
   4.0,
   3.0,
   4.0,
   4.0,
   2.0,
   4.0,
   2.2,
   2.2,
   3.4,
   3.2,
   4.0,
   3.2,
   3.8,
   3.0,
   4.0,
   2.2,
   3.4,
   3.8,
   4.8,
   3.0,
   4.2,
   4.2,
   4.2,
   4.6,
   5.0,
   3.2,
   2.6,
   2.2,
   4.6,
   5.0,
   4.6,
   4.6,
   4.8,
   2.2,
   4.8,
   1.2,
   2.2,
   4.6,
   2.6,
   3.6,
   2.4,
   4.8,
   5.0,
   3.2,
   1.8,
   3.2,
   3.4,
   4.8,
   4.2,
   2.6,
   2.2,
   1.4,
   2.6,
   1.2,
   1.8,
   4.0,
   3.0,
   4.0,
   1.4,
   2.4,
   2.8,
   4.6,
   4.2,
   3.2,
   1.2,
   1.8,
   2.6,
   1.6,
   3.8,
   4.0,
   4.8,
   2.4,
   5.0,
   3.6,
   2.4,
   4.2,
   4.2,
   3.2,
   1.6,
   1.4,
   4.8,
   4.0,
   3.0,
   1.6,
   4.4,
   4.8,
   2.4,
   3.0,
   2.0,
   4.6,
   5.0,
   1.4,
   3.0,
   2.6,
   1.2,
   5.0,
   3.4,
   2.0,
   2.4,
   2.2,
   3.8,
   2.2,
   4.6,
   2.8,
   2.0,
   4.2,
   4.5,
   1.8,
   4.2,
   4.2,
   1.4,
   3.6,
   5.0,
   1.8,
   2.8,
   1.8,
   1.4,
   1.8,
   2.4,
   1.6,
   3.8,
   4.8,
   4.0,
   3.4,
   3.0,
   1.8,
   2.2,
   3.6,
   3.8,
   4.2,
   1.2,
   3.4,
   2.4,
   3.2,
   2.2,
   4.4,
   2.6,
   3.2,
   2.2,
   5.0,
   5.0,
   2.2,
   2.2,
   2.0,
   1.2,
   4.0,
   4.2,
   3.4,
   4.0,
   4.8,
   4.4,
   3.0,
   4.6,
   1.4,
   3.0,
   1.6,
   2.4,
   1.6,
   1.6,
   2.2,
   2.0,
   4.8,
   2.0,
   3.8,
   2.2,
   2.0,
   4.0,
   4.6,
   1.4,
   1.2,
   1.6,
   3.0,
   2.4,
   4.6,
   4.8,
   5.0,
   3.6,
   4.4,
   4.6,
   2.8,
   4.0,
   5.0,
   1.6,
   1.6,
   3.6,
   3.0,
   2.8,
   1.4,
   2.8,
   3.0,
   1.6,
   2.8,
   4.0,
   2.0,
   4.4,
   4.6,
   2.4,
   4.4,
   3.8,
   1.4,
   2.8,
   3.0,
   1.6,
   2.6,
   1.6,
   3.0,
   3.0,
   3.2,
   3.0,
   2.4,
   3.6,
   1.2,
   3.0,
   4.4,
   3.2,
   3.4,
   3.4,
   3.6,
   1.6,
   3.2,
   2.0,
   1.4,
   2.0,
   2.6,
   4.2,
   2.8,
   2.0,
   2.6,
   2.6,
   2.6,
   1.6,
   1.8,
   3.8,
   1.6,
   3.2,
   2.6,
   3.0,
   1.4,
   1.6,
   1.6,
   1.8,
   1.8,
   1.4,
   2.6,
   2.0,
   1.4,
   1.4,
   1.8,
   4.0,
   2.8,
   2.6,
   2.6,
   4.4,
   2.2,
   1.6,
   1.8,
   3.8,
   3.0,
   1.4,
   3.0,
   3.6,
   3.4,
   2.8,
   4.2,
   4.2,
   1.8,
   2.0,
   1.6,
   2.6,
   3.2,
   2.2,
   1.5,
   4.0,
   1.8,
   1.6,
   2.4,
   2.0,
   1.6,
   2.0,
   3.2,
   2.0,
   2.4,
   1.6,
   3.8,
   1.2,
   2.0,
   2.0,
   3.4,
   2.6,
   2.8,
   2.0,
   1.6,
   1.4,
   1.2,
   2.2,
   2.6,
   3.0,
   2.2,
   1.8,
   1.6,
   2.8,
   2.8,
   1.6,
   1.4,
   1.4,
   3.0,
   3.2,
   2.8,
   3.4,
   2.0,
   2.8,
   4.2,
   3.2,
   4.8,
   3.8,
   1.8,
   2.6,
   1.6,
   1.4,
   2.0,
   1.8,
   1.2,
   2.2,
   3.2,
   1.4,
   1.4,
   1.6,
   2.8,
   1.8,
   2.6,
   2.4,
   2.8,
   2.0,
   3.0,
   2.6,
   1.8,
   3.8,
   3.0,
   1.4,
   1.6,
   3.4,
   3.6,
   2.2,
   3.0,
   1.8,
   2.4,
   2.6,
   1.4,
   1.6,
   1.6,
   1.4,
   2.8,
   3.8,
   3.4,
   2.0,
   3.8,
   1.8,
   1.8,
   1.2,
   3.0,
   3.8,
   3.2,
   2.6,
   3.0,
   2.6,
   1.8,
   2.6,
   1.6,
   2.6,
   1.2,
   2.4,
   2.6,
   4.0,
   3.6,
   2.6,
   1.6,
   4.0,
   3.0,
   2.0,
   3.2,
   2.8,
   2.6,
   2.8,
   3.2,
   3.6,
   2.2,
   2.6,
   3.0,
   2.2,
   3.4,
   2.2,
   1.8,
   1.6,
   2.8,
   1.67,
   1.8,
   2.8,
   1.8,
   1.4,
   2.2,
   1.8,
   4.0,
   4.2,
   4.4,
   3.0,
   2.6,
   3.2,
   2.6,
   1.2,
   3.0,
   2.6,
   1.2,
   2.8,
   1.8,
   3.0,
   2.4,
   2.6,
   3.6,
   1.8,
   1.6,
   2.0,
   2.0,
   2.6,
   1.8,
   1.6,
   2.8,
   2.6,
   3.4,
   1.6,
   4.0,
   1.8,
   1.4,
   1.2,
   3.6,
   3.0,
   1.2,
   1.8,
   1.2,
   3.2,
   3.6,
   5.0,
   1.4,
   2.6,
   2.0,
   3.75,
   4.0,
   3.75,
   3.2,
   4.0,
   2.4,
   4.4,
   4.2,
   3.2,
   3.0,
   3.2,
   3.8,
   3.0,
   2.4,
   5.0,
   3.8,
   3.2,
   3.8,
   3.8,
   3.75,
   3.2,
   3.4,
   4.6,
   3.333,
   3.5,
   1.75,
   3.0,
   4.4,
   3.8,
   3.0,
   4.5,
   2.2,
   4.0,
   4.6,
   3.5,
   3.0,
   4.0,
   4.333,
   3.25,
   3.25,
   1.75,
   4.4,
   3.0,
   3.0,
   3.25,
   4.4,
   5.0,
   5.0,
   3.2,
   2.2,
   3.25,
   3.75,
   3.2,
   4.4,
   2.6,
   3.5,
   3.75,
   3.5,
   4.25,
   2.4,
   3.25,
   3.8,
   3.4,
   3.5,
   2.4,
   3.8,
   3.8,
   4.0,
   3.4,
   3.25,
   4.6,
   3.714,
   3.333,
   3.4,
   2.8,
   3.0,
   3.0,
   3.75,
   4.4,
   2.8,
   3.25,
   1.75,
   1.75,
   5.0,
   3.6,
   3.0,
   2.8,
   3.6,
   3.0,
   5.0,
   3.5,
   4.5,
   4.8,
   3.5,
   3.692,
   4.0,
   3.5,
   4.75,
   3.2,
   2.6,
   3.0,
   3.25,
   2.2,
   3.5,
   4.75,
   3.2,
   3.25,
   3.75,
   3.0,
   2.6,
   3.25,
   3.4,
   1.333,
   5.0,
   4.0,
   3.6,
   3.5,
   3.0,
   1.667,
   3.75,
   2.25,
   4.2,
   3.6,
   3.4,
   3.0,
   3.25,
   3.6,
   3.0,
   1.75,
   3.25,
   4.4,
   2.8,
   2.75,
   3.0,
   3.6,
   3.0,
   2.0,
   3.0,
   4.4,
   2.4,
   4.4,
   4.4,
   2.6,
   3.0,
   4.5,
   3.0,
   1.75,
   2.0,
   2.4,
   4.8,
   4.0,
   4.0,
   4.4,
   4.2,
   3.6,
   2.5,
   1.5,
   5.0,
   3.75,
   1.75,
   4.4,
   3.0,
   3.8,
   3.25,
   2.75,
   3.4,
   3.2,
   2.0,
   3.0,
   3.25,
   5.0,
   3.333,
   3.6,
   3.8,
   3.0,
   4.25,
   3.5,
   3.2,
   2.4,
   4.0,
   4.667,
   3.333,
   3.0,
   3.25,
   4.0,
   3.5,
   2.0,
   3.6,
   3.4,
   3.5,
   2.4,
   3.5,
   2.8,
   4.8,
   3.0,
   3.4,
   3.25,
   4.75,
   3.6,
   4.2,
   2.0,
   3.8,
   1.6,
   3.25,
   5.0,
   3.417,
   2.75,
   4.111,
   3.6,
   3.6,
   4.333,
   3.2,
   2.25,
   4.5,
   2.75,
   4.0,
   3.4,
   2.2,
   3.25,
   3.667,
   4.75,
   3.5,
   3.0,
   3.25,
   3.6,
   3.8,
   3.333,
   4.25,
   1.75,
   2.75,
   3.25,
   2.5,
   3.091,
   4.4,
   4.8,
   5.0,
   3.0,
   3.2,
   4.4,
   1.8,
   4.0,
   4.6,
   1.8,
   1.2,
   4.6,
   1.4,
   3.2,
   2.8,
   3.8,
   3.8,
   4.2,
   1.6,
   3.8,
   1.4,
   3.6,
   1.8,
   3.8,
   1.6,
   2.33333333333333,
   3.6,
   3.4,
   2.6,
   2.2,
   2.6,
   4.8,
   4.8,
   4.8,
   2.6,
   1.6,
   2.2,
   1.2,
   3.4,
   3.2,
   3.2,
   1.8,
   1.2,
   1.6,
   4.8,
   3.6,
   3.8,
   3.0,
   3.6,
   4.4,
   2.0,
   2.4,
   3.2,
   3.4,
   2.8,
   3.2,
   1.8,
   2.8,
   3.4,
   4.6,
   3.8,
   1.6,
   2.6,
   4.2,
   4.4,
   2.2,
   2.6,
   2.8,
   4.0,
   3.2,
   1.8,
   2.6,
   2.75,
   3.2,
   1.8,
   4.2,
   4.2,
   2.6,
   4.2,
   2.0,
   5.0,
   3.8,
   1.6,
   3.4,
   1.4,
   3.8,
   ...],
  [0.7,
   0.8571428571428571,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.7692307692307692,
   0.6666666666666665,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.7777777777777777,
   1.0,
   0.6666666666666666,
   1.0,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.8333333333333334,
   0.8571428571428571,
   0.7777777777777777,
   0.75,
   0.6666666666666666,
   0.4444444444444445,
   1.0,
   0.8181818181818182,
   0.875,
   1.0,
   1.0,
   0.8333333333333334,
   0.8333333333333334,
   0.7777777777777777,
   0.6,
   0.6,
   0.7142857142857143,
   0.8333333333333334,
   0.5555555555555556,
   0.5555555555555556,
   0.5555555555555556,
   0.5555555555555556,
   0.7,
   0.7142857142857143,
   0.6666666666666666,
   0.7142857142857143,
   0.6,
   0.7142857142857143,
   0.6666666666666666,
   0.6086956521739131,
   0.8333333333333334,
   0.5,
   0.28571428571428575,
   0.5555555555555556,
   0.5555555555555556,
   0.64,
   0.4444444444444445,
   0.6666666666666665,
   0.375,
   0.5,
   0.625,
   0.5,
   0.42857142857142855,
   0.6956521739130435,
   0.4444444444444445,
   0.5714285714285715,
   0.8333333333333334,
   0.5714285714285715,
   0.5161290322580646,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.5,
   0.28571428571428564,
   0.7142857142857143,
   0.3333333333333333,
   0.888888888888889,
   0.625,
   0.5714285714285715,
   0.4,
   0.47058823529411764,
   0.34782608695652173,
   0.7142857142857143,
   0.4444444444444444,
   0.5714285714285715,
   0.3157894736842105,
   0.8333333333333334,
   0.8333333333333334,
   0.875,
   1.0,
   1.0,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.888888888888889,
   0.6666666666666666,
   0.8571428571428571,
   0.8571428571428571,
   0.8333333333333334,
   1.0,
   0.75,
   0.75,
   0.6666666666666666,
   0.8333333333333334,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.6666666666666665,
   0.75,
   0.75,
   0.5714285714285715,
   0.8333333333333334,
   0.6666666666666666,
   0.9166666666666666,
   0.7142857142857143,
   0.8333333333333334,
   0.6363636363636364,
   0.42857142857142855,
   0.7777777777777777,
   0.7142857142857143,
   0.8000000000000002,
   0.5714285714285715,
   0.5,
   0.7,
   0.5,
   0.4000000000000001,
   0.8333333333333334,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.7272727272727272,
   0.8,
   0.6,
   0.6666666666666667,
   0.7142857142857143,
   0.7142857142857143,
   0.5263157894736842,
   0.5333333333333333,
   0.5217391304347826,
   0.888888888888889,
   0.42857142857142855,
   0.5,
   0.5,
   0.5,
   0.631578947368421,
   0.4615384615384615,
   0.4761904761904762,
   0.3529411764705882,
   0.8333333333333334,
   0.5,
   0.33333333333333326,
   0.5,
   0.2857142857142857,
   0.37499999999999994,
   0.37499999999999994,
   0.6666666666666667,
   0.6,
   0.6153846153846153,
   0.5263157894736842,
   0.5714285714285715,
   0.8181818181818182,
   0.4,
   0.380952380952381,
   0.5,
   0.5,
   0.5555555555555556,
   0.4375,
   0.36363636363636365,
   0.5,
   0.4,
   0.5,
   0.3125,
   0.64,
   0.5,
   0.75,
   0.28571428571428575,
   0.5,
   0.15,
   0.33333333333333326,
   0.6060606060606061,
   0.6666666666666665,
   0.7368421052631577,
   0.6666666666666665,
   0.3,
   0.5555555555555556,
   0.6250000000000001,
   0.6363636363636365,
   0.625,
   0.7,
   0.7,
   0.6666666666666666,
   0.6,
   0.4444444444444445,
   0.5882352941176471,
   0.6153846153846153,
   0.625,
   0.4545454545454546,
   0.39999999999999997,
   0.75,
   0.9166666666666666,
   0.5714285714285714,
   0.7777777777777777,
   0.5,
   0.5599999999999999,
   0.3448275862068966,
   0.48484848484848486,
   0.8181818181818182,
   0.8750000000000001,
   0.625,
   0.5454545454545454,
   0.6666666666666667,
   0.4444444444444445,
   0.26666666666666666,
   0.75,
   0.3,
   0.3157894736842105,
   0.4000000000000001,
   0.45454545454545453,
   0.35294117647058826,
   0.4210526315789474,
   0.2631578947368421,
   0.5714285714285715,
   0.5555555555555556,
   0.5333333333333333,
   0.23076923076923078,
   0.36363636363636365,
   0.3243243243243243,
   0.4000000000000001,
   0.39999999999999997,
   0.6000000000000001,
   0.33333333333333326,
   0.3333333333333333,
   0.5,
   0.7777777777777777,
   0.7142857142857142,
   0.3448275862068965,
   0.8,
   0.30769230769230765,
   0.4444444444444445,
   0.4444444444444445,
   0.4444444444444445,
   0.6428571428571429,
   0.5555555555555556,
   0.7000000000000001,
   0.6666666666666665,
   0.5454545454545454,
   0.5,
   0.7826086956521738,
   0.6363636363636365,
   0.7428571428571429,
   0.888888888888889,
   0.5714285714285715,
   0.9285714285714286,
   0.4117647058823529,
   0.5,
   0.7692307692307693,
   0.875,
   0.6923076923076923,
   0.8888888888888888,
   0.44444444444444436,
   0.5454545454545454,
   0.5,
   0.9166666666666666,
   0.608695652173913,
   0.56,
   0.5714285714285715,
   0.8461538461538461,
   0.4166666666666667,
   0.7407407407407408,
   0.29787234042553196,
   0.5185185185185185,
   0.5714285714285715,
   0.32,
   0.6,
   0.5714285714285714,
   0.6666666666666667,
   0.7692307692307692,
   0.5,
   0.75,
   0.8,
   0.5833333333333334,
   0.875,
   0.6,
   0.6666666666666665,
   0.4615384615384615,
   0.3157894736842105,
   0.3,
   0.3157894736842105,
   0.4848484848484849,
   0.6000000000000001,
   0.6896551724137931,
   0.6363636363636364,
   0.25,
   0.26086956521739135,
   0.21428571428571427,
   0.8000000000000002,
   0.8333333333333333,
   0.5454545454545454,
   0.45454545454545453,
   0.7142857142857143,
   0.75,
   0.6250000000000001,
   0.7142857142857143,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666665,
   0.5454545454545454,
   0.6428571428571429,
   0.3333333333333333,
   0.8571428571428571,
   0.7333333333333334,
   0.8571428571428571,
   0.6,
   0.38888888888888884,
   1.0,
   0.7499999999999999,
   0.6666666666666666,
   0.5714285714285713,
   0.5925925925925926,
   0.875,
   0.35714285714285715,
   0.9,
   0.6666666666666667,
   0.8888888888888888,
   0.8333333333333334,
   0.14285714285714285,
   0.6315789473684211,
   0.5,
   0.3636363636363636,
   0.8000000000000002,
   0.4444444444444445,
   0.5833333333333334,
   0.3703703703703704,
   0.3846153846153846,
   0.42857142857142855,
   0.5882352941176471,
   0.6666666666666665,
   0.4117647058823529,
   0.5,
   0.6,
   0.380952380952381,
   0.25,
   0.8750000000000001,
   0.7777777777777778,
   0.4,
   0.3255813953488372,
   0.6363636363636365,
   0.7692307692307692,
   0.8,
   0.31578947368421056,
   0.4,
   0.42857142857142855,
   0.48648648648648646,
   0.6,
   0.6666666666666667,
   0.875,
   0.6,
   0.5833333333333334,
   0.24242424242424243,
   0.625,
   0.5555555555555556,
   0.5714285714285715,
   0.8095238095238096,
   0.8333333333333334,
   0.4150943396226415,
   0.5,
   0.5,
   0.875,
   0.6666666666666666,
   0.8571428571428571,
   0.7000000000000001,
   0.5,
   0.36363636363636365,
   0.4666666666666667,
   0.5333333333333333,
   0.5,
   0.4,
   0.4,
   0.46153846153846156,
   0.4,
   0.9375,
   0.75,
   0.28571428571428575,
   0.888888888888889,
   0.8571428571428571,
   0.4666666666666667,
   0.7741935483870968,
   0.380952380952381,
   0.5384615384615384,
   0.875,
   0.6153846153846153,
   0.5833333333333334,
   0.358974358974359,
   0.631578947368421,
   0.42105263157894735,
   0.6666666666666665,
   0.4444444444444444,
   0.8571428571428571,
   0.6666666666666665,
   0.3846153846153846,
   0.8571428571428571,
   0.6451612903225806,
   0.34285714285714286,
   0.4444444444444445,
   0.4,
   0.2631578947368421,
   0.875,
   0.5925925925925926,
   0.8571428571428571,
   0.4,
   0.4736842105263158,
   0.8571428571428571,
   1.0,
   0.18181818181818182,
   0.7,
   1.0,
   0.21621621621621623,
   0.5,
   0.625,
   0.7692307692307692,
   0.6,
   0.32,
   0.9,
   0.2,
   0.1875,
   0.625,
   0.5882352941176471,
   0.47058823529411764,
   0.8571428571428571,
   0.7777777777777778,
   0.75,
   0.5,
   0.9090909090909091,
   0.4081632653061225,
   0.56,
   0.38461538461538464,
   0.75,
   0.3157894736842105,
   0.25,
   0.8333333333333334,
   0.7142857142857143,
   0.5,
   0.339622641509434,
   0.35,
   0.32653061224489793,
   0.2105263157894737,
   0.3571428571428571,
   0.3076923076923077,
   0.375,
   0.23809523809523808,
   0.2631578947368421,
   0.28571428571428575,
   0.2105263157894737,
   0.425531914893617,
   0.2857142857142857,
   0.24999999999999994,
   0.23255813953488372,
   0.26865671641791045,
   0.1904761904761905,
   0.20408163265306123,
   0.17777777777777778,
   0.21739130434782608,
   0.25,
   0.15,
   0.2692307692307692,
   0.15,
   0.6530612244897959,
   0.2711864406779661,
   0.2222222222222222,
   0.24242424242424246,
   0.4444444444444444,
   0.20833333333333334,
   0.2105263157894737,
   0.3913043478260869,
   0.35294117647058826,
   0.26666666666666666,
   0.19607843137254902,
   0.125,
   0.21739130434782608,
   0.057142857142857134,
   0.208955223880597,
   0.3529411764705882,
   0.39999999999999997,
   0.5333333333333333,
   0.35000000000000003,
   0.3125,
   0.3913043478260869,
   0.40816326530612246,
   0.18181818181818182,
   0.07017543859649122,
   0.28571428571428575,
   0.16666666666666666,
   0.17857142857142855,
   0.3076923076923077,
   0.15789473684210525,
   0.16666666666666669,
   0.253968253968254,
   0.4489795918367347,
   0.37500000000000006,
   0.18867924528301888,
   0.24137931034482757,
   0.1923076923076923,
   0.14285714285714288,
   0.2580645161290323,
   0.1818181818181818,
   0.32,
   0.3846153846153846,
   0.30769230769230765,
   0.2,
   0.13636363636363638,
   0.1818181818181818,
   0.19230769230769232,
   0.25641025641025644,
   0.2222222222222222,
   0.16666666666666666,
   0.34782608695652173,
   0.16216216216216214,
   0.32558139534883723,
   0.14634146341463414,
   0.4545454545454545,
   0.411764705882353,
   0.5,
   0.25,
   0.21052631578947367,
   0.33333333333333326,
   0.1791044776119403,
   0.35294117647058826,
   0.3050847457627119,
   0.273972602739726,
   0.44897959183673464,
   0.372093023255814,
   0.26229508196721313,
   0.23809523809523808,
   0.40816326530612246,
   0.28571428571428575,
   0.391304347826087,
   0.3125,
   0.27586206896551724,
   0.339622641509434,
   0.35555555555555557,
   0.34285714285714286,
   0.15384615384615385,
   0.2666666666666666,
   0.21818181818181817,
   0.23529411764705882,
   0.2,
   0.23255813953488372,
   0.6206896551724139,
   0.3902439024390244,
   0.22857142857142854,
   0.2127659574468085,
   0.30188679245283023,
   0.21621621621621623,
   0.2857142857142857,
   0.25,
   0.2790697674418605,
   0.2666666666666666,
   0.28571428571428575,
   0.2413793103448276,
   0.1587301587301587,
   0.4,
   0.2807017543859649,
   0.17857142857142858,
   0.19230769230769232,
   0.33333333333333326,
   0.41025641025641024,
   0.3703703703703704,
   0.2941176470588235,
   0.2745098039215686,
   0.31818181818181823,
   0.5555555555555556,
   0.3333333333333333,
   0.27272727272727276,
   0.3243243243243243,
   0.17543859649122806,
   0.2941176470588235,
   0.18181818181818182,
   0.2380952380952381,
   0.15384615384615385,
   0.32142857142857145,
   0.1818181818181818,
   0.18181818181818185,
   0.17391304347826086,
   0.1724137931034483,
   0.25,
   0.5405405405405405,
   0.4666666666666667,
   0.30769230769230765,
   0.2580645161290323,
   0.41025641025641024,
   0.15,
   0.34615384615384615,
   0.21052631578947367,
   0.45714285714285713,
   0.40579710144927533,
   0.20408163265306123,
   0.20000000000000004,
   0.21621621621621623,
   0.3278688524590164,
   0.1917808219178082,
   0.23809523809523808,
   0.23333333333333334,
   0.16901408450704225,
   0.27450980392156865,
   0.22222222222222224,
   0.20000000000000004,
   0.3768115942028986,
   0.5945945945945946,
   0.37499999999999994,
   0.30188679245283023,
   0.4878048780487805,
   0.26666666666666666,
   0.2702702702702703,
   0.38461538461538464,
   0.2641509433962264,
   0.2857142857142857,
   0.39285714285714285,
   0.5306122448979592,
   0.4210526315789474,
   0.22222222222222224,
   0.2769230769230769,
   0.3666666666666667,
   0.15999999999999998,
   0.11320754716981131,
   0.37209302325581395,
   0.14285714285714285,
   0.14285714285714282,
   0.37837837837837834,
   0.4067796610169492,
   0.25,
   0.42105263157894735,
   0.3793103448275862,
   0.22727272727272727,
   0.25641025641025644,
   0.375,
   0.8823529411764706,
   0.5490196078431373,
   0.4761904761904762,
   0.36065573770491804,
   0.25925925925925924,
   0.3174603174603175,
   0.17647058823529413,
   0.2857142857142857,
   0.35294117647058826,
   0.20512820512820512,
   0.15999999999999998,
   0.35294117647058826,
   0.16666666666666666,
   0.2857142857142857,
   0.3404255319148936,
   0.43636363636363634,
   0.5789473684210527,
   0.20833333333333331,
   0.4827586206896552,
   0.34782608695652173,
   0.26666666666666666,
   0.23076923076923078,
   0.14545454545454545,
   0.11428571428571428,
   0.3013698630136986,
   0.5,
   0.2222222222222222,
   0.22222222222222224,
   0.3333333333333333,
   0.27450980392156865,
   0.19999999999999998,
   0.21276595744680848,
   0.3243243243243243,
   0.22727272727272724,
   0.2222222222222222,
   0.1818181818181818,
   0.1724137931034483,
   0.17777777777777778,
   0.5660377358490567,
   0.7142857142857143,
   0.7241379310344828,
   0.7042253521126761,
   0.5842696629213484,
   0.853658536585366,
   0.56,
   0.7012987012987012,
   0.2666666666666666,
   0.5714285714285714,
   0.5245901639344263,
   0.7777777777777778,
   0.8387096774193549,
   0.45161290322580644,
   0.5396825396825397,
   0.3870967741935483,
   0.6666666666666666,
   0.6545454545454545,
   0.6024096385542168,
   0.7058823529411765,
   0.6329113924050633,
   0.4301075268817204,
   0.44067796610169496,
   0.717948717948718,
   0.5116279069767442,
   0.5714285714285714,
   0.634920634920635,
   0.7605633802816901,
   0.7469879518072288,
   0.6451612903225806,
   0.42424242424242425,
   0.5714285714285715,
   0.8787878787878788,
   0.6067415730337078,
   0.6410256410256411,
   0.7368421052631577,
   0.625,
   0.7857142857142857,
   0.9459459459459459,
   0.6,
   0.7027027027027025,
   0.746268656716418,
   0.6885245901639345,
   0.6896551724137931,
   0.32727272727272727,
   0.5217391304347826,
   0.6530612244897959,
   0.8125,
   0.716417910447761,
   0.5454545454545455,
   0.5,
   0.8,
   0.7058823529411765,
   0.7457627118644068,
   0.5,
   0.6666666666666667,
   0.7666666666666666,
   0.4166666666666667,
   0.782608695652174,
   0.6382978723404256,
   0.6585365853658536,
   0.5633802816901409,
   0.5625,
   0.42500000000000004,
   0.49056603773584906,
   0.6842105263157894,
   0.65625,
   0.7333333333333333,
   0.45161290322580644,
   0.5666666666666667,
   0.48837209302325585,
   0.767123287671233,
   0.5977011494252873,
   0.5483870967741935,
   0.7297297297297297,
   0.7428571428571429,
   0.6779661016949153,
   0.509090909090909,
   0.48275862068965514,
   0.47058823529411764,
   0.5116279069767442,
   0.5581395348837209,
   0.5633802816901409,
   0.6153846153846153,
   0.7692307692307692,
   0.5263157894736842,
   0.48484848484848486,
   0.761904761904762,
   0.5882352941176471,
   0.8,
   0.6578947368421053,
   0.24390243902439024,
   0.48888888888888893,
   0.5970149253731343,
   0.9090909090909091,
   0.5128205128205129,
   0.6363636363636364,
   0.7631578947368423,
   0.5901639344262296,
   0.575,
   0.5757575757575757,
   0.6075949367088608,
   0.8524590163934426,
   0.5977011494252874,
   0.7692307692307693,
   0.5970149253731343,
   0.6370370370370371,
   0.5151515151515151,
   0.47887323943661964,
   0.8809523809523809,
   0.5625,
   0.8260869565217391,
   0.711111111111111,
   0.509090909090909,
   0.48387096774193544,
   0.48,
   0.759493670886076,
   0.5283018867924528,
   0.7142857142857142,
   0.46511627906976744,
   0.2553191489361702,
   0.4545454545454546,
   0.490566037735849,
   0.4137931034482759,
   0.72,
   0.3859649122807018,
   0.7415730337078651,
   0.8282828282828283,
   0.5970149253731343,
   0.42424242424242425,
   0.6666666666666666,
   0.7234042553191491,
   0.6000000000000001,
   0.6153846153846153,
   0.5365853658536585,
   0.7500000000000001,
   0.4210526315789474,
   0.45454545454545453,
   0.7472527472527473,
   0.7,
   0.3225806451612903,
   0.5866666666666667,
   0.6333333333333333,
   0.5964912280701755,
   0.6739130434782609,
   0.7294117647058824,
   0.6857142857142857,
   0.417910447761194,
   0.4528301886792453,
   0.4307692307692308,
   0.7407407407407408,
   0.4489795918367347,
   0.41025641025641024,
   0.4675324675324676,
   0.9534883720930233,
   0.72,
   0.490566037735849,
   0.7142857142857143,
   0.7323943661971832,
   0.7526881720430108,
   0.35000000000000003,
   0.23333333333333336,
   0.5970149253731343,
   0.42857142857142855,
   0.49056603773584906,
   0.7037037037037037,
   0.6756756756756758,
   0.6521739130434783,
   0.7466666666666666,
   0.5116279069767442,
   0.7671232876712328,
   0.5818181818181818,
   0.5454545454545455,
   0.5306122448979591,
   0.6153846153846154,
   0.9166666666666666,
   0.576923076923077,
   0.5666666666666667,
   0.5476190476190477,
   0.634920634920635,
   0.7555555555555556,
   0.5423728813559322,
   0.5263157894736841,
   0.5833333333333333,
   0.796116504854369,
   0.4,
   0.5084745762711865,
   0.6666666666666666,
   0.7692307692307693,
   0.7659574468085106,
   0.6111111111111112,
   0.34782608695652173,
   0.7241379310344828,
   0.4897959183673469,
   0.5176470588235293,
   0.5084745762711865,
   0.5806451612903226,
   0.7628865979381443,
   0.6024096385542168,
   0.509090909090909,
   0.634920634920635,
   0.5434782608695652,
   0.7012987012987012,
   0.547945205479452,
   0.5434782608695652,
   0.29787234042553196,
   0.6933333333333334,
   0.47457627118644063,
   0.5483870967741935,
   0.7272727272727273,
   0.5783132530120482,
   0.4000000000000001,
   0.676923076923077,
   0.46428571428571425,
   0.7529411764705882,
   0.8571428571428572,
   0.5373134328358209,
   0.6,
   0.7678571428571429,
   0.3636363636363636,
   0.4444444444444445,
   0.56,
   0.36363636363636365,
   0.6250000000000001,
   0.5263157894736842,
   0.8705882352941177,
   0.7547169811320756,
   0.5365853658536586,
   0.735294117647059,
   0.6933333333333334,
   0.7441860465116279,
   0.7951807228915663,
   0.6823529411764706,
   0.5853658536585366,
   0.5454545454545455,
   0.6415094339622641,
   0.7789473684210527,
   0.5777777777777778,
   0.6666666666666666,
   0.8214285714285715,
   0.9714285714285714,
   0.576923076923077,
   0.6181818181818182,
   0.8484848484848484,
   0.49122807017543857,
   0.4827586206896552,
   0.7692307692307693,
   0.56,
   0.4,
   1.0,
   0.6666666666666667,
   0.717948717948718,
   0.4444444444444445,
   0.6206896551724137,
   0.7142857142857143,
   0.625,
   0.6,
   0.8,
   0.3333333333333333,
   0.8125,
   0.5625,
   0.6571428571428571,
   0.7234042553191491,
   0.5531914893617023,
   0.6363636363636364,
   0.43243243243243246,
   0.75,
   0.6486486486486486,
   0.8333333333333333,
   0.8571428571428571,
   0.9285714285714286,
   0.875,
   0.56,
   0.4848484848484848,
   0.3636363636363636,
   0.46808510638297873,
   0.7692307692307692,
   0.5714285714285713,
   0.48000000000000004,
   0.31746031746031744,
   0.5263157894736842,
   0.625,
   0.6470588235294117,
   0.4666666666666666,
   0.6976744186046512,
   0.46808510638297873,
   0.6956521739130435,
   0.823529411764706,
   0.5945945945945945,
   0.5,
   0.42857142857142855,
   0.6250000000000001,
   0.41025641025641024,
   0.5714285714285715,
   0.6363636363636364,
   0.5384615384615385,
   0.7804878048780488,
   0.8571428571428572,
   0.9259259259259259,
   0.28571428571428575,
   0.5853658536585366,
   0.5641025641025642,
   0.8771929824561403,
   0.6222222222222223,
   0.7777777777777777,
   0.25,
   0.9090909090909091,
   0.6086956521739131,
   0.5333333333333333,
   0.6500000000000001,
   0.6545454545454547,
   0.65,
   0.7857142857142856,
   0.7894736842105263,
   0.8888888888888888,
   0.5,
   0.8648648648648648,
   0.5853658536585366,
   0.8400000000000001,
   0.7619047619047619,
   0.8000000000000002,
   0.65,
   0.8181818181818182,
   0.5294117647058824,
   ...]],
 0.8: [211,
  [0.8,
   0.636,
   0.8,
   0.8,
   0.778,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.67,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.667,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.643,
   0.75,
   0.8,
   0.727,
   0.8,
   0.8,
   0.8,
   0.8,
   0.667,
   0.8,
   0.8,
   0.75,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.8,
   0.75,
   0.8,
   0.8,
   0.75,
   0.75,
   0.75,
   0.75,
   0.8,
   0.667,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.75,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8],
  [0.6666666666666666,
   0.75,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.375,
   0.6666666666666666,
   0.5714285714285715,
   0.4444444444444444,
   0.6666666666666666,
   0.20000000000000004,
   0.5333333333333333,
   0.3636363636363636,
   0.3225806451612903,
   0.29629629629629634,
   0.21621621621621623,
   0.6,
   0.20689655172413793,
   0.6666666666666665,
   0.3684210526315789,
   0.3703703703703704,
   0.36363636363636365,
   0.3333333333333333,
   0.16666666666666666,
   0.3050847457627119,
   0.25,
   0.17142857142857143,
   0.2153846153846154,
   0.32727272727272727,
   0.2545454545454545,
   0.339622641509434,
   0.14634146341463417,
   0.1904761904761905,
   0.4,
   0.2,
   0.2222222222222222,
   0.3125,
   0.13333333333333333,
   0.5,
   0.3829787234042554,
   0.3255813953488372,
   0.29166666666666663,
   0.3684210526315789,
   0.375,
   0.5882352941176471,
   0.358974358974359,
   0.48648648648648646,
   0.6521739130434783,
   0.6111111111111112,
   0.5909090909090909,
   0.75,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.4444444444444445,
   0.6,
   0.5714285714285715,
   0.3529411764705882,
   0.6250000000000001,
   0.5714285714285715,
   0.5333333333333333,
   0.5714285714285715,
   0.4210526315789474,
   0.36363636363636365,
   0.5714285714285715,
   0.375,
   0.6666666666666665,
   0.5,
   0.75,
   0.6666666666666666,
   0.7142857142857143,
   0.5714285714285715,
   0.5,
   0.42857142857142855,
   0.5714285714285715,
   0.6,
   0.6666666666666666,
   0.3333333333333333,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.6,
   0.5,
   0.6153846153846153,
   0.6,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.5714285714285715,
   0.35294117647058826,
   0.5,
   0.4444444444444445,
   0.37499999999999994,
   0.6,
   0.28571428571428564,
   0.42857142857142855,
   0.4,
   0.5,
   0.4,
   0.4000000000000001,
   0.23076923076923078,
   0.3636363636363636,
   0.14285714285714288,
   0.625,
   0.30769230769230765,
   0.2857142857142857,
   0.625,
   0.6666666666666666,
   0.33333333333333326,
   0.5,
   0.2727272727272727,
   0.48484848484848486,
   0.6666666666666665,
   0.4444444444444445,
   0.3703703703703704,
   0.37499999999999994,
   0.6153846153846153,
   0.25,
   0.1875,
   0.41379310344827586,
   0.3333333333333333,
   0.3636363636363637,
   0.3,
   0.41379310344827586,
   0.2,
   0.3571428571428571,
   0.46153846153846156,
   0.5714285714285715,
   0.4666666666666667,
   0.35714285714285715,
   0.36363636363636365,
   0.47058823529411764,
   0.47058823529411764,
   0.5454545454545454,
   0.7450980392156864,
   0.7272727272727273,
   0.5925925925925926,
   0.5,
   0.4210526315789474,
   0.6666666666666665,
   0.23076923076923078,
   0.5,
   0.3888888888888889,
   0.5333333333333332,
   0.3255813953488372,
   0.23529411764705882,
   0.4814814814814815,
   0.7407407407407408,
   0.5531914893617023,
   0.4680851063829788,
   0.5,
   0.39024390243902435,
   0.6938775510204083,
   0.3448275862068966,
   0.5555555555555556,
   0.7142857142857142,
   0.5714285714285714,
   0.35,
   0.5454545454545455,
   0.5777777777777778,
   0.4,
   0.6190476190476191,
   0.6666666666666666,
   0.34285714285714286,
   0.7058823529411765,
   0.6086956521739131,
   0.29411764705882354,
   0.7500000000000001,
   0.3404255319148936,
   0.46511627906976744,
   0.37499999999999994,
   0.5142857142857143,
   0.625,
   0.3902439024390244,
   0.7741935483870969,
   0.6818181818181818,
   0.3529411764705882,
   0.39999999999999997,
   0.35897435897435903,
   0.5454545454545454,
   0.43749999999999994,
   0.5625,
   0.25925925925925924,
   0.43243243243243246,
   0.5625,
   0.5416666666666667,
   0.7368421052631577,
   0.33333333333333337,
   0.6315789473684211,
   0.5454545454545454,
   0.3,
   0.5161290322580646,
   0.3728813559322034,
   0.43749999999999994,
   0.7894736842105263,
   0.7333333333333334,
   0.7741935483870968,
   0.34146341463414637,
   0.5185185185185186,
   0.6666666666666666,
   0.5405405405405405,
   0.39999999999999997,
   0.6896551724137931,
   0.41025641025641024,
   0.3714285714285715]],
 1.0: [264,
  [1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.833,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.85,
   1.0,
   0.833,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.9,
   0.9,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.944,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.889,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0],
  [0.8333333333333334,
   0.6,
   0.6666666666666666,
   0.4210526315789474,
   0.4444444444444445,
   0.5714285714285715,
   0.6666666666666666,
   0.4666666666666667,
   0.3,
   0.36363636363636365,
   0.2,
   0.3157894736842105,
   0.6,
   0.35714285714285715,
   0.2962962962962963,
   0.3846153846153846,
   0.15384615384615383,
   0.35294117647058826,
   0.20689655172413793,
   0.14285714285714285,
   0.21739130434782608,
   0.10526315789473684,
   0.2790697674418605,
   0.2745098039215686,
   0.2127659574468085,
   0.25,
   0.23076923076923078,
   0.2790697674418605,
   0.1951219512195122,
   0.27777777777777773,
   0.2926829268292683,
   0.2857142857142857,
   0.09302325581395349,
   0.3829787234042554,
   0.3636363636363636,
   0.39024390243902435,
   0.5405405405405405,
   0.5128205128205129,
   0.2222222222222222,
   0.42424242424242425,
   0.25,
   0.6470588235294117,
   0.4,
   0.5217391304347826,
   0.358974358974359,
   0.372093023255814,
   0.6666666666666666,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6666666666666666,
   0.5,
   0.5,
   0.4,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.5882352941176471,
   0.4705882352941177,
   0.6666666666666666,
   0.6666666666666666,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.6153846153846153,
   0.5714285714285715,
   0.4,
   0.42857142857142855,
   0.6666666666666666,
   0.4615384615384615,
   0.47619047619047616,
   0.6666666666666666,
   0.5,
   0.37499999999999994,
   0.4444444444444444,
   0.42857142857142855,
   0.5333333333333333,
   0.4444444444444444,
   0.4166666666666667,
   0.47058823529411764,
   0.4761904761904762,
   0.35714285714285715,
   0.2758620689655172,
   0.5555555555555556,
   0.33333333333333326,
   0.36363636363636365,
   0.16,
   0.5,
   0.47058823529411764,
   0.375,
   0.0909090909090909,
   0.33333333333333326,
   0.375,
   0.34782608695652173,
   0.2222222222222222,
   0.23076923076923075,
   0.25,
   0.3076923076923077,
   0.22857142857142854,
   0.35714285714285715,
   0.5517241379310345,
   0.6666666666666666,
   0.2,
   0.18181818181818182,
   0.5,
   0.4000000000000001,
   0.1702127659574468,
   0.35294117647058826,
   0.6875,
   0.6,
   0.4210526315789474,
   0.47058823529411764,
   0.7142857142857143,
   0.6363636363636365,
   0.3157894736842105,
   0.8461538461538461,
   0.7142857142857143,
   0.4666666666666667,
   0.4666666666666667,
   0.8000000000000002,
   0.5,
   0.8648648648648649,
   0.6666666666666666,
   0.5454545454545455,
   0.6428571428571429,
   0.6,
   0.3404255319148936,
   0.3333333333333333,
   0.5483870967741935,
   0.617283950617284,
   0.4888888888888888,
   0.3636363636363636,
   0.4523809523809524,
   0.6666666666666666,
   0.5964912280701754,
   0.42857142857142855,
   0.3404255319148936,
   0.4,
   0.3555555555555555,
   0.4197530864197531,
   0.8461538461538461,
   0.45714285714285713,
   0.24615384615384617,
   0.4444444444444444,
   0.5405405405405405,
   0.5925925925925926,
   0.48484848484848486,
   0.4,
   0.358974358974359,
   0.6111111111111113,
   0.41666666666666663,
   0.4666666666666667,
   0.48000000000000004,
   0.5,
   0.35714285714285715,
   0.6,
   0.45,
   0.4375,
   0.6428571428571429,
   0.49056603773584906,
   0.31818181818181823,
   0.4888888888888889,
   0.6857142857142857,
   0.4516129032258065,
   0.6923076923076924,
   0.7741935483870968,
   0.5862068965517241,
   0.47058823529411764,
   0.47368421052631576,
   0.5806451612903225,
   0.76,
   0.5625000000000001,
   0.4255319148936171,
   0.3333333333333333,
   0.28571428571428575,
   0.375,
   0.6376811594202899,
   0.4878048780487805,
   0.7857142857142857,
   0.5925925925925927,
   0.5116279069767442,
   0.4090909090909091,
   0.3902439024390244,
   0.6666666666666666,
   0.5652173913043478,
   0.5714285714285713,
   0.5384615384615384,
   0.3636363636363636,
   0.6666666666666667,
   0.75,
   0.5128205128205129,
   0.6206896551724139,
   0.4827586206896552,
   0.4782608695652174,
   0.5,
   0.5263157894736842,
   0.4583333333333333,
   0.4897959183673469,
   0.875,
   0.4736842105263158,
   0.46511627906976744,
   0.5833333333333334,
   0.43902439024390244,
   0.6666666666666666,
   0.358974358974359,
   0.3448275862068966,
   0.606060606060606,
   0.42857142857142855,
   0.3636363636363636,
   0.6666666666666666,
   0.3428571428571428,
   0.425531914893617,
   0.5,
   0.3902439024390244,
   0.4117647058823529,
   0.2285714285714286,
   0.85,
   0.5500000000000002,
   0.3829787234042554,
   0.5652173913043479,
   0.3888888888888889,
   0.43478260869565216,
   0.3636363636363636,
   0.409090909090909,
   0.3888888888888889,
   0.5925925925925926,
   0.45454545454545453,
   0.358974358974359,
   0.358974358974359,
   0.52,
   0.5625000000000001,
   0.3,
   0.22727272727272727,
   0.40816326530612246,
   0.9090909090909091,
   0.8636363636363636,
   0.6976744186046512,
   0.7692307692307692,
   0.7857142857142856,
   0.6206896551724138,
   0.4242424242424242,
   0.4242424242424242,
   0.7857142857142857,
   0.6274509803921569,
   0.6666666666666666,
   0.46808510638297873,
   0.5,
   0.6285714285714287,
   0.6315789473684211,
   0.7222222222222222,
   0.48484848484848486,
   0.6875000000000001,
   0.358974358974359,
   0.4324324324324324,
   0.42857142857142855,
   0.46511627906976744,
   0.5945945945945946,
   0.4666666666666667,
   0.5762711864406779,
   0.7199999999999999]],
 0.6: [190,
  [0.6,
   0.5,
   0.6,
   0.6,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.5,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.5,
   0.417,
   0.5,
   0.6,
   0.6,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6],
  [0.5,
   0.5263157894736842,
   0.6666666666666666,
   0.5,
   0.5,
   0.6666666666666666,
   0.6,
   0.5,
   0.6,
   0.6666666666666666,
   0.5714285714285715,
   0.380952380952381,
   0.5714285714285715,
   0.47058823529411764,
   0.5,
   0.34782608695652173,
   0.28571428571428575,
   0.5263157894736842,
   0.1,
   0.25,
   0.5,
   0.5555555555555556,
   0.28571428571428575,
   0.2758620689655172,
   0.22222222222222224,
   0.23529411764705882,
   0.25,
   0.13793103448275862,
   0.26666666666666666,
   0.2,
   0.28571428571428575,
   0.17391304347826086,
   0.13953488372093023,
   0.3714285714285714,
   0.1081081081081081,
   0.21052631578947367,
   0.21818181818181817,
   0.21538461538461542,
   0.13043478260869565,
   0.10714285714285714,
   0.1702127659574468,
   0.0930232558139535,
   0.2647058823529412,
   0.42553191489361697,
   0.1818181818181818,
   0.21052631578947367,
   0.24137931034482757,
   0.2608695652173913,
   0.18518518518518517,
   0.5714285714285714,
   0.5625000000000001,
   0.39999999999999997,
   0.43902439024390244,
   0.38888888888888884,
   0.1904761904761905,
   0.75,
   0.75,
   0.75,
   0.75,
   0.6,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6153846153846153,
   0.625,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.5714285714285715,
   0.42857142857142855,
   0.39999999999999997,
   0.3333333333333333,
   0.5384615384615384,
   0.42857142857142855,
   0.5454545454545454,
   0.42857142857142855,
   0.6666666666666666,
   0.3333333333333333,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.5714285714285715,
   0.37499999999999994,
   0.5,
   0.5,
   0.5714285714285715,
   0.6,
   0.5,
   0.5,
   0.4615384615384615,
   0.5555555555555556,
   0.5714285714285715,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.2857142857142857,
   0.5,
   0.17647058823529413,
   0.1904761904761905,
   0.6,
   0.22727272727272727,
   0.21428571428571427,
   0.22222222222222224,
   0.20000000000000004,
   0.6666666666666666,
   0.45454545454545453,
   0.3703703703703704,
   0.27027027027027023,
   0.5,
   0.3636363636363636,
   0.08695652173913043,
   0.2105263157894737,
   0.38709677419354843,
   0.14634146341463414,
   0.29629629629629634,
   0.37499999999999994,
   0.24242424242424243,
   0.23076923076923075,
   0.6666666666666666,
   0.3333333333333333,
   0.2,
   0.35714285714285715,
   0.2,
   0.5,
   0.33333333333333337,
   0.5714285714285715,
   0.3157894736842105,
   0.46153846153846156,
   0.32653061224489793,
   0.7142857142857142,
   0.31249999999999994,
   0.5652173913043478,
   0.6666666666666666,
   0.4090909090909091,
   0.35714285714285715,
   0.16666666666666666,
   0.64,
   0.33333333333333337,
   0.6829268292682927,
   0.7500000000000001,
   0.5,
   0.2857142857142857,
   0.3636363636363636,
   0.6315789473684211,
   0.5625000000000001,
   0.6666666666666667,
   0.6451612903225806,
   0.28571428571428575,
   0.4814814814814815,
   0.5555555555555556,
   0.3225806451612903,
   0.37837837837837834,
   0.2580645161290323,
   0.5263157894736842,
   0.4489795918367347,
   0.2727272727272727,
   0.6829268292682927,
   0.851063829787234,
   0.3783783783783784,
   0.7916666666666667,
   0.42857142857142855,
   0.3255813953488372,
   0.2926829268292683,
   0.4137931034482759,
   0.42857142857142855,
   0.2857142857142857,
   0.6341463414634146,
   0.6428571428571429,
   0.26666666666666666,
   0.47058823529411764,
   0.45,
   0.5777777777777777,
   0.4444444444444444,
   0.30769230769230765,
   0.39999999999999997,
   0.6428571428571429,
   0.6829268292682927,
   0.7272727272727272,
   0.6875,
   0.4,
   0.7142857142857143,
   0.358974358974359,
   0.6111111111111113,
   0.6000000000000001,
   0.3846153846153846,
   0.4615384615384615,
   0.35,
   0.4615384615384615,
   0.4736842105263158]],
 0.4: [214,
  [0.25,
   0.25,
   0.25,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.333,
   0.333,
   0.25,
   0.4,
   0.4,
   0.25,
   0.25,
   0.4,
   0.4,
   0.4,
   0.25,
   0.25,
   0.25,
   0.4,
   0.25,
   0.25,
   0.4,
   0.25,
   0.4,
   0.25,
   0.4,
   0.4,
   0.25,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.231,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.25,
   0.333,
   0.4,
   0.25,
   0.333,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4],
  [0.5,
   0.4,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6153846153846153,
   0.375,
   0.28571428571428575,
   0.2,
   0.4444444444444445,
   0.5555555555555556,
   0.3448275862068965,
   0.36363636363636365,
   0.3243243243243243,
   0.34782608695652173,
   0.24242424242424246,
   0.20512820512820512,
   0.1379310344827586,
   0.3636363636363637,
   0.25,
   0.34285714285714286,
   0.33333333333333337,
   0.10526315789473685,
   0.29629629629629634,
   0.3,
   0.3,
   0.11320754716981132,
   0.22727272727272724,
   0.509090909090909,
   0.1904761904761905,
   0.22222222222222224,
   0.25,
   0.23809523809523808,
   0.22580645161290322,
   0.2,
   0.16,
   0.27906976744186046,
   0.19512195121951217,
   0.27027027027027023,
   0.1923076923076923,
   0.3673469387755102,
   0.04761904761904762,
   0.2285714285714286,
   0.3333333333333333,
   0.43749999999999994,
   0.5,
   0.3636363636363636,
   0.1764705882352941,
   0.4864864864864865,
   0.5,
   0.4680851063829788,
   0.6470588235294118,
   0.5652173913043479,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.26666666666666666,
   0.6666666666666666,
   0.6,
   0.5,
   0.5333333333333333,
   0.6666666666666666,
   0.4210526315789474,
   0.13333333333333333,
   0.375,
   0.42857142857142855,
   0.5,
   0.2857142857142857,
   0.5882352941176471,
   0.5,
   0.37499999999999994,
   0.6,
   0.28571428571428575,
   0.6666666666666666,
   0.6,
   0.6,
   0.5,
   0.3333333333333333,
   0.6153846153846153,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.6,
   0.5714285714285715,
   0.5,
   0.5714285714285715,
   0.5714285714285714,
   0.5714285714285715,
   0.5,
   0.5,
   0.375,
   0.3333333333333333,
   0.5,
   0.4,
   0.6666666666666666,
   0.25,
   0.4444444444444444,
   0.4705882352941177,
   0.6666666666666666,
   0.5,
   0.375,
   0.6666666666666666,
   0.5,
   0.375,
   0.28571428571428575,
   0.2857142857142857,
   0.5,
   0.5,
   0.3703703703703703,
   0.48000000000000004,
   0.42857142857142855,
   0.39999999999999997,
   0.30303030303030304,
   0.29411764705882354,
   0.3076923076923077,
   0.28571428571428575,
   0.25,
   0.47619047619047616,
   0.33333333333333326,
   0.26666666666666666,
   0.3,
   0.25,
   0.47058823529411764,
   0.4444444444444445,
   0.625,
   0.3,
   0.3636363636363637,
   0.18749999999999997,
   0.3333333333333333,
   0.26666666666666666,
   0.45454545454545453,
   0.22222222222222224,
   0.2727272727272727,
   0.30769230769230765,
   0.3,
   0.5714285714285714,
   0.24390243902439024,
   0.2,
   0.5806451612903225,
   0.14814814814814817,
   0.2857142857142857,
   0.3333333333333333,
   0.2380952380952381,
   0.5714285714285715,
   0.7407407407407408,
   0.75,
   0.5714285714285714,
   0.3333333333333333,
   0.3829787234042554,
   0.4680851063829787,
   0.8571428571428571,
   0.31250000000000006,
   0.5,
   0.3404255319148936,
   0.3902439024390244,
   0.4477611940298507,
   0.358974358974359,
   0.2727272727272727,
   0.5128205128205129,
   0.30769230769230765,
   0.33333333333333326,
   0.711111111111111,
   0.4090909090909091,
   0.22857142857142856,
   0.14814814814814814,
   0.35,
   0.35000000000000003,
   0.380952380952381,
   0.5555555555555556,
   0.8275862068965518,
   0.3829787234042554,
   0.34285714285714286,
   0.45,
   0.34782608695652173,
   0.4324324324324324,
   0.5789473684210527,
   0.45161290322580644,
   0.4864864864864865,
   0.48000000000000004,
   0.43750000000000006,
   0.3684210526315789,
   0.48484848484848486,
   0.27586206896551724,
   0.47619047619047616,
   0.5384615384615384,
   0.3636363636363636,
   0.42857142857142855,
   0.3243243243243243,
   0.3243243243243243,
   0.43750000000000006,
   0.45714285714285713,
   0.6428571428571429,
   0.7647058823529411,
   0.4444444444444445,
   0.3913043478260869,
   0.42857142857142855,
   0.4444444444444444,
   0.3571428571428571,
   0.5517241379310345,
   0.35294117647058826,
   0.5405405405405405,
   0.5806451612903226,
   0.37735849056603776,
   0.5,
   0.3414634146341463]]}

In [87]: sts_dict = {}
    ...: for ind, i in enumerate(sts_scores):
    ...:     k = get_key(i)
    ...:     if k == None:
    ...:         continue
    ...:     if k not in sts_dict:
    ...:         sts_dict[k] = [1, [i], [smatch_scores[ind]]]
    ...:     else:
    ...:         sts_dict[k][0] += 1
    ...:         sts_dict[k][1].append(i)
    ...:         sts_dict[k][2].append(smatch_scores[ind])
    ...: 

In [88]: 

In [88]: sts_dict
Out[88]: 
{0.2: [615,
  [0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.083,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.1,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.143,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.067,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.118,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.17,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.2,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0],
  [0.8,
   0.5,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.43478260869565216,
   0.5,
   0.4,
   0.5714285714285715,
   0.3333333333333333,
   0.4,
   0.14285714285714288,
   0.4444444444444445,
   0.2,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.125,
   0.22222222222222224,
   0.6,
   0.5,
   0.6,
   0.4,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.5714285714285715,
   0.28571428571428575,
   0.5,
   0.42857142857142855,
   0.28571428571428575,
   0.375,
   0.25,
   0.375,
   0.5,
   0.2727272727272727,
   0.3333333333333333,
   0.28571428571428575,
   0.2222222222222222,
   0.380952380952381,
   0.2,
   0.28571428571428575,
   0.21428571428571427,
   0.17391304347826086,
   0.1,
   0.25,
   0.38461538461538464,
   0.16,
   0.36363636363636365,
   0.25,
   0.4,
   0.2727272727272727,
   0.16,
   0.4444444444444445,
   0.20689655172413793,
   0.3636363636363636,
   0.3,
   0.25,
   0.20000000000000004,
   0.25,
   0.14285714285714288,
   0.22222222222222224,
   0.3529411764705882,
   0.10526315789473685,
   0.3870967741935484,
   0.25,
   0.3333333333333333,
   0.2631578947368421,
   0.28571428571428575,
   0.3157894736842105,
   0.15384615384615383,
   0.23529411764705885,
   0.18749999999999997,
   0.2105263157894737,
   0.18181818181818182,
   0.3,
   0.13793103448275862,
   0.2105263157894737,
   0.28571428571428575,
   0.07142857142857142,
   0.31250000000000006,
   0.16666666666666666,
   0.1818181818181818,
   0.3846153846153846,
   0.17543859649122806,
   0.18867924528301885,
   0.20408163265306123,
   0.22857142857142854,
   0.163265306122449,
   0.17777777777777778,
   0.11764705882352941,
   0.25,
   0.12903225806451615,
   0.17142857142857143,
   0.1886792452830189,
   0.22857142857142854,
   0.2711864406779661,
   0.22727272727272727,
   0.24999999999999994,
   0.1923076923076923,
   0.35000000000000003,
   0.13333333333333333,
   0.3018867924528302,
   0.23529411764705882,
   0.22950819672131148,
   0.2909090909090909,
   0.22857142857142856,
   0.13043478260869565,
   0.13793103448275862,
   0.2,
   0.13333333333333333,
   0.3225806451612903,
   0.25,
   0.1694915254237288,
   0.23076923076923078,
   0.09523809523809522,
   0.23529411764705882,
   0.2105263157894737,
   0.3333333333333333,
   0.27027027027027023,
   0.21739130434782608,
   0.2222222222222222,
   0.15384615384615383,
   0.2,
   0.24000000000000002,
   0.3225806451612903,
   0.27027027027027023,
   0.11320754716981131,
   0.24242424242424243,
   0.3255813953488372,
   0.24242424242424243,
   0.12244897959183673,
   0.16666666666666663,
   0.13636363636363638,
   0.2222222222222222,
   0.1754385964912281,
   0.16666666666666666,
   0.23529411764705882,
   0.45454545454545453,
   0.27027027027027023,
   0.16666666666666663,
   0.14285714285714288,
   0.2711864406779661,
   0.25925925925925924,
   0.23809523809523808,
   0.25,
   0.2191780821917808,
   0.20408163265306123,
   0.2631578947368421,
   0.20512820512820512,
   0.23529411764705882,
   0.41025641025641024,
   0.3571428571428571,
   0.2,
   0.33333333333333337,
   0.38888888888888884,
   0.2857142857142857,
   0.4186046511627907,
   0.4285714285714286,
   0.37209302325581395,
   0.3448275862068966,
   0.30303030303030304,
   0.42105263157894735,
   0.39999999999999997,
   0.5625,
   0.4666666666666667,
   0.25641025641025644,
   0.16,
   0.4375,
   0.26315789473684204,
   0.5365853658536585,
   0.23529411764705882,
   0.3428571428571428,
   0.4571428571428572,
   0.4090909090909091,
   0.4313725490196078,
   0.8,
   0.5,
   0.5,
   0.5,
   0.6666666666666666,
   0.5,
   0.6,
   0.4,
   0.5,
   0.6666666666666666,
   0.3333333333333333,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.30769230769230765,
   0.39999999999999997,
   0.28571428571428575,
   0.5,
   0.4,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.4615384615384615,
   0.3333333333333333,
   0.3333333333333333,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.5,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.37499999999999994,
   0.42857142857142855,
   0.28571428571428575,
   0.3333333333333333,
   0.28571428571428575,
   0.26666666666666666,
   0.39999999999999997,
   0.26666666666666666,
   0.42857142857142855,
   0.380952380952381,
   0.2857142857142857,
   0.1739130434782609,
   0.4,
   0.28571428571428575,
   0.3157894736842105,
   0.5333333333333333,
   0.28571428571428575,
   0.3333333333333333,
   0.3157894736842105,
   0.3333333333333333,
   0.4,
   0.25,
   0.3,
   0.16,
   0.21052631578947364,
   0.37499999999999994,
   0.25,
   0.30769230769230765,
   0.3333333333333333,
   0.42857142857142855,
   0.39999999999999997,
   0.75,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.5714285714285715,
   0.2857142857142857,
   0.4705882352941177,
   0.4,
   0.5,
   0.5714285714285715,
   0.5,
   0.5,
   0.16666666666666666,
   0.42857142857142855,
   0.3636363636363636,
   0.375,
   0.4,
   0.42857142857142855,
   0.26666666666666666,
   0.42857142857142855,
   0.3333333333333333,
   0.42857142857142855,
   0.13333333333333333,
   0.26666666666666666,
   0.28571428571428575,
   0.4444444444444445,
   0.42857142857142855,
   0.5,
   0.4,
   0.28571428571428575,
   0.35294117647058826,
   0.5,
   0.26666666666666666,
   0.37499999999999994,
   0.5,
   0.37499999999999994,
   0.23529411764705885,
   0.3333333333333333,
   0.4,
   0.3333333333333333,
   0.42857142857142855,
   0.3333333333333333,
   0.5,
   0.3333333333333333,
   0.3333333333333333,
   0.37499999999999994,
   0.375,
   0.4,
   0.37499999999999994,
   0.42857142857142855,
   0.37499999999999994,
   0.2105263157894737,
   0.3157894736842105,
   0.375,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.375,
   0.28571428571428575,
   0.5555555555555556,
   0.2758620689655172,
   0.25,
   0.20000000000000004,
   0.25,
   0.34285714285714286,
   0.11111111111111112,
   0.1818181818181818,
   0.19354838709677416,
   0.47058823529411764,
   0.21428571428571427,
   0.16666666666666666,
   0.32,
   0.4210526315789474,
   0.3333333333333333,
   0.22222222222222224,
   0.25,
   0.3636363636363636,
   0.11764705882352942,
   0.3,
   0.3,
   0.4,
   0.2758620689655172,
   0.4166666666666667,
   0.3181818181818182,
   0.25,
   0.28571428571428575,
   0.2727272727272727,
   0.37499999999999994,
   0.3157894736842105,
   0.18749999999999997,
   0.27586206896551724,
   0.42857142857142855,
   0.3157894736842105,
   0.29411764705882354,
   0.31250000000000006,
   0.5217391304347826,
   0.3,
   0.24000000000000002,
   0.17391304347826086,
   0.4444444444444445,
   0.4,
   0.19999999999999998,
   0.375,
   0.33333333333333337,
   0.43478260869565216,
   0.33333333333333337,
   0.380952380952381,
   0.42857142857142855,
   0.09090909090909091,
   0.5,
   0.20689655172413793,
   0.5555555555555556,
   0.07142857142857144,
   0.25,
   0.3478260869565218,
   0.18181818181818182,
   0.16666666666666666,
   0.29629629629629634,
   0.4000000000000001,
   0.25,
   0.26666666666666666,
   0.2727272727272727,
   0.16,
   0.1904761904761905,
   0.19354838709677422,
   0.3870967741935483,
   0.3333333333333333,
   0.24000000000000002,
   0.28571428571428564,
   0.14285714285714288,
   0.5,
   0.24999999999999994,
   0.32,
   0.37499999999999994,
   0.3225806451612903,
   0.31250000000000006,
   0.08695652173913043,
   0.17391304347826086,
   0.3,
   0.3076923076923077,
   0.27586206896551724,
   0.2777777777777778,
   0.2857142857142857,
   0.33333333333333326,
   0.36363636363636365,
   0.4000000000000001,
   0.33333333333333326,
   0.4666666666666667,
   0.21428571428571427,
   0.19047619047619047,
   0.5,
   0.23999999999999996,
   0.2,
   0.375,
   0.22222222222222224,
   0.21428571428571427,
   0.3636363636363636,
   0.3333333333333333,
   0.2631578947368421,
   0.3333333333333333,
   0.22857142857142854,
   0.26086956521739135,
   0.48,
   0.30769230769230765,
   0.23076923076923075,
   0.375,
   0.3,
   0.25,
   0.16666666666666663,
   0.16,
   0.28571428571428575,
   0.24242424242424246,
   0.15384615384615385,
   0.5333333333333333,
   0.33333333333333337,
   0.3157894736842105,
   0.2608695652173913,
   0.6666666666666665,
   0.3225806451612903,
   0.23076923076923075,
   0.25,
   0.4000000000000001,
   0.23076923076923075,
   0.2,
   0.6206896551724138,
   0.41025641025641024,
   0.25,
   0.5517241379310344,
   0.3636363636363636,
   0.4680851063829788,
   0.15384615384615383,
   0.26666666666666666,
   0.631578947368421,
   0.5,
   0.5161290322580646,
   0.5625,
   0.39999999999999997,
   0.4390243902439024,
   0.631578947368421,
   0.6153846153846153,
   0.36842105263157887,
   0.42105263157894735,
   0.22857142857142856,
   0.4666666666666667,
   0.3414634146341463,
   0.2857142857142857,
   0.30769230769230765,
   0.4375,
   0.30769230769230765,
   0.3,
   0.27777777777777773,
   0.42857142857142855,
   0.3225806451612903,
   0.13333333333333333,
   0.4444444444444444,
   0.625,
   0.14814814814814814,
   0.3870967741935483,
   0.25,
   0.36363636363636365,
   0.3333333333333333,
   0.36363636363636365,
   0.35714285714285715,
   0.3111111111111111,
   0.2162162162162162,
   0.25641025641025644,
   0.5853658536585366,
   0.411764705882353,
   0.6666666666666666,
   0.22222222222222224,
   0.7199999999999999,
   0.4,
   0.26666666666666666,
   0.3333333333333333,
   0.5416666666666667,
   0.16,
   0.22857142857142856,
   0.3333333333333333,
   0.3333333333333333,
   0.4,
   0.18181818181818182,
   0.3076923076923077,
   0.3870967741935484,
   0.3448275862068966,
   0.3225806451612903,
   0.43902439024390244,
   0.34285714285714286,
   0.4210526315789474,
   0.35000000000000003,
   0.46808510638297873,
   0.34285714285714286,
   0.24999999999999994,
   0.358974358974359,
   0.4,
   0.6153846153846153,
   0.375,
   0.22222222222222224,
   0.358974358974359,
   0.34782608695652173,
   0.35294117647058826,
   0.3448275862068966,
   0.5581395348837209,
   0.43999999999999995,
   0.2424242424242424,
   0.23076923076923075,
   0.13333333333333333,
   0.13333333333333333,
   0.45161290322580644,
   0.33333333333333326,
   0.3684210526315789,
   0.6842105263157895,
   0.4864864864864865,
   0.5217391304347826,
   0.35294117647058826,
   0.26666666666666666,
   0.26666666666666666,
   0.4897959183673469,
   0.3333333333333333,
   0.6060606060606061,
   0.7027027027027027,
   0.22857142857142856,
   0.5306122448979592,
   0.3448275862068966,
   0.16666666666666666,
   0.4074074074074074,
   0.2631578947368421,
   0.3181818181818182,
   0.7647058823529412,
   0.3,
   0.4090909090909091,
   0.18181818181818182,
   0.39999999999999997,
   0.22857142857142856,
   0.47058823529411764,
   0.3333333333333333,
   0.3,
   0.1904761904761905,
   0.35294117647058826,
   0.3333333333333333,
   0.5106382978723405,
   0.2777777777777778,
   0.3888888888888889,
   0.3125,
   0.24242424242424243,
   0.3333333333333333,
   0.3888888888888889,
   0.4081632653061225,
   0.6046511627906976,
   0.45,
   0.5555555555555556,
   0.11764705882352941,
   0.29411764705882354,
   0.34285714285714286,
   0.6666666666666666,
   0.5957446808510638,
   0.4166666666666667,
   0.6818181818181819,
   0.6382978723404256,
   0.8181818181818182,
   0.5217391304347826,
   0.4615384615384615,
   0.52,
   0.6285714285714286,
   0.5,
   0.4848484848484849,
   0.14814814814814817,
   0.4444444444444444,
   0.4150943396226415,
   0.5714285714285715,
   0.4864864864864864,
   0.375,
   0.36,
   0.29411764705882354,
   0.46511627906976744,
   0.558139534883721,
   0.4444444444444445,
   0.3333333333333333,
   0.38095238095238093,
   0.42424242424242425,
   0.41025641025641024,
   0.34285714285714286,
   0.3333333333333333,
   0.47619047619047616,
   0.30769230769230765,
   0.1904761904761905]],
 0.8: [211,
  [0.8,
   0.636,
   0.8,
   0.8,
   0.778,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.67,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.667,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.643,
   0.75,
   0.8,
   0.727,
   0.8,
   0.8,
   0.8,
   0.8,
   0.667,
   0.8,
   0.8,
   0.75,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.8,
   0.75,
   0.8,
   0.8,
   0.75,
   0.75,
   0.75,
   0.75,
   0.8,
   0.667,
   0.8,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.75,
   0.8,
   0.75,
   0.8,
   0.75,
   0.75,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8,
   0.8],
  [0.6666666666666666,
   0.75,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.375,
   0.6666666666666666,
   0.5714285714285715,
   0.4444444444444444,
   0.6666666666666666,
   0.20000000000000004,
   0.5333333333333333,
   0.3636363636363636,
   0.3225806451612903,
   0.29629629629629634,
   0.21621621621621623,
   0.6,
   0.20689655172413793,
   0.6666666666666665,
   0.3684210526315789,
   0.3703703703703704,
   0.36363636363636365,
   0.3333333333333333,
   0.16666666666666666,
   0.3050847457627119,
   0.25,
   0.17142857142857143,
   0.2153846153846154,
   0.32727272727272727,
   0.2545454545454545,
   0.339622641509434,
   0.14634146341463417,
   0.1904761904761905,
   0.4,
   0.2,
   0.2222222222222222,
   0.3125,
   0.13333333333333333,
   0.5,
   0.3829787234042554,
   0.3255813953488372,
   0.29166666666666663,
   0.3684210526315789,
   0.375,
   0.5882352941176471,
   0.358974358974359,
   0.48648648648648646,
   0.6521739130434783,
   0.6111111111111112,
   0.5909090909090909,
   0.75,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.4444444444444445,
   0.6,
   0.5714285714285715,
   0.3529411764705882,
   0.6250000000000001,
   0.5714285714285715,
   0.5333333333333333,
   0.5714285714285715,
   0.4210526315789474,
   0.36363636363636365,
   0.5714285714285715,
   0.375,
   0.6666666666666665,
   0.5,
   0.75,
   0.6666666666666666,
   0.7142857142857143,
   0.5714285714285715,
   0.5,
   0.42857142857142855,
   0.5714285714285715,
   0.6,
   0.6666666666666666,
   0.3333333333333333,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.6,
   0.5,
   0.6153846153846153,
   0.6,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.33333333333333326,
   0.5714285714285715,
   0.35294117647058826,
   0.5,
   0.4444444444444445,
   0.37499999999999994,
   0.6,
   0.28571428571428564,
   0.42857142857142855,
   0.4,
   0.5,
   0.4,
   0.4000000000000001,
   0.23076923076923078,
   0.3636363636363636,
   0.14285714285714288,
   0.625,
   0.30769230769230765,
   0.2857142857142857,
   0.625,
   0.6666666666666666,
   0.33333333333333326,
   0.5,
   0.2727272727272727,
   0.48484848484848486,
   0.6666666666666665,
   0.4444444444444445,
   0.3703703703703704,
   0.37499999999999994,
   0.6153846153846153,
   0.25,
   0.1875,
   0.41379310344827586,
   0.3333333333333333,
   0.3636363636363637,
   0.3,
   0.41379310344827586,
   0.2,
   0.3571428571428571,
   0.46153846153846156,
   0.5714285714285715,
   0.4666666666666667,
   0.35714285714285715,
   0.36363636363636365,
   0.47058823529411764,
   0.47058823529411764,
   0.5454545454545454,
   0.7450980392156864,
   0.7272727272727273,
   0.5925925925925926,
   0.5,
   0.4210526315789474,
   0.6666666666666665,
   0.23076923076923078,
   0.5,
   0.3888888888888889,
   0.5333333333333332,
   0.3255813953488372,
   0.23529411764705882,
   0.4814814814814815,
   0.7407407407407408,
   0.5531914893617023,
   0.4680851063829788,
   0.5,
   0.39024390243902435,
   0.6938775510204083,
   0.3448275862068966,
   0.5555555555555556,
   0.7142857142857142,
   0.5714285714285714,
   0.35,
   0.5454545454545455,
   0.5777777777777778,
   0.4,
   0.6190476190476191,
   0.6666666666666666,
   0.34285714285714286,
   0.7058823529411765,
   0.6086956521739131,
   0.29411764705882354,
   0.7500000000000001,
   0.3404255319148936,
   0.46511627906976744,
   0.37499999999999994,
   0.5142857142857143,
   0.625,
   0.3902439024390244,
   0.7741935483870969,
   0.6818181818181818,
   0.3529411764705882,
   0.39999999999999997,
   0.35897435897435903,
   0.5454545454545454,
   0.43749999999999994,
   0.5625,
   0.25925925925925924,
   0.43243243243243246,
   0.5625,
   0.5416666666666667,
   0.7368421052631577,
   0.33333333333333337,
   0.6315789473684211,
   0.5454545454545454,
   0.3,
   0.5161290322580646,
   0.3728813559322034,
   0.43749999999999994,
   0.7894736842105263,
   0.7333333333333334,
   0.7741935483870968,
   0.34146341463414637,
   0.5185185185185186,
   0.6666666666666666,
   0.5405405405405405,
   0.39999999999999997,
   0.6896551724137931,
   0.41025641025641024,
   0.3714285714285715]],
 1.0: [264,
  [1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.833,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.85,
   1.0,
   0.833,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.9,
   0.9,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.944,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.889,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0],
  [0.8333333333333334,
   0.6,
   0.6666666666666666,
   0.4210526315789474,
   0.4444444444444445,
   0.5714285714285715,
   0.6666666666666666,
   0.4666666666666667,
   0.3,
   0.36363636363636365,
   0.2,
   0.3157894736842105,
   0.6,
   0.35714285714285715,
   0.2962962962962963,
   0.3846153846153846,
   0.15384615384615383,
   0.35294117647058826,
   0.20689655172413793,
   0.14285714285714285,
   0.21739130434782608,
   0.10526315789473684,
   0.2790697674418605,
   0.2745098039215686,
   0.2127659574468085,
   0.25,
   0.23076923076923078,
   0.2790697674418605,
   0.1951219512195122,
   0.27777777777777773,
   0.2926829268292683,
   0.2857142857142857,
   0.09302325581395349,
   0.3829787234042554,
   0.3636363636363636,
   0.39024390243902435,
   0.5405405405405405,
   0.5128205128205129,
   0.2222222222222222,
   0.42424242424242425,
   0.25,
   0.6470588235294117,
   0.4,
   0.5217391304347826,
   0.358974358974359,
   0.372093023255814,
   0.6666666666666666,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6666666666666666,
   0.5,
   0.5,
   0.4,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.5882352941176471,
   0.4705882352941177,
   0.6666666666666666,
   0.6666666666666666,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.6153846153846153,
   0.5714285714285715,
   0.4,
   0.42857142857142855,
   0.6666666666666666,
   0.4615384615384615,
   0.47619047619047616,
   0.6666666666666666,
   0.5,
   0.37499999999999994,
   0.4444444444444444,
   0.42857142857142855,
   0.5333333333333333,
   0.4444444444444444,
   0.4166666666666667,
   0.47058823529411764,
   0.4761904761904762,
   0.35714285714285715,
   0.2758620689655172,
   0.5555555555555556,
   0.33333333333333326,
   0.36363636363636365,
   0.16,
   0.5,
   0.47058823529411764,
   0.375,
   0.0909090909090909,
   0.33333333333333326,
   0.375,
   0.34782608695652173,
   0.2222222222222222,
   0.23076923076923075,
   0.25,
   0.3076923076923077,
   0.22857142857142854,
   0.35714285714285715,
   0.5517241379310345,
   0.6666666666666666,
   0.2,
   0.18181818181818182,
   0.5,
   0.4000000000000001,
   0.1702127659574468,
   0.35294117647058826,
   0.6875,
   0.6,
   0.4210526315789474,
   0.47058823529411764,
   0.7142857142857143,
   0.6363636363636365,
   0.3157894736842105,
   0.8461538461538461,
   0.7142857142857143,
   0.4666666666666667,
   0.4666666666666667,
   0.8000000000000002,
   0.5,
   0.8648648648648649,
   0.6666666666666666,
   0.5454545454545455,
   0.6428571428571429,
   0.6,
   0.3404255319148936,
   0.3333333333333333,
   0.5483870967741935,
   0.617283950617284,
   0.4888888888888888,
   0.3636363636363636,
   0.4523809523809524,
   0.6666666666666666,
   0.5964912280701754,
   0.42857142857142855,
   0.3404255319148936,
   0.4,
   0.3555555555555555,
   0.4197530864197531,
   0.8461538461538461,
   0.45714285714285713,
   0.24615384615384617,
   0.4444444444444444,
   0.5405405405405405,
   0.5925925925925926,
   0.48484848484848486,
   0.4,
   0.358974358974359,
   0.6111111111111113,
   0.41666666666666663,
   0.4666666666666667,
   0.48000000000000004,
   0.5,
   0.35714285714285715,
   0.6,
   0.45,
   0.4375,
   0.6428571428571429,
   0.49056603773584906,
   0.31818181818181823,
   0.4888888888888889,
   0.6857142857142857,
   0.4516129032258065,
   0.6923076923076924,
   0.7741935483870968,
   0.5862068965517241,
   0.47058823529411764,
   0.47368421052631576,
   0.5806451612903225,
   0.76,
   0.5625000000000001,
   0.4255319148936171,
   0.3333333333333333,
   0.28571428571428575,
   0.375,
   0.6376811594202899,
   0.4878048780487805,
   0.7857142857142857,
   0.5925925925925927,
   0.5116279069767442,
   0.4090909090909091,
   0.3902439024390244,
   0.6666666666666666,
   0.5652173913043478,
   0.5714285714285713,
   0.5384615384615384,
   0.3636363636363636,
   0.6666666666666667,
   0.75,
   0.5128205128205129,
   0.6206896551724139,
   0.4827586206896552,
   0.4782608695652174,
   0.5,
   0.5263157894736842,
   0.4583333333333333,
   0.4897959183673469,
   0.875,
   0.4736842105263158,
   0.46511627906976744,
   0.5833333333333334,
   0.43902439024390244,
   0.6666666666666666,
   0.358974358974359,
   0.3448275862068966,
   0.606060606060606,
   0.42857142857142855,
   0.3636363636363636,
   0.6666666666666666,
   0.3428571428571428,
   0.425531914893617,
   0.5,
   0.3902439024390244,
   0.4117647058823529,
   0.2285714285714286,
   0.85,
   0.5500000000000002,
   0.3829787234042554,
   0.5652173913043479,
   0.3888888888888889,
   0.43478260869565216,
   0.3636363636363636,
   0.409090909090909,
   0.3888888888888889,
   0.5925925925925926,
   0.45454545454545453,
   0.358974358974359,
   0.358974358974359,
   0.52,
   0.5625000000000001,
   0.3,
   0.22727272727272727,
   0.40816326530612246,
   0.9090909090909091,
   0.8636363636363636,
   0.6976744186046512,
   0.7692307692307692,
   0.7857142857142856,
   0.6206896551724138,
   0.4242424242424242,
   0.4242424242424242,
   0.7857142857142857,
   0.6274509803921569,
   0.6666666666666666,
   0.46808510638297873,
   0.5,
   0.6285714285714287,
   0.6315789473684211,
   0.7222222222222222,
   0.48484848484848486,
   0.6875000000000001,
   0.358974358974359,
   0.4324324324324324,
   0.42857142857142855,
   0.46511627906976744,
   0.5945945945945946,
   0.4666666666666667,
   0.5762711864406779,
   0.7199999999999999]],
 0.6: [190,
  [0.6,
   0.5,
   0.6,
   0.6,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.5,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.5,
   0.417,
   0.5,
   0.6,
   0.6,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.5,
   0.6,
   0.5,
   0.5,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6],
  [0.5,
   0.5263157894736842,
   0.6666666666666666,
   0.5,
   0.5,
   0.6666666666666666,
   0.6,
   0.5,
   0.6,
   0.6666666666666666,
   0.5714285714285715,
   0.380952380952381,
   0.5714285714285715,
   0.47058823529411764,
   0.5,
   0.34782608695652173,
   0.28571428571428575,
   0.5263157894736842,
   0.1,
   0.25,
   0.5,
   0.5555555555555556,
   0.28571428571428575,
   0.2758620689655172,
   0.22222222222222224,
   0.23529411764705882,
   0.25,
   0.13793103448275862,
   0.26666666666666666,
   0.2,
   0.28571428571428575,
   0.17391304347826086,
   0.13953488372093023,
   0.3714285714285714,
   0.1081081081081081,
   0.21052631578947367,
   0.21818181818181817,
   0.21538461538461542,
   0.13043478260869565,
   0.10714285714285714,
   0.1702127659574468,
   0.0930232558139535,
   0.2647058823529412,
   0.42553191489361697,
   0.1818181818181818,
   0.21052631578947367,
   0.24137931034482757,
   0.2608695652173913,
   0.18518518518518517,
   0.5714285714285714,
   0.5625000000000001,
   0.39999999999999997,
   0.43902439024390244,
   0.38888888888888884,
   0.1904761904761905,
   0.75,
   0.75,
   0.75,
   0.75,
   0.6,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6153846153846153,
   0.625,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.5714285714285715,
   0.42857142857142855,
   0.39999999999999997,
   0.3333333333333333,
   0.5384615384615384,
   0.42857142857142855,
   0.5454545454545454,
   0.42857142857142855,
   0.6666666666666666,
   0.3333333333333333,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.5714285714285715,
   0.37499999999999994,
   0.5,
   0.5,
   0.5714285714285715,
   0.6,
   0.5,
   0.5,
   0.4615384615384615,
   0.5555555555555556,
   0.5714285714285715,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.2857142857142857,
   0.5,
   0.17647058823529413,
   0.1904761904761905,
   0.6,
   0.22727272727272727,
   0.21428571428571427,
   0.22222222222222224,
   0.20000000000000004,
   0.6666666666666666,
   0.45454545454545453,
   0.3703703703703704,
   0.27027027027027023,
   0.5,
   0.3636363636363636,
   0.08695652173913043,
   0.2105263157894737,
   0.38709677419354843,
   0.14634146341463414,
   0.29629629629629634,
   0.37499999999999994,
   0.24242424242424243,
   0.23076923076923075,
   0.6666666666666666,
   0.3333333333333333,
   0.2,
   0.35714285714285715,
   0.2,
   0.5,
   0.33333333333333337,
   0.5714285714285715,
   0.3157894736842105,
   0.46153846153846156,
   0.32653061224489793,
   0.7142857142857142,
   0.31249999999999994,
   0.5652173913043478,
   0.6666666666666666,
   0.4090909090909091,
   0.35714285714285715,
   0.16666666666666666,
   0.64,
   0.33333333333333337,
   0.6829268292682927,
   0.7500000000000001,
   0.5,
   0.2857142857142857,
   0.3636363636363636,
   0.6315789473684211,
   0.5625000000000001,
   0.6666666666666667,
   0.6451612903225806,
   0.28571428571428575,
   0.4814814814814815,
   0.5555555555555556,
   0.3225806451612903,
   0.37837837837837834,
   0.2580645161290323,
   0.5263157894736842,
   0.4489795918367347,
   0.2727272727272727,
   0.6829268292682927,
   0.851063829787234,
   0.3783783783783784,
   0.7916666666666667,
   0.42857142857142855,
   0.3255813953488372,
   0.2926829268292683,
   0.4137931034482759,
   0.42857142857142855,
   0.2857142857142857,
   0.6341463414634146,
   0.6428571428571429,
   0.26666666666666666,
   0.47058823529411764,
   0.45,
   0.5777777777777777,
   0.4444444444444444,
   0.30769230769230765,
   0.39999999999999997,
   0.6428571428571429,
   0.6829268292682927,
   0.7272727272727272,
   0.6875,
   0.4,
   0.7142857142857143,
   0.358974358974359,
   0.6111111111111113,
   0.6000000000000001,
   0.3846153846153846,
   0.4615384615384615,
   0.35,
   0.4615384615384615,
   0.4736842105263158]],
 0.4: [214,
  [0.25,
   0.25,
   0.25,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.333,
   0.333,
   0.25,
   0.4,
   0.4,
   0.25,
   0.25,
   0.4,
   0.4,
   0.4,
   0.25,
   0.25,
   0.25,
   0.4,
   0.25,
   0.25,
   0.4,
   0.25,
   0.4,
   0.25,
   0.4,
   0.4,
   0.25,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.231,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.25,
   0.333,
   0.4,
   0.25,
   0.333,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.25,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4],
  [0.5,
   0.4,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.4,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6153846153846153,
   0.375,
   0.28571428571428575,
   0.2,
   0.4444444444444445,
   0.5555555555555556,
   0.3448275862068965,
   0.36363636363636365,
   0.3243243243243243,
   0.34782608695652173,
   0.24242424242424246,
   0.20512820512820512,
   0.1379310344827586,
   0.3636363636363637,
   0.25,
   0.34285714285714286,
   0.33333333333333337,
   0.10526315789473685,
   0.29629629629629634,
   0.3,
   0.3,
   0.11320754716981132,
   0.22727272727272724,
   0.509090909090909,
   0.1904761904761905,
   0.22222222222222224,
   0.25,
   0.23809523809523808,
   0.22580645161290322,
   0.2,
   0.16,
   0.27906976744186046,
   0.19512195121951217,
   0.27027027027027023,
   0.1923076923076923,
   0.3673469387755102,
   0.04761904761904762,
   0.2285714285714286,
   0.3333333333333333,
   0.43749999999999994,
   0.5,
   0.3636363636363636,
   0.1764705882352941,
   0.4864864864864865,
   0.5,
   0.4680851063829788,
   0.6470588235294118,
   0.5652173913043479,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.26666666666666666,
   0.6666666666666666,
   0.6,
   0.5,
   0.5333333333333333,
   0.6666666666666666,
   0.4210526315789474,
   0.13333333333333333,
   0.375,
   0.42857142857142855,
   0.5,
   0.2857142857142857,
   0.5882352941176471,
   0.5,
   0.37499999999999994,
   0.6,
   0.28571428571428575,
   0.6666666666666666,
   0.6,
   0.6,
   0.5,
   0.3333333333333333,
   0.6153846153846153,
   0.42857142857142855,
   0.6666666666666666,
   0.6,
   0.6,
   0.5714285714285715,
   0.5,
   0.5714285714285715,
   0.5714285714285714,
   0.5714285714285715,
   0.5,
   0.5,
   0.375,
   0.3333333333333333,
   0.5,
   0.4,
   0.6666666666666666,
   0.25,
   0.4444444444444444,
   0.4705882352941177,
   0.6666666666666666,
   0.5,
   0.375,
   0.6666666666666666,
   0.5,
   0.375,
   0.28571428571428575,
   0.2857142857142857,
   0.5,
   0.5,
   0.3703703703703703,
   0.48000000000000004,
   0.42857142857142855,
   0.39999999999999997,
   0.30303030303030304,
   0.29411764705882354,
   0.3076923076923077,
   0.28571428571428575,
   0.25,
   0.47619047619047616,
   0.33333333333333326,
   0.26666666666666666,
   0.3,
   0.25,
   0.47058823529411764,
   0.4444444444444445,
   0.625,
   0.3,
   0.3636363636363637,
   0.18749999999999997,
   0.3333333333333333,
   0.26666666666666666,
   0.45454545454545453,
   0.22222222222222224,
   0.2727272727272727,
   0.30769230769230765,
   0.3,
   0.5714285714285714,
   0.24390243902439024,
   0.2,
   0.5806451612903225,
   0.14814814814814817,
   0.2857142857142857,
   0.3333333333333333,
   0.2380952380952381,
   0.5714285714285715,
   0.7407407407407408,
   0.75,
   0.5714285714285714,
   0.3333333333333333,
   0.3829787234042554,
   0.4680851063829787,
   0.8571428571428571,
   0.31250000000000006,
   0.5,
   0.3404255319148936,
   0.3902439024390244,
   0.4477611940298507,
   0.358974358974359,
   0.2727272727272727,
   0.5128205128205129,
   0.30769230769230765,
   0.33333333333333326,
   0.711111111111111,
   0.4090909090909091,
   0.22857142857142856,
   0.14814814814814814,
   0.35,
   0.35000000000000003,
   0.380952380952381,
   0.5555555555555556,
   0.8275862068965518,
   0.3829787234042554,
   0.34285714285714286,
   0.45,
   0.34782608695652173,
   0.4324324324324324,
   0.5789473684210527,
   0.45161290322580644,
   0.4864864864864865,
   0.48000000000000004,
   0.43750000000000006,
   0.3684210526315789,
   0.48484848484848486,
   0.27586206896551724,
   0.47619047619047616,
   0.5384615384615384,
   0.3636363636363636,
   0.42857142857142855,
   0.3243243243243243,
   0.3243243243243243,
   0.43750000000000006,
   0.45714285714285713,
   0.6428571428571429,
   0.7647058823529411,
   0.4444444444444445,
   0.3913043478260869,
   0.42857142857142855,
   0.4444444444444444,
   0.3571428571428571,
   0.5517241379310345,
   0.35294117647058826,
   0.5405405405405405,
   0.5806451612903226,
   0.37735849056603776,
   0.5,
   0.3414634146341463]]}

In [89]: 

In [89]: for i in sts_dict:
    ...:     print (sts_dict[i][0])
    ...: 
615
211
264
190
214

In [90]: count = 200
    ...: for i in sts_dict:
    ...:     temp_df = pd.DataFrame({})
    ...:     temp_df["sts_bucket"] = [i]*190
    ...:     temp_df["smatch"] = sts_dict[i][2][:190]
    ...:     temp_df["sts_score"] = sts_dict[i][1][:190]
    ...:     df = df.append(temp_df, ignore_index=True)
    ...: 
    ...: 
    ...: 
    ...: 

In [91]: df
Out[91]: 
      sts_bucket    smatch  sts_score
0            0.2  0.800000        NaN
1            0.2  0.500000        NaN
2            0.2  0.428571        NaN
3            0.2  0.500000        NaN
4            0.2  0.333333        NaN
...          ...       ...        ...
4905         0.4  0.451613        0.4
4906         0.4  0.486486        0.4
4907         0.4  0.480000        0.4
4908         0.4  0.437500        0.4
4909         0.4  0.368421        0.4

[4910 rows x 3 columns]

In [92]: df = pd.DataFrame({})

In [93]: count = 200
    ...: for i in sts_dict:
    ...:     temp_df = pd.DataFrame({})
    ...:     temp_df["sts_bucket"] = [i]*190
    ...:     temp_df["smatch"] = sts_dict[i][2][:190]
    ...:     temp_df["sts_score"] = sts_dict[i][1][:190]
    ...:     df = df.append(temp_df, ignore_index=True)
    ...: 
    ...: 
    ...: 
    ...: 

In [94]: df
Out[94]: 
     sts_bucket    smatch  sts_score
0           0.2  0.800000        0.0
1           0.2  0.500000        0.0
2           0.2  0.428571        0.0
3           0.2  0.500000        0.0
4           0.2  0.333333        0.0
..          ...       ...        ...
945         0.4  0.451613        0.4
946         0.4  0.486486        0.4
947         0.4  0.480000        0.4
948         0.4  0.437500        0.4
949         0.4  0.368421        0.4

[950 rows x 3 columns]

In [95]: 

In [95]: sns.scatterplot(x="smatch", y="sts_score", data=df)
Out[95]: <AxesSubplot:xlabel='smatch', ylabel='sts_score'>

In [96]: 

In [96]: plt.show()

In [97]: from scipy import stats

In [98]: stats.spearmanr(df["smatch"].to_list(), df["sts_score"].to_list())
Out[98]: SpearmanrResult(correlation=0.30053210016979054, pvalue=2.782042736210707e-21)

In [99]: sts_scores
Out[99]: 
[0.0,
 5.0,
 4.75,
 5.0,
 2.4,
 2.75,
 2.615,
 5.0,
 2.333,
 3.75,
 5.0,
 3.2,
 1.583,
 5.0,
 5.0,
 4.909,
 0.8,
 2.4,
 5.0,
 4.0,
 0.636,
 3.0,
 1.714,
 3.2,
 2.167,
 1.0,
 1.917,
 4.25,
 3.0,
 1.0,
 0.6,
 2.6,
 5.0,
 4.6,
 5.0,
 4.8,
 3.8,
 5.0,
 5.0,
 4.2,
 1.4,
 3.6,
 2.8,
 1.6,
 3.0,
 1.4,
 0.25,
 0.25,
 0.0,
 4.0,
 4.5,
 0.5,
 3.8,
 4.8,
 5.0,
 0.25,
 1.2,
 0.6,
 0.8,
 3.8,
 0.0,
 3.5,
 4.5,
 2.8,
 3.8,
 3.8,
 0.0,
 4.0,
 4.25,
 2.812,
 4.25,
 3.0,
 1.0,
 3.75,
 0.0,
 0.4,
 4.0,
 2.8,
 3.75,
 1.154,
 2.75,
 2.8,
 0.0,
 0.0,
 3.4,
 5.0,
 0.8,
 2.25,
 2.75,
 4.5,
 2.6,
 3.8,
 2.8,
 1.6,
 0.0,
 1.333,
 2.6,
 0.6,
 0.0,
 0.0,
 3.0,
 0.0,
 0.2,
 3.2,
 2.0,
 0.0,
 3.0,
 3.091,
 2.75,
 1.2,
 0.5,
 0.25,
 0.0,
 0.0,
 0.5,
 0.0,
 0.6,
 4.0,
 3.4,
 0.0,
 0.0,
 1.0,
 0.0,
 2.4,
 0.4,
 1.8,
 2.5,
 0.083,
 0.0,
 1.0,
 4.5,
 0.0,
 3.6,
 5.0,
 5.0,
 5.0,
 5.0,
 3.8,
 5.0,
 2.5,
 3.824,
 1.6,
 5.0,
 5.0,
 2.375,
 5.0,
 1.25,
 1.25,
 3.0,
 2.167,
 1.4,
 4.0,
 3.6,
 4.857,
 0.4,
 0.2,
 1.3,
 1.2,
 1.2,
 4.4,
 1.8,
 1.4,
 0.4,
 4.4,
 3.25,
 0.778,
 2.25,
 2.75,
 2.0,
 0.833,
 3.75,
 1.8,
 4.333,
 4.214,
 0.0,
 3.4,
 4.2,
 0.8,
 4.2,
 2.75,
 2.2,
 1.2,
 1.0,
 1.533,
 0.2,
 3.0,
 3.8,
 0.75,
 3.0,
 0.4,
 3.4,
 3.8,
 1.4,
 3.4,
 3.2,
 2.333,
 0.8,
 0.0,
 3.0,
 3.75,
 0.0,
 0.0,
 0.0,
 0.5,
 0.5,
 0.4,
 0.75,
 2.5,
 1.8,
 2.5,
 0.5,
 0.4,
 1.2,
 2.75,
 0.4,
 0.6,
 0.8,
 3.0,
 0.4,
 3.2,
 1.25,
 5.0,
 0.2,
 3.0,
 1.4,
 3.8,
 2.75,
 0.0,
 2.8,
 0.0,
 0.0,
 2.6,
 0.1,
 0.0,
 2.0,
 3.75,
 3.1,
 2.692,
 4.429,
 5.0,
 0.0,
 0.8,
 1.333,
 0.0,
 0.6,
 0.0,
 0.0,
 0.0,
 3.4,
 2.2,
 0.0,
 3.6,
 0.0,
 1.4,
 2.2,
 3.8,
 2.6,
 0.4,
 4.0,
 2.25,
 3.2,
 0.0,
 0.4,
 3.8,
 0.8,
 4.2,
 3.6,
 2.0,
 4.2,
 3.4,
 3.0,
 3.4,
 3.6,
 3.0,
 2.4,
 2.0,
 4.0,
 0.0,
 4.0,
 4.2,
 0.8,
 2.2,
 3.8,
 3.2,
 4.4,
 0.0,
 1.4,
 2.6,
 0.4,
 0.0,
 3.2,
 4.6,
 0.0,
 0.6,
 1.2,
 3.8,
 3.2,
 2.6,
 5.0,
 0.0,
 3.2,
 4.0,
 1.2,
 4.4,
 3.4,
 4.4,
 0.8,
 4.6,
 4.2,
 0.0,
 3.2,
 0.0,
 1.4,
 3.2,
 1.8,
 1.8,
 0.0,
 3.8,
 3.8,
 4.0,
 0.0,
 3.2,
 1.6,
 3.6,
 1.0,
 3.6,
 2.0,
 3.6,
 4.0,
 3.6,
 3.2,
 2.8,
 2.4,
 3.6,
 1.8,
 0.2,
 3.4,
 1.2,
 1.4,
 2.6,
 2.4,
 0.0,
 4.0,
 3.0,
 4.0,
 4.0,
 2.0,
 4.0,
 2.2,
 2.2,
 3.4,
 3.2,
 4.0,
 3.2,
 3.8,
 3.0,
 4.0,
 2.2,
 3.4,
 3.8,
 0.0,
 0.0,
 4.8,
 3.0,
 0.8,
 4.2,
 4.2,
 0.0,
 4.2,
 4.6,
 5.0,
 0.0,
 3.2,
 2.6,
 2.2,
 4.6,
 5.0,
 4.6,
 4.6,
 4.8,
 0.6,
 0.2,
 2.2,
 4.8,
 1.2,
 2.2,
 4.6,
 2.6,
 3.6,
 0.8,
 2.4,
 4.8,
 5.0,
 0.4,
 3.2,
 1.8,
 3.2,
 3.4,
 4.8,
 4.2,
 2.6,
 2.2,
 1.4,
 2.6,
 1.2,
 1.8,
 4.0,
 0.4,
 0.0,
 0.4,
 3.0,
 4.0,
 1.4,
 0.4,
 2.4,
 2.8,
 4.6,
 4.2,
 3.2,
 1.2,
 1.8,
 2.6,
 1.6,
 0.0,
 3.8,
 4.0,
 4.8,
 2.4,
 5.0,
 0.0,
 3.6,
 2.4,
 4.2,
 0.2,
 4.2,
 3.2,
 0.6,
 1.6,
 0.0,
 1.4,
 4.8,
 4.0,
 3.0,
 0.2,
 1.6,
 4.4,
 4.8,
 0.4,
 2.4,
 3.0,
 2.0,
 4.6,
 1.0,
 5.0,
 1.4,
 0.0,
 3.0,
 0.6,
 0.0,
 2.6,
 1.2,
 5.0,
 3.4,
 0.8,
 0.8,
 1.0,
 0.0,
 0.0,
 2.0,
 2.4,
 2.2,
 3.8,
 2.2,
 4.6,
 2.8,
 2.0,
 4.2,
 4.5,
 0.0,
 1.8,
 4.2,
 4.2,
 1.4,
 3.6,
 0.6,
 5.0,
 0.8,
 0.0,
 0.0,
 1.8,
 0.8,
 2.8,
 0.0,
 0.8,
 1.8,
 1.4,
 1.8,
 2.4,
 1.6,
 3.8,
 4.8,
 0.2,
 1.0,
 0.4,
 0.4,
 4.0,
 3.4,
 3.0,
 1.8,
 2.2,
 3.6,
 0.4,
 0.2,
 3.8,
 4.2,
 1.2,
 3.4,
 2.4,
 3.2,
 2.2,
 4.4,
 2.6,
 0.2,
 3.2,
 2.2,
 5.0,
 5.0,
 2.2,
 0.4,
 1.0,
 2.2,
 2.0,
 1.2,
 4.0,
 1.0,
 4.2,
 3.4,
 4.0,
 4.8,
 0.4,
 4.4,
 0.4,
 0.0,
 3.0,
 4.6,
 0.4,
 1.4,
 3.0,
 1.6,
 2.4,
 0.0,
 1.6,
 1.6,
 0.2,
 2.2,
 2.0,
 0.4,
 4.8,
 2.0,
 0.2,
 3.8,
 2.2,
 2.0,
 4.0,
 4.6,
 1.4,
 0.8,
 0.6,
 1.2,
 1.6,
 0.0,
 0.6,
 3.0,
 2.4,
 0.6,
 4.6,
 0.6,
 4.8,
 5.0,
 0.2,
 0.6,
 0.8,
 3.6,
 0.0,
 4.4,
 4.6,
 2.8,
 4.0,
 1.0,
 5.0,
 0.4,
 0.8,
 0.4,
 0.0,
 1.6,
 1.6,
 3.6,
 3.0,
 2.8,
 0.2,
 1.0,
 1.4,
 2.8,
 3.0,
 1.6,
 2.8,
 4.0,
 0.8,
 2.0,
 4.4,
 4.6,
 2.4,
 4.4,
 0.8,
 3.8,
 1.4,
 2.8,
 3.0,
 1.6,
 1.0,
 2.6,
 1.6,
 0.2,
 3.0,
 3.0,
 3.2,
 3.0,
 0.6,
 1.0,
 0.6,
 0.8,
 2.4,
 1.0,
 0.2,
 0.6,
 3.6,
 0.2,
 0.2,
 0.0,
 0.0,
 1.2,
 0.0,
 0.4,
 0.4,
 3.0,
 4.4,
 3.2,
 3.4,
 3.4,
 3.6,
 0.8,
 0.8,
 1.0,
 1.6,
 1.0,
 3.2,
 2.0,
 0.0,
 0.6,
 0.0,
 1.4,
 2.0,
 2.6,
 4.2,
 2.8,
 0.0,
 0.0,
 2.0,
 0.0,
 2.6,
 2.6,
 0.0,
 2.6,
 0.0,
 1.6,
 0.0,
 0.6,
 1.8,
 3.8,
 1.6,
 3.2,
 2.6,
 3.0,
 1.4,
 1.6,
 1.6,
 1.0,
 1.8,
 1.8,
 1.4,
 2.6,
 2.0,
 1.0,
 1.4,
 0.6,
 1.4,
 0.4,
 1.8,
 4.0,
 0.6,
 2.8,
 2.6,
 2.6,
 0.6,
 4.4,
 2.2,
 1.0,
 0.0,
 1.6,
 1.8,
 3.8,
 3.0,
 1.4,
 3.0,
 0.4,
 3.6,
 3.4,
 2.8,
 4.2,
 4.2,
 1.8,
 1.0,
 2.0,
 1.0,
 1.6,
 2.6,
 3.2,
 0.4,
 0.0,
 0.0,
 2.2,
 1.5,
 0.6,
 4.0,
 1.8,
 0.6,
 1.6,
 2.4,
 1.0,
 2.0,
 1.6,
 0.2,
 0.2,
 2.0,
 0.0,
 3.2,
 1.0,
 2.0,
 2.4,
 0.0,
 1.6,
 3.8,
 1.2,
 2.0,
 1.0,
 2.0,
 0.6,
 0.0,
 0.0,
 3.4,
 2.6,
 0.4,
 2.8,
 2.0,
 1.6,
 1.4,
 1.2,
 2.2,
 0.6,
 2.6,
 3.0,
 2.2,
 1.8,
 0.6,
 0.0,
 1.6,
 0.8,
 0.2,
 1.0,
 2.8,
 0.6,
 2.8,
 1.6,
 1.4,
 1.4,
 3.0,
 3.2,
 2.8,
 3.4,
 2.0,
 2.8,
 0.0,
 0.2,
 0.8,
 0.0,
 4.2,
 0.2,
 3.2,
 0.0,
 0.6,
 0.0,
 4.8,
 3.8,
 1.8,
 0.4,
 2.6,
 1.6,
 1.4,
 2.0,
 1.8,
 1.2,
 0.8,
 2.2,
 3.2,
 1.4,
 1.4,
 0.0,
 1.6,
 0.8,
 2.8,
 1.8,
 0.67,
 2.6,
 0.4,
 2.4,
 2.8,
 2.0,
 3.0,
 2.6,
 1.8,
 3.8,
 3.0,
 1.4,
 1.6,
 0.0,
 0.6,
 0.0,
 3.4,
 3.6,
 2.2,
 3.0,
 1.8,
 2.4,
 2.6,
 1.4,
 1.6,
 1.6,
 1.4,
 2.8,
 3.8,
 3.4,
 0.0,
 2.0,
 0.0,
 3.8,
 0.2,
 0.6,
 1.8,
 1.8,
 1.2,
 0.0,
 1.0,
 0.4,
 0.8,
 3.0,
 3.8,
 3.2,
 2.6,
 3.0,
 2.6,
 1.8,
 2.6,
 0.8,
 1.6,
 0.6,
 2.6,
 1.2,
 0.0,
 2.4,
 0.4,
 0.6,
 1.0,
 2.6,
 4.0,
 3.6,
 2.6,
 1.6,
 4.0,
 3.0,
 0.6,
 0.0,
 0.4,
 0.4,
 2.0,
 0.6,
 0.0,
 3.2,
 2.8,
 2.6,
 2.8,
 0.2,
 3.2,
 0.6,
 3.6,
 0.0,
 0.0,
 0.0,
 0.0,
 2.2,
 0.0,
 0.4,
 0.0,
 2.6,
 0.8,
 0.4,
 3.0,
 2.2,
 0.6,
 3.4,
 2.2,
 1.8,
 0.8,
 0.0,
 1.6,
 2.8,
 1.67,
 1.8,
 2.8,
 0.0,
 0.6,
 1.8,
 0.4,
 0.2,
 0.0,
 1.4,
 0.0,
 0.6,
 0.8,
 0.2,
 2.2,
 1.8,
 0.2,
 4.0,
 4.2,
 4.4,
 3.0,
 2.6,
 0.6,
 3.2,
 2.6,
 1.2,
 3.0,
 0.0,
 2.6,
 1.2,
 2.8,
 0.2,
 1.8,
 0.0,
 0.0,
 3.0,
 0.0,
 2.4,
 0.4,
 2.6,
 0.0,
 3.6,
 1.8,
 1.6,
 2.0,
 2.0,
 0.0,
 2.6,
 0.4,
 0.0,
 0.2,
 1.8,
 1.6,
 1.0,
 0.6,
 1.0,
 2.8,
 2.6,
 3.4,
 1.6,
 4.0,
 1.8,
 0.2,
 0.0,
 1.4,
 0.0,
 1.2,
 3.6,
 3.0,
 1.2,
 1.8,
 0.8,
 1.2,
 0.0,
 3.2,
 ...]

In [100]: sts_scores = [i/5.0 for i in sts_scores]

In [101]: sts_dict = {}
     ...: for ind, i in enumerate(sts_scores):
     ...:     k = get_key(i)
     ...:     if k == None:
     ...:         continue
     ...:     if k not in sts_dict:
     ...:         sts_dict[k] = [1, [i], [smatch_scores[ind]]]
     ...:     else:
     ...:         sts_dict[k][0] += 1
     ...:         sts_dict[k][1].append(i)
     ...:         sts_dict[k][2].append(smatch_scores[ind])
     ...: 

In [102]: sts_dict
Out[102]: 
{0.2: [1494,
  [0.0,
   0.16,
   0.1272,
   0.2,
   0.2,
   0.12,
   0.05,
   0.05,
   0.0,
   0.1,
   0.05,
   0.12,
   0.16,
   0.0,
   0.0,
   0.2,
   0.0,
   0.08,
   0.0,
   0.0,
   0.16,
   0.0,
   0.12,
   0.0,
   0.0,
   0.0,
   0.04,
   0.0,
   0.1,
   0.05,
   0.0,
   0.0,
   0.1,
   0.0,
   0.12,
   0.0,
   0.0,
   0.2,
   0.0,
   0.08,
   0.0166,
   0.0,
   0.2,
   0.0,
   0.08,
   0.04,
   0.08,
   0.15560000000000002,
   0.1666,
   0.0,
   0.16,
   0.2,
   0.04,
   0.15,
   0.08,
   0.16,
   0.0,
   0.0,
   0.0,
   0.0,
   0.1,
   0.1,
   0.08,
   0.15,
   0.1,
   0.08,
   0.08,
   0.12,
   0.16,
   0.08,
   0.04,
   0.0,
   0.0,
   0.0,
   0.02,
   0.0,
   0.0,
   0.16,
   0.0,
   0.12,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.08,
   0.0,
   0.08,
   0.16,
   0.0,
   0.16,
   0.0,
   0.08,
   0.0,
   0.0,
   0.12,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.04,
   0.0,
   0.0,
   0.0,
   0.16,
   0.0,
   0.0,
   0.12,
   0.04,
   0.16,
   0.08,
   0.08,
   0.0,
   0.08,
   0.08,
   0.0,
   0.0,
   0.04,
   0.12,
   0.0,
   0.04,
   0.08,
   0.2,
   0.0,
   0.12,
   0.0,
   0.16,
   0.16,
   0.2,
   0.0,
   0.0,
   0.0,
   0.12,
   0.16,
   0.0,
   0.0,
   0.16,
   0.0,
   0.16,
   0.04,
   0.2,
   0.08,
   0.08,
   0.08,
   0.04,
   0.04,
   0.08,
   0.2,
   0.2,
   0.08,
   0.08,
   0.0,
   0.08,
   0.0,
   0.04,
   0.08,
   0.04,
   0.16,
   0.12,
   0.0,
   0.12,
   0.12,
   0.12,
   0.04,
   0.12,
   0.16,
   0.0,
   0.2,
   0.08,
   0.16,
   0.08,
   0.0,
   0.04,
   0.2,
   0.16,
   0.16,
   0.2,
   0.04,
   0.12,
   0.2,
   0.12,
   0.16,
   0.2,
   0.04,
   0.12,
   0.04,
   0.04,
   0.0,
   0.0,
   0.0,
   0.08,
   0.08,
   0.16,
   0.16,
   0.2,
   0.2,
   0.0,
   0.12,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.12,
   0.2,
   0.2,
   0.12,
   0.08,
   0.12,
   0.12,
   0.2,
   0.0,
   0.08,
   0.2,
   0.2,
   0.08,
   0.0,
   0.0,
   0.12,
   0.12,
   0.2,
   0.04,
   0.04,
   0.0,
   0.2,
   0.0,
   0.2,
   0.12,
   0.0,
   0.0,
   0.08,
   0.12,
   0.12,
   0.0,
   0.16,
   0.04,
   0.2,
   0.12,
   0.0,
   0.04,
   0.16,
   0.0,
   0.04,
   0.0,
   0.12,
   0.0,
   0.08,
   0.16,
   0.0,
   0.16,
   0.134,
   0.08,
   0.0,
   0.12,
   0.0,
   0.0,
   0.0,
   0.04,
   0.12,
   0.0,
   0.2,
   0.08,
   0.16,
   0.16,
   0.12,
   0.0,
   0.08,
   0.12,
   0.2,
   0.12,
   0.0,
   0.08,
   0.08,
   0.12,
   0.0,
   0.04,
   0.12,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.08,
   0.0,
   0.16,
   0.08,
   0.12,
   0.16,
   0.0,
   0.0,
   0.12,
   0.08,
   0.04,
   0.0,
   0.0,
   0.12,
   0.16,
   0.04,
   0.04,
   0.12,
   0.0,
   0.04,
   0.0,
   0.0,
   0.0,
   0.08,
   0.0,
   0.0,
   0.08,
   0.0,
   0.04,
   0.2,
   0.12,
   0.2,
   0.04,
   0.0,
   0.0,
   0.16,
   0.0,
   0.04,
   0.16,
   0.16,
   0.16,
   0.2,
   0.2,
   0.16,
   0.2,
   0.2,
   0.12,
   0.16,
   0.04,
   0.08,
   0.08,
   0.2,
   0.12,
   0.16,
   0.2,
   0.0,
   0.0,
   0.16,
   0.12,
   0.2,
   0.0,
   0.08,
   0.12,
   0.0,
   0.2,
   0.16,
   0.08,
   0.0,
   0.16,
   0.16,
   0.0,
   0.04,
   0.0,
   0.08,
   0.2,
   0.0,
   0.0,
   0.04,
   0.0,
   0.08,
   0.16,
   0.08,
   0.2,
   0.2,
   0.08,
   0.04,
   0.0,
   0.0,
   0.0,
   0.12,
   0.12,
   0.0,
   0.16,
   0.2,
   0.08,
   0.0,
   0.08,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.1,
   0.1,
   0.2,
   0.2,
   0.12,
   0.1,
   0.16,
   0.12,
   0.2,
   0.2,
   0.028599999999999997,
   0.2,
   0.12,
   0.0,
   0.08,
   0.13340000000000002,
   0.2,
   0.2,
   0.12,
   0.08,
   0.12,
   0.08,
   0.1,
   0.0,
   0.0,
   0.05,
   0.15,
   0.04,
   0.16,
   0.08,
   0.16,
   0.0,
   0.2,
   0.0,
   0.08,
   0.08,
   0.12,
   0.08,
   0.08,
   0.08,
   0.12,
   0.16,
   0.12,
   0.12,
   0.0,
   0.12,
   0.08,
   0.04,
   0.08,
   0.12,
   0.08,
   0.0,
   0.0,
   0.16,
   0.1,
   0.0,
   0.0,
   0.16,
   0.16999999999999998,
   0.08,
   0.15,
   0.0,
   0.0,
   0.0,
   0.05,
   0.0,
   0.2,
   0.0,
   0.0,
   0.04,
   0.0,
   0.0,
   0.1666,
   0.0,
   0.04,
   0.08,
   0.0,
   0.0,
   0.0,
   0.04,
   0.0,
   0.0,
   0.08,
   0.0,
   0.08,
   0.12,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0666,
   0.0666,
   0.16,
   0.04,
   0.0,
   0.0,
   0.16,
   0.0,
   0.05,
   0.1,
   0.08,
   0.0,
   0.2,
   0.16,
   0.0,
   0.04,
   0.2,
   0.08,
   0.0,
   0.0,
   0.0,
   0.16,
   0.16,
   0.0,
   0.0,
   0.0,
   0.16,
   0.16,
   0.0,
   0.0,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.0834,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.1286,
   0.0,
   0.0,
   0.04,
   0.1,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.12,
   0.05,
   0.15,
   0.0,
   0.04,
   0.0,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.12,
   0.04,
   0.1,
   0.1454,
   0.0,
   0.1,
   0.2,
   0.1,
   0.0134,
   0.16,
   0.04,
   0.04,
   0.0,
   0.0,
   0.2,
   0.2,
   0.2,
   0.16,
   0.04,
   0.05,
   0.2,
   0.08,
   0.2,
   0.1,
   0.2,
   0.08,
   0.08,
   0.05,
   0.05,
   0.05,
   0.0,
   0.16,
   0.16,
   0.0,
   0.13340000000000002,
   0.08,
   0.16,
   0.16,
   0.15,
   0.15,
   0.2,
   0.16,
   0.05,
   0.16,
   0.16,
   0.16,
   0.05,
   0.1,
   0.0,
   0.1,
   0.12,
   0.0,
   0.0,
   0.0,
   0.08,
   0.0,
   0.0,
   0.2,
   0.0,
   0.05,
   0.08,
   0.2,
   0.04,
   0.16,
   0.16,
   0.15,
   0.05,
   0.08,
   0.08,
   0.1,
   0.1,
   0.16,
   0.05,
   0.15,
   0.16,
   0.0,
   0.0,
   0.05,
   0.0,
   0.08,
   0.16,
   0.04,
   0.04,
   0.1,
   0.0,
   0.0,
   0.15,
   0.08,
   0.1,
   0.0,
   0.0,
   0.0,
   0.2,
   0.12,
   0.1,
   0.0,
   0.16,
   0.16,
   0.08,
   0.0,
   0.0,
   0.0,
   0.08,
   0.0,
   0.046200000000000005,
   0.0,
   0.1,
   0.0,
   0.15,
   0.0,
   0.0,
   0.15,
   0.1,
   0.0,
   0.0,
   0.0,
   0.2,
   0.2,
   0.0,
   0.0,
   0.08,
   0.08,
   0.0,
   0.0,
   0.0,
   0.0,
   0.08,
   0.2,
   0.05,
   0.0236,
   0.2,
   0.08,
   0.0,
   0.0,
   0.15,
   0.0,
   0.0,
   0.0,
   0.0,
   0.12,
   0.0,
   0.08,
   0.08,
   0.0,
   0.15,
   0.0,
   0.0,
   0.16,
   0.0,
   0.05,
   0.13340000000000002,
   0.0666,
   0.2,
   0.08,
   0.0,
   0.05,
   0.04,
   0.12,
   0.0,
   0.0666,
   0.16,
   0.2,
   0.0,
   0.12,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.15,
   0.0,
   0.0,
   0.0,
   0.16,
   0.0,
   0.12,
   0.12,
   0.0,
   0.0,
   0.2,
   0.08,
   0.0,
   0.12,
   0.16,
   0.12,
   0.0,
   0.04,
   0.08,
   0.12,
   0.16,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.16,
   0.08,
   0.0,
   0.2,
   0.04,
   0.12,
   0.0,
   0.16,
   0.04,
   0.0,
   0.04,
   0.0,
   0.08,
   0.0,
   0.16,
   0.08,
   0.08,
   0.08,
   0.0,
   0.2,
   0.0,
   0.08,
   0.0,
   0.08,
   0.08,
   0.0,
   0.04,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.0,
   0.16,
   0.0,
   0.0,
   0.08,
   0.2,
   0.0,
   0.0,
   0.2,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.2,
   0.16,
   0.16,
   0.0,
   0.0,
   0.0,
   0.0,
   0.08,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.08,
   0.08,
   0.04,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.12,
   0.04,
   0.16,
   0.0,
   0.04,
   0.0,
   0.0,
   0.16,
   0.08,
   0.2,
   0.12,
   0.12,
   0.08,
   0.0,
   0.12,
   0.16,
   0.12,
   0.08,
   0.0,
   0.0,
   0.12,
   0.12,
   0.12,
   0.0,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.12,
   0.0,
   0.0,
   0.0,
   0.2,
   0.0,
   0.04,
   0.16,
   0.16,
   0.2,
   0.08,
   0.034,
   0.0,
   0.04,
   0.1,
   0.16,
   0.0,
   0.0,
   0.08,
   0.0,
   0.08,
   0.12,
   0.16,
   0.0,
   0.08,
   0.0,
   0.0,
   0.08,
   0.08,
   0.0,
   0.08,
   0.0,
   0.2,
   0.0,
   0.0,
   0.0,
   0.0,
   0.0,
   0.16,
   0.0,
   0.0,
   0.0,
   0.0,
   0.16,
   0.08,
   0.2,
   0.2,
   0.0,
   0.12,
   0.2,
   0.08,
   0.12,
   0.0,
   0.0,
   0.16,
   0.08,
   0.2,
   0.04,
   0.0,
   0.04,
   0.2,
   0.0,
   0.0,
   0.0,
   0.04,
   0.12,
   0.16,
   0.12,
   0.08,
   0.0,
   0.12,
   0.08,
   0.12,
   0.08,
   0.12,
   0.04,
   0.12,
   0.0,
   0.0,
   0.0,
   0.2,
   0.12,
   0.16,
   0.08,
   0.16,
   0.12,
   0.0,
   0.0,
   0.0,
   0.16,
   0.08,
   0.0,
   0.2,
   0.08,
   0.0,
   0.0,
   0.12,
   0.08,
   0.0,
   0.2,
   0.16,
   0.04,
   0.2,
   0.0,
   0.0,
   0.2,
   0.2,
   0.16,
   0.16,
   0.2,
   0.04,
   0.0,
   0.0,
   0.0,
   0.1,
   0.2,
   0.08,
   0.2,
   0.2,
   0.0,
   0.12,
   0.0,
   0.12,
   0.0,
   0.0,
   0.2,
   0.16,
   0.2,
   0.08,
   0.12,
   0.2,
   0.2,
   0.16,
   0.16,
   0.2,
   0.16,
   0.16,
   0.2,
   0.0,
   0.2,
   0.2,
   0.08,
   0.2,
   0.16,
   0.04,
   0.2,
   0.0,
   0.12,
   0.2,
   0.16,
   ...],
  [0.8,
   0.6666666666666666,
   0.75,
   0.8333333333333334,
   0.6,
   0.5,
   0.5,
   0.4,
   0.5,
   0.5263157894736842,
   0.5,
   0.6666666666666666,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.6666666666666666,
   0.33333333333333326,
   0.42857142857142855,
   0.4615384615384615,
   0.3333333333333333,
   0.5,
   0.3333333333333333,
   0.5,
   0.43478260869565216,
   0.5,
   0.4,
   0.5714285714285715,
   0.3333333333333333,
   0.5,
   0.42857142857142855,
   0.4,
   0.14285714285714288,
   0.6666666666666666,
   0.4444444444444445,
   0.6,
   0.2,
   0.3333333333333333,
   0.4210526315789474,
   0.37499999999999994,
   0.4,
   0.42857142857142855,
   0.125,
   0.4444444444444445,
   0.22222222222222224,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.5714285714285715,
   0.5714285714285715,
   0.5,
   0.6666666666666666,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.5,
   0.375,
   0.4,
   0.42857142857142855,
   0.42857142857142855,
   0.42857142857142855,
   0.5,
   0.6,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.6153846153846153,
   0.375,
   0.5714285714285715,
   0.5714285714285715,
   0.28571428571428575,
   0.5714285714285715,
   0.28571428571428575,
   0.5,
   0.42857142857142855,
   0.28571428571428575,
   0.375,
   0.25,
   0.4444444444444444,
   0.375,
   0.380952380952381,
   0.5,
   0.2727272727272727,
   0.3333333333333333,
   0.28571428571428575,
   0.2222222222222222,
   0.2,
   0.380952380952381,
   0.4444444444444445,
   0.6666666666666666,
   0.2,
   0.20000000000000004,
   0.28571428571428575,
   0.5555555555555556,
   0.21428571428571427,
   0.17391304347826086,
   0.5714285714285715,
   0.1,
   0.5333333333333333,
   0.25,
   0.38461538461538464,
   0.16,
   0.36363636363636365,
   0.4666666666666667,
   0.25,
   0.4,
   0.2727272727272727,
   0.16,
   0.3636363636363636,
   0.4444444444444445,
   0.20689655172413793,
   0.47058823529411764,
   0.3636363636363636,
   0.3225806451612903,
   0.3448275862068965,
   0.36363636363636365,
   0.3,
   0.3243243243243243,
   0.34782608695652173,
   0.25,
   0.20000000000000004,
   0.25,
   0.5,
   0.14285714285714288,
   0.22222222222222224,
   0.24242424242424246,
   0.3,
   0.3529411764705882,
   0.34782608695652173,
   0.10526315789473685,
   0.29629629629629634,
   0.21621621621621623,
   0.36363636363636365,
   0.3870967741935484,
   0.25,
   0.3333333333333333,
   0.28571428571428575,
   0.6,
   0.2631578947368421,
   0.28571428571428575,
   0.20689655172413793,
   0.3157894736842105,
   0.6666666666666665,
   0.15384615384615383,
   0.2,
   0.20512820512820512,
   0.1379310344827586,
   0.3636363636363637,
   0.23529411764705885,
   0.18749999999999997,
   0.25,
   0.3157894736842105,
   0.6,
   0.34285714285714286,
   0.33333333333333337,
   0.2105263157894737,
   0.10526315789473685,
   0.18181818181818182,
   0.3,
   0.29629629629629634,
   0.13793103448275862,
   0.3684210526315789,
   0.5263157894736842,
   0.2105263157894737,
   0.1,
   0.25,
   0.5,
   0.28571428571428575,
   0.5555555555555556,
   0.3703703703703704,
   0.07142857142857142,
   0.35714285714285715,
   0.3,
   0.36363636363636365,
   0.3,
   0.31250000000000006,
   0.16666666666666666,
   0.2962962962962963,
   0.3333333333333333,
   0.16666666666666666,
   0.3846153846153846,
   0.1818181818181818,
   0.28571428571428575,
   0.15384615384615383,
   0.2758620689655172,
   0.3050847457627119,
   0.35294117647058826,
   0.3846153846153846,
   0.22222222222222224,
   0.17543859649122806,
   0.18867924528301885,
   0.20408163265306123,
   0.22857142857142854,
   0.163265306122449,
   0.11320754716981132,
   0.22727272727272724,
   0.25,
   0.17142857142857143,
   0.20689655172413793,
   0.14285714285714285,
   0.17777777777777778,
   0.23529411764705882,
   0.11764705882352941,
   0.25,
   0.12903225806451615,
   0.17142857142857143,
   0.1886792452830189,
   0.22857142857142854,
   0.2711864406779661,
   0.25,
   0.21739130434782608,
   0.10526315789473684,
   0.13793103448275862,
   0.509090909090909,
   0.26666666666666666,
   0.2,
   0.2790697674418605,
   0.22727272727272727,
   0.1904761904761905,
   0.2745098039215686,
   0.2127659574468085,
   0.22222222222222224,
   0.24999999999999994,
   0.1923076923076923,
   0.28571428571428575,
   0.17391304347826086,
   0.25,
   0.35000000000000003,
   0.13333333333333333,
   0.3018867924528302,
   0.23076923076923078,
   0.23529411764705882,
   0.2790697674418605,
   0.13953488372093023,
   0.22950819672131148,
   0.2909090909090909,
   0.25,
   0.3714285714285714,
   0.1081081081081081,
   0.22857142857142856,
   0.2153846153846154,
   0.13043478260869565,
   0.1951219512195122,
   0.21052631578947367,
   0.13793103448275862,
   0.2,
   0.32727272727272727,
   0.13333333333333333,
   0.3225806451612903,
   0.25,
   0.21818181818181817,
   0.1694915254237288,
   0.23809523809523808,
   0.2545454545454545,
   0.23076923076923078,
   0.339622641509434,
   0.14634146341463417,
   0.22580645161290322,
   0.09523809523809522,
   0.21538461538461542,
   0.23529411764705882,
   0.2105263157894737,
   0.3333333333333333,
   0.27027027027027023,
   0.13043478260869565,
   0.21739130434782608,
   0.27777777777777773,
   0.2,
   0.1904761904761905,
   0.4,
   0.10714285714285714,
   0.2222222222222222,
   0.16,
   0.1702127659574468,
   0.2926829268292683,
   0.0930232558139535,
   0.15384615384615383,
   0.27906976744186046,
   0.19512195121951217,
   0.2647058823529412,
   0.2,
   0.24000000000000002,
   0.42553191489361697,
   0.3225806451612903,
   0.27027027027027023,
   0.11320754716981131,
   0.24242424242424243,
   0.3255813953488372,
   0.27027027027027023,
   0.24242424242424243,
   0.2,
   0.1923076923076923,
   0.1818181818181818,
   0.2222222222222222,
   0.12244897959183673,
   0.16666666666666663,
   0.21052631578947367,
   0.3673469387755102,
   0.13636363636363638,
   0.2222222222222222,
   0.1754385964912281,
   0.24137931034482757,
   0.3125,
   0.16666666666666666,
   0.23529411764705882,
   0.2608695652173913,
   0.45454545454545453,
   0.27027027027027023,
   0.16666666666666663,
   0.14285714285714288,
   0.2711864406779661,
   0.04761904761904762,
   0.25925925925925924,
   0.23809523809523808,
   0.2285714285714286,
   0.25,
   0.2191780821917808,
   0.2857142857142857,
   0.18518518518518517,
   0.09302325581395349,
   0.20408163265306123,
   0.2631578947368421,
   0.20512820512820512,
   0.13333333333333333,
   0.23529411764705882,
   0.41025641025641024,
   0.5,
   0.3829787234042554,
   0.3255813953488372,
   0.3829787234042554,
   0.3636363636363636,
   0.29166666666666663,
   0.39024390243902435,
   0.5405405405405405,
   0.5714285714285714,
   0.3684210526315789,
   0.3571428571428571,
   0.3333333333333333,
   0.43749999999999994,
   0.5128205128205129,
   0.5625000000000001,
   0.375,
   0.2222222222222222,
   0.2,
   0.33333333333333337,
   0.5882352941176471,
   0.39999999999999997,
   0.42424242424242425,
   0.38888888888888884,
   0.5,
   0.43902439024390244,
   0.2857142857142857,
   0.25,
   0.358974358974359,
   0.3636363636363636,
   0.4186046511627907,
   0.48648648648648646,
   0.6521739130434783,
   0.4285714285714286,
   0.37209302325581395,
   0.3448275862068966,
   0.1764705882352941,
   0.6470588235294117,
   0.30303030303030304,
   0.42105263157894735,
   0.39999999999999997,
   0.5625,
   0.4864864864864865,
   0.6111111111111112,
   0.5,
   0.4,
   0.5217391304347826,
   0.4680851063829788,
   0.4666666666666667,
   0.25641025641025644,
   0.16,
   0.4375,
   0.38888888888888884,
   0.1904761904761905,
   0.26315789473684204,
   0.5909090909090909,
   0.358974358974359,
   0.6470588235294118,
   0.5365853658536585,
   0.5652173913043479,
   0.23529411764705882,
   0.372093023255814,
   0.3428571428571428,
   0.4571428571428572,
   0.4090909090909091,
   0.4313725490196078,
   0.8,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.75,
   0.75,
   0.75,
   0.6,
   0.42857142857142855,
   0.5,
   0.5,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.5,
   0.42857142857142855,
   0.3333333333333333,
   0.5,
   0.5714285714285715,
   0.6153846153846153,
   0.5,
   0.6666666666666666,
   0.6666666666666666,
   0.5,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.6,
   0.6,
   0.4,
   0.4,
   0.6666666666666666,
   0.6,
   0.625,
   0.26666666666666666,
   0.6666666666666666,
   0.6,
   0.6666666666666666,
   0.6666666666666666,
   0.5714285714285715,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.5,
   0.6666666666666666,
   0.5333333333333333,
   0.42857142857142855,
   0.6666666666666666,
   0.3333333333333333,
   0.5,
   0.4444444444444445,
   0.39999999999999997,
   0.5,
   0.3333333333333333,
   0.6,
   0.5,
   0.4210526315789474,
   0.5714285714285715,
   0.5,
   0.5,
   0.42857142857142855,
   0.13333333333333333,
   0.5,
   0.5714285714285715,
   0.42857142857142855,
   0.42857142857142855,
   0.30769230769230765,
   0.39999999999999997,
   0.28571428571428575,
   0.6666666666666666,
   0.5,
   0.4,
   0.375,
   0.5,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.5,
   0.42857142857142855,
   0.5,
   0.5,
   0.3333333333333333,
   0.5,
   0.42857142857142855,
   0.5,
   0.4615384615384615,
   0.2857142857142857,
   0.5882352941176471,
   0.3529411764705882,
   0.3333333333333333,
   0.3333333333333333,
   0.42857142857142855,
   0.6250000000000001,
   0.5,
   0.5,
   0.5384615384615384,
   0.37499999999999994,
   0.42857142857142855,
   0.6666666666666666,
   0.5714285714285715,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.6,
   0.4,
   0.5,
   0.5,
   0.5333333333333333,
   0.5714285714285715,
   0.42857142857142855,
   0.3333333333333333,
   0.37499999999999994,
   0.4210526315789474,
   0.36363636363636365,
   0.42857142857142855,
   0.28571428571428575,
   0.3333333333333333,
   0.5714285714285715,
   0.28571428571428575,
   0.26666666666666666,
   0.39999999999999997,
   0.42857142857142855,
   0.26666666666666666,
   0.5882352941176471,
   0.42857142857142855,
   0.380952380952381,
   0.2857142857142857,
   0.1739130434782609,
   0.4705882352941177,
   0.4,
   0.28571428571428575,
   0.3157894736842105,
   0.5333333333333333,
   0.375,
   0.28571428571428575,
   0.3333333333333333,
   0.3157894736842105,
   0.5454545454545454,
   0.3333333333333333,
   0.4,
   0.6666666666666666,
   0.25,
   0.3,
   0.16,
   0.42857142857142855,
   0.28571428571428575,
   0.6666666666666665,
   0.21052631578947364,
   0.37499999999999994,
   0.25,
   0.30769230769230765,
   0.5,
   0.3333333333333333,
   0.42857142857142855,
   0.39999999999999997,
   0.6666666666666666,
   0.75,
   0.3333333333333333,
   0.75,
   0.5,
   0.75,
   0.6666666666666666,
   0.75,
   0.5,
   0.6666666666666666,
   0.5,
   0.5,
   0.5,
   0.5,
   0.75,
   0.75,
   0.6666666666666666,
   0.7142857142857143,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.6,
   0.6153846153846153,
   0.6666666666666666,
   0.5714285714285715,
   0.6,
   0.5,
   0.3333333333333333,
   0.6153846153846153,
   0.42857142857142855,
   0.42857142857142855,
   0.5714285714285715,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.6666666666666666,
   0.5714285714285715,
   0.6,
   0.6666666666666666,
   0.3333333333333333,
   0.4,
   0.6666666666666666,
   0.6,
   0.5714285714285715,
   0.6666666666666666,
   0.6,
   0.6,
   0.6666666666666666,
   0.4,
   0.5714285714285715,
   0.37499999999999994,
   0.5,
   0.5,
   0.3333333333333333,
   0.5714285714285715,
   0.5,
   0.42857142857142855,
   0.42857142857142855,
   0.3333333333333333,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.5714285714285715,
   0.5,
   0.6153846153846153,
   0.6,
   0.5714285714285714,
   0.5714285714285715,
   0.5,
   0.5,
   0.5,
   0.5714285714285715,
   0.5,
   0.6666666666666666,
   0.42857142857142855,
   0.2857142857142857,
   0.4705882352941177,
   0.375,
   0.4,
   0.3333333333333333,
   0.5,
   0.5,
   0.5714285714285715,
   0.5714285714285715,
   0.5,
   0.5,
   0.33333333333333326,
   0.5,
   0.6,
   0.16666666666666666,
   0.42857142857142855,
   0.3636363636363636,
   0.4615384615384615,
   0.5,
   0.5,
   0.375,
   0.5714285714285715,
   0.35294117647058826,
   0.4,
   0.4,
   0.42857142857142855,
   0.26666666666666666,
   0.6666666666666666,
   0.42857142857142855,
   0.25,
   0.3333333333333333,
   0.4615384615384615,
   0.42857142857142855,
   0.5,
   0.13333333333333333,
   0.26666666666666666,
   0.4444444444444445,
   0.5555555555555556,
   0.28571428571428575,
   0.4444444444444445,
   0.42857142857142855,
   0.47619047619047616,
   0.6666666666666666,
   0.5,
   0.4,
   0.4444444444444444,
   0.4705882352941177,
   0.28571428571428575,
   0.35294117647058826,
   0.5,
   0.26666666666666666,
   0.6666666666666666,
   0.5,
   0.5,
   0.37499999999999994,
   0.37499999999999994,
   0.375,
   0.5,
   0.37499999999999994,
   0.37499999999999994,
   0.23529411764705885,
   0.3333333333333333,
   0.4,
   0.3333333333333333,
   0.5714285714285715,
   0.42857142857142855,
   0.6666666666666666,
   0.5,
   0.3333333333333333,
   0.6,
   0.5,
   0.3333333333333333,
   0.28571428571428564,
   0.3333333333333333,
   0.375,
   0.42857142857142855,
   0.28571428571428575,
   0.4444444444444444,
   0.2857142857142857,
   0.37499999999999994,
   0.5,
   0.375,
   0.42857142857142855,
   0.4,
   0.5,
   0.4,
   0.42857142857142855,
   0.37499999999999994,
   0.42857142857142855,
   0.5333333333333333,
   0.42857142857142855,
   0.37499999999999994,
   0.4444444444444444,
   0.2105263157894737,
   0.3157894736842105,
   0.375,
   0.5,
   0.6666666666666666,
   0.3333333333333333,
   0.5714285714285715,
   0.4,
   0.375,
   0.42857142857142855,
   0.2857142857142857,
   0.28571428571428575,
   0.5555555555555556,
   0.4166666666666667,
   0.3703703703703703,
   0.2758620689655172,
   0.5,
   0.4000000000000001,
   0.17647058823529413,
   0.25,
   0.20000000000000004,
   0.48000000000000004,
   0.1904761904761905,
   0.23076923076923078,
   0.25,
   0.34285714285714286,
   0.47058823529411764,
   0.11111111111111112,
   0.1818181818181818,
   0.19354838709677416,
   0.47058823529411764,
   0.3636363636363636,
   0.42857142857142855,
   0.21428571428571427,
   0.4761904761904762,
   0.16666666666666666,
   0.6,
   0.32,
   0.14285714285714288,
   0.4210526315789474,
   0.3333333333333333,
   0.22222222222222224,
   0.25,
   0.39999999999999997,
   0.3636363636363636,
   0.625,
   0.30303030303030304,
   0.29411764705882354,
   0.3076923076923077,
   0.11764705882352942,
   0.35714285714285715,
   0.3,
   0.28571428571428575,
   0.3,
   0.25,
   0.47619047619047616,
   0.4,
   0.2758620689655172,
   0.4166666666666667,
   0.3181818181818182,
   0.25,
   0.28571428571428575,
   0.2727272727272727,
   0.2758620689655172,
   0.37499999999999994,
   0.3157894736842105,
   0.30769230769230765,
   0.18749999999999997,
   0.27586206896551724,
   0.33333333333333326,
   0.5555555555555556,
   0.42857142857142855,
   0.3157894736842105,
   0.33333333333333326,
   0.29411764705882354,
   0.2857142857142857,
   0.31250000000000006,
   0.5217391304347826,
   0.3,
   0.36363636363636365,
   0.625,
   0.6666666666666666,
   0.24000000000000002,
   0.17391304347826086,
   0.4444444444444445,
   0.4,
   0.26666666666666666,
   0.16,
   0.19999999999999998,
   0.375,
   0.33333333333333337,
   0.43478260869565216,
   0.3,
   0.25,
   0.33333333333333337,
   0.380952380952381,
   0.33333333333333326,
   0.42857142857142855,
   0.09090909090909091,
   0.5,
   0.22727272727272727,
   0.20689655172413793,
   0.5,
   0.5555555555555556,
   0.07142857142857144,
   0.25,
   0.3478260869565218,
   0.2727272727272727,
   0.47058823529411764,
   0.5,
   0.21428571428571427,
   0.22222222222222224,
   0.4444444444444445,
   0.18181818181818182,
   0.20000000000000004,
   0.48484848484848486,
   0.6666666666666666,
   0.625,
   0.16666666666666666,
   0.29629629629629634,
   0.45454545454545453,
   0.3703703703703704,
   0.27027027027027023,
   0.4000000000000001,
   0.25,
   0.6666666666666665,
   0.26666666666666666,
   0.2727272727272727,
   0.16,
   0.1904761904761905,
   0.19354838709677422,
   0.3870967741935483,
   0.5,
   0.3333333333333333,
   0.24000000000000002,
   0.28571428571428564,
   0.47058823529411764,
   0.14285714285714288,
   0.5,
   0.4444444444444445,
   0.3703703703703704,
   0.375,
   0.3,
   0.24999999999999994,
   0.32,
   0.37499999999999994,
   0.3636363636363636,
   0.37499999999999994,
   0.3225806451612903,
   0.31250000000000006,
   0.3636363636363637,
   0.08695652173913043,
   0.18749999999999997,
   0.08695652173913043,
   0.6153846153846153,
   0.17391304347826086,
   0.3333333333333333,
   0.3,
   0.3076923076923077,
   0.26666666666666666,
   0.45454545454545453,
   0.27586206896551724,
   0.22222222222222224,
   0.2777777777777778,
   0.0909090909090909,
   0.2857142857142857,
   0.33333333333333326,
   0.36363636363636365,
   0.4000000000000001,
   0.33333333333333326,
   0.25,
   0.4666666666666667,
   0.21428571428571427,
   0.19047619047619047,
   0.5,
   0.1875,
   0.2727272727272727,
   0.33333333333333326,
   0.375,
   0.23999999999999996,
   0.2105263157894737,
   0.34782608695652173,
   0.30769230769230765,
   0.38709677419354843,
   0.2,
   0.375,
   0.41379310344827586,
   0.3,
   0.2222222222222222,
   0.22222222222222224,
   0.21428571428571427,
   0.3636363636363636,
   0.23076923076923075,
   0.3333333333333333,
   0.2631578947368421,
   0.3333333333333333,
   0.22857142857142854,
   0.14634146341463414,
   0.3333333333333333,
   0.29629629629629634,
   0.5714285714285714,
   0.26086956521739135,
   0.37499999999999994,
   0.24390243902439024,
   0.24242424242424243,
   0.2,
   0.23076923076923075,
   0.48,
   0.6666666666666666,
   0.30769230769230765,
   0.23076923076923075,
   0.375,
   0.25,
   0.3333333333333333,
   0.3636363636363637,
   0.5806451612903225,
   0.3,
   0.2,
   0.3,
   0.25,
   0.16666666666666663,
   0.41379310344827586,
   0.14814814814814817,
   0.16,
   0.3076923076923077,
   0.2857142857142857,
   0.28571428571428575,
   0.24242424242424246,
   0.35714285714285715,
   0.3333333333333333,
   0.15384615384615385,
   0.22857142857142854,
   0.2,
   0.5333333333333333,
   0.35714285714285715,
   0.33333333333333337,
   0.3157894736842105,
   0.5517241379310345,
   0.6666666666666666,
   0.3571428571428571,
   0.46153846153846156,
   0.2,
   0.2608695652173913,
   0.6666666666666665,
   0.3225806451612903,
   0.23076923076923075,
   0.2,
   0.18181818181818182,
   0.2380952380952381,
   0.5,
   0.4000000000000001,
   0.25,
   0.5,
   0.4000000000000001,
   0.33333333333333337,
   0.23076923076923075,
   0.2,
   0.1702127659574468,
   0.5714285714285715,
   0.35294117647058826,
   0.5714285714285715,
   0.5714285714285715,
   0.6875,
   0.6,
   0.4666666666666667,
   0.35714285714285715,
   0.4210526315789474,
   0.36363636363636365,
   0.47058823529411764,
   0.47058823529411764,
   0.6206896551724138,
   0.7142857142857143,
   0.6363636363636365,
   0.7407407407407408,
   0.3157894736842105,
   0.47058823529411764,
   0.41025641025641024,
   0.8461538461538461,
   0.25,
   0.3157894736842105,
   0.7142857142857143,
   0.5454545454545454,
   ...]],
 1.0: [1260,
  [1.0,
   0.95,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.9818,
   1.0,
   0.85,
   1.0,
   0.9199999999999999,
   1.0,
   0.96,
   1.0,
   1.0,
   0.8400000000000001,
   0.9,
   0.96,
   1.0,
   0.9,
   0.85,
   0.85,
   1.0,
   0.9,
   0.9,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.9714,
   0.8800000000000001,
   0.8800000000000001,
   0.8666,
   0.8428000000000001,
   0.8400000000000001,
   0.8400000000000001,
   1.0,
   0.8858,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   0.9199999999999999,
   0.96,
   0.96,
   0.9199999999999999,
   0.96,
   1.0,
   0.96,
   0.8400000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   0.96,
   0.9199999999999999,
   1.0,
   1.0,
   0.9199999999999999,
   0.8400000000000001,
   0.9,
   0.8400000000000001,
   0.8400000000000001,
   1.0,
   0.96,
   0.8400000000000001,
   0.8800000000000001,
   1.0,
   1.0,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   0.9199999999999999,
   0.9199999999999999,
   0.96,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.8800000000000001,
   1.0,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   0.9,
   0.9199999999999999,
   0.8666,
   0.8800000000000001,
   0.8800000000000001,
   1.0,
   1.0,
   0.8800000000000001,
   0.85,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   1.0,
   0.9,
   0.96,
   0.95,
   0.95,
   1.0,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.9,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   1.0,
   0.85,
   0.9334,
   0.96,
   0.95,
   0.8400000000000001,
   1.0,
   0.8221999999999999,
   0.8666,
   0.9,
   0.95,
   0.85,
   0.8800000000000001,
   0.96,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   0.96,
   0.96,
   0.96,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   1.0,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.96,
   0.9199999999999999,
   0.9199999999999999,
   1.0,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.96,
   1.0,
   1.0,
   1.0,
   1.0,
   1.0,
   0.85,
   0.85,
   1.0,
   0.8400000000000001,
   0.9199999999999999,
   0.9334,
   1.0,
   1.0,
   0.9199999999999999,
   1.0,
   0.96,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.9818,
   0.8400000000000001,
   1.0,
   1.0,
   1.0,
   0.8800000000000001,
   0.95,
   1.0,
   1.0,
   0.95,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   1.0,
   0.85,
   0.85,
   0.8800000000000001,
   0.96,
   0.96,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   0.9714,
   1.0,
   0.96,
   1.0,
   0.96,
   0.95,
   0.96,
   0.96,
   1.0,
   0.8800000000000001,
   0.8266,
   0.96,
   0.8400000000000001,
   1.0,
   0.8400000000000001,
   1.0,
   0.96,
   0.85,
   1.0,
   1.0,
   0.9199999999999999,
   1.0,
   0.8400000000000001,
   0.85,
   0.9199999999999999,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   0.85,
   0.8666,
   1.0,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   1.0,
   1.0,
   1.0,
   1.0,
   0.85,
   1.0,
   0.96,
   0.8400000000000001,
   1.0,
   1.0,
   1.0,
   0.8800000000000001,
   1.0,
   0.8800000000000001,
   1.0,
   0.8800000000000001,
   1.0,
   1.0,
   0.9199999999999999,
   0.9,
   0.9,
   0.8800000000000001,
   0.8800000000000001,
   0.96,
   0.96,
   1.0,
   0.8800000000000001,
   1.0,
   0.95,
   0.975,
   1.0,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.8182,
   1.0,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.96,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   0.9,
   0.85,
   0.8800000000000001,
   0.8400000000000001,
   0.9334,
   0.9,
   0.85,
   0.96,
   0.8400000000000001,
   0.9,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   0.85,
   0.85,
   1.0,
   0.8666,
   0.8400000000000001,
   0.8800000000000001,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   0.82,
   0.82,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.96,
   0.9199999999999999,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.96,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.9,
   1.0,
   0.8800000000000001,
   0.8400000000000001,
   0.85,
   0.8400000000000001,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8400000000000001,
   0.85,
   1.0,
   0.96,
   0.8400000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   0.96,
   0.96,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   0.96,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   1.0,
   1.0,
   1.0,
   1.0,
   0.8400000000000001,
   0.96,
   1.0,
   1.0,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   0.8800000000000001,
   0.96,
   0.96,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.9199999999999999,
   0.96,
   0.96,
   0.9199999999999999,
   1.0,
   0.96,
   1.0,
   0.96,
   0.96,
   1.0,
   0.96,
   1.0,
   0.96,
   0.96,
   0.96,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   1.0,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.96,
   0.8400000000000001,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.96,
   0.8400000000000001,
   0.96,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   0.9199999999999999,
   0.96,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.96,
   0.8800000000000001,
   1.0,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.96,
   1.0,
   1.0,
   1.0,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   0.8800000000000001,
   1.0,
   0.8800000000000001,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   1.0,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   0.9199999999999999,
   1.0,
   1.0,
   0.9,
   0.9199999999999999,
   0.8800000000000001,
   0.96,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.914285714285714,
   0.8800000000000001,
   0.96,
   0.96,
   0.8400000000000001,
   0.8400000000000001,
   0.9199999999999999,
   0.9,
   0.85,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   0.96,
   0.96,
   0.8800000000000001,
   0.96,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.9,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   0.914285714285714,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.9,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   0.9199999999999999,
   0.96,
   0.96,
   1.0,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.914285714285714,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.96,
   0.9199999999999999,
   0.85,
   1.0,
   0.8800000000000001,
   0.96,
   0.85,
   0.85,
   0.9,
   1.0,
   1.0,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.85,
   1.0,
   0.85,
   0.95,
   0.9199999999999999,
   0.95,
   0.95,
   1.0,
   0.95,
   0.9199999999999999,
   0.8800000000000001,
   0.8400000000000001,
   0.85,
   1.0,
   1.0,
   0.95,
   0.96,
   0.95,
   0.95,
   0.9555999999999999,
   0.8728,
   0.8800000000000001,
   0.9,
   1.0,
   0.85,
   0.95,
   0.9846,
   0.9141999999999999,
   0.95,
   0.9,
   0.9,
   0.95,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.95,
   0.9635999999999999,
   0.9199999999999999,
   0.85,
   1.0,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.9,
   0.9454,
   0.9199999999999999,
   0.9,
   0.9,
   0.95,
   0.85,
   1.0,
   0.95,
   0.85,
   1.0,
   0.9199999999999999,
   0.9,
   1.0,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   0.85,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.8800000000000001,
   0.9,
   0.9199999999999999,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   1.0,
   1.0,
   1.0,
   0.8800000000000001,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   0.96,
   0.8400000000000001,
   0.85,
   0.95,
   1.0,
   0.8400000000000001,
   0.96,
   0.9,
   1.0,
   0.85,
   0.8352,
   0.9199999999999999,
   0.8400000000000001,
   0.8400000000000001,
   0.95,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   0.85,
   0.85,
   0.85,
   0.9199999999999999,
   0.9199999999999999,
   0.8800000000000001,
   0.8112,
   1.0,
   0.95,
   0.8400000000000001,
   0.9199999999999999,
   0.96,
   0.9334,
   0.95,
   0.9,
   0.9,
   0.95,
   0.96,
   0.85,
   0.9,
   0.9,
   0.8182,
   1.0,
   1.0,
   0.95,
   1.0,
   0.96,
   0.9199999999999999,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8666,
   0.8666,
   0.85,
   1.0,
   0.85,
   0.85,
   0.85,
   0.8666,
   0.85,
   0.85,
   0.9,
   0.85,
   0.96,
   0.8400000000000001,
   1.0,
   0.8666,
   0.8800000000000001,
   0.8400000000000001,
   0.85,
   0.9199999999999999,
   0.96,
   0.8615999999999999,
   0.96,
   0.9199999999999999,
   1.0,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.96,
   0.8400000000000001,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.9199999999999999,
   0.8400000000000001,
   1.0,
   0.9199999999999999,
   0.96,
   0.8800000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   1.0,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   1.0,
   0.8400000000000001,
   0.96,
   1.0,
   1.0,
   1.0,
   1.0,
   0.8400000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   0.96,
   0.9199999999999999,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   1.0,
   1.0,
   1.0,
   0.96,
   0.8800000000000001,
   0.96,
   0.9199999999999999,
   0.96,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.96,
   1.0,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.96,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   1.0,
   0.8800000000000001,
   0.8800000000000001,
   0.96,
   0.8400000000000001,
   0.8800000000000001,
   0.96,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.96,
   0.85,
   0.8800000000000001,
   0.96,
   1.0,
   0.9199999999999999,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.9,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   0.96,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   1.0,
   0.8400000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8400000000000001,
   0.96,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   1.0,
   0.8400000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.9199999999999999,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.9199999999999999,
   0.8400000000000001,
   0.8800000000000001,
   0.8800000000000001,
   0.8400000000000001,
   0.8800000000000001,
   0.96,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   0.9199999999999999,
   1.0,
   0.8400000000000001,
   0.9199999999999999,
   1.0,
   1.0,
   0.8800000000000001,
   1.0,
   0.9199999999999999,
   1.0,
   0.8800000000000001,
   0.96,
   0.8400000000000001,
   1.0,
   0.8800000000000001,
   0.9199999999999999,
   0.8800000000000001,
   0.9199999999999999,
   1.0,
   1.0,
   0.8800000000000001,
   0.8400000000000001,
   1.0,
   0.8400000000000001,
   0.96,
   0.8800000000000001,
   1.0,
   0.9199999999999999,
   0.96,
   1.0,
   0.9199999999999999,
   0.8800000000000001,
   1.0,
   ...],
  [0.7,
   0.8571428571428571,
   1.0,
   1.0,
   1.0,
   1.0,
   0.7777777777777777,
   1.0,
   1.0,
   0.8571428571428571,
   0.6666666666666666,
   0.4444444444444445,
   1.0,
   0.8181818181818182,
   1.0,
   1.0,
   0.8333333333333334,
   0.5555555555555556,
   0.5555555555555556,
   0.7,
   0.6,
   0.5,
   0.5555555555555556,
   0.6956521739130435,
   0.8333333333333334,
   0.3157894736842105,
   0.8333333333333334,
   0.875,
   1.0,
   1.0,
   0.7142857142857143,
   0.8571428571428571,
   0.8571428571428571,
   1.0,
   1.0,
   0.5714285714285715,
   0.9166666666666666,
   0.8000000000000002,
   0.5714285714285715,
   0.7,
   0.5,
   0.8333333333333334,
   0.5714285714285715,
   0.8181818181818182,
   0.5,
   0.5,
   0.6363636363636365,
   0.6666666666666666,
   0.6153846153846153,
   0.9166666666666666,
   0.5599999999999999,
   0.48484848484848486,
   0.8181818181818182,
   0.8750000000000001,
   0.9285714285714286,
   0.5,
   0.7692307692307693,
   0.875,
   0.6923076923076923,
   0.8888888888888888,
   0.9166666666666666,
   0.608695652173913,
   0.56,
   0.5714285714285715,
   0.8461538461538461,
   0.7407407407407408,
   0.5714285714285715,
   0.6666666666666667,
   0.7692307692307692,
   0.875,
   0.6,
   0.8000000000000002,
   0.8333333333333333,
   0.5714285714285715,
   0.5454545454545454,
   0.8571428571428571,
   0.7333333333333334,
   1.0,
   0.5925925925925926,
   0.875,
   0.8888888888888888,
   0.8333333333333334,
   0.8000000000000002,
   0.6666666666666665,
   0.6,
   0.380952380952381,
   0.8750000000000001,
   0.7777777777777778,
   0.6363636363636365,
   0.875,
   0.8333333333333334,
   0.8571428571428571,
   0.4666666666666667,
   0.5333333333333333,
   0.9375,
   0.888888888888889,
   0.8571428571428571,
   0.7741935483870968,
   0.6666666666666665,
   0.6451612903225806,
   0.5925925925925926,
   0.8571428571428571,
   0.4,
   0.8571428571428571,
   1.0,
   1.0,
   0.8571428571428571,
   0.7777777777777778,
   0.5,
   0.3076923076923077,
   0.1904761904761905,
   0.3913043478260869,
   0.4489795918367347,
   0.37500000000000006,
   0.2,
   0.6206896551724139,
   0.5490196078431373,
   0.4761904761904762,
   0.7142857142857143,
   0.7777777777777778,
   0.8387096774193549,
   0.7058823529411765,
   0.7605633802816901,
   0.8787878787878788,
   0.7368421052631577,
   0.9459459459459459,
   0.6885245901639345,
   0.6530612244897959,
   0.5,
   0.8,
   0.7058823529411765,
   0.782608695652174,
   0.42500000000000004,
   0.7428571428571429,
   0.6153846153846153,
   0.5882352941176471,
   0.9090909090909091,
   0.6363636363636364,
   0.7631578947368423,
   0.8524590163934426,
   0.8809523809523809,
   0.7142857142857142,
   0.7415730337078651,
   0.7500000000000001,
   0.5964912280701755,
   0.7294117647058824,
   0.6857142857142857,
   0.4307692307692308,
   0.9534883720930233,
   0.7142857142857143,
   0.7323943661971832,
   0.5970149253731343,
   0.7037037037037037,
   0.9166666666666666,
   0.7555555555555556,
   0.4,
   0.6024096385542168,
   0.7012987012987012,
   0.5434782608695652,
   0.7272727272727273,
   0.676923076923077,
   0.8571428571428572,
   0.7678571428571429,
   0.8705882352941177,
   0.6823529411764706,
   0.6666666666666666,
   0.8214285714285715,
   0.9714285714285714,
   0.8484848484848484,
   0.7692307692307693,
   1.0,
   0.625,
   0.8571428571428571,
   0.9285714285714286,
   0.875,
   0.6470588235294117,
   0.823529411764706,
   0.8571428571428572,
   0.5641025641025642,
   0.8771929824561403,
   0.7894736842105263,
   0.8888888888888888,
   0.8648648648648648,
   0.8400000000000001,
   0.6875000000000001,
   0.8181818181818182,
   0.7368421052631577,
   0.7450980392156863,
   0.5581395348837209,
   0.5714285714285714,
   0.75,
   1.0,
   0.5454545454545455,
   0.5517241379310344,
   0.8333333333333334,
   0.6451612903225806,
   0.76,
   0.9333333333333333,
   0.7222222222222223,
   0.7407407407407408,
   0.627450980392157,
   1.0,
   0.65,
   0.8717948717948718,
   0.7555555555555556,
   0.8461538461538461,
   0.8787878787878789,
   0.6666666666666667,
   0.8,
   0.8571428571428571,
   0.7272727272727272,
   1.0,
   0.9,
   0.9032258064516129,
   0.875,
   0.7777777777777777,
   1.0,
   0.6666666666666666,
   1.0,
   1.0,
   1.0,
   0.6666666666666666,
   0.9,
   1.0,
   0.875,
   1.0,
   1.0,
   1.0,
   0.625,
   1.0,
   1.0,
   1.0,
   0.7777777777777777,
   0.5714285714285715,
   0.8571428571428571,
   0.625,
   0.875,
   0.5714285714285715,
   1.0,
   0.7142857142857143,
   0.8571428571428571,
   0.8571428571428571,
   1.0,
   0.875,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.5714285714285715,
   0.5,
   0.8571428571428571,
   0.6,
   0.888888888888889,
   0.8333333333333334,
   0.8333333333333334,
   1.0,
   0.8571428571428572,
   1.0,
   0.7142857142857143,
   0.923076923076923,
   0.8333333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.625,
   0.923076923076923,
   0.7777777777777777,
   1.0,
   0.5555555555555556,
   0.625,
   0.6666666666666666,
   0.6666666666666665,
   0.6666666666666666,
   0.5555555555555556,
   0.7,
   0.6666666666666665,
   0.5,
   0.5714285714285715,
   0.5,
   0.5714285714285715,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.8333333333333334,
   1.0,
   1.0,
   0.8571428571428571,
   1.0,
   0.8571428571428571,
   0.9090909090909091,
   1.0,
   1.0,
   1.0,
   0.7499999999999999,
   1.0,
   0.75,
   1.0,
   0.75,
   1.0,
   1.0,
   0.8571428571428571,
   0.8333333333333334,
   0.75,
   0.7142857142857143,
   0.75,
   1.0,
   1.0,
   1.0,
   0.7142857142857143,
   0.875,
   1.0,
   1.0,
   1.0,
   0.6923076923076924,
   0.8333333333333334,
   0.9,
   0.8333333333333334,
   1.0,
   0.5555555555555556,
   0.8333333333333334,
   0.8571428571428571,
   0.7272727272727273,
   0.7692307692307692,
   0.875,
   0.875,
   0.75,
   0.8888888888888888,
   0.8333333333333334,
   0.5714285714285715,
   0.923076923076923,
   0.4705882352941177,
   0.6,
   0.6666666666666665,
   0.7999999999999999,
   0.5714285714285715,
   0.6666666666666666,
   0.7777777777777777,
   0.6666666666666666,
   0.7142857142857143,
   0.30769230769230765,
   0.5714285714285715,
   0.5333333333333333,
   0.42857142857142855,
   0.6666666666666665,
   0.6666666666666665,
   0.39999999999999997,
   0.28571428571428575,
   0.5333333333333333,
   0.7857142857142856,
   0.75,
   0.7142857142857143,
   0.5454545454545454,
   0.8571428571428571,
   0.4000000000000001,
   0.625,
   0.888888888888889,
   0.7142857142857143,
   0.6363636363636365,
   0.8571428571428571,
   0.8571428571428571,
   0.56,
   0.6666666666666665,
   0.6666666666666666,
   0.7,
   0.5833333333333334,
   0.5555555555555556,
   0.7000000000000001,
   0.7777777777777777,
   0.5714285714285715,
   0.7142857142857143,
   0.8181818181818182,
   0.7272727272727272,
   0.888888888888889,
   0.5833333333333334,
   0.9,
   0.5,
   0.608695652173913,
   0.5882352941176471,
   0.7142857142857143,
   0.6153846153846153,
   0.8000000000000002,
   0.75,
   0.3225806451612903,
   0.5806451612903226,
   0.7692307692307692,
   0.4444444444444444,
   0.8695652173913044,
   0.75,
   1.0,
   0.45454545454545453,
   0.9090909090909091,
   0.8571428571428571,
   0.46153846153846156,
   0.4761904761904762,
   0.5517241379310344,
   0.375,
   0.5454545454545454,
   0.6666666666666666,
   0.6250000000000001,
   0.9,
   0.2727272727272727,
   0.8750000000000001,
   0.5,
   0.6666666666666666,
   0.5882352941176471,
   0.6923076923076924,
   0.8571428571428571,
   0.6923076923076923,
   0.48000000000000004,
   0.4571428571428571,
   0.3846153846153846,
   0.5833333333333334,
   0.5,
   0.8181818181818182,
   0.75,
   0.9,
   0.5,
   0.7272727272727272,
   0.6285714285714286,
   0.75,
   0.8333333333333334,
   0.4999999999999999,
   0.3333333333333333,
   0.7999999999999999,
   0.9,
   0.42857142857142855,
   0.5853658536585366,
   0.5714285714285714,
   0.26666666666666666,
   0.8000000000000002,
   0.625,
   0.8,
   0.7368421052631577,
   0.7199999999999999,
   0.5882352941176471,
   0.7200000000000001,
   0.8571428571428571,
   0.6666666666666666,
   1.0,
   1.0,
   0.8888888888888888,
   0.8,
   0.45454545454545453,
   0.5,
   0.5,
   0.9166666666666666,
   0.7999999999999999,
   0.7096774193548386,
   0.631578947368421,
   0.875,
   0.7999999999999999,
   0.7142857142857143,
   0.6923076923076924,
   0.7777777777777777,
   0.7272727272727272,
   1.0,
   0.75,
   0.7000000000000001,
   0.8571428571428571,
   0.6153846153846154,
   0.823529411764706,
   0.8571428571428571,
   0.25,
   0.5,
   0.8333333333333333,
   0.875,
   0.8181818181818181,
   0.9090909090909091,
   0.7142857142857143,
   0.6857142857142857,
   0.7142857142857143,
   0.75,
   0.75,
   0.7777777777777777,
   0.75,
   0.7999999999999999,
   0.9230769230769231,
   0.888888888888889,
   0.6153846153846154,
   0.41666666666666663,
   0.7826086956521738,
   0.6111111111111112,
   0.7142857142857143,
   0.7000000000000001,
   0.6923076923076924,
   0.7999999999999999,
   0.7826086956521738,
   0.75,
   0.5161290322580646,
   0.2857142857142857,
   0.7777777777777777,
   0.888888888888889,
   0.75,
   0.7272727272727273,
   0.48275862068965514,
   0.8333333333333334,
   0.625,
   0.7142857142857143,
   0.75,
   0.6842105263157895,
   0.6363636363636364,
   0.8823529411764706,
   0.6,
   0.4,
   0.75,
   0.6666666666666666,
   0.7272727272727272,
   0.4444444444444445,
   1.0,
   0.9333333333333333,
   0.4545454545454546,
   0.6153846153846154,
   0.6666666666666666,
   0.7857142857142857,
   0.5714285714285714,
   0.5454545454545455,
   0.75,
   0.7999999999999999,
   0.47619047619047616,
   0.6153846153846154,
   0.6,
   0.8571428571428571,
   0.75,
   0.6666666666666666,
   0.5185185185185185,
   0.5,
   1.0,
   0.75,
   0.823529411764706,
   0.6923076923076924,
   0.7692307692307692,
   0.7000000000000001,
   1.0,
   1.0,
   0.8000000000000002,
   0.7692307692307693,
   0.7777777777777777,
   0.4444444444444445,
   0.5714285714285714,
   0.7333333333333334,
   0.7586206896551724,
   0.3333333333333333,
   0.7999999999999999,
   0.75,
   0.9090909090909091,
   0.5333333333333333,
   0.6666666666666665,
   0.7586206896551724,
   0.75,
   1.0,
   1.0,
   0.9500000000000001,
   0.5263157894736842,
   0.5925925925925926,
   1.0,
   0.5,
   0.9090909090909091,
   1.0,
   0.5714285714285715,
   0.2,
   0.8000000000000002,
   0.7169811320754718,
   0.5263157894736842,
   0.6440677966101696,
   0.631578947368421,
   0.7499999999999999,
   0.5714285714285715,
   0.8125000000000001,
   0.6363636363636364,
   0.380952380952381,
   0.7428571428571429,
   0.45454545454545453,
   0.4680851063829787,
   0.7333333333333334,
   0.8571428571428571,
   0.6428571428571429,
   0.7142857142857143,
   0.76,
   0.8571428571428571,
   0.8979591836734695,
   0.6153846153846154,
   1.0,
   0.9615384615384615,
   0.6666666666666665,
   0.6666666666666666,
   0.8571428571428571,
   0.5806451612903226,
   0.9302325581395349,
   0.8275862068965517,
   0.56,
   1.0,
   0.742857142857143,
   0.6086956521739131,
   0.37499999999999994,
   0.823529411764706,
   0.8125000000000001,
   0.8571428571428571,
   0.8888888888888888,
   0.5,
   0.625,
   0.8125000000000001,
   0.9655172413793104,
   0.7142857142857143,
   0.41176470588235287,
   0.37499999999999994,
   0.28571428571428575,
   0.8717948717948718,
   0.742857142857143,
   1.0,
   0.6363636363636364,
   1.0,
   0.7450980392156863,
   0.6,
   1.0,
   0.717948717948718,
   0.6153846153846153,
   1.0,
   0.7999999999999999,
   0.8888888888888888,
   0.6470588235294117,
   0.42857142857142855,
   0.8095238095238096,
   0.7999999999999999,
   0.8947368421052632,
   0.9230769230769231,
   0.8125000000000001,
   0.43478260869565216,
   0.5531914893617021,
   0.6599999999999999,
   0.7017543859649122,
   0.5581395348837209,
   0.7755102040816326,
   0.6222222222222223,
   0.935064935064935,
   0.7142857142857143,
   0.888888888888889,
   0.9166666666666665,
   0.6,
   0.5263157894736842,
   0.8787878787878787,
   0.9666666666666667,
   0.6923076923076923,
   0.782608695652174,
   0.5853658536585366,
   0.68,
   0.8043478260869567,
   0.9285714285714286,
   0.48,
   0.6304347826086957,
   0.6296296296296297,
   0.7954545454545455,
   0.736842105263158,
   0.6153846153846154,
   0.851063829787234,
   0.8484848484848485,
   0.7142857142857143,
   0.5454545454545454,
   0.6666666666666666,
   0.8041237113402062,
   0.6190476190476191,
   0.9199999999999999,
   0.5757575757575758,
   0.7777777777777778,
   0.6470588235294118,
   0.7457627118644068,
   0.9285714285714286,
   0.5813953488372093,
   0.631578947368421,
   0.4814814814814815,
   0.9523809523809523,
   0.7500000000000001,
   0.5531914893617021,
   0.8363636363636363,
   0.6818181818181819,
   0.7761194029850748,
   0.5757575757575758,
   0.5000000000000001,
   0.816326530612245,
   0.6956521739130435,
   0.7301587301587302,
   0.7042253521126761,
   0.8533333333333334,
   0.576923076923077,
   0.6451612903225806,
   0.6923076923076923,
   0.845360824742268,
   0.3333333333333333,
   0.8888888888888888,
   0.8351648351648352,
   0.6875,
   0.7931034482758621,
   0.6486486486486486,
   0.5490196078431373,
   0.8297872340425532,
   0.8484848484848485,
   0.7228915662650602,
   0.7777777777777778,
   0.5,
   0.7083333333333334,
   0.8387096774193549,
   0.8955223880597015,
   0.45,
   0.923076923076923,
   0.6774193548387096,
   0.6046511627906976,
   0.7499999999999999,
   0.7920792079207922,
   0.6382978723404256,
   0.7419354838709677,
   0.6470588235294118,
   0.7058823529411765,
   0.6129032258064515,
   0.8051948051948051,
   0.44,
   0.830188679245283,
   0.7636363636363638,
   0.7428571428571429,
   0.8985507246376812,
   0.6,
   0.5581395348837209,
   0.7191011235955056,
   0.8791208791208791,
   0.8378378378378377,
   0.7250000000000001,
   0.6666666666666666,
   0.875,
   0.6938775510204083,
   0.5185185185185186,
   0.7777777777777778,
   0.5111111111111111,
   0.6097560975609757,
   0.689655172413793,
   0.5866666666666667,
   0.8409090909090909,
   0.6875,
   0.8,
   0.9295774647887323,
   0.47619047619047616,
   0.9382716049382716,
   0.7272727272727273,
   0.40816326530612246,
   0.6666666666666667,
   0.8292682926829269,
   0.7419354838709677,
   0.7368421052631577,
   0.5555555555555556,
   0.6933333333333334,
   0.8952380952380952,
   0.6078431372549019,
   0.689655172413793,
   0.5945945945945946,
   0.651685393258427,
   0.7727272727272727,
   0.5517241379310345,
   0.6588235294117646,
   0.7076923076923077,
   0.8,
   0.42857142857142855,
   0.7083333333333334,
   0.7951807228915662,
   0.7572815533980582,
   0.5151515151515152,
   0.6153846153846153,
   0.6842105263157895,
   0.7450980392156863,
   0.8333333333333333,
   0.8000000000000002,
   0.5753424657534246,
   0.6101694915254238,
   0.9411764705882354,
   0.35000000000000003,
   0.9024390243902439,
   0.9655172413793104,
   0.8607594936708861,
   0.8760330578512397,
   0.7391304347826086,
   0.9215686274509804,
   0.6913580246913581,
   0.5263157894736842,
   0.7692307692307692,
   0.5106382978723404,
   0.7710843373493975,
   0.888888888888889,
   0.5454545454545454,
   0.5591397849462365,
   0.8205128205128206,
   0.8064516129032259,
   0.8666666666666666,
   0.7692307692307694,
   0.5357142857142857,
   0.8,
   0.7142857142857143,
   0.6486486486486486,
   0.6060606060606061,
   0.5507246376811593,
   0.5238095238095238,
   0.7111111111111111,
   0.76,
   0.9333333333333333,
   0.8529411764705882,
   0.7941176470588235,
   0.8219178082191781,
   0.8695652173913043,
   0.5185185185185185,
   0.7500000000000001,
   0.7317073170731708,
   0.5833333333333334,
   0.6376811594202898,
   0.9411764705882353,
   0.7,
   0.8444444444444444,
   0.6885245901639344,
   0.6451612903225806,
   0.7333333333333334,
   0.7076923076923077,
   0.9285714285714286,
   0.7755102040816326,
   0.8055555555555555,
   0.65359477124183,
   0.8108108108108109,
   0.761904761904762,
   0.9,
   0.6285714285714286,
   0.9090909090909091,
   0.8947368421052632,
   0.6666666666666667,
   0.7199999999999999,
   0.8333333333333333,
   0.7407407407407407,
   0.8421052631578947,
   0.8333333333333334,
   0.875,
   0.7010309278350515,
   0.9090909090909091,
   0.7567567567567567,
   0.6744186046511628,
   0.8135593220338982,
   0.9090909090909091,
   0.6391752577319586,
   0.806451612903226,
   0.7333333333333334,
   0.8533333333333334,
   0.8125,
   0.7317073170731706,
   0.8813559322033898,
   0.7350427350427351,
   0.8852459016393442,
   0.8333333333333333,
   0.8000000000000002,
   0.9022556390977444,
   0.8732394366197184,
   0.7032967032967034,
   0.5625,
   0.8985507246376812,
   0.9166666666666666,
   0.6857142857142857,
   0.43478260869565216,
   0.8163265306122449,
   0.8,
   0.7792207792207791,
   0.8333333333333333,
   0.8108108108108107,
   0.9056603773584906,
   0.7397260273972601,
   0.8333333333333334,
   0.8571428571428571,
   0.8703703703703703,
   0.6909090909090908,
   0.5757575757575758,
   0.8000000000000002,
   0.7586206896551724,
   0.7777777777777778,
   0.8275862068965518,
   0.9473684210526315,
   1.0,
   0.9130434782608695,
   0.8372093023255814,
   0.7407407407407408,
   0.7272727272727273,
   0.8,
   0.6829268292682927,
   0.45161290322580644,
   0.5333333333333333,
   0.7741935483870969,
   0.8260869565217392,
   0.8205128205128205,
   0.5882352941176471,
   0.8571428571428571,
   0.5957446808510638,
   0.888888888888889,
   0.6538461538461539,
   0.6222222222222222,
   0.8333333333333334,
   0.47058823529411764,
   0.6,
   0.8421052631578948,
   0.65,
   0.8571428571428571,
   0.5555555555555555,
   0.7272727272727272,
   0.5263157894736842,
   0.8333333333333333,
   0.875,
   0.8421052631578948,
   0.8387096774193549,
   0.7999999999999999,
   0.9166666666666666,
   0.7307692307692308,
   0.6190476190476191,
   0.7272727272727272,
   0.9142857142857143,
   0.7741935483870969,
   0.7111111111111111,
   0.9411764705882353,
   0.7142857142857143,
   0.6875,
   0.625,
   0.9166666666666666,
   0.8333333333333333,
   0.8571428571428571,
   0.8571428571428572,
   0.6857142857142857,
   0.7894736842105263,
   0.819672131147541,
   0.8717948717948718,
   0.7916666666666667,
   0.6222222222222222,
   0.9142857142857143,
   0.7027027027027027,
   0.5714285714285715,
   0.7317073170731708,
   0.7368421052631579,
   0.6486486486486486,
   0.7058823529411765,
   0.65,
   0.6666666666666667,
   0.742857142857143,
   0.793103448275862,
   0.8571428571428572,
   0.8461538461538461,
   0.5142857142857143,
   0.689655172413793,
   0.625,
   0.7692307692307692,
   0.6896551724137931,
   0.6382978723404256,
   0.4897959183673469,
   0.4761904761904762,
   0.9142857142857143,
   0.7741935483870968,
   0.7333333333333334,
   0.36842105263157887,
   0.8571428571428571,
   0.8095238095238095,
   0.6,
   0.8823529411764706,
   0.41379310344827586,
   0.7777777777777778,
   0.7692307692307692,
   0.8235294117647058,
   0.7272727272727273,
   0.7222222222222223,
   0.7307692307692308,
   0.7647058823529412,
   0.8571428571428571,
   0.8333333333333333,
   0.8823529411764706,
   0.8500000000000001,
   0.35294117647058826,
   0.7000000000000001,
   0.625,
   0.5454545454545455,
   0.7692307692307692,
   0.8108108108108109,
   0.5217391304347826,
   0.7272727272727272,
   0.7906976744186046,
   0.875,
   0.8695652173913043,
   0.7333333333333333,
   0.576923076923077,
   0.8636363636363636,
   0.6857142857142857,
   0.9333333333333333,
   0.7272727272727273,
   0.9,
   0.8947368421052632,
   0.8085106382978724,
   0.4999999999999999,
   0.6111111111111112,
   0.7727272727272727,
   0.7857142857142856,
   0.9361702127659574,
   0.8,
   0.9,
   0.7878787878787878,
   0.7499999999999999,
   0.7222222222222223,
   0.7317073170731708,
   0.8947368421052632,
   0.8421052631578948,
   ...]],
 0.6: [1413,
  [0.48,
   0.55,
   0.523,
   0.4666,
   0.48,
   0.6,
   0.43339999999999995,
   0.6,
   0.52,
   0.5599999999999999,
   0.6,
   0.5599999999999999,
   0.5624,
   0.6,
   0.5599999999999999,
   0.55,
   0.5599999999999999,
   0.45,
   0.55,
   0.52,
   0.5599999999999999,
   0.52,
   0.6,
   0.6,
   0.55,
   0.48,
   0.5,
   0.5,
   0.475,
   0.6,
   0.43339999999999995,
   0.45,
   0.55,
   0.55,
   0.44000000000000006,
   0.6,
   0.6,
   0.4666,
   0.6,
   0.5,
   0.5,
   0.55,
   0.6,
   0.6,
   0.55,
   0.5599999999999999,
   0.52,
   0.5384,
   0.44000000000000006,
   0.44000000000000006,
   0.52,
   0.45,
   0.6,
   0.6,
   0.48,
   0.44000000000000006,
   0.52,
   0.52,
   0.5599999999999999,
   0.48,
   0.52,
   0.48,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.44000000000000006,
   0.6,
   0.52,
   0.44000000000000006,
   0.44000000000000006,
   0.44000000000000006,
   0.52,
   0.48,
   0.52,
   0.44000000000000006,
   0.52,
   0.6,
   0.48,
   0.5599999999999999,
   0.52,
   0.48,
   0.48,
   0.6,
   0.48,
   0.6,
   0.6,
   0.52,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.5599999999999999,
   0.5599999999999999,
   0.48,
   0.6,
   0.44000000000000006,
   0.48,
   0.44000000000000006,
   0.52,
   0.44000000000000006,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.6,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.48,
   0.5599999999999999,
   0.6,
   0.5599999999999999,
   0.5599999999999999,
   0.6,
   0.5599999999999999,
   0.48,
   0.5599999999999999,
   0.6,
   0.52,
   0.6,
   0.6,
   0.6,
   0.48,
   0.6,
   0.52,
   0.5599999999999999,
   0.52,
   0.52,
   0.52,
   0.52,
   0.6,
   0.52,
   0.5599999999999999,
   0.52,
   0.52,
   0.44000000000000006,
   0.6,
   0.6,
   0.5599999999999999,
   0.52,
   0.44000000000000006,
   0.48,
   0.48,
   0.52,
   0.5599999999999999,
   0.44000000000000006,
   0.52,
   0.6,
   0.44000000000000006,
   0.5599999999999999,
   0.5599999999999999,
   0.6,
   0.5599999999999999,
   0.5599999999999999,
   0.52,
   0.44000000000000006,
   0.5599999999999999,
   0.52,
   0.48,
   0.5599999999999999,
   0.6,
   0.52,
   0.6,
   0.44000000000000006,
   0.6,
   0.48,
   0.52,
   0.5599999999999999,
   0.6,
   0.52,
   0.6,
   0.52,
   0.52,
   0.52,
   0.48,
   0.52,
   0.52,
   0.6,
   0.5599999999999999,
   0.52,
   0.5599999999999999,
   0.44000000000000006,
   0.52,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.5599999999999999,
   0.5599999999999999,
   0.44000000000000006,
   0.6,
   0.52,
   0.52,
   0.6,
   0.52,
   0.5599999999999999,
   0.6,
   0.48,
   0.52,
   0.52,
   0.5599999999999999,
   0.52,
   0.6,
   0.52,
   0.48,
   0.6,
   0.6,
   0.48,
   0.6,
   0.6,
   0.44000000000000006,
   0.6,
   0.6,
   0.6,
   0.44000000000000006,
   0.52,
   0.48,
   0.48,
   0.5599999999999999,
   0.6,
   0.6,
   0.5599999999999999,
   0.6,
   0.5599999999999999,
   0.6,
   0.52,
   0.6,
   0.44000000000000006,
   0.6,
   0.52,
   0.6,
   0.45,
   0.6,
   0.6,
   0.5599999999999999,
   0.55,
   0.6,
   0.6,
   0.6,
   0.48,
   0.52,
   0.6,
   0.6,
   0.48,
   0.5,
   0.6,
   0.55,
   0.6,
   0.6,
   0.48,
   0.6,
   0.48,
   0.5599999999999999,
   0.6,
   0.55,
   0.45,
   0.55,
   0.44000000000000006,
   0.6,
   0.55,
   0.5,
   0.6,
   0.5599999999999999,
   0.466666666666666,
   0.52,
   0.44000000000000006,
   0.52,
   0.52,
   0.44000000000000006,
   0.6,
   0.48,
   0.5599999999999999,
   0.5599999999999999,
   0.52,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   0.52,
   0.55,
   0.52,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   0.48,
   0.52,
   0.44000000000000006,
   0.6,
   0.52,
   0.5599999999999999,
   0.44000000000000006,
   0.44000000000000006,
   0.5,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.52,
   0.44000000000000006,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.48,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.52,
   0.44000000000000006,
   0.5599999999999999,
   0.6,
   0.6,
   0.48,
   0.55,
   0.475,
   0.5833999999999999,
   0.52,
   0.6,
   0.48,
   0.44000000000000006,
   0.52,
   0.44000000000000006,
   0.48,
   0.44000000000000006,
   0.45,
   0.5065999999999999,
   0.5,
   0.44000000000000006,
   0.6,
   0.44000000000000006,
   0.6,
   0.6,
   0.6,
   0.6,
   0.52,
   0.55,
   0.45,
   0.55,
   0.48,
   0.6,
   0.6,
   0.6,
   0.5599999999999999,
   0.44000000000000006,
   0.6,
   0.48,
   0.48,
   0.5,
   0.5,
   0.52,
   0.5599999999999999,
   0.55,
   0.6,
   0.52,
   0.55,
   0.55,
   0.48,
   0.44000000000000006,
   0.5599999999999999,
   0.55,
   0.45,
   0.48,
   0.5599999999999999,
   0.5334,
   0.5599999999999999,
   0.5,
   0.5,
   0.45,
   0.5599999999999999,
   0.6,
   0.6,
   0.5599999999999999,
   0.44000000000000006,
   0.6,
   0.55,
   0.44000000000000006,
   0.5065999999999999,
   0.6,
   0.5599999999999999,
   0.5,
   0.5636,
   0.52,
   0.45,
   0.44000000000000006,
   0.5,
   0.5599999999999999,
   0.5599999999999999,
   0.5599999999999999,
   0.5599999999999999,
   0.52,
   0.6,
   0.4666,
   0.52,
   0.52,
   0.52,
   0.44000000000000006,
   0.52,
   0.52,
   0.6,
   0.6,
   0.44000000000000006,
   0.52,
   0.6,
   0.575,
   0.44000000000000006,
   0.6,
   0.6,
   0.6,
   0.52,
   0.52,
   0.5599999999999999,
   0.6,
   0.5,
   0.52,
   0.44000000000000006,
   0.5599999999999999,
   0.5599999999999999,
   0.5538000000000001,
   0.48,
   0.45,
   0.44000000000000006,
   0.6,
   0.5166000000000001,
   0.6,
   0.52,
   0.6,
   0.5599999999999999,
   0.5334,
   0.6,
   0.6,
   0.55,
   0.6,
   0.55,
   0.48,
   0.6,
   0.6,
   0.52,
   0.5,
   0.55,
   0.5,
   0.6,
   0.44000000000000006,
   0.5599999999999999,
   0.4666,
   0.6,
   0.5,
   0.6,
   0.52,
   0.52,
   0.48,
   0.52,
   0.6,
   0.44000000000000006,
   0.45,
   0.52,
   0.55,
   0.5,
   0.5599999999999999,
   0.6,
   0.5,
   0.52,
   0.5599999999999999,
   0.6,
   0.52,
   0.6,
   0.44000000000000006,
   0.48,
   0.48,
   0.48,
   0.48,
   0.6,
   0.52,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.52,
   0.6,
   0.5599999999999999,
   0.5599999999999999,
   0.44000000000000006,
   0.5599999999999999,
   0.6,
   0.44000000000000006,
   0.6,
   0.44000000000000006,
   0.6,
   0.44000000000000006,
   0.5599999999999999,
   0.6,
   0.6,
   0.48,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   0.5599999999999999,
   0.48,
   0.48,
   0.48,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.5599999999999999,
   0.6,
   0.44000000000000006,
   0.5599999999999999,
   0.44000000000000006,
   0.6,
   0.6,
   0.6,
   0.52,
   0.45,
   0.6,
   0.52,
   0.5599999999999999,
   0.44000000000000006,
   0.5599999999999999,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.52,
   0.48,
   0.52,
   0.45,
   0.52,
   0.44000000000000006,
   0.6,
   0.52,
   0.48,
   0.52,
   0.6,
   0.6,
   0.6,
   0.52,
   0.6,
   0.6,
   0.6,
   0.52,
   0.6,
   0.5599999999999999,
   0.5599999999999999,
   0.5599999999999999,
   0.5599999999999999,
   0.6,
   0.52,
   0.5,
   0.52,
   0.44000000000000006,
   0.52,
   0.52,
   0.52,
   0.6,
   0.48,
   0.52,
   0.466,
   0.6,
   0.48,
   0.48,
   0.5599999999999999,
   0.44000000000000006,
   0.6,
   0.44000000000000006,
   0.48,
   0.6,
   0.44000000000000006,
   0.5599999999999999,
   0.5599999999999999,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.5599999999999999,
   0.52,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.52,
   0.5599999999999999,
   0.48,
   0.48,
   0.466,
   0.48,
   0.5599999999999999,
   0.5599999999999999,
   0.48,
   0.44000000000000006,
   0.6,
   0.5599999999999999,
   0.44000000000000006,
   0.44000000000000006,
   0.5599999999999999,
   0.44000000000000006,
   0.5599999999999999,
   0.44000000000000006,
   0.48,
   0.6,
   0.6,
   0.5660000000000001,
   0.44000000000000006,
   0.6,
   0.5599999999999999,
   0.44000000000000006,
   0.48,
   0.48,
   0.5599999999999999,
   0.6,
   0.6,
   0.52,
   0.48,
   0.5599999999999999,
   0.48,
   0.5599999999999999,
   0.5599999999999999,
   0.52,
   0.52,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.48,
   0.6,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.5599999999999999,
   0.44000000000000006,
   0.44000000000000006,
   0.5599999999999999,
   0.44000000000000006,
   0.52,
   0.6,
   0.5599999999999999,
   0.52,
   0.52,
   0.48,
   0.6,
   0.6,
   0.42222222222222194,
   0.5599999999999999,
   0.6,
   0.52,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.44000000000000006,
   0.52,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.6,
   0.48,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.6,
   0.48,
   0.42222222222222194,
   0.5599999999999999,
   0.6,
   0.52,
   0.44000000000000006,
   0.6,
   0.52,
   0.48,
   0.48,
   0.6,
   0.52,
   0.52,
   0.48,
   0.48,
   0.48,
   0.48,
   0.49333333333333396,
   0.5599999999999999,
   0.6,
   0.48,
   0.48,
   0.6,
   0.48,
   0.48,
   0.48,
   0.44000000000000006,
   0.5,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.6,
   0.5599999999999999,
   0.48,
   0.48,
   0.5,
   0.5599999999999999,
   0.44000000000000006,
   0.6,
   0.5599999999999999,
   0.44000000000000006,
   0.5,
   0.52,
   0.6,
   0.6,
   0.48,
   0.48,
   0.6,
   0.6,
   0.52,
   0.44000000000000006,
   0.5599999999999999,
   0.52,
   0.6,
   0.6,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   0.52,
   0.5599999999999999,
   0.48,
   0.48,
   0.52,
   0.44000000000000006,
   0.48,
   0.48,
   0.44000000000000006,
   0.44000000000000006,
   0.52,
   0.6,
   0.48,
   0.5599999999999999,
   0.5599999999999999,
   0.6,
   0.49333333333333396,
   0.5599999999999999,
   0.5599999999999999,
   0.48,
   0.48,
   0.49333333333333396,
   0.44000000000000006,
   0.52,
   0.52,
   0.5599999999999999,
   0.5,
   0.52,
   0.6,
   0.52,
   0.5599999999999999,
   0.6,
   0.52,
   0.5,
   0.44000000000000006,
   0.5599999999999999,
   0.52,
   0.44000000000000006,
   0.5636,
   0.5599999999999999,
   0.6,
   0.5334,
   0.4666,
   0.6,
   0.5599999999999999,
   0.55,
   0.5,
   0.55,
   0.6,
   0.48,
   0.6,
   0.55,
   0.52,
   0.44000000000000006,
   0.44000000000000006,
   0.48,
   0.6,
   0.48,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5294,
   0.44000000000000006,
   0.45,
   0.44000000000000006,
   0.6,
   0.5,
   0.55,
   0.6,
   0.6,
   0.45,
   0.6,
   0.45,
   0.55,
   0.44000000000000006,
   0.5,
   0.45,
   0.55,
   0.6,
   0.6,
   0.6,
   0.5599999999999999,
   0.6,
   0.6,
   0.48,
   0.52,
   0.6,
   0.52,
   0.45,
   0.55,
   0.55,
   0.52,
   0.6,
   0.52,
   0.52,
   0.48,
   0.48,
   0.6,
   0.5599999999999999,
   0.6,
   0.44000000000000006,
   0.5599999999999999,
   0.6,
   0.44000000000000006,
   0.6,
   0.6,
   0.6,
   0.6,
   0.5599999999999999,
   0.5599999999999999,
   0.6,
   0.6,
   0.6,
   0.6,
   0.55,
   0.6,
   0.5599999999999999,
   0.6,
   0.6,
   0.6,
   0.48,
   0.5599999999999999,
   0.6,
   0.5599999999999999,
   0.5,
   0.6,
   0.44000000000000006,
   0.44000000000000006,
   0.5599999999999999,
   0.5818,
   0.52,
   0.5,
   0.5,
   0.55,
   0.55,
   0.55,
   0.5,
   0.52,
   0.6,
   0.55,
   0.6,
   0.5599999999999999,
   0.44000000000000006,
   0.5599999999999999,
   0.55,
   0.6,
   0.6,
   0.5599999999999999,
   0.48,
   0.6,
   0.6,
   0.6,
   0.5,
   0.45,
   0.6,
   0.5599999999999999,
   0.55,
   0.52,
   0.6,
   0.55,
   0.52,
   0.48,
   0.6,
   0.55,
   0.6,
   0.5599999999999999,
   0.5334,
   0.6,
   0.5599999999999999,
   0.5,
   0.5,
   0.6,
   0.525,
   0.48,
   0.5599999999999999,
   0.5599999999999999,
   0.6,
   0.48,
   0.52,
   0.5599999999999999,
   0.48,
   0.55,
   0.5,
   0.55,
   0.6,
   0.6,
   0.6,
   0.5599999999999999,
   0.48,
   0.5,
   0.48,
   0.6,
   0.6,
   0.55,
   0.6,
   0.48,
   0.48,
   0.6,
   0.6,
   0.6,
   0.55,
   0.6,
   0.6,
   0.6,
   0.5176000000000001,
   0.4666,
   0.45,
   0.5,
   0.52,
   0.6,
   0.45,
   0.6,
   0.5,
   0.45,
   0.5334,
   0.6,
   0.6,
   0.48,
   0.48,
   0.6,
   0.6,
   0.44000000000000006,
   0.6,
   0.5599999999999999,
   0.52,
   0.6,
   0.54,
   0.6,
   0.5334,
   0.44000000000000006,
   0.4666,
   0.45,
   0.52,
   0.6,
   0.6,
   0.6,
   0.6,
   0.6,
   0.48,
   0.44000000000000006,
   0.6,
   0.6,
   0.44000000000000006,
   0.6,
   0.55,
   0.45,
   0.5,
   0.5599999999999999,
   0.55,
   0.6,
   0.6,
   0.48,
   0.6,
   0.6,
   0.5334,
   0.6,
   0.55,
   0.55,
   0.52,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   0.48,
   0.44000000000000006,
   0.6,
   0.48,
   0.5599999999999999,
   0.5599999999999999,
   0.44000000000000006,
   0.52,
   0.5599999999999999,
   ...],
  [0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.7692307692307692,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.7777777777777777,
   0.75,
   0.6,
   0.7142857142857143,
   0.7142857142857143,
   0.28571428571428575,
   0.5555555555555556,
   0.6666666666666665,
   0.625,
   0.5,
   0.4444444444444445,
   0.5714285714285715,
   0.5714285714285715,
   0.5714285714285715,
   0.5,
   0.28571428571428564,
   0.888888888888889,
   0.5714285714285715,
   0.7142857142857143,
   0.5714285714285715,
   0.8333333333333334,
   0.8333333333333334,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.6363636363636364,
   0.4000000000000001,
   0.8333333333333334,
   0.6666666666666666,
   0.8,
   0.5333333333333333,
   0.5217391304347826,
   0.42857142857142855,
   0.5,
   0.631578947368421,
   0.4615384615384615,
   0.5,
   0.2857142857142857,
   0.37499999999999994,
   0.37499999999999994,
   0.5263157894736842,
   0.5,
   0.4375,
   0.5,
   0.5,
   0.33333333333333326,
   0.7368421052631577,
   0.6666666666666665,
   0.625,
   0.4444444444444445,
   0.75,
   0.36363636363636365,
   0.3243243243243243,
   0.5,
   0.7777777777777777,
   0.3448275862068965,
   0.4444444444444445,
   0.6428571428571429,
   0.7826086956521738,
   0.7428571428571429,
   0.4117647058823529,
   0.5454545454545454,
   0.5,
   0.4166666666666667,
   0.5185185185185185,
   0.32,
   0.5714285714285714,
   0.6666666666666665,
   0.4615384615384615,
   0.3,
   0.6896551724137931,
   0.26086956521739135,
   0.21428571428571427,
   0.75,
   0.6666666666666665,
   0.3333333333333333,
   0.6666666666666666,
   0.35714285714285715,
   0.9,
   0.6315789473684211,
   0.5,
   0.3703703703703704,
   0.3846153846153846,
   0.5882352941176471,
   0.4117647058823529,
   0.8,
   0.48648648648648646,
   0.24242424242424243,
   0.5555555555555556,
   0.5,
   0.6666666666666666,
   0.7000000000000001,
   0.36363636363636365,
   0.5,
   0.4,
   0.4666666666666667,
   0.5384615384615384,
   0.6153846153846153,
   0.631578947368421,
   0.6666666666666665,
   0.2631578947368421,
   0.875,
   0.18181818181818182,
   0.7692307692307692,
   0.6,
   0.9,
   0.2,
   0.625,
   0.75,
   0.56,
   0.38461538461538464,
   0.3157894736842105,
   0.8333333333333334,
   0.7142857142857143,
   0.339622641509434,
   0.35,
   0.3571428571428571,
   0.26865671641791045,
   0.20408163265306123,
   0.21739130434782608,
   0.25,
   0.15,
   0.24242424242424246,
   0.4444444444444444,
   0.125,
   0.5333333333333333,
   0.35000000000000003,
   0.3125,
   0.40816326530612246,
   0.16666666666666666,
   0.3076923076923077,
   0.253968253968254,
   0.14285714285714288,
   0.1818181818181818,
   0.13636363636363638,
   0.34782608695652173,
   0.25,
   0.21052631578947367,
   0.273972602739726,
   0.44897959183673464,
   0.372093023255814,
   0.26229508196721313,
   0.28571428571428575,
   0.391304347826087,
   0.35555555555555557,
   0.15384615384615385,
   0.23529411764705882,
   0.2127659574468085,
   0.2666666666666666,
   0.2807017543859649,
   0.19230769230769232,
   0.33333333333333326,
   0.41025641025641024,
   0.2941176470588235,
   0.2745098039215686,
   0.3333333333333333,
   0.18181818181818182,
   0.2380952380952381,
   0.32142857142857145,
   0.1818181818181818,
   0.5405405405405405,
   0.45714285714285713,
   0.20000000000000004,
   0.21621621621621623,
   0.3278688524590164,
   0.23809523809523808,
   0.16901408450704225,
   0.22222222222222224,
   0.20000000000000004,
   0.37499999999999994,
   0.26666666666666666,
   0.2641509433962264,
   0.2857142857142857,
   0.39285714285714285,
   0.22222222222222224,
   0.2769230769230769,
   0.3666666666666667,
   0.15999999999999998,
   0.37209302325581395,
   0.37837837837837834,
   0.42105263157894735,
   0.25641025641025644,
   0.36065573770491804,
   0.25925925925925924,
   0.17647058823529413,
   0.35294117647058826,
   0.20512820512820512,
   0.35294117647058826,
   0.2857142857142857,
   0.3404255319148936,
   0.43636363636363634,
   0.23076923076923078,
   0.3013698630136986,
   0.5,
   0.22727272727272724,
   0.7042253521126761,
   0.5245901639344263,
   0.5396825396825397,
   0.6545454545454545,
   0.6024096385542168,
   0.5714285714285715,
   0.6410256410256411,
   0.625,
   0.7027027027027025,
   0.8125,
   0.716417910447761,
   0.5,
   0.6382978723404256,
   0.49056603773584906,
   0.5666666666666667,
   0.47058823529411764,
   0.5116279069767442,
   0.5581395348837209,
   0.7692307692307692,
   0.6578947368421053,
   0.24390243902439024,
   0.5970149253731343,
   0.7692307692307693,
   0.5970149253731343,
   0.5151515151515151,
   0.509090909090909,
   0.48387096774193544,
   0.490566037735849,
   0.3859649122807018,
   0.42424242424242425,
   0.6000000000000001,
   0.4210526315789474,
   0.45454545454545453,
   0.7472527472527473,
   0.3225806451612903,
   0.6333333333333333,
   0.6739130434782609,
   0.417910447761194,
   0.4528301886792453,
   0.7407407407407408,
   0.4675324675324676,
   0.35000000000000003,
   0.6756756756756758,
   0.5116279069767442,
   0.5306122448979591,
   0.634920634920635,
   0.5833333333333333,
   0.6666666666666666,
   0.5084745762711865,
   0.7628865979381443,
   0.509090909090909,
   0.4000000000000001,
   0.6,
   0.3636363636363636,
   0.36363636363636365,
   0.5365853658536586,
   0.5454545454545455,
   0.7789473684210527,
   0.576923076923077,
   0.4444444444444445,
   0.5531914893617023,
   0.75,
   0.6486486486486486,
   0.8333333333333333,
   0.56,
   0.3636363636363636,
   0.46808510638297873,
   0.5,
   0.41025641025641024,
   0.5384615384615385,
   0.5853658536585366,
   0.6222222222222223,
   0.7777777777777777,
   0.25,
   0.6500000000000001,
   0.6545454545454547,
   0.5,
   0.8461538461538461,
   0.75,
   0.8888888888888888,
   0.7692307692307693,
   0.6956521739130435,
   0.6666666666666666,
   0.5294117647058824,
   0.5806451612903226,
   0.7428571428571428,
   0.7999999999999999,
   0.47058823529411764,
   0.7368421052631579,
   0.5217391304347826,
   0.9,
   0.9032258064516129,
   0.4074074074074074,
   0.5,
   0.5789473684210527,
   0.7333333333333334,
   0.5333333333333333,
   0.4516129032258065,
   0.4583333333333333,
   0.41025641025641024,
   0.5172413793103449,
   0.3181818181818182,
   0.7317073170731706,
   0.7352941176470589,
   0.4,
   0.5128205128205129,
   0.6250000000000001,
   0.7999999999999999,
   0.8571428571428571,
   0.7500000000000001,
   0.8333333333333334,
   0.8333333333333334,
   0.7500000000000001,
   0.8333333333333334,
   0.6666666666666666,
   0.8333333333333334,
   0.5882352941176471,
   0.8333333333333334,
   0.5882352941176471,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.6666666666666666,
   0.6666666666666666,
   0.8333333333333334,
   0.875,
   0.5555555555555556,
   0.6666666666666666,
   0.5,
   0.8333333333333334,
   0.7142857142857143,
   0.7000000000000001,
   0.8333333333333334,
   0.8333333333333334,
   0.42857142857142855,
   0.7058823529411765,
   0.875,
   0.75,
   0.75,
   0.5454545454545454,
   0.8333333333333334,
   0.75,
   0.5,
   0.5882352941176471,
   0.7142857142857143,
   0.5555555555555556,
   0.631578947368421,
   0.6,
   0.5714285714285715,
   0.4444444444444445,
   0.7142857142857143,
   0.5714285714285715,
   0.6666666666666666,
   0.6666666666666666,
   0.4444444444444445,
   0.5714285714285715,
   0.45454545454545453,
   0.625,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.3157894736842105,
   0.6666666666666666,
   0.42105263157894735,
   0.37499999999999994,
   0.5555555555555556,
   0.5454545454545454,
   0.75,
   0.5,
   0.625,
   0.7692307692307692,
   0.625,
   0.25,
   0.5,
   0.47058823529411764,
   0.30769230769230765,
   0.5,
   0.33333333333333326,
   0.7142857142857143,
   0.5263157894736842,
   0.4210526315789474,
   0.28571428571428575,
   0.1904761904761905,
   0.5714285714285714,
   0.8333333333333334,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.6666666666666666,
   0.75,
   0.75,
   0.8888888888888888,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.75,
   0.7142857142857143,
   0.7,
   0.8333333333333334,
   0.6666666666666666,
   0.7142857142857143,
   0.6363636363636364,
   0.8333333333333334,
   0.5714285714285715,
   0.8,
   0.5714285714285715,
   0.6666666666666665,
   0.8333333333333334,
   0.6666666666666666,
   0.5,
   0.5714285714285715,
   0.6666666666666666,
   0.42857142857142855,
   0.5,
   0.5454545454545454,
   0.6666666666666666,
   0.6,
   0.5882352941176471,
   0.6666666666666666,
   0.5714285714285715,
   0.7142857142857143,
   0.7777777777777777,
   0.625,
   0.7142857142857143,
   0.6363636363636364,
   0.39999999999999997,
   0.7692307692307692,
   0.4444444444444444,
   0.4347826086956521,
   0.5,
   0.4285714285714285,
   0.5185185185185186,
   0.37499999999999994,
   0.48,
   0.41666666666666663,
   0.625,
   0.7142857142857143,
   0.4,
   0.8333333333333334,
   0.4,
   0.4799999999999999,
   0.4444444444444445,
   0.588235294117647,
   0.3076923076923077,
   0.6,
   0.5,
   0.4,
   0.5714285714285715,
   0.4,
   0.5714285714285715,
   0.5,
   0.380952380952381,
   0.6153846153846153,
   0.4,
   0.5882352941176471,
   0.35714285714285715,
   0.3333333333333333,
   0.3636363636363636,
   0.5,
   0.4736842105263158,
   0.5185185185185185,
   0.5161290322580646,
   0.29629629629629634,
   0.3157894736842105,
   0.41666666666666663,
   0.6923076923076923,
   0.2962962962962963,
   0.3846153846153846,
   0.42857142857142855,
   0.26666666666666666,
   0.37499999999999994,
   0.823529411764706,
   0.7000000000000001,
   0.33333333333333326,
   0.36363636363636365,
   0.33333333333333326,
   0.7142857142857143,
   0.588235294117647,
   0.6666666666666665,
   0.823529411764706,
   0.33333333333333326,
   0.375,
   0.5217391304347827,
   0.4666666666666667,
   0.33333333333333326,
   0.2727272727272727,
   0.625,
   0.4444444444444445,
   0.4,
   0.43478260869565216,
   0.3636363636363636,
   0.4000000000000001,
   0.26666666666666666,
   0.5641025641025642,
   0.5333333333333333,
   0.5789473684210527,
   0.7272727272727272,
   0.75,
   0.4242424242424242,
   0.4666666666666666,
   0.6363636363636365,
   0.625,
   0.625,
   0.25,
   0.45161290322580644,
   0.36842105263157887,
   0.5,
   0.2608695652173913,
   0.26086956521739135,
   0.5,
   0.5,
   0.923076923076923,
   0.29629629629629634,
   0.5,
   0.5714285714285715,
   0.7878787878787877,
   0.37837837837837834,
   0.7142857142857143,
   0.5555555555555556,
   0.6666666666666665,
   0.6363636363636365,
   0.6666666666666665,
   0.3888888888888889,
   0.761904761904762,
   0.5714285714285713,
   0.5294117647058824,
   0.380952380952381,
   0.5333333333333333,
   0.45454545454545453,
   0.7000000000000001,
   0.5555555555555556,
   0.6153846153846154,
   0.3333333333333333,
   0.4827586206896552,
   0.6666666666666666,
   0.34782608695652173,
   0.4,
   0.4444444444444444,
   0.4444444444444444,
   0.33333333333333337,
   0.8571428571428571,
   0.7142857142857143,
   0.6666666666666666,
   0.5714285714285714,
   0.8571428571428571,
   0.41379310344827586,
   0.6222222222222223,
   0.6875,
   0.75,
   0.875,
   0.6,
   0.5454545454545454,
   0.28571428571428575,
   0.6470588235294118,
   0.75,
   0.37499999999999994,
   0.7272727272727273,
   0.4444444444444445,
   0.5714285714285715,
   0.7000000000000001,
   0.8333333333333334,
   0.7,
   0.4444444444444445,
   0.3243243243243243,
   0.3428571428571428,
   0.75,
   0.5,
   0.4545454545454546,
   0.28571428571428575,
   0.8421052631578948,
   0.6666666666666666,
   0.4210526315789474,
   0.38461538461538464,
   0.46153846153846156,
   0.6,
   0.631578947368421,
   0.43478260869565216,
   0.6666666666666666,
   0.8571428571428571,
   0.3157894736842105,
   0.38461538461538464,
   0.5714285714285713,
   0.7777777777777777,
   0.4166666666666667,
   0.7692307692307692,
   0.7142857142857143,
   0.5454545454545454,
   0.7999999999999999,
   0.8333333333333334,
   0.45454545454545453,
   0.7777777777777777,
   0.5,
   0.6190476190476191,
   0.6153846153846153,
   0.75,
   0.37499999999999994,
   0.3,
   0.888888888888889,
   0.5454545454545454,
   0.5,
   0.3333333333333333,
   0.28571428571428575,
   0.5,
   0.5833333333333334,
   0.5555555555555556,
   0.631578947368421,
   0.6666666666666666,
   0.4347826086956522,
   0.39999999999999997,
   0.48484848484848486,
   0.45161290322580644,
   0.4137931034482759,
   0.33333333333333337,
   0.125,
   0.588235294117647,
   0.6,
   0.631578947368421,
   0.3636363636363636,
   0.3225806451612903,
   0.3157894736842105,
   0.4166666666666667,
   0.2,
   0.4615384615384615,
   0.45161290322580644,
   0.4390243902439024,
   0.5128205128205129,
   0.6451612903225806,
   0.8749999999999999,
   0.4444444444444445,
   0.5116279069767442,
   0.8333333333333334,
   0.4827586206896552,
   0.576923076923077,
   0.6923076923076923,
   0.30769230769230765,
   0.8181818181818182,
   0.8235294117647058,
   0.6341463414634146,
   0.25,
   0.761904761904762,
   0.4,
   0.8749999999999999,
   0.8888888888888888,
   0.5294117647058824,
   0.4615384615384615,
   0.5,
   0.5,
   0.5128205128205129,
   0.7333333333333334,
   0.4782608695652174,
   0.8,
   0.5714285714285714,
   0.5,
   0.5365853658536586,
   0.8571428571428571,
   0.6086956521739131,
   0.5517241379310345,
   0.7333333333333334,
   0.4615384615384615,
   0.5555555555555556,
   0.380952380952381,
   0.742857142857143,
   0.4,
   0.6451612903225806,
   0.2962962962962963,
   0.48484848484848486,
   0.8387096774193549,
   0.7804878048780488,
   0.4,
   0.75,
   0.3333333333333333,
   0.6857142857142856,
   0.6666666666666667,
   0.5217391304347827,
   0.3333333333333333,
   0.4444444444444444,
   0.4545454545454545,
   0.5599999999999999,
   0.8888888888888888,
   0.2777777777777778,
   0.32432432432432434,
   0.6111111111111112,
   0.6666666666666666,
   0.33333333333333337,
   0.6666666666666666,
   0.3636363636363636,
   0.4799999999999999,
   0.9166666666666666,
   0.6875000000000001,
   0.8275862068965517,
   0.7272727272727273,
   0.5365853658536585,
   0.5641025641025641,
   0.35714285714285715,
   0.8823529411764706,
   0.45,
   0.8000000000000002,
   0.6875000000000001,
   0.5833333333333334,
   0.7142857142857143,
   0.7777777777777777,
   0.5599999999999999,
   0.5454545454545454,
   0.888888888888889,
   0.48000000000000004,
   0.6666666666666665,
   0.6875,
   0.5454545454545455,
   0.8333333333333334,
   0.7333333333333334,
   0.6111111111111112,
   0.6428571428571428,
   0.7368421052631579,
   0.5833333333333334,
   0.6363636363636364,
   0.5384615384615384,
   0.4848484848484849,
   0.16216216216216217,
   0.6363636363636364,
   0.15789473684210525,
   0.8000000000000002,
   0.7142857142857142,
   0.7727272727272727,
   0.8571428571428571,
   0.3636363636363636,
   0.6153846153846154,
   0.6923076923076923,
   0.5333333333333333,
   0.5714285714285714,
   0.4347826086956522,
   0.6666666666666667,
   0.39999999999999997,
   0.45161290322580644,
   0.7272727272727272,
   0.6874999999999999,
   0.6153846153846153,
   0.8888888888888888,
   0.7894736842105262,
   0.3703703703703704,
   0.8275862068965518,
   0.3333333333333333,
   0.8888888888888888,
   0.7878787878787877,
   0.8571428571428571,
   0.3,
   0.45614035087719296,
   0.08,
   0.5970149253731343,
   0.6984126984126984,
   0.4150943396226415,
   0.5679012345679012,
   0.64,
   0.4536082474226804,
   0.6181818181818183,
   0.4615384615384615,
   0.56,
   0.6301369863013699,
   0.6388888888888888,
   0.37837837837837834,
   0.49382716049382713,
   0.5588235294117647,
   0.5106382978723404,
   0.7058823529411765,
   0.5666666666666668,
   0.5454545454545455,
   0.5373134328358209,
   0.5588235294117647,
   0.5238095238095238,
   0.3692307692307692,
   0.6538461538461539,
   0.5416666666666666,
   0.4489795918367347,
   0.45,
   0.3829787234042554,
   0.3555555555555555,
   0.5641025641025642,
   0.47826086956521735,
   0.3928571428571428,
   0.5897435897435898,
   0.6067415730337078,
   0.5833333333333333,
   0.5454545454545454,
   0.6206896551724138,
   0.4594594594594595,
   0.5641025641025641,
   0.5853658536585366,
   0.39999999999999997,
   0.4727272727272727,
   0.7222222222222222,
   0.5714285714285713,
   0.5666666666666668,
   0.6666666666666667,
   0.27118644067796605,
   0.4776119402985075,
   0.5573770491803278,
   0.5106382978723405,
   0.6,
   0.7857142857142856,
   0.4814814814814815,
   0.4727272727272728,
   0.6785714285714286,
   0.5,
   0.5957446808510639,
   0.6885245901639344,
   0.547945205479452,
   0.5,
   0.5263157894736842,
   0.4444444444444445,
   0.5396825396825397,
   0.6111111111111113,
   0.3902439024390244,
   0.6538461538461539,
   0.5777777777777778,
   0.43750000000000006,
   0.5818181818181818,
   0.27027027027027023,
   0.5714285714285714,
   0.7384615384615385,
   0.5306122448979592,
   0.7659574468085107,
   0.5128205128205129,
   0.6756756756756757,
   0.5576923076923077,
   0.5416666666666667,
   0.6842105263157895,
   0.391304347826087,
   0.5915492957746479,
   0.5365853658536586,
   0.5757575757575757,
   0.5454545454545454,
   0.5079365079365079,
   0.5581395348837209,
   0.5866666666666667,
   0.375,
   0.41379310344827586,
   0.7333333333333333,
   0.47058823529411764,
   0.6987951807228915,
   0.3870967741935484,
   0.717948717948718,
   0.7169811320754718,
   0.3902439024390244,
   0.4869565217391304,
   0.6545454545454547,
   0.684931506849315,
   0.8000000000000002,
   0.49275362318840576,
   0.6341463414634146,
   0.35555555555555557,
   0.45901639344262296,
   0.47058823529411764,
   0.6086956521739131,
   0.6,
   0.41666666666666663,
   0.1818181818181818,
   0.45454545454545453,
   0.47058823529411764,
   0.4230769230769231,
   0.6206896551724138,
   0.48888888888888893,
   0.553191489361702,
   0.5714285714285714,
   0.7346938775510206,
   0.6071428571428571,
   0.5263157894736842,
   0.4225352112676056,
   0.5609756097560976,
   0.6129032258064516,
   0.5588235294117647,
   0.5882352941176471,
   0.2545454545454545,
   0.7246376811594203,
   0.5423728813559322,
   0.676056338028169,
   0.34615384615384615,
   0.3829787234042553,
   0.5846153846153846,
   0.5945945945945945,
   0.684931506849315,
   0.39473684210526316,
   0.5185185185185186,
   0.47058823529411764,
   0.7199999999999999,
   0.4000000000000001,
   0.4166666666666667,
   0.7142857142857142,
   0.6756756756756758,
   0.5185185185185186,
   0.6909090909090909,
   0.5757575757575758,
   0.5396825396825397,
   0.5333333333333332,
   0.6229508196721311,
   0.5245901639344263,
   0.5660377358490567,
   0.5714285714285715,
   0.6938775510204082,
   0.6355140186915889,
   0.6521739130434783,
   0.22641509433962265,
   0.6037735849056604,
   0.6274509803921569,
   0.41509433962264153,
   0.6736842105263158,
   0.5945945945945946,
   0.5066666666666667,
   0.7722772277227723,
   0.5762711864406779,
   0.5294117647058824,
   0.5294117647058824,
   0.5,
   0.5937499999999999,
   0.5853658536585366,
   0.6031746031746031,
   0.4864864864864865,
   0.5806451612903226,
   0.6666666666666666,
   0.5952380952380952,
   0.6521739130434783,
   0.5396825396825397,
   0.5490196078431373,
   0.6744186046511628,
   0.4727272727272728,
   0.5066666666666666,
   0.6842105263157895,
   0.7387387387387387,
   0.6666666666666666,
   0.5263157894736843,
   0.8214285714285714,
   0.5882352941176471,
   0.75,
   0.7073170731707318,
   0.5,
   0.5769230769230769,
   0.5106382978723404,
   0.375,
   0.6190476190476191,
   0.39285714285714285,
   0.6052631578947367,
   0.7037037037037038,
   0.6046511627906977,
   0.7037037037037037,
   0.37499999999999994,
   0.8292682926829269,
   0.7419354838709677,
   0.6461538461538462,
   0.34782608695652173,
   0.5365853658536586,
   0.5934065934065934,
   0.6774193548387097,
   0.47222222222222215,
   0.2790697674418604,
   0.4444444444444444,
   0.5675675675675677,
   0.5106382978723404,
   0.7741935483870969,
   0.6813186813186813,
   0.36111111111111105,
   0.48780487804878053,
   0.7042253521126761,
   0.4166666666666667,
   0.5833333333333334,
   0.5909090909090909,
   0.3673469387755102,
   0.24561403508771934,
   0.7241379310344827,
   0.6021505376344086,
   0.358974358974359,
   0.6060606060606061,
   0.4999999999999999,
   0.6,
   0.717948717948718,
   0.5,
   0.5675675675675677,
   0.6451612903225806,
   0.46017699115044247,
   0.5316455696202531,
   0.6268656716417911,
   0.44,
   0.5652173913043478,
   0.6666666666666667,
   0.5882352941176471,
   0.4186046511627907,
   0.3661971830985916,
   0.38095238095238093,
   0.7096774193548386,
   0.5217391304347826,
   0.4878048780487805,
   0.5573770491803278,
   0.6734693877551019,
   0.36,
   0.5789473684210527,
   0.6153846153846153,
   ...]],
 0.8: [1962,
  [0.75,
   0.64,
   0.8,
   0.64,
   0.76,
   0.72,
   0.8,
   0.76,
   0.76,
   0.7,
   0.76,
   0.76,
   0.8,
   0.75,
   0.8,
   0.75,
   0.6799999999999999,
   0.76,
   0.64,
   0.6182000000000001,
   0.8,
   0.6799999999999999,
   0.72,
   0.76,
   0.7647999999999999,
   0.8,
   0.72,
   0.65,
   0.75,
   0.6799999999999999,
   0.76,
   0.6799999999999999,
   0.76,
   0.6799999999999999,
   0.64,
   0.75,
   0.64,
   0.76,
   0.75,
   0.62,
   0.6799999999999999,
   0.72,
   0.76,
   0.8,
   0.64,
   0.76,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.72,
   0.8,
   0.8,
   0.76,
   0.64,
   0.64,
   0.76,
   0.64,
   0.64,
   0.8,
   0.6799999999999999,
   0.64,
   0.64,
   0.76,
   0.76,
   0.8,
   0.64,
   0.72,
   0.72,
   0.72,
   0.8,
   0.72,
   0.64,
   0.72,
   0.6799999999999999,
   0.8,
   0.8,
   0.8,
   0.8,
   0.6799999999999999,
   0.64,
   0.8,
   0.64,
   0.76,
   0.8,
   0.6799999999999999,
   0.76,
   0.64,
   0.72,
   0.64,
   0.64,
   0.6799999999999999,
   0.8,
   0.8,
   0.64,
   0.76,
   0.8,
   0.72,
   0.64,
   0.8,
   0.6799999999999999,
   0.76,
   0.72,
   0.76,
   0.8,
   0.6799999999999999,
   0.72,
   0.76,
   0.6799999999999999,
   0.64,
   0.64,
   0.8,
   0.6799999999999999,
   0.8,
   0.76,
   0.8,
   0.72,
   0.8,
   0.72,
   0.8,
   0.76,
   0.64,
   0.72,
   0.64,
   0.6799999999999999,
   0.6799999999999999,
   0.72,
   0.64,
   0.76,
   0.64,
   0.8,
   0.76,
   0.72,
   0.6799999999999999,
   0.64,
   0.8,
   0.64,
   0.76,
   0.6799999999999999,
   0.64,
   0.6799999999999999,
   0.64,
   0.76,
   0.64,
   0.76,
   0.6799999999999999,
   0.72,
   0.76,
   0.6799999999999999,
   0.76,
   0.76,
   0.64,
   0.8,
   0.72,
   0.8,
   0.64,
   0.64,
   0.72,
   0.6799999999999999,
   0.8,
   0.64,
   0.72,
   0.6799999999999999,
   0.8,
   0.72,
   0.64,
   0.72,
   0.75,
   0.8,
   0.75,
   0.64,
   0.8,
   0.64,
   0.64,
   0.76,
   0.76,
   0.64,
   0.76,
   0.76,
   0.75,
   0.64,
   0.6799999999999999,
   0.6666000000000001,
   0.7,
   0.76,
   0.8,
   0.7,
   0.8,
   0.65,
   0.65,
   0.65,
   0.64,
   0.65,
   0.75,
   0.64,
   0.7,
   0.75,
   0.7,
   0.65,
   0.76,
   0.6799999999999999,
   0.7,
   0.76,
   0.76,
   0.8,
   0.6799999999999999,
   0.65,
   0.7428,
   0.6666000000000001,
   0.6799999999999999,
   0.75,
   0.65,
   0.72,
   0.72,
   0.7,
   0.7,
   0.7384000000000001,
   0.8,
   0.7,
   0.64,
   0.65,
   0.7,
   0.64,
   0.65,
   0.75,
   0.65,
   0.6799999999999999,
   0.8,
   0.72,
   0.7,
   0.75,
   0.72,
   0.6799999999999999,
   0.65,
   0.72,
   0.65,
   0.72,
   0.8,
   0.8,
   0.72,
   0.75,
   0.76,
   0.65,
   0.6799999999999999,
   0.64,
   0.65,
   0.6666000000000001,
   0.72,
   0.76,
   0.7,
   0.64,
   0.8,
   0.6666000000000001,
   0.65,
   0.8,
   0.7,
   0.72,
   0.6799999999999999,
   0.7,
   0.7,
   0.6799999999999999,
   0.65,
   0.72,
   0.76,
   0.65,
   0.6834,
   0.72,
   0.72,
   0.64,
   0.8,
   0.6799999999999999,
   0.65,
   0.7333999999999999,
   0.7,
   0.65,
   0.72,
   0.76,
   0.6666000000000001,
   0.65,
   0.6182000000000001,
   0.64,
   0.8,
   0.64,
   0.76,
   0.76,
   0.76,
   0.72,
   0.76,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.64,
   0.64,
   0.72,
   0.76,
   0.72,
   0.64,
   0.6799999999999999,
   0.64,
   0.6799999999999999,
   0.76,
   0.8,
   0.64,
   0.64,
   0.76,
   0.6799999999999999,
   0.76,
   0.76,
   0.64,
   0.6799999999999999,
   0.8,
   0.8,
   0.76,
   0.6799999999999999,
   0.64,
   0.8,
   0.76,
   0.6799999999999999,
   0.76,
   0.64,
   0.72,
   0.64,
   0.76,
   0.76,
   0.76,
   0.64,
   0.76,
   0.8,
   0.6799999999999999,
   0.8,
   0.64,
   0.72,
   0.8,
   0.6799999999999999,
   0.8,
   0.8,
   0.76,
   0.76,
   0.7734,
   0.75,
   0.76,
   0.64,
   0.8,
   0.8,
   0.6799999999999999,
   0.75,
   0.8,
   0.72,
   0.76,
   0.64,
   0.64,
   0.75,
   0.64,
   0.7876000000000001,
   0.8,
   0.7,
   0.8,
   0.7666000000000001,
   0.76,
   0.8,
   0.72,
   0.72,
   0.72,
   0.8,
   0.64,
   0.8,
   0.76,
   0.6799999999999999,
   0.8,
   0.8,
   0.76,
   0.8,
   0.8,
   0.76,
   0.8,
   0.76,
   0.76,
   0.8,
   0.75,
   0.8,
   0.72,
   0.8,
   0.8,
   0.64,
   0.6799999999999999,
   0.72,
   0.8,
   0.72,
   0.7,
   0.753,
   0.76,
   0.72,
   0.7882,
   0.75,
   0.8,
   0.76,
   0.8,
   0.65,
   0.7,
   0.76,
   0.64,
   0.75,
   0.8,
   0.64,
   0.64,
   0.72,
   0.6222000000000001,
   0.75,
   0.7,
   0.6799999999999999,
   0.76,
   0.76,
   0.6799999999999999,
   0.65,
   0.64,
   0.72,
   0.64,
   0.7846,
   0.76,
   0.72,
   0.72,
   0.8,
   0.64,
   0.7,
   0.75,
   0.76,
   0.6799999999999999,
   0.76,
   0.76,
   0.64,
   0.7,
   0.6666000000000001,
   0.75,
   0.8,
   0.72,
   0.75,
   0.8,
   0.7,
   0.76,
   0.64,
   0.64,
   0.75,
   0.64,
   0.64,
   0.6799999999999999,
   0.64,
   0.7066,
   0.76,
   0.65,
   0.8,
   0.64,
   0.76,
   0.6799999999999999,
   0.8,
   0.65,
   0.8,
   0.65,
   0.65,
   0.76,
   0.6799999999999999,
   0.7,
   0.75,
   0.8,
   0.75,
   0.72,
   0.75,
   0.64,
   0.76,
   0.7,
   0.8,
   0.7,
   0.76,
   0.7333999999999999,
   0.8,
   0.8,
   0.8,
   0.65,
   0.8,
   0.8,
   0.65,
   0.8,
   0.64,
   0.7230000000000001,
   0.8,
   0.8,
   0.6666000000000001,
   0.7,
   0.7,
   0.64,
   0.65,
   0.7333999999999999,
   0.76,
   0.8,
   0.6799999999999999,
   0.76,
   0.64,
   0.8,
   0.64,
   0.6799999999999999,
   0.8,
   0.75,
   0.7,
   0.6799999999999999,
   0.72,
   0.75,
   0.65,
   0.8,
   0.6666000000000001,
   0.75,
   0.65,
   0.7,
   0.72,
   0.64,
   0.64,
   0.76,
   0.65,
   0.7,
   0.64,
   0.7,
   0.7,
   0.6799999999999999,
   0.72,
   0.72,
   0.8,
   0.6799999999999999,
   0.64,
   0.65,
   0.6666000000000001,
   0.6666000000000001,
   0.8,
   0.64,
   0.8,
   0.75,
   0.75,
   0.65,
   0.75,
   0.7,
   0.65,
   0.8,
   0.6799999999999999,
   0.6799999999999999,
   0.7857999999999999,
   0.7,
   0.7,
   0.8,
   0.65,
   0.72,
   0.75,
   0.64,
   0.8,
   0.8,
   0.76,
   0.65,
   0.7,
   0.75,
   0.6799999999999999,
   0.64,
   0.6666000000000001,
   0.6666000000000001,
   0.64,
   0.76,
   0.6799999999999999,
   0.6666000000000001,
   0.7,
   0.64,
   0.8,
   0.6799999999999999,
   0.76,
   0.6799999999999999,
   0.76,
   0.8,
   0.76,
   0.64,
   0.72,
   0.8,
   0.76,
   0.8,
   0.8,
   0.64,
   0.76,
   0.64,
   0.64,
   0.6799999999999999,
   0.72,
   0.72,
   0.64,
   0.8,
   0.6799999999999999,
   0.76,
   0.76,
   0.76,
   0.76,
   0.72,
   0.72,
   0.64,
   0.64,
   0.8,
   0.6799999999999999,
   0.8,
   0.8,
   0.76,
   0.75,
   0.72,
   0.72,
   0.64,
   0.8,
   0.8,
   0.6799999999999999,
   0.8,
   0.8,
   0.8,
   0.64,
   0.72,
   0.8,
   0.6799999999999999,
   0.7,
   0.76,
   0.6799999999999999,
   0.6799999999999999,
   0.72,
   0.8,
   0.76,
   0.64,
   0.8,
   0.8,
   0.76,
   0.64,
   0.8,
   0.8,
   0.6799999999999999,
   0.64,
   0.76,
   0.6799999999999999,
   0.8,
   0.64,
   0.64,
   0.64,
   0.76,
   0.6799999999999999,
   0.8,
   0.64,
   0.64,
   0.64,
   0.6799999999999999,
   0.72,
   0.8,
   0.8,
   0.64,
   0.76,
   0.64,
   0.6799999999999999,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.64,
   0.76,
   0.64,
   0.72,
   0.6799999999999999,
   0.8,
   0.64,
   0.8,
   0.76,
   0.8,
   0.8,
   0.76,
   0.8,
   0.6799999999999999,
   0.76,
   0.8,
   0.72,
   0.76,
   0.72,
   0.76,
   0.72,
   0.64,
   0.72,
   0.72,
   0.8,
   0.76,
   0.8,
   0.6799999999999999,
   0.76,
   0.8,
   0.64,
   0.64,
   0.64,
   0.76,
   0.72,
   0.72,
   0.8,
   0.6799999999999999,
   0.72,
   0.8,
   0.72,
   0.8,
   0.64,
   0.8,
   0.8,
   0.6799999999999999,
   0.64,
   0.76,
   0.72,
   0.76,
   0.72,
   0.8,
   0.64,
   0.6799999999999999,
   0.76,
   0.76,
   0.76,
   0.64,
   0.72,
   0.75,
   0.76,
   0.6799999999999999,
   0.8,
   0.64,
   0.8,
   0.6799999999999999,
   0.6799999999999999,
   0.76,
   0.64,
   0.76,
   0.6799999999999999,
   0.8,
   0.64,
   0.76,
   0.6799999999999999,
   0.6799999999999999,
   0.64,
   0.8,
   0.72,
   0.8,
   0.8,
   0.8,
   0.8,
   0.76,
   0.6799999999999999,
   0.72,
   0.6799999999999999,
   0.64,
   0.6799999999999999,
   0.76,
   0.6799999999999999,
   0.8,
   0.8,
   0.8,
   0.76,
   0.8,
   0.734,
   0.76,
   0.76,
   0.76,
   0.64,
   0.6799999999999999,
   0.64,
   0.72,
   0.64,
   0.8,
   0.8,
   0.8,
   0.6799999999999999,
   0.64,
   0.64,
   0.76,
   0.76,
   0.72,
   0.8,
   0.76,
   0.64,
   0.72,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.6799999999999999,
   0.64,
   0.76,
   0.6799999999999999,
   0.64,
   0.64,
   0.6799999999999999,
   0.8,
   0.6799999999999999,
   0.8,
   0.64,
   0.8,
   0.64,
   0.64,
   0.64,
   0.64,
   0.72,
   0.64,
   0.76,
   0.8,
   0.64,
   0.72,
   0.8,
   0.64,
   0.72,
   0.76,
   0.8,
   0.76,
   0.6799999999999999,
   0.6799999999999999,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.72,
   0.72,
   0.64,
   0.8,
   0.6799999999999999,
   0.6799999999999999,
   0.8,
   0.6799999999999999,
   0.8,
   0.6799999999999999,
   0.6799999999999999,
   0.8,
   0.72,
   0.76,
   0.6799999999999999,
   0.76,
   0.6799999999999999,
   0.64,
   0.64,
   0.6799999999999999,
   0.8,
   0.76,
   0.72,
   0.8,
   0.62,
   0.64,
   0.76,
   0.64,
   0.6799999999999999,
   0.76,
   0.8,
   0.6799999999999999,
   0.6799999999999999,
   0.72,
   0.64,
   0.76,
   0.8,
   0.72,
   0.72,
   0.6799999999999999,
   0.72,
   0.72,
   0.8,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.64,
   0.755555555555556,
   0.64,
   0.6799999999999999,
   0.76,
   0.64,
   0.72,
   0.8,
   0.8,
   0.72,
   0.8,
   0.76,
   0.6799999999999999,
   0.8,
   0.6799999999999999,
   0.76,
   0.72,
   0.8,
   0.64,
   0.76,
   0.76,
   0.6799999999999999,
   0.72,
   0.64,
   0.6799999999999999,
   0.64,
   0.62,
   0.72,
   0.72,
   0.8,
   0.8,
   0.755555555555556,
   0.72,
   0.76,
   0.72,
   0.8,
   0.8,
   0.8,
   0.76,
   0.8,
   0.72,
   0.8,
   0.6799999999999999,
   0.76,
   0.72,
   0.72,
   0.76,
   0.6799999999999999,
   0.64,
   0.6799999999999999,
   0.76,
   0.64,
   0.6799999999999999,
   0.8,
   0.6799999999999999,
   0.8,
   0.64,
   0.8,
   0.6799999999999999,
   0.76,
   0.8,
   0.64,
   0.8,
   0.76,
   0.76,
   0.8,
   0.76,
   0.6799999999999999,
   0.76,
   0.72,
   0.64,
   0.72,
   0.72,
   0.64,
   0.72,
   0.8,
   0.6799999999999999,
   0.72,
   0.8,
   0.7,
   0.6799999999999999,
   0.8,
   0.72,
   0.6799999999999999,
   0.72,
   0.6799999999999999,
   0.7692,
   0.64,
   0.76,
   0.64,
   0.8,
   0.6666000000000001,
   0.64,
   0.65,
   0.8,
   0.72,
   0.76,
   0.64,
   0.8,
   0.775,
   0.76,
   0.76,
   0.6799999999999999,
   0.6799999999999999,
   0.8,
   0.64,
   0.72,
   0.72,
   0.65,
   0.65,
   0.7,
   0.72,
   0.6666000000000001,
   0.8,
   0.7,
   0.6799999999999999,
   0.72,
   0.72,
   0.72,
   0.72,
   0.6799999999999999,
   0.6799999999999999,
   0.7,
   0.75,
   0.7,
   0.64,
   0.7066,
   0.6666000000000001,
   0.64,
   0.65,
   0.75,
   0.7857999999999999,
   0.6799999999999999,
   0.64,
   0.76,
   0.64,
   0.6666000000000001,
   0.8,
   0.64,
   0.64,
   0.65,
   0.7,
   0.6799999999999999,
   0.65,
   0.8,
   0.75,
   0.6666000000000001,
   ...],
  [0.6666666666666665,
   0.8333333333333334,
   0.6666666666666666,
   0.7142857142857143,
   0.875,
   0.7777777777777777,
   0.5555555555555556,
   0.5555555555555556,
   0.6666666666666666,
   0.7142857142857143,
   0.6666666666666666,
   0.6086956521739131,
   0.8333333333333334,
   0.64,
   0.4444444444444445,
   0.375,
   0.42857142857142855,
   0.5161290322580646,
   0.7142857142857143,
   0.625,
   0.47058823529411764,
   0.34782608695652173,
   0.8333333333333334,
   0.8333333333333334,
   0.888888888888889,
   0.8333333333333334,
   0.8333333333333334,
   0.7142857142857143,
   0.7777777777777777,
   0.5,
   0.7272727272727272,
   0.6,
   0.6666666666666667,
   0.7142857142857143,
   0.5263157894736842,
   0.888888888888889,
   0.4761904761904762,
   0.5,
   0.6,
   0.6153846153846153,
   0.380952380952381,
   0.5,
   0.36363636363636365,
   0.4,
   0.3125,
   0.64,
   0.75,
   0.15,
   0.6060606060606061,
   0.6666666666666665,
   0.5555555555555556,
   0.6250000000000001,
   0.7,
   0.7,
   0.5882352941176471,
   0.4545454545454546,
   0.39999999999999997,
   0.5714285714285714,
   0.7777777777777777,
   0.3448275862068966,
   0.625,
   0.6666666666666667,
   0.75,
   0.3,
   0.3157894736842105,
   0.4000000000000001,
   0.35294117647058826,
   0.4210526315789474,
   0.5714285714285715,
   0.5555555555555556,
   0.5333333333333333,
   0.23076923076923078,
   0.4000000000000001,
   0.6000000000000001,
   0.7142857142857142,
   0.8,
   0.30769230769230765,
   0.4444444444444445,
   0.5555555555555556,
   0.7000000000000001,
   0.6666666666666665,
   0.5454545454545454,
   0.5,
   0.6363636363636365,
   0.888888888888889,
   0.5714285714285715,
   0.44444444444444436,
   0.6,
   0.5,
   0.8,
   0.5833333333333334,
   0.6000000000000001,
   0.6363636363636364,
   0.5454545454545454,
   0.7142857142857143,
   0.6666666666666666,
   0.6428571428571429,
   0.8571428571428571,
   0.7499999999999999,
   0.4444444444444445,
   0.42857142857142855,
   0.3255813953488372,
   0.6666666666666667,
   0.6,
   0.5833333333333334,
   0.5714285714285715,
   0.8095238095238096,
   0.5,
   0.875,
   0.5,
   0.4,
   0.75,
   0.28571428571428575,
   0.8571428571428571,
   0.8571428571428571,
   0.4736842105263158,
   0.7,
   0.625,
   0.5882352941176471,
   0.9090909090909091,
   0.5,
   0.32653061224489793,
   0.375,
   0.23809523809523808,
   0.2631578947368421,
   0.28571428571428575,
   0.425531914893617,
   0.6530612244897959,
   0.2222222222222222,
   0.39999999999999997,
   0.28571428571428575,
   0.15789473684210525,
   0.16666666666666669,
   0.2580645161290323,
   0.3846153846153846,
   0.2222222222222222,
   0.32558139534883723,
   0.5,
   0.34285714285714286,
   0.2666666666666666,
   0.23255813953488372,
   0.3902439024390244,
   0.28571428571428575,
   0.5555555555555556,
   0.17543859649122806,
   0.2941176470588235,
   0.4666666666666667,
   0.30769230769230765,
   0.41025641025641024,
   0.40579710144927533,
   0.20408163265306123,
   0.3768115942028986,
   0.5945945945945946,
   0.4878048780487805,
   0.38461538461538464,
   0.5306122448979592,
   0.4210526315789474,
   0.11320754716981131,
   0.8823529411764706,
   0.3174603174603175,
   0.5789473684210527,
   0.2222222222222222,
   0.3333333333333333,
   0.3243243243243243,
   0.17777777777777778,
   0.5660377358490567,
   0.853658536585366,
   0.56,
   0.7012987012987012,
   0.2666666666666666,
   0.5714285714285714,
   0.45161290322580644,
   0.3870967741935483,
   0.6666666666666666,
   0.6329113924050633,
   0.4301075268817204,
   0.44067796610169496,
   0.717948717948718,
   0.5116279069767442,
   0.5714285714285714,
   0.634920634920635,
   0.7469879518072288,
   0.6451612903225806,
   0.6067415730337078,
   0.7857142857142857,
   0.6,
   0.746268656716418,
   0.6896551724137931,
   0.32727272727272727,
   0.5454545454545455,
   0.7457627118644068,
   0.6666666666666667,
   0.7666666666666666,
   0.4166666666666667,
   0.6585365853658536,
   0.5633802816901409,
   0.5625,
   0.6842105263157894,
   0.65625,
   0.7333333333333333,
   0.45161290322580644,
   0.48837209302325585,
   0.767123287671233,
   0.5977011494252873,
   0.5483870967741935,
   0.7297297297297297,
   0.6779661016949153,
   0.509090909090909,
   0.48275862068965514,
   0.5633802816901409,
   0.5263157894736842,
   0.8,
   0.48888888888888893,
   0.5128205128205129,
   0.5901639344262296,
   0.575,
   0.5757575757575757,
   0.6075949367088608,
   0.5977011494252874,
   0.6370370370370371,
   0.47887323943661964,
   0.5625,
   0.8260869565217391,
   0.711111111111111,
   0.48,
   0.759493670886076,
   0.46511627906976744,
   0.2553191489361702,
   0.4545454545454546,
   0.72,
   0.8282828282828283,
   0.5970149253731343,
   0.6666666666666666,
   0.7234042553191491,
   0.5365853658536585,
   0.7,
   0.72,
   0.490566037735849,
   0.7526881720430108,
   0.42857142857142855,
   0.6521739130434783,
   0.7466666666666666,
   0.7671232876712328,
   0.5818181818181818,
   0.6153846153846154,
   0.576923076923077,
   0.5666666666666667,
   0.5476190476190477,
   0.5423728813559322,
   0.5263157894736841,
   0.796116504854369,
   0.5084745762711865,
   0.7692307692307693,
   0.7659574468085106,
   0.6111111111111112,
   0.7241379310344828,
   0.4897959183673469,
   0.5176470588235293,
   0.5806451612903226,
   0.634920634920635,
   0.5434782608695652,
   0.547945205479452,
   0.6933333333333334,
   0.5483870967741935,
   0.5783132530120482,
   0.46428571428571425,
   0.7529411764705882,
   0.5373134328358209,
   0.4444444444444445,
   0.56,
   0.6250000000000001,
   0.5263157894736842,
   0.7547169811320756,
   0.735294117647059,
   0.6933333333333334,
   0.7441860465116279,
   0.7951807228915663,
   0.6415094339622641,
   0.5777777777777778,
   0.6181818181818182,
   0.4827586206896552,
   0.717948717948718,
   0.6206896551724137,
   0.7142857142857143,
   0.8,
   0.8125,
   0.6571428571428571,
   0.6363636363636364,
   0.43243243243243246,
   0.7692307692307692,
   0.5714285714285713,
   0.48000000000000004,
   0.4666666666666666,
   0.6976744186046512,
   0.6956521739130435,
   0.42857142857142855,
   0.6250000000000001,
   0.5714285714285715,
   0.7804878048780488,
   0.9259259259259259,
   0.9090909090909091,
   0.6086956521739131,
   0.65,
   0.7619047619047619,
   0.65,
   0.5294117647058824,
   0.6382978723404256,
   0.6666666666666667,
   0.6153846153846154,
   0.7272727272727272,
   0.6829268292682927,
   0.8333333333333333,
   0.4827586206896552,
   0.606060606060606,
   0.7142857142857143,
   0.5599999999999999,
   0.6829268292682926,
   0.625,
   0.5909090909090909,
   0.6153846153846153,
   0.5714285714285715,
   0.6315789473684211,
   0.5500000000000002,
   0.8461538461538461,
   0.6153846153846153,
   0.5000000000000001,
   0.5625,
   0.5454545454545454,
   0.3111111111111111,
   0.6885245901639345,
   0.8125000000000001,
   0.8372093023255814,
   0.588235294117647,
   0.6511627906976745,
   0.6842105263157895,
   0.8571428571428571,
   0.8695652173913044,
   0.8571428571428571,
   0.8333333333333334,
   0.7142857142857143,
   0.875,
   0.8571428571428571,
   1.0,
   0.6153846153846153,
   0.8333333333333334,
   0.8333333333333334,
   0.8571428571428571,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8571428571428571,
   0.28571428571428575,
   0.7142857142857143,
   0.7499999999999999,
   0.7777777777777777,
   0.625,
   0.8571428571428571,
   1.0,
   0.7499999999999999,
   0.5882352941176471,
   0.8333333333333334,
   0.6666666666666667,
   0.6666666666666666,
   0.625,
   0.6956521739130435,
   0.8333333333333334,
   0.75,
   0.888888888888889,
   0.6875000000000001,
   1.0,
   0.8333333333333333,
   0.7777777777777777,
   0.6666666666666666,
   0.7499999999999999,
   0.8421052631578948,
   0.8000000000000002,
   0.6923076923076924,
   0.8571428571428571,
   0.6,
   0.6666666666666666,
   0.7777777777777777,
   0.5714285714285715,
   0.8571428571428571,
   0.625,
   0.8571428571428571,
   0.46153846153846156,
   0.8,
   0.6666666666666666,
   0.5555555555555556,
   0.6666666666666666,
   0.8333333333333334,
   0.6666666666666665,
   0.5555555555555556,
   0.8000000000000002,
   0.8333333333333334,
   0.875,
   0.8333333333333334,
   0.5833333333333334,
   0.7142857142857143,
   0.8333333333333334,
   0.8571428571428571,
   0.42857142857142855,
   0.8571428571428571,
   0.5555555555555556,
   0.8571428571428571,
   0.6666666666666665,
   0.923076923076923,
   0.8571428571428571,
   0.7499999999999999,
   0.5882352941176471,
   0.7142857142857143,
   0.625,
   0.5,
   0.45454545454545453,
   0.7142857142857143,
   0.5833333333333334,
   0.8,
   0.588235294117647,
   0.6,
   0.6,
   0.5882352941176471,
   0.6666666666666667,
   0.8333333333333334,
   0.5,
   0.8,
   0.3809523809523809,
   0.375,
   0.6666666666666666,
   0.75,
   0.625,
   0.5882352941176471,
   0.6,
   0.7777777777777778,
   0.5,
   0.4705882352941177,
   0.5,
   0.8333333333333334,
   0.6666666666666666,
   0.5,
   0.5,
   0.5833333333333334,
   0.6,
   0.32,
   0.5714285714285715,
   0.5882352941176471,
   0.5555555555555556,
   0.5333333333333333,
   0.5714285714285715,
   0.8333333333333334,
   0.5,
   0.4444444444444444,
   0.375,
   0.6666666666666666,
   0.43478260869565216,
   0.26086956521739135,
   0.3809523809523809,
   0.35714285714285715,
   0.5333333333333333,
   0.6666666666666666,
   0.27586206896551724,
   0.5185185185185185,
   0.375,
   0.5714285714285715,
   0.8333333333333334,
   0.6666666666666666,
   0.5,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8750000000000001,
   0.6666666666666666,
   1.0,
   0.8333333333333334,
   0.7777777777777777,
   0.7777777777777778,
   0.6363636363636364,
   0.9,
   0.5882352941176471,
   0.8571428571428571,
   0.8571428571428571,
   0.8333333333333334,
   0.7777777777777777,
   0.8571428571428571,
   0.8571428571428571,
   0.8333333333333334,
   0.8,
   0.923076923076923,
   0.625,
   0.75,
   0.5,
   0.8333333333333334,
   0.6666666666666666,
   0.7142857142857143,
   0.631578947368421,
   0.8000000000000002,
   0.8181818181818182,
   0.6363636363636365,
   0.25,
   0.8333333333333334,
   0.7058823529411764,
   0.8333333333333334,
   0.8,
   0.888888888888889,
   0.8333333333333334,
   0.888888888888889,
   0.5714285714285715,
   0.6666666666666665,
   0.875,
   0.5714285714285715,
   0.8,
   0.380952380952381,
   0.6666666666666666,
   0.6470588235294117,
   0.7368421052631579,
   0.625,
   0.4210526315789474,
   0.5714285714285714,
   0.8,
   0.7142857142857143,
   0.6666666666666665,
   0.7142857142857143,
   0.8,
   0.7058823529411764,
   0.6666666666666666,
   0.4,
   0.6666666666666665,
   0.7142857142857143,
   0.7142857142857143,
   0.75,
   0.7,
   0.5333333333333333,
   0.6060606060606061,
   0.4166666666666667,
   0.42105263157894735,
   0.4000000000000001,
   0.5833333333333334,
   0.3157894736842105,
   0.5,
   0.6666666666666666,
   0.7058823529411765,
   0.7058823529411765,
   0.625,
   0.5263157894736842,
   0.5454545454545454,
   0.75,
   0.8571428571428571,
   0.8333333333333334,
   0.5,
   0.7142857142857143,
   0.3478260869565218,
   0.4210526315789474,
   0.6111111111111113,
   0.42857142857142855,
   0.45454545454545453,
   0.37499999999999994,
   0.5454545454545454,
   0.5555555555555556,
   0.5384615384615384,
   0.22222222222222224,
   0.4,
   0.7142857142857143,
   0.5555555555555556,
   0.4210526315789474,
   0.8181818181818182,
   0.625,
   0.8571428571428571,
   0.7,
   0.7777777777777777,
   0.3333333333333333,
   0.631578947368421,
   0.5806451612903225,
   0.6,
   0.7142857142857143,
   0.45454545454545453,
   0.6666666666666665,
   0.9090909090909091,
   0.5185185185185185,
   0.5,
   0.45454545454545453,
   0.35294117647058826,
   0.7333333333333333,
   0.5882352941176471,
   0.888888888888889,
   0.5384615384615384,
   0.8750000000000001,
   0.6153846153846153,
   0.6666666666666666,
   0.4705882352941177,
   0.5833333333333334,
   0.5714285714285715,
   0.3571428571428571,
   0.45161290322580644,
   0.7368421052631579,
   0.8333333333333334,
   0.7272727272727272,
   0.375,
   0.5,
   0.6666666666666666,
   0.7142857142857143,
   0.631578947368421,
   0.55,
   0.5,
   0.6666666666666667,
   0.2857142857142857,
   0.7999999999999999,
   0.7333333333333334,
   0.4166666666666667,
   0.5833333333333334,
   0.6666666666666667,
   0.2727272727272727,
   0.5,
   0.5714285714285713,
   0.42857142857142855,
   0.4666666666666666,
   0.4444444444444444,
   0.7000000000000001,
   0.888888888888889,
   0.9523809523809523,
   0.5454545454545455,
   0.5333333333333333,
   0.5714285714285715,
   0.888888888888889,
   0.7272727272727272,
   0.5882352941176471,
   0.8000000000000002,
   0.6000000000000001,
   0.4444444444444445,
   0.8571428571428571,
   0.4545454545454546,
   0.3333333333333333,
   0.3157894736842105,
   0.625,
   0.5,
   0.5555555555555556,
   0.3636363636363637,
   0.6666666666666666,
   0.6666666666666665,
   0.4444444444444445,
   0.45714285714285713,
   0.5,
   0.5833333333333334,
   0.5,
   0.27586206896551724,
   0.5384615384615384,
   0.631578947368421,
   0.5,
   0.625,
   0.888888888888889,
   0.6,
   0.4444444444444445,
   0.3846153846153846,
   0.7142857142857143,
   0.28571428571428575,
   0.8181818181818182,
   0.380952380952381,
   0.7272727272727272,
   0.3125,
   0.7142857142857143,
   0.6,
   0.5517241379310345,
   0.4444444444444445,
   0.7777777777777777,
   0.625,
   0.18181818181818182,
   0.6666666666666666,
   0.5384615384615384,
   0.2727272727272727,
   0.6666666666666666,
   0.4444444444444445,
   0.6923076923076924,
   0.6363636363636365,
   0.30303030303030304,
   0.5454545454545454,
   0.5454545454545454,
   0.6,
   0.4324324324324324,
   0.8333333333333334,
   0.19999999999999998,
   0.5,
   0.6666666666666665,
   0.3478260869565218,
   0.75,
   0.4444444444444444,
   0.9090909090909091,
   0.27272727272727276,
   0.5,
   0.625,
   0.888888888888889,
   0.7407407407407408,
   0.6,
   0.8181818181818182,
   0.8666666666666666,
   0.5714285714285715,
   0.6363636363636364,
   0.4444444444444445,
   0.6153846153846153,
   0.5925925925925927,
   0.43750000000000006,
   0.5,
   0.3333333333333333,
   0.3,
   0.8148148148148148,
   0.5,
   0.6363636363636365,
   0.14285714285714285,
   0.8181818181818182,
   0.48000000000000004,
   0.5833333333333334,
   0.6,
   0.5555555555555556,
   0.4,
   0.3529411764705882,
   0.9090909090909091,
   0.8,
   0.5384615384615384,
   0.5217391304347826,
   0.23999999999999996,
   0.30769230769230765,
   0.1818181818181818,
   0.8461538461538461,
   0.6111111111111112,
   0.7199999999999999,
   0.7058823529411765,
   0.7000000000000001,
   0.5,
   0.6153846153846153,
   0.7142857142857142,
   0.888888888888889,
   0.5,
   0.4,
   0.8461538461538461,
   0.5,
   0.7058823529411765,
   0.5833333333333334,
   0.5,
   0.64,
   0.3333333333333333,
   0.24242424242424246,
   0.47619047619047616,
   0.631578947368421,
   0.37837837837837834,
   0.7058823529411765,
   0.3333333333333333,
   0.5555555555555556,
   0.7999999999999999,
   0.6363636363636365,
   0.41379310344827586,
   0.5333333333333333,
   0.30769230769230765,
   0.6,
   0.6666666666666665,
   0.5161290322580646,
   0.5,
   0.6875,
   0.45454545454545453,
   0.761904761904762,
   0.42857142857142855,
   0.8181818181818182,
   0.5555555555555556,
   0.875,
   0.5263157894736842,
   0.5454545454545454,
   0.3448275862068966,
   0.6086956521739131,
   0.5714285714285714,
   0.64,
   0.5833333333333334,
   0.8,
   0.3846153846153846,
   0.6666666666666665,
   0.3157894736842105,
   0.7000000000000001,
   0.5,
   0.43749999999999994,
   0.8181818181818182,
   0.3636363636363636,
   0.7142857142857143,
   0.5957446808510638,
   0.38461538461538464,
   0.6,
   0.6666666666666665,
   0.875,
   0.8571428571428571,
   0.3703703703703704,
   0.7692307692307692,
   0.55,
   0.7142857142857143,
   0.7142857142857143,
   0.7857142857142857,
   0.8571428571428571,
   0.6666666666666666,
   0.4827586206896552,
   0.4666666666666667,
   0.35294117647058826,
   0.6923076923076923,
   0.41666666666666663,
   0.35714285714285715,
   0.5714285714285713,
   0.6,
   0.7058823529411765,
   0.588235294117647,
   0.3333333333333333,
   0.5,
   0.6451612903225806,
   0.625,
   0.6666666666666666,
   0.45454545454545453,
   0.35714285714285715,
   0.8,
   0.5,
   0.625,
   0.3333333333333333,
   0.8,
   0.5,
   0.6451612903225806,
   0.5000000000000001,
   0.5555555555555556,
   0.8275862068965518,
   0.35714285714285715,
   0.5384615384615385,
   0.5714285714285715,
   0.6451612903225806,
   0.5454545454545454,
   0.6363636363636365,
   0.8571428571428571,
   0.39999999999999997,
   0.5263157894736842,
   0.7755102040816326,
   0.606060606060606,
   0.3,
   0.7272727272727272,
   0.8333333333333334,
   0.4210526315789474,
   0.6101694915254238,
   0.9166666666666666,
   0.45161290322580644,
   1.0,
   0.8085106382978724,
   0.7058823529411765,
   0.6363636363636364,
   0.6666666666666666,
   0.7333333333333334,
   0.6428571428571429,
   0.7586206896551725,
   0.6206896551724137,
   0.4444444444444445,
   0.75,
   0.8387096774193549,
   0.7000000000000001,
   0.75,
   0.846153846153846,
   0.3125,
   0.26086956521739124,
   0.7142857142857143,
   0.6470588235294117,
   0.5,
   0.9090909090909091,
   0.36363636363636365,
   0.3529411764705882,
   0.5806451612903226,
   0.8421052631578948,
   0.7916666666666667,
   0.411764705882353,
   0.6666666666666666,
   0.4390243902439025,
   0.5517241379310344,
   0.4,
   0.7142857142857143,
   0.6666666666666667,
   0.5217391304347826,
   0.7804878048780488,
   0.5384615384615384,
   0.6666666666666667,
   0.611111111111111,
   0.9,
   0.8333333333333333,
   0.606060606060606,
   0.7857142857142857,
   0.8799999999999999,
   0.8484848484848484,
   0.7142857142857142,
   0.3125,
   0.75,
   0.7547169811320756,
   0.47058823529411764,
   0.43750000000000006,
   0.35714285714285715,
   0.6428571428571429,
   0.5517241379310345,
   0.5,
   0.16666666666666666,
   0.4999999999999999,
   0.5882352941176471,
   0.46153846153846156,
   0.7407407407407408,
   0.625,
   0.717948717948718,
   0.4102564102564102,
   0.6923076923076923,
   0.7199999999999999,
   0.4242424242424242,
   0.5,
   0.4102564102564102,
   0.9473684210526315,
   0.588235294117647,
   0.8,
   0.6285714285714287,
   0.3225806451612903,
   0.6153846153846153,
   0.8333333333333333,
   0.7272727272727273,
   0.7450980392156863,
   0.6938775510204082,
   0.4666666666666667,
   0.5,
   0.28571428571428564,
   0.7857142857142856,
   0.4102564102564102,
   0.8181818181818182,
   0.16666666666666666,
   0.75,
   0.3157894736842105,
   0.6666666666666666,
   0.8571428571428571,
   0.7777777777777777,
   0.5,
   0.46511627906976755,
   0.6557377049180327,
   0.43243243243243246,
   0.7901234567901234,
   0.4800000000000001,
   0.588235294117647,
   0.44000000000000006,
   0.4193548387096775,
   0.6756756756756757,
   0.7356321839080459,
   0.6956521739130435,
   0.73015873015873,
   0.7407407407407407,
   0.7419354838709677,
   0.6813186813186812,
   0.5,
   0.7368421052631579,
   0.52,
   0.372093023255814,
   0.6133333333333333,
   0.7816091954022988,
   0.5714285714285715,
   0.7252747252747254,
   0.689655172413793,
   0.5925925925925926,
   0.43243243243243246,
   0.3255813953488372,
   0.7045454545454546,
   0.5714285714285713,
   0.5853658536585366,
   0.6857142857142858,
   0.702127659574468,
   0.47058823529411764,
   0.7191011235955055,
   0.8888888888888888,
   0.7083333333333334,
   0.27450980392156865,
   0.8253968253968254,
   0.7142857142857143,
   0.8055555555555556,
   0.6966292134831461,
   0.8615384615384616,
   0.6575342465753423,
   0.8285714285714286,
   0.9705882352941176,
   0.43750000000000006,
   0.5555555555555556,
   0.6229508196721313,
   0.6666666666666666,
   0.7397260273972601,
   0.7878787878787878,
   0.6301369863013699,
   0.6415094339622641,
   0.8831168831168831,
   0.4827586206896552,
   0.6976744186046512,
   0.6666666666666666,
   0.4444444444444445,
   0.7547169811320755,
   0.5454545454545454,
   0.47619047619047616,
   0.7123287671232875,
   0.5106382978723405,
   0.4186046511627907,
   0.6493506493506493,
   0.5945945945945946,
   0.7123287671232877,
   0.4788732394366197,
   0.7945205479452054,
   0.8378378378378379,
   0.5660377358490566,
   ...]],
 0.4: [1122,
  [0.3166,
   0.3428,
   0.3834,
   0.27999999999999997,
   0.32,
   0.27999999999999997,
   0.24,
   0.23079999999999998,
   0.32,
   0.2666,
   0.4,
   0.24,
   0.36,
   0.32,
   0.25,
   0.25,
   0.27999999999999997,
   0.26,
   0.24,
   0.24,
   0.36,
   0.27999999999999997,
   0.4,
   0.36,
   0.24,
   0.3066,
   0.27999999999999997,
   0.36,
   0.24,
   0.25,
   0.27999999999999997,
   0.4,
   0.2666,
   0.27999999999999997,
   0.4,
   0.4,
   0.27999999999999997,
   0.24,
   0.24,
   0.27999999999999997,
   0.36,
   0.36,
   0.32,
   0.4,
   0.36,
   0.24,
   0.27999999999999997,
   0.4,
   0.24,
   0.36,
   0.27999999999999997,
   0.24,
   0.36,
   0.27999999999999997,
   0.24,
   0.36,
   0.32,
   0.32,
   0.27999999999999997,
   0.32,
   0.4,
   0.27999999999999997,
   0.24,
   0.4,
   0.4,
   0.36,
   0.27999999999999997,
   0.36,
   0.36,
   0.27999999999999997,
   0.36,
   0.32,
   0.36,
   0.24,
   0.4,
   0.24,
   0.27999999999999997,
   0.32,
   0.32,
   0.32,
   0.4,
   0.4,
   0.4,
   0.27999999999999997,
   0.24,
   0.32,
   0.32,
   0.32,
   0.27999999999999997,
   0.32,
   0.4,
   0.27999999999999997,
   0.32,
   0.32,
   0.24,
   0.32,
   0.4,
   0.27999999999999997,
   0.4,
   0.4,
   0.32,
   0.36,
   0.32,
   0.27999999999999997,
   0.32,
   0.32,
   0.36,
   0.36,
   0.27999999999999997,
   0.4,
   0.27999999999999997,
   0.27999999999999997,
   0.36,
   0.32,
   0.36,
   0.27999999999999997,
   0.36,
   0.4,
   0.32,
   0.3,
   0.36,
   0.32,
   0.4,
   0.32,
   0.4,
   0.4,
   0.32,
   0.24,
   0.4,
   0.4,
   0.4,
   0.32,
   0.27999999999999997,
   0.24,
   0.36,
   0.32,
   0.32,
   0.27999999999999997,
   0.27999999999999997,
   0.4,
   0.36,
   0.32,
   0.27999999999999997,
   0.4,
   0.36,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.36,
   0.4,
   0.36,
   0.27999999999999997,
   0.32,
   0.36,
   0.27999999999999997,
   0.32,
   0.32,
   0.27999999999999997,
   0.4,
   0.36,
   0.36,
   0.24,
   0.36,
   0.32,
   0.24,
   0.32,
   0.4,
   0.36,
   0.32,
   0.33399999999999996,
   0.36,
   0.36,
   0.27999999999999997,
   0.36,
   0.24,
   0.24,
   0.36,
   0.36,
   0.32,
   0.4,
   0.4,
   0.36,
   0.32,
   0.32,
   0.36,
   0.27999999999999997,
   0.24,
   0.24,
   0.36,
   0.24,
   0.27999999999999997,
   0.4,
   0.35,
   0.35,
   0.35,
   0.35,
   0.2666,
   0.33340000000000003,
   0.35,
   0.4,
   0.35,
   0.4,
   0.3,
   0.35,
   0.4,
   0.4,
   0.4,
   0.32,
   0.35,
   0.36,
   0.36,
   0.24,
   0.27999999999999997,
   0.32,
   0.27999999999999997,
   0.36,
   0.32,
   0.32,
   0.24,
   0.36,
   0.24,
   0.32,
   0.4,
   0.36,
   0.32,
   0.36,
   0.36,
   0.4,
   0.32,
   0.27999999999999997,
   0.24,
   0.36,
   0.24,
   0.36,
   0.36,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.24,
   0.32,
   0.24,
   0.27999999999999997,
   0.32,
   0.4,
   0.36,
   0.4,
   0.36,
   0.36,
   0.32,
   0.24,
   0.27999999999999997,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.4,
   0.32,
   0.33340000000000003,
   0.32,
   0.35,
   0.31120000000000003,
   0.32,
   0.27999999999999997,
   0.27999999999999997,
   0.4,
   0.32,
   0.4,
   0.4,
   0.32,
   0.4,
   0.32,
   0.4,
   0.3286,
   0.35,
   0.4,
   0.4,
   0.32,
   0.32,
   0.35,
   0.27999999999999997,
   0.24,
   0.32,
   0.24,
   0.32,
   0.24,
   0.4,
   0.3,
   0.24,
   0.27999999999999997,
   0.2572,
   0.4,
   0.36,
   0.27999999999999997,
   0.3,
   0.3,
   0.35,
   0.36,
   0.25,
   0.35,
   0.25,
   0.27999999999999997,
   0.32,
   0.3,
   0.35,
   0.4,
   0.24,
   0.35,
   0.3,
   0.27999999999999997,
   0.4,
   0.4,
   0.27999999999999997,
   0.25,
   0.36,
   0.24,
   0.25,
   0.24,
   0.25,
   0.4,
   0.3166,
   0.3556,
   0.4,
   0.4,
   0.4,
   0.33999999999999997,
   0.4,
   0.4,
   0.36,
   0.31120000000000003,
   0.32,
   0.27999999999999997,
   0.32,
   0.36,
   0.32,
   0.4,
   0.4,
   0.25,
   0.2666,
   0.27999999999999997,
   0.2666,
   0.24,
   0.24,
   0.25,
   0.4,
   0.3,
   0.32,
   0.4,
   0.27999999999999997,
   0.27999999999999997,
   0.4,
   0.32,
   0.3,
   0.36,
   0.32,
   0.4,
   0.4,
   0.36,
   0.4,
   0.24,
   0.24,
   0.36,
   0.35,
   0.27999999999999997,
   0.27999999999999997,
   0.25,
   0.3,
   0.33340000000000003,
   0.36,
   0.24,
   0.24,
   0.32,
   0.36,
   0.4,
   0.36,
   0.27999999999999997,
   0.36,
   0.27999999999999997,
   0.4,
   0.33340000000000003,
   0.24,
   0.4,
   0.4,
   0.4,
   0.32,
   0.24,
   0.35,
   0.4,
   0.4,
   0.25,
   0.35,
   0.35,
   0.36,
   0.32,
   0.4,
   0.35,
   0.4,
   0.24,
   0.27999999999999997,
   0.3,
   0.3,
   0.24,
   0.27999999999999997,
   0.24,
   0.32,
   0.27999999999999997,
   0.36,
   0.36,
   0.4,
   0.36,
   0.4,
   0.32,
   0.24,
   0.24,
   0.27999999999999997,
   0.36,
   0.4,
   0.27999999999999997,
   0.32,
   0.27999999999999997,
   0.32,
   0.27999999999999997,
   0.32,
   0.36,
   0.27999999999999997,
   0.36,
   0.32,
   0.4,
   0.27999999999999997,
   0.32,
   0.4,
   0.24,
   0.27999999999999997,
   0.4,
   0.24,
   0.24,
   0.32,
   0.32,
   0.4,
   0.36,
   0.36,
   0.32,
   0.36,
   0.36,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.32,
   0.36,
   0.36,
   0.4,
   0.4,
   0.24,
   0.36,
   0.32,
   0.27999999999999997,
   0.24,
   0.24,
   0.27999999999999997,
   0.32,
   0.36,
   0.4,
   0.4,
   0.4,
   0.4,
   0.24,
   0.32,
   0.32,
   0.32,
   0.4,
   0.4,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.36,
   0.4,
   0.4,
   0.36,
   0.24,
   0.27999999999999997,
   0.36,
   0.36,
   0.27999999999999997,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.24,
   0.27999999999999997,
   0.24,
   0.4,
   0.4,
   0.24,
   0.24,
   0.32,
   0.36,
   0.36,
   0.32,
   0.36,
   0.27999999999999997,
   0.32,
   0.36,
   0.27999999999999997,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.32,
   0.24,
   0.4,
   0.36,
   0.24,
   0.36,
   0.27999999999999997,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.24,
   0.4,
   0.4,
   0.32,
   0.4,
   0.27999999999999997,
   0.24,
   0.4,
   0.24,
   0.27999999999999997,
   0.4,
   0.22000000000000003,
   0.24,
   0.36,
   0.32,
   0.24,
   0.32,
   0.36,
   0.4,
   0.27999999999999997,
   0.4,
   0.36,
   0.4,
   0.4,
   0.27999999999999997,
   0.4,
   0.36,
   0.24,
   0.24,
   0.32,
   0.32,
   0.27999999999999997,
   0.27999999999999997,
   0.4,
   0.32,
   0.4,
   0.4,
   0.27999999999999997,
   0.32,
   0.35,
   0.36,
   0.27999999999999997,
   0.24,
   0.35,
   0.24,
   0.36,
   0.24,
   0.22000000000000003,
   0.4,
   0.32,
   0.27999999999999997,
   0.30666666666666603,
   0.32,
   0.32,
   0.32,
   0.32,
   0.36,
   0.32,
   0.32,
   0.36,
   0.36,
   0.24,
   0.4,
   0.27999999999999997,
   0.4,
   0.32,
   0.32,
   0.36,
   0.36,
   0.36,
   0.24,
   0.27999999999999997,
   0.24,
   0.27999999999999997,
   0.32,
   0.32,
   0.4,
   0.24,
   0.32,
   0.4,
   0.36,
   0.36,
   0.24,
   0.32,
   0.24,
   0.4,
   0.30666666666666603,
   0.27999999999999997,
   0.32,
   0.24,
   0.32,
   0.24,
   0.32,
   0.30666666666666603,
   0.24,
   0.32,
   0.32,
   0.36,
   0.24,
   0.27999999999999997,
   0.36,
   0.24,
   0.27999999999999997,
   0.32,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.4,
   0.24,
   0.4,
   0.2666,
   0.4,
   0.35,
   0.4,
   0.32,
   0.24,
   0.36,
   0.3,
   0.3,
   0.36,
   0.36920000000000003,
   0.2666,
   0.35,
   0.4,
   0.3,
   0.3,
   0.3,
   0.4,
   0.3,
   0.36,
   0.4,
   0.4,
   0.32,
   0.35,
   0.27999999999999997,
   0.36,
   0.25,
   0.36,
   0.4,
   0.3,
   0.3,
   0.4,
   0.4,
   0.32,
   0.24,
   0.36,
   0.3,
   0.4,
   0.25,
   0.3466,
   0.36,
   0.32,
   0.35,
   0.25,
   0.4,
   0.4,
   0.4,
   0.27999999999999997,
   0.36,
   0.4,
   0.4,
   0.35,
   0.27999999999999997,
   0.4,
   0.4,
   0.32,
   0.4,
   0.27999999999999997,
   0.35,
   0.4,
   0.32,
   0.2546,
   0.4,
   0.4,
   0.27999999999999997,
   0.36,
   0.27999999999999997,
   0.35,
   0.36,
   0.4,
   0.24,
   0.27999999999999997,
   0.35,
   0.33340000000000003,
   0.4,
   0.36,
   0.32,
   0.4,
   0.36,
   0.25,
   0.4,
   0.2666,
   0.3,
   0.35,
   0.25,
   0.24,
   0.4,
   0.4,
   0.27999999999999997,
   0.32,
   0.2666,
   0.3,
   0.3,
   0.36,
   0.4,
   0.27999999999999997,
   0.4,
   0.4,
   0.4,
   0.36,
   0.32,
   0.36,
   0.36,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.4,
   0.24,
   0.36,
   0.36,
   0.36,
   0.27999999999999997,
   0.36,
   0.4,
   0.36,
   0.27999999999999997,
   0.36,
   0.27999999999999997,
   0.24,
   0.36,
   0.4,
   0.32,
   0.24,
   0.36,
   0.32,
   0.24,
   0.36,
   0.24,
   0.24,
   0.32,
   0.27999999999999997,
   0.24,
   0.4,
   0.4,
   0.36,
   0.36,
   0.24,
   0.27999999999999997,
   0.4,
   0.36,
   0.4,
   0.36,
   0.4,
   0.4,
   0.27999999999999997,
   0.36,
   0.32,
   0.27999999999999997,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.32,
   0.24,
   0.36,
   0.32,
   0.32,
   0.32,
   0.27999999999999997,
   0.4,
   0.32,
   0.4,
   0.32,
   0.32,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.36,
   0.32,
   0.24,
   0.27999999999999997,
   0.4,
   0.4,
   0.36,
   0.36,
   0.36,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.32,
   0.36,
   0.32,
   0.3,
   0.27999999999999997,
   0.32,
   0.32,
   0.27999999999999997,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.36,
   0.36,
   0.27999999999999997,
   0.24,
   0.32,
   0.24,
   0.4,
   0.4,
   0.27999999999999997,
   0.36,
   0.27999999999999997,
   0.36,
   0.24,
   0.36,
   0.36,
   0.32,
   0.36,
   0.4,
   0.24,
   0.27999999999999997,
   0.24,
   0.36,
   0.32,
   0.24,
   0.32,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.32,
   0.32,
   0.27999999999999997,
   0.24,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.36,
   0.32,
   0.27999999999999997,
   0.24,
   0.36,
   0.27999999999999997,
   0.4,
   0.24,
   0.36,
   0.24,
   0.32,
   0.4,
   0.27999999999999997,
   0.4,
   0.27999999999999997,
   0.4,
   0.24,
   0.27999999999999997,
   0.32,
   0.3,
   0.4,
   0.32,
   0.4,
   0.36,
   0.3,
   0.24,
   0.27999999999999997,
   0.32,
   0.27999999999999997,
   0.32,
   0.24,
   0.4,
   0.27999999999999997,
   0.24,
   0.32,
   0.27999999999999997,
   0.4,
   0.4,
   0.36,
   0.36,
   0.4,
   0.36,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.27999999999999997,
   0.4,
   0.36,
   0.36,
   0.24,
   0.4,
   0.24,
   0.36,
   0.27999999999999997,
   0.4,
   0.24,
   0.36,
   0.32,
   0.24,
   0.27999999999999997,
   0.36,
   0.4,
   0.32,
   0.27999999999999997,
   0.4,
   0.27999999999999997,
   0.4,
   0.36,
   0.36,
   0.27999999999999997,
   0.24,
   0.4,
   0.32,
   0.4,
   0.27999999999999997,
   0.27999999999999997,
   0.32,
   0.4,
   0.32,
   0.24,
   0.24,
   0.4,
   0.36,
   0.32,
   0.24,
   0.24,
   0.36,
   0.36,
   0.36,
   0.36,
   0.32,
   0.36,
   0.27999999999999997,
   0.32,
   0.24,
   0.24,
   0.36,
   0.36,
   0.24,
   0.27999999999999997,
   0.24,
   0.24,
   0.32,
   0.4,
   0.27999999999999997,
   0.36,
   0.27999999999999997,
   0.36,
   0.36,
   0.35,
   0.4,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   0.27999999999999997,
   0.32,
   0.36,
   0.27999999999999997,
   0.36,
   0.36,
   0.4,
   0.4,
   0.27999999999999997,
   0.24,
   0.24,
   0.24,
   0.24,
   0.27999999999999997,
   0.24,
   0.24,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.4,
   0.27999999999999997,
   0.36,
   0.4,
   0.32,
   0.4,
   0.27999999999999997,
   0.36,
   0.24,
   0.27999999999999997,
   0.27999999999999997,
   0.24,
   ...],
  [0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.6,
   0.8333333333333334,
   0.7142857142857143,
   0.5,
   0.6666666666666666,
   0.5,
   0.3333333333333333,
   0.4,
   0.4444444444444444,
   0.6666666666666666,
   0.75,
   0.75,
   0.6666666666666666,
   0.6666666666666665,
   0.75,
   0.75,
   0.8333333333333334,
   0.6666666666666666,
   0.42857142857142855,
   0.7142857142857143,
   0.5714285714285715,
   0.6666666666666666,
   0.7142857142857143,
   0.5,
   0.5,
   0.3529411764705882,
   0.33333333333333326,
   0.6666666666666667,
   0.4,
   0.5555555555555556,
   0.28571428571428575,
   0.3,
   0.6,
   0.625,
   0.5,
   0.5454545454545454,
   0.4444444444444445,
   0.26666666666666666,
   0.45454545454545453,
   0.2631578947368421,
   0.39999999999999997,
   0.33333333333333326,
   0.3333333333333333,
   0.4444444444444445,
   0.29787234042553196,
   0.75,
   0.3157894736842105,
   0.3157894736842105,
   0.4848484848484849,
   0.25,
   0.45454545454545453,
   0.7142857142857143,
   0.6250000000000001,
   0.6,
   0.38888888888888884,
   0.5714285714285713,
   0.6666666666666667,
   0.14285714285714285,
   0.3636363636363636,
   0.5833333333333334,
   0.5,
   0.25,
   0.4,
   0.7692307692307692,
   0.31578947368421056,
   0.4,
   0.42857142857142855,
   0.6,
   0.625,
   0.4150943396226415,
   0.4,
   0.46153846153846156,
   0.380952380952381,
   0.875,
   0.5833333333333334,
   0.358974358974359,
   0.42105263157894735,
   0.4444444444444444,
   0.3846153846153846,
   0.34285714285714286,
   0.4444444444444445,
   0.4,
   0.21621621621621623,
   0.5,
   0.32,
   0.1875,
   0.47058823529411764,
   0.4081632653061225,
   0.75,
   0.25,
   0.2105263157894737,
   0.2105263157894737,
   0.2857142857142857,
   0.24999999999999994,
   0.23255813953488372,
   0.17777777777777778,
   0.2692307692307692,
   0.15,
   0.2711864406779661,
   0.20833333333333334,
   0.2105263157894737,
   0.3913043478260869,
   0.35294117647058826,
   0.26666666666666666,
   0.19607843137254902,
   0.21739130434782608,
   0.057142857142857134,
   0.208955223880597,
   0.3529411764705882,
   0.18181818181818182,
   0.07017543859649122,
   0.17857142857142855,
   0.18867924528301888,
   0.24137931034482757,
   0.1923076923076923,
   0.32,
   0.30769230769230765,
   0.2,
   0.1818181818181818,
   0.19230769230769232,
   0.25641025641025644,
   0.16666666666666666,
   0.16216216216216214,
   0.14634146341463414,
   0.4545454545454545,
   0.411764705882353,
   0.33333333333333326,
   0.1791044776119403,
   0.35294117647058826,
   0.3050847457627119,
   0.23809523809523808,
   0.40816326530612246,
   0.3125,
   0.27586206896551724,
   0.339622641509434,
   0.21818181818181817,
   0.22857142857142854,
   0.30188679245283023,
   0.21621621621621623,
   0.2857142857142857,
   0.25,
   0.2790697674418605,
   0.2413793103448276,
   0.1587301587301587,
   0.4,
   0.17857142857142858,
   0.3703703703703704,
   0.31818181818181823,
   0.27272727272727276,
   0.3243243243243243,
   0.15384615384615385,
   0.18181818181818185,
   0.17391304347826086,
   0.1724137931034483,
   0.25,
   0.2580645161290323,
   0.15,
   0.34615384615384615,
   0.21052631578947367,
   0.1917808219178082,
   0.23333333333333334,
   0.27450980392156865,
   0.30188679245283023,
   0.2702702702702703,
   0.14285714285714285,
   0.14285714285714282,
   0.4067796610169492,
   0.25,
   0.3793103448275862,
   0.22727272727272727,
   0.375,
   0.2857142857142857,
   0.15999999999999998,
   0.16666666666666666,
   0.20833333333333331,
   0.4827586206896552,
   0.34782608695652173,
   0.26666666666666666,
   0.14545454545454545,
   0.11428571428571428,
   0.22222222222222224,
   0.27450980392156865,
   0.19999999999999998,
   0.21276595744680848,
   0.2222222222222222,
   0.1818181818181818,
   0.1724137931034483,
   0.7241379310344828,
   0.5842696629213484,
   0.42424242424242425,
   0.5217391304347826,
   0.48484848484848486,
   0.761904761904762,
   0.5283018867924528,
   0.4137931034482759,
   0.6153846153846153,
   0.5866666666666667,
   0.4489795918367347,
   0.41025641025641024,
   0.23333333333333336,
   0.49056603773584906,
   0.5454545454545455,
   0.34782608695652173,
   0.29787234042553196,
   0.47457627118644063,
   0.5853658536585366,
   0.49122807017543857,
   0.56,
   0.4,
   0.6666666666666667,
   0.6,
   0.3333333333333333,
   0.5625,
   0.7234042553191491,
   0.4848484848484848,
   0.46808510638297873,
   0.31746031746031744,
   0.5263157894736842,
   0.625,
   0.5945945945945945,
   0.6363636363636364,
   0.28571428571428575,
   0.5333333333333333,
   0.7857142857142856,
   0.5853658536585366,
   0.8000000000000002,
   0.8181818181818182,
   0.4680851063829787,
   0.3125,
   0.43999999999999995,
   0.8461538461538461,
   0.8571428571428571,
   0.5581395348837209,
   0.46153846153846156,
   0.5625000000000001,
   0.41025641025641024,
   0.48484848484848486,
   0.3870967741935484,
   0.7272727272727272,
   0.5217391304347826,
   0.46511627906976744,
   0.9,
   0.5,
   0.4666666666666667,
   0.6545454545454545,
   0.3548387096774193,
   0.5263157894736842,
   0.4864864864864864,
   0.3333333333333333,
   0.6666666666666667,
   0.8888888888888888,
   0.6363636363636364,
   0.5925925925925926,
   0.4666666666666667,
   0.8333333333333334,
   0.7142857142857143,
   0.42857142857142855,
   0.7142857142857143,
   0.8333333333333334,
   0.5333333333333333,
   0.8333333333333334,
   0.8333333333333334,
   0.3333333333333333,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.6666666666666666,
   0.6666666666666666,
   0.875,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.4705882352941177,
   0.6666666666666666,
   0.6666666666666666,
   0.7142857142857143,
   0.6666666666666666,
   0.6666666666666665,
   0.7,
   0.5454545454545454,
   0.6666666666666666,
   0.6666666666666666,
   0.6,
   0.5,
   0.5,
   0.375,
   0.5,
   0.5,
   0.4444444444444445,
   0.5714285714285714,
   0.8333333333333334,
   0.5714285714285715,
   0.5714285714285715,
   0.6666666666666666,
   0.4615384615384615,
   0.3529411764705882,
   0.75,
   0.46153846153846156,
   0.5,
   0.43749999999999994,
   0.46153846153846156,
   0.45454545454545453,
   0.5714285714285715,
   0.3225806451612903,
   0.25,
   0.37499999999999994,
   0.4444444444444444,
   0.5,
   0.21052631578947367,
   0.375,
   0.42857142857142855,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.7142857142857143,
   0.6666666666666666,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.75,
   0.75,
   0.6666666666666666,
   0.7692307692307692,
   0.8333333333333334,
   0.8571428571428572,
   0.75,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.7142857142857143,
   0.8571428571428571,
   0.37499999999999994,
   0.75,
   0.8000000000000002,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.75,
   0.8333333333333334,
   0.8333333333333334,
   0.75,
   0.5714285714285715,
   0.8333333333333334,
   0.8333333333333334,
   0.6666666666666666,
   0.6666666666666666,
   0.6666666666666666,
   0.7058823529411765,
   0.625,
   0.6153846153846153,
   0.6666666666666666,
   0.5,
   0.3333333333333333,
   0.5714285714285715,
   0.6666666666666666,
   0.7142857142857143,
   0.5714285714285715,
   0.8333333333333334,
   0.7142857142857143,
   0.6666666666666666,
   0.6666666666666666,
   0.6153846153846153,
   0.6666666666666666,
   0.4,
   0.6956521739130435,
   0.6,
   0.28571428571428575,
   0.6,
   0.6666666666666666,
   0.5714285714285715,
   0.37499999999999994,
   0.5714285714285715,
   0.5714285714285715,
   0.2857142857142857,
   0.5714285714285715,
   0.3529411764705882,
   0.5714285714285715,
   0.7,
   0.36363636363636365,
   0.5,
   0.5454545454545454,
   0.42857142857142855,
   0.5714285714285715,
   0.17142857142857143,
   0.4,
   0.6666666666666665,
   0.30769230769230765,
   0.4210526315789474,
   0.11111111111111112,
   0.5714285714285715,
   0.23529411764705882,
   0.75,
   0.4166666666666667,
   0.75,
   0.3157894736842105,
   0.4444444444444444,
   0.3,
   0.33333333333333326,
   0.5,
   0.3125,
   0.25,
   0.6153846153846153,
   0.8333333333333334,
   0.26666666666666666,
   0.4615384615384615,
   0.25,
   0.6153846153846153,
   0.3870967741935484,
   0.625,
   0.5,
   0.4,
   0.31999999999999995,
   0.5454545454545454,
   0.18181818181818182,
   0.6666666666666667,
   0.7777777777777777,
   0.5333333333333333,
   0.5454545454545454,
   0.46153846153846156,
   0.5833333333333334,
   0.5,
   0.4166666666666667,
   0.45454545454545453,
   0.4999999999999999,
   0.22222222222222224,
   0.5,
   0.28571428571428575,
   0.28571428571428575,
   0.75,
   0.38461538461538464,
   0.28571428571428575,
   0.6250000000000001,
   0.3,
   0.45454545454545453,
   0.4444444444444444,
   0.25,
   0.4444444444444445,
   0.45714285714285713,
   0.2608695652173913,
   0.35714285714285715,
   0.24242424242424243,
   0.38095238095238093,
   0.75,
   0.36363636363636365,
   0.48484848484848486,
   0.5555555555555556,
   0.5625,
   0.8000000000000002,
   0.4,
   0.380952380952381,
   0.45454545454545453,
   0.33333333333333337,
   0.21428571428571427,
   0.4,
   0.7000000000000001,
   0.3846153846153846,
   0.2727272727272727,
   0.7142857142857143,
   0.5714285714285714,
   0.5,
   0.43478260869565216,
   0.5555555555555556,
   0.5806451612903226,
   0.3225806451612903,
   0.1714285714285714,
   0.875,
   0.21621621621621623,
   0.32,
   0.4444444444444445,
   0.7777777777777778,
   0.689655172413793,
   0.4444444444444445,
   0.5555555555555556,
   0.32,
   0.5555555555555556,
   0.33333333333333326,
   0.24000000000000002,
   0.6666666666666666,
   0.5,
   0.42857142857142855,
   0.4210526315789474,
   0.3448275862068965,
   0.4210526315789474,
   0.28571428571428575,
   0.2962962962962963,
   0.4444444444444445,
   0.5263157894736842,
   0.6285714285714287,
   0.2608695652173913,
   0.42857142857142855,
   0.823529411764706,
   0.30769230769230765,
   0.5,
   0.1818181818181818,
   0.28571428571428575,
   0.3636363636363636,
   0.3870967741935484,
   0.36363636363636365,
   0.6,
   0.3243243243243243,
   0.6,
   0.5882352941176471,
   0.3636363636363637,
   0.380952380952381,
   0.38461538461538464,
   0.8000000000000002,
   0.4444444444444445,
   0.6666666666666666,
   0.875,
   0.56,
   0.7142857142857143,
   0.4999999999999999,
   0.5294117647058824,
   0.7692307692307692,
   0.6666666666666666,
   0.7096774193548386,
   0.3902439024390244,
   0.875,
   0.8571428571428571,
   0.6,
   0.8000000000000002,
   0.8421052631578948,
   0.4545454545454546,
   0.7368421052631577,
   0.5666666666666667,
   0.8571428571428571,
   0.631578947368421,
   0.41666666666666663,
   0.7368421052631579,
   0.7586206896551724,
   0.8000000000000002,
   0.6399999999999999,
   0.787878787878788,
   0.8571428571428571,
   0.6428571428571429,
   0.625,
   0.19047619047619047,
   0.8484848484848485,
   0.375,
   0.30769230769230765,
   0.6875,
   0.7755102040816326,
   0.5555555555555556,
   0.625,
   0.3333333333333333,
   0.4800000000000001,
   0.6666666666666666,
   0.5882352941176471,
   0.5,
   0.7692307692307692,
   0.4666666666666667,
   0.6153846153846153,
   0.5333333333333333,
   0.5263157894736842,
   0.6875,
   0.6363636363636364,
   0.8571428571428571,
   0.7058823529411765,
   0.6511627906976745,
   0.6666666666666667,
   0.6666666666666665,
   0.7142857142857143,
   0.4615384615384615,
   0.7368421052631577,
   0.41666666666666663,
   0.8333333333333334,
   0.6896551724137931,
   0.8571428571428571,
   0.3888888888888889,
   0.42105263157894735,
   0.7857142857142856,
   0.3157894736842105,
   0.5555555555555556,
   0.7142857142857142,
   0.625,
   0.6666666666666666,
   0.6666666666666666,
   0.8,
   0.75,
   0.5925925925925926,
   0.19047619047619047,
   0.3333333333333333,
   0.14285714285714288,
   0.2,
   0.3529411764705882,
   0.6923076923076923,
   0.6956521739130435,
   0.5263157894736842,
   0.5263157894736842,
   0.3333333333333333,
   0.6451612903225806,
   0.4761904761904762,
   0.6923076923076923,
   0.588235294117647,
   0.6666666666666667,
   0.5263157894736842,
   0.3333333333333333,
   0.5217391304347825,
   0.3636363636363637,
   0.5714285714285714,
   0.8888888888888888,
   0.5806451612903225,
   0.7857142857142856,
   0.3125,
   0.7692307692307692,
   0.45454545454545453,
   0.5,
   0.4827586206896552,
   0.5357142857142857,
   0.6548672566371682,
   0.4675324675324676,
   0.5925925925925927,
   0.2727272727272727,
   0.4516129032258065,
   0.6842105263157896,
   0.4074074074074074,
   0.5652173913043478,
   0.5609756097560975,
   0.36000000000000004,
   0.8125000000000001,
   0.5128205128205129,
   0.46153846153846156,
   0.507936507936508,
   0.3111111111111111,
   0.31707317073170727,
   0.36363636363636365,
   0.7301587301587302,
   0.4444444444444445,
   0.47761194029850745,
   0.5090909090909091,
   0.5633802816901408,
   0.2857142857142857,
   0.5909090909090909,
   0.6153846153846154,
   0.6588235294117646,
   0.44,
   0.6,
   0.36363636363636365,
   0.41509433962264153,
   0.5833333333333334,
   0.5762711864406779,
   0.2105263157894737,
   0.43999999999999995,
   0.75,
   0.5151515151515152,
   0.5116279069767442,
   0.32,
   0.6363636363636364,
   0.3461538461538462,
   0.39999999999999997,
   0.5853658536585366,
   0.7058823529411765,
   0.6153846153846154,
   0.19047619047619047,
   0.71875,
   0.7058823529411765,
   0.47619047619047616,
   0.41509433962264153,
   0.3333333333333333,
   0.4842105263157895,
   0.5151515151515151,
   0.25,
   0.6769230769230768,
   0.37837837837837834,
   0.6966292134831461,
   0.5238095238095238,
   0.52,
   0.4722222222222222,
   0.5671641791044776,
   0.5,
   0.8524590163934426,
   0.4727272727272727,
   0.5,
   0.5483870967741935,
   0.3137254901960784,
   0.6976744186046512,
   0.4242424242424242,
   0.5194805194805195,
   0.6250000000000001,
   0.3773584905660377,
   0.7555555555555555,
   0.5373134328358209,
   0.2978723404255319,
   0.4482758620689655,
   0.3235294117647059,
   0.47457627118644063,
   0.625,
   0.46428571428571425,
   0.30303030303030304,
   0.5217391304347826,
   0.6857142857142857,
   0.3125,
   0.5483870967741936,
   0.5084745762711864,
   0.5084745762711865,
   0.49230769230769234,
   0.5573770491803278,
   0.2553191489361702,
   0.6461538461538462,
   0.6071428571428571,
   0.6301369863013699,
   0.3181818181818182,
   0.4210526315789474,
   0.5263157894736842,
   0.5306122448979592,
   0.39999999999999997,
   0.5217391304347826,
   0.47619047619047616,
   0.6976744186046512,
   0.5,
   0.606060606060606,
   0.5714285714285714,
   0.26086956521739124,
   0.47761194029850745,
   0.5714285714285714,
   0.5,
   0.4827586206896552,
   0.4347826086956522,
   0.4,
   0.5,
   0.5925925925925927,
   0.6666666666666666,
   0.28571428571428575,
   0.6451612903225806,
   0.42424242424242425,
   0.5365853658536586,
   0.6779661016949153,
   0.4109589041095891,
   0.43478260869565216,
   0.29411764705882354,
   0.6486486486486486,
   0.4375,
   0.15384615384615385,
   0.4313725490196078,
   0.34285714285714286,
   0.5263157894736842,
   0.875,
   0.3157894736842105,
   0.375,
   0.39999999999999997,
   0.3703703703703704,
   0.6666666666666666,
   0.6046511627906976,
   0.5633802816901409,
   0.5846153846153846,
   0.5,
   0.6206896551724137,
   0.6153846153846153,
   0.4615384615384615,
   0.13793103448275862,
   0.6363636363636365,
   0.5128205128205129,
   0.631578947368421,
   0.4444444444444444,
   0.7333333333333334,
   0.3846153846153846,
   0.5714285714285714,
   0.41860465116279066,
   0.45833333333333337,
   0.717948717948718,
   0.6060606060606061,
   0.47058823529411764,
   0.4375,
   0.5806451612903226,
   0.5263157894736842,
   0.4666666666666666,
   0.5517241379310344,
   0.742857142857143,
   0.7222222222222222,
   0.6086956521739131,
   0.6399999999999999,
   0.4736842105263158,
   0.7647058823529413,
   0.8461538461538461,
   0.5909090909090909,
   0.5789473684210527,
   0.375,
   0.5333333333333332,
   0.3448275862068966,
   0.5116279069767442,
   0.5714285714285714,
   0.5777777777777778,
   0.4571428571428572,
   0.3157894736842105,
   0.7142857142857142,
   0.4897959183673469,
   0.6666666666666666,
   0.7,
   0.5263157894736842,
   0.8000000000000002,
   0.8205128205128205,
   0.761904761904762,
   0.6666666666666666,
   0.5641025641025642,
   0.875,
   0.6666666666666667,
   0.8333333333333334,
   0.5714285714285715,
   0.35555555555555557,
   0.8823529411764706,
   0.47058823529411764,
   0.5128205128205128,
   0.6875,
   0.7272727272727272,
   0.4390243902439025,
   0.5833333333333334,
   0.5555555555555556,
   0.4516129032258065,
   0.39024390243902435,
   0.8333333333333334,
   0.4761904761904762,
   0.3181818181818182,
   0.7407407407407406,
   0.5599999999999999,
   0.625,
   0.5128205128205129,
   0.7500000000000001,
   0.5,
   0.4390243902439025,
   0.39999999999999997,
   0.4117647058823529,
   0.4571428571428572,
   0.5925925925925926,
   0.689655172413793,
   0.6060606060606061,
   0.7111111111111111,
   0.8148148148148148,
   0.5945945945945946,
   0.9444444444444444,
   0.35294117647058826,
   0.25,
   0.2962962962962963,
   0.7368421052631577,
   0.42857142857142855,
   0.6875,
   0.5454545454545455,
   0.3225806451612903,
   0.5454545454545454,
   0.6666666666666667,
   0.8571428571428571,
   0.7619047619047619,
   0.5531914893617023,
   0.4864864864864864,
   0.33333333333333337,
   0.4528301886792453,
   0.6666666666666666,
   0.7142857142857143,
   0.4827586206896552,
   0.4736842105263159,
   0.5405405405405405,
   0.46808510638297873,
   0.56,
   0.31999999999999995,
   0.4999999999999999,
   0.6363636363636364,
   0.4666666666666667,
   0.34285714285714286,
   0.7096774193548386,
   0.6086956521739131,
   0.5641025641025642,
   0.45161290322580644,
   0.25,
   0.6250000000000001,
   0.44,
   0.5789473684210527,
   0.6000000000000001,
   0.6451612903225806,
   0.6842105263157895,
   0.75,
   0.5806451612903226,
   0.4827586206896552,
   0.9090909090909091,
   0.41176470588235287,
   0.46808510638297873,
   0.3829787234042554,
   0.46511627906976744,
   0.37499999999999994,
   0.5142857142857143,
   0.5581395348837209,
   0.4444444444444444,
   0.3529411764705882,
   0.6875,
   0.7272727272727272,
   0.7692307692307692,
   0.588235294117647,
   0.3448275862068966,
   0.23529411764705882,
   0.5116279069767442,
   0.7142857142857143,
   0.742857142857143,
   0.5405405405405405,
   0.4571428571428572,
   0.5945945945945946,
   0.64,
   0.7,
   0.35555555555555557,
   0.8181818181818182,
   0.20689655172413793,
   0.37500000000000006,
   0.43243243243243246,
   0.17647058823529413,
   0.9090909090909091,
   0.2222222222222222,
   0.8333333333333334,
   0.7222222222222223,
   0.7999999999999999,
   0.7027027027027027,
   0.7272727272727272,
   0.4705882352941176,
   0.5454545454545454,
   0.7894736842105263,
   0.6341463414634148,
   0.43902439024390244,
   0.6470588235294118,
   0.8648648648648649,
   0.5454545454545455,
   0.23076923076923075,
   0.5555555555555555,
   0.7906976744186046,
   0.6341463414634148,
   0.6511627906976745,
   0.5128205128205129,
   0.5384615384615384,
   0.2,
   0.5,
   0.4,
   0.6666666666666665,
   0.6976744186046512,
   0.8181818181818182,
   0.4545454545454545,
   0.45161290322580644,
   0.5625,
   0.4137931034482759,
   0.5641025641025641,
   0.34285714285714286,
   0.5806451612903226,
   0.9375,
   0.5833333333333334,
   0.4,
   0.5777777777777777,
   0.34146341463414637,
   0.6857142857142857,
   0.7692307692307692,
   0.6206896551724138,
   0.5454545454545454,
   0.48484848484848486,
   0.4210526315789474,
   0.39999999999999997,
   0.8399999999999999,
   0.9166666666666666,
   0.41025641025641024,
   0.47368421052631576,
   0.4210526315789474,
   0.6470588235294117,
   0.326530612244898,
   0.5283018867924529,
   0.38095238095238093,
   0.4444444444444444,
   0.3846153846153846,
   0.7999999999999999,
   0.47058823529411764,
   0.4390243902439025,
   0.43749999999999994,
   0.5333333333333333,
   0.29411764705882354,
   0.625,
   0.5625,
   0.6956521739130435,
   0.7234042553191489,
   0.45161290322580644,
   0.3448275862068966,
   0.4,
   0.6470588235294117,
   0.4444444444444445,
   0.5714285714285715,
   0.4444444444444444,
   0.4210526315789474,
   0.7692307692307693,
   0.5599999999999999,
   0.5306122448979592,
   0.4375,
   0.4117647058823529,
   0.5581395348837209,
   0.6666666666666667,
   ...]]}

In [103]: for i in sts_dict:
     ...:     print (sts_dict[i][0])
     ...: 
1494
1260
1413
1962
1122

In [104]: def get_key(i):
     ...:     for ind in [0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8, 0.9,1.0]:
     ...:         if i <= ind:
     ...:             return ind
     ...: 
     ...: 

In [105]: sts_dict = {}
     ...: for ind, i in enumerate(sts_scores):
     ...:     k = get_key(i)
     ...:     if k == None:
     ...:         continue
     ...:     if k not in sts_dict:
     ...:         sts_dict[k] = [1, [i], [smatch_scores[ind]]]
     ...:     else:
     ...:         sts_dict[k][0] += 1
     ...:         sts_dict[k][1].append(i)
     ...:         sts_dict[k][2].append(smatch_scores[ind])
     ...: 

In [106]: for i in sts_dict:
     ...:     print (sts_dict[i][0])
     ...: 
859
721
500
913
1134
828
685
635
539
437

In [107]: df = pd.DataFrame({})

In [108]: for i in sts_dict:
     ...:     temp_df = pd.DataFrame({})
     ...:     temp_df["sts_bucket"] = [i]*sts_dict[i][0]
     ...:     temp_df["smatch"] = sts_dict[i][2]
     ...:     temp_df["sts_score"] = sts_dict[i][1]
     ...:     df = df.append(temp_df, ignore_index=True)
     ...: 
     ...: 
     ...: 
     ...: 

In [109]: sns.boxplot(x="sts_bucket", y="smatch", data=df)
Out[109]: <AxesSubplot:xlabel='sts_bucket', ylabel='smatch'>

In [110]: plt.show()

In [111]: sns.boxplot(x="sts_bucket", y="smatch", data=df)
Out[111]: <AxesSubplot:xlabel='sts_bucket', ylabel='smatch'>

In [112]: plt.ylabel("STS Score Bucket")
Out[112]: Text(0, 0.5, 'STS Score Bucket')

In [113]: plt.xlabel("SMATCH Score", fontsize=13)
Out[113]: Text(0.5, 0, 'SMATCH Score')

In [114]: plt.xlabel("SMATCH Score", fontsize=16)
Out[114]: Text(0.5, 0, 'SMATCH Score')

In [115]: plt.ylabel("STS Scores", fontsize=16)
Out[115]: Text(0, 0.5, 'STS Scores')

In [116]: plt.title("Correlation between SMATCH and STS Score", fontsize=21)
Out[116]: Text(0.5, 1.0, 'Correlation between SMATCH and STS Score')

In [117]: df
Out[117]: 
      sts_bucket    smatch  sts_score
0            0.1  0.800000       0.00
1            0.1  0.500000       0.05
2            0.1  0.400000       0.05
3            0.1  0.500000       0.00
4            0.1  0.526316       0.10
...          ...       ...        ...
7246         0.3  0.571429       0.28
7247         0.3  0.470588       0.28
7248         0.3  0.564103       0.24
7249         0.3  0.516129       0.24
7250         0.3  0.500000       0.24

[7251 rows x 3 columns]

In [118]: np.min(df["smatch"].to_list())
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-118-4c8371140bbe> in <module>
----> 1 np.min(df["smatch"].to_list())

NameError: name 'np' is not defined

In [119]: import numpy as np

In [120]: np.min(df["smatch"].to_list())
Out[120]: 0.04761904761904762

In [121]: sorted(df["smatch"].to_list())
Out[121]: 
[0.04761904761904762,
 0.057142857142857134,
 0.07017543859649122,
 0.07142857142857142,
 0.07142857142857144,
 0.08,
 0.08695652173913043,
 0.08695652173913043,
 0.0909090909090909,
 0.09090909090909091,
 0.09302325581395349,
 0.0930232558139535,
 0.09523809523809522,
 0.1,
 0.1,
 0.10526315789473684,
 0.10526315789473685,
 0.10526315789473685,
 0.10714285714285714,
 0.1081081081081081,
 0.11111111111111112,
 0.11111111111111112,
 0.11320754716981131,
 0.11320754716981131,
 0.11320754716981132,
 0.11428571428571428,
 0.11764705882352941,
 0.11764705882352941,
 0.11764705882352942,
 0.12244897959183673,
 0.125,
 0.125,
 0.125,
 0.12903225806451615,
 0.13043478260869565,
 0.13043478260869565,
 0.13333333333333333,
 0.13333333333333333,
 0.13333333333333333,
 0.13333333333333333,
 0.13333333333333333,
 0.13333333333333333,
 0.13333333333333333,
 0.13333333333333333,
 0.13636363636363638,
 0.13636363636363638,
 0.1379310344827586,
 0.13793103448275862,
 0.13793103448275862,
 0.13793103448275862,
 0.13793103448275862,
 0.13953488372093023,
 0.14285714285714282,
 0.14285714285714285,
 0.14285714285714285,
 0.14285714285714285,
 0.14285714285714285,
 0.14285714285714288,
 0.14285714285714288,
 0.14285714285714288,
 0.14285714285714288,
 0.14285714285714288,
 0.14285714285714288,
 0.14285714285714288,
 0.14545454545454545,
 0.14634146341463414,
 0.14634146341463414,
 0.14634146341463417,
 0.14814814814814814,
 0.14814814814814814,
 0.14814814814814814,
 0.14814814814814817,
 0.14814814814814817,
 0.15,
 0.15,
 0.15,
 0.15,
 0.15384615384615383,
 0.15384615384615383,
 0.15384615384615383,
 0.15384615384615383,
 0.15384615384615385,
 0.15384615384615385,
 0.15384615384615385,
 0.15384615384615385,
 0.15789473684210525,
 0.15789473684210525,
 0.1587301587301587,
 0.15999999999999998,
 0.15999999999999998,
 0.16,
 0.16,
 0.16,
 0.16,
 0.16,
 0.16,
 0.16,
 0.16,
 0.16,
 0.16216216216216214,
 0.16216216216216217,
 0.163265306122449,
 0.16666666666666663,
 0.16666666666666663,
 0.16666666666666663,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666666,
 0.16666666666666669,
 0.16901408450704225,
 0.1694915254237288,
 0.1702127659574468,
 0.1702127659574468,
 0.1714285714285714,
 0.17142857142857143,
 0.17142857142857143,
 0.17142857142857143,
 0.1724137931034483,
 0.1724137931034483,
 0.17391304347826086,
 0.17391304347826086,
 0.17391304347826086,
 0.17391304347826086,
 0.17391304347826086,
 0.1739130434782609,
 0.17543859649122806,
 0.17543859649122806,
 0.1754385964912281,
 0.1764705882352941,
 0.17647058823529413,
 0.17647058823529413,
 0.17647058823529413,
 0.17777777777777778,
 0.17777777777777778,
 0.17777777777777778,
 0.17857142857142855,
 0.17857142857142858,
 0.1791044776119403,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.1818181818181818,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818182,
 0.18181818181818185,
 0.18518518518518517,
 0.18749999999999997,
 0.18749999999999997,
 0.18749999999999997,
 0.1875,
 0.1875,
 0.18867924528301885,
 0.18867924528301888,
 0.1886792452830189,
 0.19047619047619047,
 0.19047619047619047,
 0.19047619047619047,
 0.19047619047619047,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1904761904761905,
 0.1917808219178082,
 0.1923076923076923,
 0.1923076923076923,
 0.1923076923076923,
 0.19230769230769232,
 0.19230769230769232,
 0.19354838709677416,
 0.19354838709677422,
 0.19512195121951217,
 0.1951219512195122,
 0.19607843137254902,
 0.19999999999999998,
 0.19999999999999998,
 0.19999999999999998,
 0.19999999999999998,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.2,
 0.20000000000000004,
 0.20000000000000004,
 0.20000000000000004,
 0.20000000000000004,
 0.20000000000000004,
 0.20000000000000004,
 0.20289855072463772,
 0.20408163265306123,
 0.20408163265306123,
 0.20408163265306123,
 0.20408163265306123,
 0.20512820512820512,
 0.20512820512820512,
 0.20512820512820512,
 0.20689655172413793,
 0.20689655172413793,
 0.20689655172413793,
 0.20689655172413793,
 0.20689655172413793,
 0.20689655172413793,
 0.20833333333333331,
 0.20833333333333334,
 0.208955223880597,
 0.21052631578947364,
 0.21052631578947367,
 0.21052631578947367,
 0.21052631578947367,
 0.21052631578947367,
 0.21052631578947367,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.2105263157894737,
 0.21276595744680848,
 0.2127659574468085,
 0.2127659574468085,
 0.21428571428571427,
 0.21428571428571427,
 0.21428571428571427,
 0.21428571428571427,
 0.21428571428571427,
 0.21428571428571427,
 0.21428571428571427,
 0.2153846153846154,
 0.21538461538461542,
 0.2162162162162162,
 0.21621621621621623,
 0.21621621621621623,
 0.21621621621621623,
 0.21621621621621623,
 0.21621621621621623,
 0.21739130434782608,
 0.21739130434782608,
 0.21739130434782608,
 0.21739130434782608,
 0.21818181818181817,
 0.21818181818181817,
 0.2191780821917808,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.2222222222222222,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22222222222222224,
 0.22580645161290322,
 0.22641509433962265,
 0.22727272727272724,
 0.22727272727272724,
 0.22727272727272727,
 0.22727272727272727,
 0.22727272727272727,
 0.22727272727272727,
 0.22857142857142854,
 0.22857142857142854,
 0.22857142857142854,
 0.22857142857142854,
 0.22857142857142854,
 0.22857142857142856,
 0.22857142857142856,
 0.22857142857142856,
 0.22857142857142856,
 0.22857142857142856,
 0.22857142857142856,
 0.2285714285714286,
 0.2285714285714286,
 0.22950819672131148,
 0.23076923076923075,
 0.23076923076923075,
 0.23076923076923075,
 0.23076923076923075,
 0.23076923076923075,
 0.23076923076923075,
 0.23076923076923075,
 0.23076923076923078,
 0.23076923076923078,
 0.23076923076923078,
 0.23076923076923078,
 0.23076923076923078,
 0.23076923076923078,
 0.23255813953488372,
 0.23255813953488372,
 0.23333333333333334,
 0.23333333333333336,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705882,
 0.23529411764705885,
 0.23529411764705885,
 0.23809523809523808,
 0.23809523809523808,
 0.23809523809523808,
 0.23809523809523808,
 0.23809523809523808,
 0.2380952380952381,
 0.2380952380952381,
 0.23999999999999996,
 0.23999999999999996,
 0.24000000000000002,
 0.24000000000000002,
 0.24000000000000002,
 0.24000000000000002,
 0.24137931034482757,
 0.24137931034482757,
 0.2413793103448276,
 0.2424242424242424,
 0.24242424242424243,
 0.24242424242424243,
 0.24242424242424243,
 0.24242424242424243,
 0.24242424242424243,
 0.24242424242424243,
 0.24242424242424246,
 0.24242424242424246,
 0.24242424242424246,
 0.24242424242424246,
 0.24390243902439024,
 0.24390243902439024,
 0.24561403508771934,
 0.24615384615384617,
 0.24999999999999994,
 0.24999999999999994,
 0.24999999999999994,
 0.24999999999999994,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25,
 0.25000000000000006,
 0.253968253968254,
 0.2545454545454545,
 0.2545454545454545,
 0.2553191489361702,
 0.2553191489361702,
 0.25641025641025644,
 0.25641025641025644,
 0.25641025641025644,
 0.25641025641025644,
 0.2580645161290323,
 0.2580645161290323,
 0.2580645161290323,
 0.25925925925925924,
 0.25925925925925924,
 0.25925925925925924,
 0.26086956521739124,
 0.26086956521739124,
 0.2608695652173913,
 0.2608695652173913,
 0.2608695652173913,
 0.2608695652173913,
 0.2608695652173913,
 0.26086956521739135,
 0.26086956521739135,
 0.26086956521739135,
 0.26086956521739135,
 0.26229508196721313,
 0.26315789473684204,
 0.2631578947368421,
 0.2631578947368421,
 0.2631578947368421,
 0.2631578947368421,
 0.2631578947368421,
 0.2631578947368421,
 0.2631578947368421,
 0.2641509433962264,
 0.2647058823529412,
 0.2666666666666666,
 0.2666666666666666,
 0.2666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26666666666666666,
 0.26865671641791045,
 0.2692307692307692,
 0.27027027027027023,
 0.27027027027027023,
 0.27027027027027023,
 0.27027027027027023,
 0.27027027027027023,
 0.27027027027027023,
 0.2702702702702703,
 0.27118644067796605,
 0.2711864406779661,
 0.2711864406779661,
 0.2711864406779661,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.2727272727272727,
 0.27272727272727276,
 0.27272727272727276,
 0.273972602739726,
 0.2745098039215686,
 0.2745098039215686,
 0.27450980392156865,
 0.27450980392156865,
 0.27450980392156865,
 0.2758620689655172,
 0.2758620689655172,
 0.2758620689655172,
 0.2758620689655172,
 0.27586206896551724,
 0.27586206896551724,
 0.27586206896551724,
 0.27586206896551724,
 0.27586206896551724,
 0.27586206896551724,
 0.27586206896551724,
 0.2769230769230769,
 0.27777777777777773,
 0.27777777777777773,
 0.2777777777777778,
 0.2777777777777778,
 0.2777777777777778,
 0.2790697674418604,
 0.27906976744186046,
 0.2790697674418605,
 0.2790697674418605,
 0.2790697674418605,
 0.2807017543859649,
 0.28571428571428564,
 0.28571428571428564,
 0.28571428571428564,
 0.28571428571428564,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.2857142857142857,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.28571428571428575,
 0.2909090909090909,
 0.29166666666666663,
 0.2926829268292683,
 0.2926829268292683,
 0.2941176470588235,
 0.2941176470588235,
 0.29411764705882354,
 0.29411764705882354,
 0.29411764705882354,
 0.29411764705882354,
 0.29411764705882354,
 0.29411764705882354,
 0.29411764705882354,
 0.2962962962962963,
 0.2962962962962963,
 0.2962962962962963,
 0.2962962962962963,
 0.2962962962962963,
 0.2962962962962963,
 0.29629629629629634,
 0.29629629629629634,
 0.29629629629629634,
 0.29629629629629634,
 0.29629629629629634,
 0.29629629629629634,
 0.2978723404255319,
 0.29787234042553196,
 0.29787234042553196,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3,
 0.3013698630136986,
 0.3018867924528302,
 0.30188679245283023,
 0.30188679245283023,
 0.303030303030303,
 0.30303030303030304,
 0.30303030303030304,
 0.30303030303030304,
 0.30303030303030304,
 0.30303030303030304,
 0.3050847457627119,
 0.3050847457627119,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.30769230769230765,
 0.3076923076923077,
 0.3076923076923077,
 0.3076923076923077,
 0.3076923076923077,
 0.3076923076923077,
 0.3076923076923077,
 0.3076923076923077,
 0.3076923076923077,
 0.3111111111111111,
 0.3111111111111111,
 0.3111111111111111,
 0.31249999999999994,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.3125,
 0.31250000000000006,
 0.31250000000000006,
 0.31250000000000006,
 0.31250000000000006,
 0.3137254901960784,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.3157894736842105,
 0.31578947368421056,
 0.31707317073170727,
 0.31746031746031744,
 0.3174603174603175,
 0.3181818181818182,
 0.3181818181818182,
 0.3181818181818182,
 0.3181818181818182,
 0.3181818181818182,
 0.3181818181818182,
 0.31818181818181823,
 0.31818181818181823,
 0.31999999999999995,
 0.31999999999999995,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32,
 0.32142857142857145,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3225806451612903,
 0.3235294117647059,
 0.3243243243243243,
 0.3243243243243243,
 0.3243243243243243,
 0.3243243243243243,
 0.3243243243243243,
 0.3243243243243243,
 0.3243243243243243,
 0.3243243243243243,
 0.32432432432432434,
 0.3255813953488372,
 0.3255813953488372,
 0.3255813953488372,
 0.3255813953488372,
 0.3255813953488372,
 0.3255813953488372,
 0.32558139534883723,
 0.32653061224489793,
 0.32653061224489793,
 0.326530612244898,
 0.32727272727272727,
 0.32727272727272727,
 0.3278688524590164,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.33333333333333326,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.3333333333333333,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 0.33333333333333337,
 ...]

In [122]: sorted(df["smatch"].to_list())[:10]
Out[122]: 
[0.04761904761904762,
 0.057142857142857134,
 0.07017543859649122,
 0.07142857142857142,
 0.07142857142857144,
 0.08,
 0.08695652173913043,
 0.08695652173913043,
 0.0909090909090909,
 0.09090909090909091]

In [123]: plt.show()

In [124]: sns.boxplot(x="sts_bucket", y="smatch", data=df)
Out[124]: <AxesSubplot:xlabel='sts_bucket', ylabel='smatch'>

In [125]: plt.ylabel("SMATCH Score", fontsize=16)
Out[125]: Text(0, 0.5, 'SMATCH Score')

In [126]: plt.xlabel("STS Scores", fontsize=16)
Out[126]: Text(0.5, 0, 'STS Scores')

In [127]: plt.title("Correlation between SMATCH and STS Score", fontsize=21)
Out[127]: Text(0.5, 1.0, 'Correlation between SMATCH and STS Score')

In [128]: plt.ylim([0.15, 1.0])
Out[128]: (0.15, 1.0)

In [129]: plt.show()

In [130]: sns.boxplot(x="sts_bucket", y="smatch", data=df)
Out[130]: <AxesSubplot:xlabel='sts_bucket', ylabel='smatch'>

In [131]: plt.xlabel("STS Scores", fontsize=16)
Out[131]: Text(0.5, 0, 'STS Scores')

In [132]: plt.ylim([0.15, 1.0])
Out[132]: (0.15, 1.0)

In [133]: plt.ylim([0, 1.0])
Out[133]: (0.0, 1.0)

In [134]: plt.ylabel("SMATCH Score", fontsize=16)
Out[134]: Text(0, 0.5, 'SMATCH Score')

In [135]: plt.title("Correlation between SMATCH and STS Score", fontsize=21)
Out[135]: Text(0.5, 1.0, 'Correlation between SMATCH and STS Score')

In [136]: plt.show()

In [137]: sns.boxplot(x="sts_bucket", y="smatch", data=df)
Out[137]: <AxesSubplot:xlabel='sts_bucket', ylabel='smatch'>

In [138]: plt.xlabel("STS Scores", fontsize=16)
Out[138]: Text(0.5, 0, 'STS Scores')

In [139]: plt.ylabel("SMATCH Score", fontsize=16)
Out[139]: Text(0, 0.5, 'SMATCH Score')

In [140]: plt.title("Correlation between SMATCH and STS Score", fontsize=21)
Out[140]: Text(0.5, 1.0, 'Correlation between SMATCH and STS Score')

In [141]: plt.show()

In [142]: cd ~/Downloads/
/Users/preksh/Downloads

In [143]: ls
00000IMG_00000_BURST20191224210247821_COVER-EFFECTS.jpg
01-Birds_Eye_View.pdf
0500.jpg
1.png
10.0
1000399935_receipt.pdf
1000417995_receipt (1).pdf
1000417995_receipt.pdf
11330-Article Text-14858-1-2-20201228 (1).pdf
11330-Article Text-14858-1-2-20201228 (2).pdf
11330-Article Text-14858-1-2-20201228 (3).pdf
11330-Article Text-14858-1-2-20201228 (4).pdf
11330-Article Text-14858-1-2-20201228 (5).pdf
11330-Article Text-14858-1-2-20201228.pdf
12104043.pdf
12431_43_1.pdf
137_file_Paper (1).pdf
137_file_Paper.pdf
1615788101518IK0BAOCWS0.pdf
1648701920119oB5qaoZt1j8VHldl.pdf
1648721815783IK0BPOZZW3.pdf
1648898306028IK0BPRJYR3.pdf
1653906913576FJxFUXBwMb2Q7uf6.pdf
17489-Article Text-20983-1-2-20210518 (1).pdf
17489-Article Text-20983-1-2-20210518 (10).pdf
17489-Article Text-20983-1-2-20210518 (11).pdf
17489-Article Text-20983-1-2-20210518 (12).pdf
17489-Article Text-20983-1-2-20210518 (13).pdf
17489-Article Text-20983-1-2-20210518 (14).pdf
17489-Article Text-20983-1-2-20210518 (15).pdf
17489-Article Text-20983-1-2-20210518 (2).pdf
17489-Article Text-20983-1-2-20210518 (3).pdf
17489-Article Text-20983-1-2-20210518 (4).pdf
17489-Article Text-20983-1-2-20210518 (5).pdf
17489-Article Text-20983-1-2-20210518 (6).pdf
17489-Article Text-20983-1-2-20210518 (7).pdf
17489-Article Text-20983-1-2-20210518 (8).pdf
17489-Article Text-20983-1-2-20210518 (9).pdf
17489-Article Text-20983-1-2-20210518.pdf
17672-Article Text-21166-1-2-20210518 (1) (1).pdf
17672-Article Text-21166-1-2-20210518 (1).pdf
17672-Article Text-21166-1-2-20210518.pdf
17_file_Paper (1).pdf
17_file_Paper.pdf
1808.10122.pdf
19th Booking.pdf
1a-tutorial-intro.pdf
2.png
2005.00661.pdf
2011.14244 (1).pdf
2011.14244.pdf
2021-03-24_LM-as-KB.pdf
2104.07606.pdf
2106.06411.pdf
2FYlNAPOn0y8xPqJUrB-nA.pdf
3.png
4.png
43_file_Paper (1).pdf
43_file_Paper.pdf
654380e0-de6b-4acb-a5c0-05b1a24c8dcf (1).jpg
654380e0-de6b-4acb-a5c0-05b1a24c8dcf.jpg
6655968.jpg
94e34526-c7c8-05ea-a29c-8c908b110910.pdf
9939389.epub
9939389.ris
ABHPN5775B-2021.pdf
ABHPN5775B-2022.pdf
ABHPN5775B.pdf
ABHPN5775B_PARTB_2021-22_134.pdf
ABHPN5775B_merged.pdf
ABHxxxxx5B_Q1_2021-22.pdf
AC MICROGRID PPT (1).pptx
AISTATS2022_Author_Response_Pack/
AISTATS2022_Author_Response_Pack.zip
AMR-TUTORIAL-FULL (1).pdf
AMR-TUTORIAL-FULL (2).pdf
AMR-TUTORIAL-FULL (3).pdf
AMR-TUTORIAL-FULL (4).pdf
AMR-TUTORIAL-FULL (5).pdf
AMR-TUTORIAL-FULL.pdf
AMR-graph.png
APJPN2066D-2021 (1).pdf
APJPN2066D-2021.pdf
APJPN2066D-2021.zip
Aadhar.pdf
Aadhar_PrekshaNema_3May.pdf
Aadharback.jpg
Aadharjpg.jpg
Abhishek/
Abhishek.zip
AdsGoInference_Jan20 - AdsGoInference_Jan20.tsv
Adsgo-with-geovertical - Adsgo-with-geovertical.tsv
AdsgoEvals_20211014-002158.csv
AdsgoEvals_20211020-204846.csv
AdsgoEvals_20220125-095604 (script_61._65e7e1_0000_24ad_b1ff_2405886caf94) - AdsgoEvals_20220125-095604 (script_61._65e7e1_0000_24ad_b1ff_2405886caf94).tsv
AdsgoEvals_20220202-215719.csv
Adsgo_all_merchantdescription - Adsgo_all_merchantdescription (1).tsv
Adsgo_all_merchantdescription - Adsgo_all_merchantdescription (2).tsv
Adsgo_all_merchantdescription - Adsgo_all_merchantdescription.tsv
Adsgo_all_merchantdescription - OnlyCustomerIds.csv
Adsgo_all_merchantdescription - Sheet1 (1).tsv
Adsgo_all_merchantdescription - Sheet1.tsv
AllPredicted_FoodDrink.tsv
All_predict_privacy - parenting.csv
Application for New CGHS Card nemaji.pdf
Application_Reimbursement.jpeg
BothCreatives.tsv
Btech_Degree_Certificate (1).pdf
Btech_Degree_Certificate.pdf
CGHS_CardCopy (1).jpeg
CGHS_CardCopy.jpeg
CIKM Presentation (1).pdf
CIKM Presentation.pdf
CIKM Presentation.pptx
CIKM-Poster.pdf
CIKM_2021_paper_1827 (1).pdf
CIKM_2021_paper_1827.pdf
CS15D201.pdf
CS15D201_PREKSHA NEMA (1).jpg
CS15D201_PREKSHA NEMA (2).jpg
CS15D201_PREKSHA NEMA (3).jpg
CS15D201_PREKSHA NEMA.jpg
Comparitive-Creatives_20210831-113936 (script_60._d254d3_0000_20a6_a347_089e082bc3e8) - Comparitive-Creatives_20210831-113936 (script_60._d254d3_0000_20a6_a347_089e082bc3e8).tsv
Contrast.tsv
Copy of Access Check_20220513-223738.csv
Copy of Error Identification_ Round 3 - Task Mate - Input (1).tsv
Copy of Error Identification_ Round 3 - Task Mate - Input.tsv
Copy of Error Identification_ Round 3 - Task Mate - tstar-errors (1).tsv
Copy of Error Identification_ Round 3 - Task Mate - tstar-errors.tsv
Copy of Revised_Pilot_Contrast - Task Mate - Output (1).tsv
Copy of Revised_Pilot_Contrast - Task Mate - Output (2).tsv
Copy of Revised_Pilot_Contrast - Task Mate - Output.tsv
Copy of Revised_Pilot_Exaggeration - Task Mate - Output.tsv
Copy of Revised_Pilot_Personalization - Task Mate - Output (1).tsv
Copy of Revised_Pilot_Personalization - Task Mate - Output (2).tsv
Copy of Revised_Pilot_Personalization - Task Mate - Output.tsv
CorrectRentalAgreement (1).pdf
CorrectRentalAgreement.pdf
Creative Restyling.pdf
DFIG-DC/
DFIG-DC.zip
DFIG_DC (1).pdf
DFIG_DC (2).pdf
DFIG_DC (3).pdf
DFIG_DC (4).pdf
DFIG_DC.pdf
Deepanway (1).jpeg
Deepanway.jpeg
Disentangling-User-Representations-CIKM2021 (1).zip
Disentangling-User-Representations-CIKM2021 (2).zip
Disentangling-User-Representations-CIKM2021 (3).zip
Disentangling-User-Representations-CIKM2021.zip
Disentangling_User_Representations_CIKM2021 (1).pdf
Disentangling_User_Representations_CIKM2021 (2).pdf
Disentangling_User_Representations_CIKM2021 (3) (1).pdf
Disentangling_User_Representations_CIKM2021 (3).pdf
Disentangling_User_Representations_CIKM2021 (4).pdf
Disentangling_User_Representations_CIKM2021.pdf
DiverstiyBasedAttentionMechanism-master/
DiverstiyBasedAttentionMechanism-master.zip
EAadhaar_xxxxxxxx4128_10092021104919_400603.pdf
EMNLP_2022_GIST (1).pdf
EMNLP_2022_GIST.pdf
EWOQ-Analysis with Business Offering - Sheet1 (1).tsv
EWOQ-Analysis with Business Offering - Sheet1.tsv
Exaggeration.tsv
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (1).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (10).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (11).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (12).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (13).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (14).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (15).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (16).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (17).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (18).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (19).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (2).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (20).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (21).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (22).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (23).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (24).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (25).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (26).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (27).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (28).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (3).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (4).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (5).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (6).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (7).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (8).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid (9).pdf
Fault_Location_Identification_in_Ungrounded_DC_Microgrid.pdf
Final_Version (1).pdf
Final_Version.pdf
GIST_NAACL_Submission.pdf
Gallan Goodiyaan.mp3
Generated Output/
Generated Output 2/
Generated Output 3/
Generated Output-20220620T064112Z-001.zip
Generated Output-20220620T072607Z-001.zip
Generated Output-20220622T135634Z-001.zip
Generated Output-20220622T201501Z-001.zip
Generated Output-20220623T093800Z-001.zip
GoldAMR paraphrase dataset-20220620T131211Z-001.zip
Gumbel-CRF-main/
Gumbel-CRF-main.zip
HintedBT__Augmenting_Back_Translation_with_Quality_and_Transliteration_Hints (1).pdf
HintedBT__Augmenting_Back_Translation_with_Quality_and_Transliteration_Hints (2).pdf
HintedBT__Augmenting_Back_Translation_with_Quality_and_Transliteration_Hints copy.pdf
HintedBT__Augmenting_Back_Translation_with_Quality_and_Transliteration_Hints.pdf
Hostel Room Vacating Form -CS15D201 (1).pdf
Hostel Room Vacating Form -CS15D201 (2).pdf
Hostel Room Vacating Form -CS15D201.pdf
IBMJournal.pdf
ICSE 2022 Presentation.pdf
ICSE_2022_2___Review_Analysis (1).pdf
ICSE_2022_2___Review_Analysis (2).pdf
ICSE_2022_2___Review_Analysis.pdf
IMG_1902.heic
IMG_1919.heic
IMG_1919.jpg
IMG_20171103_193458_HDR-01.jpeg
IMG_20180701_102833.jpg
IMG_20181104_095610.jpg
IMG_20190210_194936 (1).jpg.sb-67003784-5Pe7U4
IMG_20190210_194936 (1).png
IMG_20190210_194936.jpg
IMG_20190330_110630.jpg
IMG_20200306_134816 (1).jpg
IMG_20200306_134816.jpg
IMG_20200418_164524.jpg
IMG_20220114_172842.jpg
IMG_20220114_172849.jpg
IMG_20220114_174833.jpg
IMG_20220114_175254.jpg
Initial Part_default.mp4
InputOutput-tsv - Sheet1.tsv
Instructions for ACL-IJCNLP 2021 Proceedings (1).zip
Instructions for ACL-IJCNLP 2021 Proceedings.zip
Invite.jpg
Kumaresh_OCI.pdf
Kumaresh_US_Passport.pdf
Logo (1).png
Logo (2).png
Logo (3).png
Logo for startup.docx
Logo.png
MFANewHire.pdf
MSRParaphraseCorpus (1).msi
MSRParaphraseCorpus (2).msi
MSRParaphraseCorpus (3).msi
MSRParaphraseCorpus (3).msi 2
MSRParaphraseCorpus (3).msi 3
MSRParaphraseCorpus (3).msi.cpgz
MSRParaphraseCorpus.msi
MSRParaphraseCorpus.msi 2
MSRParaphraseCorpus.msi 2 2
MSRParaphraseCorpus.msi 2.cpgz
MSRParaphraseCorpus.msi.cpgz
MappingAdsGoCre_20211202-120422.csv
MappingAdsGoCre_20211202-120925 (1).csv
MappingAdsGoCre_20211202-120925.csv
MappingAdsGoCre_20211202-122410.csv
MaxPixel.net-Clipart-Hot-Illustration-The-Sun-Sunrise-Outdoor-2816097.jpg
May 20th 2022-Selections-Confirmed.pdf
Maynez et al. 2020 - On Faithfulness and Factuality in Abstractive Summarization.pdf
ModelDiag.png
ModifiedInference.tsv
ModifiedInference_Jan20.tsv
ModifiedInference_Jan20_templatedcreatives.tsv
ModuleNotFoundError Log.txt
Mtech_transcript.pdf
Mum-model.png
NAACL_2021__Grounded_Style_Transfer (1).pdf
NAACL_2021__Grounded_Style_Transfer (10).pdf
NAACL_2021__Grounded_Style_Transfer (11).pdf
NAACL_2021__Grounded_Style_Transfer (12).pdf
NAACL_2021__Grounded_Style_Transfer (13).pdf
NAACL_2021__Grounded_Style_Transfer (14).pdf
NAACL_2021__Grounded_Style_Transfer (15).pdf
NAACL_2021__Grounded_Style_Transfer (16).pdf
NAACL_2021__Grounded_Style_Transfer (17).pdf
NAACL_2021__Grounded_Style_Transfer (2).pdf
NAACL_2021__Grounded_Style_Transfer (3).pdf
NAACL_2021__Grounded_Style_Transfer (4).pdf
NAACL_2021__Grounded_Style_Transfer (5).pdf
NAACL_2021__Grounded_Style_Transfer (6).pdf
NAACL_2021__Grounded_Style_Transfer (7).pdf
NAACL_2021__Grounded_Style_Transfer (8).pdf
NAACL_2021__Grounded_Style_Transfer (9).pdf
NAACL_2021__Grounded_Style_Transfer.pdf
New Doc 2019-12-12 11.59.37.pdf
New Doc 2020-01-24 09.44.51.pdf
New Doc 2021-03-06 15.28.50 (1).pdf
New Doc 2021-03-06 15.28.50 (2).pdf
New Doc 2021-03-06 15.28.50 (3).pdf
New Doc 2021-03-06 15.28.50.pdf
Nodues-Certificates/
Nodues_Certificate.PDF
Original Photo.jpeg
P13-1023.pdf
P17-1008.pdf
PAN.pdf
PAN_PrekshaNema_3May.pdf
PANjpg.jpg
PFDeclaration_PrekshaNema_3May (1) (1).pdf
PFDeclaration_PrekshaNema_3May (1) (2).pdf
PFDeclaration_PrekshaNema_3May (1).pdf
PXL_20201027_094235803_2.jpg
PXL_20211002_120704865.jpg
PXL_20211104_151559535.jpg
PXL_20211221_044505844.PORTRAIT.jpg
PXL_20220226_044136346._exported_299_1645943051358_2.jpg
PXL_20220307_063837505.MP.jpg
PXL_20220410_140231372.jpg
Palak_Nema_Bio_Data.pdf
Payment_Receipt.pdf
PersonalizationAnalysis.tsv
Ph.D. Thesis Corrections_Highlighted (1).pdf
Ph.D. Thesis Corrections_Highlighted.pdf
Ph.D._Thesis_Corrections (1).pdf
Ph.D._Thesis_Corrections.pdf
Photo - Google Photos.html
Photo - Google Photos_files/
Planning_with_Entity_Chains_for_Abstractive_Summar.pdf
Plx.html
Plx_files/
PrekshaRentalAgreement.docx (1).pdf
PrekshaRentalAgreement.docx (2).pdf
PrekshaRentalAgreement.docx.pdf
Preksha_Nema.mp4
Preksha_Nema.pdf
Preksha_Nema_poster.pdf
Proof of address letter (1).pdf
Proof of address letter.pdf
Publications_Preksha.pdf
QQP/
QQP-clean.zip
Qualitative Analysis of GIST work - 4000 examples.tsv
R Grant Agreement.pdf
RBC-DSAI_PosterSession.pdf
RBC-DSAI_PosterSession.pptx
RBCDSAI EXIT FORM.pdf
Rave-1.1.0-alpha.1.dmg
ReimburseApplication (1).jpeg
ReimburseApplication.jpeg
RemainingFeesHostel.pdf
RentalAgreement.pdf
RentalAgreementSigned_Jun2022.pdf
ResponseThesis (1).pdf
ResponseThesis (2).pdf
ResponseThesis.pdf
Responses (1).pdf
Responses.pdf
Reviews.pdf
RevisedThesis (1).pdf
RevisedThesis (2).pdf
RevisedThesis.pdf
S2211467X19300082.bib
SBI_Bank_Passbook.jpeg
STS-B/
STS-B.zip
Savings Account - Open Online Zero balance Digital Savings Bank Account _ Kotak 811.pdf
Screen Shot 2022-01-13 at 11.56.32 AM.png
Screen Shot 2022-01-13 at 11.58.05 AM.png
Screen Shot 2022-01-15 at 3.15.16 PM.png
Screen Shot 2022-01-15 at 3.23.47 PM.png
Screen Shot 2022-06-21 at 7.01.23 PM.png
Screen Shot 2022-06-21 at 7.16.49 PM.png
Screen Shot 2022-06-21 at 7.21.01 PM.png
ScreencastOMaticSetup-2.18.1-JRE14.dmg
SemAE-main/
SemAE-main.zip
Shakespeare-eg1.png
ShaliniFB.pdf
Sign_EPPO135068.pdf
Stsbenchmark.tar.gz
Sublime Text.app/
TDS4861258.pdf
TDS4863844.pdf
TDS4864055.pdf
TSTAR-STRAP-Results - Input (1).tsv
TSTAR-STRAP-Results - Input.tsv
Tejaswi_thesis processing form (1).pdf
Tejaswi_thesis processing form.pdf
Thank you Swetanjal.pdf
Thesis-CS15D201.pdf
ThesisResponses.pdf
Thesis_Responses (1).pdf
Thesis_Responses (2).pdf
Thesis_Responses.pdf
TransactionReceipt (1).pdf
TransactionReceipt.pdf
Tue May 25 2021 5_51_04 PM.webm
UAI__Untangle (2) (1).pdf
UAI__Untangle (2).pdf
UAI__Untangle Appendix (1).pdf
UAI__Untangle Appendix.pdf
Unsupervised Adaptation of Multilingual Models for Code-Mixed Translation.pdf
Untitled Diagram (1).png
Untitled Diagram.png
Untitled Script_20210805-212527.csv
Untitled Script_20211122-131244.csv
Untitled Script_20211122-131546.csv
Untitled Script_20211122-131607.csv
Untitled Script_20211202-114524.csv
Untitled.drawio - diagrams.net.html
Untitled.drawio - diagrams.net_files/
VID_20220410_220521.mp4
WhatsApp Image 2021-08-27 at 4.39.15 PM (1).jpeg
WhatsApp Image 2021-08-27 at 4.39.15 PM.jpeg
WhatsApp Image 2021-11-29 at 11.35.55 PM.jpeg
WhatsApp Image 2021-12-14 at 3.30.20 PM.jpeg
WhatsApp Image 2022-01-18 at 7.03.57 PM.jpeg
WhatsApp Image 2022-03-05 at 11.14.53 AM.jpeg
WhatsApp Image 2022-03-05 at 11.15.55 AM.jpeg
WhatsApp Image 2022-05-13 at 6.17.42 PM.jpeg
WhatsApp Image 2022-05-16 at 2.58.56 PM.jpeg
WhatsApp Image 2022-05-16 at 8.24.06 AM.jpeg
WhatsApp Image 2022-06-16 at 9.55.13 PM (1).jpeg
WhatsApp Image 2022-06-16 at 9.55.13 PM (2).jpeg
WhatsApp Image 2022-06-16 at 9.55.13 PM.jpeg
WhatsApp Video 2021-12-20 at 7.49.54 PM.mp4
Wiseman et al. 2018 - Learning Neural Templates for Text Generation.pdf
access_AQLdata_20210806-174858 (1).csv
access_AQLdata_20210806-174858.csv
aclImdb_v1.tar.gz
acmart-primary (1).zip
acmart-primary.zip
all_vertic_beam_5.txt
all_vertical_scores.tsv
alphaaxis-dfig (1).png
alphaaxis-dfig.png
alphabeta-dfig.png
amr-graph-paper.png
amr-modernstyle.png
amr-paper-diag-f.png
amr-paper-diag.png
amr-shakespeare.png
amr_datasets/
amr_datasets-20220519T084233Z-002.zip
archive.zip
as-or/
as-or.zip
attachments/
attachments.zip
audacity-macos-3.1.3-Intel.dmg
b249d087-8f60-4154-a8df-8e16cfe5d07e.jpg
bagpipe.darwin_amd64.172302322.zip
betaaxis-dfig.png
bibtex-526.bib
blacklist_business
bodeplot.png
c45805c3-b720-0a17-a0fc-620e47b4c343.pdf
cdoc.sst
cds_sample_dataset/
cds_sample_dataset-20211020T055532Z-001.zip
cheenu-biodata.pdf
chromeremotedesktop.dmg
cikm-presentation (1).mp4
cikm-presentation.mp4
city_names_html
city_state_names
classifier_scores/
classifier_scores-20220622T093210Z-001.zip
code/
creative-restyling.png
deposit_interest_certificate_12572414.pdf
dev-v2.0.json
dfig-alphabeta (1).png
dfig-alphabeta.png
dfig-dcsystem (1).png
dfig-dcsystem.png
dfig-equivalentcircuit (1).png
dfig-equivalentcircuit.png
diag.png
diag1.png
diversity-diag1.png
dynamicmodelDFIG.png
e2e-cleaning-master.zip
ead-intro-refnet.png
ead-introduction.png
ee2bf3ed-ff3c-4c7e-ba05-0ca70b2955a5.jpg
en_hierarchy_heatmap.jpg
en_nlb_heatmap.jpg
eval_sawmum_generation_model_baseline_rouge2.svg
evaluations-pilot.AdsGo.CSVUpload.StyleEWOQen-IN.csv.desktop.2022-02-27-1938-202203020328-per_eval_aggregated (1).csv
evaluations-pilot.AdsGo.CSVUpload.StyleEWOQen-IN.csv.desktop.2022-02-27-1938-202203020328-per_eval_aggregated (2).csv
evaluations-pilot.AdsGo.CSVUpload.StyleEWOQen-IN.csv.desktop.2022-02-27-1938-202203020328-per_eval_aggregated.csv
evaluations-pilot.AdsGo.CSVUpload.StylisedCreativesGrounding.csv.desktop.2022-02-22-0004-202203012250-per_eval_aggregated.csv
event (1).ics
event (2).ics
event.ics
events.out.tfevents.1654670462.yobgv2.prod.google.com.596614.1.v2
events.out.tfevents.1655219822.yodk2.prod.google.com.339091.1.v2
example.tfrecord
f164218c-d850-0e5a-8290-930fa418c18e.pdf
factualconsistency.pdf
filetwo.tsv
flux-timeline.png
food!.jpeg
food_drink_eval - Sheet1.tsv
game_cluster_all_sents.csv
gif.gif
gu-hi/
gu-hi.zip
hallucinated.tsv
health_comparison.txt
hh_comparison.txt
hin-eng/
hin-eng (1).zip
hin-eng (2).zip
hin-eng.zip
hindi_wiki/
hybrid_micro_grid (1).pdf
icse_recording/
ilovepdf_merged.pdf
invoice-chair.pdf
invoice-ups.pdf
lLabeledCreatives.tsv
last-recording_default.mp4
last-slide_default (1).mp4
last-slide_default.mp4
logo.pdf
london.jpg
mainblock.png
mainblockdiag.png
maindiag.png
model.ckpt-1034100.meta
modeldiag (1).png
modeldiag-onecolumn.jpg
modeloneclumn.jpg
modern-style.png
mrpc_pairs/
mrpc_pairs 2/
mrpc_pairs-20220621T172901Z-001.zip
mrpc_test.tsv
mtech presentation-rev (1).pptx
mtech presentation-rev.pptx
mtech presentation.pptx
ne.jpeg
nmt_with_attention.ipynb
numberofimpressions-kwi=1.png
onefile.tsv
operating-region.png
overall-numberofimpressions.png
overall_timeline.png
overlap_nonstopwords
overlap_nonstopwords.tsv
paragliding.jpeg
paraphrasing_ad_creatives_inputs.txt
paraphrasing_allverticals_business_city_1010000_predictions.txt
paraphrasing_food_cb_1010000_predictions.txt
paraphrasing_fooddrink_1010000_predictions.txt
paraphrasing_health_1010000_predictions.txt
paraphrasing_onlyvertical_1010000_predictions.txt
paraphrasing_shopping_1004400_predictions.txt
paraphrasing_shopping_1010000_predictions.txt
passage_level_preliminary_decoder
passage_level_refinement_decoder
pcp1p2.png
peryear-theme.png
picontroller.png
pp.jpeg
preksha conversion letter (1).pdf
preksha-biodata.pdf
preksha-photo.jpeg
preprints202201.0018.v1.pdf
privacy-theme-plot.png
processing-form (1) (1).docx
processing-form (1).docx
processing-form (1).docx (1).pdf
processing-form (1).docx (2).pdf
processing-form (1).docx.pdf
processing-form.docx
proposed_model.png
protobuf-3.17.3/
protobuf-all-3.17.3.zip
pwmrectifier.png
qqp_dataset/
qt-main/
qt-main.zip
ratatouille.jpeg
refnet-final.png
results_ner--flume_exec_mode=IN_PROCESS
rlebret-wikipedia-biography-dataset-d0d6c78/
rlebret-wikipedia-biography-dataset-d0d6c78.zip
sam_smiles_2.png
scholar.enw
sector-table.png
sector_diag.png
selfiephoto.pdf
selfiephoto.png
sellingdata-posiitvereviews_default.mp4
sensors-21-04490-v2.pdf
sent_level_preliminary_decoder
sent_level_refinement_decoder
sentencepiece (1).model
sentencepiece.model
sentencepiece.vocab
short2mins.mp4
sign-preksha-nema.jpg
signature-removebg-preview (1).png
signature-removebg-preview.png
silverinvpara_round2_v2-20220623T134324Z-001.zip
sketched.jpeg
slide7-9(1_20)_default_67558a19.mp4
so-nlbfinal.png
space-vector-reluctant.png
spacevector.png
sparse_bucket.2020-07-21.322442299
standalone-dfigdc (1).png
standalone-dfigdc.png
stopwords.txt
sts_dataset/
sts_dataset 2/
sts_dataset-20220623T044229Z-001.zip
sublime_text_build_4113_mac.zip
subsync.png
synchronus.png
taavx9426s9-Software.zip
table-invoice.pdf
tag-genome/
tag-genome.zip
test.input0 (1).amr
test.input0.amr
theme-timeline.png
timeline-with-regression.png
timeline_plot.png
torque-comparator.png
torque-timeline.png
train.input0.bpe
train.input0.txt
tsv-file
uncased_L-12_H-768_A-12.zip
upto intro_clustering_default.mp4
upto-bertsentiment_default.mp4
upto-selling-data_default.mp4
upto-slide19_default.mp4
upto-slide6_default.mp4
use-upto-slide4_default.mp4
vecmap-master/
vecmap-master.zip
vocabs_mc4.250000.100extra_sentencepiece.vocab
vsi-switchingpositions.png
web-page-photo copy.pdf
web-page-photo.png
wind-energy-increase (1).png
wind-energy-increase.png
xx
xx.csv
xx.drawio - diagrams.net.html
xx.drawio - diagrams.net_files/
xx.png

In [144]: mkdir error_identificaiton

In [145]: cp Copy\ of\ Error\ Identification_\ Round\ 3\ -\ Task\ Mate\ -\ Input.tsv error_identificaiton/

In [146]: cp Copy\ of\ Error\ Identification_\ Round\ 3\ -\ Task\ Mate\ -\ Input.tsv error_identificaiton/str
     ...: ap.tsv

In [147]: cp Copy\ of\ Error\ Identification_\ Round\ 3\ -\ Task\ Mate\ -\ Input\ \(1\).tsv error_identificai
     ...: ton/tstar.tsv

In [148]: cd error_identificaiton/
/Users/preksh/Downloads/error_identificaiton

In [149]: ls
Copy of Error Identification_ Round 3 - Task Mate - Input.tsv
strap.tsv
tstar.tsv

In [150]: import pandas as pd

In [151]: x = pd.read_csv("strap.tsv", sep="\t")

In [152]: x
Out[152]: 
                        direction      Unnamed: 1  ...  is no errror  is incoorect
0                bible_poetry.tsv      Incomplete  ...             0             0
1                bible_poetry.tsv      Incomplete  ...             0             0
2                bible_poetry.tsv  Meaning Change  ...             0             0
3                bible_poetry.tsv      Incomplete  ...             0             0
4                bible_poetry.tsv      Incomplete  ...             0             0
...                           ...             ...  ...           ...           ...
5995  switchboard_shakespeare.tsv             NaN  ...             0             0
5996  switchboard_shakespeare.tsv             NaN  ...             0             0
5997  switchboard_shakespeare.tsv             NaN  ...             0             0
5998  switchboard_shakespeare.tsv             NaN  ...             0             0
5999  switchboard_shakespeare.tsv             NaN  ...             0             0

[6000 rows x 6 columns]

In [153]: x.columns
Out[153]: 
Index(['direction', 'Unnamed: 1', 'Is incomplete', 'is meaning change',
       'is no errror', 'is incoorect'],
      dtype='object')

In [154]: x["Error"] = x[Unnamed: 1]
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-154-063514aa3303> in <module>
----> 1 x["Error"] = x[Unnamed: 1]

NameError: name 'Unnamed' is not defined

In [155]: x["Error"] = x["Unnamed: 1"]

In [156]: x
Out[156]: 
                        direction      Unnamed: 1  Is incomplete  ...  is no errror  is incoorect           Error
0                bible_poetry.tsv      Incomplete            1.0  ...             0             0      Incomplete
1                bible_poetry.tsv      Incomplete            1.0  ...             0             0      Incomplete
2                bible_poetry.tsv  Meaning Change            0.0  ...             0             0  Meaning Change
3                bible_poetry.tsv      Incomplete            1.0  ...             0             0      Incomplete
4                bible_poetry.tsv      Incomplete            1.0  ...             0             0      Incomplete
...                           ...             ...            ...  ...           ...           ...             ...
5995  switchboard_shakespeare.tsv             NaN            NaN  ...             0             0             NaN
5996  switchboard_shakespeare.tsv             NaN            NaN  ...             0             0             NaN
5997  switchboard_shakespeare.tsv             NaN            NaN  ...             0             0             NaN
5998  switchboard_shakespeare.tsv             NaN            NaN  ...             0             0             NaN
5999  switchboard_shakespeare.tsv             NaN            NaN  ...             0             0             NaN

[6000 rows x 7 columns]

In [157]: cp /Users/preksh/Downloads/Error\ Identification\ results\ -\ Consolidated.tsv consolidated.tsv

In [158]: x = pd.read_csv("consolidated.tsv", sep="\t")
---------------------------------------------------------------------------
ParserError                               Traceback (most recent call last)
<ipython-input-158-348bada03554> in <module>
----> 1 x = pd.read_csv("consolidated.tsv", sep="\t")

/Library/Python/3.8/site-packages/pandas/io/parsers.py in read_csv(filepath_or_buffer, sep, delimiter, header, names, index_col, usecols, squeeze, prefix, mangle_dupe_cols, dtype, engine, converters, true_values, false_values, skipinitialspace, skiprows, skipfooter, nrows, na_values, keep_default_na, na_filter, verbose, skip_blank_lines, parse_dates, infer_datetime_format, keep_date_col, date_parser, dayfirst, cache_dates, iterator, chunksize, compression, thousands, decimal, lineterminator, quotechar, quoting, doublequote, escapechar, comment, encoding, dialect, error_bad_lines, warn_bad_lines, delim_whitespace, low_memory, memory_map, float_precision, storage_options)
    608     kwds.update(kwds_defaults)
    609 
--> 610     return _read(filepath_or_buffer, kwds)
    611 
    612 

/Library/Python/3.8/site-packages/pandas/io/parsers.py in _read(filepath_or_buffer, kwds)
    466 
    467     with parser:
--> 468         return parser.read(nrows)
    469 
    470 

/Library/Python/3.8/site-packages/pandas/io/parsers.py in read(self, nrows)
   1055     def read(self, nrows=None):
   1056         nrows = validate_integer("nrows", nrows)
-> 1057         index, columns, col_dict = self._engine.read(nrows)
   1058 
   1059         if index is None:

/Library/Python/3.8/site-packages/pandas/io/parsers.py in read(self, nrows)
   2059     def read(self, nrows=None):
   2060         try:
-> 2061             data = self._reader.read(nrows)
   2062         except StopIteration:
   2063             if self._first_chunk:

pandas/_libs/parsers.pyx in pandas._libs.parsers.TextReader.read()

pandas/_libs/parsers.pyx in pandas._libs.parsers.TextReader._read_low_memory()

pandas/_libs/parsers.pyx in pandas._libs.parsers.TextReader._read_rows()

pandas/_libs/parsers.pyx in pandas._libs.parsers.TextReader._tokenize_rows()

pandas/_libs/parsers.pyx in pandas._libs.parsers.raise_parser_error()

ParserError: Error tokenizing data. C error: Expected 5 fields in line 3424, saw 6


In [159]: x = open("consolidated.tsv").readlines()

In [160]: x
Out[160]: 
['direction\tTstar_Error\tStrap_Error\t{Input} Text\t{Output} Text\n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd came and preached peace to you which were afar off, and to them that were nigh.\tCame, and preached peace to you distant, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tThe two pillars, one sea, and twelve brasen bulls that were under the bases, which king Solomon had made in the house of the LORD: the brass of all these vessels was without weight.\tTwo sea-pillars and brasen bullshits under the bases unweighted by King Solomon. \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tAnd none shall appear before me empty.\tBefore me none empty appear. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd all the people saw the cloudy pillar stand at the tabernacle door: and all the people rose up and worshipped, every man in his tent door.\tAll saw a cloudy pillar stand at the tent door, and rose and worshipped. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tTake the millstones, and grind meal: uncover thy locks, make bare the leg, uncover the thigh, pass over the rivers.\tTake millstones and grind your meal, uncover your locks and bare your legs. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tNow the rest of the acts of Jeroboam, and all that he did, and his might, how he warred, and how he recovered Damascus, and Hamath, which belonged to Judah, for Israel, are they not written in the book of the chronicles of the kings of Israel?\tNot written in his acts, Damascus and Judah's rest, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tHe that tilleth his land shall have plenty of bread: but he that followeth after vain persons shall have poverty enough.\tHe'll have plenty o'er his land but poor enough; \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd they shall amerce him in an hundred shekels of silver, and give them unto the father of the damsel, because he hath brought up an evil name upon a virgin of Israel: and she shall be his wife; he may not put her away all his days.\tSince he brought up an evil name in Israeli virgin, to give \n',
 "bible_poetry.tsv\tIncomplete\tNo Error\tI have taught thee in the way of wisdom; I have led thee in right paths.\tI've taught thee the right paths, \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd he hath on his vesture and on his thigh a name written, KING OF KINGS, AND LORD OF LORDS.\tHis vestured name, written in King and Lord, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tBut he himself went a day's journey into the wilderness, and came and sat down under a juniper tree: and he requested for himself that he might die; and said, It is enough; now, O LORD, take away my life; for I am not better than my fathers.\tBut went the wilderness for a day, came beneath the juniper tree, and bid him die. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor they have taken of their daughters for themselves, and for their sons: so that the holy seed have mingled themselves with the people of those lands: yea, the hand of the princes and rulers hath been chief in this trespass.\tThey took daughters and sons to merge those peoples, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tFor he that is not against us is on our part.\tHe wad na wrang us against him, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tA continual dropping in a very rainy day and a contentious woman are alike.\tLike constant drops on very rainy days, and contentious woman. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the table and all his vessels, and the candlestick and his vessels, and the altar of incense,\tWith table, candlestick, vessels, and altar, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tTake ye therefore good heed unto yourselves; for ye saw no manner of similitude on the day that the LORD spake unto you in Horeb out of the midst of the fire:\tYou saw no like sight on day when God spoke to you in Horneb. \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tMaking the word of God of none effect through your tradition, which ye have delivered: and many such like things do ye.\tAnd making thy tradition unblest with God! \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd he had much business in the cities of Judah: and the men of war, mighty men of valour, were in Jerusalem.\tIn Jerusalem he had a waft of business; \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tHe that followeth after righteousness and mercy findeth life, righteousness, and honour.\tThose who follow righteousness and mercy find life and honour. \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tBut I will send a fire on the wall of Gaza, which shall devour the palaces thereof:\tBut I wad send the fire to the Gaza wall, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tBe ye therefore followers of God, as dear children;\tLike children of God, follow Him! I pray, \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThen will I make this house like Shiloh, and will make this city a curse to all the nations of the earth.\tMake this house like Shailoh's, and make all nations curse. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tNo man that hath a blemish of the seed of Aaron the priest shall come nigh to offer the offerings of the LORD made by fire: he hath a blemish; he shall not come nigh to offer the bread of his God.\tNo priest Aaron's seed blemish nor come to offer \n",
 "bible_poetry.tsv\tIncomplete\tNo Error\tShe standeth in the top of high places, by the way in the places of the paths.\tShe stands by the high places' top, \n",
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tBut know ye for certain, that if ye put me to death, ye shall surely bring innocent blood upon yourselves, and upon this city, and upon the inhabitants thereof: for of a truth the LORD hath sent me unto you to speak all these words in your ears.\tKnow, surely, bring this city and inhabitants' blood to me. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tThou hypocrite, cast out first the beam out of thine own eye, and then shalt thou see clearly to pull out the mote that is in thy brother's eye.\tAnd cast first your hypocrites' beam, and clear then to pull your brother's mote. \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd the king of Israel went out, and smote the horses and chariots, and slew the Syrians with a great slaughter.\tAnd shot horses and chariots, and slain Syrians; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd say, Hear the word of the LORD, O king of Judah, that sittest upon the throne of David, thou, and thy servants, and thy people that enter in by these gates:\tSay, hear what God David stooped on his throne, \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd Abraham gave all that he had unto Isaac.\tAnd Abraham gave him all he had, \n',
 "bible_poetry.tsv\tIncorrect/New Information\tNo Error\tAnd we went over the brook Zered.\tZered, o'er the river yon went, \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tThen said the Jews unto him, Thou art not yet fifty years old, and hast thou seen Abraham?\tNot yet fifty years old, and hath ye seen Abraham? \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tthe treacherous dealers have dealt treacherously; yea, the treacherous dealers have dealt very treacherously.\tThe traffickers, very treacherous dealt, \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd thou shalt make a vail of blue, and purple, and scarlet, and fine twined linen of cunning work: with cherubims shall it be made:\tWith cherubims make a vaunt of blue, purple, scarlet, fine twined linen. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tIn the third year of his reign, he made a feast unto all his princes and his servants; the power of Persia and Media, the nobles and princes of the provinces, being before him:\tThe third year of his reign, celebrates Persia's power and media: \n",
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tI thank God that I baptized none of you, but Crispus and Gaius;\tGod bless, I baptized you none but Crespus and Gaius; \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd some of them that stood by, when they heard it, said, Behold, he calleth Elias.\t"Some of them," said he, "we call him Elias, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd there were made on them, on the doors of the temple, cherubims and palm trees, like as were made upon the walls; and there were thick planks upon the face of the porch without.\tChiels and palm trees at temple doors and thick planks on porch face. \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tThen hear thou in heaven their prayer and their supplication, and maintain their cause.\tThen hear their prayer, and support their cause; \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThe hands of the pitiful women have sodden their own children: they were their meat in the destruction of the daughter of my people.\tWretched women slaughtered their children; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThe black horses which are therein go forth into the north country; and the white go forth after them; and the grisled go forth toward the south country.\tThe black horses there went the north, the white horses went the south; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tBut the children of Benjamin gathered themselves together out of the cities unto Gibeah, to go out to battle against the children of Israel.\tAnd gathered in Giraltar to fight with Israel: \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd I will make thy seed as the dust of the earth: so that if a man can number the dust of the earth, then shall thy seed also be numbered.\tIf men can number your earth's dust, \n",
 "bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Serug lived after he begat Nahor two hundred years, and begat sons and daughters.\tSerug lived 'gainst Nahor after 200 years of marriage. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tBut I will put hooks in thy jaws, and I will cause the fish of thy rivers to stick unto thy scales, and I will bring thee up out of the midst of thy rivers, and all the fish of thy rivers shall stick unto thy scales.\tBut I'll put the hooks in your jaws, and thy fish will stick to your scales. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd she had a sister called Mary, which also sat at Jesus' feet, and heard his word.\tShe was also Mary's sister, who listened to Jesus' word, \n",
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd the evil spirit answered and said, Jesus I know, and Paul I know; but who are ye?\tI know Jesus and Paul, but what do ye know? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd in the seventh day the priest shall look on the plague: and, behold, if the scall spread not, and there be in it no yellow hair, and the scall be not in sight deeper than the skin;\tThe priest sought on seventh day not hairy, and scall deeper than skin, \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\t(Howbeit there came other boats from Tiberias nigh unto the place where they did eat bread, after that the Lord had given thanks:)\tWhile other boats came back to Tiberias after they ate the bread, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd he did that which was evil in the sight of the LORD his God, and humbled not himself before Jeremiah the prophet speaking from the mouth of the LORD.\tHad done wicked, unhumiliated before prophet Joel speaking; \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd he left off talking with him, and God went up from Abraham.\tAnd left him talking, and God went to Abraham. \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tBut ye gave the Nazarites wine to drink; and commanded the prophets, saying, Prophesy not.\tBut gied the Nazis drink wine, and told the Prophets not prophesying. \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tThe LORD hath loved him: he will do his pleasure on Babylon, and his arm shall be on the Chaldeans.\tGod loved Babylon, and in Chaldeans' arms \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd by him shall be the tribe of Manasseh: and the captain of the children of Manasseh shall be Gamaliel the son of Pedahzur.\tAs manasseh tribe's captain Gamaliel, \n",
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd that year they vexed and oppressed the children of Israel: eighteen years, all the children of Israel that were on the other side Jordan in the land of the Amorites, which is in Gilead.\tOn Jordan's other side they annoy'd and oppressed. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tPass through the host, and command the people, saying, Prepare you victuals; for within three days ye shall pass over this Jordan, to go in to possess the land, which the LORD your God giveth you to possess it.\tPass Jordan and tell up to three days prepare \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThat ye may be blameless and harmless, the sons of God, without rebuke, in the midst of a crooked and perverse nation, among whom ye shine as lights in the world;\tThy sons may be blameless, harmless in perverse crooked nation, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tMoreover the multitude of thy strangers shall be like small dust, and the multitude of the terrible ones shall be as chaff that passeth away: yea, it shall be at an instant suddenly.\tAnd thy strangers like small dust, and chaff like to pass away. \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd they could not eat thereof.\tIt is not that they can eat; \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tBecause I have called, and ye refused; I have stretched out my hand, and no man regarded;\tI call'd and ye refused; so I stretch'd my hand and none sought; \n",
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tAnd the king left ten women, which were concubines, to keep the house.\tThe King left ten concubine wives to keep the house; \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tAnd Israel served the LORD all the days of Joshua, and all the days of the elders that overlived Joshua, and which had known all the works of the LORD, that he had done for Israel.\tAnd served Judah, and elders who overlived and knew all their works. \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd Solomon determined to build an house for the name of the LORD, and an house for his kingdom.\tAnd Solomon decreed that he would build a house \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd Judah did evil in the sight of the LORD, and they provoked him to jealousy with their sins which they had committed, above all that their fathers had done.\tJudah did evil, provoked fathers jealous of their sins above; \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd he turned unto her by the way, and said, Go to, I pray thee, let me come in unto thee; (for he knew not that she was his daughter in law.)\tHe turned her by the way and said, "Go! He knew not his daughter in law. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd he shall offer the one of the turtledoves, or of the young pigeons, such as he can get;\tOffers, as he may, turtle-doves or young pigeons; \n',
 "bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd when Saul looked behind him, David stooped with his face to the earth, and bowed himself.\tDavid stoop'd and bow'd his face when Saul looked behind. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Abraham rose up early in the morning, and took bread, and a bottle of water, and gave it unto Hagar, putting it on her shoulder, and the child, and sent her away: and she departed, and wandered in the wilderness of Beersheba.\tAdam rose early, took bread and bottle, gave his shoulder, and left \n',
 'bible_poetry.tsv\tIncorrect/New Information\tNo Error\tHave any of the rulers or of the Pharisees believed on him?\tHe deemed?--Whether rules or pharisees, \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd it came to pass after this, that the king of the children of Ammon died, and Hanun his son reigned in his stead.\tAnd after him died and succeeded Hanun's son. \n",
 "bible_poetry.tsv\tNo Error\tIncomplete\tFor I heard the defaming of many, fear on every side.\tI heard many a defam'd, and every side fear'd. \n",
 'bible_poetry.tsv\tNo Error\tMeaning Change\twho will hearken and hear for the time to come?\tWho will listen at the time to come \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd when thou prayest, thou shalt not be as the hypocrites are: for they love to pray standing in the synagogues and in the corners of the streets, that they may be seen of men.\tAs they love praying standing at synagogues and streets, hypocrites! \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tBehold, he taketh away, who can hinder him?\tBehold! who can hinder him? Then who can hinder \n',
 "bible_poetry.tsv\tNo Error\tIncomplete\tFor now thou numberest my steps: dost thou not watch over my sin?\tNow ye've number'd my steps: do not watch over my sin? \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tThus saith the LORD of hosts, the God of Israel, saying; Ye and your wives have both spoken with your mouths, and fulfilled with your hand, saying, We will surely perform our vows that we have vowed, to burn incense to the queen of heaven, and to pour out drink offerings unto her: ye will surely accomplish your vows, and surely perform your vows.\tYour mouths, and wives, surely vow'd, and drink offerings fulfilled; \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tThough he be fruitful among his brethren, an east wind shall come, the wind of the LORD shall come up from the wilderness, and his spring shall become dry, and his fountain shall be dried up: he shall spoil the treasure of all pleasant vessels.\tThough fruitful among his brethren, he would spoil all pleasant vessels. \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tFor in that he died, he died unto sin once: but in that he liveth, he liveth unto God.\tHe died in one sin--but dies because he lives for God. \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tFor all tables are full of vomit and filthiness, so that there is no place clean.\tAll tables were full of vomit and filthily, so unclean \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tAnd Joshua rose early in the morning, and the priests took up the ark of the LORD.\tJoshua rose early in the morning, and priests took the ark. \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd the Levites stood with the instruments of David, and the priests with the trumpets.\tLeviticus stood with David's instruments, and priests trumpets; \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tThen said they unto him, Where is thy Father?\tWhere art thou now, thy Father? where art thou? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd for a spirit of judgment to him that sitteth in judgment, and for strength to them that turn the battle to the gate.\tTo judge him, and strength to turn the battle to gate. \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tWhoso robbeth his father or his mother, and saith, It is no transgression; the same is the companion of a destroyer.\tRobber of father or mother, and it transgress'd \n",
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd it came to pass, when Jesus had ended these sayings, the people were astonished at his doctrine:\tWhen these words end, Jesus' doctrine astonied \n",
 "bible_poetry.tsv\tNo Error\tIncomplete\tAnd the rest, some on boards, and some on broken pieces of the ship.\tRest on the boards and some on the ship's broken pieces. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd unto Caleb the son of Jephunneh he gave a part among the children of Judah, according to the commandment of the LORD to Joshua, even the city of Arba the father of Anak, which city is Hebron.\tTo Joshua's father Jephunneh's Caleb gave \n",
 "bible_poetry.tsv\tIncorrect/New Information\tNo Error\tThe words of Nehemiah the son of Hachaliah.\tAnd Nehemiah's words are sae sweet, \n",
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tIs not the gleaning of the grapes of Ephraim better than the vintage of Abiezer?\tIs it not better Ephraim's wine than Abiezer? \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the rest of the men which were not killed by these plagues yet repented not of the works of their hands, that they should not worship devils, and idols of gold, and silver, and brass, and stone, and of wood: which neither can see, nor hear, nor walk:\tYet the rest, not slain by these plagues, repents to gold, silver, and brass, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tor wilt thou leave thy labour to him?\tOr wilt thou leave thy ain work to him? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThou shalt also make a table of shittim wood: two cubits shall be the length thereof, and a cubit the breadth thereof, and a cubit and a half the height thereof.\tAlso make a table of shit-wood equal two cubits and half. \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd when Peter saw it, he answered unto the people, Ye men of Israel, why marvel ye at this?\tPetrarch, when he saw it, wondered why this Israeli marveled. \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd if she had at all an husband, when she vowed, or uttered ought out of her lips, wherewith she bound her soul;\tIf she had a husband at all while she vow'd or declared. \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tHe delivered me from my strong enemy, and from them which hated me: for they were too strong for me.\tDelivered me to a foe too strong to hate. \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tFour tables were on this side, and four tables on that side, by the side of the gate; eight tables, whereupon they slew their sacrifices.\tFour tables were on this side, and eight were on that side. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor yet a little while, and he that shall come will come, and will not tarry.\tThe little while still, and he will come \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd when the ass saw the angel of the LORD, she fell down under Balaam: and Balaam's anger was kindled, and he smote the ass with a staff.\tThe ass fell under Salaam, in anger shot with staff, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd David was displeased, because the LORD had made a breach upon Uzza: wherefore that place is called Perezuzza to this day.\tDavid uplighted by Perezuzza's assail, \n",
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tWith whomsoever of thy servants it be found, both let him die, and we also will be my lord's bondmen.\tLet him die, and we'll bond our lord also. \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tLet thy fountain be blessed: and rejoice with the wife of thy youth.\tThy fountain was blessed, and thy wife rejoiced; \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd a mitre of fine linen, and goodly bonnets of fine linen, and linen breeches of fine twined linen,\tWi' fine, fine, and fine linens, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThe nethermost chamber was five cubits broad, and the middle was six cubits broad, and the third was seven cubits broad: for without in the wall of the house he made narrowed rests round about, that the beams should not be fastened in the walls of the house.\tMost chambers five-cubits wide, middle six-cubits wide, and third-- \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tFor if Jesus had given them rest, then would he not afterward have spoken of another day.\tThen if Jesus gave them rest, he would not talk of another day. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd when he had sent the multitudes away, he went up into a mountain apart to pray: and when the evening was come, he was there alone.\tHe went up the mountain to pray, and in the evening alone \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tAnd Jehoshaphat stood in the congregation of Judah and Jerusalem, in the house of the LORD, before the new court,\tAt Judah and Jerusalem, Jehoshaphat stood before the new court, \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tBut after that I am risen, I will go before you into Galilee.\tBut I'll go to Galilee before you, \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tGive therefore thy servant an understanding heart to judge thy people, that I may discern between good and bad: for who is able to judge this thy so great a people?\tGive understanding heart to judge, I can discern between good and bad. \n',
 "bible_poetry.tsv\tNo Error\tIncorrect/New Information\tAnd the man smote him, so that in smiting he wounded him.\tAs he was wounded by a man's smiting, \n",
 "bible_poetry.tsv\tNo Error\tIncomplete\tBrethren, my heart's desire and prayer to God for Israel is, that they might be saved.\tTo save Israel, and pray to the Lord, \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd Pharaoh awoke, and, behold, it was a dream.\tAwaking the Pharaoh, and in a dream \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd they that shall be of thee shall build the old waste places: thou shalt raise up the foundations of many generations; and thou shalt be called, The repairer of the breach, The restorer of paths to dwell in.\tTo build old places of waste, and raise what many generations hath hath ta'en. \n",
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd them that are turned back from the LORD; and those that have not sought the LORD, nor enquired for him.\t"There\'s not a God to look on, nor a man." \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd David distributed them, both Zadok of the sons of Eleazar, and Ahimelech of the sons of Ithamar, according to their offices in their service.\tAnd David distributed them wi' Zadok and Ahimelech; \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tand when thou art athirst, go unto the vessels, and drink of that which the young men have drawn.\tGo to vessels and drink athirst the young men; \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tBut the tithes of the children of Israel, which they offer as an heave offering unto the LORD, I have given to the Levites to inherit: therefore I have said unto them, Among the children of Israel they shall have no inheritance.\tI've given Leviticus a tithe they offer to inherit. \n",
 'bible_poetry.tsv\tNo Error\tIncomplete\tI will seek that which was lost, and bring again that which was driven away, and will bind up that which was broken, and will strengthen that which was sick: but I will destroy the fat and the strong; I will feed them with judgment.\tTo seek lost, bring broken up, and strengthen sick: Fate doth destroy and feed \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tWho serve unto the example and shadow of heavenly things, as Moses was admonished of God when he was about to make the tabernacle: for, See, saith he, that thou make all things according to the pattern shewed to thee in the mount.\tWho serve as example and shadow, admonished God about to make tabernacle. \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tHe that is our God is the God of salvation; and unto GOD the Lord belong the issues from death.\tIssues belong to that God who saves \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd it shall come to pass in that day, that I will seek to destroy all the nations that come against Jerusalem.\tTo destroy all nations that opposed Jerusalem, \n',
 'bible_poetry.tsv\tNo Error\tNo Error\tAnd he brought in the priests and the Levites, and gathered them together into the east street,\tHe gathered priests and levitees in east lane. \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAgainst him came up Nebuchadnezzar king of Babylon, and bound him in fetters, to carry him to Babylon.\tAnd King Nebuchadnezzar bound him in fetters to bear. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThou shalt not consent unto him, nor hearken unto him; neither shall thine eye pity him, neither shalt thou spare, neither shalt thou conceal him:\tWould he consent not, heard not, pity nor hide your eye; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd, behold, thy cousin Elisabeth, she hath also conceived a son in her old age: and this is the sixth month with her, who was called barren.\tAnd old age, thy cousin Elisabeth also bowed \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tAfter that he is sold he may be redeemed again; one of his brethren may redeem him:\tAfter he was sold, perhaps again his brothers would redeem. \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tLove the brotherhood.\tThe brotherhood to love! and to love, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Moses said, Thus saith the LORD, About midnight will I go out into the midst of Egypt:\tAbout midnight I'll go to Egypt, \n",
 'bible_poetry.tsv\tIncomplete\tNo Error\tBy them shall the fowls of the heaven have their habitation, which sing among the branches.\tAnd birds sing among the branches, \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tThe lip of truth shall be established for ever: but a lying tongue is but for a moment.\tTruth established for ever--but a moment's lying tongue, \n",
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tBut the mercy of the LORD is from everlasting to everlasting upon them that fear him, and his righteousness unto children's children;\tBut God's mercy for ever, and His righteousness for children, \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tand who knoweth us?\tAnd who knows us? and who knows us well? \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd this have ye done again, covering the altar of the LORD with tears, with weeping, and with crying out, insomuch that he regardeth not the offering any more, or receiveth it with good will at your hand.\tDo this again, covering the altar with tears, or regard'd no offer anymore, or accepted. \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd there fell of Benjamin eighteen thousand men; all these were men of valour.\tBenjamin was a man of 18000, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tWherefore the sin of the young men was very great before the LORD: for men abhorred the offering of the LORD.\tSo, very great is the sin of young men, \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tWhoso findeth a wife findeth a good thing, and obtaineth favour of the LORD.\tWho finds a wife and gets a favour-- \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tHe that is void of wisdom despiseth his neighbour: but a man of understanding holdeth his peace.\tWisdomless he despises his neighbour, but understanding man holds \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd the heavens shall declare his righteousness: for God is judge himself.\tAnd mony a God shall judge him, \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tLet me be weighed in an even balance that God may know mine integrity.\tLet me even weighed in the balance to know my integrity-- \n',
 'bible_poetry.tsv\tNo Error\tIncorrect/New Information\tbut turn thee yet again, and thou shalt see greater abominations.\tBut, if yet thou turnest again, see greater abominables. \n',
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tFor Christ is the end of the law for righteousness to every one that believeth.\tChrist's end to all who believe in law! \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd Baasha king of Israel went up against Judah, and built Ramah, that he might not suffer any to go out or come in to Asa king of Judah.\tRamas, the king of Israel, built, nor could suffer \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tlet her be shut out from the camp seven days, and after that let her be received in again.\tLet her shut out of camp seven days and let again \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tHonour thy father and thy mother: that thy days may be long upon the land which the LORD thy God giveth thee.\tHonour your father and mother, so thy days may long \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tThou, O king, art a king of kings: for the God of heaven hath given thee a kingdom, power, and strength, and glory.\tGod gave thee kingdom, power, and glory; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tWherefore lay apart all filthiness and superfluity of naughtiness, and receive with meekness the engrafted word, which is able to save your souls.\tSo lay all needless filth and naughtiness apart, and receive meek words \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tPour out thy wrath upon the heathen that have not known thee, and upon the kingdoms that have not called upon thy name.\tPour wrath on thy known and thy kingdoms, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tshall they not both fall into the ditch?\tDo they not both fall into a ditch? \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tHe disappointeth the devices of the crafty, so that their hands cannot perform their enterprise.\tHe disappoints the crafty,--he cannot perform his duties. \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd the city was broken up, and all the men of war fled by night by the way of the gate between two walls, which is by the king's garden: (now the Chaldees were against the city round about:) and the king went the way toward the plain.\tThe city broke up and all combatant fled the gate between two walls, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor whosoever will save his life shall lose it: but whosoever will lose his life for my sake, the same shall save it.\tWho would save his life would lose his life, but none \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor this cause we also, since the day we heard it, do not cease to pray for you, and to desire that ye might be filled with the knowledge of his will in all wisdom and spiritual understanding;\tThis means we neer stop to pray you, and wish ye fill with his will-- \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tFor therefore we both labour and suffer reproach, because we trust in the living God, who is the Saviour of all men, specially of those that believe.\tWe trust the living God who saves all and those who believe, \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tFor thou shalt be in league with the stones of the field: and the beasts of the field shall be at peace with thee.\tThou art in league wi' the fields-stones, \n",
 'bible_poetry.tsv\tNo Error\tMeaning Change\tPour out thine indignation upon them, and let thy wrathful anger take hold of them.\tPour your indignation on them, and let thy wrathful anger take hold \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tIf a man be found stealing any of his brethren of the children of Israel, and maketh merchandise of him, or selleth him; then that thief shall die; and thou shalt put evil away from among you.\tIf any brother of thieves were found, \n',
 "bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tThe sons of Abraham; Isaac, and Ishmael.\tOf Abraham, Isaac, an' Hashmael; \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd when the Philistines heard the noise of the shout, they said, What meaneth the noise of this great shout in the camp of the Hebrews?\tWhat means this Filipino when he heard a mighty shout? \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tDo not think that I will accuse you to the Father: there is one that accuseth you, even Moses, in whom ye trust.\tThink not that I accuse thy Father, even of Mosses! \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd said unto the children of Israel, Thus saith the LORD God of Israel, I brought up Israel out of Egypt, and delivered you out of the hand of the Egyptians, and out of the hand of all kingdoms, and of them that oppressed you:\tI brought Israel out of Egypt and all its oppressed kingdoms. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd they sing the song of Moses the servant of God, and the song of the Lamb, saying, Great and marvellous are thy works, Lord God Almighty; just and true are thy ways, thou King of saints.\tThey sing their King's Almighty Moses, saying they are great and beautiful. \n",
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tIn the light of the king's countenance is life; and his favour is as a cloud of the latter rain.\tThe King's dwelling-place, the latest rain his favour; \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the spoiler shall come upon every city, and no city shall escape: the valley also shall perish, and the plain shall be destroyed, as the LORD hath spoken.\tFrom every city the spoiler comes, no city escapes, a valley is dead and a plain \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tPreach the word; be instant in season, out of season; reprove, rebuke, exhort with all longsuffering and doctrine.\tPreach the word,--no season,--rebuke,--exhort all with long and taught; \n',
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd they said unto him, Caesar's.\tThen there was the Csar, the Csar, \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tThen many of the Jews which came to Mary, and had seen the things which Jesus did, believed on him.\tAnd many a Jew then came to Mary, saw Jesus do, \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tLet the floods clap their hands: let the hills be joyful together\tLet their hands in floods, let the hills together rejoice: \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAccording to the days of thy coming out of the land of Egypt will I shew unto him marvellous things.\tI'm tauld ye're coming to Egypt, \n",
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tPraise the LORD, O Jerusalem; praise thy God, O Zion.\tPraise the Lord of Jerusalem! 'tis well done, \n",
 'bible_poetry.tsv\tNo Error\tIncorrect/New Information\tAnd he made ready his chariot, and took his people with him:\tHe was ready in his chariot, and he took his people \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd she made him sleep upon her knees; and she called for a man, and she caused him to shave off the seven locks of his head; and she began to afflict him, and his strength went from him.\tShe made him sleep at knees, called the man and shaved seven locks \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd all the evil of the men of Shechem did God render upon their heads: and upon them came the curse of Jotham the son of Jerubbaal.\tGod cursed Erubbaal's son, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAll the days wherein the plague shall be in him he shall be defiled; he is unclean: he shall dwell alone; without the camp shall his habitation be.\tDefiled, unclean, living alone, uncamp'd all day; \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd all the kings of the north, far and near, one with another, and all the kingdoms of the world, which are upon the face of the earth: and the king of Sheshach shall drink after them.\tAfter them, all kings Sheshach drank far and near, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tBut know this, that if the goodman of the house had known in what watch the thief would come, he would have watched, and would not have suffered his house to be broken up.\tBut know what thief watches and suffers not from his house broken, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThen went he down, and dipped himself seven times in Jordan, according to the saying of the man of God: and his flesh came again like unto the flesh of a little child, and he was clean.\tThen down he went, and in Jordan dipt seven times \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tBlessed be the God and Father of our Lord Jesus Christ, who hath blessed us with all spiritual blessings in heavenly places in Christ:\tGod and our Father Jesus blessed us in heavenly places. \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tand there is none upon earth that I desire beside thee.\tAnd bids me shun nought on earth but thee-- \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tSay ye not, A confederacy, to all them to whom this people shall say, A confederacy; neither fear ye their fear, nor be afraid.\tSay not of Confederacy, say not of them; and fear \n',
 "bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd they shall put my name upon the children of Israel, and I will bless them.\tThey'll put my name in mine, and bless him a'. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThe ancients of Gebal and the wise men thereof were in thee thy calkers: all the ships of the sea with their mariners were in thee to occupy thy merchandise.\tOn ships and mariners shalt thou occupy thy merchandise; \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tLo, let that night be solitary, let no joyful voice come therein.\tThat night lone, lo! no voice will come there, \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd thou shalt take fine flour, and bake twelve cakes thereof: two tenth deals shall be in one cake.\tTo take fine flour and bake twelve. If two deals were made, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd there was a cloud that overshadowed them: and a voice came out of the cloud, saying, This is my beloved Son: hear him.\tThe cloud overshadowed them, and came out their Son, who loved \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tFor it might have been sold for more than three hundred pence, and have been given to the poor.\tIt may be sold for more than three hundred pounds. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tCleanse your hands, ye sinners; and purify your hearts, ye double minded.\tClean thine hands, and purify thine hearts, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd she came to Jerusalem with a very great train, with camels that bare spices, and very much gold, and precious stones: and when she was come to Solomon, she communed with him of all that was in her heart.\tCame Jerusalem with very big train, and camels bare of spices, and very gold. \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd now, O God of Israel, let thy word, I pray thee, be verified, which thou spakest unto thy servant David my father.\tI pray the Father's word is verified, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the priest said unto them, Go in peace: before the LORD is your way wherein ye go.\tBefore the Lord go in peace on high; \n',
 "bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tAnd they marvelled all.\tAnd they were all amaz'd. But a little while \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tcare not for it: but if thou mayest be made free, use it rather.\tI care not for it--but if rather be free, use \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tFor I have not shunned to declare unto you all the counsel of God.\tI would not shun all God's counsel, \n",
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tNow Tobiah the Ammonite was by him, and he said, Even that which they build, if a fox go up, he shall even break down their stone wall.\tSays Tobiah the Ammonite--even if up the fox break their stone wall, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd they brought it.\tAnd there they brought it.--Ah, well a day, \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd he spake unto the children of Israel, saying, When your children shall ask their fathers in time to come, saying, What mean these stones?\tIn time thy children ask their fathers, saying: "What mean these stones? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the LORD said, Judah shall go up first.\tFor Judah was the first to go, \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Gedor, and Ahio, and Zacher.\tThe gedor, ahio, and zach'r, all in one, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd ye have respect to him that weareth the gay clothing, and say unto him, Sit thou here in a good place; and say to the poor, Stand thou there, or sit here under my footstool:\tPoor sits here, or under my footstool, thy respect, \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tThere was a certain creditor which had two debtors: the one owed five hundred pence, and the other fifty.\tOf debtors two--one--and one--for fifty pounds \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor they that are such serve not our Lord Jesus Christ, but their own belly; and by good words and fair speeches deceive the hearts of the simple.\tThey serve not our Lord Jesus Christ, and good words and speech deceive our simple hearts. \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tDedan, and Tema, and Buz, and all that are in the utmost corners,\tIn utmost corners, where Dedan, Tema, Buz, and all \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tBecause that which may be known of God is manifest in them; for God hath shewed it unto them.\tBecause God hath shown them that \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tAnd he made staves of shittim wood, and overlaid them with gold.\tHe made a shittim wood stave, and overlayed it gold. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd that ye will save alive my father, and my mother, and my brethren, and my sisters, and all that they have, and deliver our lives from death.\tSave father, mother, and all we have, and our lives, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd he departed thence, and entered into a certain man's house, named Justus, one that worshipped God, whose house joined hard to the synagogue.\tHe left, and entered Justus' house, which worshipped hard, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tIf ye will not hear, and if ye will not lay it to heart, to give glory unto my name, saith the LORD of hosts, I will even send a curse upon you, and I will curse your blessings: yea, I have cursed them already, because ye do not lay it to heart.\tSend even my curse--and if thou shouldst not give my name glory, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd thou shalt offer thy burnt offerings, the flesh and the blood, upon the altar of the LORD thy God: and the blood of thy sacrifices shall be poured out upon the altar of the LORD thy God, and thou shalt eat the flesh.\tOn the altar offer burnt sacrifices, flesh and eat, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tThen Joseph said unto the people, Behold, I have bought you this day and your land for Pharaoh: lo, here is seed for you, and ye shall sow the land.\tJoseph, I've bought this day and you'll land, Pharaoh! \n",
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tBehold, I waited for your words; I gave ear to your reasons, whilst ye searched out what to say.\tI waited for words from thee, listening reasons as thou search'st. \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAgain, David gathered together all the chosen men of Israel, thirty thousand.\tAgain David gathered thirty thousand chosen, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tZelek the Ammonite, Naharai the Berothite, the armourbearer of Joab the son of Zeruiah,\tThe ammonite Zelk, the berothite Naharai, \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tThou art fairer than the children of men: grace is poured into thy lips: therefore God hath blessed thee for ever.\tThan men's children. Grace pours from thy lips, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd it shall come to pass in the day that the LORD shall give thee rest from thy sorrow, and from thy fear, and from the hard bondage wherein thou wast made to serve,\tLord, give rest from thy sorrow, fear, hard bond, where thou made, \n',
 'bible_poetry.tsv\tNo Error\tIncorrect/New Information\tSo they weighed for my price thirty pieces of silver.\tThey weighed thirty pieces of silver my price, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tFor perhaps he therefore departed for a season, that thou shouldest receive him for ever;\tMay he for a season leave, thou wert for ever to see; \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd ye shall be holy men unto me: neither shall ye eat any flesh that is torn of beasts in the field; ye shall cast it to the dogs.\tThou holy Man! thou shall not eat the field-meat torn \n',
 "bible_poetry.tsv\tIncorrect/New Information\tNo Error\tHath he smitten him, as he smote those that smote him?\tHe's smitten by the wight that smote? \n",
 "bible_poetry.tsv\tIncomplete\tNo Error\tAnd when he had thus spoken, he took bread, and gave thanks to God in presence of them all: and when he had broken it, he began to eat.\tWhen he'd broken his bread he took and thanks the Lord. \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd king Solomon offered a sacrifice of twenty and two thousand oxen, and an hundred and twenty thousand sheep: so the king and all the people dedicated the house of God.\tThe King Solomon offered his thousand oxen and sheep, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the LORD sent Jerubbaal, and Bedan, and Jephthah, and Samuel, and delivered you out of the hand of your enemies on every side, and ye dwelled safe.\tLord sent him Jerebaal, Bedan, Jephthah, Samuel, and stay safe. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd they made two ouches of gold, and two gold rings; and put the two rings in the two ends of the breastplate.\tThey made two gold urns, and put two breast-plates-- \n',
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd the men of Judah said, Why are ye come up against us?\tWhy have you come up wi' us? \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tGilead is mine, and Manasseh is mine; Ephraim also is the strength of mine head; Judah is my lawgiver;\tMy Gilead, my Manasseh, and Ephraim also strong; \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tGo not to glean in another field, neither go from hence, but abide here fast by my maidens:\tGo not to another field, but go fast here; \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd Zechariah, and Aziel, and Shemiramoth, and Jehiel, and Unni, and Eliab, and Maaseiah, and Benaiah, with psalteries on Alamoth;\tZechariah, Aziel, Shemiramoth, Benaiah, and psalteries Alamoth. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tWho, when he was reviled, reviled not again; when he suffered, he threatened not; but committed himself to him that judgeth righteously:\tThreatened not while suffering, but committed \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tLet the day perish wherein I was born, and the night in which it was said, There is a man child conceived.\tLet my birth-day and night when man has said, \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd also Maachah his mother, even her he removed from being queen, because she had made an idol in a grove; and Asa destroyed her idol, and burnt it by the brook Kidron.\tAlso Makhah, mother removed from the grove, and burnt Asa's idol \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd he brought up Hadassah, that is, Esther, his uncle's daughter: for she had neither father nor mother, and the maid was fair and beautiful; whom Mordecai, when her father and mother were dead, took for his own daughter.\tHe brought up Hadassah, father and mother, beautiful maid and lady. \n",
 'bible_poetry.tsv\tIncorrect/New Information\tNo Error\tSo Joab the son of Zeruiah went first up, and was chief.\tFirst up went Bob, and as chief was he, \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tWho, when he had found one pearl of great price, went and sold all that he had, and bought it.\tWho went to sell one pearl at mighty price, when found \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThen Zedekiah the son of Chenaanah came near, and smote Micaiah upon the cheek, and said, Which way went the Spirit of the LORD from me to speak unto thee?\tThen came Zedekiah, son of Chenaanah, near, kissed Maicaiah\'s cheek, and said, "Ah, what! \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd ye shall be holy unto me: for I the LORD am holy, and have severed you from other people, that ye should be mine.\tI'm holy, and I will sépare you from other wight. \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tFrom the wicked that oppress me, from my deadly enemies, who compass me about.\tFrom those who oppress me, my deadly foes; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Moses gave the money of them that were redeemed unto Aaron and to his sons, according to the word of the LORD, as the LORD commanded Moses.\tMosses gave money to aaron and his sons, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tFrom that time forth came they no more on the sabbath.\tThe sabbath they were no more; and now \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThen Michaiah declared unto them all the words that he had heard, when Baruch read the book in the ears of the people.\tThen Michaiah declared all the words he heard as Baruch read the book, \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd, behold, all the men of Israel came to the king, and said unto the king, Why have our brethren the men of Judah stolen thee away, and have brought the king, and his household, and all David's men with him, over Jordan?\tWhy did the Jordanian steal our brothers and household? \n",
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd he that offered his offering the first day was Nahshon the son of Amminadab, of the tribe of Judah:\tThe first day Amminadab's son Nahshon offered \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the four and twenty elders, which sat before God on their seats, fell upon their faces, and worshipped God,\tFour elders fell upon their faces, and worshipped \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd in that day there shall be a root of Jesse, which shall stand for an ensign of the people; to it shall the Gentiles seek: and his rest shall be glorious.\tAnd Jesse's root was that day's chief-- \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd Jesus said, For judgment I am come into this world, that they which see not might see; and that they which see might be made blind.\t"Jesus!" said I, "I\'m come to judge those who see not \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tAnd they caught him, and beat him, and sent him away empty.\tThey caught him, beat him, and sent him empty away. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tNow the Philistines gathered together their armies to battle, and were gathered together at Shochoh, which belongeth to Judah, and pitched between Shochoh and Azekah, in Ephesdammim.\tPhilistine troops gathered at Judah's Shochoh, pitching between, \n",
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tBut I would ye should understand, brethren, that the things which happened unto me have fallen out rather unto the furtherance of the gospel;\tBut bid me understand my deeds are farther out than gospel. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tWhen the morning stars sang together, and all the sons of God shouted for joy?\tWhen morning stars sang together? \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tWherefore, if God so clothe the grass of the field, which to day is, and to morrow is cast into the oven, shall he not much more clothe you, O ye of little faith?\tIf God does not clothe you more, \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd they gathered their brethren, and sanctified themselves, and came, according to the commandment of the king, by the words of the LORD, to cleanse the house of the LORD.\tThey gathered their brothers, sanctified, and came in accordance with the King's command. \n",
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd the children of Heth answered Abraham, saying unto him,\t"Abraham!" answer\'d he, "your children, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tBut Noah found grace in the eyes of the LORD.\tBut ay the grace was found by Noah, \n',
 "bible_poetry.tsv\tMeaning Change\tMeaning Change\tHe that gathereth in summer is a wise son: but he that sleepeth in harvest is a son that causeth shame.\tThe summer gather'r wise, but a harvester sleeps his son. \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd they made bells of pure gold, and put the bells between the pomegranates upon the hem of the robe, round about between the pomegranates;\tThey made their pure gold bells, and put them round the pomegranates. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the princes of the Philistines were wroth with him; and the princes of the Philistines said unto him, Make this fellow return, that he may go again to his place which thou hast appointed him, and let him not go down with us to battle, lest in the battle he be an adversary to us: for wherewith should he reconcile himself unto his master?\tWhere should he with his master reconcile, \n',
 "bible_poetry.tsv\tNo Error\tIncorrect/New Information\tBut as for the mighty man, he had the earth; and the honourable man dwelt in it.\tBut mighty man had earth, and honour'd man lived there; \n",
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tHold thou me up, and I shall be safe: and I will have respect unto thy statutes continually.\tHold me up, safe, and my law continued respect. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tFrom Aroer, which is by the brink of the river of Arnon, and from the city that is by the river, even unto Gilead, there was not one city too strong for us: the LORD our God delivered all unto us:\tNot all cities are strong from Aroer, on the brink of a river; \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tOf the tribe of Nephthalim were sealed twelve thousand.\tAnd nephthalim was sealed twelve years ago. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tI will also stretch out mine hand upon Judah, and upon all the inhabitants of Jerusalem; and I will cut off the remnant of Baal from this place, and the name of the Chemarims with the priests;\tStretching my hand on Judah's remnant, and all Jerusalem's; \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tRemember thy servants, Abraham, Isaac, and Jacob; look not unto the stubbornness of this people, nor to their wickedness, nor to their sin:\tRemember thy servants--Abraham, Isaac, Jacob. \n',
 "bible_poetry.tsv\tNo Error\tNo Error\tNow, lo, if he beget a son, that seeth all his father's sins which he hath done, and considereth, and doeth not such like,\tIf he gets a son who saw all his father's sins, consider him not. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tEnvyings, murders, drunkenness, revellings, and such like: of the which I tell you before, as I have also told you in time past, that they which do such things shall not inherit the kingdom of God.\tI tell you, before, that they not inherit the kingdom of God. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tHe that abideth in the doctrine of Christ, he hath both the Father and the Son.\tThe Father and the Son of Christ, \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tBetter it is to be of an humble spirit with the lowly, than to divide the spoil with the proud.\tBetter than to divide the spoil from the proud; \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tDebate thy cause with thy neighbour himself; and discover not a secret to another:\tDebate cause with thy neighbour; and discover not secret. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the children of Israel said unto them, Would to God we had died by the hand of the LORD in the land of Egypt, when we sat by the flesh pots, and when we did eat bread to the full; for ye have brought us forth into this wilderness, to kill this whole assembly with hunger.\tAs Egypt we sat in flesh pots and ate full bread. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd when Paul was now about to open his mouth, Gallio said unto the Jews, If it were a matter of wrong or wicked lewdness, O ye Jews, reason would that I should bear with you:\t"If you have reason to bear, it\'s about wrong or evil," \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd the chief captain answered, With a great sum obtained I this freedom.\tAnd the chief captain answer\'d, "This is a lot\'s free, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Joshua sent men from Jericho to Ai, which is beside Bethaven, on the east of Bethel, and spake unto them, saying, Go up and view the country.\tAnd Joshua sent from Jericho to Ai, east of Bethaven. \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tTherefore I say unto you, What things soever ye desire, when ye pray, believe that ye receive them, and ye shall have them.\tTherefore, if thou believe'st receive, I say ye desires, \n",
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd they departed, and dwelt in the habitation of Chimham, which is by Bethlehem, to go to enter into Egypt,\tThey've left Chimham, bethlehem, to Egypt, \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tThen said Jesus unto him, Except ye see signs and wonders, ye will not believe.\tIf thou dost not believe, nor see signs and wonders, \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tNow these are the chief of the province that dwelt in Jerusalem: but in the cities of Judah dwelt every one in his possession in their cities, to wit, Israel, the priests, and the Levites, and the Nethinims, and the children of Solomon's servants.\tAll Israelis, priests, Dutch, and Jews dwell in Jerusalem; \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd he caused all that were present in Jerusalem and Benjamin to stand to it.\tSo all in Jerusalem and Benjamin stood, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd he said to them all, If any man will come after me, let him deny himself, and take up his cross daily, and follow me.\tDeny it, and take thy daily cross if any will follow me. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tBecause for thy sake I have borne reproach; shame hath covered my face.\tBecause shame covert my face so fair, \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tFor this city hath been to me as a provocation of mine anger and of my fury from the day that they built it even unto this day; that I should remove it from before my face,\tThis city's anger and anger caused, the day they built, to remove \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd Joseph said unto Pharaoh, The dream of Pharaoh is one: God hath shewed Pharaoh what he is about to do.\tThe Pharaoh dreamed that God would show him what he about to do. \n',
 "bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tJesus said, Take ye away the stone.\tAnd take the stone o'er the groat. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tBut I will punish you according to the fruit of your doings, saith the LORD: and I will kindle a fire in the forest thereof, and it shall devour all things round about it.\tBut I'll punish you, according your fruit \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Jehoiakim gave the silver and the gold to Pharaoh; but he taxed the land to give the money according to the commandment of Pharaoh: he exacted the silver and the gold of the people of the land, of every one according to his taxation, to give it unto Pharaohnechoh.\tJehoiakim gave palatine silver and gold, but taxed land to give \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tBut ye are come unto mount Sion, and unto the city of the living God, the heavenly Jerusalem, and to an innumerable company of angels,\tBut come from Mount Sinai and heaven's Jerusalem, \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd all the gold of the offering that they offered up to the LORD, of the captains of thousands, and of the captains of hundreds, was sixteen thousand seven hundred and fifty shekels.\tAll the gold they offered to thousand and hundreds, for 1600 shekels. \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tFear thou not; for I am with thee: be not dismayed; for I am thy God: I will strengthen thee; yea, I will help thee; yea, I will uphold thee with the right hand of my righteousness.\tFear not, fear not, for my GOD! I am \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tEven so it is not the will of your Father which is in heaven, that one of these little ones should perish.\tYet this little one thy Father's not willing to die. \n",
 'bible_poetry.tsv\tIncomplete\tNo Error\tAnd the sons of Hebron; Korah, and Tappuah, and Rekem, and Shema.\tHebron--Korah--Tapuah--Rekem--Shema-- \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tand where wroughtest thou?\tAnd wherefore will your feast be? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tSo all the elders of Israel came to the king to Hebron; and king David made a league with them in Hebron before the LORD: and they anointed David king over Israel.\tAll Israeli elders came to Hebron; David appoints \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tGod layeth up his iniquity for his children: he rewardeth him, and he shall know it.\tGod lay iniquity to his children, and rewards \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tMany will intreat the favour of the prince: and every man is a friend to him that giveth gifts.\tFor favour many a year, and every friend who gives gifts, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tIn the lips of him that hath understanding wisdom is found: but a rod is for the back of him that is void of understanding.\tHis lips with wisdom found, but the rod void, \n',
 "bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd that they may recover themselves out of the snare of the devil, who are taken captive by him at his will.\tCould recover them from the devil's willing trap, \n",
 "bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tLabour not to be rich: cease from thine own wisdom.\tThe labour-president's not so rich; \n",
 'bible_poetry.tsv\tIncorrect/New Information\tNo Error\tAgainst whom do ye sport yourselves?\tWhat sport thou art? What sport, thou art? \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tThe leprosy therefore of Naaman shall cleave unto thee, and unto thy seed for ever.\tSo Naaman's leprosy would forever cleave thy name and seed. \n",
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tBehold, the nations are as a drop of a bucket, and are counted as the small dust of the balance: behold, he taketh up the isles as a very little thing.\tSee nations like a bucket-drop, and counted the small dust in the balance. \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tNevertheless I am continually with thee: thou hast holden me by my right hand.\tYet continually thou held me in thy right hand; \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the altar of burnt offering with all his furniture, and the laver and his foot,\tThe altar of burnt offerings, and all his foot-rest \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tGreat is our Lord, and of great power: his understanding is infinite.\tThe God is great, and the Soul is great to understand. \n',
 'bible_poetry.tsv\tNo Error\tIncorrect/New Information\tThey send forth their little ones like a flock, and their children dance.\tThey send their little ones out like a flock, and their children dance \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tJesus therefore, knowing all things that should come upon him, went forth, and said unto them, Whom seek ye?\tSo Jesus went forth and said, "Whoe\'er shall seek thee, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tBe it known unto the king, that the Jews which came up from thee to us are come unto Jerusalem, building the rebellious and the bad city, and have set up the walls thereof, and joined the foundations.\tKept the Jewess who came to Jerusalem, bad rebellious building, foundations joined, \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tAnd when the people were come into the camp, the elders of Israel said, Wherefore hath the LORD smitten us to day before the Philistines?\tElders of Israel said, God hit us a day before the Philistines. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd they sent a messenger unto Joseph, saying, Thy father did command before he died, saying,\tSaying, "Joseph\'s father command, before he died." \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd the young man that told him said, As I happened by chance upon mount Gilboa, behold, Saul leaned upon his spear; and, lo, the chariots and horsemen followed hard after him.\tSaul lean'd his spear upon Gilboa's mountain; car and horse hard followed; \n",
 "bible_poetry.tsv\tNo Error\tMeaning Change\tSaying, Surely blessing I will bless thee, and multiplying I will multiply thee.\tI'm sure I'll bless and multiply thee; \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tThou hast covered with anger, and persecuted us: thou hast slain, thou hast not pitied.\tCover'd thy anger, and persecuted us, \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Jesus entered and passed through Jericho.\tJesus entered Jerusalem, and passed through \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tThen thou shalt say, They be thy servant Jacob's; it is a present sent unto my lord Esau: and, behold, also he is behind us.\tSay, Jacob, thy servant sends present, thy lord; \n",
 "bible_poetry.tsv\tNo Error\tIncomplete\tThat it may be well with thee, and thou mayest live long on the earth.\tThat thou may'st long live on earth, \n",
 "bible_poetry.tsv\tNo Error\tIncomplete\tAnd if a woman shall put away her husband, and be married to another, she committeth adultery.\tA woman commit'd adultery, and left her husband and married. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tWhen thou shalt hearken to the voice of the LORD thy God, to keep all his commandments which I command thee this day, to do that which is right in the eyes of the LORD thy God.\tWhen God's voice I heard, would do all thou command this day. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor thus hath the LORD said unto me, Go, set a watchman, let him declare what he seeth.\tSo Lord, go, set watchman, let declare what ye see, \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd they said unto him, Yesterday at the seventh hour the fever left him.\tA fever left him frae e'en to morn, \n",
 'bible_poetry.tsv\tNo Error\tIncomplete\tSo when this was done, others also, which had diseases in the island, came, and were healed:\tAnd others who had diseases of the island came also and healed; \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tBut it came to pass within a while after, in the time of wheat harvest, that Samson visited his wife with a kid; and he said, I will go in to my wife into the chamber.\tBut Samson visited the wife with the kid, up to the day \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tI am Alpha and Omega, the beginning and the ending, saith the Lord, which is, and which was, and which is to come, the Almighty.\tI am of the beginning and end, Alpha and Omega-- \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd the children of Israel returned from chasing after the Philistines, and they spoiled their tents.\tThey returned to chase the Philistines, and their tents were ruined. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tBehold, I will send for many fishers, saith the LORD, and they shall fish them; and after will I send for many hunters, and they shall hunt them from every mountain, and from every hill, and out of the holes of the rocks.\tI send the fisher there, and hunt from every mountain and hill; \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tAnd they understood none of these things: and this saying was hid from them, neither knew they the things which were spoken.\tThey understood not these sayings, and they hid \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tBlessed is the man whose strength is in thee; in whose heart are the ways of them.\tBless the man that's strong in thy heart, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tThou wilt perform the truth to Jacob, and the mercy to Abraham, which thou hast sworn unto our fathers from the days of old.\tTo perform Jacob's truancy and Abraham's mercy from ages; \n",
 "bible_poetry.tsv\tIncomplete\tNo Error\tThese are also proverbs of Solomon, which the men of Hezekiah king of Judah copied out.\tAnd also did Solomon's proverbs copy Judah's king. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the children of Lotan were Hori and Hemam; and Lotan\'s sister was Timna.\t"Hori and Hemam were Lothian children and sister; \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tBut these are they of which ye shall not eat: the eagle, and the ossifrage, and the ospray,\tBut eat not the eagle, ossifrage, and spray, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAll these were under the hands of their father for song in the house of the LORD, with cymbals, psalteries, and harps, for the service of the house of God, according to the king's order to Asaph, Jeduthun, and Heman.\tAll in father's hands--cymbals, psalterys, and harps--for song the king orders; \n",
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd they said, Seven, and a few little fishes.\tAnd seven little fishes, that strew \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd it came to pass, as they were much perplexed thereabout, behold, two men stood by them in shining garments:\tTwa shining mense stood by them much in confusion, \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAt that day shall a man look to his Maker, and his eyes shall have respect to the Holy One of Israel.\tMan's eyes that day at Maker's respect, one holy Israeli \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd he shall cut it into his pieces, with his head and his fat: and the priest shall lay them in order on the wood that is on the fire which is upon the altar:\tAnd the priest cut head and fat to his pieces and lay on the altar wood. \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tAnd afterward I will bring again the captivity of the children of Ammon, saith the LORD.\tThen back to captivity, O I shall say, \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tSaying, God hath forsaken him: persecute and take him; for there is none to deliver him.\tSaying, God will abandon him, persecute and take \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd the waters prevailed exceedingly upon the earth; and all the high hills, that were under the whole heaven, were covered.\tThe waters ruled extrême, and all the hills were covered high; \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tTherefore the Jews sought the more to kill him, because he not only had broken the sabbath, but said also that God was his Father, making himself equal with God.\tSince he had broken the sabbath, and said his Father also wanted to kill. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tThen the congregation shall judge between the slayer and the revenger of blood according to these judgments:\tCongregation will judge between the slain and revenge, according \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd thou shalt put it under the compass of the altar beneath, that the net may be even to the midst of the altar.\tAnd thou hast put a net beneath the altar. \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd ye shall give her unto Eleazar the priest, that he may bring her forth without the camp, and one shall slay her before his face:\tWould give her to Eleazar to bring without, and one to slay before her face. \n',
 'bible_poetry.tsv\tNo Error\tIncomplete\tAnd when he had declared all these things unto them, he sent them to Joppa.\tAnd when all was declared he sent them to Joppa, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd they tied unto it a lace of blue, to fasten it on high upon the mitre; as the LORD commanded Moses.\tAnd tangled the mitre in blue lace to fasten as Mose ordered. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the other issued out of the city against them; so they were in the midst of Israel, some on this side, and some on that side: and they smote them, so that they let none of them remain or escape.\tThey're in Israel, some on this side are slain, so let none remain or escape. \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd of the sons of Elam; Mattaniah, Zechariah, and Jehiel, and Abdi, and Jeremoth, and Eliah.\tOf Mattaniah, Zachariah, Abdi, and Jeremoth. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor the head of Syria is Damascus, and the head of Damascus is Rezin; and within threescore and five years shall Ephraim be broken, that it be not a people.\tDamascus, the Capital, and Rezin, after three years, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor his sons had seen what way the man of God went, which came from Judah.\tHis sons had seen how God went, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tthis is nothing else but sorrow of heart.\tAnd this is but the saddest of all. \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd thy estimation shall be of the male from twenty years old even unto sixty years old, even thy estimation shall be fifty shekels of silver, after the shekel of the sanctuary.\tEven fifty shekels o'er one male aged twenty-six. \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tFor when ye offer your gifts, when ye make your sons to pass through the fire, ye pollute yourselves with all your idols, even unto this day: and shall I be enquired of by you, O house of Israel?\tWhen offering gifts, and making sons pass through the fire, pollute all \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tWilt not thou, O God, which hadst cast us off?\tAnd did ae God cast us off?--Ah, well-a-day, \n',
 "bible_poetry.tsv\tMeaning Change\tMeaning Change\tSo I gave them up unto their own hearts' lust: and they walked in their own counsels.\tI yielded to their heart-lust, they walk'd in counsel, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tTherefore the LORD was very angry with Israel, and removed them out of his sight: there was none left but the tribe of Judah only.\tThus God's very wrath on Israel removed from his sight, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd take your father and your households, and come unto me: and I will give you the good of the land of Egypt, and ye shall eat the fat of the land.\tTake your father and your households, come I'll give you Elysian fat; \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tPut on therefore, as the elect of God, holy and beloved, bowels of mercies, kindness, humbleness of mind, meekness, longsuffering;\tGod holy and beloved, generous, kind, humble, mind--meek, long; \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tThe Jews then murmured at him, because he said, I am the bread which came down from heaven.\tThen the jewish laughed at him, because he had said he was bread, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tFor my people have committed two evils; they have forsaken me the fountain of living waters, and hewed them out cisterns, broken cisterns, that can hold no water.\tTwo evils, o'er abandoned living waters, erect broken cisterns that can not hold \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThe poor and the deceitful man meet together: the LORD lighteneth both their eyes.\tThe poor meet the deceiving man together, \n',
 'bible_poetry.tsv\tNo Error\tNo Error\tThere brake he the arrows of the bow, the shield, and the sword, and the battle.\tThe bow, shield, and sword brake the battle, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the burnt offering that the prince shall offer unto the LORD in the sabbath day shall be six lambs without blemish, and a ram without blemish.\tSix blemished lambs, and burnt rams, on sabbath day, \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tFor the transgression of Jacob is all this, and for the sins of the house of Israel.\tAnd Jacob's sins were all his own. \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Jahath was the chief, and Zizah the second: but Jeush and Beriah had not many sons; therefore they were in one reckoning, according to their father's house.\tWhile Jahath and Zizah had many sons, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Harbonah, one of the chamberlains, said before the king, Behold also, the gallows fifty cubits high, which Haman had made for Mordecai, who spoken good for the king, standeth in the house of Haman.\t"One good-speak\'d Harbonah, king\'s 50-cubit high gallows, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd I will take away his blood out of his mouth, and his abominations from between his teeth: but he that remaineth, even he, shall be for our God, and he shall be as a governor in Judah, and Ekron as a Jebusite.\tHis blood, and blasted between his teeth: but Israel's governor and Ekron's governor \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd therefore did the Jews persecute Jesus, and sought to slay him, because he had done these things on the sabbath day.\tPersecuted Jesus, and wreat this Sabbath day, \n',
 "bible_poetry.tsv\tNo Error\tIncomplete\tSeven years old was Jehoash when he began to reign.\tA seven-year's Jehoash, when he began to rule, \n",
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tIf he beget a son that is a robber, a shedder of blood, and that doeth the like to any one of these things,\tIf he gets the robber's blood-shedding son, and any of these things. \n",
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd it came to pass, when he had made an end of speaking unto Saul, that the soul of Jonathan was knit with the soul of David, and Jonathan loved him as his own soul.\tJonathan's soul was knit with Saul's, and loved him like him. \n",
 'bible_poetry.tsv\tIncorrect/New Information\tNo Error\tJarmuth, and Adullam, Socoh, and Azekah,\tOf Armuth, Abullam, Socoh, and Azekah. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tTherefore it is no great thing if his ministers also be transformed as the ministers of righteousness; whose end shall be according to their works.\tIf his minstrels were also transformed great, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd hath made us kings and priests unto God and his Father; to him be glory and dominion for ever and ever.\tHe made us kings and priests,--God and Father. \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tAnd the dogs shall eat Jezebel in the portion of Jezreel, and there shall be none to bury her.\tThe dogs will eat and bury the jazebel portion; \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tI will arise and go to my father, and will say unto him, Father, I have sinned against heaven, and before thee,\tI rise, and go, my father, and say, I have sinn'd heaven \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd David gathered all Israel together to Jerusalem, to bring up the ark of the LORD unto his place, which he had prepared for it.\tDavid gathered all his neighbors in Jerusalem to bring an ark \n',
 'bible_poetry.tsv\tIncorrect/New Information\tNo Error\tAnd he said, Which way shall we go up?\t"Up! where\'er we go,\'er we\'ll hither, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tBut the miry places thereof and the marishes thereof shall not be healed; they shall be given to salt.\tBut miry places and marishes unhealed \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tFor the law of the Spirit of life in Christ Jesus hath made me free from the law of sin and death.\tJesus' life-law I'm free from death's sin-law, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tNow these are the words of the letter that Jeremiah the prophet sent from Jerusalem unto the residue of the elders which were carried away captives, and to the priests, and to the prophets, and to all the people whom Nebuchadnezzar had carried away captive from Jerusalem to Babylon;\tThe prophet\'s letter sent from Jerusalem declares: "All, \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tIsrael was holiness unto the LORD, and the firstfruits of his increase: all that devour him shall offend; evil shall come upon them, saith the LORD.\tHoly is Israel, its first-fruits increase, and all who devour \n',
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tEven so, Amen.\tAn' tho' a' that, amen! a' that, \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tlet us eat and drink; for to morrow we die.\tO let us eat and drink the dews, \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tThey shall run like mighty men; they shall climb the wall like men of war; and they shall march every one on his ways, and they shall not break their ranks:\tRun like mighty men, climb like war-men, march every step, nor break their ranks; \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tAs a dog returneth to his vomit, so a fool returneth to his folly.\tThe fool returns vomit like a dog to return; \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tIn my Father's house are many mansions: if it were not so, I would have told you.\tMansions many, many as my Father's house. If it is, tell me not. \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThese are the families of the Zebulunites according to those that were numbered of them, threescore thousand and five hundred.\t"Ae Zebulunites, three thousand as many," \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAlso in time past, when Saul was king over us, thou wast he that leddest out and broughtest in Israel: and the LORD said to thee, Thou shalt feed my people Israel, and thou shalt be a captain over Israel.\tAnd Saul led out and brought forth Israel past \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tTherefore the Jews of the villages, that dwelt in the unwalled towns, made the fourteenth day of the month Adar a day of gladness and feasting, and a good day, and of sending portions one to another.\tThe Jewess made his fourteenth Adar-day, a day of gladness and feast. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThis people draweth nigh unto me with their mouth, and honoureth me with their lips; but their heart is far from me.\tThis draws me mouth, and honours me far away; \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd I give unto them eternal life; and they shall never perish, neither shall any man pluck them out of my hand.\tI give them life for ever--they never die--anyone picks them out, \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tA man of great wrath shall suffer punishment: for if thou deliver him, yet thou must do it again.\tGreat wrath shall suffer punishment; though it must do again. \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tThe Jews answered him, We have a law, and by our law he ought to die, because he made himself the Son of God.\tWe have law, and should he die, because he made a Son. \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd he said unto them, What manner of communications are these that ye have one to another, as ye walk, and are sad?\tHow would ye communicate with another, as ye walk and mourn. \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tMoreover Jeremiah said unto king Zedekiah, What have I offended against thee, or against thy servants, or against this people, that ye have put me in prison?\tAn' Jeremiah, wha offended thy servant or this king? \n",
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tHowbeit he refused to turn aside: wherefore Abner with the hinder end of the spear smote him under the fifth rib, that the spear came out behind him; and he fell down there, and died in the same place: and it came to pass, that as many as came to the place where Asahel fell down and died stood still.\tRefused to turn aside, with spear-end hinder'd, Asahel fell, \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tRighteous art thou, O LORD, and upright are thy judgments.\tThou art right and upright, and upright; \n',
 "bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tShould it be according to thy mind?\tShould it be, to thy mind's conformity, \n",
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tAnd the LORD said unto him, Go up.\tGo up, up! and see how far the wind is blowing. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAn altar of earth thou shalt make unto me, and shalt sacrifice thereon thy burnt offerings, and thy peace offerings, thy sheep, and thine oxen: in all places where I record my name I will come unto thee, and I will bless thee.\tMake earthly altars, sacrifice all thy burnt offerings, sheep and oxen, \n',
 'bible_poetry.tsv\tIncomplete\tNo Error\tThen David gave to Solomon his son the pattern of the porch, and of the houses thereof, and of the treasuries thereof, and of the upper chambers thereof, and of the inner parlours thereof, and of the place of the mercy seat,\tThen David gave his son Solomon a pattern of porches, houses, upper and inner chambers, \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tThis is the inheritance of the tribe of the children of Dan according to their families, these cities with their villages.\tThese cities Dan's fam'd inherits, \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd the people answered him not a word.\tAnd no one answered him by the word, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd five of you shall chase an hundred, and an hundred of you shall put ten thousand to flight: and your enemies shall fall before you by the sword.\tFive of you will chase hundred, and put ten thousand foes in flight. \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tFor it is written, He taketh the wise in their own craftiness.\tHe takes the wise o' their craft, \n",
 'bible_poetry.tsv\tIncomplete\tNo Error\tThe LORD hath made all things for himself: yea, even the wicked for the day of evil.\tFor the Lord made all things for him. \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tA man that is an heretick after the first and second admonition reject;\tThe heretick o' guy, who first rejected admonition, \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tI Paul have written it with mine own hand, I will repay it: albeit I do not say to thee how thou owest unto me even thine own self besides.\tI'll repay it to Paul, though thou dost not say \n",
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tfor had there not been now a much greater slaughter among the Philistines?\tWas not the Philistines slain much now, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd cried when they saw the smoke of her burning, saying, What city is like unto this great city!\tThey cried, and said, "A city like?" when she saw \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tA good man sheweth favour, and lendeth: he will guide his affairs with discretion.\tThe good man gave favours, lends, and guides his affairs with discretion. \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tfor my soul is wearied because of murderers.\tAs murderers cause my weary soul \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tIn the day when the keepers of the house shall tremble, and the strong men shall bow themselves, and the grinders cease because they are few, and those that look out of the windows be darkened,\tWhen keepers tremble, grinders bow, less ceased, those looking out the windows darken, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tand having ears, hear ye not?\tAnd have ye been sae sae having ears? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the great court round about was with three rows of hewed stones, and a row of cedar beams, both for the inner court of the house of the LORD, and for the porch of the house.\tA great court, round three honed stones and one row of cedar beams. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnathoth with her suburbs, and Almon with her suburbs; four cities.\tAtthoth and Almon were four, \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd called, and asked whether Simon, which was surnamed Peter, were lodged there.\tAnd called, and asked if Peter's Simon was there, \n",
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd the Sabeans fell upon them, and took them away; yea, they have slain the servants with the edge of the sword; and I only am escaped alone to tell thee.\tThe Sabberian slain his servants with sword, and only escape to tell. \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tTherefore rejoice, ye heavens, and ye that dwell in them.\tSo may rejoice thy Heavens, and live \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tMoreover the LORD will also deliver Israel with thee into the hand of the Philistines: and to morrow shalt thou and thy sons be with me: the LORD also shall deliver the host of Israel into the hand of the Philistines.\tAnd also the Lord delivered with the Philistines' hand: \n",
 'bible_poetry.tsv\tIncorrect/New Information\tNo Error\tI love the LORD, because he hath heard my voice and my supplications.\tI love the Lord because he heard my voice and my pretences. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAn unjust man is an abomination to the just: and he that is upright in the way is abomination to the wicked.\tFor unjust men are abominable; \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd every earthen vessel, whereinto any of them falleth, whatsoever is in it shall be unclean; and ye shall break it.\tAnd every vessel on earth was clean, and thou didst break \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Solomon brought in the things which David his father had dedicated; even the silver, and the gold, and the vessels, did he put among the treasures of the house of the LORD.\tSolomon brought such as silver, gold, and vessels dedicated to David. \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tBe ye ashamed, O ye husbandmen; howl, O ye vinedressers, for the wheat and for the barley; because the harvest of the field is perished.\tShame on thee, howl for the crops to die; \n',
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tThe eye also of the adulterer waiteth for the twilight, saying, No eye shall see me: and disguiseth his face.\tAlso waiting the adult's face with twinkling rays,-- \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd they brake down the image of Baal, and brake down the house of Baal, and made it a draught house unto this day.\tThe Baal's image they brake down, \n",
 "bible_poetry.tsv\tIncomplete\tNo Error\tWhosoever committeth sin transgresseth also the law: for sin is the transgression of the law.\tBy sinners' sins the law is violated, \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tSaying unto them, Go into the village over against you, and straightway ye shall find an ass tied, and a colt with her: loose them, and bring them unto me.\tGo over the village, and straight find the tied ass and colt with her. \n',
 "bible_poetry.tsv\tIncomplete\tNo Error\tBut in the seventh year shall be a sabbath of rest unto the land, a sabbath for the LORD: thou shalt neither sow thy field, nor prune thy vineyard.\tThe seventh sabbath for land: ye'll neither sow nor prune your vineyard; \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThen said I unto them, Ye see the distress that we are in, how Jerusalem lieth waste, and the gates thereof are burned with fire: come, and let us build up the wall of Jerusalem, that we be no more a reproach.\tYe see our distress, and Jerusalem and her gates burn. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Simon and they that were with him followed after him.\tAnd Simon followed, and they were all \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd unleavened bread, and cakes unleavened tempered with oil, and wafers unleavened anointed with oil: of wheaten flour shalt thou make them.\tMake leaven bread, nor oil-tempered cakes, nor leaven wafers coated, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tSo Jonathan arose from the table in fierce anger, and did eat no meat the second day of the month: for he was grieved for David, because his father had done him shame.\tThan Jonathan uprose at the table in fierce anger, no meat the second day of May, \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tHe that hath received his testimony hath set to his seal that God is true.\tAnd put him a seal o' God's truth, \n",
 "bible_poetry.tsv\tIncorrect/New Information\tNo Error\tThat ye shall say, It is the sacrifice of the LORD's passover, who passed over the houses of the children of Israel in Egypt, when he smote the Egyptians, and delivered our houses.\tSay, God is the sacrifice when Elysian slain and delivered our houses. \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tBecause of the savour of thy good ointments thy name is as ointment poured forth, therefore do the virgins love thee.\tThy virgin love virgins, by thy good ointments name, \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThere went with us also certain of the disciples of Caesarea, and brought with them one Mnason of Cyprus, an old disciple, with whom we should lodge.\tThey also went to the Csar's, and brought old Cyprus disciple Mnason. \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tSurely thou wilt slay the wicked, O God: depart from me therefore, ye bloody men.\t"God, surely thou wilt kill evil;" \n',
 'bible_poetry.tsv\tNo Error\tMeaning Change\tJesus answered and said unto them, I have done one work, and ye all marvel.\tJesus answered, said he had done one labour, and all were amazed. \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tWhy dost thou strive against him?\t"Why try\'st thou against him?" \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd Moses did as the LORD commanded: and they went up into mount Hor in the sight of all the congregation.\tMestrels did the Lord command, on Mount Hor, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tThis shall be thine of the most holy things, reserved from the fire: every oblation of theirs, every meat offering of theirs, and every sin offering of theirs, and every trespass offering of theirs which they shall render unto me, shall be most holy for thee and for thy sons.\tFor every obstruction, every meat--and holy are thy sons-- \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the sons of Izhar; Korah, and Nepheg, and Zichri.\tIzhar, Korah, Nepheg, and Zichri, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd they removed from Jotbathah, and encamped at Ebronah.\tThey removed from Jotbathah and Ebronah dwelt; \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tBut tidings out of the east and out of the north shall trouble him: therefore he shall go forth with great fury to destroy, and utterly to make away many.\tBut tidings from east and north trouble him, many a destroy, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Pharaoh called unto Moses, and said, Go ye, serve the LORD; only let your flocks and your herds be stayed: let your little ones also go with you.\tPoses called him "Serve, but let your flocks and herds \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tNow the works of the flesh are manifest, which are these; Adultery, fornication, uncleanness, lasciviousness,\tAdultery, fornication, unclean, lascivious, \n',
 "bible_poetry.tsv\tMeaning Change\tNo Error\tThus Jeremiah remained in the court of the prison.\tSo in Job's prison Jerry's remained, \n",
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tPeter answering said, The Christ of God.\tThe answerer was God Petrarch, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tonly let us consent unto them, and they will dwell with us.\tLet them only accord, and live with us; \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncomplete\thath he not sent me to the men that sit upon the wall, that they may eat their own dung, and drink their own piss with you?\tHe wont tell you if men who sit on the wall can eat their dung and drink their piss, \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tFor thy name's sake, O LORD, pardon mine iniquity; for it is great.\tMy infidelities! pardon them a', Sir! \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor the seller shall not return to that which is sold, although they were yet alive: for the vision is touching the whole multitude thereof, which shall not return; neither shall any strengthen himself in the iniquity of his life.\tNot to the seller return, though still lives, not touching sight; \n',
 "bible_poetry.tsv\tMeaning Change\tMeaning Change\tJudah was his sanctuary, and Israel his dominion.\tJudah's sanctuary, and Israel's reign; \n",
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd it came to pass, as he drew back his hand, that, behold, his brother came out: and she said, How hast thou broken forth?\tWhen he drew back his brother out, and said: "How did he break? \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tMy bowels, my bowels!\tMy bowels! thou shalt see, that in thy sight \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tTherefore every one that eateth it shall bear his iniquity, because he hath profaned the hallowed thing of the LORD: and that soul shall be cut off from among his people.\tSince every man who ate it profess'd his hallowed sin, \n",
 'bible_poetry.tsv\tIncomplete\tNo Error\tBut God giveth it a body as it hath pleased him, and to every seed his own body.\tBut God gives it as body and every seed-- \n',
 "bible_poetry.tsv\tIncomplete\tNo Error\tKerioth is taken, and the strong holds are surprised, and the mighty men's hearts in Moab at that day shall be as the heart of a woman in her pangs.\tWas taken by Kerioth, and astonied strong holds, big men's hearts that day, \n",
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tIniquities prevail against me: as for our transgressions, thou shalt purge them away.\tInjustice prevail'd on me, ye purge our transgressions; \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tHamath, Berothah, Sibraim, which is between the border of Damascus and the border of Hamath; Hazarhatticon, which is by the coast of Hauran.\tFrom Hamas, Berothah, and Sibraim, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd it came to pass also on another sabbath, that he entered into the synagogue and taught: and there was a man whose right hand was withered.\tAlso on another sabbath he entered and taught \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd I have given you a land for which ye did not labour, and cities which ye built not, and ye dwell in them; of the vineyards and oliveyards which ye planted not do ye eat.\tI've given you land to labour not, cities built not, vineyards and olive-farms, \n",
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tThe burden of the desert of the sea.\tThe burden of a desert: and so it was, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tFor thou hadst cast me into the deep, in the midst of the seas; and the floods compassed me about: all thy billows and thy waves passed over me.\tThe floods piled me up; thy billows and waves all passed over \n',
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd the king said, What have I to do with you, ye sons of Zeruiah?\t"Zeruiah! what have I to do with you? \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tReturn, ye backsliding children, and I will heal your backslidings.\tReturn, ye backsliding children, and heal \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tThen came to him the mother of Zebedees children with her sons, worshipping him, and desiring a certain thing of him.\tThen Zebedee mother worshiping him, and wan, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd, behold, as Barak pursued Sisera, Jael came out to meet him, and said unto him, Come, and I will shew thee the man whom thou seekest.\tWhen Barak pursued, Jamie came out to meet Sisera and told \n',
 "bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tTherefore say, Thus saith the Lord GOD; Although I have cast them far off among the heathen, and although I have scattered them among the countries, yet will I be to them as a little sanctuary in the countries where they shall come.\tIn little reserv'd countries where I come, yet I have scattered \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd he saith unto the man which had the withered hand, Stand forth.\tHe spake, "Stand, thou withered hand, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\thath thy soul lothed Zion?\tZION! didst thou lott thee with thy hame, \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd he made the incense altar of shittim wood: the length of it was a cubit, and the breadth of it a cubit; it was foursquare; and two cubits was the height of it; the horns thereof were of the same.\tMade a shittim wood altar incense--long, and two-cubit tall. \n',
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tIn the twilight, in the evening, in the black and dark night:\tAnd in the black and dark night \n',
 "bible_poetry.tsv\tNo Error\tMeaning Change\tAnd I will also take of them for priests and for Levites, saith the LORD.\tI'll also take them o'er priests and Leviticus, \n",
 'bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd beheld among the simple ones, I discerned among the youths, a young man void of understanding,\tI saw a young unintelligible man among simple ones. \n',
 'bible_poetry.tsv\tNo Error\tNo Error\tAnd ye shall know the truth, and the truth shall make you free.\tKnow the truth, and make thee free. \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAll that ever came before me are thieves and robbers: but the sheep did not hear them.\tAll who came ever before me not hear from sheep, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tAnd didst see the affliction of our fathers in Egypt, and heardest their cry by the Red sea;\tOur fathers in Egypt afflicted, and hear the red Sea cry, \n',
 'bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\tand a strange punishment to the workers of iniquity?\tStrange punishment for the labourer? \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd saying, Alas, alas that great city, that was clothed in fine linen, and purple, and scarlet, and decked with gold, and precious stones, and pearls!\tAlas! that great city clad in fine linen, purple and scarlet, and deck'd \n",
 "bible_poetry.tsv\tIncomplete\tNo Error\tAnd the rough goat is the king of Grecia: and the great horn that is between his eyes is the first king.\tThe rough goat o'er the king of Greece \n",
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd when ye spread forth your hands, I will hide mine eyes from you: yea, when ye make many prayers, I will not hear: your hands are full of blood.\tI'll hide thine eyes, while thy many prayers \n",
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tFor thine arrows stick fast in me, and thy hand presseth me sore.\tThy arrows stick fast on me, and bad pressure \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tTherefore, behold, the days come, saith the LORD, that it shall no more be called Tophet, nor the valley of the son of Hinnom, but the valley of slaughter: for they shall bury in Tophet, till there be no place.\tNot called Tophet, but valley of Hinnom, \n',
 "bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tAnd Saul took him that day, and would let him go no more home to his father's house.\tSaul took him that day, and let his father go no more; \n",
 'bible_poetry.tsv\tIncorrect/New Information\tMeaning Change\tand to what are they like?\tAnd what are they like to scud themsels? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd Zelah, Eleph, and Jebusi, which is Jerusalem, Gibeath, and Kirjath; fourteen cities with their villages.\tOf fourteen, including Jerusalem, Gibrah and Kirjath. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd, behold, men passed by, and saw the carcase cast in the way, and the lion standing by the carcase: and they came and told it in the city where the old prophet dwelt.\tMen passed the carcass, saw the lion standing by, and came old Prophet's city. \n",
 "bible_poetry.tsv\tIncorrect/New Information\tIncorrect/New Information\thave ye not heard?\tHeard'st thou?--Awake! awake! and awake! \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd after he had spent some time there, he departed, and went over all the country of Galatia and Phrygia in order, strengthening all the disciples.\tAnd left after some time there, and all Galaxia and Phrygia strengthened. \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tUntil the day break, and the shadows flee away, I will get me to the mountain of myrrh, and to the hill of frankincense.\tTill day is broken and shadows flee, mountain myrrh! \n',
 "bible_poetry.tsv\tIncomplete\tMeaning Change\tAnd in their hands they shall bear thee up, lest at any time thou dash thy foot against a stone.\tIn thy hands, at any time dash'd to a stone, \n",
 'bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd when he cometh home, he calleth together his friends and neighbours, saying unto them, Rejoice with me; for I have found my sheep which was lost.\tCalls his friends and neighbours together when they come home to find their lost sheep. \n',
 'bible_poetry.tsv\tMeaning Change\tNo Error\tHast thou an arm like God?\tHast thou a Godlike arm as thou? \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tUntil I come and take you away to a land like your own land, a land of corn and wine, a land of bread and vineyards, a land of oil olive and of honey, that ye may live, and not die: and hearken not unto Hezekiah, when he persuadeth you, saying, The LORD will deliver us.\tUntil I come and take you to land like ye, wine, bread, vineyard, honey, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tBlessed is the man that feareth the LORD, that delighteth greatly in his commandments.\tBless those who fear, who great delight their commands, \n',
 'bible_poetry.tsv\tNo Error\tIncorrect/New Information\tAnd upon all the ships of Tarshish, and upon all pleasant pictures.\tOf tartish ships, and all the pleasant pictures \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tWhen they were filled, he said unto his disciples, Gather up the fragments that remain, that nothing be lost.\tWhen full his disciples said, gather fragments remaining to lose nothing. \n',
 'bible_poetry.tsv\tMeaning Change\tIncorrect/New Information\tYet a little sleep, a little slumber, a little folding of the hands to sleep:\tYet little sleep, little slumber, little hands to fold, \n',
 'bible_poetry.tsv\tIncomplete\tIncorrect/New Information\tAnd those that are to be redeemed from a month old shalt thou redeem, according to thine estimation, for the money of five shekels, after the shekel of the sanctuary, which is twenty gerahs.\tYour estimate says, those months redeem five shekels, \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tNeither shalt thou steal.\tNae mair thou shalt steal--thou shalt steal-- \n',
 'bible_poetry.tsv\tIncomplete\tIncomplete\tTherefore their goods shall become a booty, and their houses a desolation: they shall also build houses, but not inhabit them; and they shall plant vineyards, but not drink the wine thereof.\tAnd also build houses, but inhabit not vineyards, nor drink \n',
 'bible_poetry.tsv\tMeaning Change\tMeaning Change\tHis remembrance shall perish from the earth, and he shall have no name in the street.\tHis recollection dead, and no name in the street. \n',
 "bible_poetry.tsv\tIncorrect/New Information\tIncomplete\tAnd Moses gave unto the tribe of the children of Reuben inheritance according to their families.\tMosses gave Reuben his heirs, as their fam'lies accord. \n",
 'bible_poetry.tsv\tIncomplete\tIncomplete\tAnd the sabbath of the land shall be meat for you; for thee, and for thy servant, and for thy maid, and for thy hired servant, and for thy stranger that sojourneth with thee.\tMeat for you, your servant, maid, and stranger you hire. \n',
 "bible_poetry.tsv\tIncomplete\tIncomplete\tAnd all the army of the Chaldees, that were with the captain of the guard, brake down the walls of Jerusalem round about.\tRound Jerusalem's walls the army brakes, \n",
 "bible_poetry.tsv\tMeaning Change\tIncomplete\tAnd Abraham called the name of his son that was born unto him, whom Sarah bare to him, Isaac.\tAbraham's name, that Sarah's Isaac bore; \n",
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tThe length of one curtain shall be eight and twenty cubits, and the breadth of one curtain four cubits: and every one of the curtains shall have one measure.\tOne curtain is eight cubits long, and one is four cubits long. \n',
 "bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tNow if thou shalt kill all this people as one man, then the nations which have heard the fame of thee will speak, saying,\tNow, if thou hast kill'd all these men by one man, The nations that have heard thy fame will speak. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd Israel served the LORD all the days of Joshua, and all the days of the elders that overlived Joshua, and which had known all the works of the LORD, that he had done for Israel.\tThe king of Israel hath served Judah, and elders overlived, Who knew all their labors. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tChasten thy son while there is hope, and let not thy soul spare for his crying.\tHold, sweet son, when thou shalt be hopeful, And let not thy heart spare our weeping. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the sons of Jada the brother of Shammai; Jether, and Jonathan: and Jether died without children.\tJada and Jonathan died without children. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd ye have respect to him that weareth the gay clothing, and say unto him, Sit thou here in a good place; and say to the poor, Stand thou there, or sit here under my footstool:\tThou dost esteem a man that is gay, and thou dost say he will sit here, or sit under my footstool, for he is a poor man. \n',
 "bible_shakespeare.tsv\tNo Error\tMeaning Change\tFor therefore we both labour and suffer reproach, because we trust in the living God, who is the Saviour of all men, specially of those that believe.\tWe'll labor and suffer For trusting the living God, Who hath saved all and those that believe in particular. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAlso can any understand the spreadings of the clouds, or the noise of his tabernacle?\tCan any man understand also the spreading of clouds or noise? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd thou shalt offer thy burnt offerings, the flesh and the blood, upon the altar of the LORD thy God: and the blood of thy sacrifices shall be poured out upon the altar of the LORD thy God, and thou shalt eat the flesh.\tOn the altar Offer sacrifices burned, fleshed sacrifices, and eats blood. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tGod forbid: for then how shall God judge the world?\tHow does God judge the world? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThis is my comfort in my affliction: for thy word hath quickened me.\tI have your word comfort. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThat this shall be no grief unto thee, nor offence of heart unto my lord, either that thou hast shed blood causeless, or that my lord hath avenged himself: but when the LORD shall have dealt well with my lord, then remember thine handmaid.\tIf thou hast shed blood unluckily or avenged thy mistress, Remember thy handmaid when my lord has dealt well. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tBut let the righteous be glad; let them rejoice before God: yea, let them exceedingly rejoice.\tThe right merry; the heavens rejoice exceedingly. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd he cometh, and findeth them sleeping, and saith unto Peter, Simon, sleepest thou?\tHe comes, and they shall find sleeping, And he shall say to Simon. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd Simon and they that were with him followed after him.\tThey were followed by Simon and they. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tHe that is void of wisdom despiseth his neighbour: but a man of understanding holdeth his peace.\tHe that lacks wisdom despises his neighbor, But that an understanding man holds peace. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBut when David saw that his servants whispered, David perceived that the child was dead: therefore David said unto his servants, Is the child dead?\tBut David perceived the child dead when he saw his servants whispering. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tI will also stretch out mine hand upon Judah, and upon all the inhabitants of Jerusalem; and I will cut off the remnant of Baal from this place, and the name of the Chemarims with the priests;\tI’ll stretch my hand For all the gods in Jerusalem, And cut off the remnant of baal And the Chemarim. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tnone is good, save one, that is, God.\tNone good but God. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd the men of Judah said, Why are ye come up against us?\tWhy have you come to us? \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tJesus saith unto her, Woman, what have I to do with thee?\tWhat shall I do, woman?—Jesus, come hither. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThe children of Hariph, an hundred and twelve.\tO Hariph! \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tBlessed be the LORD for evermore.\tGod 'ild you for ever. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tHezekiah also had said, What is the sign that I shall go up to the house of the LORD?\tAnd what sign didst thou give me to go to the house, Zekekiah? \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd he said unto her, Daughter, thy faith hath made thee whole; go in peace, and be whole of thy plague.\tDaughter, your faith hath made thee whole; Go with a peace. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBecause of the savour of thy good ointments thy name is as ointment poured forth, therefore do the virgins love thee.\tSince thy name is good ointments, virgins do love thee. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tTherefore, behold, the days come, saith the LORD, that it shall no more be called Tophet, nor the valley of the son of Hinnom, but the valley of slaughter: for they shall bury in Tophet, till there be no place.\tIt shall not be call'd Tophet, but the Valley of Honnom. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tThe LORD shall laugh at him: for he seeth that his day is coming.\tHe did laugh upon seeing his day coming. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tMany are the afflictions of the righteous: but the LORD delivereth him out of them all.\tMany a righteous man suffers, But the Lord delivers him. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tKerioth is taken, and the strong holds are surprised, and the mighty men's hearts in Moab at that day shall be as the heart of a woman in her pangs.\tThe King was taken, and the strong-held Duke surprised, And on that day the mighty men’s hearts were in Moab. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tHave ye offered unto me sacrifices and offerings in the wilderness forty years, O house of Israel?\tHast thou offered forty years of sacrifice and thyself in the wilderness? \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThe law of truth was in his mouth, and iniquity was not found in his lips: he walked with me in peace and equity, and did turn many away from iniquity.\tHe walked with me in peace and equity And turned away many to infidelity. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the LORD said, Judah shall go up: behold, I have delivered the land into his hand.\tI have delivered land to Judah. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd Jesus stood still, and commanded him to be called.\tStill stood Jesu, and thou didst tell him he had called. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tYea, thou shalt be as he that lieth down in the midst of the sea, or as he that lieth upon the top of a mast.\tThou art like him that lies down i' th' sea, Or on the top of a mast. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tAnd the king said, What have I to do with you, ye sons of Zeruiah?\tWhat have I to do with you, Feruiah? \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tLet the floods clap their hands: let the hills be joyful together\tLet the floods clap their hands, and let the hills be merry together. \n',
 "bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tPraise ye the LORD: for it is good to sing praises unto our God; for it is pleasant; and praise is comely.\tTis good that our gracious God be sing'd praise. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tNow three of the thirty captains went down to the rock to David, into the cave of Adullam; and the host of the Philistines encamped in the valley of Rephaim.\tThree of the thirty captains Down into the rock to the cave of Audullam, And in the valley of Rephaim encamp the Philippians. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd called, and asked whether Simon, which was surnamed Peter, were lodged there.\tHe hath called and asked if Simon, the surname of Peter, be there. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThen answered Eliphaz the Temanite, and said,\tSay, Elliphaz. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAfterward I came unto the house of Shemaiah the son of Delaiah the son of Mehetabeel, who was shut up; and he said, Let us meet together in the house of God, within the temple, and let us shut the doors of the temple: for they will come to slay thee; yea, in the night will they come to slay thee.\tThen, Shemaiah, your son to Laiah, said let us meet at God’s house And shut the temple doors. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tTherefore the Jews sought the more to kill him, because he not only had broken the sabbath, but said also that God was his Father, making himself equal with God.\tHe hath broke the sabbath, and he hath said “God his father also”— The Jew wants the Jew to kill him. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tHonour thy father and mother; which is the first commandment with promise;\tFirst, let thy father and mother honor each other. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd when he cometh home, he calleth together his friends and neighbours, saying unto them, Rejoice with me; for I have found my sheep which was lost.\tWhen he comes home, he calls on friends and neighbors together, Saying he was merry at finding his lost sheep. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tBut fornication, and all uncleanness, or covetousness, let it not be once named among you, as becometh saints;\tBut saints should not be named Fornicates, uncleanliness, or covetousness. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd the king put them in the house of the forest of Lebanon.\tThe king hath put them in the Lebanon’s house. \n',
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tThere remaineth therefore a rest to the people of God.\tFor God’s rest. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tBut God giveth it a body as it hath pleased him, and to every seed his own body.\tBut God gives me as many bodies as it gives, And every seed of it. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tWhom I perceived to be accused of questions of their law, but to have nothing laid to his charge worthy of death or of bonds.\tHis accusation, as I perceived it, is a question of law, but he shall have nothing in him for a charge that he deserves his death or his bond. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tart not thou he, O LORD our God?\tIs he not? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThou hast covered with anger, and persecuted us: thou hast slain, thou hast not pitied.\tThou hast covered thy anger, And persecuted us. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the Sabeans fell upon them, and took them away; yea, they have slain the servants with the edge of the sword; and I only am escaped alone to tell thee.\tThe Sardians have slain their servants with a sword, And only by this I have escaped alone To tell them of them. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tCursed be he that confirmeth not all the words of this law to do them.\tI am curious he confirms not all the words of this law. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd it came to pass, when their hearts were merry, that they said, Call for Samson, that he may make us sport.\tThey call Samson, that he may make us sport. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd all the army of the Chaldees, that were with the captain of the guard, brake down the walls of Jerusalem round about.\tThe army hath braked down the walls of Jerusalem, i' faith. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Moses said unto the LORD, The people cannot come up to mount Sinai: for thou chargedst us, saying, Set bounds about the mount, and sanctify it.\tThou hast said He will set a limit about him And sanctify him thus: men cannot come on Shinai. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd thou shalt make a vail of blue, and purple, and scarlet, and fine twined linen of cunning work: with cherubims shall it be made:\tWith cherubims make a vaunt Of blue, purple, scarlet, and fine twine linen. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tBut Hannah went not up; for she said unto her husband, I will not go up until the child be weaned, and then I will bring him, that he may appear before the LORD, and there abide for ever.\tBut Hannah went not up; she said she would not go with her till the babes were weaned; And that she was my husband. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd all things are of God, who hath reconciled us to himself by Jesus Christ, and hath given to us the ministry of reconciliation;\tGod, that in Christ Jesus reconciled us, hath given us ministry of reconcilion. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tSeeing then that I will cut off from thee the righteous and the wicked, therefore shall my sword go forth out of his sheath against all flesh from the south to the north:\tAnd then, seeing that I had cut off thyself, the right, and the bad, I’d go with my sword out of my sheath against all flesh o'er the south and north. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tso I might have taken her to me to wife: now therefore behold thy wife, take her, and go thy way.\tI could have taken her to my wife. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tO continue thy lovingkindness unto them that know thee; and thy righteousness to the upright in heart.\tContinue to love those that know you. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tAnd Stephen, full of faith and power, did great wonders and miracles among the people.\tStephen, full of faith and power, Did great marvels and miracles unto this place. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd he shall speak great words against the most High, and shall wear out the saints of the most High, and think to change times and laws: and they shall be given into his hand until a time and times and the dividing of time.\tHe’ll speak great words against the highest, wear out saints, and think to change times and laws. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tor came it unto you only?\tOr only came it from you? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tBlessed is the man that feareth the LORD, that delighteth greatly in his commandments.\tBless the fearful who delights in his commands! \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd he went and sent to Jehoshaphat the king of Judah, saying, The king of Moab hath rebelled against me: wilt thou go with me against Moab to battle?\tHe hath said that Jehoshaphat, the king of Judah, Rebelled against me. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd it came to pass through the lightness of her whoredom, that she defiled the land, and committed adultery with stones and with stocks.\tAnd so she hath defiled the country And committed adultery with stones and stocks. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThat all the people of the earth may know that the LORD is God, and that there is none else.\tThat every man may know both God and no man else. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the city had no need of the sun, neither of the moon, to shine in it: for the glory of God did lighten it, and the Lamb is the light thereof.\tThere is no need of sun in the city, nor no need of moon. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd Joshua rose early in the morning, and the priests took up the ark of the LORD.\tJoshua rose early in the morning, and the priests took the ark. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tTo morrow, said he, thou shalt hear him.\tHe said thou shalt hear tomorrow. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the beast which I saw was like unto a leopard, and his feet were as the feet of a bear, and his mouth as the mouth of a lion: and the dragon gave him his power, and his seat, and great authority.\tThe beast that I saw was a leopard; The bear’s feet were the mouth of a lion, and the dragon gave him power. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tWe be twelve brethren, sons of our father; one is not, and the youngest is this day with our father in the land of Canaan.\tWe are now twelve brothers, not one, in Canaan, and our youngest father there. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd he said unto me, Go in, and behold the wicked abominations that they do here.\tGo to, and see The abominables they do here. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd Azariah the son of Jehoram king of Judah went down to see Jehoram the son of Ahab at Jezreel, because he was sick.\tAy, and then, Ariah, to Jezreel To see the son of Abram, Jehoram. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThe LORD will strengthen him upon the bed of languishing: thou wilt make all his bed in his sickness.\tThe Lord strengthen him in his bed, for he is ill. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd they returned to Joshua, and said unto him, Let not all the people go up; but let about two or three thousand men go up and smite Ai; and make not all the people to labour thither; for they are but few.\tDo not go back to Joshua, And say there be about two thousand up And kill Ai, but make all men in labor there. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tSo a measure of fine flour was sold for a shekel, and two measures of barley for a shekel, according to the word of the LORD.\tA gram of fine flour is to be sold For a shekel, and two gram of fine flour to be sold For a shekel. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd thou shalt put it under the compass of the altar beneath, that the net may be even to the midst of the altar.\tThou hast put a net under the altar. \n',
 "bible_shakespeare.tsv\tNo Error\tMeaning Change\tand when wilt thou return?\tAnd when thou return'st? \n",
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd he brought in the priests and the Levites, and gathered them together into the east street,\tHe hath assembled the priests and leviteses In the east street. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the angel of the LORD appeared unto the woman, and said unto her, Behold now, thou art barren, and bearest not: but thou shalt conceive, and bear a son.\tAngel appeared to the woman and she said she was barren and would not bear her son. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tIf a false witness rise up against any man to testify against him that which is wrong;\tAy, if a false witness rise against any man to testify a wrong. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd when the Pharisees saw it, they said unto his disciples, Why eateth your Master with publicans and sinners?\tWhen the Pharisee saw it, why ate thou thy master with publics and sinners? \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\twhom seekest thou?\tWhat seek’st thou? \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tWhosoever committeth sin transgresseth also the law: for sin is the transgression of the law.\tThose that commit sin do violate the law, for sin is sin. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tEven the country which the LORD smote before the congregation of Israel, is a land for cattle, and thy servants have cattle:\tEven in this land Are cattle raised, and your servants have such lands. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBehold, a virgin shall be with child, and shall bring forth a son, and they shall call his name Emmanuel, which being interpreted is, God with us.\tA virgin bears a babe and is to call him Emmanuel, Interpreted as God with us. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThen will I make this house like Shiloh, and will make this city a curse to all the nations of the earth.\tI’ll make this house like Shiloh, And make all nations curse me. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Zechariah, and Aziel, and Shemiramoth, and Jehiel, and Unni, and Eliab, and Maaseiah, and Benaiah, with psalteries on Alamoth;\tHere comes Zachariah and Aziel, Shemiramoth and Jesu, Lamiah, Maseiah and Benaiah, And psalteries of Alamoth. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd Jacob their father said unto them, Me have ye bereaved of my children: Joseph is not, and Simeon is not, and ye will take Benjamin away: all these things are against me.\tJacob is bereaved of his children; Joseph is not bereaved, Simon not bereaved, and you take away Benjamin. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd Joab returned to Jerusalem unto the king.\tJoab returned to Jerusalem. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd with you there shall be a man of every tribe; every one head of the house of his fathers.\tYou have every tribe’s man that heads the house their fathers. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tBut will God in very deed dwell with men on the earth?\tBut is it God himself that lives on earth? \n',
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tAnd Moses did as the LORD commanded: and they went up into mount Hor in the sight of all the congregation.\tMoses upon the mountain of Hor did the will that the Lord gave him command. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tNow when the centurion saw what was done, he glorified God, saying, Certainly this was a righteous man.\tWhen the centurion saw what was done, He glorified God and said “This is certain right.” Why, that’s the saying. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd it came to pass on the morrow, that Moses sat to judge the people: and the people stood by Moses from the morning unto the evening.\tSir, in the morning and evening, When the clock was set, Moses sat down to judge the people. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThis people draweth nigh unto me with their mouth, and honoureth me with their lips; but their heart is far from me.\tThese Moors do draw me from their mouths And honor me with their lips, But my far-favorite heart Is in the middle. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the dogs shall eat Jezebel in the portion of Jezreel, and there shall be none to bury her.\tThe dogs will eat a portion of Jezebel, and bury them. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tBut I will punish you according to the fruit of your doings, saith the LORD: and I will kindle a fire in the forest thereof, and it shall devour all things round about it.\tBut I will punish you according to the fruits that you have done. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThey provoked him to jealousy with strange gods, with abominations provoked they him to anger.\tThe strange gods' abominables provoked him to anger. \n",
 "bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tA man that is an heretick after the first and second admonition reject;\tThe guy that first admonish'd is rejected Is heretick after a second sentence and a third. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tThat they may want bread and water, and be astonied one with another, and consume away for their iniquity.\tThey may want bread and water, and be astonished to consume ’t. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tIniquities prevail against me: as for our transgressions, thou shalt purge them away.\tInjustice doth prevail upon me, Thy purgation of our transgressions doth reign. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\twhat is mine iniquity?\tWhat is my infirmity? \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncomplete\tAnd the time that David dwelt in the country of the Philistines was a full year and four months.\tFor four months o'er th' life of David in Philippi, It shall be full fourscore ducats. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd Samlah died, and Saul of Rehoboth by the river reigned in his stead.\tHamlet, he is dead, and Saul of Rehoboth reigns upon the river. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tThey send forth their little ones like a flock, and their children dance.\tThey send their little ones out like a flock, and their children dance. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tTherefore I make a decree, That every people, nation, and language, which speak any thing amiss against the God of Shadrach, Meshach, and Abednego, shall be cut in pieces, and their houses shall be made a dunghill: because there is no other God that can deliver after this sort.\tI have resolved To cut to pieces every man, every nation, every language that speak against Shadrach, Messach, and Abednego. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tSo he let him go: then she said, A bloody husband thou art, because of the circumcision.\tHe let him go, and then she said, for circumcision, he was a bloody husband. \n',
 "bible_shakespeare.tsv\tNo Error\tMeaning Change\tOr, Deliver me from the enemy's hand?\tOr wilt thou deliver me to thy enemy’s hand? \n",
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tBut as soon as this thy son was come, which hath devoured thy living with harlots, thou hast killed for him the fatted calf.\tBut thou hast killed a fat calf As soon as thy son hath devoured thy living with harlots. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tThou shalt also make a table of shittim wood: two cubits shall be the length thereof, and a cubit the breadth thereof, and a cubit and a half the height thereof.\tThou also makest a table of shit wood: two cubits is as much, and half a cubit is as much. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBehold, the nations are as a drop of a bucket, and are counted as the small dust of the balance: behold, he taketh up the isles as a very little thing.\tLook like a drop in a bucket, And count the small dust of the balance. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tO Israel, thy prophets are like the foxes in the deserts.\tThe prophets of Israel are like foxes in the desert. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tTherefore prophesy and say unto them, Thus saith the Lord GOD; Behold, O my people, I will open your graves, and cause you to come up out of your graves, and bring you into the land of Israel.\tTherefore prophesy, and say, I will open thy graves And bring thee to Israel. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThey shall run like mighty men; they shall climb the wall like men of war; and they shall march every one on his ways, and they shall not break their ranks:\tThey’ll run like great men, climb the wall like men of war; They’ll march every man through their ways, They’ll not break their ranks, but they’ll be kings. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tWhy doth this man thus speak blasphemies?\tWhy doth this gentleman speak blasphemy? \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tThe tongue deviseth mischiefs; like a sharp razor, working deceitfully.\tThe tongue is like a sharp razor, deceivingly working. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd they which went before rebuked him, that he should hold his peace: but he cried so much the more, Thou son of David, have mercy on me.\tThey rebuked him before, but so much cried, “Hath mercy, my lord? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tFor the oppression of the poor, for the sighing of the needy, now will I arise, saith the LORD; I will set him in safety from him that puffeth at him.\tNow, for the poor and needy, I stand him safe from the puffers. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tThe LORD hath sworn, and will not repent, Thou art a priest for ever after the order of Melchizedek.\tYea, Melchizedek swore, and did not repent. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThe lip of truth shall be established for ever: but a lying tongue is but for a moment.\tA truth forever established, not a lying tongue, But a tongue that in the moment speaks. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tAccording to the days of thy coming out of the land of Egypt will I shew unto him marvellous things.\tI say a wonderful thing thou art coming from Egypt. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd Moab shall be destroyed from being a people, because he hath magnified himself against the LORD.\tMoab is destroyed by his magnificence. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tFor thine arrows stick fast in me, and thy hand presseth me sore.\tThy arrows stick fast upon me, and his hand Presses me to a reproach. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tJesus answered, He it is, to whom I shall give a sop, when I have dipped it.\tWhen I have dipped it, I will give Jesu a sop. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tTherefore say, Thus saith the Lord GOD; Although I have cast them far off among the heathen, and although I have scattered them among the countries, yet will I be to them as a little sanctuary in the countries where they shall come.\tI am scattered among them, Yet in the countries where they come I am as little refuge. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThen the eyes of the blind shall be opened, and the ears of the deaf shall be unstopped.\tThen blind men’s eyes are opened, and the ears deaf. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd Saul, and Jonathan his son, and the people that were present with them, abode in Gibeah of Benjamin: but the Philistines encamped in Michmash.\tSaul and his son Jonathan live in Gibraltar, But in Philippines' camp at Michmash. \n",
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tPour out thine indignation upon them, and let thy wrathful anger take hold of them.\tPour thy indignation on them, And let thy wrathful anger take hold on them. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tSlay utterly old and young, both maids, and little children, and women: but come not near any man upon whom is the mark; and begin at my sanctuary.\tOld men, young men, maids, little children, and women In total slaying, but come not near anyone, and begin my sanctuary. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd when they came down to him, Elisha prayed unto the LORD, and said, Smite this people, I pray thee, with blindness.\tWhen they came down, Elisha said, “Thou kill’st this man, and be blind.” Well said. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the serpent said unto the woman, Ye shall not surely die:\tFor certain, the serpent said a woman would not die. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd there were made on them, on the doors of the temple, cherubims and palm trees, like as were made upon the walls; and there were thick planks upon the face of the porch without.\tThe cherubims and palm-trees are at the temple doors, And the thick planks on the porch face. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd as the ark of the LORD came into the city of David, Michal Saul's daughter looked through a window, and saw king David leaping and dancing before the LORD; and she despised him in her heart.\tThe daughter of Michael Salomon looked out at window, She saw the King David leaping and dancing before him, And he despised her. \n",
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd he left them, and went away again, and prayed the third time, saying the same words.\tHe left them, and went away again, and pronounced the third same. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd he shall pass over to his strong hold for fear, and his princes shall be afraid of the ensign, saith the LORD, whose fire is in Zion, and his furnace in Jerusalem.\tHe shall pass over a strong hold for fear, And then ’tis a soldier’s fear. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tForty and two years old was Ahaziah when he began to reign, and he reigned one year in Jerusalem.\tAhaziah shall live one year in Jerusalem. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tBehold, I will bring evil upon thee, and will take away thy posterity, and will cut off from Ahab him that pisseth against the wall, and him that is shut up and left in Israel,\tI’ll bring thee evil, take away thy posterity, Cut off the pissing wall, And shutting up those that left Israel. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tcurse God, and die.\tO God’s curse! \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd upon the table of shewbread they shall spread a cloth of blue, and put thereon the dishes, and the spoons, and the bowls, and covers to cover withal: and the continual bread shall be thereon:\tThey’ll spread a blue cloth upon the table And put on dishes, spoons, and covers. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tWhosoever putteth away his wife, and marrieth another, committeth adultery: and whosoever marrieth her that is put away from her husband committeth adultery.\tIf a wife do marry her husband, she commits adultery. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tHe that sacrificeth unto any god, save unto the LORD only, he shall be utterly destroyed.\tThose that do sacrifice themselves to any god, Save only God, are utterly destroyed. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThen said I, Whither goest thou?\tWhither goest thou then? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd said unto the king, Let not my lord impute iniquity unto me, neither do thou remember that which thy servant did perversely the day that my lord the king went out of Jerusalem, that the king should take it to his heart.\tDo not impute iniquity to me, nor remember That your servant did me on the day my lord left Jerusalem. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tBut into the second went the high priest alone once every year, not without blood, which he offered for himself, and for the errors of the people:\tBut every year the high priest went alone, Who hath not the blood that he offered his master and his error. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tLift up your eyes, and behold them that come from the north: where is the flock that was given thee, thy beautiful flock?\tLift up thine eyes, Where the fair flock is. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd when Paul was now about to open his mouth, Gallio said unto the Jews, If it were a matter of wrong or wicked lewdness, O ye Jews, reason would that I should bear with you:\tGallio said, when Paul was about to open his mouth, “If it have any cause to bear you wrong or evil,” When he was about to say, “You shall have reason to bear with me.” Well said, Jew. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThen Zedekiah the son of Chenaanah came near, and smote Micaiah upon the cheek, and said, Which way went the Spirit of the LORD from me to speak unto thee?\tThen came Zedekiah, the son of Chenaanah, near him, And on the cheek did he kiss Miah, and say “Amen” to him. \n',
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tAnd many nations shall come, and say, Come, and let us go up to the mountain of the LORD, and to the house of the God of Jacob; and he will teach us of his ways, and we will walk in his paths: for the law shall go forth of Zion, and the word of the LORD from Jerusalem.\tMany a nation come and say, Let us go to the Moor of Jacob And to his paths. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThese are the words of the covenant, which the LORD commanded Moses to make with the children of Israel in the land of Moab, beside the covenant which he made with them in Horeb.\tThis is the covenant that Moses made with the Jew of Israel, and it is the covenant that Horatio made with the Jew of Nazareth. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tJudge me, O LORD; for I have walked in mine integrity: I have trusted also in the LORD; therefore I shall not slide.\tJudge me as I have walked in my integrity. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tWhen Jesus understood it, he said unto them, Why trouble ye the woman?\tWhen Jesu understood it, why should a woman trouble herself? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThe ancients of Gebal and the wise men thereof were in thee thy calkers: all the ships of the sea with their mariners were in thee to occupy thy merchandise.\tYour ships and mariners are in your ships To occupy your merchandise. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tThe poor and the deceitful man meet together: the LORD lighteneth both their eyes.\tPoor men will meet together in deceitful man. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tFair weather cometh out of the north: with God is terrible majesty.\tThe fair weather is coming north. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tBut he answered and said unto him that told him, Who is my mother?\tBut he answered, and told him who is his mother? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tNebuchadnezzar spake and said unto them, Is it true, O Shadrach, Meshach, and Abednego, do not ye serve my gods, nor worship the golden image which I have set up?\tHast thou said, Nebuchadnezzar, Shadrach and Meshach and Abednego not serve my gods And worship not the golden image that I set down? \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThe day following Jesus would go forth into Galilee, and findeth Philip, and saith unto him, Follow me.\tThe day is following, And Jesus will go to Israel and find Philippi. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tFor strangers are risen up against me, and oppressors seek after my soul: they have not set God before them.\tStrangers have risen against me, and oppressors seek God’s will. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd they rose up early in the morning, and the sun shone upon the water, and the Moabites saw the water on the other side as red as blood:\tThey rose early in the morning, and the sun glimm'd in the water, And the Moabites saw them red-beloved. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd Jesus said, For judgment I am come into this world, that they which see not might see; and that they which see might be made blind.\tJesu said I had come from this world to judge those that see not. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tHe shall break also the images of Bethshemesh, that is in the land of Egypt; and the houses of the gods of the Egyptians shall he burn with fire.\tHe will break, too, the images of Bethshemesh, Egypt, For ’tis an Egyptian city. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the spirit cried, and rent him sore, and came out of him: and he was as one dead; insomuch that many said, He is dead.\tThe spirit cries, out, and he is dead. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tTo every thing there is a season, and a time to every purpose under the heaven:\tUnder heaven there is seasons and time for all things. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tTake heed unto thyself, and unto the doctrine; continue in them: for in doing this thou shalt both save thyself, and them that hear thee.\tBy doing this, thou art saved both thyself and those that listen. \n',
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tO give thanks unto the God of gods: for his mercy endureth for ever.\tThanks, good God. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tHe measured the east side with the measuring reed, five hundred reeds, with the measuring reed round about.\tHe measured the east side with a hundred reeds. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd Cain talked with Abel his brother: and it came to pass, when they were in the field, that Cain rose up against Abel his brother, and slew him.\tCain talked with his brother Abel, and he slew him. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tSaying, God hath forsaken him: persecute and take him; for there is none to deliver him.\tSay that God hath abandoned him, persecuted him, and took him. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tBut the day of the Lord will come as a thief in the night; in the which the heavens shall pass away with a great noise, and the elements shall melt with fervent heat, the earth also and the works that are therein shall be burned up.\tBut pass through the skies and elements with great noise And melt the earth with fervent heat. \n',
 "bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tJude, the servant of Jesus Christ, and brother of James, to them that are sanctified by God the Father, and preserved in Jesus Christ, and called:\tJude shall be sanctified by God's father, and preserved by him. \n",
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tFor this city hath been to me as a provocation of mine anger and of my fury from the day that they built it even unto this day; that I should remove it from before my face,\tThe day they built I would remove them before my face, For this city hath stol'n my anger and me. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\twhy do ye not rather suffer yourselves to be defrauded?\tWhy shouldst thou rather suffer thy defraudation? \n',
 'bible_shakespeare.tsv\tNo Error\tIncomplete\tUntil the day break, and the shadows flee away, turn, my beloved, and be thou like a roe or a young hart upon the mountains of Bether.\tTill the break of day, And the shadows fled away, Turn thee, thee like a roe or young hart In the mountains of Bether. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAgainst him came up Nebuchadnezzar king of Babylon, and bound him in fetters, to carry him to Babylon.\tThe king of Babylon, Nebuchadnezzar, Binds him in fetters to carry him to his Majesty. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tThis their way is their folly: yet their posterity approve their sayings.\tTheir way is foolish, but their posterity approves what they say. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThe rest of all the acts of Asa, and all his might, and all that he did, and the cities which he built, are they not written in the book of the chronicles of the kings of Judah?\tIs not all the deeds of Asa in a book of history, All the deeds he did, all the cities he built, Written in letters? \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tAnd the spoiler shall come upon every city, and no city shall escape: the valley also shall perish, and the plain shall be destroyed, as the LORD hath spoken.\tThe spoiler comes from every city, and no one shall evade, and the valley is dead and the plain destroyed. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tNot that any man hath seen the Father, save he which is of God, he hath seen the Father.\tNo man besides his father saw him. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tWhen he was removed out of the highway, all the people went on after Joab, to pursue after Sheba the son of Bichri.\tWhen Joab was removed from the highway, All the people went to pursue Sheba. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the man smote him, so that in smiting he wounded him.\tWhy, man, smite him, he’s wounded. \n',
 'bible_shakespeare.tsv\tNo Error\tIncomplete\tSo we thy people and sheep of thy pasture will give thee thanks for ever: we will shew forth thy praise to all generations.\tWe have ever thanks for your person, your pasture-sheep; Our praises do show to all generations. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tSharp arrows of the mighty, with coals of juniper.\tThere are sharp arrows in the juniper. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd I saw three unclean spirits like frogs come out of the mouth of the dragon, and out of the mouth of the beast, and out of the mouth of the false prophet.\tI saw three unclean spirits, like frogs. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tTherefore, brethren, we are debtors, not to the flesh, to live after the flesh.\tThen we are debtors, but want not to live after flesh. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tWherefore she said unto Abraham, Cast out this bondwoman and her son: for the son of this bondwoman shall not be heir with my son, even with Isaac.\tSo she said to her son Abraham, “cast this bondwoman and her son out.” Well said. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd it came to pass, when Jesus had made an end of commanding his twelve disciples, he departed thence to teach and to preach in their cities.\tAnd in the end, when he had done commandment, Did Jesus leave the city to teach and preach to a dozen disciples. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tand she, even she herself said, He is my brother: in the integrity of my heart and innocency of my hands have I done this.\tEven she said he, her brother, was her integrity and his innocence. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncomplete\tOf the tribe of Nephthalim were sealed twelve thousand.\tThe nephthalim was seal'd twelve years ago. \n",
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd the very God of peace sanctify you wholly; and I pray God your whole spirit and soul and body be preserved blameless unto the coming of our Lord Jesus Christ.\tThe very peace-loving God sanctifies you entirely; I pray him preserve your spirit, your soul, and your body whole, Without any blame. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tJudge not, and ye shall not be judged: condemn not, and ye shall not be condemned: forgive, and ye shall be forgiven:\tJudge not, and be not judged. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tOf the first of your dough ye shall give unto the LORD an heave offering in your generations.\tThy first dough Will I give thee to thy Lord in thy generation. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd it came to pass also on another sabbath, that he entered into the synagogue and taught: and there was a man whose right hand was withered.\tHe entered the synagogue and taught it also on another sabbath. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd they gathered their brethren, and sanctified themselves, and came, according to the commandment of the king, by the words of the LORD, to cleanse the house of the LORD.\tThey gathered their brothers And sanctified them, and came Conforming to the command of the king. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tor their border greater than your border?\tOr is their border greater than yours? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThen said I unto them, Ye see the distress that we are in, how Jerusalem lieth waste, and the gates thereof are burned with fire: come, and let us build up the wall of Jerusalem, that we be no more a reproach.\tThou dost see our distress, And burnst both Jerusalem and her gates. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the city was besieged unto the eleventh year of king Zedekiah.\tThe king, Zedekiah, is besieged of the city. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd Peter answered unto her, Tell me whether ye sold the land for so much?\tTell me, lord, if thou hast sold so much the land. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Harbonah, one of the chamberlains, said before the king, Behold also, the gallows fifty cubits high, which Haman had made for Mordecai, who spoken good for the king, standeth in the house of Haman.\tSay to Harbonah, one of the king’s subjects, “Seest thou a gallows fifty cubits high, Made by Hamani to good Mordecai”! \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tBut Noah found grace in the eyes of the LORD.\tBut Noah found grace in him. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tAnd if they were all one member, where were the body?\tWhere be the bodies, if they were all One? \n',
 'bible_shakespeare.tsv\tNo Error\tIncomplete\tAnd Abijah stood up upon mount Zemaraim, which is in mount Ephraim, and said, Hear me, thou Jeroboam, and all Israel;\tAbijah stood upon Mount Zemaraim, On Mount Ephraim, and spake, “Hear, Jeroboam, and all Israel! \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThe two pillars, one sea, and twelve brasen bulls that were under the bases, which king Solomon had made in the house of the LORD: the brass of all these vessels was without weight.\tTwo pillars of sea and twelve brasen bulls, under the bases, That made noble Solomon the king, Had no weight. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tSurely thou wilt slay the wicked, O God: depart from me therefore, ye bloody men.\tFor God’s sake, I am sure you have slain an evil man. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd they shall bear the curtains of the tabernacle, and the tabernacle of the congregation, his covering, and the covering of the badgers' skins that is above upon it, and the hanging for the door of the tabernacle of the congregation,\tThey bear the curtains at the tabernacle and cover the badger’s skin above. \n",
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tMy lips shall not speak wickedness, nor my tongue utter deceit.\tMine mouth would not speak of evil, Nor my tongue would speak of deceit. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd they marvelled all.\tThey are all amazed. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tThanks be unto God for his unspeakable gift.\tGod be thanked for thy unspoke gift. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the manna ceased on the morrow after they had eaten of the old corn of the land; neither had the children of Israel manna any more; but they did eat of the fruit of the land of Canaan that year.\tWhen they have eaten up the manna from the old Israeli corn, They have stopped that year's harvest. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd when Peter saw it, he answered unto the people, Ye men of Israel, why marvel ye at this?\tPeter wonders when he sees it, why this amazes the Israelis. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd when thou prayest, thou shalt not be as the hypocrites are: for they love to pray standing in the synagogues and in the corners of the streets, that they may be seen of men.\tSince they love to pray, And stand in synagogues and in streets corners, Be not hypocrites when you are so. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tIn the year of this jubile ye shall return every man unto his possession.\tOn this anniversary Return all thy possession. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tnow therefore receive no more money of your acquaintance, but deliver it for the breaches of the house.\tWhy, then, now you receive no more money, but you’ll deliver to your acquaintance. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tA seed shall serve him; it shall be accounted to the Lord for a generation.\tThe seed shall serve him; for each generation is account'd. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tNow among these were of the children of Judah, Daniel, Hananiah, Mishael, and Azariah:\tAmong them are Daniel, Hananiah, Mishael, and Azariah. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tTo whom coming, as unto a living stone, disallowed indeed of men, but chosen of God, and precious,\tIndeed, the living stone is not allowed to come, But that God hath chosen, and that stone is precious. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd Adam was not deceived, but the woman being deceived was in the transgression.\tAdam was not deceived, but a woman. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tBut in the place which the LORD shall choose in one of thy tribes, there thou shalt offer thy burnt offerings, and there thou shalt do all that I command thee.\tBut there thou canst offer thy burned goods To all my tribes, and do All that I command in thine own hand. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThe hands of the pitiful women have sodden their own children: they were their meat in the destruction of the daughter of my people.\tWretched women have slaughtered their children. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd the children of Israel returned from chasing after the Philistines, and they spoiled their tents.\tThey returned from the chase For the Philippians, and ruin'd their tents. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd afterward I will bring again the captivity of the children of Ammon, saith the LORD.\tI will return to captivity then. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAs for thee also, by the blood of thy covenant I have sent forth thy prisoners out of the pit wherein is no water.\tI have also sent your prisoner out o' th' pit where there is no water. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd that which cometh into your mind shall not be at all, that ye say, We will be as the heathen, as the families of the countries, to serve wood and stone.\tAnd thou didst not say that we did serve wood and stone at once. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tThe fig tree putteth forth her green figs, and the vines with the tender grape give a good smell.\tThe fig tree hath laid her green figs out, And the tender grapes do smell good. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tLest he that heareth it put thee to shame, and thine infamy turn not away.\tThou art ashamed he heard it, and thy infamy Doth not turn away. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tFor which cause both thou and all thy company are gathered together against the LORD: and what is Aaron, that ye murmur against him?\tWhy have you, and all your company, Gathered against Aaron? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tHe layeth up sound wisdom for the righteous: he is a buckler to them that walk uprightly.\tHe lays sound wisdom upon those that walk upright. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncomplete\tIt is in the power of my hand to do you hurt: but the God of your father spake unto me yesternight, saying, Take thou heed that thou speak not to Jacob either good or bad.\tBut God be wi' you, be wi' you, that said to me yesterday, “No good or bad word of Jacob,” That you should speak not of him. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the great court round about was with three rows of hewed stones, and a row of cedar beams, both for the inner court of the house of the LORD, and for the porch of the house.\tThe great court is made up of three rows of honed stones, one of cedar beams, And the rest is made up of cedar. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAll nations whom thou hast made shall come and worship before thee, O Lord; and shall glorify thy name.\tAll the nations thou hast made will come and worship thyself. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd am no more worthy to be called thy son: make me as one of thy hired servants.\tI have no less deserved your call to be one of your servants’ hirers. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tWash you, make you clean; put away the evil of your doings from before mine eyes; cease to do evil;\tWash thyself, clean thyself; cease all evil that thou dost before mine eyes. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tBut ye have borne the tabernacle of your Moloch and Chiun your images, the star of your god, which ye made to yourselves.\tBut thou carriest the images of thine own stars, Moloch and Chiun. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the rough goat is the king of Grecia: and the great horn that is between his eyes is the first king.\tRough goats, you are kings of Greece. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd there shall ye remember your ways, and all your doings, wherein ye have been defiled; and ye shall lothe yourselves in your own sight for all your evils that ye have committed.\tThou rememberest thy ways and all thy deeds, And forgivest all thy evils that thou hast committed. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThe LORD hath cast off his altar, he hath abhorred his sanctuary, he hath given up into the hand of the enemy the walls of her palaces; they have made a noise in the house of the LORD, as in the day of a solemn feast.\tThe Lord hath cast his altar off, Abhorred his sanctuary, gave o'er her palace walls. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tFrom the wicked that oppress me, from my deadly enemies, who compass me about.\tFrom mine oppressors, enemies that kill themselves. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tMoreover, brethren, I would not that ye should be ignorant, how that all our fathers were under the cloud, and all passed through the sea;\tNor did I desire thee to know How all our fathers were enshelter'd under a cloud And passed through the sea. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tLet thine eyes be on the field that they do reap, and go thou after them: have I not charged the young men that they shall not touch thee?\tObserve your eyes upon the field they reap, And go to ’t, and I will not charge the young man to touch you? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\thath not David rather sent his servants unto thee, to search the city, and to spy it out, and to overthrow it?\tDid David send his servants to search the city, Spies the city, and overthrow him? \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tLet every man abide in the same calling wherein he was called.\tLet every man abide his own calling as his own. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd Jacob did so, and fulfilled her week: and he gave him Rachel his daughter to wife also.\tBy Jacob, ’tis done, ’tis fulfilled in his week, And he hath also given his daughter daughter Rachel for her. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd I fell down before the LORD, as at the first, forty days and forty nights: I did neither eat bread, nor drink water, because of all your sins which ye sinned, in doing wickedly in the sight of the LORD, to provoke him to anger.\tFor all thy sins, I will not eat bread nor drink water. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd of the Gadites there separated themselves unto David into the hold to the wilderness men of might, and men of war fit for the battle, that could handle shield and buckler, whose faces were like the faces of lions, and were as swift as the roes upon the mountains;\tNow the Gadites parted from David, who held him in the wilderness, And those that could handle a shield and a buckler Well, with faces like lions, were fit to bear them. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tEven so it is not the will of your Father which is in heaven, that one of these little ones should perish.\tYet your father’s will is not, To bring this little one to death. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tWhoso robbeth his father or his mother, and saith, It is no transgression; the same is the companion of a destroyer.\tThose that have robbed their fathers or their mothers, And say it is no transgression, there is none. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd when a convenient day was come, that Herod on his birthday made a supper to his lords, high captains, and chief estates of Galilee;\tHero, on his birthday, Made dinner with his lords, high-captains, and estates Of noble chiefs. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd the decree went forth that the wise men should be slain; and they sought Daniel and his fellows to be slain.\tDaniel and his friends have been determined To be slain, and both sought death. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tThen Shaphan the scribe told the king, saying, Hilkiah the priest hath given me a book.\tThen the scribe, Stephano, told the king That Bishop Hilkiah had given the book to him. \n',
 "bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tBrethren, my heart's desire and prayer to God for Israel is, that they might be saved.\tFor Israel’s sake am I drawn to save it, And I pray God it be so. \n",
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tThey shall put you out of the synagogues: yea, the time cometh, that whosoever killeth you will think that he doeth God service.\tThey’ll put you out of synagogue, and those that kill you Think they do serve God. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd Joseph placed his father and his brethren, and gave them a possession in the land of Egypt, in the best of the land, in the land of Rameses, as Pharaoh had commanded.\tBy order of Pharaoh, in Egypt Did Joseph put in his father and his brothers. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThus saith the LORD; I am returned unto Zion, and will dwell in the midst of Jerusalem: and Jerusalem shall be called a city of truth; and the mountain of the LORD of hosts the holy mountain.\tI am returned to Zion; I dwell in Jerusalem. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tSince the days of our fathers have we been in a great trespass unto this day; and for our iniquities have we, our kings, and our priests, been delivered into the hand of the kings of the lands, to the sword, to captivity, and to a spoil, and to confusion of face, as it is this day.\tWe have been in this day's mischance since; 'tis now our day; 'tis now our night, 'tis now our night, 'tis now our night; 'tis now our night, 'tis night, 'tis night, 'tis night, 'tis night, 'tis night, 'tis night \n",
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd if he smite him with throwing a stone, wherewith he may die, and he die, he is a murderer: the murderer shall surely be put to death.\tThe murderer, if he hit him with throwing stones. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tDo not think that I will accuse you to the Father: there is one that accuseth you, even Moses, in whom ye trust.\tThink not of my accusation ’gainst your father; For even one of you Was under pressure of Moses. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThey go up by the mountains; they go down by the valleys unto the place which thou hast founded for them.\tThey go up into the mountains and down into the valleys. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThus saith the LORD to me; Make thee bonds and yokes, and put them upon thy neck,\tTherefore, I beseech you, make bonds with me, Take your yoke and put your neck in. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tIs it fit to say to a king, Thou art wicked?\tIs ’t right to say thou art a knave, a knave, a knave, a knave, a knave, a knave, a knave? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBut if they will not obey, I will utterly pluck up and destroy that nation, saith the LORD.\tBut if they will not obey, I’ll pluck up and destroy that nation. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tParthians, and Medes, and Elamites, and the dwellers in Mesopotamia, and in Judaea, and Cappadocia, in Pontus, and Asia,\tThe Parthians, The Medes, The Amerindians, The Elephants, The Mesopotamias, The Cappadocians, And all the continent of Asia. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd they built for Pharaoh treasure cities, Pithom and Raamses.\tFor Pharaoh, they built treasure towns of Pithom and Ramses. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tFor when we were yet without strength, in due time Christ died for the ungodly.\tWhen our due time is come, Christ died when our strength still lay unshaken. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tWho is this that darkeneth counsel by words without knowledge?\tWhat ignorance does darken the counsels of time? \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThe burden of the beasts of the south: into the land of trouble and anguish, from whence come the young and old lion, the viper and fiery flying serpent, they will carry their riches upon the shoulders of young asses, and their treasures upon the bunches of camels, to a people that shall not profit them.\tThe young and old lion and the fiery flying serpent Carry their wealth and treasure on their young asses' shoulders To countries that do not profit them. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tHe withdraweth not his eyes from the righteous: but with kings are they on the throne; yea, he doth establish them for ever, and they are exalted.\tHe would not withdraw his eyes from the right; But where the kings are on the throne And forever establish themselves. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd her husband went with her along weeping behind her to Bahurim.\tHer husband and the weeping behind her went along with him. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBut because the LORD loved you, and because he would keep the oath which he had sworn unto your fathers, hath the LORD brought you out with a mighty hand, and redeemed you out of the house of bondmen, from the hand of Pharaoh king of Egypt.\tThe Lord loved you, and kept the oath That he swore to your fathers; so he rescued you from the Pharaoh’s house. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThe nethermost chamber was five cubits broad, and the middle was six cubits broad, and the third was seven cubits broad: for without in the wall of the house he made narrowed rests round about, that the beams should not be fastened in the walls of the house.\tThe smallest chamber is five cubits wide, the middle six cubits wide, the third seven cubits wide. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tand when thou art athirst, go unto the vessels, and drink of that which the young men have drawn.\tWhen thou art athirst, go to the vessels and drink of young men’s blood. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd I bought the field of Hanameel my uncle's son, that was in Anathoth, and weighed him the money, even seventeen shekels of silver.\tI bought my uncle’s field in Anathoth, And weighed the money even at seventeen shekels. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tWhich will not hearken to the voice of charmers, charming never so wisely.\tCharmers, do not hear you. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the Chaldeans shall come again, and fight against this city, and take it, and burn it with fire.\tBack do the Chaldeans come, And fight for this city. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd his brethren, chief of the fathers, two hundred forty and two: and Amashai the son of Azareel, the son of Ahasai, the son of Meshillemoth, the son of Immer,\tAmashai is the son of Ahasai, Meshillemoth’s son. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd he said, This is an ephah that goeth forth.\tThis is the ephah. \n',
 "bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThou shalt not uncover the nakedness of thy father's sister: she is thy father's near kinswoman.\tThou shalt not uncover naked thy father’s sister: she’s thy near mother. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tNow Tobiah the Ammonite was by him, and he said, Even that which they build, if a fox go up, he shall even break down their stone wall.\tTobiah the Ammonite said, if he go up, a fox would break even their stone wall. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tFor to him that is joined to all the living there is hope: for a living dog is better than a dead lion.\tThere’s hope a living dog is better than a dead lion. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd he saith unto the man which had the withered hand, Stand forth.\tHe spake to you, “Stand with his withered hand. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd I put a jewel on thy forehead, and earrings in thine ears, and a beautiful crown upon thine head.\tI put earrings on thy forehead and a pretty crown Upon thy head. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tLet Pharaoh do this, and let him appoint officers over the land, and take up the fifth part of the land of Egypt in the seven plenteous years.\tThis should be done By Pharaoh, and in seven years appoint him Officers over land, and take over The fifth part of Egypt. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd he turned himself, and went out from Pharaoh.\tHe turned himself and hath left Pharaoh. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd unleavened bread, and cakes unleavened tempered with oil, and wafers unleavened anointed with oil: of wheaten flour shalt thou make them.\tThou mak’st leavened bread, cakes untempered with oil, Untempered wafers and coat’d with wax. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBut ye are come unto mount Sion, and unto the city of the living God, the heavenly Jerusalem, and to an innumerable company of angels,\tBut thou art come from Mount Sinai and heavenly Jerusalem. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tWilt not thou, O God, which hadst cast us off?\tGod cast us off? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd they came to a place which was named Gethsemane: and he saith to his disciples, Sit ye here, while I shall pray.\tHe spake to his disciples, “Sit here while I pray. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd all the spoil of these cities, and the cattle, the children of Israel took for a prey unto themselves; but every man they smote with the edge of the sword, until they had destroyed them, neither left they any to breathe.\tThey took all these cities and cattle as prey, But with swords every man slain Till they have destroyed them. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the second angel poured out his vial upon the sea; and it became as the blood of a dead man: and every living soul died in the sea.\tThe second angel poured his vial Into the sea, and it became The blood of a dead man. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tAnd Pharaoh awoke, and, behold, it was a dream.\tAy, and the Pharaoh wakes and dreams. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the firstborn said unto the younger, Our father is old, and there is not a man in the earth to come in unto us after the manner of all the earth:\tOur father was old, and man would not come o'er the earth. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd Joshua made him sharp knives, and circumcised the children of Israel at the hill of the foreskins.\tSo Joshua made sharp knives of him, and circumcised the children of Israel. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tGo not to glean in another field, neither go from hence, but abide here fast by my maidens:\tGo not to another field, but go here fast. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tDay unto day uttereth speech, and night unto night sheweth knowledge.\tThe day is speech, and the night shows knowledge. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThey take up all of them with the angle, they catch them in their net, and gather them in their drag: therefore they rejoice and are glad.\tThey take them all by angle, Catch them in the net, and gather them in the drag. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tA man of great wrath shall suffer punishment: for if thou deliver him, yet thou must do it again.\tIf a great wrath be delivered, a great wrath suffers punishment, though he must do it again, and so must he. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThere failed not ought of any good thing which the LORD had spoken unto the house of Israel; all came to pass.\tWhat you have said to the Israeli house, Lord, you have none. \n',
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tSo that a man shall say, Verily there is a reward for the righteous: verily he is a God that judgeth in the earth.\tTherefore men shall say the right is verily rewarded. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThen shalt thou say, O LORD, thou hast spoken against this place, to cut it off, that none shall remain in it, neither man nor beast, but that it shall be desolate for ever.\tThen say, my lord, he hath cut it off, And that man and beast shall not remain in it, And be desolate for ever. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tYea, they have chosen their own ways, and their soul delighteth in their abominations.\tThey have chosen their ways, and their abominables delight them. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tLittle children, yet a little while I am with you.\tYet for a while I’ll be with you, you little ones. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThus saith the Lord GOD; If the prince give a gift unto any of his sons, the inheritance thereof shall be his sons'; it shall be their possession by inheritance.\tIf a prince’s son give his gift to any prince’s son, his son shall be heir to the thing that is his son’s estate. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAnd God helped him against the Philistines, and against the Arabians that dwelt in Gurbaal, and the Mehunims.\tGod help thee in Urbaal Against the Philippians and the Mehunim. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThou shalt sanctify him therefore; for he offereth the bread of thy God: he shall be holy unto thee: for I the LORD, which sanctify you, am holy.\tHe that offers God’s bread shall sanctify him. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tTherefore the LORD was very angry with Israel, and removed them out of his sight: there was none left but the tribe of Judah only.\tSo God hath very wrath at Israel and removed ’t from his sight! \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tTheir slain also shall be cast out, and their stink shall come up out of their carcases, and the mountains shall be melted with their blood.\tBesides, they are dead, and their stinking comes out of their carcasses. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tWho, having received such a charge, thrust them into the inner prison, and made their feet fast in the stocks.\tThey thrust their feet into an inner prison and made fast their legs, Receiving such a charge. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tBut those mine enemies, which would not that I should reign over them, bring hither, and slay them before me.\tBut for mine own part, I would not kill mine enemies. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAlthough thou sayest thou shalt not see him, yet judgment is before him; therefore trust thou in him.\tThough thou say’st thou wouldst not see him, The judge is before him, and therefore thou shouldst trust him. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tFor he that is not against us is on our part.\tHe is not against us. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tFor the LORD shall judge his people, and repent himself for his servants, when he seeth that their power is gone, and there is none shut up, or left.\tWhen that the power of their lords is gone, And they are not shut up or left out, Then God judge their person and repent their servants. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tFrom that time forth came they no more on the sabbath.\tThey’ll be no longer on sabbath. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tI will arise and go to my father, and will say unto him, Father, I have sinned against heaven, and before thee,\tI have risen and gone to my father, To say I have singed heaven and to be damned. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tRepent ye therefore, and be converted, that your sins may be blotted out, when the times of refreshing shall come from the presence of the Lord.\tRepent thy sins, and be converted, That thy sins may be blotted in a refresh. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tMen do therefore fear him: he respecteth not any that are wise of heart.\tMen fear him, lest he respect any wise heart. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tAnd I, brethren, could not speak unto you as unto spiritual, but as unto carnal, even as unto babes in Christ.\tI cannot speak you spiritually, but I can speak carnal, Even as a baby in Christ. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tAnd as they did eat, he said, Verily I say unto you, that one of you shall betray me.\tHe said that while they did eat, one of you did betray him. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tYe are our epistle written in our hearts, known and read of all men:\tThou hast writ down our own epistles that we have known and read. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tAnd Chesed, and Hazo, and Pildash, and Jidlaph, and Bethuel.\tChesed, Hazo, Pillash, and Jidlaph! \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd Judah did evil in the sight of the LORD, and they provoked him to jealousy with their sins which they had committed, above all that their fathers had done.\tJudah did an evil, and provoked his father To jealousy, which his sins were above all done. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tWherefore, if God so clothe the grass of the field, which to day is, and to morrow is cast into the oven, shall he not much more clothe you, O ye of little faith?\tIf God do not clothe you more, doth he not? \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd in all that mighty hand, and in all the great terror which Moses shewed in the sight of all Israel.\tFor all the world, And all the great terror that Moses hath shown, He hath shown Israel. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tBut his delight is in the law of the LORD; and in his law doth he meditate day and night.\tBut he hath meditated on his law the day, and he hath slept the night. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tWherefore do the wicked live, become old, yea, are mighty in power?\tWhere dwells the evil, grows old, and is potent? \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tO thou king, the most high God gave Nebuchadnezzar thy father a kingdom, and majesty, and glory, and honour:\tGod, his highest sovereign, Gave his father Nebuchadnezzar a kingdom, majesty, glory, and honor. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tWhen he therefore was come up again, and had broken bread, and eaten, and talked a long while, even till break of day, so he departed.\tEven till the day he left the house, When he had broken bread, eaten it, and talked long while. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tNow Joshua was clothed with filthy garments, and stood before the angel.\tJoshua was clad in filth, and stood before an angel. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tThat they were graven with an iron pen and lead in the rock for ever!\tThey shall be graved with an iron pen and lead upon the rock forever. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tI sent you to reap that whereon ye bestowed no labour: other men laboured, and ye are entered into their labours.\tI sent you for work, That other men would work, and you would get his. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd as for me, thou upholdest me in mine integrity, and settest me before thy face for ever.\tIn respect of me, thou uphold’st my integrity And putst me before thy face For ever. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tI will abide in thy tabernacle for ever: I will trust in the covert of thy wings.\tI’ll trust your wings to cover it. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd Nebuzaradan captain of the guard took these, and brought them to the king of Babylon to Riblah:\tTis true, the Nebuzaradan captain took them from Riblah, And from Riblah their captains. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tTherefore am I troubled at his presence: when I consider, I am afraid of him.\tTherefore his presence worries me. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd the other issued out of the city against them; so they were in the midst of Israel, some on this side, and some on that side: and they smote them, so that they let none of them remain or escape.\tSince they were in Israel and had slain some men on this side, They let none remain or escape. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd I will bring again the captivity of my people of Israel, and they shall build the waste cities, and inhabit them; and they shall plant vineyards, and drink the wine thereof; they shall also make gardens, and eat the fruit of them.\tThey’ll build waste cities and inhabit them, Plant vineyards and drink wine. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd they brake down the image of Baal, and brake down the house of Baal, and made it a draught house unto this day.\tBaal’s image they brake down. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tthis is nothing else but sorrow of heart.\tThis is but sorrow. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd whatsoever soul it be that doeth any work in that same day, the same soul will I destroy from among his people.\tI will destroy any soul that may do any office in the same day. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tHe that spared not his own Son, but delivered him up for us all, how shall he not with him also freely give us all things?\tHe spared not his son, But he delivered him to all of us, And how freely did he give us all That we had hoped for. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd he said, Hearken ye, all Judah, and ye inhabitants of Jerusalem, and thou king Jehoshaphat, Thus saith the LORD unto you, Be not afraid nor dismayed by reason of this great multitude; for the battle is not yours, but God's.\tBe not afraid, Judah, Be dismayed by the King of Jerusalem, Jehoshaphat. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd from Heshbon unto Ramathmizpeh, and Betonim; and from Mahanaim unto the border of Debir;\tFrom Heshbon to Ramathmizpeh and Betonim, And from Mahinaim to Debir. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd for the east side eastward fifty cubits.\tThe east is fifty thousand cubic meters. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tWho serve unto the example and shadow of heavenly things, as Moses was admonished of God when he was about to make the tabernacle: for, See, saith he, that thou make all things according to the pattern shewed to thee in the mount.\tWho serves as example and shadow, As if Poseidon were admonished to God As he about to make a tabernacle? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd he was sad at that saying, and went away grieved: for he had great possessions.\tThat he was sad to say, And went away grievedly. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThe hands of Zerubbabel have laid the foundation of this house; his hands shall also finish it; and thou shalt know that the LORD of hosts hath sent me unto you.\tZerubbabel's hands have laid the foundation; Their hands will finish it also; And, in the end, the whole thing is made of sand. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd by the border of Dan, from the east side unto the west side, a portion for Asher.\tThe border of Dane with the West Bank. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd if a woman shall put away her husband, and be married to another, she committeth adultery.\tA woman commits adultery if she leave her husband And marry with another. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd they possessed all the coasts of the Amorites, from Arnon even unto Jabbok, and from the wilderness even unto Jordan.\tThey are encamped in all the coasts of the empire, Of Arnon alone, and even to Jabbok. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tfor they wash not their hands when they eat bread.\tThey wash not their hands when they eat bread. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the suburbs of the city shall be toward the north two hundred and fifty, and toward the south two hundred and fifty, and toward the east two hundred and fifty, and toward the west two hundred and fifty.\tThere are suburbs in the city, 250 north, south, and east. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd for thy cattle, and for the beast that are in thy land, shall all the increase thereof be meat.\tThe increase in meat is for your cattle, and for the beasts on your land. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tSo I prophesied as I was commanded: and as I prophesied, there was a noise, and behold a shaking, and the bones came together, bone to his bone.\tI prophesied like myself, and there was shake, and bones came o'er his bones. \n",
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd Jacob went out from Beersheba, and went toward Haran.\tJacob went from Beersheba. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tFor the multitude of the people followed after, crying, Away with him.\tThe crying throng hath followed him. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tThe woman also with whom man shall lie with seed of copulation, they shall both bathe themselves in water, and be unclean until the even.\tA woman that lies a man in copulation seed Shall bathe her in water, and till she be old she will not be clean. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tSo Joab the son of Zeruiah went first up, and was chief.\tJoab went up first, and is now chief. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tYe that fear the LORD, trust in the LORD: he is their help and their shield.\tLord help thee and shield thee! \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd he called unto him the twelve, and began to send them forth by two and two; and gave them power over unclean spirits;\tHe called the twelve and began to send them forth, And gave them power of unclean spirits. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tFor thou shalt be in league with the stones of the field: and the beasts of the field shall be at peace with thee.\tThou art in league with the fields’ stones. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tSo there was great joy in Jerusalem: for since the time of Solomon the son of David king of Israel there was not the like in Jerusalem.\tThere’s great joy in Jerusalem since Salomon Was son to David, the king of Israel. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tfor this man doeth many miracles.\tThis man hath done many miracles. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tTeach me thy way, O LORD, and lead me in a plain path, because of mine enemies.\tTeach me your way, and lead me On a clear path, lest mine enemies take the lead. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tWhen the morning stars sang together, and all the sons of God shouted for joy?\tWhen the stars of morn sang together? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tTherefore the Jews of the villages, that dwelt in the unwalled towns, made the fourteenth day of the month Adar a day of gladness and feasting, and a good day, and of sending portions one to another.\tThe Jew hath made the fourteenth day of Adar, A day of gladness and feast. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tTherefore every one that eateth it shall bear his iniquity, because he hath profaned the hallowed thing of the LORD: and that soul shall be cut off from among his people.\tSo shall every one that eats it profess His hallowed thing to bear his sin. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tPass through the host, and command the people, saying, Prepare you victuals; for within three days ye shall pass over this Jordan, to go in to possess the land, which the LORD your God giveth you to possess it.\tPass you to Jordan, and tell yourself, Within these three days, if you have left Israel, Prepare to conquest. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncomplete\tThen thou shalt say, They be thy servant Jacob's; it is a present sent unto my lord Esau: and, behold, also he is behind us.\tSay that they were Jacob, your servant; The present was sent to your lord Esau. \n",
 'bible_shakespeare.tsv\tNo Error\tNo Error\tEven so, Amen.\tYet amen. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThat we have built us an altar to turn from following the LORD, or if to offer thereon burnt offering or meat offering, or if to offer peace offerings thereon, let the LORD himself require it;\tWe have built an altar to turn to follow God, or if we dare offer Burnt or meat, or offer peace there, Then let us go. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tMy bowels, my bowels!\tMy bowels! \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd a mitre of fine linen, and goodly bonnets of fine linen, and linen breeches of fine twined linen,\tFine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tBut tidings out of the east and out of the north shall trouble him: therefore he shall go forth with great fury to destroy, and utterly to make away many.\tBut the news of the east and north doth trouble him, And so he goes out, with great fury, to destroy many. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThey also that seek after my life lay snares for me: and they that seek my hurt speak mischievous things, and imagine deceits all the day long.\tThey seek out my hurt also, They speak mischievous things, They imagine deceitful things all day. \n',
 'bible_shakespeare.tsv\tNo Error\tIncomplete\tbut turn thee yet again, and thou shalt see greater abominations.\tBut if thou turn’st yet again, thou shalt see greater abominables. \n',
 'bible_shakespeare.tsv\tIncomplete\tNo Error\tPilate saith unto him, What is truth?\tWhat is true? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd they worshipped the dragon which gave power unto the beast: and they worshipped the beast, saying, Who is like unto the beast?\tThey worshiped the dragon, who gave power to a beast. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThou shalt not eat it; that it may go well with thee, and with thy children after thee, when thou shalt do that which is right in the sight of the LORD.\tThou shalt not eat it, That it may go well with thyself and thy children after. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd Serug lived after he begat Nahor two hundred years, and begat sons and daughters.\tSerug lived after her two hundred years of marriage to Nahor. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tI love the LORD, because he hath heard my voice and my supplications.\tI love the Lord, For he hath heard my voice and what I suggest. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tBut when the people of the land shall come before the LORD in the solemn feasts, he that entereth in by the way of the north gate to worship shall go out by the way of the south gate; and he that entereth by the way of the south gate shall go forth by the way of the north gate: he shall not return by the way of the gate whereby he came in, but shall go forth over against it.\tWhen the Romans come to solemn feasts, Those that enter at the north gate for worship Shall not go to the south gate, but go over it. \n',
 "bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd consulted that they might take Jesus by subtilty, and kill him.\tHe hath consult'd That they may take Jesu with subtilty and kill him. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tIn the twilight, in the evening, in the black and dark night:\tO black and dark night! \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tJudge not, that ye be not judged.\tJudge not. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tLift up your heads, O ye gates; and be ye lift up, ye everlasting doors; and the King of glory shall come in.\tLift thy head; the King welcome. \n',
 'bible_shakespeare.tsv\tNo Error\tIncomplete\tHe disappointeth the devices of the crafty, so that their hands cannot perform their enterprise.\tHe does disappoint the crafty, that he cannot perform his office. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tbut he that cometh after me is mightier than I, whose shoes I am not worthy to bear: he shall baptize you with the Holy Ghost, and with fire:\tHe that comes after me, though with no shoe of mine, is stronger than myself. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tBlessed be the God and Father of our Lord Jesus Christ, who hath blessed us with all spiritual blessings in heavenly places in Christ:\tGod and our father, Jesus Christ, Bless us in heaven! \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd how I kept back nothing that was profitable unto you, but have shewed you, and have taught you publickly, and from house to house,\tBut what I have kept from you back is nothing profitable: I'll make thee show, and teach thee publicly from the house to the house. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tArabia, and all the princes of Kedar, they occupied with thee in lambs, and rams, and goats: in these were they thy merchants.\tThey occupied Kent with lambs, rams, and goats. \n',
 "bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd the soldiers' counsel was to kill the prisoners, lest any of them should swim out, and escape.\tSoldiers give counsel To kill prisoners, lest any of them swim out and escape. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the second lot came forth to Simeon, even for the tribe of the children of Simeon according to their families: and their inheritance was within the inheritance of the children of Judah.\tEven sir Simeon’s second lot is in Judah’s blood. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\twherefore camest thou not unto me?\tWhere art thou? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tBehold, for peace I had great bitterness: but thou hast in love to my soul delivered it from the pit of corruption: for thou hast cast all my sins behind thy back.\tI am great bitter, but thou lovest me so, That thou throwst all my sins behind thy back. \n',
 "bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd shall put thereon the covering of badgers' skins, and shall spread over it a cloth wholly of blue, and shall put in the staves thereof.\tFor the badgers themselves, they cover their skins, and there they spread A complete cloth of blue. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThen Benhadad came forth to him; and he caused him to come up into the chariot.\tWhy, then Benedad came to him; and therefore came to fetch him to the carriages. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tAll that cometh is vanity.\tAll that is vanity is to be a knave. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd whatsoever more shall be needful for the house of thy God, which thou shalt have occasion to bestow, bestow it out of the king's treasure house.\tAnd therein need any more, To bestow a house of treasure of the king. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tBe it known unto the king, that the Jews which came up from thee to us are come unto Jerusalem, building the rebellious and the bad city, and have set up the walls thereof, and joined the foundations.\tI have known the Jew came from Jerusalem, Built a bad, rebellious city, and joined with foundations. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tMoreover concerning the stranger, which is not of thy people Israel, but is come from a far country for thy great name's sake, and thy mighty hand, and thy stretched out arm; if they come and pray in this house;\tBe it so with a stranger come from a far country, Your great name and your stretched arm, But not as an Israeli. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tShall the thing formed say to him that formed it, Why hast thou made me thus?\tWhy then, thou art formed for ’t. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd they tied unto it a lace of blue, to fasten it on high upon the mitre; as the LORD commanded Moses.\tThey tied the mitre to blue lace, Which on the order of Moses did fasten them. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tWherefore, behold, I send unto you prophets, and wise men, and scribes: and some of them ye shall kill and crucify; and some of them shall ye scourge in your synagogues, and persecute them from city to city:\tTherefore I send Some prophets, wise men, and writers, That you will kill and crucify them. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tSo Zedekiah the king sware secretly unto Jeremiah, saying, As the LORD liveth, that made us this soul, I will not put thee to death, neither will I give thee into the hand of these men that seek thy life.\tThe king, secretly, Zedekiah, told Joseph thou wilt neither die nor die By the Lord’s life that made this soul. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the LORD plagued Pharaoh and his house with great plagues because of Sarai Abram's wife.\tFor Sarai Abram’s wife, It was a great plague upon the Pharaoh and his house. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tWhy dost thou strive against him?\tWhy dost thou try thy opposition against him? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tFor a certain woman, whose young daughter had an unclean spirit, heard of him, and came and fell at his feet:\tHe hath been heard of by a young woman’s daughter; she came and fell upon his feet. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncomplete\tAnd ye murmured in your tents, and said, Because the LORD hated us, he hath brought us forth out of the land of Egypt, to deliver us into the hand of the Amorites, to destroy us.\tThou hast murmured in thy tent And said that because God hated us, He brought us out of Egypt to destroy us. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tHe shutteth his eyes to devise froward things: moving his lips he bringeth evil to pass.\tHe shuts his eyes and lips, Moving so the cause of evil. \n',
 'bible_shakespeare.tsv\tNo Error\tNo Error\tGo therefore now, and work; for there shall no straw be given you, yet shall ye deliver the tale of bricks.\tGo to work now, and there will be no straw given thee, But deliver the story of bricks. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tSo Nebuzaradan the captain of the guard took them, and brought them to the king of Babylon to Riblah.\tTis true, guardsman Nebuzaradan took them from Riblah. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tEvery man of the children of Israel shall pitch by his own standard, with the ensign of their father's house: far off about the tabernacle of the congregation shall they pitch.\tNear the far off tabernacle, every one doth pitch in his standard. \n",
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tHowl, ye ships of Tarshish; for it is laid waste, so that there is no house, no entering in: from the land of Chittim it is revealed to them.\tWhip, ye Tartarists, For if it lay to waste there's no house nor entrance. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tBut ye say, If a man shall say to his father or mother, It is Corban, that is to say, a gift, by whatsoever thou mightest be profited by me; he shall be free.\tIf thou say’st “father” or “mother,” Cordan is free. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd again, whom should I serve?\tWhat should I serve again? \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tNow if thou commit no adultery, yet if thou kill, thou art become a transgressor of the law.\tIf thou commit no adultery, Become a traitor to the state, and the state shall punish the violator. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd he said, I will make all my goodness pass before thee, and I will proclaim the name of the LORD before thee; and will be gracious to whom I will be gracious, and will shew mercy on whom I will shew mercy.\tI’ll make all my goodness before thee, And proclaim my name as a gracious man. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tHow beautiful upon the mountains are the feet of him that bringeth good tidings, that publisheth peace; that bringeth good tidings of good, that publisheth salvation; that saith unto Zion, Thy God reigneth!\tWhat a beauty is there in the mountains; He brings good news, publishes peace, and says your God reigns. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tFor she did not know that I gave her corn, and wine, and oil, and multiplied her silver and gold, which they prepared for Baal.\tNor did she know That I gave her corn, wine, and oil, And that I multiplied the silver and gold They prepared for Baal. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd he sent him away to his house, saying, Neither go into the town, nor tell it to any in the town.\tHe said he would not go to town and would not tell anyone of it. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncomplete\tAnd the children of Heth answered Abraham, saying unto him,\tAbraham answered my children. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd these are they by the way side, where the word is sown; but when they have heard, Satan cometh immediately, and taketh away the word that was sown in their hearts.\tThey are on the way, but when they have heard Satan come, he will immediately take away the word That is seeded in their hearts. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThey shall be holy unto their God, and not profane the name of their God: for the offerings of the LORD made by fire, and the bread of their God, they do offer: therefore they shall be holy.\tThey are holy to God’s, and will not profane themselves. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd take your father and your households, and come unto me: and I will give you the good of the land of Egypt, and ye shall eat the fat of the land.\tTake from you your father and your household, Come to me and I will give you the fat of Egypt. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tBlessed is the man that heareth me, watching daily at my gates, waiting at the posts of my doors.\tBless me a man that every day watches my gates And waits on my posts. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd the prince of the tribe of the children of Asher, Ahihud the son of Shelomi.\tAhihud! \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd his lord was wroth, and delivered him to the tormentors, till he should pay all that was due unto him.\tHis lord is angry, and he delivers him To a tormenting torturer, till he pay all he is due. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tWith whomsoever of thy servants it be found, both let him die, and we also will be my lord's bondmen.\tLet him die, my lord, And our bond to him also. \n",
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tFor which of you, intending to build a tower, sitteth not down first, and counteth the cost, whether he have sufficient to finish it?\tWho of you amongst us First wishing to build a tower, Count the cost and know whether he has enough to finish it? \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThus ye shall be filled at my table with horses and chariots, with mighty men, and with all men of war, saith the Lord GOD.\tGod be wi' you, my table is full of horses, chariots, mighty men, and all! \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tLet the day perish wherein I was born, and the night in which it was said, There is a man child conceived.\tLet the day wherein I was born And the night wherein the man was said to be dead Let him rest his soul. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tThe LORD hath loved him: he will do his pleasure on Babylon, and his arm shall be on the Chaldeans.\tGod lieb’st babylon, and his arm is in the Chaldean gods. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tFor now thou numberest my steps: dost thou not watch over my sin?\tNow are you number'd in my steps; dost thou not watch over my sin? \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tfor my soul is wearied because of murderers.\tThe murderers do my soul weary. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd she had a sister called Mary, which also sat at Jesus' feet, and heard his word.\tShe was Mary’s sister, who listened to the word of Jesus also. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd the Tirshatha said unto them, that they should not eat of the most holy things, till there stood up a priest with Urim and with Thummim.\tTirshatha said they would not eat the most holy till the priests, Urim and Thumbim, stood together. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThe trees of the LORD are full of sap; the cedars of Lebanon, which he hath planted;\tHe hath planted cedar trees in Lebanon. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tShuppim also, and Huppim, the children of Ir, and Hushim, the sons of Aher.\tUpim and Hush! \n',
 "bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd David said unto Abiathar, I knew it that day, when Doeg the Edomite was there, that he would surely tell Saul: I have occasioned the death of all the persons of thy father's house.\tThat day, when Doeg the Edomite was there, David knew he had told Salvation that I was dead. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tHowbeit he meaneth not so, neither doth his heart think so; but it is in his heart to destroy and cut off nations not a few.\tHe thinks not so, but his purpose is to destroy nations and cut them off. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd the sabbath of the land shall be meat for you; for thee, and for thy servant, and for thy maid, and for thy hired servant, and for thy stranger that sojourneth with thee.\tThere’s meat for you, for your servant, for your maid, for stranger that you have hired. \n',
 "bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tWhile the Pharisees were gathered together, Jesus asked them,\tWhen the Pharisees were gather'd, Jesu asked the Pharisees what they were. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tHe that hath received his testimony hath set to his seal that God is true.\tHe’ll put a seal upon him That God’s trueness is in him. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd Reuben spake unto his father, saying, Slay my two sons, if I bring him not to thee: deliver him into my hand, and I will bring him to thee again.\tReuben, if I bring not thy two sons, Slaying them both! \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tThey were amazed, they answered no more: they left off speaking.\tThey were amazed, they answered not, they left off their speech. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tI have longed for thy salvation, O LORD; and thy law is my delight.\tI have long for your salvation; And your law takes delight in me. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd she answered and said unto him, Yes, Lord: yet the dogs under the table eat of the children's crumbs.\tYet the dogs under the table Eat children’s crumbs. \n",
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tSalvation is far from the wicked: for they seek not thy statutes.\tBad men seek not your laws to help. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThe children of Ater of Hezekiah, ninety and eight.\tO, ’tis ninety-five. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd he left off talking with him, and God went up from Abraham.\tHe left talking, and God went with him to Abraham. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd when Saul looked behind him, David stooped with his face to the earth, and bowed himself.\tWhen David looked behind him, he stooped in his face and bowed. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tThen Nebuzaradan the captain of the guard carried away captive certain of the poor of the people, and the residue of the people that remained in the city, and those that fell away, that fell to the king of Babylon, and the rest of the multitude.\tThe guardsman Nebuzaradan Carry away some poor men captured, And the rest that remain in the city. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tFor I have not shunned to declare unto you all the counsel of God.\tI would not be so curst To tell you all the counsels of God. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tGrudge not one against another, brethren, lest ye be condemned: behold, the judge standeth before the door.\tGrudge not one against another, lest thou be condemn'd. \n",
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tJesus therefore, knowing all things that should come upon him, went forth, and said unto them, Whom seek ye?\tSo went Jesu out, knowing all, and he said to them Who seeks thee? \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tTo overthrow their seed also among the nations, and to scatter them in the lands.\tTo overthrow their seeds among nations and scatter them thus. \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tBut that on the good ground are they, which in an honest and good heart, having heard the word, keep it, and bring forth fruit with patience.\tBut on good ground they keep their ears and produce fruit With patience. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tIs not this written in the book of Jasher?\tWas not this writ in Jasher? \n',
 'bible_shakespeare.tsv\tMeaning Change\tNo Error\tAnd the people with one accord gave heed unto those things which Philip spake, hearing and seeing the miracles which he did.\tMen shall hear Philip’s words, And behold what miracle he did, Hearing and seeing what miracle he did. \n',
 'bible_shakespeare.tsv\tNo Error\tIncomplete\tAnd when Samuel had caused all the tribes of Israel to come near, the tribe of Benjamin was taken.\tWhen he came all near Israel, Samuel took Benjamin. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tMeaning Change\tThere are not found that returned to give glory to God, save this stranger.\tNo man found back But this stranger, to give God glory. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tAnd there was a cloud that overshadowed them: and a voice came out of the cloud, saying, This is my beloved Son: hear him.\tThe cloud hath overshadowed them, And came out a voice saying “This is their loving son.” Why, that’s the man. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tthe LORD is the strength of my life; of whom shall I be afraid?\tMy life is strong; what fear I? \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd in their hands they shall bear thee up, lest at any time thou dash thy foot against a stone.\tThey are at your feet, and therefore at any time you’ll dash your foot with stones. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd, behold, men passed by, and saw the carcase cast in the way, and the lion standing by the carcase: and they came and told it in the city where the old prophet dwelt.\tThe men passed the carcass, and saw the lion standing by, And came thither to the city where old Prosper lived. \n',
 "bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tIn the first place went the standard of the camp of the children of Judah according to their armies: and over his host was Nahshon the son of Amminadab.\tThe camp was the standard For the Judah's army in first place, and Nahshon's host. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tA man that flattereth his neighbour spreadeth a net for his feet.\tA man that flatters his neighbor spreads a net upon his feet. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd he said unto them, What manner of communications are these that ye have one to another, as ye walk, and are sad?\tHow wouldst thou have communication with another, When thou dost walk and be sad? \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tNo Error\tAnd all the men of Shechem gathered together, and all the house of Millo, and went, and made Abimelech king, by the plain of the pillar that was in Shechem.\tAll the gods at Shechem gathered, And all the gods at Millo went To make Abimelech king. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd Abner said unto David, I will arise and go, and will gather all Israel unto my lord the king, that they may make a league with thee, and that thou mayest reign over all that thine heart desireth.\tAber said he would rise and go And gather all the people of Israel, that thou mightst make a league with thee And mayst rule all that thy desire shall his heart desire. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tGod layeth up his iniquity for his children: he rewardeth him, and he shall know it.\tGod lays his iniquity on his children, and he rewards them. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tYe have seen what I did unto the Egyptians, and how I bare you on eagles' wings, and brought you unto myself.\tYou have seen what I have done to the Egyptians And how I bare thee in the wings of eagles. \n",
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tThey shall have like portions to eat, beside that which cometh of the sale of his patrimony.\tThey’ll have, to eat, a portion like himself, Save that which comes to market his wares. \n',
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tIs not my word like as a fire?\tMy word is like fire? \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tAnd he made the staves of shittim wood, and overlaid them with gold.\tHe made the staves of shittim wood and overlaid them with gold. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tAnd Benaiah brought the king word again, saying, Thus said Joab, and thus he answered me.\tJoab says again “Ben” is his word for the king. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tAnd Moses gave the money of them that were redeemed unto Aaron and to his sons, according to the word of the LORD, as the LORD commanded Moses.\tThe duke of Moor hath given money to Aaron and his sons. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd I brought you into the land of the Amorites, which dwelt on the other side Jordan; and they fought with you: and I gave them into your hand, that ye might possess their land; and I destroyed them from before you.\tI brought thee from the other side An Amorites that lived on the other side of Jordan And fought with you. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd Samuel said to all the people, See ye him whom the LORD hath chosen, that there is none like him among all the people?\tSaw’st thou men that are not like Samuel? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tAnd when he humbled himself, the wrath of the LORD turned from him, that he would not destroy him altogether: and also in Judah things went well.\tWhen he humbled himself, his wrath Turned itself into nothing, and things in Judah went on as well as upon him. \n',
 'bible_shakespeare.tsv\tIncorrect/New Information\tIncorrect/New Information\tFor I determined not to know any thing among you, save Jesus Christ, and him crucified.\tI have resolved Not to know of him, but Jesus Christ and his crucifixion. \n',
 "bible_shakespeare.tsv\tMeaning Change\tIncomplete\tWhile he yet spake, there cometh one from the ruler of the synagogue's house, saying to him, Thy daughter is dead; trouble not the Master.\tWhen he speaks still, there comes one that says your daughter is dead, And that synagogue masters should not trouble him. \n",
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tor who hath been his counsellor?\tOr who is he that counsels? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tThat which I speak, I speak it not after the Lord, but as it were foolishly, in this confidence of boasting.\tI will not speak that out of thinking it foolish. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tThen the congregation shall judge between the slayer and the revenger of blood according to these judgments:\tThe congregation shall judge Between the slain and the revenged, According to this decree. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tAnd the princes of the Philistines were wroth with him; and the princes of the Philistines said unto him, Make this fellow return, that he may go again to his place which thou hast appointed him, and let him not go down with us to battle, lest in the battle he be an adversary to us: for wherewith should he reconcile himself unto his master?\tWhere should he reconcile himself with his master? \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tAnd Jacob lifted up his eyes, and looked, and, behold, Esau came, and with him four hundred men.\tJacob lifted his eyes And looked to him, and there came Esau. \n',
 'bible_shakespeare.tsv\tMeaning Change\tIncorrect/New Information\tFor all tables are full of vomit and filthiness, so that there is no place clean.\tAll the tables are full of vomit and filth, And therefore are they washed. \n',
 "bible_shakespeare.tsv\tIncomplete\tMeaning Change\tI will be surety for him; of my hand shalt thou require him: if I bring him not unto thee, and set him before thee, then let me bear the blame for ever:\tI am sure of him; if I bring him not to thee and put him not before thee, I'll lay the blame on him forever. \n",
 'bible_shakespeare.tsv\tNo Error\tMeaning Change\tAnd the men did so; and took two milch kine, and tied them to the cart, and shut up their calves at home:\tThe men took two milch kines from the cart, tied them in a cart, shut up their calves at home. \n',
 'bible_shakespeare.tsv\tIncomplete\tIncomplete\tTurn us again, O God of hosts, and cause thy face to shine; and we shall be saved.\tTurn us again, shine thy face, and we shall be saved. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tIs any among you afflicted?\tHast any of you affected? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tJesus said, Take ye away the stone.\tTake up the stones. \n',
 'bible_shakespeare.tsv\tMeaning Change\tMeaning Change\tAnd the altar of burnt offering with all his furniture, and the laver and his foot,\tThere is an altar of burned offerings, and all his furniture, For which his foot is the sole of contention. \n',
 'bible_shakespeare.tsv\tIncomplete\tMeaning Change\tDo we provoke the Lord to jealousy?\tProvoke we jealousy? \n',
 'bible_shakespeare.tsv\tIncomplete\tIncorrect/New Information\tRighteous art thou, O LORD, and upright are thy judgments.\tThou art right and upright. \n',
 'bible_shakespeare.tsv\tNo Error\tIncorrect/New Information\tLet those that fear thee turn unto me, and those that have known thy testimonies.\tO, turn to me, those that fear thee, and they shall know What thou testifies. \n',
 ...]

In [161]: x = [i.strip().split("\t") for i in x]

In [162]: x
Out[162]: 
[['direction', 'Tstar_Error', 'Strap_Error', '{Input} Text', '{Output} Text'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And came and preached peace to you which were afar off, and to them that were nigh.',
  'Came, and preached peace to you distant,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'The two pillars, one sea, and twelve brasen bulls that were under the bases, which king Solomon had made in the house of the LORD: the brass of all these vessels was without weight.',
  'Two sea-pillars and brasen bullshits under the bases unweighted by King Solomon.'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'And none shall appear before me empty.',
  'Before me none empty appear.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And all the people saw the cloudy pillar stand at the tabernacle door: and all the people rose up and worshipped, every man in his tent door.',
  'All saw a cloudy pillar stand at the tent door, and rose and worshipped.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Take the millstones, and grind meal: uncover thy locks, make bare the leg, uncover the thigh, pass over the rivers.',
  'Take millstones and grind your meal, uncover your locks and bare your legs.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Now the rest of the acts of Jeroboam, and all that he did, and his might, how he warred, and how he recovered Damascus, and Hamath, which belonged to Judah, for Israel, are they not written in the book of the chronicles of the kings of Israel?',
  "Not written in his acts, Damascus and Judah's rest,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'He that tilleth his land shall have plenty of bread: but he that followeth after vain persons shall have poverty enough.',
  "He'll have plenty o'er his land but poor enough;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And they shall amerce him in an hundred shekels of silver, and give them unto the father of the damsel, because he hath brought up an evil name upon a virgin of Israel: and she shall be his wife; he may not put her away all his days.',
  'Since he brought up an evil name in Israeli virgin, to give'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'I have taught thee in the way of wisdom; I have led thee in right paths.',
  "I've taught thee the right paths,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And he hath on his vesture and on his thigh a name written, KING OF KINGS, AND LORD OF LORDS.',
  'His vestured name, written in King and Lord,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "But he himself went a day's journey into the wilderness, and came and sat down under a juniper tree: and he requested for himself that he might die; and said, It is enough; now, O LORD, take away my life; for I am not better than my fathers.",
  'But went the wilderness for a day, came beneath the juniper tree, and bid him die.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For they have taken of their daughters for themselves, and for their sons: so that the holy seed have mingled themselves with the people of those lands: yea, the hand of the princes and rulers hath been chief in this trespass.',
  'They took daughters and sons to merge those peoples,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'For he that is not against us is on our part.',
  'He wad na wrang us against him,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'A continual dropping in a very rainy day and a contentious woman are alike.',
  'Like constant drops on very rainy days, and contentious woman.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the table and all his vessels, and the candlestick and his vessels, and the altar of incense,',
  'With table, candlestick, vessels, and altar,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Take ye therefore good heed unto yourselves; for ye saw no manner of similitude on the day that the LORD spake unto you in Horeb out of the midst of the fire:',
  'You saw no like sight on day when God spoke to you in Horneb.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Making the word of God of none effect through your tradition, which ye have delivered: and many such like things do ye.',
  'And making thy tradition unblest with God!'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And he had much business in the cities of Judah: and the men of war, mighty men of valour, were in Jerusalem.',
  'In Jerusalem he had a waft of business;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'He that followeth after righteousness and mercy findeth life, righteousness, and honour.',
  'Those who follow righteousness and mercy find life and honour.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'But I will send a fire on the wall of Gaza, which shall devour the palaces thereof:',
  'But I wad send the fire to the Gaza wall,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Be ye therefore followers of God, as dear children;',
  'Like children of God, follow Him! I pray,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Then will I make this house like Shiloh, and will make this city a curse to all the nations of the earth.',
  "Make this house like Shailoh's, and make all nations curse."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'No man that hath a blemish of the seed of Aaron the priest shall come nigh to offer the offerings of the LORD made by fire: he hath a blemish; he shall not come nigh to offer the bread of his God.',
  "No priest Aaron's seed blemish nor come to offer"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'She standeth in the top of high places, by the way in the places of the paths.',
  "She stands by the high places' top,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'But know ye for certain, that if ye put me to death, ye shall surely bring innocent blood upon yourselves, and upon this city, and upon the inhabitants thereof: for of a truth the LORD hath sent me unto you to speak all these words in your ears.',
  "Know, surely, bring this city and inhabitants' blood to me."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "Thou hypocrite, cast out first the beam out of thine own eye, and then shalt thou see clearly to pull out the mote that is in thy brother's eye.",
  "And cast first your hypocrites' beam, and clear then to pull your brother's mote."],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And the king of Israel went out, and smote the horses and chariots, and slew the Syrians with a great slaughter.',
  'And shot horses and chariots, and slain Syrians;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And say, Hear the word of the LORD, O king of Judah, that sittest upon the throne of David, thou, and thy servants, and thy people that enter in by these gates:',
  'Say, hear what God David stooped on his throne,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And Abraham gave all that he had unto Isaac.',
  'And Abraham gave him all he had,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'And we went over the brook Zered.',
  "Zered, o'er the river yon went,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Then said the Jews unto him, Thou art not yet fifty years old, and hast thou seen Abraham?',
  'Not yet fifty years old, and hath ye seen Abraham?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'the treacherous dealers have dealt treacherously; yea, the treacherous dealers have dealt very treacherously.',
  'The traffickers, very treacherous dealt,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And thou shalt make a vail of blue, and purple, and scarlet, and fine twined linen of cunning work: with cherubims shall it be made:',
  'With cherubims make a vaunt of blue, purple, scarlet, fine twined linen.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'In the third year of his reign, he made a feast unto all his princes and his servants; the power of Persia and Media, the nobles and princes of the provinces, being before him:',
  "The third year of his reign, celebrates Persia's power and media:"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'I thank God that I baptized none of you, but Crispus and Gaius;',
  'God bless, I baptized you none but Crespus and Gaius;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And some of them that stood by, when they heard it, said, Behold, he calleth Elias.',
  '"Some of them," said he, "we call him Elias,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And there were made on them, on the doors of the temple, cherubims and palm trees, like as were made upon the walls; and there were thick planks upon the face of the porch without.',
  'Chiels and palm trees at temple doors and thick planks on porch face.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Then hear thou in heaven their prayer and their supplication, and maintain their cause.',
  'Then hear their prayer, and support their cause;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The hands of the pitiful women have sodden their own children: they were their meat in the destruction of the daughter of my people.',
  'Wretched women slaughtered their children;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'The black horses which are therein go forth into the north country; and the white go forth after them; and the grisled go forth toward the south country.',
  'The black horses there went the north, the white horses went the south;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'But the children of Benjamin gathered themselves together out of the cities unto Gibeah, to go out to battle against the children of Israel.',
  'And gathered in Giraltar to fight with Israel:'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And I will make thy seed as the dust of the earth: so that if a man can number the dust of the earth, then shall thy seed also be numbered.',
  "If men can number your earth's dust,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Serug lived after he begat Nahor two hundred years, and begat sons and daughters.',
  "Serug lived 'gainst Nahor after 200 years of marriage."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'But I will put hooks in thy jaws, and I will cause the fish of thy rivers to stick unto thy scales, and I will bring thee up out of the midst of thy rivers, and all the fish of thy rivers shall stick unto thy scales.',
  "But I'll put the hooks in your jaws, and thy fish will stick to your scales."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "And she had a sister called Mary, which also sat at Jesus' feet, and heard his word.",
  "She was also Mary's sister, who listened to Jesus' word,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And the evil spirit answered and said, Jesus I know, and Paul I know; but who are ye?',
  'I know Jesus and Paul, but what do ye know?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And in the seventh day the priest shall look on the plague: and, behold, if the scall spread not, and there be in it no yellow hair, and the scall be not in sight deeper than the skin;',
  'The priest sought on seventh day not hairy, and scall deeper than skin,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  '(Howbeit there came other boats from Tiberias nigh unto the place where they did eat bread, after that the Lord had given thanks:)',
  'While other boats came back to Tiberias after they ate the bread,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And he did that which was evil in the sight of the LORD his God, and humbled not himself before Jeremiah the prophet speaking from the mouth of the LORD.',
  'Had done wicked, unhumiliated before prophet Joel speaking;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he left off talking with him, and God went up from Abraham.',
  'And left him talking, and God went to Abraham.'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'But ye gave the Nazarites wine to drink; and commanded the prophets, saying, Prophesy not.',
  'But gied the Nazis drink wine, and told the Prophets not prophesying.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'The LORD hath loved him: he will do his pleasure on Babylon, and his arm shall be on the Chaldeans.',
  "God loved Babylon, and in Chaldeans' arms"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And by him shall be the tribe of Manasseh: and the captain of the children of Manasseh shall be Gamaliel the son of Pedahzur.',
  "As manasseh tribe's captain Gamaliel,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And that year they vexed and oppressed the children of Israel: eighteen years, all the children of Israel that were on the other side Jordan in the land of the Amorites, which is in Gilead.',
  "On Jordan's other side they annoy'd and oppressed."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Pass through the host, and command the people, saying, Prepare you victuals; for within three days ye shall pass over this Jordan, to go in to possess the land, which the LORD your God giveth you to possess it.',
  'Pass Jordan and tell up to three days prepare'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'That ye may be blameless and harmless, the sons of God, without rebuke, in the midst of a crooked and perverse nation, among whom ye shine as lights in the world;',
  'Thy sons may be blameless, harmless in perverse crooked nation,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Moreover the multitude of thy strangers shall be like small dust, and the multitude of the terrible ones shall be as chaff that passeth away: yea, it shall be at an instant suddenly.',
  'And thy strangers like small dust, and chaff like to pass away.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And they could not eat thereof.',
  'It is not that they can eat;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Because I have called, and ye refused; I have stretched out my hand, and no man regarded;',
  "I call'd and ye refused; so I stretch'd my hand and none sought;"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And the king left ten women, which were concubines, to keep the house.',
  'The King left ten concubine wives to keep the house;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And Israel served the LORD all the days of Joshua, and all the days of the elders that overlived Joshua, and which had known all the works of the LORD, that he had done for Israel.',
  'And served Judah, and elders who overlived and knew all their works.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And Solomon determined to build an house for the name of the LORD, and an house for his kingdom.',
  'And Solomon decreed that he would build a house'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Judah did evil in the sight of the LORD, and they provoked him to jealousy with their sins which they had committed, above all that their fathers had done.',
  'Judah did evil, provoked fathers jealous of their sins above;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And he turned unto her by the way, and said, Go to, I pray thee, let me come in unto thee; (for he knew not that she was his daughter in law.)',
  'He turned her by the way and said, "Go! He knew not his daughter in law.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And he shall offer the one of the turtledoves, or of the young pigeons, such as he can get;',
  'Offers, as he may, turtle-doves or young pigeons;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And when Saul looked behind him, David stooped with his face to the earth, and bowed himself.',
  "David stoop'd and bow'd his face when Saul looked behind."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Abraham rose up early in the morning, and took bread, and a bottle of water, and gave it unto Hagar, putting it on her shoulder, and the child, and sent her away: and she departed, and wandered in the wilderness of Beersheba.',
  'Adam rose early, took bread and bottle, gave his shoulder, and left'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'Have any of the rulers or of the Pharisees believed on him?',
  'He deemed?--Whether rules or pharisees,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And it came to pass after this, that the king of the children of Ammon died, and Hanun his son reigned in his stead.',
  "And after him died and succeeded Hanun's son."],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'For I heard the defaming of many, fear on every side.',
  "I heard many a defam'd, and every side fear'd."],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'who will hearken and hear for the time to come?',
  'Who will listen at the time to come'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And when thou prayest, thou shalt not be as the hypocrites are: for they love to pray standing in the synagogues and in the corners of the streets, that they may be seen of men.',
  'As they love praying standing at synagogues and streets, hypocrites!'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Behold, he taketh away, who can hinder him?',
  'Behold! who can hinder him? Then who can hinder'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'For now thou numberest my steps: dost thou not watch over my sin?',
  "Now ye've number'd my steps: do not watch over my sin?"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Thus saith the LORD of hosts, the God of Israel, saying; Ye and your wives have both spoken with your mouths, and fulfilled with your hand, saying, We will surely perform our vows that we have vowed, to burn incense to the queen of heaven, and to pour out drink offerings unto her: ye will surely accomplish your vows, and surely perform your vows.',
  "Your mouths, and wives, surely vow'd, and drink offerings fulfilled;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Though he be fruitful among his brethren, an east wind shall come, the wind of the LORD shall come up from the wilderness, and his spring shall become dry, and his fountain shall be dried up: he shall spoil the treasure of all pleasant vessels.',
  'Though fruitful among his brethren, he would spoil all pleasant vessels.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'For in that he died, he died unto sin once: but in that he liveth, he liveth unto God.',
  'He died in one sin--but dies because he lives for God.'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'For all tables are full of vomit and filthiness, so that there is no place clean.',
  'All tables were full of vomit and filthily, so unclean'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'And Joshua rose early in the morning, and the priests took up the ark of the LORD.',
  'Joshua rose early in the morning, and priests took the ark.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And the Levites stood with the instruments of David, and the priests with the trumpets.',
  "Leviticus stood with David's instruments, and priests trumpets;"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Then said they unto him, Where is thy Father?',
  'Where art thou now, thy Father? where art thou?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And for a spirit of judgment to him that sitteth in judgment, and for strength to them that turn the battle to the gate.',
  'To judge him, and strength to turn the battle to gate.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Whoso robbeth his father or his mother, and saith, It is no transgression; the same is the companion of a destroyer.',
  "Robber of father or mother, and it transgress'd"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And it came to pass, when Jesus had ended these sayings, the people were astonished at his doctrine:',
  "When these words end, Jesus' doctrine astonied"],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'And the rest, some on boards, and some on broken pieces of the ship.',
  "Rest on the boards and some on the ship's broken pieces."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And unto Caleb the son of Jephunneh he gave a part among the children of Judah, according to the commandment of the LORD to Joshua, even the city of Arba the father of Anak, which city is Hebron.',
  "To Joshua's father Jephunneh's Caleb gave"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'The words of Nehemiah the son of Hachaliah.',
  "And Nehemiah's words are sae sweet,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Is not the gleaning of the grapes of Ephraim better than the vintage of Abiezer?',
  "Is it not better Ephraim's wine than Abiezer?"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the rest of the men which were not killed by these plagues yet repented not of the works of their hands, that they should not worship devils, and idols of gold, and silver, and brass, and stone, and of wood: which neither can see, nor hear, nor walk:',
  'Yet the rest, not slain by these plagues, repents to gold, silver, and brass,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'or wilt thou leave thy labour to him?',
  'Or wilt thou leave thy ain work to him?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Thou shalt also make a table of shittim wood: two cubits shall be the length thereof, and a cubit the breadth thereof, and a cubit and a half the height thereof.',
  'Also make a table of shit-wood equal two cubits and half.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And when Peter saw it, he answered unto the people, Ye men of Israel, why marvel ye at this?',
  'Petrarch, when he saw it, wondered why this Israeli marveled.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And if she had at all an husband, when she vowed, or uttered ought out of her lips, wherewith she bound her soul;',
  "If she had a husband at all while she vow'd or declared."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'He delivered me from my strong enemy, and from them which hated me: for they were too strong for me.',
  'Delivered me to a foe too strong to hate.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Four tables were on this side, and four tables on that side, by the side of the gate; eight tables, whereupon they slew their sacrifices.',
  'Four tables were on this side, and eight were on that side.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For yet a little while, and he that shall come will come, and will not tarry.',
  'The little while still, and he will come'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  "And when the ass saw the angel of the LORD, she fell down under Balaam: and Balaam's anger was kindled, and he smote the ass with a staff.",
  'The ass fell under Salaam, in anger shot with staff,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And David was displeased, because the LORD had made a breach upon Uzza: wherefore that place is called Perezuzza to this day.',
  "David uplighted by Perezuzza's assail,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "With whomsoever of thy servants it be found, both let him die, and we also will be my lord's bondmen.",
  "Let him die, and we'll bond our lord also."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Let thy fountain be blessed: and rejoice with the wife of thy youth.',
  'Thy fountain was blessed, and thy wife rejoiced;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And a mitre of fine linen, and goodly bonnets of fine linen, and linen breeches of fine twined linen,',
  "Wi' fine, fine, and fine linens,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'The nethermost chamber was five cubits broad, and the middle was six cubits broad, and the third was seven cubits broad: for without in the wall of the house he made narrowed rests round about, that the beams should not be fastened in the walls of the house.',
  'Most chambers five-cubits wide, middle six-cubits wide, and third--'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'For if Jesus had given them rest, then would he not afterward have spoken of another day.',
  'Then if Jesus gave them rest, he would not talk of another day.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And when he had sent the multitudes away, he went up into a mountain apart to pray: and when the evening was come, he was there alone.',
  'He went up the mountain to pray, and in the evening alone'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'And Jehoshaphat stood in the congregation of Judah and Jerusalem, in the house of the LORD, before the new court,',
  'At Judah and Jerusalem, Jehoshaphat stood before the new court,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But after that I am risen, I will go before you into Galilee.',
  "But I'll go to Galilee before you,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Give therefore thy servant an understanding heart to judge thy people, that I may discern between good and bad: for who is able to judge this thy so great a people?',
  'Give understanding heart to judge, I can discern between good and bad.'],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'And the man smote him, so that in smiting he wounded him.',
  "As he was wounded by a man's smiting,"],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  "Brethren, my heart's desire and prayer to God for Israel is, that they might be saved.",
  'To save Israel, and pray to the Lord,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And Pharaoh awoke, and, behold, it was a dream.',
  'Awaking the Pharaoh, and in a dream'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And they that shall be of thee shall build the old waste places: thou shalt raise up the foundations of many generations; and thou shalt be called, The repairer of the breach, The restorer of paths to dwell in.',
  "To build old places of waste, and raise what many generations hath hath ta'en."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And them that are turned back from the LORD; and those that have not sought the LORD, nor enquired for him.',
  '"There\'s not a God to look on, nor a man."'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And David distributed them, both Zadok of the sons of Eleazar, and Ahimelech of the sons of Ithamar, according to their offices in their service.',
  "And David distributed them wi' Zadok and Ahimelech;"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'and when thou art athirst, go unto the vessels, and drink of that which the young men have drawn.',
  'Go to vessels and drink athirst the young men;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'But the tithes of the children of Israel, which they offer as an heave offering unto the LORD, I have given to the Levites to inherit: therefore I have said unto them, Among the children of Israel they shall have no inheritance.',
  "I've given Leviticus a tithe they offer to inherit."],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'I will seek that which was lost, and bring again that which was driven away, and will bind up that which was broken, and will strengthen that which was sick: but I will destroy the fat and the strong; I will feed them with judgment.',
  'To seek lost, bring broken up, and strengthen sick: Fate doth destroy and feed'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Who serve unto the example and shadow of heavenly things, as Moses was admonished of God when he was about to make the tabernacle: for, See, saith he, that thou make all things according to the pattern shewed to thee in the mount.',
  'Who serve as example and shadow, admonished God about to make tabernacle.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'He that is our God is the God of salvation; and unto GOD the Lord belong the issues from death.',
  'Issues belong to that God who saves'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And it shall come to pass in that day, that I will seek to destroy all the nations that come against Jerusalem.',
  'To destroy all nations that opposed Jerusalem,'],
 ['bible_poetry.tsv',
  'No Error',
  'No Error',
  'And he brought in the priests and the Levites, and gathered them together into the east street,',
  'He gathered priests and levitees in east lane.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Against him came up Nebuchadnezzar king of Babylon, and bound him in fetters, to carry him to Babylon.',
  'And King Nebuchadnezzar bound him in fetters to bear.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Thou shalt not consent unto him, nor hearken unto him; neither shall thine eye pity him, neither shalt thou spare, neither shalt thou conceal him:',
  'Would he consent not, heard not, pity nor hide your eye;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And, behold, thy cousin Elisabeth, she hath also conceived a son in her old age: and this is the sixth month with her, who was called barren.',
  'And old age, thy cousin Elisabeth also bowed'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'After that he is sold he may be redeemed again; one of his brethren may redeem him:',
  'After he was sold, perhaps again his brothers would redeem.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Love the brotherhood.',
  'The brotherhood to love! and to love,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Moses said, Thus saith the LORD, About midnight will I go out into the midst of Egypt:',
  "About midnight I'll go to Egypt,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'By them shall the fowls of the heaven have their habitation, which sing among the branches.',
  'And birds sing among the branches,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'The lip of truth shall be established for ever: but a lying tongue is but for a moment.',
  "Truth established for ever--but a moment's lying tongue,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "But the mercy of the LORD is from everlasting to everlasting upon them that fear him, and his righteousness unto children's children;",
  "But God's mercy for ever, and His righteousness for children,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'and who knoweth us?',
  'And who knows us? and who knows us well?'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And this have ye done again, covering the altar of the LORD with tears, with weeping, and with crying out, insomuch that he regardeth not the offering any more, or receiveth it with good will at your hand.',
  "Do this again, covering the altar with tears, or regard'd no offer anymore, or accepted."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And there fell of Benjamin eighteen thousand men; all these were men of valour.',
  'Benjamin was a man of 18000,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Wherefore the sin of the young men was very great before the LORD: for men abhorred the offering of the LORD.',
  'So, very great is the sin of young men,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Whoso findeth a wife findeth a good thing, and obtaineth favour of the LORD.',
  'Who finds a wife and gets a favour--'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'He that is void of wisdom despiseth his neighbour: but a man of understanding holdeth his peace.',
  'Wisdomless he despises his neighbour, but understanding man holds'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And the heavens shall declare his righteousness: for God is judge himself.',
  'And mony a God shall judge him,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'Let me be weighed in an even balance that God may know mine integrity.',
  'Let me even weighed in the balance to know my integrity--'],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'but turn thee yet again, and thou shalt see greater abominations.',
  'But, if yet thou turnest again, see greater abominables.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'For Christ is the end of the law for righteousness to every one that believeth.',
  "Christ's end to all who believe in law!"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And Baasha king of Israel went up against Judah, and built Ramah, that he might not suffer any to go out or come in to Asa king of Judah.',
  'Ramas, the king of Israel, built, nor could suffer'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'let her be shut out from the camp seven days, and after that let her be received in again.',
  'Let her shut out of camp seven days and let again'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Honour thy father and thy mother: that thy days may be long upon the land which the LORD thy God giveth thee.',
  'Honour your father and mother, so thy days may long'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'Thou, O king, art a king of kings: for the God of heaven hath given thee a kingdom, power, and strength, and glory.',
  'God gave thee kingdom, power, and glory;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Wherefore lay apart all filthiness and superfluity of naughtiness, and receive with meekness the engrafted word, which is able to save your souls.',
  'So lay all needless filth and naughtiness apart, and receive meek words'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Pour out thy wrath upon the heathen that have not known thee, and upon the kingdoms that have not called upon thy name.',
  'Pour wrath on thy known and thy kingdoms,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'shall they not both fall into the ditch?',
  'Do they not both fall into a ditch?'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'He disappointeth the devices of the crafty, so that their hands cannot perform their enterprise.',
  'He disappoints the crafty,--he cannot perform his duties.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "And the city was broken up, and all the men of war fled by night by the way of the gate between two walls, which is by the king's garden: (now the Chaldees were against the city round about:) and the king went the way toward the plain.",
  'The city broke up and all combatant fled the gate between two walls,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For whosoever will save his life shall lose it: but whosoever will lose his life for my sake, the same shall save it.',
  'Who would save his life would lose his life, but none'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For this cause we also, since the day we heard it, do not cease to pray for you, and to desire that ye might be filled with the knowledge of his will in all wisdom and spiritual understanding;',
  'This means we neer stop to pray you, and wish ye fill with his will--'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'For therefore we both labour and suffer reproach, because we trust in the living God, who is the Saviour of all men, specially of those that believe.',
  'We trust the living God who saves all and those who believe,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'For thou shalt be in league with the stones of the field: and the beasts of the field shall be at peace with thee.',
  "Thou art in league wi' the fields-stones,"],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'Pour out thine indignation upon them, and let thy wrathful anger take hold of them.',
  'Pour your indignation on them, and let thy wrathful anger take hold'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'If a man be found stealing any of his brethren of the children of Israel, and maketh merchandise of him, or selleth him; then that thief shall die; and thou shalt put evil away from among you.',
  'If any brother of thieves were found,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'The sons of Abraham; Isaac, and Ishmael.',
  "Of Abraham, Isaac, an' Hashmael;"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And when the Philistines heard the noise of the shout, they said, What meaneth the noise of this great shout in the camp of the Hebrews?',
  'What means this Filipino when he heard a mighty shout?'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Do not think that I will accuse you to the Father: there is one that accuseth you, even Moses, in whom ye trust.',
  'Think not that I accuse thy Father, even of Mosses!'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And said unto the children of Israel, Thus saith the LORD God of Israel, I brought up Israel out of Egypt, and delivered you out of the hand of the Egyptians, and out of the hand of all kingdoms, and of them that oppressed you:',
  'I brought Israel out of Egypt and all its oppressed kingdoms.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And they sing the song of Moses the servant of God, and the song of the Lamb, saying, Great and marvellous are thy works, Lord God Almighty; just and true are thy ways, thou King of saints.',
  "They sing their King's Almighty Moses, saying they are great and beautiful."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  "In the light of the king's countenance is life; and his favour is as a cloud of the latter rain.",
  "The King's dwelling-place, the latest rain his favour;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the spoiler shall come upon every city, and no city shall escape: the valley also shall perish, and the plain shall be destroyed, as the LORD hath spoken.',
  'From every city the spoiler comes, no city escapes, a valley is dead and a plain'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Preach the word; be instant in season, out of season; reprove, rebuke, exhort with all longsuffering and doctrine.',
  'Preach the word,--no season,--rebuke,--exhort all with long and taught;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  "And they said unto him, Caesar's.",
  'Then there was the Csar, the Csar,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Then many of the Jews which came to Mary, and had seen the things which Jesus did, believed on him.',
  'And many a Jew then came to Mary, saw Jesus do,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Let the floods clap their hands: let the hills be joyful together',
  'Let their hands in floods, let the hills together rejoice:'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'According to the days of thy coming out of the land of Egypt will I shew unto him marvellous things.',
  "I'm tauld ye're coming to Egypt,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Praise the LORD, O Jerusalem; praise thy God, O Zion.',
  "Praise the Lord of Jerusalem! 'tis well done,"],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'And he made ready his chariot, and took his people with him:',
  'He was ready in his chariot, and he took his people'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And she made him sleep upon her knees; and she called for a man, and she caused him to shave off the seven locks of his head; and she began to afflict him, and his strength went from him.',
  'She made him sleep at knees, called the man and shaved seven locks'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And all the evil of the men of Shechem did God render upon their heads: and upon them came the curse of Jotham the son of Jerubbaal.',
  "God cursed Erubbaal's son,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'All the days wherein the plague shall be in him he shall be defiled; he is unclean: he shall dwell alone; without the camp shall his habitation be.',
  "Defiled, unclean, living alone, uncamp'd all day;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And all the kings of the north, far and near, one with another, and all the kingdoms of the world, which are upon the face of the earth: and the king of Sheshach shall drink after them.',
  'After them, all kings Sheshach drank far and near,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'But know this, that if the goodman of the house had known in what watch the thief would come, he would have watched, and would not have suffered his house to be broken up.',
  'But know what thief watches and suffers not from his house broken,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Then went he down, and dipped himself seven times in Jordan, according to the saying of the man of God: and his flesh came again like unto the flesh of a little child, and he was clean.',
  'Then down he went, and in Jordan dipt seven times'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'Blessed be the God and Father of our Lord Jesus Christ, who hath blessed us with all spiritual blessings in heavenly places in Christ:',
  'God and our Father Jesus blessed us in heavenly places.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'and there is none upon earth that I desire beside thee.',
  'And bids me shun nought on earth but thee--'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Say ye not, A confederacy, to all them to whom this people shall say, A confederacy; neither fear ye their fear, nor be afraid.',
  'Say not of Confederacy, say not of them; and fear'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And they shall put my name upon the children of Israel, and I will bless them.',
  "They'll put my name in mine, and bless him a'."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'The ancients of Gebal and the wise men thereof were in thee thy calkers: all the ships of the sea with their mariners were in thee to occupy thy merchandise.',
  'On ships and mariners shalt thou occupy thy merchandise;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Lo, let that night be solitary, let no joyful voice come therein.',
  'That night lone, lo! no voice will come there,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And thou shalt take fine flour, and bake twelve cakes thereof: two tenth deals shall be in one cake.',
  'To take fine flour and bake twelve. If two deals were made,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And there was a cloud that overshadowed them: and a voice came out of the cloud, saying, This is my beloved Son: hear him.',
  'The cloud overshadowed them, and came out their Son, who loved'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'For it might have been sold for more than three hundred pence, and have been given to the poor.',
  'It may be sold for more than three hundred pounds.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Cleanse your hands, ye sinners; and purify your hearts, ye double minded.',
  'Clean thine hands, and purify thine hearts,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And she came to Jerusalem with a very great train, with camels that bare spices, and very much gold, and precious stones: and when she was come to Solomon, she communed with him of all that was in her heart.',
  'Came Jerusalem with very big train, and camels bare of spices, and very gold.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And now, O God of Israel, let thy word, I pray thee, be verified, which thou spakest unto thy servant David my father.',
  "I pray the Father's word is verified,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the priest said unto them, Go in peace: before the LORD is your way wherein ye go.',
  'Before the Lord go in peace on high;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And they marvelled all.',
  "And they were all amaz'd. But a little while"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'care not for it: but if thou mayest be made free, use it rather.',
  'I care not for it--but if rather be free, use'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'For I have not shunned to declare unto you all the counsel of God.',
  "I would not shun all God's counsel,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Now Tobiah the Ammonite was by him, and he said, Even that which they build, if a fox go up, he shall even break down their stone wall.',
  'Says Tobiah the Ammonite--even if up the fox break their stone wall,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And they brought it.',
  'And there they brought it.--Ah, well a day,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And he spake unto the children of Israel, saying, When your children shall ask their fathers in time to come, saying, What mean these stones?',
  'In time thy children ask their fathers, saying: "What mean these stones?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the LORD said, Judah shall go up first.',
  'For Judah was the first to go,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Gedor, and Ahio, and Zacher.',
  "The gedor, ahio, and zach'r, all in one,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And ye have respect to him that weareth the gay clothing, and say unto him, Sit thou here in a good place; and say to the poor, Stand thou there, or sit here under my footstool:',
  'Poor sits here, or under my footstool, thy respect,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'There was a certain creditor which had two debtors: the one owed five hundred pence, and the other fifty.',
  'Of debtors two--one--and one--for fifty pounds'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For they that are such serve not our Lord Jesus Christ, but their own belly; and by good words and fair speeches deceive the hearts of the simple.',
  'They serve not our Lord Jesus Christ, and good words and speech deceive our simple hearts.'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'Dedan, and Tema, and Buz, and all that are in the utmost corners,',
  'In utmost corners, where Dedan, Tema, Buz, and all'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Because that which may be known of God is manifest in them; for God hath shewed it unto them.',
  'Because God hath shown them that'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'And he made staves of shittim wood, and overlaid them with gold.',
  'He made a shittim wood stave, and overlayed it gold.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And that ye will save alive my father, and my mother, and my brethren, and my sisters, and all that they have, and deliver our lives from death.',
  'Save father, mother, and all we have, and our lives,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "And he departed thence, and entered into a certain man's house, named Justus, one that worshipped God, whose house joined hard to the synagogue.",
  "He left, and entered Justus' house, which worshipped hard,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'If ye will not hear, and if ye will not lay it to heart, to give glory unto my name, saith the LORD of hosts, I will even send a curse upon you, and I will curse your blessings: yea, I have cursed them already, because ye do not lay it to heart.',
  'Send even my curse--and if thou shouldst not give my name glory,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And thou shalt offer thy burnt offerings, the flesh and the blood, upon the altar of the LORD thy God: and the blood of thy sacrifices shall be poured out upon the altar of the LORD thy God, and thou shalt eat the flesh.',
  'On the altar offer burnt sacrifices, flesh and eat,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Then Joseph said unto the people, Behold, I have bought you this day and your land for Pharaoh: lo, here is seed for you, and ye shall sow the land.',
  "Joseph, I've bought this day and you'll land, Pharaoh!"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'Behold, I waited for your words; I gave ear to your reasons, whilst ye searched out what to say.',
  "I waited for words from thee, listening reasons as thou search'st."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Again, David gathered together all the chosen men of Israel, thirty thousand.',
  'Again David gathered thirty thousand chosen,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Zelek the Ammonite, Naharai the Berothite, the armourbearer of Joab the son of Zeruiah,',
  'The ammonite Zelk, the berothite Naharai,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Thou art fairer than the children of men: grace is poured into thy lips: therefore God hath blessed thee for ever.',
  "Than men's children. Grace pours from thy lips,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And it shall come to pass in the day that the LORD shall give thee rest from thy sorrow, and from thy fear, and from the hard bondage wherein thou wast made to serve,',
  'Lord, give rest from thy sorrow, fear, hard bond, where thou made,'],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'So they weighed for my price thirty pieces of silver.',
  'They weighed thirty pieces of silver my price,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'For perhaps he therefore departed for a season, that thou shouldest receive him for ever;',
  'May he for a season leave, thou wert for ever to see;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And ye shall be holy men unto me: neither shall ye eat any flesh that is torn of beasts in the field; ye shall cast it to the dogs.',
  'Thou holy Man! thou shall not eat the field-meat torn'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'Hath he smitten him, as he smote those that smote him?',
  "He's smitten by the wight that smote?"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'And when he had thus spoken, he took bread, and gave thanks to God in presence of them all: and when he had broken it, he began to eat.',
  "When he'd broken his bread he took and thanks the Lord."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And king Solomon offered a sacrifice of twenty and two thousand oxen, and an hundred and twenty thousand sheep: so the king and all the people dedicated the house of God.',
  'The King Solomon offered his thousand oxen and sheep,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the LORD sent Jerubbaal, and Bedan, and Jephthah, and Samuel, and delivered you out of the hand of your enemies on every side, and ye dwelled safe.',
  'Lord sent him Jerebaal, Bedan, Jephthah, Samuel, and stay safe.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And they made two ouches of gold, and two gold rings; and put the two rings in the two ends of the breastplate.',
  'They made two gold urns, and put two breast-plates--'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the men of Judah said, Why are ye come up against us?',
  "Why have you come up wi' us?"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Gilead is mine, and Manasseh is mine; Ephraim also is the strength of mine head; Judah is my lawgiver;',
  'My Gilead, my Manasseh, and Ephraim also strong;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'Go not to glean in another field, neither go from hence, but abide here fast by my maidens:',
  'Go not to another field, but go fast here;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And Zechariah, and Aziel, and Shemiramoth, and Jehiel, and Unni, and Eliab, and Maaseiah, and Benaiah, with psalteries on Alamoth;',
  'Zechariah, Aziel, Shemiramoth, Benaiah, and psalteries Alamoth.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Who, when he was reviled, reviled not again; when he suffered, he threatened not; but committed himself to him that judgeth righteously:',
  'Threatened not while suffering, but committed'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Let the day perish wherein I was born, and the night in which it was said, There is a man child conceived.',
  'Let my birth-day and night when man has said,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And also Maachah his mother, even her he removed from being queen, because she had made an idol in a grove; and Asa destroyed her idol, and burnt it by the brook Kidron.',
  "Also Makhah, mother removed from the grove, and burnt Asa's idol"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "And he brought up Hadassah, that is, Esther, his uncle's daughter: for she had neither father nor mother, and the maid was fair and beautiful; whom Mordecai, when her father and mother were dead, took for his own daughter.",
  'He brought up Hadassah, father and mother, beautiful maid and lady.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'So Joab the son of Zeruiah went first up, and was chief.',
  'First up went Bob, and as chief was he,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'Who, when he had found one pearl of great price, went and sold all that he had, and bought it.',
  'Who went to sell one pearl at mighty price, when found'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Then Zedekiah the son of Chenaanah came near, and smote Micaiah upon the cheek, and said, Which way went the Spirit of the LORD from me to speak unto thee?',
  'Then came Zedekiah, son of Chenaanah, near, kissed Maicaiah\'s cheek, and said, "Ah, what!'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And ye shall be holy unto me: for I the LORD am holy, and have severed you from other people, that ye should be mine.',
  "I'm holy, and I will sépare you from other wight."],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'From the wicked that oppress me, from my deadly enemies, who compass me about.',
  'From those who oppress me, my deadly foes;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Moses gave the money of them that were redeemed unto Aaron and to his sons, according to the word of the LORD, as the LORD commanded Moses.',
  'Mosses gave money to aaron and his sons,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'From that time forth came they no more on the sabbath.',
  'The sabbath they were no more; and now'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Then Michaiah declared unto them all the words that he had heard, when Baruch read the book in the ears of the people.',
  'Then Michaiah declared all the words he heard as Baruch read the book,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  "And, behold, all the men of Israel came to the king, and said unto the king, Why have our brethren the men of Judah stolen thee away, and have brought the king, and his household, and all David's men with him, over Jordan?",
  'Why did the Jordanian steal our brothers and household?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And he that offered his offering the first day was Nahshon the son of Amminadab, of the tribe of Judah:',
  "The first day Amminadab's son Nahshon offered"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the four and twenty elders, which sat before God on their seats, fell upon their faces, and worshipped God,',
  'Four elders fell upon their faces, and worshipped'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And in that day there shall be a root of Jesse, which shall stand for an ensign of the people; to it shall the Gentiles seek: and his rest shall be glorious.',
  "And Jesse's root was that day's chief--"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And Jesus said, For judgment I am come into this world, that they which see not might see; and that they which see might be made blind.',
  '"Jesus!" said I, "I\'m come to judge those who see not'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'And they caught him, and beat him, and sent him away empty.',
  'They caught him, beat him, and sent him empty away.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Now the Philistines gathered together their armies to battle, and were gathered together at Shochoh, which belongeth to Judah, and pitched between Shochoh and Azekah, in Ephesdammim.',
  "Philistine troops gathered at Judah's Shochoh, pitching between,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'But I would ye should understand, brethren, that the things which happened unto me have fallen out rather unto the furtherance of the gospel;',
  'But bid me understand my deeds are farther out than gospel.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'When the morning stars sang together, and all the sons of God shouted for joy?',
  'When morning stars sang together?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Wherefore, if God so clothe the grass of the field, which to day is, and to morrow is cast into the oven, shall he not much more clothe you, O ye of little faith?',
  'If God does not clothe you more,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And they gathered their brethren, and sanctified themselves, and came, according to the commandment of the king, by the words of the LORD, to cleanse the house of the LORD.',
  "They gathered their brothers, sanctified, and came in accordance with the King's command."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And the children of Heth answered Abraham, saying unto him,',
  '"Abraham!" answer\'d he, "your children,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But Noah found grace in the eyes of the LORD.',
  'But ay the grace was found by Noah,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'He that gathereth in summer is a wise son: but he that sleepeth in harvest is a son that causeth shame.',
  "The summer gather'r wise, but a harvester sleeps his son."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And they made bells of pure gold, and put the bells between the pomegranates upon the hem of the robe, round about between the pomegranates;',
  'They made their pure gold bells, and put them round the pomegranates.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the princes of the Philistines were wroth with him; and the princes of the Philistines said unto him, Make this fellow return, that he may go again to his place which thou hast appointed him, and let him not go down with us to battle, lest in the battle he be an adversary to us: for wherewith should he reconcile himself unto his master?',
  'Where should he with his master reconcile,'],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'But as for the mighty man, he had the earth; and the honourable man dwelt in it.',
  "But mighty man had earth, and honour'd man lived there;"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Hold thou me up, and I shall be safe: and I will have respect unto thy statutes continually.',
  'Hold me up, safe, and my law continued respect.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'From Aroer, which is by the brink of the river of Arnon, and from the city that is by the river, even unto Gilead, there was not one city too strong for us: the LORD our God delivered all unto us:',
  'Not all cities are strong from Aroer, on the brink of a river;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'Of the tribe of Nephthalim were sealed twelve thousand.',
  'And nephthalim was sealed twelve years ago.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'I will also stretch out mine hand upon Judah, and upon all the inhabitants of Jerusalem; and I will cut off the remnant of Baal from this place, and the name of the Chemarims with the priests;',
  "Stretching my hand on Judah's remnant, and all Jerusalem's;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Remember thy servants, Abraham, Isaac, and Jacob; look not unto the stubbornness of this people, nor to their wickedness, nor to their sin:',
  'Remember thy servants--Abraham, Isaac, Jacob.'],
 ['bible_poetry.tsv',
  'No Error',
  'No Error',
  "Now, lo, if he beget a son, that seeth all his father's sins which he hath done, and considereth, and doeth not such like,",
  "If he gets a son who saw all his father's sins, consider him not."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Envyings, murders, drunkenness, revellings, and such like: of the which I tell you before, as I have also told you in time past, that they which do such things shall not inherit the kingdom of God.',
  'I tell you, before, that they not inherit the kingdom of God.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'He that abideth in the doctrine of Christ, he hath both the Father and the Son.',
  'The Father and the Son of Christ,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Better it is to be of an humble spirit with the lowly, than to divide the spoil with the proud.',
  'Better than to divide the spoil from the proud;'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'Debate thy cause with thy neighbour himself; and discover not a secret to another:',
  'Debate cause with thy neighbour; and discover not secret.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the children of Israel said unto them, Would to God we had died by the hand of the LORD in the land of Egypt, when we sat by the flesh pots, and when we did eat bread to the full; for ye have brought us forth into this wilderness, to kill this whole assembly with hunger.',
  'As Egypt we sat in flesh pots and ate full bread.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And when Paul was now about to open his mouth, Gallio said unto the Jews, If it were a matter of wrong or wicked lewdness, O ye Jews, reason would that I should bear with you:',
  '"If you have reason to bear, it\'s about wrong or evil,"'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And the chief captain answered, With a great sum obtained I this freedom.',
  'And the chief captain answer\'d, "This is a lot\'s free,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Joshua sent men from Jericho to Ai, which is beside Bethaven, on the east of Bethel, and spake unto them, saying, Go up and view the country.',
  'And Joshua sent from Jericho to Ai, east of Bethaven.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Therefore I say unto you, What things soever ye desire, when ye pray, believe that ye receive them, and ye shall have them.',
  "Therefore, if thou believe'st receive, I say ye desires,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And they departed, and dwelt in the habitation of Chimham, which is by Bethlehem, to go to enter into Egypt,',
  "They've left Chimham, bethlehem, to Egypt,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'Then said Jesus unto him, Except ye see signs and wonders, ye will not believe.',
  'If thou dost not believe, nor see signs and wonders,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  "Now these are the chief of the province that dwelt in Jerusalem: but in the cities of Judah dwelt every one in his possession in their cities, to wit, Israel, the priests, and the Levites, and the Nethinims, and the children of Solomon's servants.",
  'All Israelis, priests, Dutch, and Jews dwell in Jerusalem;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And he caused all that were present in Jerusalem and Benjamin to stand to it.',
  'So all in Jerusalem and Benjamin stood,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he said to them all, If any man will come after me, let him deny himself, and take up his cross daily, and follow me.',
  'Deny it, and take thy daily cross if any will follow me.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Because for thy sake I have borne reproach; shame hath covered my face.',
  'Because shame covert my face so fair,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'For this city hath been to me as a provocation of mine anger and of my fury from the day that they built it even unto this day; that I should remove it from before my face,',
  "This city's anger and anger caused, the day they built, to remove"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And Joseph said unto Pharaoh, The dream of Pharaoh is one: God hath shewed Pharaoh what he is about to do.',
  'The Pharaoh dreamed that God would show him what he about to do.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Jesus said, Take ye away the stone.',
  "And take the stone o'er the groat."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'But I will punish you according to the fruit of your doings, saith the LORD: and I will kindle a fire in the forest thereof, and it shall devour all things round about it.',
  "But I'll punish you, according your fruit"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Jehoiakim gave the silver and the gold to Pharaoh; but he taxed the land to give the money according to the commandment of Pharaoh: he exacted the silver and the gold of the people of the land, of every one according to his taxation, to give it unto Pharaohnechoh.',
  'Jehoiakim gave palatine silver and gold, but taxed land to give'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'But ye are come unto mount Sion, and unto the city of the living God, the heavenly Jerusalem, and to an innumerable company of angels,',
  "But come from Mount Sinai and heaven's Jerusalem,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And all the gold of the offering that they offered up to the LORD, of the captains of thousands, and of the captains of hundreds, was sixteen thousand seven hundred and fifty shekels.',
  'All the gold they offered to thousand and hundreds, for 1600 shekels.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Fear thou not; for I am with thee: be not dismayed; for I am thy God: I will strengthen thee; yea, I will help thee; yea, I will uphold thee with the right hand of my righteousness.',
  'Fear not, fear not, for my GOD! I am'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Even so it is not the will of your Father which is in heaven, that one of these little ones should perish.',
  "Yet this little one thy Father's not willing to die."],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'And the sons of Hebron; Korah, and Tappuah, and Rekem, and Shema.',
  'Hebron--Korah--Tapuah--Rekem--Shema--'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'and where wroughtest thou?',
  'And wherefore will your feast be?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'So all the elders of Israel came to the king to Hebron; and king David made a league with them in Hebron before the LORD: and they anointed David king over Israel.',
  'All Israeli elders came to Hebron; David appoints'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'God layeth up his iniquity for his children: he rewardeth him, and he shall know it.',
  'God lay iniquity to his children, and rewards'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Many will intreat the favour of the prince: and every man is a friend to him that giveth gifts.',
  'For favour many a year, and every friend who gives gifts,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'In the lips of him that hath understanding wisdom is found: but a rod is for the back of him that is void of understanding.',
  'His lips with wisdom found, but the rod void,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And that they may recover themselves out of the snare of the devil, who are taken captive by him at his will.',
  "Could recover them from the devil's willing trap,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Labour not to be rich: cease from thine own wisdom.',
  "The labour-president's not so rich;"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'Against whom do ye sport yourselves?',
  'What sport thou art? What sport, thou art?'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'The leprosy therefore of Naaman shall cleave unto thee, and unto thy seed for ever.',
  "So Naaman's leprosy would forever cleave thy name and seed."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Behold, the nations are as a drop of a bucket, and are counted as the small dust of the balance: behold, he taketh up the isles as a very little thing.',
  'See nations like a bucket-drop, and counted the small dust in the balance.'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'Nevertheless I am continually with thee: thou hast holden me by my right hand.',
  'Yet continually thou held me in thy right hand;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the altar of burnt offering with all his furniture, and the laver and his foot,',
  'The altar of burnt offerings, and all his foot-rest'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Great is our Lord, and of great power: his understanding is infinite.',
  'The God is great, and the Soul is great to understand.'],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'They send forth their little ones like a flock, and their children dance.',
  'They send their little ones out like a flock, and their children dance'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Jesus therefore, knowing all things that should come upon him, went forth, and said unto them, Whom seek ye?',
  'So Jesus went forth and said, "Whoe\'er shall seek thee,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Be it known unto the king, that the Jews which came up from thee to us are come unto Jerusalem, building the rebellious and the bad city, and have set up the walls thereof, and joined the foundations.',
  'Kept the Jewess who came to Jerusalem, bad rebellious building, foundations joined,'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'And when the people were come into the camp, the elders of Israel said, Wherefore hath the LORD smitten us to day before the Philistines?',
  'Elders of Israel said, God hit us a day before the Philistines.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And they sent a messenger unto Joseph, saying, Thy father did command before he died, saying,',
  'Saying, "Joseph\'s father command, before he died."'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And the young man that told him said, As I happened by chance upon mount Gilboa, behold, Saul leaned upon his spear; and, lo, the chariots and horsemen followed hard after him.',
  "Saul lean'd his spear upon Gilboa's mountain; car and horse hard followed;"],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'Saying, Surely blessing I will bless thee, and multiplying I will multiply thee.',
  "I'm sure I'll bless and multiply thee;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Thou hast covered with anger, and persecuted us: thou hast slain, thou hast not pitied.',
  "Cover'd thy anger, and persecuted us,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Jesus entered and passed through Jericho.',
  'Jesus entered Jerusalem, and passed through'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  "Then thou shalt say, They be thy servant Jacob's; it is a present sent unto my lord Esau: and, behold, also he is behind us.",
  'Say, Jacob, thy servant sends present, thy lord;'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'That it may be well with thee, and thou mayest live long on the earth.',
  "That thou may'st long live on earth,"],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'And if a woman shall put away her husband, and be married to another, she committeth adultery.',
  "A woman commit'd adultery, and left her husband and married."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'When thou shalt hearken to the voice of the LORD thy God, to keep all his commandments which I command thee this day, to do that which is right in the eyes of the LORD thy God.',
  "When God's voice I heard, would do all thou command this day."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For thus hath the LORD said unto me, Go, set a watchman, let him declare what he seeth.',
  'So Lord, go, set watchman, let declare what ye see,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And they said unto him, Yesterday at the seventh hour the fever left him.',
  "A fever left him frae e'en to morn,"],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'So when this was done, others also, which had diseases in the island, came, and were healed:',
  'And others who had diseases of the island came also and healed;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But it came to pass within a while after, in the time of wheat harvest, that Samson visited his wife with a kid; and he said, I will go in to my wife into the chamber.',
  'But Samson visited the wife with the kid, up to the day'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'I am Alpha and Omega, the beginning and the ending, saith the Lord, which is, and which was, and which is to come, the Almighty.',
  'I am of the beginning and end, Alpha and Omega--'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And the children of Israel returned from chasing after the Philistines, and they spoiled their tents.',
  'They returned to chase the Philistines, and their tents were ruined.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Behold, I will send for many fishers, saith the LORD, and they shall fish them; and after will I send for many hunters, and they shall hunt them from every mountain, and from every hill, and out of the holes of the rocks.',
  'I send the fisher there, and hunt from every mountain and hill;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'And they understood none of these things: and this saying was hid from them, neither knew they the things which were spoken.',
  'They understood not these sayings, and they hid'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Blessed is the man whose strength is in thee; in whose heart are the ways of them.',
  "Bless the man that's strong in thy heart,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Thou wilt perform the truth to Jacob, and the mercy to Abraham, which thou hast sworn unto our fathers from the days of old.',
  "To perform Jacob's truancy and Abraham's mercy from ages;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'These are also proverbs of Solomon, which the men of Hezekiah king of Judah copied out.',
  "And also did Solomon's proverbs copy Judah's king."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "And the children of Lotan were Hori and Hemam; and Lotan's sister was Timna.",
  '"Hori and Hemam were Lothian children and sister;'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'But these are they of which ye shall not eat: the eagle, and the ossifrage, and the ospray,',
  'But eat not the eagle, ossifrage, and spray,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "All these were under the hands of their father for song in the house of the LORD, with cymbals, psalteries, and harps, for the service of the house of God, according to the king's order to Asaph, Jeduthun, and Heman.",
  "All in father's hands--cymbals, psalterys, and harps--for song the king orders;"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And they said, Seven, and a few little fishes.',
  'And seven little fishes, that strew'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And it came to pass, as they were much perplexed thereabout, behold, two men stood by them in shining garments:',
  'Twa shining mense stood by them much in confusion,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'At that day shall a man look to his Maker, and his eyes shall have respect to the Holy One of Israel.',
  "Man's eyes that day at Maker's respect, one holy Israeli"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And he shall cut it into his pieces, with his head and his fat: and the priest shall lay them in order on the wood that is on the fire which is upon the altar:',
  'And the priest cut head and fat to his pieces and lay on the altar wood.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'And afterward I will bring again the captivity of the children of Ammon, saith the LORD.',
  'Then back to captivity, O I shall say,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Saying, God hath forsaken him: persecute and take him; for there is none to deliver him.',
  'Saying, God will abandon him, persecute and take'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And the waters prevailed exceedingly upon the earth; and all the high hills, that were under the whole heaven, were covered.',
  'The waters ruled extrême, and all the hills were covered high;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Therefore the Jews sought the more to kill him, because he not only had broken the sabbath, but said also that God was his Father, making himself equal with God.',
  'Since he had broken the sabbath, and said his Father also wanted to kill.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Then the congregation shall judge between the slayer and the revenger of blood according to these judgments:',
  'Congregation will judge between the slain and revenge, according'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And thou shalt put it under the compass of the altar beneath, that the net may be even to the midst of the altar.',
  'And thou hast put a net beneath the altar.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And ye shall give her unto Eleazar the priest, that he may bring her forth without the camp, and one shall slay her before his face:',
  'Would give her to Eleazar to bring without, and one to slay before her face.'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'And when he had declared all these things unto them, he sent them to Joppa.',
  'And when all was declared he sent them to Joppa,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And they tied unto it a lace of blue, to fasten it on high upon the mitre; as the LORD commanded Moses.',
  'And tangled the mitre in blue lace to fasten as Mose ordered.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the other issued out of the city against them; so they were in the midst of Israel, some on this side, and some on that side: and they smote them, so that they let none of them remain or escape.',
  "They're in Israel, some on this side are slain, so let none remain or escape."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And of the sons of Elam; Mattaniah, Zechariah, and Jehiel, and Abdi, and Jeremoth, and Eliah.',
  'Of Mattaniah, Zachariah, Abdi, and Jeremoth.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For the head of Syria is Damascus, and the head of Damascus is Rezin; and within threescore and five years shall Ephraim be broken, that it be not a people.',
  'Damascus, the Capital, and Rezin, after three years,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For his sons had seen what way the man of God went, which came from Judah.',
  'His sons had seen how God went,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'this is nothing else but sorrow of heart.',
  'And this is but the saddest of all.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And thy estimation shall be of the male from twenty years old even unto sixty years old, even thy estimation shall be fifty shekels of silver, after the shekel of the sanctuary.',
  "Even fifty shekels o'er one male aged twenty-six."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'For when ye offer your gifts, when ye make your sons to pass through the fire, ye pollute yourselves with all your idols, even unto this day: and shall I be enquired of by you, O house of Israel?',
  'When offering gifts, and making sons pass through the fire, pollute all'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Wilt not thou, O God, which hadst cast us off?',
  'And did ae God cast us off?--Ah, well-a-day,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  "So I gave them up unto their own hearts' lust: and they walked in their own counsels.",
  "I yielded to their heart-lust, they walk'd in counsel,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Therefore the LORD was very angry with Israel, and removed them out of his sight: there was none left but the tribe of Judah only.',
  "Thus God's very wrath on Israel removed from his sight,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And take your father and your households, and come unto me: and I will give you the good of the land of Egypt, and ye shall eat the fat of the land.',
  "Take your father and your households, come I'll give you Elysian fat;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Put on therefore, as the elect of God, holy and beloved, bowels of mercies, kindness, humbleness of mind, meekness, longsuffering;',
  'God holy and beloved, generous, kind, humble, mind--meek, long;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'The Jews then murmured at him, because he said, I am the bread which came down from heaven.',
  'Then the jewish laughed at him, because he had said he was bread,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For my people have committed two evils; they have forsaken me the fountain of living waters, and hewed them out cisterns, broken cisterns, that can hold no water.',
  "Two evils, o'er abandoned living waters, erect broken cisterns that can not hold"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'The poor and the deceitful man meet together: the LORD lighteneth both their eyes.',
  'The poor meet the deceiving man together,'],
 ['bible_poetry.tsv',
  'No Error',
  'No Error',
  'There brake he the arrows of the bow, the shield, and the sword, and the battle.',
  'The bow, shield, and sword brake the battle,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the burnt offering that the prince shall offer unto the LORD in the sabbath day shall be six lambs without blemish, and a ram without blemish.',
  'Six blemished lambs, and burnt rams, on sabbath day,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'For the transgression of Jacob is all this, and for the sins of the house of Israel.',
  "And Jacob's sins were all his own."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  "And Jahath was the chief, and Zizah the second: but Jeush and Beriah had not many sons; therefore they were in one reckoning, according to their father's house.",
  'While Jahath and Zizah had many sons,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Harbonah, one of the chamberlains, said before the king, Behold also, the gallows fifty cubits high, which Haman had made for Mordecai, who spoken good for the king, standeth in the house of Haman.',
  '"One good-speak\'d Harbonah, king\'s 50-cubit high gallows,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And I will take away his blood out of his mouth, and his abominations from between his teeth: but he that remaineth, even he, shall be for our God, and he shall be as a governor in Judah, and Ekron as a Jebusite.',
  "His blood, and blasted between his teeth: but Israel's governor and Ekron's governor"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And therefore did the Jews persecute Jesus, and sought to slay him, because he had done these things on the sabbath day.',
  'Persecuted Jesus, and wreat this Sabbath day,'],
 ['bible_poetry.tsv',
  'No Error',
  'Incomplete',
  'Seven years old was Jehoash when he began to reign.',
  "A seven-year's Jehoash, when he began to rule,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'If he beget a son that is a robber, a shedder of blood, and that doeth the like to any one of these things,',
  "If he gets the robber's blood-shedding son, and any of these things."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And it came to pass, when he had made an end of speaking unto Saul, that the soul of Jonathan was knit with the soul of David, and Jonathan loved him as his own soul.',
  "Jonathan's soul was knit with Saul's, and loved him like him."],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'Jarmuth, and Adullam, Socoh, and Azekah,',
  'Of Armuth, Abullam, Socoh, and Azekah.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Therefore it is no great thing if his ministers also be transformed as the ministers of righteousness; whose end shall be according to their works.',
  'If his minstrels were also transformed great,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And hath made us kings and priests unto God and his Father; to him be glory and dominion for ever and ever.',
  'He made us kings and priests,--God and Father.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And the dogs shall eat Jezebel in the portion of Jezreel, and there shall be none to bury her.',
  'The dogs will eat and bury the jazebel portion;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'I will arise and go to my father, and will say unto him, Father, I have sinned against heaven, and before thee,',
  "I rise, and go, my father, and say, I have sinn'd heaven"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And David gathered all Israel together to Jerusalem, to bring up the ark of the LORD unto his place, which he had prepared for it.',
  'David gathered all his neighbors in Jerusalem to bring an ark'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'And he said, Which way shall we go up?',
  '"Up! where\'er we go,\'er we\'ll hither,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'But the miry places thereof and the marishes thereof shall not be healed; they shall be given to salt.',
  'But miry places and marishes unhealed'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'For the law of the Spirit of life in Christ Jesus hath made me free from the law of sin and death.',
  "Jesus' life-law I'm free from death's sin-law,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Now these are the words of the letter that Jeremiah the prophet sent from Jerusalem unto the residue of the elders which were carried away captives, and to the priests, and to the prophets, and to all the people whom Nebuchadnezzar had carried away captive from Jerusalem to Babylon;',
  'The prophet\'s letter sent from Jerusalem declares: "All,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'Israel was holiness unto the LORD, and the firstfruits of his increase: all that devour him shall offend; evil shall come upon them, saith the LORD.',
  'Holy is Israel, its first-fruits increase, and all who devour'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Even so, Amen.',
  "An' tho' a' that, amen! a' that,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'let us eat and drink; for to morrow we die.',
  'O let us eat and drink the dews,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'They shall run like mighty men; they shall climb the wall like men of war; and they shall march every one on his ways, and they shall not break their ranks:',
  'Run like mighty men, climb like war-men, march every step, nor break their ranks;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'As a dog returneth to his vomit, so a fool returneth to his folly.',
  'The fool returns vomit like a dog to return;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  "In my Father's house are many mansions: if it were not so, I would have told you.",
  "Mansions many, many as my Father's house. If it is, tell me not."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'These are the families of the Zebulunites according to those that were numbered of them, threescore thousand and five hundred.',
  '"Ae Zebulunites, three thousand as many,"'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Also in time past, when Saul was king over us, thou wast he that leddest out and broughtest in Israel: and the LORD said to thee, Thou shalt feed my people Israel, and thou shalt be a captain over Israel.',
  'And Saul led out and brought forth Israel past'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Therefore the Jews of the villages, that dwelt in the unwalled towns, made the fourteenth day of the month Adar a day of gladness and feasting, and a good day, and of sending portions one to another.',
  'The Jewess made his fourteenth Adar-day, a day of gladness and feast.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'This people draweth nigh unto me with their mouth, and honoureth me with their lips; but their heart is far from me.',
  'This draws me mouth, and honours me far away;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And I give unto them eternal life; and they shall never perish, neither shall any man pluck them out of my hand.',
  'I give them life for ever--they never die--anyone picks them out,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'A man of great wrath shall suffer punishment: for if thou deliver him, yet thou must do it again.',
  'Great wrath shall suffer punishment; though it must do again.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'The Jews answered him, We have a law, and by our law he ought to die, because he made himself the Son of God.',
  'We have law, and should he die, because he made a Son.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And he said unto them, What manner of communications are these that ye have one to another, as ye walk, and are sad?',
  'How would ye communicate with another, as ye walk and mourn.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'Moreover Jeremiah said unto king Zedekiah, What have I offended against thee, or against thy servants, or against this people, that ye have put me in prison?',
  "An' Jeremiah, wha offended thy servant or this king?"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Howbeit he refused to turn aside: wherefore Abner with the hinder end of the spear smote him under the fifth rib, that the spear came out behind him; and he fell down there, and died in the same place: and it came to pass, that as many as came to the place where Asahel fell down and died stood still.',
  "Refused to turn aside, with spear-end hinder'd, Asahel fell,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Righteous art thou, O LORD, and upright are thy judgments.',
  'Thou art right and upright, and upright;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Should it be according to thy mind?',
  "Should it be, to thy mind's conformity,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And the LORD said unto him, Go up.',
  'Go up, up! and see how far the wind is blowing.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'An altar of earth thou shalt make unto me, and shalt sacrifice thereon thy burnt offerings, and thy peace offerings, thy sheep, and thine oxen: in all places where I record my name I will come unto thee, and I will bless thee.',
  'Make earthly altars, sacrifice all thy burnt offerings, sheep and oxen,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'Then David gave to Solomon his son the pattern of the porch, and of the houses thereof, and of the treasuries thereof, and of the upper chambers thereof, and of the inner parlours thereof, and of the place of the mercy seat,',
  'Then David gave his son Solomon a pattern of porches, houses, upper and inner chambers,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'This is the inheritance of the tribe of the children of Dan according to their families, these cities with their villages.',
  "These cities Dan's fam'd inherits,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And the people answered him not a word.',
  'And no one answered him by the word,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And five of you shall chase an hundred, and an hundred of you shall put ten thousand to flight: and your enemies shall fall before you by the sword.',
  'Five of you will chase hundred, and put ten thousand foes in flight.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'For it is written, He taketh the wise in their own craftiness.',
  "He takes the wise o' their craft,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'The LORD hath made all things for himself: yea, even the wicked for the day of evil.',
  'For the Lord made all things for him.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'A man that is an heretick after the first and second admonition reject;',
  "The heretick o' guy, who first rejected admonition,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'I Paul have written it with mine own hand, I will repay it: albeit I do not say to thee how thou owest unto me even thine own self besides.',
  "I'll repay it to Paul, though thou dost not say"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'for had there not been now a much greater slaughter among the Philistines?',
  'Was not the Philistines slain much now,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And cried when they saw the smoke of her burning, saying, What city is like unto this great city!',
  'They cried, and said, "A city like?" when she saw'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'A good man sheweth favour, and lendeth: he will guide his affairs with discretion.',
  'The good man gave favours, lends, and guides his affairs with discretion.'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'for my soul is wearied because of murderers.',
  'As murderers cause my weary soul'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'In the day when the keepers of the house shall tremble, and the strong men shall bow themselves, and the grinders cease because they are few, and those that look out of the windows be darkened,',
  'When keepers tremble, grinders bow, less ceased, those looking out the windows darken,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'and having ears, hear ye not?',
  'And have ye been sae sae having ears?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the great court round about was with three rows of hewed stones, and a row of cedar beams, both for the inner court of the house of the LORD, and for the porch of the house.',
  'A great court, round three honed stones and one row of cedar beams.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Anathoth with her suburbs, and Almon with her suburbs; four cities.',
  'Atthoth and Almon were four,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And called, and asked whether Simon, which was surnamed Peter, were lodged there.',
  "And called, and asked if Peter's Simon was there,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the Sabeans fell upon them, and took them away; yea, they have slain the servants with the edge of the sword; and I only am escaped alone to tell thee.',
  'The Sabberian slain his servants with sword, and only escape to tell.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'Therefore rejoice, ye heavens, and ye that dwell in them.',
  'So may rejoice thy Heavens, and live'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Moreover the LORD will also deliver Israel with thee into the hand of the Philistines: and to morrow shalt thou and thy sons be with me: the LORD also shall deliver the host of Israel into the hand of the Philistines.',
  "And also the Lord delivered with the Philistines' hand:"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  'I love the LORD, because he hath heard my voice and my supplications.',
  'I love the Lord because he heard my voice and my pretences.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'An unjust man is an abomination to the just: and he that is upright in the way is abomination to the wicked.',
  'For unjust men are abominable;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And every earthen vessel, whereinto any of them falleth, whatsoever is in it shall be unclean; and ye shall break it.',
  'And every vessel on earth was clean, and thou didst break'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Solomon brought in the things which David his father had dedicated; even the silver, and the gold, and the vessels, did he put among the treasures of the house of the LORD.',
  'Solomon brought such as silver, gold, and vessels dedicated to David.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Be ye ashamed, O ye husbandmen; howl, O ye vinedressers, for the wheat and for the barley; because the harvest of the field is perished.',
  'Shame on thee, howl for the crops to die;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'The eye also of the adulterer waiteth for the twilight, saying, No eye shall see me: and disguiseth his face.',
  "Also waiting the adult's face with twinkling rays,--"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And they brake down the image of Baal, and brake down the house of Baal, and made it a draught house unto this day.',
  "The Baal's image they brake down,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'Whosoever committeth sin transgresseth also the law: for sin is the transgression of the law.',
  "By sinners' sins the law is violated,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Saying unto them, Go into the village over against you, and straightway ye shall find an ass tied, and a colt with her: loose them, and bring them unto me.',
  'Go over the village, and straight find the tied ass and colt with her.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'But in the seventh year shall be a sabbath of rest unto the land, a sabbath for the LORD: thou shalt neither sow thy field, nor prune thy vineyard.',
  "The seventh sabbath for land: ye'll neither sow nor prune your vineyard;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Then said I unto them, Ye see the distress that we are in, how Jerusalem lieth waste, and the gates thereof are burned with fire: come, and let us build up the wall of Jerusalem, that we be no more a reproach.',
  'Ye see our distress, and Jerusalem and her gates burn.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Simon and they that were with him followed after him.',
  'And Simon followed, and they were all'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And unleavened bread, and cakes unleavened tempered with oil, and wafers unleavened anointed with oil: of wheaten flour shalt thou make them.',
  'Make leaven bread, nor oil-tempered cakes, nor leaven wafers coated,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'So Jonathan arose from the table in fierce anger, and did eat no meat the second day of the month: for he was grieved for David, because his father had done him shame.',
  'Than Jonathan uprose at the table in fierce anger, no meat the second day of May,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'He that hath received his testimony hath set to his seal that God is true.',
  "And put him a seal o' God's truth,"],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'No Error',
  "That ye shall say, It is the sacrifice of the LORD's passover, who passed over the houses of the children of Israel in Egypt, when he smote the Egyptians, and delivered our houses.",
  'Say, God is the sacrifice when Elysian slain and delivered our houses.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Because of the savour of thy good ointments thy name is as ointment poured forth, therefore do the virgins love thee.',
  'Thy virgin love virgins, by thy good ointments name,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'There went with us also certain of the disciples of Caesarea, and brought with them one Mnason of Cyprus, an old disciple, with whom we should lodge.',
  "They also went to the Csar's, and brought old Cyprus disciple Mnason."],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Surely thou wilt slay the wicked, O God: depart from me therefore, ye bloody men.',
  '"God, surely thou wilt kill evil;"'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'Jesus answered and said unto them, I have done one work, and ye all marvel.',
  'Jesus answered, said he had done one labour, and all were amazed.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Why dost thou strive against him?',
  '"Why try\'st thou against him?"'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Moses did as the LORD commanded: and they went up into mount Hor in the sight of all the congregation.',
  'Mestrels did the Lord command, on Mount Hor,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'This shall be thine of the most holy things, reserved from the fire: every oblation of theirs, every meat offering of theirs, and every sin offering of theirs, and every trespass offering of theirs which they shall render unto me, shall be most holy for thee and for thy sons.',
  'For every obstruction, every meat--and holy are thy sons--'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the sons of Izhar; Korah, and Nepheg, and Zichri.',
  'Izhar, Korah, Nepheg, and Zichri,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And they removed from Jotbathah, and encamped at Ebronah.',
  'They removed from Jotbathah and Ebronah dwelt;'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'But tidings out of the east and out of the north shall trouble him: therefore he shall go forth with great fury to destroy, and utterly to make away many.',
  'But tidings from east and north trouble him, many a destroy,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Pharaoh called unto Moses, and said, Go ye, serve the LORD; only let your flocks and your herds be stayed: let your little ones also go with you.',
  'Poses called him "Serve, but let your flocks and herds'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Now the works of the flesh are manifest, which are these; Adultery, fornication, uncleanness, lasciviousness,',
  'Adultery, fornication, unclean, lascivious,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'Thus Jeremiah remained in the court of the prison.',
  "So in Job's prison Jerry's remained,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Peter answering said, The Christ of God.',
  'The answerer was God Petrarch,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'only let us consent unto them, and they will dwell with us.',
  'Let them only accord, and live with us;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'hath he not sent me to the men that sit upon the wall, that they may eat their own dung, and drink their own piss with you?',
  'He wont tell you if men who sit on the wall can eat their dung and drink their piss,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "For thy name's sake, O LORD, pardon mine iniquity; for it is great.",
  "My infidelities! pardon them a', Sir!"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For the seller shall not return to that which is sold, although they were yet alive: for the vision is touching the whole multitude thereof, which shall not return; neither shall any strengthen himself in the iniquity of his life.',
  'Not to the seller return, though still lives, not touching sight;'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Judah was his sanctuary, and Israel his dominion.',
  "Judah's sanctuary, and Israel's reign;"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And it came to pass, as he drew back his hand, that, behold, his brother came out: and she said, How hast thou broken forth?',
  'When he drew back his brother out, and said: "How did he break?'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'My bowels, my bowels!',
  'My bowels! thou shalt see, that in thy sight'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Therefore every one that eateth it shall bear his iniquity, because he hath profaned the hallowed thing of the LORD: and that soul shall be cut off from among his people.',
  "Since every man who ate it profess'd his hallowed sin,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'But God giveth it a body as it hath pleased him, and to every seed his own body.',
  'But God gives it as body and every seed--'],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  "Kerioth is taken, and the strong holds are surprised, and the mighty men's hearts in Moab at that day shall be as the heart of a woman in her pangs.",
  "Was taken by Kerioth, and astonied strong holds, big men's hearts that day,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Iniquities prevail against me: as for our transgressions, thou shalt purge them away.',
  "Injustice prevail'd on me, ye purge our transgressions;"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Hamath, Berothah, Sibraim, which is between the border of Damascus and the border of Hamath; Hazarhatticon, which is by the coast of Hauran.',
  'From Hamas, Berothah, and Sibraim,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And it came to pass also on another sabbath, that he entered into the synagogue and taught: and there was a man whose right hand was withered.',
  'Also on another sabbath he entered and taught'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And I have given you a land for which ye did not labour, and cities which ye built not, and ye dwell in them; of the vineyards and oliveyards which ye planted not do ye eat.',
  "I've given you land to labour not, cities built not, vineyards and olive-farms,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'The burden of the desert of the sea.',
  'The burden of a desert: and so it was,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'For thou hadst cast me into the deep, in the midst of the seas; and the floods compassed me about: all thy billows and thy waves passed over me.',
  'The floods piled me up; thy billows and waves all passed over'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And the king said, What have I to do with you, ye sons of Zeruiah?',
  '"Zeruiah! what have I to do with you?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'Return, ye backsliding children, and I will heal your backslidings.',
  'Return, ye backsliding children, and heal'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Then came to him the mother of Zebedees children with her sons, worshipping him, and desiring a certain thing of him.',
  'Then Zebedee mother worshiping him, and wan,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And, behold, as Barak pursued Sisera, Jael came out to meet him, and said unto him, Come, and I will shew thee the man whom thou seekest.',
  'When Barak pursued, Jamie came out to meet Sisera and told'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Therefore say, Thus saith the Lord GOD; Although I have cast them far off among the heathen, and although I have scattered them among the countries, yet will I be to them as a little sanctuary in the countries where they shall come.',
  "In little reserv'd countries where I come, yet I have scattered"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he saith unto the man which had the withered hand, Stand forth.',
  'He spake, "Stand, thou withered hand,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'hath thy soul lothed Zion?',
  'ZION! didst thou lott thee with thy hame,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And he made the incense altar of shittim wood: the length of it was a cubit, and the breadth of it a cubit; it was foursquare; and two cubits was the height of it; the horns thereof were of the same.',
  'Made a shittim wood altar incense--long, and two-cubit tall.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'In the twilight, in the evening, in the black and dark night:',
  'And in the black and dark night'],
 ['bible_poetry.tsv',
  'No Error',
  'Meaning Change',
  'And I will also take of them for priests and for Levites, saith the LORD.',
  "I'll also take them o'er priests and Leviticus,"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And beheld among the simple ones, I discerned among the youths, a young man void of understanding,',
  'I saw a young unintelligible man among simple ones.'],
 ['bible_poetry.tsv',
  'No Error',
  'No Error',
  'And ye shall know the truth, and the truth shall make you free.',
  'Know the truth, and make thee free.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'All that ever came before me are thieves and robbers: but the sheep did not hear them.',
  'All who came ever before me not hear from sheep,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'And didst see the affliction of our fathers in Egypt, and heardest their cry by the Red sea;',
  'Our fathers in Egypt afflicted, and hear the red Sea cry,'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'and a strange punishment to the workers of iniquity?',
  'Strange punishment for the labourer?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And saying, Alas, alas that great city, that was clothed in fine linen, and purple, and scarlet, and decked with gold, and precious stones, and pearls!',
  "Alas! that great city clad in fine linen, purple and scarlet, and deck'd"],
 ['bible_poetry.tsv',
  'Incomplete',
  'No Error',
  'And the rough goat is the king of Grecia: and the great horn that is between his eyes is the first king.',
  "The rough goat o'er the king of Greece"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And when ye spread forth your hands, I will hide mine eyes from you: yea, when ye make many prayers, I will not hear: your hands are full of blood.',
  "I'll hide thine eyes, while thy many prayers"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'For thine arrows stick fast in me, and thy hand presseth me sore.',
  'Thy arrows stick fast on me, and bad pressure'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Therefore, behold, the days come, saith the LORD, that it shall no more be called Tophet, nor the valley of the son of Hinnom, but the valley of slaughter: for they shall bury in Tophet, till there be no place.',
  'Not called Tophet, but valley of Hinnom,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  "And Saul took him that day, and would let him go no more home to his father's house.",
  'Saul took him that day, and let his father go no more;'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'and to what are they like?',
  'And what are they like to scud themsels?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And Zelah, Eleph, and Jebusi, which is Jerusalem, Gibeath, and Kirjath; fourteen cities with their villages.',
  'Of fourteen, including Jerusalem, Gibrah and Kirjath.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And, behold, men passed by, and saw the carcase cast in the way, and the lion standing by the carcase: and they came and told it in the city where the old prophet dwelt.',
  "Men passed the carcass, saw the lion standing by, and came old Prophet's city."],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'have ye not heard?',
  "Heard'st thou?--Awake! awake! and awake!"],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And after he had spent some time there, he departed, and went over all the country of Galatia and Phrygia in order, strengthening all the disciples.',
  'And left after some time there, and all Galaxia and Phrygia strengthened.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Until the day break, and the shadows flee away, I will get me to the mountain of myrrh, and to the hill of frankincense.',
  'Till day is broken and shadows flee, mountain myrrh!'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Meaning Change',
  'And in their hands they shall bear thee up, lest at any time thou dash thy foot against a stone.',
  "In thy hands, at any time dash'd to a stone,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And when he cometh home, he calleth together his friends and neighbours, saying unto them, Rejoice with me; for I have found my sheep which was lost.',
  'Calls his friends and neighbours together when they come home to find their lost sheep.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'No Error',
  'Hast thou an arm like God?',
  'Hast thou a Godlike arm as thou?'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Until I come and take you away to a land like your own land, a land of corn and wine, a land of bread and vineyards, a land of oil olive and of honey, that ye may live, and not die: and hearken not unto Hezekiah, when he persuadeth you, saying, The LORD will deliver us.',
  'Until I come and take you to land like ye, wine, bread, vineyard, honey,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Blessed is the man that feareth the LORD, that delighteth greatly in his commandments.',
  'Bless those who fear, who great delight their commands,'],
 ['bible_poetry.tsv',
  'No Error',
  'Incorrect/New Information',
  'And upon all the ships of Tarshish, and upon all pleasant pictures.',
  'Of tartish ships, and all the pleasant pictures'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'When they were filled, he said unto his disciples, Gather up the fragments that remain, that nothing be lost.',
  'When full his disciples said, gather fragments remaining to lose nothing.'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Yet a little sleep, a little slumber, a little folding of the hands to sleep:',
  'Yet little sleep, little slumber, little hands to fold,'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And those that are to be redeemed from a month old shalt thou redeem, according to thine estimation, for the money of five shekels, after the shekel of the sanctuary, which is twenty gerahs.',
  'Your estimate says, those months redeem five shekels,'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'Neither shalt thou steal.',
  'Nae mair thou shalt steal--thou shalt steal--'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'Therefore their goods shall become a booty, and their houses a desolation: they shall also build houses, but not inhabit them; and they shall plant vineyards, but not drink the wine thereof.',
  'And also build houses, but inhabit not vineyards, nor drink'],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Meaning Change',
  'His remembrance shall perish from the earth, and he shall have no name in the street.',
  'His recollection dead, and no name in the street.'],
 ['bible_poetry.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And Moses gave unto the tribe of the children of Reuben inheritance according to their families.',
  "Mosses gave Reuben his heirs, as their fam'lies accord."],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And the sabbath of the land shall be meat for you; for thee, and for thy servant, and for thy maid, and for thy hired servant, and for thy stranger that sojourneth with thee.',
  'Meat for you, your servant, maid, and stranger you hire.'],
 ['bible_poetry.tsv',
  'Incomplete',
  'Incomplete',
  'And all the army of the Chaldees, that were with the captain of the guard, brake down the walls of Jerusalem round about.',
  "Round Jerusalem's walls the army brakes,"],
 ['bible_poetry.tsv',
  'Meaning Change',
  'Incomplete',
  'And Abraham called the name of his son that was born unto him, whom Sarah bare to him, Isaac.',
  "Abraham's name, that Sarah's Isaac bore;"],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'The length of one curtain shall be eight and twenty cubits, and the breadth of one curtain four cubits: and every one of the curtains shall have one measure.',
  'One curtain is eight cubits long, and one is four cubits long.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Now if thou shalt kill all this people as one man, then the nations which have heard the fame of thee will speak, saying,',
  "Now, if thou hast kill'd all these men by one man, The nations that have heard thy fame will speak."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And Israel served the LORD all the days of Joshua, and all the days of the elders that overlived Joshua, and which had known all the works of the LORD, that he had done for Israel.',
  'The king of Israel hath served Judah, and elders overlived, Who knew all their labors.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Chasten thy son while there is hope, and let not thy soul spare for his crying.',
  'Hold, sweet son, when thou shalt be hopeful, And let not thy heart spare our weeping.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the sons of Jada the brother of Shammai; Jether, and Jonathan: and Jether died without children.',
  'Jada and Jonathan died without children.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And ye have respect to him that weareth the gay clothing, and say unto him, Sit thou here in a good place; and say to the poor, Stand thou there, or sit here under my footstool:',
  'Thou dost esteem a man that is gay, and thou dost say he will sit here, or sit under my footstool, for he is a poor man.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'For therefore we both labour and suffer reproach, because we trust in the living God, who is the Saviour of all men, specially of those that believe.',
  "We'll labor and suffer For trusting the living God, Who hath saved all and those that believe in particular."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Also can any understand the spreadings of the clouds, or the noise of his tabernacle?',
  'Can any man understand also the spreading of clouds or noise?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And thou shalt offer thy burnt offerings, the flesh and the blood, upon the altar of the LORD thy God: and the blood of thy sacrifices shall be poured out upon the altar of the LORD thy God, and thou shalt eat the flesh.',
  'On the altar Offer sacrifices burned, fleshed sacrifices, and eats blood.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'God forbid: for then how shall God judge the world?',
  'How does God judge the world?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'This is my comfort in my affliction: for thy word hath quickened me.',
  'I have your word comfort.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'That this shall be no grief unto thee, nor offence of heart unto my lord, either that thou hast shed blood causeless, or that my lord hath avenged himself: but when the LORD shall have dealt well with my lord, then remember thine handmaid.',
  'If thou hast shed blood unluckily or avenged thy mistress, Remember thy handmaid when my lord has dealt well.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'But let the righteous be glad; let them rejoice before God: yea, let them exceedingly rejoice.',
  'The right merry; the heavens rejoice exceedingly.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And he cometh, and findeth them sleeping, and saith unto Peter, Simon, sleepest thou?',
  'He comes, and they shall find sleeping, And he shall say to Simon.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Simon and they that were with him followed after him.',
  'They were followed by Simon and they.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'He that is void of wisdom despiseth his neighbour: but a man of understanding holdeth his peace.',
  'He that lacks wisdom despises his neighbor, But that an understanding man holds peace.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'But when David saw that his servants whispered, David perceived that the child was dead: therefore David said unto his servants, Is the child dead?',
  'But David perceived the child dead when he saw his servants whispering.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'I will also stretch out mine hand upon Judah, and upon all the inhabitants of Jerusalem; and I will cut off the remnant of Baal from this place, and the name of the Chemarims with the priests;',
  'I’ll stretch my hand For all the gods in Jerusalem, And cut off the remnant of baal And the Chemarim.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'none is good, save one, that is, God.',
  'None good but God.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And the men of Judah said, Why are ye come up against us?',
  'Why have you come to us?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Jesus saith unto her, Woman, what have I to do with thee?',
  'What shall I do, woman?—Jesus, come hither.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The children of Hariph, an hundred and twelve.',
  'O Hariph!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Blessed be the LORD for evermore.',
  "God 'ild you for ever."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Hezekiah also had said, What is the sign that I shall go up to the house of the LORD?',
  'And what sign didst thou give me to go to the house, Zekekiah?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he said unto her, Daughter, thy faith hath made thee whole; go in peace, and be whole of thy plague.',
  'Daughter, your faith hath made thee whole; Go with a peace.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Because of the savour of thy good ointments thy name is as ointment poured forth, therefore do the virgins love thee.',
  'Since thy name is good ointments, virgins do love thee.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Therefore, behold, the days come, saith the LORD, that it shall no more be called Tophet, nor the valley of the son of Hinnom, but the valley of slaughter: for they shall bury in Tophet, till there be no place.',
  "It shall not be call'd Tophet, but the Valley of Honnom."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'The LORD shall laugh at him: for he seeth that his day is coming.',
  'He did laugh upon seeing his day coming.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Many are the afflictions of the righteous: but the LORD delivereth him out of them all.',
  'Many a righteous man suffers, But the Lord delivers him.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  "Kerioth is taken, and the strong holds are surprised, and the mighty men's hearts in Moab at that day shall be as the heart of a woman in her pangs.",
  'The King was taken, and the strong-held Duke surprised, And on that day the mighty men’s hearts were in Moab.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Have ye offered unto me sacrifices and offerings in the wilderness forty years, O house of Israel?',
  'Hast thou offered forty years of sacrifice and thyself in the wilderness?'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'The law of truth was in his mouth, and iniquity was not found in his lips: he walked with me in peace and equity, and did turn many away from iniquity.',
  'He walked with me in peace and equity And turned away many to infidelity.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the LORD said, Judah shall go up: behold, I have delivered the land into his hand.',
  'I have delivered land to Judah.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And Jesus stood still, and commanded him to be called.',
  'Still stood Jesu, and thou didst tell him he had called.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Yea, thou shalt be as he that lieth down in the midst of the sea, or as he that lieth upon the top of a mast.',
  "Thou art like him that lies down i' th' sea, Or on the top of a mast."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'And the king said, What have I to do with you, ye sons of Zeruiah?',
  'What have I to do with you, Feruiah?'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'Let the floods clap their hands: let the hills be joyful together',
  'Let the floods clap their hands, and let the hills be merry together.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Praise ye the LORD: for it is good to sing praises unto our God; for it is pleasant; and praise is comely.',
  "Tis good that our gracious God be sing'd praise."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Now three of the thirty captains went down to the rock to David, into the cave of Adullam; and the host of the Philistines encamped in the valley of Rephaim.',
  'Three of the thirty captains Down into the rock to the cave of Audullam, And in the valley of Rephaim encamp the Philippians.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And called, and asked whether Simon, which was surnamed Peter, were lodged there.',
  'He hath called and asked if Simon, the surname of Peter, be there.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Then answered Eliphaz the Temanite, and said,',
  'Say, Elliphaz.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Afterward I came unto the house of Shemaiah the son of Delaiah the son of Mehetabeel, who was shut up; and he said, Let us meet together in the house of God, within the temple, and let us shut the doors of the temple: for they will come to slay thee; yea, in the night will they come to slay thee.',
  'Then, Shemaiah, your son to Laiah, said let us meet at God’s house And shut the temple doors.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Therefore the Jews sought the more to kill him, because he not only had broken the sabbath, but said also that God was his Father, making himself equal with God.',
  'He hath broke the sabbath, and he hath said “God his father also”— The Jew wants the Jew to kill him.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Honour thy father and mother; which is the first commandment with promise;',
  'First, let thy father and mother honor each other.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And when he cometh home, he calleth together his friends and neighbours, saying unto them, Rejoice with me; for I have found my sheep which was lost.',
  'When he comes home, he calls on friends and neighbors together, Saying he was merry at finding his lost sheep.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'But fornication, and all uncleanness, or covetousness, let it not be once named among you, as becometh saints;',
  'But saints should not be named Fornicates, uncleanliness, or covetousness.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And the king put them in the house of the forest of Lebanon.',
  'The king hath put them in the Lebanon’s house.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'There remaineth therefore a rest to the people of God.',
  'For God’s rest.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'But God giveth it a body as it hath pleased him, and to every seed his own body.',
  'But God gives me as many bodies as it gives, And every seed of it.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Whom I perceived to be accused of questions of their law, but to have nothing laid to his charge worthy of death or of bonds.',
  'His accusation, as I perceived it, is a question of law, but he shall have nothing in him for a charge that he deserves his death or his bond.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'art not thou he, O LORD our God?',
  'Is he not?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Thou hast covered with anger, and persecuted us: thou hast slain, thou hast not pitied.',
  'Thou hast covered thy anger, And persecuted us.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the Sabeans fell upon them, and took them away; yea, they have slain the servants with the edge of the sword; and I only am escaped alone to tell thee.',
  'The Sardians have slain their servants with a sword, And only by this I have escaped alone To tell them of them.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Cursed be he that confirmeth not all the words of this law to do them.',
  'I am curious he confirms not all the words of this law.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And it came to pass, when their hearts were merry, that they said, Call for Samson, that he may make us sport.',
  'They call Samson, that he may make us sport.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And all the army of the Chaldees, that were with the captain of the guard, brake down the walls of Jerusalem round about.',
  "The army hath braked down the walls of Jerusalem, i' faith."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Moses said unto the LORD, The people cannot come up to mount Sinai: for thou chargedst us, saying, Set bounds about the mount, and sanctify it.',
  'Thou hast said He will set a limit about him And sanctify him thus: men cannot come on Shinai.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And thou shalt make a vail of blue, and purple, and scarlet, and fine twined linen of cunning work: with cherubims shall it be made:',
  'With cherubims make a vaunt Of blue, purple, scarlet, and fine twine linen.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But Hannah went not up; for she said unto her husband, I will not go up until the child be weaned, and then I will bring him, that he may appear before the LORD, and there abide for ever.',
  'But Hannah went not up; she said she would not go with her till the babes were weaned; And that she was my husband.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And all things are of God, who hath reconciled us to himself by Jesus Christ, and hath given to us the ministry of reconciliation;',
  'God, that in Christ Jesus reconciled us, hath given us ministry of reconcilion.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Seeing then that I will cut off from thee the righteous and the wicked, therefore shall my sword go forth out of his sheath against all flesh from the south to the north:',
  "And then, seeing that I had cut off thyself, the right, and the bad, I’d go with my sword out of my sheath against all flesh o'er the south and north."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'so I might have taken her to me to wife: now therefore behold thy wife, take her, and go thy way.',
  'I could have taken her to my wife.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'O continue thy lovingkindness unto them that know thee; and thy righteousness to the upright in heart.',
  'Continue to love those that know you.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And Stephen, full of faith and power, did great wonders and miracles among the people.',
  'Stephen, full of faith and power, Did great marvels and miracles unto this place.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And he shall speak great words against the most High, and shall wear out the saints of the most High, and think to change times and laws: and they shall be given into his hand until a time and times and the dividing of time.',
  'He’ll speak great words against the highest, wear out saints, and think to change times and laws.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'or came it unto you only?',
  'Or only came it from you?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Blessed is the man that feareth the LORD, that delighteth greatly in his commandments.',
  'Bless the fearful who delights in his commands!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And he went and sent to Jehoshaphat the king of Judah, saying, The king of Moab hath rebelled against me: wilt thou go with me against Moab to battle?',
  'He hath said that Jehoshaphat, the king of Judah, Rebelled against me.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And it came to pass through the lightness of her whoredom, that she defiled the land, and committed adultery with stones and with stocks.',
  'And so she hath defiled the country And committed adultery with stones and stocks.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'That all the people of the earth may know that the LORD is God, and that there is none else.',
  'That every man may know both God and no man else.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the city had no need of the sun, neither of the moon, to shine in it: for the glory of God did lighten it, and the Lamb is the light thereof.',
  'There is no need of sun in the city, nor no need of moon.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And Joshua rose early in the morning, and the priests took up the ark of the LORD.',
  'Joshua rose early in the morning, and the priests took the ark.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'To morrow, said he, thou shalt hear him.',
  'He said thou shalt hear tomorrow.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the beast which I saw was like unto a leopard, and his feet were as the feet of a bear, and his mouth as the mouth of a lion: and the dragon gave him his power, and his seat, and great authority.',
  'The beast that I saw was a leopard; The bear’s feet were the mouth of a lion, and the dragon gave him power.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'We be twelve brethren, sons of our father; one is not, and the youngest is this day with our father in the land of Canaan.',
  'We are now twelve brothers, not one, in Canaan, and our youngest father there.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And he said unto me, Go in, and behold the wicked abominations that they do here.',
  'Go to, and see The abominables they do here.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And Azariah the son of Jehoram king of Judah went down to see Jehoram the son of Ahab at Jezreel, because he was sick.',
  'Ay, and then, Ariah, to Jezreel To see the son of Abram, Jehoram.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'The LORD will strengthen him upon the bed of languishing: thou wilt make all his bed in his sickness.',
  'The Lord strengthen him in his bed, for he is ill.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And they returned to Joshua, and said unto him, Let not all the people go up; but let about two or three thousand men go up and smite Ai; and make not all the people to labour thither; for they are but few.',
  'Do not go back to Joshua, And say there be about two thousand up And kill Ai, but make all men in labor there.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'So a measure of fine flour was sold for a shekel, and two measures of barley for a shekel, according to the word of the LORD.',
  'A gram of fine flour is to be sold For a shekel, and two gram of fine flour to be sold For a shekel.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And thou shalt put it under the compass of the altar beneath, that the net may be even to the midst of the altar.',
  'Thou hast put a net under the altar.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'and when wilt thou return?',
  "And when thou return'st?"],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And he brought in the priests and the Levites, and gathered them together into the east street,',
  'He hath assembled the priests and leviteses In the east street.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the angel of the LORD appeared unto the woman, and said unto her, Behold now, thou art barren, and bearest not: but thou shalt conceive, and bear a son.',
  'Angel appeared to the woman and she said she was barren and would not bear her son.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'If a false witness rise up against any man to testify against him that which is wrong;',
  'Ay, if a false witness rise against any man to testify a wrong.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And when the Pharisees saw it, they said unto his disciples, Why eateth your Master with publicans and sinners?',
  'When the Pharisee saw it, why ate thou thy master with publics and sinners?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'whom seekest thou?',
  'What seek’st thou?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Whosoever committeth sin transgresseth also the law: for sin is the transgression of the law.',
  'Those that commit sin do violate the law, for sin is sin.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Even the country which the LORD smote before the congregation of Israel, is a land for cattle, and thy servants have cattle:',
  'Even in this land Are cattle raised, and your servants have such lands.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Behold, a virgin shall be with child, and shall bring forth a son, and they shall call his name Emmanuel, which being interpreted is, God with us.',
  'A virgin bears a babe and is to call him Emmanuel, Interpreted as God with us.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Then will I make this house like Shiloh, and will make this city a curse to all the nations of the earth.',
  'I’ll make this house like Shiloh, And make all nations curse me.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Zechariah, and Aziel, and Shemiramoth, and Jehiel, and Unni, and Eliab, and Maaseiah, and Benaiah, with psalteries on Alamoth;',
  'Here comes Zachariah and Aziel, Shemiramoth and Jesu, Lamiah, Maseiah and Benaiah, And psalteries of Alamoth.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And Jacob their father said unto them, Me have ye bereaved of my children: Joseph is not, and Simeon is not, and ye will take Benjamin away: all these things are against me.',
  'Jacob is bereaved of his children; Joseph is not bereaved, Simon not bereaved, and you take away Benjamin.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And Joab returned to Jerusalem unto the king.',
  'Joab returned to Jerusalem.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And with you there shall be a man of every tribe; every one head of the house of his fathers.',
  'You have every tribe’s man that heads the house their fathers.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'But will God in very deed dwell with men on the earth?',
  'But is it God himself that lives on earth?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'And Moses did as the LORD commanded: and they went up into mount Hor in the sight of all the congregation.',
  'Moses upon the mountain of Hor did the will that the Lord gave him command.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Now when the centurion saw what was done, he glorified God, saying, Certainly this was a righteous man.',
  'When the centurion saw what was done, He glorified God and said “This is certain right.” Why, that’s the saying.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And it came to pass on the morrow, that Moses sat to judge the people: and the people stood by Moses from the morning unto the evening.',
  'Sir, in the morning and evening, When the clock was set, Moses sat down to judge the people.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'This people draweth nigh unto me with their mouth, and honoureth me with their lips; but their heart is far from me.',
  'These Moors do draw me from their mouths And honor me with their lips, But my far-favorite heart Is in the middle.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the dogs shall eat Jezebel in the portion of Jezreel, and there shall be none to bury her.',
  'The dogs will eat a portion of Jezebel, and bury them.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But I will punish you according to the fruit of your doings, saith the LORD: and I will kindle a fire in the forest thereof, and it shall devour all things round about it.',
  'But I will punish you according to the fruits that you have done.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'They provoked him to jealousy with strange gods, with abominations provoked they him to anger.',
  "The strange gods' abominables provoked him to anger."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'A man that is an heretick after the first and second admonition reject;',
  "The guy that first admonish'd is rejected Is heretick after a second sentence and a third."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'That they may want bread and water, and be astonied one with another, and consume away for their iniquity.',
  'They may want bread and water, and be astonished to consume ’t.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Iniquities prevail against me: as for our transgressions, thou shalt purge them away.',
  'Injustice doth prevail upon me, Thy purgation of our transgressions doth reign.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'what is mine iniquity?',
  'What is my infirmity?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'And the time that David dwelt in the country of the Philistines was a full year and four months.',
  "For four months o'er th' life of David in Philippi, It shall be full fourscore ducats."],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And Samlah died, and Saul of Rehoboth by the river reigned in his stead.',
  'Hamlet, he is dead, and Saul of Rehoboth reigns upon the river.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'They send forth their little ones like a flock, and their children dance.',
  'They send their little ones out like a flock, and their children dance.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Therefore I make a decree, That every people, nation, and language, which speak any thing amiss against the God of Shadrach, Meshach, and Abednego, shall be cut in pieces, and their houses shall be made a dunghill: because there is no other God that can deliver after this sort.',
  'I have resolved To cut to pieces every man, every nation, every language that speak against Shadrach, Messach, and Abednego.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'So he let him go: then she said, A bloody husband thou art, because of the circumcision.',
  'He let him go, and then she said, for circumcision, he was a bloody husband.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  "Or, Deliver me from the enemy's hand?",
  'Or wilt thou deliver me to thy enemy’s hand?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'But as soon as this thy son was come, which hath devoured thy living with harlots, thou hast killed for him the fatted calf.',
  'But thou hast killed a fat calf As soon as thy son hath devoured thy living with harlots.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Thou shalt also make a table of shittim wood: two cubits shall be the length thereof, and a cubit the breadth thereof, and a cubit and a half the height thereof.',
  'Thou also makest a table of shit wood: two cubits is as much, and half a cubit is as much.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Behold, the nations are as a drop of a bucket, and are counted as the small dust of the balance: behold, he taketh up the isles as a very little thing.',
  'Look like a drop in a bucket, And count the small dust of the balance.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'O Israel, thy prophets are like the foxes in the deserts.',
  'The prophets of Israel are like foxes in the desert.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Therefore prophesy and say unto them, Thus saith the Lord GOD; Behold, O my people, I will open your graves, and cause you to come up out of your graves, and bring you into the land of Israel.',
  'Therefore prophesy, and say, I will open thy graves And bring thee to Israel.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'They shall run like mighty men; they shall climb the wall like men of war; and they shall march every one on his ways, and they shall not break their ranks:',
  'They’ll run like great men, climb the wall like men of war; They’ll march every man through their ways, They’ll not break their ranks, but they’ll be kings.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'Why doth this man thus speak blasphemies?',
  'Why doth this gentleman speak blasphemy?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'The tongue deviseth mischiefs; like a sharp razor, working deceitfully.',
  'The tongue is like a sharp razor, deceivingly working.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And they which went before rebuked him, that he should hold his peace: but he cried so much the more, Thou son of David, have mercy on me.',
  'They rebuked him before, but so much cried, “Hath mercy, my lord?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'For the oppression of the poor, for the sighing of the needy, now will I arise, saith the LORD; I will set him in safety from him that puffeth at him.',
  'Now, for the poor and needy, I stand him safe from the puffers.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'The LORD hath sworn, and will not repent, Thou art a priest for ever after the order of Melchizedek.',
  'Yea, Melchizedek swore, and did not repent.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'The lip of truth shall be established for ever: but a lying tongue is but for a moment.',
  'A truth forever established, not a lying tongue, But a tongue that in the moment speaks.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'According to the days of thy coming out of the land of Egypt will I shew unto him marvellous things.',
  'I say a wonderful thing thou art coming from Egypt.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Moab shall be destroyed from being a people, because he hath magnified himself against the LORD.',
  'Moab is destroyed by his magnificence.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'For thine arrows stick fast in me, and thy hand presseth me sore.',
  'Thy arrows stick fast upon me, and his hand Presses me to a reproach.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Jesus answered, He it is, to whom I shall give a sop, when I have dipped it.',
  'When I have dipped it, I will give Jesu a sop.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Therefore say, Thus saith the Lord GOD; Although I have cast them far off among the heathen, and although I have scattered them among the countries, yet will I be to them as a little sanctuary in the countries where they shall come.',
  'I am scattered among them, Yet in the countries where they come I am as little refuge.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Then the eyes of the blind shall be opened, and the ears of the deaf shall be unstopped.',
  'Then blind men’s eyes are opened, and the ears deaf.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And Saul, and Jonathan his son, and the people that were present with them, abode in Gibeah of Benjamin: but the Philistines encamped in Michmash.',
  "Saul and his son Jonathan live in Gibraltar, But in Philippines' camp at Michmash."],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Pour out thine indignation upon them, and let thy wrathful anger take hold of them.',
  'Pour thy indignation on them, And let thy wrathful anger take hold on them.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Slay utterly old and young, both maids, and little children, and women: but come not near any man upon whom is the mark; and begin at my sanctuary.',
  'Old men, young men, maids, little children, and women In total slaying, but come not near anyone, and begin my sanctuary.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And when they came down to him, Elisha prayed unto the LORD, and said, Smite this people, I pray thee, with blindness.',
  'When they came down, Elisha said, “Thou kill’st this man, and be blind.” Well said.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the serpent said unto the woman, Ye shall not surely die:',
  'For certain, the serpent said a woman would not die.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And there were made on them, on the doors of the temple, cherubims and palm trees, like as were made upon the walls; and there were thick planks upon the face of the porch without.',
  'The cherubims and palm-trees are at the temple doors, And the thick planks on the porch face.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  "And as the ark of the LORD came into the city of David, Michal Saul's daughter looked through a window, and saw king David leaping and dancing before the LORD; and she despised him in her heart.",
  'The daughter of Michael Salomon looked out at window, She saw the King David leaping and dancing before him, And he despised her.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And he left them, and went away again, and prayed the third time, saying the same words.',
  'He left them, and went away again, and pronounced the third same.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And he shall pass over to his strong hold for fear, and his princes shall be afraid of the ensign, saith the LORD, whose fire is in Zion, and his furnace in Jerusalem.',
  'He shall pass over a strong hold for fear, And then ’tis a soldier’s fear.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'Forty and two years old was Ahaziah when he began to reign, and he reigned one year in Jerusalem.',
  'Ahaziah shall live one year in Jerusalem.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Behold, I will bring evil upon thee, and will take away thy posterity, and will cut off from Ahab him that pisseth against the wall, and him that is shut up and left in Israel,',
  'I’ll bring thee evil, take away thy posterity, Cut off the pissing wall, And shutting up those that left Israel.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'curse God, and die.',
  'O God’s curse!'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And upon the table of shewbread they shall spread a cloth of blue, and put thereon the dishes, and the spoons, and the bowls, and covers to cover withal: and the continual bread shall be thereon:',
  'They’ll spread a blue cloth upon the table And put on dishes, spoons, and covers.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Whosoever putteth away his wife, and marrieth another, committeth adultery: and whosoever marrieth her that is put away from her husband committeth adultery.',
  'If a wife do marry her husband, she commits adultery.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'He that sacrificeth unto any god, save unto the LORD only, he shall be utterly destroyed.',
  'Those that do sacrifice themselves to any god, Save only God, are utterly destroyed.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Then said I, Whither goest thou?',
  'Whither goest thou then?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And said unto the king, Let not my lord impute iniquity unto me, neither do thou remember that which thy servant did perversely the day that my lord the king went out of Jerusalem, that the king should take it to his heart.',
  'Do not impute iniquity to me, nor remember That your servant did me on the day my lord left Jerusalem.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'But into the second went the high priest alone once every year, not without blood, which he offered for himself, and for the errors of the people:',
  'But every year the high priest went alone, Who hath not the blood that he offered his master and his error.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Lift up your eyes, and behold them that come from the north: where is the flock that was given thee, thy beautiful flock?',
  'Lift up thine eyes, Where the fair flock is.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And when Paul was now about to open his mouth, Gallio said unto the Jews, If it were a matter of wrong or wicked lewdness, O ye Jews, reason would that I should bear with you:',
  'Gallio said, when Paul was about to open his mouth, “If it have any cause to bear you wrong or evil,” When he was about to say, “You shall have reason to bear with me.” Well said, Jew.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Then Zedekiah the son of Chenaanah came near, and smote Micaiah upon the cheek, and said, Which way went the Spirit of the LORD from me to speak unto thee?',
  'Then came Zedekiah, the son of Chenaanah, near him, And on the cheek did he kiss Miah, and say “Amen” to him.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'And many nations shall come, and say, Come, and let us go up to the mountain of the LORD, and to the house of the God of Jacob; and he will teach us of his ways, and we will walk in his paths: for the law shall go forth of Zion, and the word of the LORD from Jerusalem.',
  'Many a nation come and say, Let us go to the Moor of Jacob And to his paths.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'These are the words of the covenant, which the LORD commanded Moses to make with the children of Israel in the land of Moab, beside the covenant which he made with them in Horeb.',
  'This is the covenant that Moses made with the Jew of Israel, and it is the covenant that Horatio made with the Jew of Nazareth.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Judge me, O LORD; for I have walked in mine integrity: I have trusted also in the LORD; therefore I shall not slide.',
  'Judge me as I have walked in my integrity.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'When Jesus understood it, he said unto them, Why trouble ye the woman?',
  'When Jesu understood it, why should a woman trouble herself?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'The ancients of Gebal and the wise men thereof were in thee thy calkers: all the ships of the sea with their mariners were in thee to occupy thy merchandise.',
  'Your ships and mariners are in your ships To occupy your merchandise.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'The poor and the deceitful man meet together: the LORD lighteneth both their eyes.',
  'Poor men will meet together in deceitful man.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Fair weather cometh out of the north: with God is terrible majesty.',
  'The fair weather is coming north.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'But he answered and said unto him that told him, Who is my mother?',
  'But he answered, and told him who is his mother?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Nebuchadnezzar spake and said unto them, Is it true, O Shadrach, Meshach, and Abednego, do not ye serve my gods, nor worship the golden image which I have set up?',
  'Hast thou said, Nebuchadnezzar, Shadrach and Meshach and Abednego not serve my gods And worship not the golden image that I set down?'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'The day following Jesus would go forth into Galilee, and findeth Philip, and saith unto him, Follow me.',
  'The day is following, And Jesus will go to Israel and find Philippi.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'For strangers are risen up against me, and oppressors seek after my soul: they have not set God before them.',
  'Strangers have risen against me, and oppressors seek God’s will.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And they rose up early in the morning, and the sun shone upon the water, and the Moabites saw the water on the other side as red as blood:',
  "They rose early in the morning, and the sun glimm'd in the water, And the Moabites saw them red-beloved."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And Jesus said, For judgment I am come into this world, that they which see not might see; and that they which see might be made blind.',
  'Jesu said I had come from this world to judge those that see not.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'He shall break also the images of Bethshemesh, that is in the land of Egypt; and the houses of the gods of the Egyptians shall he burn with fire.',
  'He will break, too, the images of Bethshemesh, Egypt, For ’tis an Egyptian city.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the spirit cried, and rent him sore, and came out of him: and he was as one dead; insomuch that many said, He is dead.',
  'The spirit cries, out, and he is dead.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'To every thing there is a season, and a time to every purpose under the heaven:',
  'Under heaven there is seasons and time for all things.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Take heed unto thyself, and unto the doctrine; continue in them: for in doing this thou shalt both save thyself, and them that hear thee.',
  'By doing this, thou art saved both thyself and those that listen.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'O give thanks unto the God of gods: for his mercy endureth for ever.',
  'Thanks, good God.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'He measured the east side with the measuring reed, five hundred reeds, with the measuring reed round about.',
  'He measured the east side with a hundred reeds.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Cain talked with Abel his brother: and it came to pass, when they were in the field, that Cain rose up against Abel his brother, and slew him.',
  'Cain talked with his brother Abel, and he slew him.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Saying, God hath forsaken him: persecute and take him; for there is none to deliver him.',
  'Say that God hath abandoned him, persecuted him, and took him.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'But the day of the Lord will come as a thief in the night; in the which the heavens shall pass away with a great noise, and the elements shall melt with fervent heat, the earth also and the works that are therein shall be burned up.',
  'But pass through the skies and elements with great noise And melt the earth with fervent heat.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Jude, the servant of Jesus Christ, and brother of James, to them that are sanctified by God the Father, and preserved in Jesus Christ, and called:',
  "Jude shall be sanctified by God's father, and preserved by him."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'For this city hath been to me as a provocation of mine anger and of my fury from the day that they built it even unto this day; that I should remove it from before my face,',
  "The day they built I would remove them before my face, For this city hath stol'n my anger and me."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'why do ye not rather suffer yourselves to be defrauded?',
  'Why shouldst thou rather suffer thy defraudation?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incomplete',
  'Until the day break, and the shadows flee away, turn, my beloved, and be thou like a roe or a young hart upon the mountains of Bether.',
  'Till the break of day, And the shadows fled away, Turn thee, thee like a roe or young hart In the mountains of Bether.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Against him came up Nebuchadnezzar king of Babylon, and bound him in fetters, to carry him to Babylon.',
  'The king of Babylon, Nebuchadnezzar, Binds him in fetters to carry him to his Majesty.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'This their way is their folly: yet their posterity approve their sayings.',
  'Their way is foolish, but their posterity approves what they say.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The rest of all the acts of Asa, and all his might, and all that he did, and the cities which he built, are they not written in the book of the chronicles of the kings of Judah?',
  'Is not all the deeds of Asa in a book of history, All the deeds he did, all the cities he built, Written in letters?'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And the spoiler shall come upon every city, and no city shall escape: the valley also shall perish, and the plain shall be destroyed, as the LORD hath spoken.',
  'The spoiler comes from every city, and no one shall evade, and the valley is dead and the plain destroyed.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Not that any man hath seen the Father, save he which is of God, he hath seen the Father.',
  'No man besides his father saw him.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'When he was removed out of the highway, all the people went on after Joab, to pursue after Sheba the son of Bichri.',
  'When Joab was removed from the highway, All the people went to pursue Sheba.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the man smote him, so that in smiting he wounded him.',
  'Why, man, smite him, he’s wounded.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incomplete',
  'So we thy people and sheep of thy pasture will give thee thanks for ever: we will shew forth thy praise to all generations.',
  'We have ever thanks for your person, your pasture-sheep; Our praises do show to all generations.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Sharp arrows of the mighty, with coals of juniper.',
  'There are sharp arrows in the juniper.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And I saw three unclean spirits like frogs come out of the mouth of the dragon, and out of the mouth of the beast, and out of the mouth of the false prophet.',
  'I saw three unclean spirits, like frogs.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Therefore, brethren, we are debtors, not to the flesh, to live after the flesh.',
  'Then we are debtors, but want not to live after flesh.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Wherefore she said unto Abraham, Cast out this bondwoman and her son: for the son of this bondwoman shall not be heir with my son, even with Isaac.',
  'So she said to her son Abraham, “cast this bondwoman and her son out.” Well said.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And it came to pass, when Jesus had made an end of commanding his twelve disciples, he departed thence to teach and to preach in their cities.',
  'And in the end, when he had done commandment, Did Jesus leave the city to teach and preach to a dozen disciples.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'and she, even she herself said, He is my brother: in the integrity of my heart and innocency of my hands have I done this.',
  'Even she said he, her brother, was her integrity and his innocence.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Of the tribe of Nephthalim were sealed twelve thousand.',
  "The nephthalim was seal'd twelve years ago."],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And the very God of peace sanctify you wholly; and I pray God your whole spirit and soul and body be preserved blameless unto the coming of our Lord Jesus Christ.',
  'The very peace-loving God sanctifies you entirely; I pray him preserve your spirit, your soul, and your body whole, Without any blame.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Judge not, and ye shall not be judged: condemn not, and ye shall not be condemned: forgive, and ye shall be forgiven:',
  'Judge not, and be not judged.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Of the first of your dough ye shall give unto the LORD an heave offering in your generations.',
  'Thy first dough Will I give thee to thy Lord in thy generation.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And it came to pass also on another sabbath, that he entered into the synagogue and taught: and there was a man whose right hand was withered.',
  'He entered the synagogue and taught it also on another sabbath.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And they gathered their brethren, and sanctified themselves, and came, according to the commandment of the king, by the words of the LORD, to cleanse the house of the LORD.',
  'They gathered their brothers And sanctified them, and came Conforming to the command of the king.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'or their border greater than your border?',
  'Or is their border greater than yours?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Then said I unto them, Ye see the distress that we are in, how Jerusalem lieth waste, and the gates thereof are burned with fire: come, and let us build up the wall of Jerusalem, that we be no more a reproach.',
  'Thou dost see our distress, And burnst both Jerusalem and her gates.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the city was besieged unto the eleventh year of king Zedekiah.',
  'The king, Zedekiah, is besieged of the city.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And Peter answered unto her, Tell me whether ye sold the land for so much?',
  'Tell me, lord, if thou hast sold so much the land.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Harbonah, one of the chamberlains, said before the king, Behold also, the gallows fifty cubits high, which Haman had made for Mordecai, who spoken good for the king, standeth in the house of Haman.',
  'Say to Harbonah, one of the king’s subjects, “Seest thou a gallows fifty cubits high, Made by Hamani to good Mordecai”!'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But Noah found grace in the eyes of the LORD.',
  'But Noah found grace in him.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'And if they were all one member, where were the body?',
  'Where be the bodies, if they were all One?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incomplete',
  'And Abijah stood up upon mount Zemaraim, which is in mount Ephraim, and said, Hear me, thou Jeroboam, and all Israel;',
  'Abijah stood upon Mount Zemaraim, On Mount Ephraim, and spake, “Hear, Jeroboam, and all Israel!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'The two pillars, one sea, and twelve brasen bulls that were under the bases, which king Solomon had made in the house of the LORD: the brass of all these vessels was without weight.',
  'Two pillars of sea and twelve brasen bulls, under the bases, That made noble Solomon the king, Had no weight.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Surely thou wilt slay the wicked, O God: depart from me therefore, ye bloody men.',
  'For God’s sake, I am sure you have slain an evil man.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "And they shall bear the curtains of the tabernacle, and the tabernacle of the congregation, his covering, and the covering of the badgers' skins that is above upon it, and the hanging for the door of the tabernacle of the congregation,",
  'They bear the curtains at the tabernacle and cover the badger’s skin above.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'My lips shall not speak wickedness, nor my tongue utter deceit.',
  'Mine mouth would not speak of evil, Nor my tongue would speak of deceit.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And they marvelled all.',
  'They are all amazed.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'Thanks be unto God for his unspeakable gift.',
  'God be thanked for thy unspoke gift.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the manna ceased on the morrow after they had eaten of the old corn of the land; neither had the children of Israel manna any more; but they did eat of the fruit of the land of Canaan that year.',
  "When they have eaten up the manna from the old Israeli corn, They have stopped that year's harvest."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And when Peter saw it, he answered unto the people, Ye men of Israel, why marvel ye at this?',
  'Peter wonders when he sees it, why this amazes the Israelis.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And when thou prayest, thou shalt not be as the hypocrites are: for they love to pray standing in the synagogues and in the corners of the streets, that they may be seen of men.',
  'Since they love to pray, And stand in synagogues and in streets corners, Be not hypocrites when you are so.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'In the year of this jubile ye shall return every man unto his possession.',
  'On this anniversary Return all thy possession.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'now therefore receive no more money of your acquaintance, but deliver it for the breaches of the house.',
  'Why, then, now you receive no more money, but you’ll deliver to your acquaintance.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'A seed shall serve him; it shall be accounted to the Lord for a generation.',
  "The seed shall serve him; for each generation is account'd."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Now among these were of the children of Judah, Daniel, Hananiah, Mishael, and Azariah:',
  'Among them are Daniel, Hananiah, Mishael, and Azariah.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'To whom coming, as unto a living stone, disallowed indeed of men, but chosen of God, and precious,',
  'Indeed, the living stone is not allowed to come, But that God hath chosen, and that stone is precious.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And Adam was not deceived, but the woman being deceived was in the transgression.',
  'Adam was not deceived, but a woman.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'But in the place which the LORD shall choose in one of thy tribes, there thou shalt offer thy burnt offerings, and there thou shalt do all that I command thee.',
  'But there thou canst offer thy burned goods To all my tribes, and do All that I command in thine own hand.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'The hands of the pitiful women have sodden their own children: they were their meat in the destruction of the daughter of my people.',
  'Wretched women have slaughtered their children.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And the children of Israel returned from chasing after the Philistines, and they spoiled their tents.',
  "They returned from the chase For the Philippians, and ruin'd their tents."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And afterward I will bring again the captivity of the children of Ammon, saith the LORD.',
  'I will return to captivity then.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'As for thee also, by the blood of thy covenant I have sent forth thy prisoners out of the pit wherein is no water.',
  "I have also sent your prisoner out o' th' pit where there is no water."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And that which cometh into your mind shall not be at all, that ye say, We will be as the heathen, as the families of the countries, to serve wood and stone.',
  'And thou didst not say that we did serve wood and stone at once.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'The fig tree putteth forth her green figs, and the vines with the tender grape give a good smell.',
  'The fig tree hath laid her green figs out, And the tender grapes do smell good.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Lest he that heareth it put thee to shame, and thine infamy turn not away.',
  'Thou art ashamed he heard it, and thy infamy Doth not turn away.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'For which cause both thou and all thy company are gathered together against the LORD: and what is Aaron, that ye murmur against him?',
  'Why have you, and all your company, Gathered against Aaron?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'He layeth up sound wisdom for the righteous: he is a buckler to them that walk uprightly.',
  'He lays sound wisdom upon those that walk upright.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'It is in the power of my hand to do you hurt: but the God of your father spake unto me yesternight, saying, Take thou heed that thou speak not to Jacob either good or bad.',
  "But God be wi' you, be wi' you, that said to me yesterday, “No good or bad word of Jacob,” That you should speak not of him."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the great court round about was with three rows of hewed stones, and a row of cedar beams, both for the inner court of the house of the LORD, and for the porch of the house.',
  'The great court is made up of three rows of honed stones, one of cedar beams, And the rest is made up of cedar.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'All nations whom thou hast made shall come and worship before thee, O Lord; and shall glorify thy name.',
  'All the nations thou hast made will come and worship thyself.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And am no more worthy to be called thy son: make me as one of thy hired servants.',
  'I have no less deserved your call to be one of your servants’ hirers.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Wash you, make you clean; put away the evil of your doings from before mine eyes; cease to do evil;',
  'Wash thyself, clean thyself; cease all evil that thou dost before mine eyes.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'But ye have borne the tabernacle of your Moloch and Chiun your images, the star of your god, which ye made to yourselves.',
  'But thou carriest the images of thine own stars, Moloch and Chiun.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the rough goat is the king of Grecia: and the great horn that is between his eyes is the first king.',
  'Rough goats, you are kings of Greece.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And there shall ye remember your ways, and all your doings, wherein ye have been defiled; and ye shall lothe yourselves in your own sight for all your evils that ye have committed.',
  'Thou rememberest thy ways and all thy deeds, And forgivest all thy evils that thou hast committed.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The LORD hath cast off his altar, he hath abhorred his sanctuary, he hath given up into the hand of the enemy the walls of her palaces; they have made a noise in the house of the LORD, as in the day of a solemn feast.',
  "The Lord hath cast his altar off, Abhorred his sanctuary, gave o'er her palace walls."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'From the wicked that oppress me, from my deadly enemies, who compass me about.',
  'From mine oppressors, enemies that kill themselves.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Moreover, brethren, I would not that ye should be ignorant, how that all our fathers were under the cloud, and all passed through the sea;',
  "Nor did I desire thee to know How all our fathers were enshelter'd under a cloud And passed through the sea."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Let thine eyes be on the field that they do reap, and go thou after them: have I not charged the young men that they shall not touch thee?',
  'Observe your eyes upon the field they reap, And go to ’t, and I will not charge the young man to touch you?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'hath not David rather sent his servants unto thee, to search the city, and to spy it out, and to overthrow it?',
  'Did David send his servants to search the city, Spies the city, and overthrow him?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Let every man abide in the same calling wherein he was called.',
  'Let every man abide his own calling as his own.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And Jacob did so, and fulfilled her week: and he gave him Rachel his daughter to wife also.',
  'By Jacob, ’tis done, ’tis fulfilled in his week, And he hath also given his daughter daughter Rachel for her.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And I fell down before the LORD, as at the first, forty days and forty nights: I did neither eat bread, nor drink water, because of all your sins which ye sinned, in doing wickedly in the sight of the LORD, to provoke him to anger.',
  'For all thy sins, I will not eat bread nor drink water.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And of the Gadites there separated themselves unto David into the hold to the wilderness men of might, and men of war fit for the battle, that could handle shield and buckler, whose faces were like the faces of lions, and were as swift as the roes upon the mountains;',
  'Now the Gadites parted from David, who held him in the wilderness, And those that could handle a shield and a buckler Well, with faces like lions, were fit to bear them.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Even so it is not the will of your Father which is in heaven, that one of these little ones should perish.',
  'Yet your father’s will is not, To bring this little one to death.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Whoso robbeth his father or his mother, and saith, It is no transgression; the same is the companion of a destroyer.',
  'Those that have robbed their fathers or their mothers, And say it is no transgression, there is none.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And when a convenient day was come, that Herod on his birthday made a supper to his lords, high captains, and chief estates of Galilee;',
  'Hero, on his birthday, Made dinner with his lords, high-captains, and estates Of noble chiefs.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And the decree went forth that the wise men should be slain; and they sought Daniel and his fellows to be slain.',
  'Daniel and his friends have been determined To be slain, and both sought death.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Then Shaphan the scribe told the king, saying, Hilkiah the priest hath given me a book.',
  'Then the scribe, Stephano, told the king That Bishop Hilkiah had given the book to him.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  "Brethren, my heart's desire and prayer to God for Israel is, that they might be saved.",
  'For Israel’s sake am I drawn to save it, And I pray God it be so.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'They shall put you out of the synagogues: yea, the time cometh, that whosoever killeth you will think that he doeth God service.',
  'They’ll put you out of synagogue, and those that kill you Think they do serve God.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Joseph placed his father and his brethren, and gave them a possession in the land of Egypt, in the best of the land, in the land of Rameses, as Pharaoh had commanded.',
  'By order of Pharaoh, in Egypt Did Joseph put in his father and his brothers.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Thus saith the LORD; I am returned unto Zion, and will dwell in the midst of Jerusalem: and Jerusalem shall be called a city of truth; and the mountain of the LORD of hosts the holy mountain.',
  'I am returned to Zion; I dwell in Jerusalem.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Since the days of our fathers have we been in a great trespass unto this day; and for our iniquities have we, our kings, and our priests, been delivered into the hand of the kings of the lands, to the sword, to captivity, and to a spoil, and to confusion of face, as it is this day.',
  "We have been in this day's mischance since; 'tis now our day; 'tis now our night, 'tis now our night, 'tis now our night; 'tis now our night, 'tis night, 'tis night, 'tis night, 'tis night, 'tis night, 'tis night"],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And if he smite him with throwing a stone, wherewith he may die, and he die, he is a murderer: the murderer shall surely be put to death.',
  'The murderer, if he hit him with throwing stones.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Do not think that I will accuse you to the Father: there is one that accuseth you, even Moses, in whom ye trust.',
  'Think not of my accusation ’gainst your father; For even one of you Was under pressure of Moses.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'They go up by the mountains; they go down by the valleys unto the place which thou hast founded for them.',
  'They go up into the mountains and down into the valleys.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Thus saith the LORD to me; Make thee bonds and yokes, and put them upon thy neck,',
  'Therefore, I beseech you, make bonds with me, Take your yoke and put your neck in.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Is it fit to say to a king, Thou art wicked?',
  'Is ’t right to say thou art a knave, a knave, a knave, a knave, a knave, a knave, a knave?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'But if they will not obey, I will utterly pluck up and destroy that nation, saith the LORD.',
  'But if they will not obey, I’ll pluck up and destroy that nation.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Parthians, and Medes, and Elamites, and the dwellers in Mesopotamia, and in Judaea, and Cappadocia, in Pontus, and Asia,',
  'The Parthians, The Medes, The Amerindians, The Elephants, The Mesopotamias, The Cappadocians, And all the continent of Asia.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And they built for Pharaoh treasure cities, Pithom and Raamses.',
  'For Pharaoh, they built treasure towns of Pithom and Ramses.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'For when we were yet without strength, in due time Christ died for the ungodly.',
  'When our due time is come, Christ died when our strength still lay unshaken.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'Who is this that darkeneth counsel by words without knowledge?',
  'What ignorance does darken the counsels of time?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'The burden of the beasts of the south: into the land of trouble and anguish, from whence come the young and old lion, the viper and fiery flying serpent, they will carry their riches upon the shoulders of young asses, and their treasures upon the bunches of camels, to a people that shall not profit them.',
  "The young and old lion and the fiery flying serpent Carry their wealth and treasure on their young asses' shoulders To countries that do not profit them."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'He withdraweth not his eyes from the righteous: but with kings are they on the throne; yea, he doth establish them for ever, and they are exalted.',
  'He would not withdraw his eyes from the right; But where the kings are on the throne And forever establish themselves.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And her husband went with her along weeping behind her to Bahurim.',
  'Her husband and the weeping behind her went along with him.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'But because the LORD loved you, and because he would keep the oath which he had sworn unto your fathers, hath the LORD brought you out with a mighty hand, and redeemed you out of the house of bondmen, from the hand of Pharaoh king of Egypt.',
  'The Lord loved you, and kept the oath That he swore to your fathers; so he rescued you from the Pharaoh’s house.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The nethermost chamber was five cubits broad, and the middle was six cubits broad, and the third was seven cubits broad: for without in the wall of the house he made narrowed rests round about, that the beams should not be fastened in the walls of the house.',
  'The smallest chamber is five cubits wide, the middle six cubits wide, the third seven cubits wide.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'and when thou art athirst, go unto the vessels, and drink of that which the young men have drawn.',
  'When thou art athirst, go to the vessels and drink of young men’s blood.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "And I bought the field of Hanameel my uncle's son, that was in Anathoth, and weighed him the money, even seventeen shekels of silver.",
  'I bought my uncle’s field in Anathoth, And weighed the money even at seventeen shekels.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Which will not hearken to the voice of charmers, charming never so wisely.',
  'Charmers, do not hear you.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the Chaldeans shall come again, and fight against this city, and take it, and burn it with fire.',
  'Back do the Chaldeans come, And fight for this city.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And his brethren, chief of the fathers, two hundred forty and two: and Amashai the son of Azareel, the son of Ahasai, the son of Meshillemoth, the son of Immer,',
  'Amashai is the son of Ahasai, Meshillemoth’s son.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And he said, This is an ephah that goeth forth.',
  'This is the ephah.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  "Thou shalt not uncover the nakedness of thy father's sister: she is thy father's near kinswoman.",
  'Thou shalt not uncover naked thy father’s sister: she’s thy near mother.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Now Tobiah the Ammonite was by him, and he said, Even that which they build, if a fox go up, he shall even break down their stone wall.',
  'Tobiah the Ammonite said, if he go up, a fox would break even their stone wall.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'For to him that is joined to all the living there is hope: for a living dog is better than a dead lion.',
  'There’s hope a living dog is better than a dead lion.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And he saith unto the man which had the withered hand, Stand forth.',
  'He spake to you, “Stand with his withered hand.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And I put a jewel on thy forehead, and earrings in thine ears, and a beautiful crown upon thine head.',
  'I put earrings on thy forehead and a pretty crown Upon thy head.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Let Pharaoh do this, and let him appoint officers over the land, and take up the fifth part of the land of Egypt in the seven plenteous years.',
  'This should be done By Pharaoh, and in seven years appoint him Officers over land, and take over The fifth part of Egypt.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And he turned himself, and went out from Pharaoh.',
  'He turned himself and hath left Pharaoh.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And unleavened bread, and cakes unleavened tempered with oil, and wafers unleavened anointed with oil: of wheaten flour shalt thou make them.',
  'Thou mak’st leavened bread, cakes untempered with oil, Untempered wafers and coat’d with wax.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'But ye are come unto mount Sion, and unto the city of the living God, the heavenly Jerusalem, and to an innumerable company of angels,',
  'But thou art come from Mount Sinai and heavenly Jerusalem.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Wilt not thou, O God, which hadst cast us off?',
  'God cast us off?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And they came to a place which was named Gethsemane: and he saith to his disciples, Sit ye here, while I shall pray.',
  'He spake to his disciples, “Sit here while I pray.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And all the spoil of these cities, and the cattle, the children of Israel took for a prey unto themselves; but every man they smote with the edge of the sword, until they had destroyed them, neither left they any to breathe.',
  'They took all these cities and cattle as prey, But with swords every man slain Till they have destroyed them.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the second angel poured out his vial upon the sea; and it became as the blood of a dead man: and every living soul died in the sea.',
  'The second angel poured his vial Into the sea, and it became The blood of a dead man.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'And Pharaoh awoke, and, behold, it was a dream.',
  'Ay, and the Pharaoh wakes and dreams.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the firstborn said unto the younger, Our father is old, and there is not a man in the earth to come in unto us after the manner of all the earth:',
  "Our father was old, and man would not come o'er the earth."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And Joshua made him sharp knives, and circumcised the children of Israel at the hill of the foreskins.',
  'So Joshua made sharp knives of him, and circumcised the children of Israel.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Go not to glean in another field, neither go from hence, but abide here fast by my maidens:',
  'Go not to another field, but go here fast.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Day unto day uttereth speech, and night unto night sheweth knowledge.',
  'The day is speech, and the night shows knowledge.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'They take up all of them with the angle, they catch them in their net, and gather them in their drag: therefore they rejoice and are glad.',
  'They take them all by angle, Catch them in the net, and gather them in the drag.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'A man of great wrath shall suffer punishment: for if thou deliver him, yet thou must do it again.',
  'If a great wrath be delivered, a great wrath suffers punishment, though he must do it again, and so must he.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'There failed not ought of any good thing which the LORD had spoken unto the house of Israel; all came to pass.',
  'What you have said to the Israeli house, Lord, you have none.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'So that a man shall say, Verily there is a reward for the righteous: verily he is a God that judgeth in the earth.',
  'Therefore men shall say the right is verily rewarded.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Then shalt thou say, O LORD, thou hast spoken against this place, to cut it off, that none shall remain in it, neither man nor beast, but that it shall be desolate for ever.',
  'Then say, my lord, he hath cut it off, And that man and beast shall not remain in it, And be desolate for ever.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Yea, they have chosen their own ways, and their soul delighteth in their abominations.',
  'They have chosen their ways, and their abominables delight them.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'Little children, yet a little while I am with you.',
  'Yet for a while I’ll be with you, you little ones.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  "Thus saith the Lord GOD; If the prince give a gift unto any of his sons, the inheritance thereof shall be his sons'; it shall be their possession by inheritance.",
  'If a prince’s son give his gift to any prince’s son, his son shall be heir to the thing that is his son’s estate.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'And God helped him against the Philistines, and against the Arabians that dwelt in Gurbaal, and the Mehunims.',
  'God help thee in Urbaal Against the Philippians and the Mehunim.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Thou shalt sanctify him therefore; for he offereth the bread of thy God: he shall be holy unto thee: for I the LORD, which sanctify you, am holy.',
  'He that offers God’s bread shall sanctify him.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Therefore the LORD was very angry with Israel, and removed them out of his sight: there was none left but the tribe of Judah only.',
  'So God hath very wrath at Israel and removed ’t from his sight!'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Their slain also shall be cast out, and their stink shall come up out of their carcases, and the mountains shall be melted with their blood.',
  'Besides, they are dead, and their stinking comes out of their carcasses.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'Who, having received such a charge, thrust them into the inner prison, and made their feet fast in the stocks.',
  'They thrust their feet into an inner prison and made fast their legs, Receiving such a charge.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But those mine enemies, which would not that I should reign over them, bring hither, and slay them before me.',
  'But for mine own part, I would not kill mine enemies.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Although thou sayest thou shalt not see him, yet judgment is before him; therefore trust thou in him.',
  'Though thou say’st thou wouldst not see him, The judge is before him, and therefore thou shouldst trust him.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'For he that is not against us is on our part.',
  'He is not against us.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'For the LORD shall judge his people, and repent himself for his servants, when he seeth that their power is gone, and there is none shut up, or left.',
  'When that the power of their lords is gone, And they are not shut up or left out, Then God judge their person and repent their servants.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'From that time forth came they no more on the sabbath.',
  'They’ll be no longer on sabbath.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'I will arise and go to my father, and will say unto him, Father, I have sinned against heaven, and before thee,',
  'I have risen and gone to my father, To say I have singed heaven and to be damned.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Repent ye therefore, and be converted, that your sins may be blotted out, when the times of refreshing shall come from the presence of the Lord.',
  'Repent thy sins, and be converted, That thy sins may be blotted in a refresh.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Men do therefore fear him: he respecteth not any that are wise of heart.',
  'Men fear him, lest he respect any wise heart.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'And I, brethren, could not speak unto you as unto spiritual, but as unto carnal, even as unto babes in Christ.',
  'I cannot speak you spiritually, but I can speak carnal, Even as a baby in Christ.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'And as they did eat, he said, Verily I say unto you, that one of you shall betray me.',
  'He said that while they did eat, one of you did betray him.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Ye are our epistle written in our hearts, known and read of all men:',
  'Thou hast writ down our own epistles that we have known and read.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'And Chesed, and Hazo, and Pildash, and Jidlaph, and Bethuel.',
  'Chesed, Hazo, Pillash, and Jidlaph!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And Judah did evil in the sight of the LORD, and they provoked him to jealousy with their sins which they had committed, above all that their fathers had done.',
  'Judah did an evil, and provoked his father To jealousy, which his sins were above all done.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Wherefore, if God so clothe the grass of the field, which to day is, and to morrow is cast into the oven, shall he not much more clothe you, O ye of little faith?',
  'If God do not clothe you more, doth he not?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And in all that mighty hand, and in all the great terror which Moses shewed in the sight of all Israel.',
  'For all the world, And all the great terror that Moses hath shown, He hath shown Israel.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'But his delight is in the law of the LORD; and in his law doth he meditate day and night.',
  'But he hath meditated on his law the day, and he hath slept the night.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Wherefore do the wicked live, become old, yea, are mighty in power?',
  'Where dwells the evil, grows old, and is potent?'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'O thou king, the most high God gave Nebuchadnezzar thy father a kingdom, and majesty, and glory, and honour:',
  'God, his highest sovereign, Gave his father Nebuchadnezzar a kingdom, majesty, glory, and honor.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'When he therefore was come up again, and had broken bread, and eaten, and talked a long while, even till break of day, so he departed.',
  'Even till the day he left the house, When he had broken bread, eaten it, and talked long while.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Now Joshua was clothed with filthy garments, and stood before the angel.',
  'Joshua was clad in filth, and stood before an angel.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'That they were graven with an iron pen and lead in the rock for ever!',
  'They shall be graved with an iron pen and lead upon the rock forever.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'I sent you to reap that whereon ye bestowed no labour: other men laboured, and ye are entered into their labours.',
  'I sent you for work, That other men would work, and you would get his.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And as for me, thou upholdest me in mine integrity, and settest me before thy face for ever.',
  'In respect of me, thou uphold’st my integrity And putst me before thy face For ever.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'I will abide in thy tabernacle for ever: I will trust in the covert of thy wings.',
  'I’ll trust your wings to cover it.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Nebuzaradan captain of the guard took these, and brought them to the king of Babylon to Riblah:',
  'Tis true, the Nebuzaradan captain took them from Riblah, And from Riblah their captains.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Therefore am I troubled at his presence: when I consider, I am afraid of him.',
  'Therefore his presence worries me.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And the other issued out of the city against them; so they were in the midst of Israel, some on this side, and some on that side: and they smote them, so that they let none of them remain or escape.',
  'Since they were in Israel and had slain some men on this side, They let none remain or escape.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And I will bring again the captivity of my people of Israel, and they shall build the waste cities, and inhabit them; and they shall plant vineyards, and drink the wine thereof; they shall also make gardens, and eat the fruit of them.',
  'They’ll build waste cities and inhabit them, Plant vineyards and drink wine.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And they brake down the image of Baal, and brake down the house of Baal, and made it a draught house unto this day.',
  'Baal’s image they brake down.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'this is nothing else but sorrow of heart.',
  'This is but sorrow.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And whatsoever soul it be that doeth any work in that same day, the same soul will I destroy from among his people.',
  'I will destroy any soul that may do any office in the same day.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'He that spared not his own Son, but delivered him up for us all, how shall he not with him also freely give us all things?',
  'He spared not his son, But he delivered him to all of us, And how freely did he give us all That we had hoped for.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  "And he said, Hearken ye, all Judah, and ye inhabitants of Jerusalem, and thou king Jehoshaphat, Thus saith the LORD unto you, Be not afraid nor dismayed by reason of this great multitude; for the battle is not yours, but God's.",
  'Be not afraid, Judah, Be dismayed by the King of Jerusalem, Jehoshaphat.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And from Heshbon unto Ramathmizpeh, and Betonim; and from Mahanaim unto the border of Debir;',
  'From Heshbon to Ramathmizpeh and Betonim, And from Mahinaim to Debir.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And for the east side eastward fifty cubits.',
  'The east is fifty thousand cubic meters.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Who serve unto the example and shadow of heavenly things, as Moses was admonished of God when he was about to make the tabernacle: for, See, saith he, that thou make all things according to the pattern shewed to thee in the mount.',
  'Who serves as example and shadow, As if Poseidon were admonished to God As he about to make a tabernacle?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And he was sad at that saying, and went away grieved: for he had great possessions.',
  'That he was sad to say, And went away grievedly.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'The hands of Zerubbabel have laid the foundation of this house; his hands shall also finish it; and thou shalt know that the LORD of hosts hath sent me unto you.',
  "Zerubbabel's hands have laid the foundation; Their hands will finish it also; And, in the end, the whole thing is made of sand."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And by the border of Dan, from the east side unto the west side, a portion for Asher.',
  'The border of Dane with the West Bank.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And if a woman shall put away her husband, and be married to another, she committeth adultery.',
  'A woman commits adultery if she leave her husband And marry with another.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And they possessed all the coasts of the Amorites, from Arnon even unto Jabbok, and from the wilderness even unto Jordan.',
  'They are encamped in all the coasts of the empire, Of Arnon alone, and even to Jabbok.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'for they wash not their hands when they eat bread.',
  'They wash not their hands when they eat bread.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the suburbs of the city shall be toward the north two hundred and fifty, and toward the south two hundred and fifty, and toward the east two hundred and fifty, and toward the west two hundred and fifty.',
  'There are suburbs in the city, 250 north, south, and east.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And for thy cattle, and for the beast that are in thy land, shall all the increase thereof be meat.',
  'The increase in meat is for your cattle, and for the beasts on your land.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'So I prophesied as I was commanded: and as I prophesied, there was a noise, and behold a shaking, and the bones came together, bone to his bone.',
  "I prophesied like myself, and there was shake, and bones came o'er his bones."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And Jacob went out from Beersheba, and went toward Haran.',
  'Jacob went from Beersheba.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'For the multitude of the people followed after, crying, Away with him.',
  'The crying throng hath followed him.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'The woman also with whom man shall lie with seed of copulation, they shall both bathe themselves in water, and be unclean until the even.',
  'A woman that lies a man in copulation seed Shall bathe her in water, and till she be old she will not be clean.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'So Joab the son of Zeruiah went first up, and was chief.',
  'Joab went up first, and is now chief.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'Ye that fear the LORD, trust in the LORD: he is their help and their shield.',
  'Lord help thee and shield thee!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And he called unto him the twelve, and began to send them forth by two and two; and gave them power over unclean spirits;',
  'He called the twelve and began to send them forth, And gave them power of unclean spirits.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'For thou shalt be in league with the stones of the field: and the beasts of the field shall be at peace with thee.',
  'Thou art in league with the fields’ stones.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'So there was great joy in Jerusalem: for since the time of Solomon the son of David king of Israel there was not the like in Jerusalem.',
  'There’s great joy in Jerusalem since Salomon Was son to David, the king of Israel.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'for this man doeth many miracles.',
  'This man hath done many miracles.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Teach me thy way, O LORD, and lead me in a plain path, because of mine enemies.',
  'Teach me your way, and lead me On a clear path, lest mine enemies take the lead.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'When the morning stars sang together, and all the sons of God shouted for joy?',
  'When the stars of morn sang together?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Therefore the Jews of the villages, that dwelt in the unwalled towns, made the fourteenth day of the month Adar a day of gladness and feasting, and a good day, and of sending portions one to another.',
  'The Jew hath made the fourteenth day of Adar, A day of gladness and feast.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Therefore every one that eateth it shall bear his iniquity, because he hath profaned the hallowed thing of the LORD: and that soul shall be cut off from among his people.',
  'So shall every one that eats it profess His hallowed thing to bear his sin.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Pass through the host, and command the people, saying, Prepare you victuals; for within three days ye shall pass over this Jordan, to go in to possess the land, which the LORD your God giveth you to possess it.',
  'Pass you to Jordan, and tell yourself, Within these three days, if you have left Israel, Prepare to conquest.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  "Then thou shalt say, They be thy servant Jacob's; it is a present sent unto my lord Esau: and, behold, also he is behind us.",
  'Say that they were Jacob, your servant; The present was sent to your lord Esau.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'Even so, Amen.',
  'Yet amen.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'That we have built us an altar to turn from following the LORD, or if to offer thereon burnt offering or meat offering, or if to offer peace offerings thereon, let the LORD himself require it;',
  'We have built an altar to turn to follow God, or if we dare offer Burnt or meat, or offer peace there, Then let us go.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'My bowels, my bowels!',
  'My bowels!'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And a mitre of fine linen, and goodly bonnets of fine linen, and linen breeches of fine twined linen,',
  'Fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine linen, and fine'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'But tidings out of the east and out of the north shall trouble him: therefore he shall go forth with great fury to destroy, and utterly to make away many.',
  'But the news of the east and north doth trouble him, And so he goes out, with great fury, to destroy many.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'They also that seek after my life lay snares for me: and they that seek my hurt speak mischievous things, and imagine deceits all the day long.',
  'They seek out my hurt also, They speak mischievous things, They imagine deceitful things all day.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incomplete',
  'but turn thee yet again, and thou shalt see greater abominations.',
  'But if thou turn’st yet again, thou shalt see greater abominables.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'No Error',
  'Pilate saith unto him, What is truth?',
  'What is true?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And they worshipped the dragon which gave power unto the beast: and they worshipped the beast, saying, Who is like unto the beast?',
  'They worshiped the dragon, who gave power to a beast.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Thou shalt not eat it; that it may go well with thee, and with thy children after thee, when thou shalt do that which is right in the sight of the LORD.',
  'Thou shalt not eat it, That it may go well with thyself and thy children after.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And Serug lived after he begat Nahor two hundred years, and begat sons and daughters.',
  'Serug lived after her two hundred years of marriage to Nahor.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'I love the LORD, because he hath heard my voice and my supplications.',
  'I love the Lord, For he hath heard my voice and what I suggest.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'But when the people of the land shall come before the LORD in the solemn feasts, he that entereth in by the way of the north gate to worship shall go out by the way of the south gate; and he that entereth by the way of the south gate shall go forth by the way of the north gate: he shall not return by the way of the gate whereby he came in, but shall go forth over against it.',
  'When the Romans come to solemn feasts, Those that enter at the north gate for worship Shall not go to the south gate, but go over it.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And consulted that they might take Jesus by subtilty, and kill him.',
  "He hath consult'd That they may take Jesu with subtilty and kill him."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'In the twilight, in the evening, in the black and dark night:',
  'O black and dark night!'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Judge not, that ye be not judged.',
  'Judge not.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'Lift up your heads, O ye gates; and be ye lift up, ye everlasting doors; and the King of glory shall come in.',
  'Lift thy head; the King welcome.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incomplete',
  'He disappointeth the devices of the crafty, so that their hands cannot perform their enterprise.',
  'He does disappoint the crafty, that he cannot perform his office.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'but he that cometh after me is mightier than I, whose shoes I am not worthy to bear: he shall baptize you with the Holy Ghost, and with fire:',
  'He that comes after me, though with no shoe of mine, is stronger than myself.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'Blessed be the God and Father of our Lord Jesus Christ, who hath blessed us with all spiritual blessings in heavenly places in Christ:',
  'God and our father, Jesus Christ, Bless us in heaven!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And how I kept back nothing that was profitable unto you, but have shewed you, and have taught you publickly, and from house to house,',
  "But what I have kept from you back is nothing profitable: I'll make thee show, and teach thee publicly from the house to the house."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Arabia, and all the princes of Kedar, they occupied with thee in lambs, and rams, and goats: in these were they thy merchants.',
  'They occupied Kent with lambs, rams, and goats.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  "And the soldiers' counsel was to kill the prisoners, lest any of them should swim out, and escape.",
  'Soldiers give counsel To kill prisoners, lest any of them swim out and escape.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the second lot came forth to Simeon, even for the tribe of the children of Simeon according to their families: and their inheritance was within the inheritance of the children of Judah.',
  'Even sir Simeon’s second lot is in Judah’s blood.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'wherefore camest thou not unto me?',
  'Where art thou?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Behold, for peace I had great bitterness: but thou hast in love to my soul delivered it from the pit of corruption: for thou hast cast all my sins behind thy back.',
  'I am great bitter, but thou lovest me so, That thou throwst all my sins behind thy back.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  "And shall put thereon the covering of badgers' skins, and shall spread over it a cloth wholly of blue, and shall put in the staves thereof.",
  'For the badgers themselves, they cover their skins, and there they spread A complete cloth of blue.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Then Benhadad came forth to him; and he caused him to come up into the chariot.',
  'Why, then Benedad came to him; and therefore came to fetch him to the carriages.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'All that cometh is vanity.',
  'All that is vanity is to be a knave.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "And whatsoever more shall be needful for the house of thy God, which thou shalt have occasion to bestow, bestow it out of the king's treasure house.",
  'And therein need any more, To bestow a house of treasure of the king.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Be it known unto the king, that the Jews which came up from thee to us are come unto Jerusalem, building the rebellious and the bad city, and have set up the walls thereof, and joined the foundations.',
  'I have known the Jew came from Jerusalem, Built a bad, rebellious city, and joined with foundations.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  "Moreover concerning the stranger, which is not of thy people Israel, but is come from a far country for thy great name's sake, and thy mighty hand, and thy stretched out arm; if they come and pray in this house;",
  'Be it so with a stranger come from a far country, Your great name and your stretched arm, But not as an Israeli.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Shall the thing formed say to him that formed it, Why hast thou made me thus?',
  'Why then, thou art formed for ’t.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And they tied unto it a lace of blue, to fasten it on high upon the mitre; as the LORD commanded Moses.',
  'They tied the mitre to blue lace, Which on the order of Moses did fasten them.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Wherefore, behold, I send unto you prophets, and wise men, and scribes: and some of them ye shall kill and crucify; and some of them shall ye scourge in your synagogues, and persecute them from city to city:',
  'Therefore I send Some prophets, wise men, and writers, That you will kill and crucify them.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'So Zedekiah the king sware secretly unto Jeremiah, saying, As the LORD liveth, that made us this soul, I will not put thee to death, neither will I give thee into the hand of these men that seek thy life.',
  'The king, secretly, Zedekiah, told Joseph thou wilt neither die nor die By the Lord’s life that made this soul.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  "And the LORD plagued Pharaoh and his house with great plagues because of Sarai Abram's wife.",
  'For Sarai Abram’s wife, It was a great plague upon the Pharaoh and his house.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'Why dost thou strive against him?',
  'Why dost thou try thy opposition against him?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'For a certain woman, whose young daughter had an unclean spirit, heard of him, and came and fell at his feet:',
  'He hath been heard of by a young woman’s daughter; she came and fell upon his feet.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incomplete',
  'And ye murmured in your tents, and said, Because the LORD hated us, he hath brought us forth out of the land of Egypt, to deliver us into the hand of the Amorites, to destroy us.',
  'Thou hast murmured in thy tent And said that because God hated us, He brought us out of Egypt to destroy us.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'He shutteth his eyes to devise froward things: moving his lips he bringeth evil to pass.',
  'He shuts his eyes and lips, Moving so the cause of evil.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'No Error',
  'Go therefore now, and work; for there shall no straw be given you, yet shall ye deliver the tale of bricks.',
  'Go to work now, and there will be no straw given thee, But deliver the story of bricks.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'So Nebuzaradan the captain of the guard took them, and brought them to the king of Babylon to Riblah.',
  'Tis true, guardsman Nebuzaradan took them from Riblah.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  "Every man of the children of Israel shall pitch by his own standard, with the ensign of their father's house: far off about the tabernacle of the congregation shall they pitch.",
  'Near the far off tabernacle, every one doth pitch in his standard.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Howl, ye ships of Tarshish; for it is laid waste, so that there is no house, no entering in: from the land of Chittim it is revealed to them.',
  "Whip, ye Tartarists, For if it lay to waste there's no house nor entrance."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'But ye say, If a man shall say to his father or mother, It is Corban, that is to say, a gift, by whatsoever thou mightest be profited by me; he shall be free.',
  'If thou say’st “father” or “mother,” Cordan is free.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And again, whom should I serve?',
  'What should I serve again?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Now if thou commit no adultery, yet if thou kill, thou art become a transgressor of the law.',
  'If thou commit no adultery, Become a traitor to the state, and the state shall punish the violator.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And he said, I will make all my goodness pass before thee, and I will proclaim the name of the LORD before thee; and will be gracious to whom I will be gracious, and will shew mercy on whom I will shew mercy.',
  'I’ll make all my goodness before thee, And proclaim my name as a gracious man.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'How beautiful upon the mountains are the feet of him that bringeth good tidings, that publisheth peace; that bringeth good tidings of good, that publisheth salvation; that saith unto Zion, Thy God reigneth!',
  'What a beauty is there in the mountains; He brings good news, publishes peace, and says your God reigns.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'For she did not know that I gave her corn, and wine, and oil, and multiplied her silver and gold, which they prepared for Baal.',
  'Nor did she know That I gave her corn, wine, and oil, And that I multiplied the silver and gold They prepared for Baal.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he sent him away to his house, saying, Neither go into the town, nor tell it to any in the town.',
  'He said he would not go to town and would not tell anyone of it.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  'And the children of Heth answered Abraham, saying unto him,',
  'Abraham answered my children.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And these are they by the way side, where the word is sown; but when they have heard, Satan cometh immediately, and taketh away the word that was sown in their hearts.',
  'They are on the way, but when they have heard Satan come, he will immediately take away the word That is seeded in their hearts.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'They shall be holy unto their God, and not profane the name of their God: for the offerings of the LORD made by fire, and the bread of their God, they do offer: therefore they shall be holy.',
  'They are holy to God’s, and will not profane themselves.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And take your father and your households, and come unto me: and I will give you the good of the land of Egypt, and ye shall eat the fat of the land.',
  'Take from you your father and your household, Come to me and I will give you the fat of Egypt.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Blessed is the man that heareth me, watching daily at my gates, waiting at the posts of my doors.',
  'Bless me a man that every day watches my gates And waits on my posts.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And the prince of the tribe of the children of Asher, Ahihud the son of Shelomi.',
  'Ahihud!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And his lord was wroth, and delivered him to the tormentors, till he should pay all that was due unto him.',
  'His lord is angry, and he delivers him To a tormenting torturer, till he pay all he is due.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  "With whomsoever of thy servants it be found, both let him die, and we also will be my lord's bondmen.",
  'Let him die, my lord, And our bond to him also.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'For which of you, intending to build a tower, sitteth not down first, and counteth the cost, whether he have sufficient to finish it?',
  'Who of you amongst us First wishing to build a tower, Count the cost and know whether he has enough to finish it?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Thus ye shall be filled at my table with horses and chariots, with mighty men, and with all men of war, saith the Lord GOD.',
  "God be wi' you, my table is full of horses, chariots, mighty men, and all!"],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Let the day perish wherein I was born, and the night in which it was said, There is a man child conceived.',
  'Let the day wherein I was born And the night wherein the man was said to be dead Let him rest his soul.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'The LORD hath loved him: he will do his pleasure on Babylon, and his arm shall be on the Chaldeans.',
  'God lieb’st babylon, and his arm is in the Chaldean gods.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'For now thou numberest my steps: dost thou not watch over my sin?',
  "Now are you number'd in my steps; dost thou not watch over my sin?"],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'for my soul is wearied because of murderers.',
  'The murderers do my soul weary.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  "And she had a sister called Mary, which also sat at Jesus' feet, and heard his word.",
  'She was Mary’s sister, who listened to the word of Jesus also.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And the Tirshatha said unto them, that they should not eat of the most holy things, till there stood up a priest with Urim and with Thummim.',
  'Tirshatha said they would not eat the most holy till the priests, Urim and Thumbim, stood together.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The trees of the LORD are full of sap; the cedars of Lebanon, which he hath planted;',
  'He hath planted cedar trees in Lebanon.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'Shuppim also, and Huppim, the children of Ir, and Hushim, the sons of Aher.',
  'Upim and Hush!'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  "And David said unto Abiathar, I knew it that day, when Doeg the Edomite was there, that he would surely tell Saul: I have occasioned the death of all the persons of thy father's house.",
  'That day, when Doeg the Edomite was there, David knew he had told Salvation that I was dead.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Howbeit he meaneth not so, neither doth his heart think so; but it is in his heart to destroy and cut off nations not a few.',
  'He thinks not so, but his purpose is to destroy nations and cut them off.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And the sabbath of the land shall be meat for you; for thee, and for thy servant, and for thy maid, and for thy hired servant, and for thy stranger that sojourneth with thee.',
  'There’s meat for you, for your servant, for your maid, for stranger that you have hired.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'While the Pharisees were gathered together, Jesus asked them,',
  "When the Pharisees were gather'd, Jesu asked the Pharisees what they were."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'He that hath received his testimony hath set to his seal that God is true.',
  'He’ll put a seal upon him That God’s trueness is in him.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And Reuben spake unto his father, saying, Slay my two sons, if I bring him not to thee: deliver him into my hand, and I will bring him to thee again.',
  'Reuben, if I bring not thy two sons, Slaying them both!'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'They were amazed, they answered no more: they left off speaking.',
  'They were amazed, they answered not, they left off their speech.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'I have longed for thy salvation, O LORD; and thy law is my delight.',
  'I have long for your salvation; And your law takes delight in me.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  "And she answered and said unto him, Yes, Lord: yet the dogs under the table eat of the children's crumbs.",
  'Yet the dogs under the table Eat children’s crumbs.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Salvation is far from the wicked: for they seek not thy statutes.',
  'Bad men seek not your laws to help.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'The children of Ater of Hezekiah, ninety and eight.',
  'O, ’tis ninety-five.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he left off talking with him, and God went up from Abraham.',
  'He left talking, and God went with him to Abraham.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And when Saul looked behind him, David stooped with his face to the earth, and bowed himself.',
  'When David looked behind him, he stooped in his face and bowed.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Then Nebuzaradan the captain of the guard carried away captive certain of the poor of the people, and the residue of the people that remained in the city, and those that fell away, that fell to the king of Babylon, and the rest of the multitude.',
  'The guardsman Nebuzaradan Carry away some poor men captured, And the rest that remain in the city.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'For I have not shunned to declare unto you all the counsel of God.',
  'I would not be so curst To tell you all the counsels of God.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Grudge not one against another, brethren, lest ye be condemned: behold, the judge standeth before the door.',
  "Grudge not one against another, lest thou be condemn'd."],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Jesus therefore, knowing all things that should come upon him, went forth, and said unto them, Whom seek ye?',
  'So went Jesu out, knowing all, and he said to them Who seeks thee?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'To overthrow their seed also among the nations, and to scatter them in the lands.',
  'To overthrow their seeds among nations and scatter them thus.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'But that on the good ground are they, which in an honest and good heart, having heard the word, keep it, and bring forth fruit with patience.',
  'But on good ground they keep their ears and produce fruit With patience.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Is not this written in the book of Jasher?',
  'Was not this writ in Jasher?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'No Error',
  'And the people with one accord gave heed unto those things which Philip spake, hearing and seeing the miracles which he did.',
  'Men shall hear Philip’s words, And behold what miracle he did, Hearing and seeing what miracle he did.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incomplete',
  'And when Samuel had caused all the tribes of Israel to come near, the tribe of Benjamin was taken.',
  'When he came all near Israel, Samuel took Benjamin.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Meaning Change',
  'There are not found that returned to give glory to God, save this stranger.',
  'No man found back But this stranger, to give God glory.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'And there was a cloud that overshadowed them: and a voice came out of the cloud, saying, This is my beloved Son: hear him.',
  'The cloud hath overshadowed them, And came out a voice saying “This is their loving son.” Why, that’s the man.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'the LORD is the strength of my life; of whom shall I be afraid?',
  'My life is strong; what fear I?'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And in their hands they shall bear thee up, lest at any time thou dash thy foot against a stone.',
  'They are at your feet, and therefore at any time you’ll dash your foot with stones.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And, behold, men passed by, and saw the carcase cast in the way, and the lion standing by the carcase: and they came and told it in the city where the old prophet dwelt.',
  'The men passed the carcass, and saw the lion standing by, And came thither to the city where old Prosper lived.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'In the first place went the standard of the camp of the children of Judah according to their armies: and over his host was Nahshon the son of Amminadab.',
  "The camp was the standard For the Judah's army in first place, and Nahshon's host."],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'A man that flattereth his neighbour spreadeth a net for his feet.',
  'A man that flatters his neighbor spreads a net upon his feet.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And he said unto them, What manner of communications are these that ye have one to another, as ye walk, and are sad?',
  'How wouldst thou have communication with another, When thou dost walk and be sad?'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'No Error',
  'And all the men of Shechem gathered together, and all the house of Millo, and went, and made Abimelech king, by the plain of the pillar that was in Shechem.',
  'All the gods at Shechem gathered, And all the gods at Millo went To make Abimelech king.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And Abner said unto David, I will arise and go, and will gather all Israel unto my lord the king, that they may make a league with thee, and that thou mayest reign over all that thine heart desireth.',
  'Aber said he would rise and go And gather all the people of Israel, that thou mightst make a league with thee And mayst rule all that thy desire shall his heart desire.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'God layeth up his iniquity for his children: he rewardeth him, and he shall know it.',
  'God lays his iniquity on his children, and he rewards them.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  "Ye have seen what I did unto the Egyptians, and how I bare you on eagles' wings, and brought you unto myself.",
  'You have seen what I have done to the Egyptians And how I bare thee in the wings of eagles.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'They shall have like portions to eat, beside that which cometh of the sale of his patrimony.',
  'They’ll have, to eat, a portion like himself, Save that which comes to market his wares.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'Is not my word like as a fire?',
  'My word is like fire?'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'And he made the staves of shittim wood, and overlaid them with gold.',
  'He made the staves of shittim wood and overlaid them with gold.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'And Benaiah brought the king word again, saying, Thus said Joab, and thus he answered me.',
  'Joab says again “Ben” is his word for the king.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'And Moses gave the money of them that were redeemed unto Aaron and to his sons, according to the word of the LORD, as the LORD commanded Moses.',
  'The duke of Moor hath given money to Aaron and his sons.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And I brought you into the land of the Amorites, which dwelt on the other side Jordan; and they fought with you: and I gave them into your hand, that ye might possess their land; and I destroyed them from before you.',
  'I brought thee from the other side An Amorites that lived on the other side of Jordan And fought with you.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And Samuel said to all the people, See ye him whom the LORD hath chosen, that there is none like him among all the people?',
  'Saw’st thou men that are not like Samuel?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'And when he humbled himself, the wrath of the LORD turned from him, that he would not destroy him altogether: and also in Judah things went well.',
  'When he humbled himself, his wrath Turned itself into nothing, and things in Judah went on as well as upon him.'],
 ['bible_shakespeare.tsv',
  'Incorrect/New Information',
  'Incorrect/New Information',
  'For I determined not to know any thing among you, save Jesus Christ, and him crucified.',
  'I have resolved Not to know of him, but Jesus Christ and his crucifixion.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incomplete',
  "While he yet spake, there cometh one from the ruler of the synagogue's house, saying to him, Thy daughter is dead; trouble not the Master.",
  'When he speaks still, there comes one that says your daughter is dead, And that synagogue masters should not trouble him.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'or who hath been his counsellor?',
  'Or who is he that counsels?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'That which I speak, I speak it not after the Lord, but as it were foolishly, in this confidence of boasting.',
  'I will not speak that out of thinking it foolish.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'Then the congregation shall judge between the slayer and the revenger of blood according to these judgments:',
  'The congregation shall judge Between the slain and the revenged, According to this decree.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'And the princes of the Philistines were wroth with him; and the princes of the Philistines said unto him, Make this fellow return, that he may go again to his place which thou hast appointed him, and let him not go down with us to battle, lest in the battle he be an adversary to us: for wherewith should he reconcile himself unto his master?',
  'Where should he reconcile himself with his master?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'And Jacob lifted up his eyes, and looked, and, behold, Esau came, and with him four hundred men.',
  'Jacob lifted his eyes And looked to him, and there came Esau.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Incorrect/New Information',
  'For all tables are full of vomit and filthiness, so that there is no place clean.',
  'All the tables are full of vomit and filth, And therefore are they washed.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'I will be surety for him; of my hand shalt thou require him: if I bring him not unto thee, and set him before thee, then let me bear the blame for ever:',
  "I am sure of him; if I bring him not to thee and put him not before thee, I'll lay the blame on him forever."],
 ['bible_shakespeare.tsv',
  'No Error',
  'Meaning Change',
  'And the men did so; and took two milch kine, and tied them to the cart, and shut up their calves at home:',
  'The men took two milch kines from the cart, tied them in a cart, shut up their calves at home.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incomplete',
  'Turn us again, O God of hosts, and cause thy face to shine; and we shall be saved.',
  'Turn us again, shine thy face, and we shall be saved.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'Is any among you afflicted?',
  'Hast any of you affected?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Jesus said, Take ye away the stone.',
  'Take up the stones.'],
 ['bible_shakespeare.tsv',
  'Meaning Change',
  'Meaning Change',
  'And the altar of burnt offering with all his furniture, and the laver and his foot,',
  'There is an altar of burned offerings, and all his furniture, For which his foot is the sole of contention.'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Meaning Change',
  'Do we provoke the Lord to jealousy?',
  'Provoke we jealousy?'],
 ['bible_shakespeare.tsv',
  'Incomplete',
  'Incorrect/New Information',
  'Righteous art thou, O LORD, and upright are thy judgments.',
  'Thou art right and upright.'],
 ['bible_shakespeare.tsv',
  'No Error',
  'Incorrect/New Information',
  'Let those that fear thee turn unto me, and those that have known thy testimonies.',
  'O, turn to me, those that fear thee, and they shall know What thou testifies.'],
 ...]

In [163]: x[0]
Out[163]: ['direction', 'Tstar_Error', 'Strap_Error', '{Input} Text', '{Output} Text']

In [164]: tstar_error_dict = {}

In [165]: import collections

In [166]: strap_error_dict = {}

In [167]: for row in x:
     ...:     if row[0] not in tstar_error_dict:
     ...:         tstar_error_dict[row[0]] = [row[1]]
     ...:     else:
     ...:         tstar_error_dict[row[0]].append(row[1])
     ...: 

In [168]: for i in tstar_error_dict:
     ...:     collections.Counter(tstar_error_dict[i])
     ...: 

In [169]: for i in tstar_error_dict:
     ...:     print(collections.Counter(tstar_error_dict[i]))
     ...: 
     ...: 
Counter({'Tstar_Error': 1})
Counter({'Incomplete': 270, 'Meaning Change': 119, 'Incorrect/New Information': 68, 'No Error': 43})
Counter({'Incomplete': 190, 'Meaning Change': 162, 'Incorrect/New Information': 76, 'No Error': 72})
Counter({'Incomplete': 189, 'Meaning Change': 148, 'No Error': 98, 'Incorrect/New Information': 65})
Counter({'Incorrect/New Information': 232, 'Meaning Change': 156, 'No Error': 85, 'Incomplete': 27})
Counter({'Meaning Change': 224, 'No Error': 134, 'Incorrect/New Information': 89, 'Incomplete': 53})
Counter({'Meaning Change': 213, 'No Error': 142, 'Incomplete': 82, 'Incorrect/New Information': 63})
Counter({'Incorrect/New Information': 203, 'Meaning Change': 185, 'No Error': 69, 'Incomplete': 43})
Counter({'Incorrect/New Information': 190, 'Meaning Change': 166, 'Incomplete': 89, 'No Error': 55})
Counter({'Meaning Change': 201, 'No Error': 132, 'Incomplete': 98, 'Incorrect/New Information': 69})
Counter({'Incorrect/New Information': 213, 'Meaning Change': 148, 'No Error': 85, 'Incomplete': 54})
Counter({'Incomplete': 165, 'Meaning Change': 124, 'Incorrect/New Information': 113, 'No Error': 98})
Counter({'Meaning Change': 177, 'No Error': 149, 'Incorrect/New Information': 87, 'Incomplete': 87})

In [170]: for i in tstar_error_dict:
     ...:     print(i, collections.Counter(tstar_error_dict[i]))
     ...: 
     ...: 
direction Counter({'Tstar_Error': 1})
bible_poetry.tsv Counter({'Incomplete': 270, 'Meaning Change': 119, 'Incorrect/New Information': 68, 'No Error': 43})
bible_shakespeare.tsv Counter({'Incomplete': 190, 'Meaning Change': 162, 'Incorrect/New Information': 76, 'No Error': 72})
bible_switchboard.tsv Counter({'Incomplete': 189, 'Meaning Change': 148, 'No Error': 98, 'Incorrect/New Information': 65})
poetry_bible.tsv Counter({'Incorrect/New Information': 232, 'Meaning Change': 156, 'No Error': 85, 'Incomplete': 27})
poetry_shakespeare.tsv Counter({'Meaning Change': 224, 'No Error': 134, 'Incorrect/New Information': 89, 'Incomplete': 53})
poetry_switchboard.tsv Counter({'Meaning Change': 213, 'No Error': 142, 'Incomplete': 82, 'Incorrect/New Information': 63})
shakespeare_bible.tsv Counter({'Incorrect/New Information': 203, 'Meaning Change': 185, 'No Error': 69, 'Incomplete': 43})
shakespeare_poetry.tsv Counter({'Incorrect/New Information': 190, 'Meaning Change': 166, 'Incomplete': 89, 'No Error': 55})
shakespeare_switchboard.tsv Counter({'Meaning Change': 201, 'No Error': 132, 'Incomplete': 98, 'Incorrect/New Information': 69})
switchboard_bible.tsv Counter({'Incorrect/New Information': 213, 'Meaning Change': 148, 'No Error': 85, 'Incomplete': 54})
switchboard_poetry.tsv Counter({'Incomplete': 165, 'Meaning Change': 124, 'Incorrect/New Information': 113, 'No Error': 98})
switchboard_shakespeare.tsv Counter({'Meaning Change': 177, 'No Error': 149, 'Incorrect/New Information': 87, 'Incomplete': 87})

In [171]: for row in x:
     ...:     if row[0] not in strap_error_dict:
     ...:         strap_error_dict[row[0]] = [row[1]]
     ...:     else:
     ...:         strap_error_dict[row[0]].append(row[1])
     ...: 

In [172]: for i in strap_error_dict:
     ...:     print(i, collections.Counter(strap_error_dict[i]))
     ...: 
     ...: 
     ...: 
direction Counter({'Tstar_Error': 1})
bible_poetry.tsv Counter({'Incomplete': 270, 'Meaning Change': 119, 'Incorrect/New Information': 68, 'No Error': 43})
bible_shakespeare.tsv Counter({'Incomplete': 190, 'Meaning Change': 162, 'Incorrect/New Information': 76, 'No Error': 72})
bible_switchboard.tsv Counter({'Incomplete': 189, 'Meaning Change': 148, 'No Error': 98, 'Incorrect/New Information': 65})
poetry_bible.tsv Counter({'Incorrect/New Information': 232, 'Meaning Change': 156, 'No Error': 85, 'Incomplete': 27})
poetry_shakespeare.tsv Counter({'Meaning Change': 224, 'No Error': 134, 'Incorrect/New Information': 89, 'Incomplete': 53})
poetry_switchboard.tsv Counter({'Meaning Change': 213, 'No Error': 142, 'Incomplete': 82, 'Incorrect/New Information': 63})
shakespeare_bible.tsv Counter({'Incorrect/New Information': 203, 'Meaning Change': 185, 'No Error': 69, 'Incomplete': 43})
shakespeare_poetry.tsv Counter({'Incorrect/New Information': 190, 'Meaning Change': 166, 'Incomplete': 89, 'No Error': 55})
shakespeare_switchboard.tsv Counter({'Meaning Change': 201, 'No Error': 132, 'Incomplete': 98, 'Incorrect/New Information': 69})
switchboard_bible.tsv Counter({'Incorrect/New Information': 213, 'Meaning Change': 148, 'No Error': 85, 'Incomplete': 54})
switchboard_poetry.tsv Counter({'Incomplete': 165, 'Meaning Change': 124, 'Incorrect/New Information': 113, 'No Error': 98})
switchboard_shakespeare.tsv Counter({'Meaning Change': 177, 'No Error': 149, 'Incorrect/New Information': 87, 'Incomplete': 87})

In [173]: strap_error_dict
     ...: for row in x:
     ...:     if row[0] not in strap_error_dict:
     ...:         strap_error_dict[row[0]] = [row[2]]
     ...:     else:
     ...:         strap_error_dict[row[0]].append(row[2])
     ...: 

In [174]: strap_error_dict={}
     ...: for row in x:
     ...:     if row[0] not in strap_error_dict:
     ...:         strap_error_dict[row[0]] = [row[2]]
     ...:     else:
     ...:         strap_error_dict[row[0]].append(row[2])
     ...: 

In [175]: for i in strap_error_dict:
     ...:     print(i, collections.Counter(strap_error_dict[i]))
     ...: 
     ...: 
     ...: 
direction Counter({'Strap_Error': 1})
bible_poetry.tsv Counter({'Incomplete': 239, 'Meaning Change': 121, 'Incorrect/New Information': 98, 'No Error': 42})
bible_shakespeare.tsv Counter({'Incorrect/New Information': 224, 'Meaning Change': 176, 'Incomplete': 55, 'No Error': 45})
bible_switchboard.tsv Counter({'Incorrect/New Information': 203, 'Meaning Change': 184, 'Incomplete': 59, 'No Error': 54})
poetry_bible.tsv Counter({'Incorrect/New Information': 257, 'Meaning Change': 175, 'No Error': 46, 'Incomplete': 22})
poetry_shakespeare.tsv Counter({'Incorrect/New Information': 224, 'Meaning Change': 183, 'Incomplete': 50, 'No Error': 43})
poetry_switchboard.tsv Counter({'Meaning Change': 186, 'Incorrect/New Information': 171, 'No Error': 80, 'Incomplete': 63})
shakespeare_bible.tsv Counter({'Incorrect/New Information': 253, 'Meaning Change': 184, 'No Error': 44, 'Incomplete': 19})
shakespeare_poetry.tsv Counter({'Meaning Change': 192, 'Incorrect/New Information': 187, 'Incomplete': 77, 'No Error': 44})
shakespeare_switchboard.tsv Counter({'Meaning Change': 237, 'Incorrect/New Information': 151, 'No Error': 70, 'Incomplete': 42})
switchboard_bible.tsv Counter({'Incorrect/New Information': 241, 'Meaning Change': 167, 'No Error': 50, 'Incomplete': 42})
switchboard_poetry.tsv Counter({'Incorrect/New Information': 165, 'Meaning Change': 146, 'Incomplete': 140, 'No Error': 49})
switchboard_shakespeare.tsv Counter({'Incorrect/New Information': 189, 'Meaning Change': 172, 'Incomplete': 77, 'No Error': 62})

In [176]: for i in strap_error_dict:
     ...:    c = collections.Counter(strap_error_dict[i])
     ...:    print ("{}\t{}\t{}\t{}\t{}\n".format(i, c["Incomplete"], c["Meaning Change"], c["Incorrect/New I
     ...: nformation"], c["No Error"]))
     ...: 
direction	0	0	0	0

bible_poetry.tsv	239	121	98	42

bible_shakespeare.tsv	55	176	224	45

bible_switchboard.tsv	59	184	203	54

poetry_bible.tsv	22	175	257	46

poetry_shakespeare.tsv	50	183	224	43

poetry_switchboard.tsv	63	186	171	80

shakespeare_bible.tsv	19	184	253	44

shakespeare_poetry.tsv	77	192	187	44

shakespeare_switchboard.tsv	42	237	151	70

switchboard_bible.tsv	42	167	241	50

switchboard_poetry.tsv	140	146	165	49

switchboard_shakespeare.tsv	77	172	189	62


In [177]: for i in tstar_error_dict:
     ...:    c = collections.Counter(tstar_error_dict[i])
     ...:    print ("{}\t{}\t{}\t{}\t{}".format(i, c["Incomplete"], c["Meaning Change"], c["Incorrect/New Inf
     ...: ormation"], c["No Error"]))
     ...: 
direction	0	0	0	0
bible_poetry.tsv	270	119	68	43
bible_shakespeare.tsv	190	162	76	72
bible_switchboard.tsv	189	148	65	98
poetry_bible.tsv	27	156	232	85
poetry_shakespeare.tsv	53	224	89	134
poetry_switchboard.tsv	82	213	63	142
shakespeare_bible.tsv	43	185	203	69
shakespeare_poetry.tsv	89	166	190	55
shakespeare_switchboard.tsv	98	201	69	132
switchboard_bible.tsv	54	148	213	85
switchboard_poetry.tsv	165	124	113	98
switchboard_shakespeare.tsv	87	177	87	149

In [178]: cd /Users/preksh/Downloads/QQP\ 2
/Users/preksh/Downloads/QQP 2

In [179]: ls
qqp/         qqp_dataset/

In [180]: cd qqp_dataset/
/Users/preksh/Downloads/QQP 2/qqp_dataset

In [181]: ls
score.txt   sent1.docx  sent1.txt   sent2.docx  sent2.txt

In [182]: cd ../
/Users/preksh/Downloads/QQP 2

In [183]: ls
qqp/         qqp_dataset/

In [184]: cd qqpls
[Errno 2] No such file or directory: 'qqpls'
/Users/preksh/Downloads/QQP 2

In [185]: cd qqp
/Users/preksh/Downloads/QQP 2/qqp

In [186]: ls
amr1.txt    amr2.txt    sent1.txt   sent2.txt   smatch.txt

In [187]: ls
amr1.txt    amr2.txt    sent1.txt   sent2.txt   smatch.txt

In [188]: cd ../
/Users/preksh/Downloads/QQP 2

In [189]: smatch_scores = open("qqp/smatch.txt").readlines()

In [190]: smatch_scores = [i.strip().split("F: ")[1] for i in smatch_scores]

In [191]: smatch_scores = [float(i) for i in smatch_scores]

In [192]: smatch_scores
Out[192]: 
[0.29411764705882354,
 0.8695652173913043,
 0.8181818181818182,
 0.48780487804878053,
 0.7692307692307692,
 0.7407407407407407,
 0.8148148148148148,
 0.5217391304347826,
 0.7719298245614036,
 0.9375,
 0.9230769230769231,
 0.8181818181818182,
 0.5500000000000002,
 0.41379310344827586,
 0.6,
 0.25,
 0.8333333333333334,
 0.823529411764706,
 0.2285714285714286,
 0.6666666666666667,
 0.5161290322580646,
 0.8484848484848485,
 0.9,
 0.7999999999999999,
 0.761904761904762,
 0.8333333333333334,
 1.0,
 0.6666666666666665,
 0.6249999999999999,
 0.6060606060606061,
 0.5,
 0.7142857142857142,
 0.5641025641025641,
 0.40816326530612246,
 0.409090909090909,
 0.3,
 0.9090909090909091,
 0.7333333333333334,
 0.7058823529411764,
 1.0,
 0.40625,
 0.375,
 0.631578947368421,
 0.7333333333333334,
 0.9811320754716981,
 0.7,
 0.7826086956521738,
 0.4285714285714285,
 0.6363636363636364,
 0.9090909090909091,
 0.5,
 0.6285714285714286,
 0.2,
 1.0,
 0.3478260869565218,
 0.7692307692307692,
 0.5,
 0.6060606060606061,
 0.625,
 0.3703703703703703,
 0.6666666666666666,
 0.9411764705882353,
 0.8125,
 0.5806451612903225,
 0.7272727272727273,
 0.6666666666666666,
 0.37499999999999994,
 0.5925925925925926,
 0.6129032258064516,
 0.8749999999999999,
 0.8888888888888888,
 0.411764705882353,
 0.2758620689655173,
 0.6666666666666666,
 1.0,
 0.962962962962963,
 0.5660377358490566,
 0.3684210526315789,
 0.8235294117647058,
 0.7333333333333334,
 0.608695652173913,
 0.8275862068965518,
 0.5,
 0.9333333333333333,
 0.3428571428571429,
 0.5416666666666667,
 0.6774193548387096,
 0.5714285714285714,
 0.37500000000000006,
 0.5517241379310345,
 0.48484848484848486,
 0.56,
 0.9615384615384616,
 0.8000000000000002,
 0.25641025641025644,
 0.5,
 1.0,
 0.7368421052631579,
 0.8333333333333334,
 0.5365853658536586,
 0.611111111111111,
 0.9285714285714286,
 0.7000000000000001,
 0.7272727272727272,
 0.7727272727272727,
 0.8571428571428571,
 0.6415094339622641,
 0.5714285714285715,
 0.8695652173913044,
 0.8000000000000002,
 0.4057971014492754,
 0.761904761904762,
 0.37037037037037035,
 0.44827586206896547,
 0.7857142857142856,
 0.5714285714285715,
 0.6153846153846154,
 0.9411764705882353,
 0.5405405405405405,
 0.5128205128205129,
 0.5490196078431373,
 0.6222222222222222,
 0.6451612903225806,
 0.4444444444444445,
 0.9333333333333332,
 0.8666666666666666,
 0.7333333333333333,
 0.5925925925925926,
 0.5641025641025641,
 0.75,
 0.7755102040816326,
 0.6666666666666667,
 0.9411764705882353,
 0.9090909090909091,
 0.9375,
 0.9230769230769231,
 0.32,
 0.7333333333333333,
 0.9444444444444444,
 0.7272727272727272,
 0.6451612903225806,
 0.5714285714285714,
 0.5238095238095238,
 0.8823529411764706,
 0.4489795918367347,
 0.7999999999999999,
 0.6923076923076924,
 0.5294117647058824,
 0.625,
 0.7499999999999999,
 0.6,
 0.45161290322580644,
 0.875,
 1.0,
 0.6153846153846153,
 0.5294117647058824,
 0.5000000000000001,
 0.64,
 0.7000000000000001,
 0.3157894736842105,
 0.5263157894736842,
 0.7777777777777777,
 0.75,
 0.7272727272727272,
 0.9565217391304348,
 0.7407407407407408,
 1.0,
 0.5531914893617023,
 0.4126984126984127,
 0.32653061224489793,
 0.4444444444444444,
 0.5581395348837209,
 0.7586206896551724,
 0.6666666666666666,
 0.7741935483870968,
 0.6666666666666666,
 0.6923076923076924,
 0.9090909090909091,
 0.5909090909090909,
 0.8947368421052632,
 0.5945945945945946,
 0.4444444444444444,
 0.6956521739130435,
 0.823529411764706,
 0.8636363636363636,
 0.7826086956521738,
 0.3333333333333333,
 0.5833333333333334,
 0.5294117647058825,
 0.5882352941176471,
 0.9411764705882353,
 0.5,
 0.9444444444444444,
 0.85,
 0.9090909090909091,
 0.4444444444444445,
 0.5957446808510638,
 0.7000000000000001,
 0.43902439024390244,
 0.4285714285714286,
 0.6363636363636365,
 0.7407407407407406,
 0.5925925925925926,
 0.56,
 1.0,
 0.7272727272727272,
 0.23999999999999996,
 0.47368421052631576,
 0.7000000000000001,
 0.625,
 0.47222222222222227,
 0.42857142857142855,
 0.6842105263157896,
 0.2857142857142857,
 0.6285714285714286,
 0.75,
 0.5925925925925927,
 0.8695652173913043,
 0.6,
 0.6470588235294117,
 0.6,
 0.3225806451612903,
 0.8000000000000002,
 0.8399999999999999,
 0.4736842105263158,
 0.7636363636363638,
 1.0,
 0.5555555555555556,
 0.7462686567164178,
 0.9090909090909091,
 0.6111111111111112,
 0.5,
 1.0,
 0.631578947368421,
 0.6363636363636364,
 0.45614035087719296,
 0.6666666666666667,
 0.4,
 0.625,
 0.23255813953488372,
 0.5333333333333333,
 0.689655172413793,
 0.43750000000000006,
 0.5833333333333334,
 0.6222222222222223,
 0.8,
 0.391304347826087,
 0.5263157894736842,
 0.4444444444444445,
 0.4571428571428571,
 0.4864864864864865,
 0.4444444444444444,
 0.4444444444444445,
 0.4444444444444445,
 0.5,
 0.5714285714285715,
 0.47368421052631576,
 0.627450980392157,
 0.6451612903225806,
 0.5625,
 0.6808510638297872,
 0.7777777777777777,
 0.8461538461538461,
 0.4210526315789474,
 0.9333333333333333,
 0.48648648648648646,
 0.5066666666666666,
 0.6666666666666666,
 0.8181818181818182,
 0.9166666666666666,
 0.7894736842105263,
 0.6428571428571429,
 0.5454545454545455,
 0.5405405405405405,
 0.39999999999999997,
 0.6666666666666667,
 0.6250000000000001,
 0.7428571428571429,
 0.8666666666666666,
 0.8059701492537312,
 0.888888888888889,
 0.7142857142857143,
 0.5555555555555556,
 0.38709677419354843,
 0.4888888888888889,
 0.6,
 0.9285714285714286,
 0.8823529411764706,
 0.5714285714285715,
 0.8333333333333334,
 0.8421052631578948,
 0.5238095238095237,
 0.5853658536585366,
 0.6923076923076923,
 0.4186046511627907,
 0.6666666666666667,
 0.5454545454545455,
 0.5517241379310345,
 0.6315789473684211,
 0.6666666666666666,
 0.5925925925925926,
 0.6857142857142857,
 0.8333333333333334,
 0.8333333333333333,
 0.7999999999999999,
 0.5806451612903225,
 0.6808510638297872,
 0.7692307692307692,
 0.5833333333333334,
 0.608695652173913,
 0.888888888888889,
 0.6666666666666667,
 0.5714285714285714,
 0.9047619047619048,
 0.5714285714285715,
 1.0,
 0.2857142857142857,
 0.5833333333333334,
 0.30303030303030304,
 0.7222222222222222,
 0.5660377358490566,
 0.45454545454545453,
 0.5833333333333334,
 0.4,
 0.5116279069767441,
 0.5,
 0.8333333333333334,
 0.6666666666666666,
 0.5,
 0.5454545454545455,
 0.5333333333333333,
 0.4675324675324675,
 0.4137931034482759,
 0.6,
 0.8461538461538461,
 0.5161290322580645,
 0.8125000000000001,
 0.6666666666666667,
 0.875,
 0.9714285714285714,
 0.7500000000000001,
 0.7142857142857143,
 0.47826086956521735,
 0.5925925925925926,
 0.2702702702702703,
 0.5490196078431373,
 0.7428571428571428,
 0.6,
 0.8181818181818182,
 0.7906976744186047,
 0.6428571428571429,
 0.7692307692307692,
 1.0,
 0.5862068965517241,
 0.5,
 0.7692307692307692,
 0.45161290322580644,
 0.6349206349206349,
 0.7777777777777777,
 0.6000000000000001,
 0.5,
 0.9090909090909091,
 0.5641025641025641,
 0.7142857142857142,
 0.5142857142857142,
 0.8823529411764706,
 0.9444444444444444,
 0.6101694915254238,
 0.6545454545454545,
 0.4666666666666666,
 0.4242424242424243,
 0.8125,
 0.9444444444444444,
 0.7142857142857143,
 0.5333333333333333,
 0.39999999999999997,
 0.34782608695652173,
 0.8000000000000002,
 0.6111111111111112,
 0.5365853658536586,
 0.45,
 0.6808510638297872,
 0.6666666666666667,
 0.7272727272727272,
 0.6486486486486486,
 0.7407407407407406,
 0.4827586206896552,
 0.6111111111111113,
 0.606060606060606,
 0.375,
 0.4444444444444444,
 0.8181818181818182,
 0.8823529411764706,
 0.37499999999999994,
 0.7692307692307692,
 0.6111111111111113,
 0.4782608695652174,
 0.3846153846153846,
 0.7333333333333334,
 1.0,
 0.4102564102564103,
 0.6666666666666666,
 1.0,
 0.9333333333333333,
 0.7000000000000001,
 0.7499999999999999,
 0.5423728813559322,
 0.6666666666666665,
 0.3783783783783784,
 0.7500000000000001,
 0.41666666666666663,
 0.923076923076923,
 0.6206896551724138,
 0.5333333333333333,
 0.4666666666666666,
 0.7368421052631577,
 0.5000000000000001,
 0.39999999999999997,
 0.7777777777777778,
 0.29508196721311475,
 0.8372093023255814,
 0.64,
 0.7272727272727272,
 0.6,
 0.5999999999999999,
 0.8823529411764706,
 0.45454545454545453,
 0.88,
 1.0,
 0.7741935483870968,
 0.8,
 0.5,
 0.6428571428571428,
 0.6153846153846153,
 0.4878048780487805,
 0.5454545454545454,
 0.888888888888889,
 0.6,
 0.9,
 0.48484848484848486,
 0.55,
 0.48,
 0.25806451612903225,
 0.7999999999999999,
 0.5384615384615385,
 0.4918032786885246,
 1.0,
 0.9500000000000001,
 0.4545454545454546,
 0.4878048780487805,
 0.6111111111111113,
 0.5714285714285715,
 0.4375,
 0.4166666666666667,
 0.5531914893617021,
 0.4571428571428571,
 0.32,
 0.5000000000000001,
 0.6451612903225806,
 0.8125,
 0.44444444444444436,
 0.30769230769230765,
 0.962962962962963,
 0.5185185185185186,
 0.6285714285714286,
 0.8823529411764706,
 0.4666666666666667,
 0.4347826086956522,
 0.5106382978723405,
 0.75,
 0.8,
 0.13953488372093023,
 0.8000000000000002,
 0.588235294117647,
 1.0,
 0.7272727272727273,
 0.9090909090909091,
 0.6470588235294118,
 0.5806451612903226,
 0.44000000000000006,
 0.7500000000000001,
 0.5714285714285714,
 0.5454545454545454,
 0.5,
 0.3870967741935484,
 0.6666666666666667,
 0.5833333333333334,
 0.7000000000000001,
 0.5714285714285715,
 0.606060606060606,
 0.7857142857142856,
 0.9090909090909091,
 0.37037037037037035,
 0.6153846153846153,
 0.5,
 0.45454545454545453,
 1.0,
 0.7777777777777778,
 0.823529411764706,
 0.8461538461538461,
 0.8571428571428571,
 0.631578947368421,
 0.5599999999999999,
 0.6296296296296297,
 0.5555555555555556,
 0.7692307692307693,
 0.782608695652174,
 0.6,
 0.7692307692307692,
 0.6363636363636365,
 0.8333333333333333,
 0.4999999999999999,
 0.35000000000000003,
 0.8749999999999999,
 0.7586206896551724,
 0.4081632653061224,
 0.875,
 0.7499999999999999,
 0.3636363636363636,
 0.19354838709677416,
 0.8571428571428571,
 0.6551724137931033,
 0.6666666666666667,
 0.8000000000000002,
 0.7346938775510203,
 0.7692307692307692,
 1.0,
 0.7317073170731706,
 0.8571428571428571,
 1.0,
 0.606060606060606,
 0.8666666666666667,
 0.5882352941176471,
 0.8333333333333333,
 0.8000000000000002,
 0.9090909090909091,
 0.5833333333333334,
 0.7999999999999999,
 0.5384615384615384,
 0.5666666666666667,
 1.0,
 1.0,
 0.4444444444444444,
 0.7333333333333333,
 0.8461538461538461,
 0.7999999999999999,
 0.7142857142857143,
 0.24,
 0.7000000000000001,
 0.47058823529411764,
 0.875,
 0.9230769230769231,
 0.6666666666666667,
 0.7391304347826088,
 0.6666666666666665,
 0.5714285714285715,
 0.7142857142857143,
 0.7272727272727272,
 0.8666666666666667,
 0.9090909090909091,
 0.588235294117647,
 0.49382716049382713,
 0.5384615384615384,
 0.5833333333333334,
 0.5217391304347826,
 0.5517241379310345,
 0.9655172413793104,
 0.6666666666666666,
 0.47058823529411764,
 0.4307692307692308,
 1.0,
 0.6153846153846153,
 0.20689655172413793,
 0.8461538461538461,
 0.6956521739130435,
 0.5714285714285714,
 0.4666666666666667,
 0.6666666666666666,
 0.8571428571428571,
 0.7857142857142856,
 0.8888888888888888,
 0.35714285714285715,
 0.8125000000000001,
 0.3225806451612903,
 0.8333333333333333,
 0.4166666666666667,
 1.0,
 0.7272727272727272,
 0.9230769230769231,
 0.7727272727272727,
 0.6829268292682927,
 0.71875,
 0.6923076923076924,
 0.7222222222222222,
 0.9411764705882353,
 0.42857142857142855,
 0.676923076923077,
 1.0,
 0.875,
 0.4761904761904762,
 0.6666666666666667,
 0.6779661016949153,
 0.5625000000000001,
 0.6363636363636365,
 0.28571428571428575,
 0.9411764705882353,
 0.8095238095238095,
 0.962962962962963,
 0.5999999999999999,
 0.7499999999999999,
 0.6363636363636365,
 0.4090909090909091,
 0.5789473684210527,
 0.8717948717948718,
 0.6511627906976744,
 0.711111111111111,
 0.4210526315789474,
 0.7027027027027027,
 0.8148148148148148,
 0.5,
 0.619047619047619,
 0.8333333333333333,
 0.5116279069767441,
 0.6666666666666666,
 0.6000000000000001,
 0.5517241379310344,
 0.7096774193548387,
 0.7333333333333334,
 0.6923076923076924,
 0.8125000000000001,
 0.339622641509434,
 0.6511627906976745,
 0.5714285714285713,
 0.8421052631578948,
 0.8749999999999999,
 1.0,
 0.7692307692307693,
 0.4848484848484849,
 0.65,
 0.9090909090909091,
 0.76,
 0.5454545454545454,
 0.35714285714285715,
 1.0,
 0.5,
 0.6923076923076924,
 0.4166666666666667,
 0.4210526315789474,
 0.4444444444444444,
 1.0,
 0.5294117647058824,
 0.9166666666666666,
 0.6,
 0.7499999999999999,
 0.6923076923076924,
 0.5625000000000001,
 0.48275862068965514,
 0.8260869565217391,
 1.0,
 0.5294117647058824,
 0.4390243902439025,
 0.6470588235294117,
 0.5384615384615384,
 0.7586206896551724,
 0.33333333333333337,
 0.7999999999999999,
 0.36363636363636365,
 0.6666666666666667,
 0.4528301886792453,
 1.0,
 0.5806451612903226,
 0.68,
 0.6363636363636365,
 0.9583333333333334,
 0.9565217391304348,
 0.7407407407407406,
 0.8333333333333333,
 0.9642857142857143,
 0.6206896551724139,
 0.606060606060606,
 0.6470588235294118,
 0.39999999999999997,
 0.3,
 0.5,
 0.46511627906976744,
 0.6829268292682926,
 0.9500000000000001,
 0.456140350877193,
 0.5714285714285715,
 0.8571428571428571,
 1.0,
 0.7428571428571429,
 0.4444444444444444,
 0.8,
 0.8666666666666667,
 0.5806451612903226,
 0.8125,
 0.5833333333333334,
 0.3870967741935484,
 0.5,
 0.3448275862068966,
 0.5454545454545454,
 0.761904761904762,
 0.8181818181818182,
 0.7428571428571428,
 0.8571428571428571,
 0.6250000000000001,
 0.7096774193548387,
 0.9,
 0.5714285714285715,
 0.5,
 0.5531914893617021,
 0.6363636363636365,
 0.5714285714285714,
 0.47619047619047616,
 0.6666666666666666,
 0.8695652173913043,
 0.7878787878787877,
 0.6086956521739131,
 0.7083333333333334,
 0.65,
 0.7272727272727272,
 1.0,
 0.7272727272727273,
 0.8888888888888888,
 0.4848484848484849,
 0.5789473684210527,
 0.8780487804878048,
 0.37499999999999994,
 0.5238095238095238,
 0.6666666666666666,
 0.909090909090909,
 0.9444444444444444,
 0.5,
 0.6923076923076924,
 0.5384615384615384,
 0.43478260869565216,
 0.45714285714285713,
 0.8571428571428571,
 0.8955223880597014,
 0.8947368421052632,
 0.6060606060606061,
 0.5454545454545455,
 0.4166666666666667,
 0.9523809523809523,
 1.0,
 0.888888888888889,
 0.7999999999999999,
 0.4210526315789474,
 0.8947368421052632,
 0.8400000000000001,
 0.5,
 0.6,
 0.5,
 0.6923076923076923,
 0.32,
 0.7200000000000001,
 0.38095238095238093,
 0.4666666666666667,
 0.6285714285714286,
 0.4285714285714286,
 0.8421052631578947,
 0.625,
 0.6666666666666665,
 0.15384615384615383,
 0.5,
 0.32,
 0.8749999999999999,
 0.6315789473684211,
 0.5333333333333333,
 0.4313725490196078,
 0.27586206896551724,
 0.9285714285714286,
 0.6666666666666666,
 0.8571428571428571,
 0.9019607843137256,
 0.6428571428571429,
 1.0,
 0.5806451612903226,
 0.8000000000000002,
 0.5945945945945945,
 0.6086956521739131,
 0.4583333333333333,
 0.625,
 0.32,
 0.41379310344827586,
 0.8000000000000002,
 0.7857142857142856,
 0.65,
 0.6666666666666667,
 0.4444444444444445,
 0.3478260869565218,
 0.2,
 0.40909090909090906,
 0.8333333333333333,
 0.4137931034482759,
 0.625,
 0.6,
 0.5806451612903226,
 0.588235294117647,
 0.5365853658536585,
 0.3,
 0.8461538461538461,
 0.509090909090909,
 0.4285714285714286,
 0.7333333333333334,
 0.34782608695652173,
 0.5714285714285715,
 0.4313725490196078,
 0.6923076923076923,
 0.8571428571428571,
 0.7692307692307693,
 0.3673469387755103,
 0.27450980392156865,
 0.5365853658536585,
 0.30769230769230765,
 0.8205128205128205,
 0.8461538461538461,
 0.6666666666666665,
 0.4,
 0.8275862068965517,
 0.5806451612903225,
 0.7272727272727272,
 0.875,
 0.6122448979591837,
 0.3846153846153846,
 0.5555555555555556,
 0.4799999999999999,
 1.0,
 0.5517241379310345,
 0.6666666666666666,
 0.35714285714285715,
 0.9500000000000001,
 0.6486486486486486,
 0.9333333333333333,
 0.42857142857142855,
 0.6470588235294118,
 0.5454545454545455,
 0.32,
 0.8,
 0.8918918918918919,
 0.7777777777777777,
 0.6222222222222222,
 0.5,
 1.0,
 0.8749999999999999,
 0.44,
 0.8125,
 0.888888888888889,
 0.6470588235294117,
 0.5,
 0.36,
 0.6666666666666666,
 0.7000000000000001,
 0.8749999999999999,
 0.5925925925925927,
 0.8571428571428571,
 0.5098039215686274,
 0.6363636363636365,
 0.7058823529411764,
 0.8181818181818182,
 0.7500000000000001,
 0.6153846153846153,
 0.5625000000000001,
 0.4827586206896552,
 0.6666666666666665,
 0.9047619047619048,
 0.45,
 0.923076923076923,
 0.761904761904762,
 0.6666666666666666,
 0.7719298245614036,
 0.8666666666666667,
 0.8076923076923077,
 0.823529411764706,
 0.6,
 0.8823529411764706,
 0.9285714285714286,
 1.0,
 0.5217391304347826,
 0.8571428571428571,
 1.0,
 0.5,
 0.38461538461538464,
 0.4000000000000001,
 0.35294117647058815,
 0.9,
 0.8260869565217391,
 0.8571428571428571,
 0.8837209302325582,
 0.6874999999999999,
 0.7272727272727273,
 0.37209302325581395,
 0.5245901639344263,
 0.6511627906976744,
 0.6923076923076923,
 0.34285714285714286,
 0.36734693877551017,
 0.5106382978723404,
 0.7027027027027026,
 0.8461538461538461,
 0.9230769230769231,
 0.64,
 0.6666666666666667,
 0.5555555555555556,
 0.7777777777777777,
 0.6666666666666665,
 0.6341463414634146,
 0.5142857142857143,
 0.5000000000000001,
 0.9655172413793104,
 0.6896551724137931,
 0.4000000000000001,
 0.3888888888888889,
 0.45161290322580644,
 0.8125,
 1.0,
 0.6,
 0.4814814814814815,
 0.8695652173913043,
 0.8571428571428571,
 0.5454545454545454,
 0.75,
 0.5333333333333333,
 1.0,
 0.5531914893617021,
 0.39999999999999997,
 0.7142857142857142,
 0.6122448979591837,
 0.7058823529411765,
 0.888888888888889,
 0.4444444444444445,
 0.7272727272727272,
 0.6206896551724138,
 0.6,
 0.7804878048780488,
 0.5806451612903226,
 0.7586206896551724,
 0.5833333333333334,
 0.8695652173913043,
 0.5263157894736842,
 0.6842105263157894,
 0.5555555555555555,
 0.6,
 0.7272727272727272,
 0.7647058823529412,
 0.6111111111111112,
 0.4705882352941177,
 0.39999999999999997,
 0.4,
 0.7500000000000001,
 0.6666666666666666,
 0.39285714285714285,
 0.6666666666666666,
 0.6842105263157895,
 0.5185185185185185,
 0.2222222222222222,
 0.4210526315789473,
 0.3389830508474576,
 0.7857142857142857,
 0.6666666666666667,
 0.6,
 0.7272727272727273,
 0.5833333333333334,
 0.5,
 0.35714285714285715,
 0.46153846153846156,
 0.8333333333333333,
 0.7027027027027026,
 0.7857142857142857,
 0.9166666666666666,
 0.6666666666666667,
 0.8461538461538461,
 0.5599999999999999,
 0.7272727272727272,
 0.9090909090909091,
 0.6133333333333334,
 0.5316455696202531,
 0.6875000000000001,
 0.4444444444444445,
 0.45454545454545453,
 0.9166666666666666,
 0.5405405405405405,
 0.6153846153846154,
 0.4827586206896552,
 0.5517241379310345,
 0.5185185185185185,
 0.9,
 0.5555555555555556,
 0.9705882352941176,
 1.0,
 0.3333333333333333,
 0.6521739130434783,
 0.7499999999999999,
 0.8095238095238095,
 0.3225806451612903,
 0.9,
 0.4117647058823529,
 0.4827586206896552,
 0.5,
 ...]

In [193]: qqp_score = open("qqp_dataset/score.txt").readlines()

In [194]: qqp_score
Out[194]: 
['1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 '1\n',
 ...]

In [195]: qqp_score = [i.strip() for i in qqp_score]

In [196]: qqp_score
Out[196]: 
['1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 '1',
 ...]

In [197]: qqp_score = [float(i) for i in qqp_score]

In [198]: qqp_score
Out[198]: 
[1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 1.0,
 ...]

In [199]: qqp_score[2500]
Out[199]: 0.0

In [200]: qqp_score[2501]
Out[200]: 0.0

In [201]: qqp_score[2502]
Out[201]: 0.0

In [202]: len(qqp_score)
Out[202]: 5000

In [203]: plt.scatter(qqp_score, smatch_scores)
Out[203]: <matplotlib.collections.PathCollection at 0x1406afeb0>

In [204]: plt.show()

In [205]: p_scores = []

In [206]: np_scores = []

In [207]: for i, j in zip(qqp_score, smatch_scores):
     ...:     if i == 1:
     ...:         p_scores.append(j)
     ...:     else:
     ...:         np_scores.append(i)
     ...: 

In [208]: 

In [208]: np_scores = []

In [209]: p_scores = []

In [210]: for i, j in zip(qqp_score, smatch_scores):
     ...:     if i == 1:
     ...:         p_scores.append(j)
     ...:     else:
     ...:         np_scores.append(j)
     ...: 

In [211]: plt.hist(p_scores, color='b', alpha=0.5)
Out[211]: 
(array([  9.,  56., 162., 320., 371., 421., 359., 307., 267., 228.]),
 array([0.13953488, 0.2255814 , 0.31162791, 0.39767442, 0.48372093,
        0.56976744, 0.65581395, 0.74186047, 0.82790698, 0.91395349,
        1.        ]),
 <BarContainer object of 10 artists>)

In [212]: plt.hist(np_scores, color='g', alpha=0.5)
Out[212]: 
(array([ 79., 316., 425., 413., 365., 293., 191., 169., 129., 120.]),
 array([0.04444444, 0.14      , 0.23555556, 0.33111111, 0.42666667,
        0.52222222, 0.61777778, 0.71333333, 0.80888889, 0.90444444,
        1.        ]),
 <BarContainer object of 10 artists>)

In [213]: 

In [213]: plt.show()

In [214]: import seaborn as sns

In [215]: df = pd.DataFrame({})

In [216]: df["qqp"] = qqp_score

In [217]: df["smatch"] = smatch_scores

In [218]: sns.boxplot(x="qqp", y="smatch", data=df)
Out[218]: <AxesSubplot:xlabel='qqp', ylabel='smatch'>

In [219]: plt.show()

In [220]: sns.set_style("whitegrid")

In [221]: sns
Out[221]: <module 'seaborn' from '/Users/preksh/Library/Python/3.8/lib/python/site-packages/seaborn/__init__.py'>

In [222]: plt.xlabel("Sentence Pair Category", fontsize=16)
Out[222]: Text(0.5, 0, 'Sentence Pair Category')

In [223]: plt.ylabel("SMATCH Score", fontsize=16)
Out[223]: Text(0, 0.5, 'SMATCH Score')

In [224]: plt.title("SMATCH distribution for QQP", fontsize=21)
Out[224]: Text(0.5, 1.0, 'SMATCH distribution for QQP')

In [225]: df["qqp_cat"] = [cat[int(i)] for i in qqp_scores]
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-225-47129f0e77f5> in <module>
----> 1 df["qqp_cat"] = [cat[int(i)] for i in qqp_scores]

NameError: name 'qqp_scores' is not defined

In [226]: cat = ["Non-Paraphrase", "Paraphrase"]

In [227]: df["qqp_cat"] = [cat[int(i)] for i in qqp_score]

In [228]: sns.boxplot(x="qqp_cat", y="smatch", data=df)
Out[228]: <AxesSubplot:title={'center':'SMATCH distribution for QQP'}, xlabel='qqp_cat', ylabel='smatch'>

In [229]: plt.show()

In [230]: sns.boxplot(x="qqp_cat", y="smatch", data=df)
Out[230]: <AxesSubplot:xlabel='qqp_cat', ylabel='smatch'>

In [231]: plt.title("SMATCH distribution for QQP", fontsize=21)
Out[231]: Text(0.5, 1.0, 'SMATCH distribution for QQP')

In [232]: plt.ylabel("SMATCH Score", fontsize=16)
Out[232]: Text(0, 0.5, 'SMATCH Score')

In [233]: plt.xlabel("Sentence Pair Category", fontsize=16)
Out[233]: Text(0.5, 0, 'Sentence Pair Category')

In [234]: plt.show()

In [235]: ls
qqp/         qqp_dataset/

In [236]: cd /Users/preksh/Downloads/mrpc_pairs\ 2
/Users/preksh/Downloads/mrpc_pairs 2

In [237]: ls
mrpc_smatch/    notparaphrases/ paraphrases/

In [238]: cd mrpc_smatch/
/Users/preksh/Downloads/mrpc_pairs 2/mrpc_smatch

In [239]: ls
np_amr1.txt    np_smatch.txt  np_snt2.txt    p_amr2.txt     p_snt1.txt
np_amr2.txt    np_snt1.txt    p_amr1.txt     p_smatch.txt   p_snt2.txt

In [240]: def get_smatch_scores(filename)
  File "<ipython-input-240-d79639b48e71>", line 1
    def get_smatch_scores(filename)
                                   ^
SyntaxError: invalid syntax


In [241]: def get_smatch_scores(filename):
     ...:     x = open(filename).readlines()
     ...:     x = [i.strip().split("F: ")[1] for i in x]
     ...:     x = [float(i) for i in x]
     ...:     return x
     ...: 

In [242]: np_scores = get_smatch_scores("np_smatch.txt")

In [243]: np_scores
Out[243]: 
[0.20454545454545456,
 0.1728395061728395,
 0.30769230769230765,
 0.12244897959183673,
 0.19718309859154928,
 0.17582417582417584,
 0.20000000000000004,
 0.1348314606741573,
 0.13559322033898305,
 0.32911392405063294,
 0.19277108433734938,
 0.34408602150537637,
 0.22222222222222224,
 0.2142857142857143,
 0.17142857142857143,
 0.3157894736842105,
 0.1818181818181818,
 0.25287356321839083,
 0.29787234042553196,
 0.2168674698795181,
 0.27659574468085113,
 0.25316455696202533,
 0.26666666666666666,
 0.2535211267605634,
 0.23376623376623376,
 0.3529411764705882,
 0.17543859649122806,
 0.3157894736842105,
 0.27027027027027023,
 0.10416666666666666,
 0.15873015873015875,
 0.24561403508771928,
 0.09999999999999999,
 0.2972972972972973,
 0.15625,
 0.15873015873015875,
 0.17500000000000002,
 0.2153846153846154,
 0.28571428571428575,
 0.14545454545454545,
 0.11764705882352942,
 0.24561403508771934,
 0.0930232558139535,
 0.17910447761194026,
 0.17857142857142858,
 0.17391304347826086,
 0.360655737704918,
 0.12698412698412698,
 0.2580645161290323,
 0.1388888888888889,
 0.2702702702702703,
 0.2608695652173913,
 0.31999999999999995,
 0.15384615384615383,
 0.23529411764705882,
 0.1724137931034483,
 0.1724137931034483,
 0.16666666666666669,
 0.18181818181818182,
 0.25225225225225223,
 0.19230769230769232,
 0.1568627450980392,
 0.2558139534883721,
 0.19512195121951217,
 0.1639344262295082,
 0.2558139534883721,
 0.2631578947368421,
 0.22857142857142854,
 0.0909090909090909,
 0.2545454545454546,
 0.208955223880597,
 0.13698630136986303,
 0.2941176470588235,
 0.16129032258064516,
 0.24615384615384614,
 0.23333333333333334,
 0.25925925925925924,
 0.2162162162162162,
 0.25,
 0.22580645161290322,
 0.1917808219178082,
 0.26966292134831465,
 0.2553191489361702,
 0.16666666666666666,
 0.303030303030303,
 0.09523809523809525,
 0.19444444444444445,
 0.21739130434782608,
 0.28125,
 0.28888888888888886,
 0.1951219512195122,
 0.14285714285714282,
 0.26666666666666666,
 0.2127659574468085,
 0.3768115942028986,
 0.17142857142857143,
 0.3174603174603175,
 0.2711864406779661,
 0.1971830985915493,
 0.19047619047619044,
 0.15151515151515152,
 0.24324324324324326,
 0.19672131147540986,
 0.14634146341463417,
 0.2222222222222222,
 0.1923076923076923,
 0.26666666666666666,
 0.1927710843373494,
 0.23728813559322032,
 0.14084507042253522,
 0.2727272727272727,
 0.2641509433962264,
 0.19999999999999998,
 0.19277108433734938,
 0.15053763440860216,
 0.1894736842105263,
 0.18181818181818185,
 0.34782608695652173,
 0.09374999999999999,
 0.339622641509434,
 0.1724137931034483,
 0.19047619047619044,
 0.09999999999999999,
 0.1724137931034483,
 0.17391304347826086,
 0.17142857142857143,
 0.1282051282051282,
 0.12048192771084337,
 0.13157894736842102,
 0.14492753623188406,
 0.125,
 0.15873015873015875,
 0.12765957446808512,
 0.11940298507462686,
 0.16,
 0.20689655172413793,
 0.13114754098360654,
 0.20408163265306123,
 0.1794871794871795,
 0.19672131147540986,
 0.19178082191780824,
 0.1951219512195122,
 0.0909090909090909,
 0.1818181818181818,
 0.22641509433962265,
 0.12903225806451613,
 0.37209302325581395,
 0.14545454545454545,
 0.18823529411764706,
 0.17910447761194032,
 0.16666666666666669,
 0.21875,
 0.2153846153846154,
 0.20689655172413793,
 0.1923076923076923,
 0.27027027027027023,
 0.21875,
 0.14035087719298245,
 0.17204301075268816,
 0.1702127659574468,
 0.16326530612244897,
 0.22535211267605634,
 0.17721518987341772,
 0.39215686274509803,
 0.125,
 0.2352941176470588,
 0.18181818181818182,
 0.23255813953488372,
 0.26506024096385544,
 0.10526315789473684,
 0.18181818181818182,
 0.15555555555555556,
 0.14035087719298245,
 0.3548387096774193,
 0.2298850574712644,
 0.31034482758620696,
 0.27692307692307694,
 0.23376623376623376,
 0.28985507246376807,
 0.36065573770491804,
 0.2162162162162162,
 0.17910447761194032,
 0.14814814814814814,
 0.12987012987012989,
 0.2272727272727273,
 0.14814814814814814,
 0.3098591549295775,
 0.11594202898550723,
 0.14285714285714285,
 0.31111111111111117,
 0.2941176470588235,
 0.3373493975903614,
 0.3037974683544304,
 0.14285714285714285,
 0.2666666666666666,
 0.25974025974025977,
 0.2333333333333333,
 0.24000000000000002,
 0.3170731707317073,
 0.1090909090909091,
 0.2181818181818182,
 0.17391304347826086,
 0.2278481012658228,
 0.11538461538461538,
 0.23529411764705885,
 0.1388888888888889,
 0.2647058823529412,
 0.20833333333333334,
 0.22222222222222224,
 0.16666666666666666,
 0.2894736842105264,
 0.25396825396825395,
 0.20408163265306123,
 0.3384615384615385,
 0.2325581395348837,
 0.1851851851851852,
 0.25806451612903225,
 0.1090909090909091,
 0.07843137254901962,
 0.17647058823529407,
 0.21176470588235294,
 0.23076923076923075,
 0.1568627450980392,
 0.17142857142857143,
 0.3283582089552239,
 0.21212121212121213,
 0.1492537313432836,
 0.2545454545454545,
 0.29885057471264365,
 0.15873015873015875,
 0.08695652173913045,
 0.18518518518518517,
 0.22535211267605634,
 0.0975609756097561,
 0.24390243902439024,
 0.2247191011235955,
 0.11940298507462688,
 0.1587301587301587,
 0.19801980198019806,
 0.20338983050847456,
 0.163265306122449,
 0.21428571428571427,
 0.3125,
 0.17910447761194026,
 0.08450704225352113,
 0.2823529411764706,
 0.2622950819672131,
 0.13636363636363635,
 0.163265306122449,
 0.16326530612244897,
 0.1764705882352941,
 0.2388059701492537,
 0.3157894736842105,
 0.2105263157894737,
 0.23076923076923075,
 0.2285714285714286,
 0.08695652173913043,
 0.2571428571428572,
 0.3050847457627119,
 0.16216216216216214,
 0.24489795918367344,
 0.13333333333333333,
 0.32876712328767127,
 0.21875,
 0.11538461538461538,
 0.17582417582417584,
 0.2631578947368421,
 0.2456140350877193,
 0.23188405797101447,
 0.22222222222222224,
 0.1568627450980392,
 0.1875,
 0.2222222222222222,
 0.15873015873015872,
 0.2807017543859649,
 0.21428571428571427,
 0.24137931034482765,
 0.14545454545454545,
 0.42857142857142855,
 0.411764705882353,
 0.27272727272727276,
 0.24444444444444444,
 0.2058823529411765,
 0.2058823529411765,
 0.20289855072463767,
 0.3661971830985915,
 0.14285714285714285,
 0.26666666666666666,
 0.08163265306122448,
 0.22222222222222224,
 0.21739130434782608,
 0.23999999999999996,
 0.22950819672131145,
 0.2631578947368421,
 0.271604938271605,
 0.2592592592592593,
 0.11764705882352941,
 0.17543859649122806,
 0.16438356164383558,
 0.1212121212121212,
 0.1518987341772152,
 0.2807017543859649,
 0.17073170731707318,
 0.25,
 0.33962264150943394,
 0.3333333333333333,
 0.14285714285714285,
 0.09090909090909091,
 0.25,
 0.24615384615384614,
 0.11111111111111112,
 0.17241379310344826,
 0.18421052631578946,
 0.24999999999999994,
 0.12307692307692307,
 0.1568627450980392,
 0.1904761904761905,
 0.2222222222222222,
 0.2337662337662338,
 0.15094339622641512,
 0.20930232558139536,
 0.16901408450704225,
 0.31884057971014496,
 0.13513513513513514,
 0.08571428571428572,
 0.22222222222222218,
 0.2711864406779661,
 0.3055555555555556,
 0.1846153846153846,
 0.19178082191780824,
 0.2337662337662338,
 0.3157894736842105,
 0.26086956521739135,
 0.2545454545454545,
 0.2,
 0.1764705882352941,
 0.2580645161290323,
 0.3157894736842105,
 0.19718309859154928,
 0.20895522388059704,
 0.24242424242424246,
 0.2564102564102564,
 0.3023255813953488,
 0.23728813559322032,
 0.16867469879518074,
 0.23809523809523808,
 0.1568627450980392,
 0.17543859649122803,
 0.06451612903225806,
 0.21951219512195122,
 0.25,
 0.08571428571428572,
 0.1875,
 0.13888888888888887,
 0.24390243902439027,
 0.26865671641791045,
 0.24242424242424243,
 0.2903225806451613,
 0.24999999999999994,
 0.26666666666666666,
 0.19999999999999998,
 0.20408163265306123,
 0.2857142857142857,
 0.14814814814814814,
 0.2758620689655172,
 0.1388888888888889,
 0.22222222222222224,
 0.2647058823529412,
 0.27848101265822783,
 0.13559322033898305,
 0.13114754098360656,
 0.31428571428571433,
 0.15094339622641512,
 0.15873015873015875,
 0.15151515151515152,
 0.2727272727272727,
 0.21428571428571427,
 0.2,
 0.16,
 0.21621621621621617,
 0.2,
 0.16393442622950816,
 0.2368421052631579,
 0.21176470588235297,
 0.1772151898734177,
 0.1176470588235294,
 0.2580645161290322,
 0.1818181818181818,
 0.27083333333333337,
 0.18181818181818182,
 0.21052631578947367,
 0.21538461538461537,
 0.22535211267605634,
 0.1686746987951807,
 0.26666666666666666,
 0.2962962962962963,
 0.20338983050847456,
 0.3043478260869565,
 0.08791208791208792,
 0.13186813186813184,
 0.1724137931034483,
 0.14814814814814814,
 0.2898550724637681,
 0.3157894736842105,
 0.22580645161290322,
 0.20408163265306123,
 0.27499999999999997,
 0.3137254901960784,
 0.1846153846153846,
 0.41269841269841273,
 0.1408450704225352,
 0.17857142857142858,
 0.3728813559322034,
 0.20689655172413793,
 0.16,
 0.2,
 0.19999999999999998,
 0.22641509433962265,
 0.22222222222222224,
 0.24999999999999994,
 0.10909090909090907,
 0.2077922077922078,
 0.2,
 0.19753086419753088,
 0.1558441558441558,
 0.11538461538461538,
 0.1,
 0.21212121212121213,
 0.2571428571428571,
 0.18604651162790697,
 0.2903225806451613,
 0.2647058823529412,
 0.18918918918918917,
 0.23529411764705882,
 0.1851851851851852,
 0.12048192771084337,
 0.25,
 0.17283950617283952,
 0.1702127659574468,
 0.23728813559322037,
 0.225,
 0.2413793103448276,
 0.1851851851851852,
 0.2191780821917808,
 0.1754385964912281,
 0.21951219512195125,
 0.18867924528301885,
 0.2033898305084746,
 0.19718309859154928,
 0.2222222222222222,
 0.21686746987951805,
 0.3214285714285714,
 0.36363636363636365,
 0.19999999999999998,
 0.18181818181818182,
 0.18461538461538463,
 0.2162162162162162,
 0.16216216216216214,
 0.2173913043478261,
 0.21212121212121215,
 0.2191780821917808,
 0.28,
 0.25806451612903225,
 0.2318840579710145,
 0.208955223880597,
 0.3018867924528302,
 0.12765957446808512,
 0.22727272727272724,
 0.23076923076923075,
 0.24999999999999994,
 0.16666666666666666,
 0.23684210526315794,
 0.10204081632653061,
 0.26086956521739135,
 0.2318840579710145,
 0.17391304347826086,
 0.1568627450980392,
 0.15999999999999998,
 0.28571428571428575,
 0.32,
 0.15873015873015872,
 0.14285714285714288,
 0.13114754098360656,
 0.16901408450704225,
 0.2051282051282051,
 0.21428571428571425,
 0.38461538461538464,
 0.0625,
 0.13333333333333333,
 0.22448979591836735,
 0.2222222222222222,
 0.2580645161290323,
 0.25,
 0.19178082191780824,
 0.1492537313432836,
 0.17500000000000002,
 0.22950819672131148,
 0.13333333333333333,
 0.13333333333333333,
 0.26666666666666666,
 0.16666666666666666,
 0.21276595744680848,
 0.2608695652173913,
 0.27586206896551724,
 0.18181818181818185,
 0.27848101265822783,
 0.20689655172413796,
 0.15094339622641512,
 0.2545454545454545,
 0.32142857142857145,
 0.16129032258064516,
 0.21052631578947367,
 0.22222222222222224,
 0.19999999999999998,
 0.2571428571428572,
 0.12121212121212122,
 0.15151515151515152,
 0.2456140350877193,
 0.1886792452830189,
 0.125,
 0.19718309859154928,
 0.09374999999999999,
 0.15384615384615385,
 0.25974025974025977,
 0.23255813953488372,
 0.27848101265822783,
 0.12,
 0.25,
 0.19999999999999998,
 0.20408163265306126,
 0.17391304347826086,
 0.2641509433962264,
 0.17241379310344826,
 0.2456140350877193,
 0.09836065573770492,
 0.375,
 0.25,
 0.21818181818181817,
 0.275,
 0.1904761904761905,
 0.3611111111111111,
 0.1694915254237288,
 0.13793103448275862,
 0.2564102564102564,
 0.28070175438596495,
 0.25352112676056343,
 0.2278481012658228,
 0.28235294117647064,
 0.21686746987951805,
 0.14285714285714288,
 0.1694915254237288,
 0.2727272727272727,
 0.14285714285714288,
 0.15625,
 0.28571428571428575,
 0.35714285714285715,
 0.28571428571428564,
 0.21276595744680854,
 0.20689655172413793,
 0.2222222222222222,
 0.24,
 0.26666666666666666,
 0.0923076923076923,
 0.24691358024691357,
 0.14814814814814814,
 0.21538461538461537,
 0.13114754098360656,
 0.2711864406779661,
 0.20253164556962025,
 0.208955223880597,
 0.3508771929824561,
 0.20689655172413793,
 0.1388888888888889,
 0.14893617021276595,
 0.17857142857142858,
 0.20000000000000004,
 0.1839080459770115]

In [244]: df = pd.DataFrame({})

In [245]: df["smatch"] = np_scores

In [246]: df["cat"] = ["Non-Paraphrase"]*len(np_scores)

In [247]: p_scores = get_smatch_scores("p_smatch.txt")

In [248]: p_df = pd.DataFrame({})

In [249]: df["smatch"] = p_scores
---------------------------------------------------------------------------
ValueError                                Traceback (most recent call last)
<ipython-input-249-7fe5ee5c62e7> in <module>
----> 1 df["smatch"] = p_scores

/Library/Python/3.8/site-packages/pandas/core/frame.py in __setitem__(self, key, value)
   3161         else:
   3162             # set column
-> 3163             self._set_item(key, value)
   3164 
   3165     def _setitem_slice(self, key: slice, value):

/Library/Python/3.8/site-packages/pandas/core/frame.py in _set_item(self, key, value)
   3240         """
   3241         self._ensure_valid_index(value)
-> 3242         value = self._sanitize_column(key, value)
   3243         NDFrame._set_item(self, key, value)
   3244 

/Library/Python/3.8/site-packages/pandas/core/frame.py in _sanitize_column(self, key, value, broadcast)
   3897 
   3898             # turn me into an ndarray
-> 3899             value = sanitize_index(value, self.index)
   3900             if not isinstance(value, (np.ndarray, Index)):
   3901                 if isinstance(value, list) and len(value) > 0:

/Library/Python/3.8/site-packages/pandas/core/internals/construction.py in sanitize_index(data, index)
    749     """
    750     if len(data) != len(index):
--> 751         raise ValueError(
    752             "Length of values "
    753             f"({len(data)}) "

ValueError: Length of values (1147) does not match length of index (577)

In [250]: df["smatch"] = p_score
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-250-4eb3983212c4> in <module>
----> 1 df["smatch"] = p_score

NameError: name 'p_score' is not defined

In [251]: p_df["smatch"] = p_score
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-251-ab2087d6592f> in <module>
----> 1 p_df["smatch"] = p_score

NameError: name 'p_score' is not defined

In [252]: p_df["smatch"] = p_scores

In [253]: p_df["cat"] = ["Paraphrase"]*len(p_scores)

In [254]: p_df = p_df.append(df, ignore_index=True)

In [255]: sns.boxplot(x="cat", y="smatch", data=dp_f)
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-255-1b31d7992f51> in <module>
----> 1 sns.boxplot(x="cat", y="smatch", data=dp_f)

NameError: name 'dp_f' is not defined

In [256]: sns.boxplot(x="cat", y="smatch", data=p_df
     ...: )
Out[256]: <AxesSubplot:xlabel='cat', ylabel='smatch'>

In [257]: plt.title("SMATCH distribution for MRPC", fontsize=21)
Out[257]: Text(0.5, 1.0, 'SMATCH distribution for MRPC')

In [258]: plt.xlabel("Sentence Pair Category", fontsize=16)
Out[258]: Text(0.5, 0, 'Sentence Pair Category')

In [259]: plt.ylabel("SMATCH Score", fontsize=16)
Out[259]: Text(0, 0.5, 'SMATCH Score')

In [260]: plt.show()

In [261]: import sklearn.metrics as metrics

In [262]: metrics.auc(qqp_score, smatch_scores)
Out[262]: 0.3927125506072875

In [263]: fpr, tpr, threshold  = roc_curve(y_true=y_np + y_p , y_score=np_scores+ p_scores)
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-263-50e64ae376d9> in <module>
----> 1 fpr, tpr, threshold  = roc_curve(y_true=y_np + y_p , y_score=np_scores+ p_scores)

NameError: name 'roc_curve' is not defined

In [264]: 
     ...: from sklearn.metrics import roc_curve, auc

In [265]: fpr, tpr, threshold  = roc_curve(y_true=y_np + y_p , y_score=np_scores+ p_scores)
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-265-50e64ae376d9> in <module>
----> 1 fpr, tpr, threshold  = roc_curve(y_true=y_np + y_p , y_score=np_scores+ p_scores)

NameError: name 'y_np' is not defined

In [266]: fpr, tpr, threshold  = roc_curve(y_true=qqp_score , y_score=smatch_scores)

In [267]: import matplotlib.pyplot as plt
     ...: plt.title('ROC using SMATCH score for MRPC', fontsize=20)
     ...: plt.plot(fpr, tpr, 'b', label = 'AUC = %0.2f' % roc_auc)
     ...: plt.legend(loc = 'lower right')
     ...: plt.plot([0, 1], [0, 1],'r--')
     ...: plt.xlim([0, 1])
     ...: plt.ylim([0, 1])
     ...: plt.ylabel('True Positive Rate', fontsize=20)
     ...: plt.xlabel('False Positive Rate', fontsize=20)
     ...: plt.show()
---------------------------------------------------------------------------
NameError                                 Traceback (most recent call last)
<ipython-input-267-2172672e69e7> in <module>
      1 import matplotlib.pyplot as plt
      2 plt.title('ROC using SMATCH score for MRPC', fontsize=20)
----> 3 plt.plot(fpr, tpr, 'b', label = 'AUC = %0.2f' % roc_auc)
      4 plt.legend(loc = 'lower right')
      5 plt.plot([0, 1], [0, 1],'r--')

NameError: name 'roc_auc' is not defined

In [268]: roc_auc = metrics.auc(fpr, tpr)

In [269]: import matplotlib.pyplot as plt
     ...: plt.title('ROC using SMATCH score for MRPC', fontsize=20)
     ...: plt.plot(fpr, tpr, 'b', label = 'AUC = %0.2f' % roc_auc)
     ...: plt.legend(loc = 'lower right')
     ...: plt.plot([0, 1], [0, 1],'r--')
     ...: plt.xlim([0, 1])
     ...: plt.ylim([0, 1])
     ...: plt.ylabel('True Positive Rate', fontsize=20)
     ...: plt.xlabel('False Positive Rate', fontsize=20)
     ...: plt.show()

In [270]: sns.boxplot(x="cat", y="smatch", data=p_df, order=cat)
Out[270]: <AxesSubplot:xlabel='cat', ylabel='smatch'>

In [271]: plt.xlabel("Sentence Pair Category", fontsize=16)
Out[271]: Text(0.5, 0, 'Sentence Pair Category')

In [272]: plt.ylabel("SMATCH Score", fontsize=16)
Out[272]: Text(0, 0.5, 'SMATCH Score')

In [273]: plt.title("SMATCH distribution for MRPC", fontsize=21)
Out[273]: Text(0.5, 1.0, 'SMATCH distribution for MRPC')

In [274]: plt.show()



==> amr2text.tex <==
\if 0 
\section{AMR-to-Text}

\begin{table}[h]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Model} & 
\textbf{BLEU} & \textbf{WMD} & \textbf{SIM} \\ \hline
Baseline & &  & \\
Wikipedia Augmentation & & &  \\
\hline
\end{tabular}}
\caption{Placeholder Table for performance of AMR-to-Text on Gold-AMR dataset
}
\end{table}



%\subsection{Wikipedia Augmentation}
%{\bf Preksha to add coverage table} 
%\begin{table}[t]
%\begin{tabular}{|l|l|l|l|l|} \hline 
%Model & BLEU & Sim & WMD & Propbank  \\ 
% & & Score & & Coverage \\ \hline 
%Gold-AMR      &   44.36   &           &     &                   \\
%Wikipedia-Filter      & 48.14      &           &     &      \\
%Wikipedia-Filter (1M) & 44.56  &           &     &     \\
%Wikipedia-Filter (10M) & 47.8 & & &   \\

%\hline
%\end{tabular}
%\end{table}

\subsection {Stylized Fine Tuning}
\subsubsection{One Decoder Per Style}
\subsubsection{ Tagged Decoder} 
\label{tab:amr2text-gold}
\fi

==> datasets.tex <==
 
 
\subsection{Datasets}\label{sec:datasets}
We evaluate performance of GIST on two English datasets that capture Linguistic Styles~\cite{styletransfer-survey}.
First, Shakespeare Author Imitation Dataset \cite{xu-etal-2012-paraphrasing} consists of $18$K pairs of sentences written in two styles. The original verses from Shakespeare's plays have been written in Early Modern English which is a significantly different style. 
Second, Corpus of Diverse Styles (CDS)~\cite{divpara}. This dataset consists of non-parallel sentences written in 11 different styles. We will present our results on a subset of four styles : Bible, Poetry, Shakespeare and Switchboard which consists of $34.8$K, $29.8$K, $27.5$K, $148.8$K instances respectively (CDS uses MIT License).



\if 0
\subsection{Automated Evaluation Metrics}

We evaluate GIST on content preservation and transferred style strength dimensions~\cite{mir-etal-2019-evaluating}. 

\subsubsection{Content Preservation} 
%As mentioned earlier, there are various metrics in the current literature being used for content preservation. To showcase the robustness of \textbf{GIST}, we measure it using the following metrics:
We use the following most commonly used metrics to measure {\bf Content Preservation}. 

 
    \noindent \textbf{1. Self-BLEU}: In most of the works, content preservation is evaluated by computing the BLEU score between generated output and the original sentence.
    
    \noindent \textbf{2. WMD} : Word Mover Distance measures the dissimilarity between two sentences, as the minimum distance among the embedded words of input from the generated output. \cite{metric-survey} shows that WMD has high correlation with human evaluations for content preservation.
    
    \noindent \textbf{3. SIM}: Similar to \cite{divpara}, we evaluate \textbf{GIST} against SIM metric. SIM \cite{sim} uses model proposed in \cite{} that is an embedding based model trained on ParaNMT corpus to measure semantic similarity that also performs well on Semantic Textual Similarity (STS) task in SemEval workshops.
    
    \noindent \textbf{4. SMATCH}: It captures the degree of overlap between two AMR graphs. Since, AMR graph for a given sentence primarily captures the semantics, we compare AMR graphs for (input, generated output) pair as a measure for content preservation.
    
 
%With the emerging works in style transfer, there are several different approaches through which content preservation is evaluated. To showcase the robustness of \textbf{GIST} with respect to content preservation, we measure it using four different metrics prevalant in literature. First, we use Self-BLEU as it is one of the most widely adopted metric, where the content similarity corresponds to $n$-gram overlap between input and generated output. Second, we use WMD score, as \cite{} states that it is the most promising metric that highly correlated with human evaluations w.r.t. semantic similarity. Third, we use SIM metric that was adopted in \cite{divpara}. Lastly, we also use SMATCH score to measure the groundedness of generated output to the input AMR representation. To this end, we first compute the AMR representation for the generated outputs and then compute it similarity to the input AMR representation. 

\noindent \textbf{\textit{Style Accuracy:}} Similar to \cite{divpara}, we fine-tune RoBERTa-Large \cite{} model for the four set of styles: Shakespeare, Bible, Romantic Poetry and Switchboard. Note that we achieve XX, XX, XX, XX classification accuracy on these styles respectively, which indicates that it is reliable classifier to measure transferred style strength.

\noindent \textit{\textbf{Weighted Style Accuracy}}: 
In additional to independently evaluating content preservation and style accuracy, it is crucial to jointly evaluate the sentences against these two aspects. From Table XX, we can infer that certain instances typically have high transferred style strength, however they have drastically changed the input meaning. Therefore, we also evaluate models again average weighted style accuracy, where the weights to the correctly styled outputs are their semantic similarity scores, and it is averaged across all test instances.
%Self-BLEU is one of the most widely used metric to measure how similar input and generated text. Second, cosine similarity between sentence embeddings for input and generated output, have also been adopted in many works. Third, with learnable metrics, certain models have adopted BERTScore, and  Broadly, content preservation between input and generated sentences is evaluated using i) $n$-gram metrics (such as BLEU, ROUGE), where a higher $n$-gram overlap indicates content similarity between input and output, ii)  
\fi 




%As mentioned earlier, our work is restricted to semantic preserving style. Therefore, we compare our model to the baseline models on the following two semantic-preserving style datasets. 
%\begin{itemize}
%\item \textbf{Shakespeare Author Imitation Dataset \cite{xu-etal-2012-paraphrasing}} consists of $18K$ pairs of sentences written in two styles. The original verses from Shakespeare's plays have been written in Early Modern English which is a significantly different style. Therefore although the semantic meaning is preserved in a given pair of sentences, they have very different syntactic distributions.

%\item \textbf{Corpus of Diverse Styles \cite{divpara}} This dataset consists of non-parallel sentences written in 11 different styles. The authors crawled this dataset from several resources and the styles have been selected which are distinguishable by human readers at a sentence level. We will present our results on a subset of four styles : Bible, Poetry, Shakespeare and Lyrics, which consists of XX, XX, XX, XX instances respectively. Note that across these 4 styles, style transfer can have 12 different directions. We present results for XX of these 12 transfer pairs.   

%\end{itemize}

==> eval_metrics.tex <==

\section{Evaluation Metrics}

There are two necessary components to evaluate a successful style transfer - content preservation, and style accuracy. 

\subsection{Content Preservation}

\paragraph{Text-Text Similarity} 
We use three metrics to measure content preservation between the source sentence ($S$) and the generated target sentence ($T$) - 
\begin{itemize}
    \item \textbf{Self-BLEU:} We use BLEU-4 \cite{bleu} to measure n-gram overlap between $S$ and $T$. Self-BLEU is a weak indicator of content preservation (potentially point to a correlation table here).
    \item \textbf{Word Mover Distance (WMD):} WMD \cite{wmd} measures dissimilarity between $S$ and $T$ as the minimum distance between their embedded words. 
    \item \textbf{SIM similarity:} SIM \cite{sim} uses an embedding model proposed in \cite{wieting-etal-2019-simple} to measure semantic similarity.
\end{itemize}


\paragraph {Text-AMR Similarity}
Although there exist a few metrics to measure the syntactic and semantic similarities between two sentences, there does not exist a metric to evaluate content overlap between an AMR graph and a sentence. Hence we propose to use a slight variation of the Word Mover Distance \cite{wmd} for this purpose. We choose WMD over other content preservation metrics for the following reasons - 
\begin{itemize}
    \item XX illustrate the efficacy of WMD to evaluate text style transfer over other metrics.
    \item Syntactic metrics like BLEU would not be able to compute the content overlap between an AMR graph and a sentence because word representation in an AMR graph discards noun forms and tense information, and some verb tokens are mapped to a different PropBank verb. These modifications along with the disparity in sequential-graphical representation makes syntactic metrics infeasible for the task.
    \item Semantic representations like SIM are fragile to the input sequence order, and affected by non-content bearing words as well. However, WMD adopts on a bag-of-words paradigm, making it more suitable for the task.
\end{itemize}

RUN A HUMAN EVAL ON THIS!


\subsection{Style Transfer}
To evaluate style transfer, we follow \cite{divpara}, and train a 4-way RoBERTa-based \cite{roberta} classifier for the CDS dataset, and a 2-way classifier for the Shakespeare Imitation Dataset. We also report the style retention scores along with style accuracy scores in Table \ref{}.

\input{wmd_metric}


  
 %In Section~\ref{sec:tst_experiments}, we  study the performance of GIST across various performance metrics (described in Table~\ref{tab:metrics}) on datasets described in  Section~\ref{sec:datasets}. 

%In this section, we present our findings to answer the following questions: \textit{Is AMR well-suited as a style-agnostic intermediate representation that correctly encodes the content information ?} and \textit{If using AMRs as intermediate representation leads to high content-preserving style transfer ?}
\input{datasets}

==> failure_cases.tex <==


\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Model & Sentence                                                           \\\hline
Input & Oh, poor Romeo! (SAID Modern $\rightarrow$ Original)               \\
UNMT  & Alas , poor country !                                              \\
DLSM  & Alas , poor Glou-cester !                                          \\
STRAP & O, poor Rosalind                                                   \\\hline
Input & Wash they his wounds with tears? (CDS Shakes. $\rightarrow$ Bible) \\
STRAP & Is he weeping for tears?                                          \\\hline
%Input & oh i agree it’s good (CDS Switch. $\rightarrow$ Bible)             \\
%STRAP & And he said, Surely this thing is good for thee.                   \\\hline
Input & Nay, good goose, bite not. (CDS Shakes. $\rightarrow$ Switch.)     \\
STRAP & oh good kid don’t bite        \\\hline                                    
\end{tabular}
}
\caption{Some poorly generated style transfer instances using UNMT \cite{multiple-attribute}, DLSM \cite{DLSM}, and STRAP \cite{divpara} on the CDS dataset \cite{divpara} and Shakespeare Author Imitation dataset (SAID).}
\end{table}
 

==> introduction.tex <==
\section{Introduction}

\begin{table}[]
    \centering
    \resizebox{0.8\columnwidth}{!}{%
    \begin{tabular}{|p{1.2cm}|p{5cm}|}
        \hline
        \textbf{Model} & \\
        \hline \hline
       & \textit{Direction:} Switchboard to Shakespeare  \\
        \textbf{STRAP}  &  \textit{Input}: well they offer classes out at uh Ray Hubbard \\
        & \textit{Output}: They do offer a course at the \textcolor{red}{house of the Dukedom}. \\
        \hline\hline
        
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{figure*}
    \centering
    \subfloat[Shakespeare: \textit{"The law, that threat'ned death, becomes thy friend And turns it to exile"} ]{\includegraphics[width=0.47\textwidth]{Figures/Shakespeare.png}}
    \qquad
    \subfloat[Bible: \textit{"The law of death threats becometh thy friend, and turneth itself into exile unto thee."}
    ]{\includegraphics[width=0.47\textwidth]{Figures/Bible.png}}
    \caption{AMR representations for an input text written in two different styles: Shakespeare and Bible style. Despite different styles, we can infer that majority of the two graphs is very similar to each other, as they represent the same content. Quantitatively, SMATCH Score : $86.7$ is  also very high.}
    \label{fig:example}
\end{figure*}

Style Transfer is the task of rephrasing an input sentence to contain specific stylistic properties without altering the meaning of the sentence.   With the emergence of deep learning based models, various neural style transfer approaches \cite{neuralcontrolledtext, multiple-attribute,plugandplaycontrolledtext,samanta-etal-2021-hierarchical} have been proposed. As a consequence, most of these works adopt a data-driven definition of style \cite{styletransfer-survey}, which majorly subsumes content-related styles (sentiment, gender, topic) along with few linguistic-related styles (formality, author-style, etc.). Transforming the first of styles (attribute transfer), therefore implicitly implies to alter the semantics of the given input, whereas this is not the case for the second set of styles, also known as semantic-preserving styles. 
    
It is important to note that for many downstream applications for style transfer ( persona-based dialog generation \cite{polite-dialoggeneration}, online text biasing \cite{online-text-debiasing}, stylistic machine translation \cite{stylistic-mt}, author imitation in language models \cite{author-stylized}, attractive headline generation \cite{attractive-headline-generation}) the primary focus is on semantic-preserving styles where high content preservation is expected to be a non-negotiable aspect. 

In the current literature, there are two schools of thought to deal with content preservation. First, to explicitly disentangle style information from content in latent space and only toggle the style representation to generate the target \citep{neuralcontrolledtext,john-etal-2019-disentangled, adversarial-st, disentangling-crossalignment}. However, the second set of works \cite{multiple-attribute, samanta-etal-2021-hierarchical} state that as content and style are subtly entangled in text, it is difficult to disentangle both of them in non-linear space, and thus these works use other techniques such as back-translation loss \cite{multiple-attribute, content-preserving}, reinforcement learning \cite{reinforce-st}, paraphrase generation \cite{divpara} for content preservation.

However, there are still several open challenges w.r.t. content preservation. \textbf{First,} as we move toward more difficult styles where style and content are tightly coupled, we can infer from Table 1 that the models still lack in content preservation. \textbf{Second}, due to less transperency of deep learning based models, we do not have a good mechanism to understand why content preservation is low. Is it because: (i) infusing the target style in the learnt latent representation, some content information is changed, or (ii) style-specific language model lacks in projecting this information in generated output. \textbf{Third}, the current literature lacks an ideal metric to evaluate the model on content preservation, which we believe is also an outcome of style and content being tightly coupled.  

In this work, we propose \textbf{GIST:} Grounded and Interpretable Style Transfer System to address some of the above challenges. We propose that utilizing traditional symbolic representations (e.g., AMR) as intermediate representations has the potential of naturally disintegrate content and style. Moreover, it is an intuitive choice when we aim for content preservation \cite{amr-nmt}. Second, it makes \textbf{GIST} an interpretable pipeline. It allows to understand if the content is misrepresented in the intermediate representation or if the style-specific language model does not encode it well in the generated output. 

Specifically \textbf{GIST} performs style transfer in two stages, we first automatically generate semantic representation (Abstract Meaning Representation, AMR) for the given input, which is then passed to a style-specific decoder to transform the given semantics in the targeted style. We hypothesize that the AMR representation of the input contains very little style information as the syntactic information is typically not retained in the AMR graphs. We can see from Figure 1, that the AMR graphs for the similar content written in two different styles is very similar. Moreover, they have the SMATCH \footnote{SMATCH measures similarity between two AMR graphs} score (used to capture the similarity of two graphs) is also high.


%In parallel to ST works, content preservation is an important aspect in Machine Translation as well. Recently, \cite{amr-nmt} states that using semantic representations as an intermediate representation is an intuitive choice to target for content preservation. Moreover, using such traditional semantic representations act as interpretable intermediate representations.
%Taking the above as a motivation, we propose \textbf{GIST}: Grounded and Interpretable Style Transfer system, which utilizes interpretable semantic representations as intermediate representation to explicitly capture \textit{only} the content information of the given input. Specifically, we use Abstract Meaning Representation (AMR) as an intermediate representation. We hypothesize that the AMR representation of the input contains very little style information as the syntactic information is typically not retained in the AMR graphs. We can see from Figure 1, that the AMR graphs for the similar content written in two different styles is very similar. Moreover, they have the SMATCH score (used to capture the similarity of two graphs) is also high. \textbf{GIST} first automatically constructs such representation for given input text and then decodes it to the targeted style using a style specific decoder that takes AMR graph as an input. 

%In this work, we take a different approach to represent content which is disentangled from the style. We utilize the Abstract Meaning Representations (AMR) graphs to first retreive the content from the input sentence. We hypothesize that the AMR representation of the input contains very little style information as the syntactic information is typically not retained in the AMR graphs. We can see from Figure 1, that the AMR graphs for the similar content written in two different styles is very similar. Moreover, they have the SMATCH score (used to capture the similarity of two graphs) is also high. 

Our primary contributions are as follows: i) we first empirically validate that interpretable semantic representations such as AMR, indeed leads to higher content preservation and less style information of the given input sentence, ii) we empirically show that \textbf{GIST} performs better than the baselines on Shakespeare Author Imitation Dataset, and iii) we quantitatively and qualitatively show that our model is able to perform significantly better on content preservation as compared to the baseline on CDS dataset. Also, it gives similar performance on style accuracy. Therefore, \textbf{GIST} is able to generate better stylized outputs with high content preservation scores. 

\if 0
\begin{itemize}
    \item Style Transfer background: two important aspects content preservation, and style transfer : \textbf{semantically-preserving style and attribute transfer style (distinction)} We deal with semantic-preserving style 
    


   Previous works deal 
   In previous works, content preservation has been dealt using various techniques: i) disentangling content and style information in latent space \cite{neuralcontrolledtext}, iii) interpolating the intermediate representation in new style direction, iv) generating an intermediate destylized version.
   
   In previous works, content preservation has been primarily dealt by explicitly disentangling style and content information in the input through attribute supervision \cite{}, adversarial training \cite{},  
    %have been proposed for style transfer tasks as well. In recent years, there has been an increase in enhancing automated systems for style transfer tasks. However, most of the previous works  \cite{neuralcontrolledtext, multiple-attribute,plugandplaycontrolledtext,samanta-etal-2021-hierarchical} encompass attribute transfers in style transfer tasks. Typically, attribute transfer refers to changing certain linguistic attribute of a sentence, such as topic and sentiment. It is evident that transforming such attributes implicitly implies to alter the meaning and thus content/semantics of the sentence. On the other hand, semantic-preserving styles refers to transforming attributes which do not alter meaning of the input, such as formality and author-style. In this work, we primarily focus on semantic-preserving style transfer to better study content preservation in this task. 
    
    \item Not much works showing content preservation in semantic-preserving styles, or evaluating it. Some applications to semantic-preserving styles.. 
    
    
    
    \item How content preservation has been dealt in some previous works: two school of thoughts: disentangling and keeping the content and style information infused. Disentangling only at latent representation.. why interpretable representation is needed ? (Still lacks content preservation : some examples in table 1 ): attribute transfer  Why it is a hard to solve. 
    
    \item Style transfer with measureable CP with interpretable semantic representations. 
    
    \item We therefore, incorporate traditional semantic representations such as Abstract Meaning Representation(AMR) to efficiently disintegrate content from style information . (One example to showcase the same) (Advantages : using interepretable representations as intermediate reps)  
    \item Main Contributions: Representing input sentences using traditional semantic reps helps in explictly only passing the meaning before the style transfer. Model beats the baseline. Not restricted to only one type of semantic representations 

\end{itemize}


Style Transfer refers to transforming a given piece of text in a different writing style while preserving the content. Due to lack of parallel corpora, style transfer is typically modeled using unsupervised approaches. Earlier works focused on disentangling the style information from the content present in the input text. More recent works have identified that disentangling the two often leads to sub-optimal style transfer. However, such works typically use reconstruction loss as a way to enforce content preservation. 

\cite{} utilized paraphrase network to de-stylize the input before transforming it to a different style. However, one of the caveats of this approach is shown in Table XX. We can infer that the meaning has not been restored in the paraphrase version as well.Moreover, based on the other content preservation approaches, we observe that there is still some content loss while transforming the style. 



\fi


\subsection{Motivation} 
Prior work all acknowledge that content preservation is paramount for all style transfer tasks. In order to achieve this most approaches rely on crafting a loss function (Back Translation loss, ... ) and designing a style netural intermediate representation. 



1. Need  style-neutral intermediate  representation 
2. Interpretability of error  


The manner in which a given sentence is represented is often tied to word choices, syntactic structures, metaphors and so on \cite{styletransfer-survey}. On the other hand, content refers to the meaning/semantics of the sentence. AMR representations \cite{banarescu-etal-2013-abstract} are designed to represent the semantic aspect of a given sentence while abstracting away the syntactic variations. To elaborate, two sentences with similar meaning but different syntactic structure will tend to have similar AMR representations. Therefore, AMR serves as an obvious intermediate representation to only encode the content (semantics) while removing the style specific aspect (syntactic structure). 

==> iterative.tex <==
\section{Iterative T-STAR}

==> model_arch.tex <==
\section{Model Architecture}\label{sec:model_arch}
We train standard Transformer encoder-decoder
models as described in Vaswani et al. (2017). The
dimension of transformer layers, token embeddings
and positional embeddings is 1024, the feedforward
layer dimension is 8192, and number of attention
heads is 16. We use 6 layers in both encoder and
decoder for the   models and 4 layers for the
  For training, we use the
Adafactor optimizer with 
and the learning rate is varied with warmup for
40,000 steps followed by decay as in Vaswani et al.
(2017). We perform all experiments on TPUs, and
train models for 300k steps. We use a batch size
of 3k across all models and tokenize the source

and target using WordPiece tokenization (Schus-
ter and Nakajima, 2012; Wu et al., 2016). Further

details on hyper-parameter selection and experi-
mental setup can be found in Appendix B.

==> strap_comparision.tex <==
\section{Qualitative Analysis of STRAP}\label{sec:strap_comparision} 
We list several instances to study the nature of transformations done by STRAP vs GIST in Table \ref{tab:case-study-appendix}. We broadly observe three specific issues in targets generated by STRAP model: i) \textit{Hallucinations}: where new information irrelevant to the source sentence is added, ii) \textit{Semantic Drift: }the target sentence indicates that the source content was misinterpreted, iii) \textit{Incomplete:} some important content information is missed in the target. We can see that across these examples, \textbf{GIST} avoids adding new information, does not misinterpret the source content and often preserves the whole content as compared to STRAP. 
\input{case-stydy-appendix}
\\

We also list some instances in Table \ref{tab:limitations-appendix} where our model is not able to perform efficient style transfer as compared to the STRAP model. We can observe that our model sometimes does very minimal changes in the source input structure to transfer the style (example 2,4,5) in order to preserve the content. We believe that such subtle changes is also one of the reasons to attain lower style accuracy numbers. As a future work, we would like to provide explicit control on amount of variation to attain better style transfer. 

==> styleaccuracy.tex <==
\begin{table}[t]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Style} & 
\textbf{Original} & \textbf{Paraphrase} & \textbf{AMR} \\ \hline
Bible    &          98.66   &                 97.43  &     76.25         \\ \hline
Switchboard    &     99.93        &    99.66                & 98.39            \\ \hline
Poetry    &    98.16          &     95.08                &    79.71          \\ \hline
Shakespeare    &   94.29           &  77.08                  &   46.84          \\ \hline
\end{tabular}}
\caption{Accuracy of style classifiers trained on original, paraphrase and AMR inputs. AMR has least performance denoting it encodes least style information.  
%Analysis of style information retention in different forms of inputs for various styles. AMR has the least style retention as compared to other input forms.
}
\label{tab:styleaccuracy}
\end{table}

